Influence of Stellar Multiplicity On Planet Formation. II. Planets Are Less Common in Multiple-Star Systems with Separations Smaller than 1500 AU

Almost half of the stellar systems in the solar neighborhood are made up of multiple stars. In multiple-star systems, planet formation is under the dynamical influence of stellar companions, and the planet occurrence rate is expected to be different from that for single stars. There have been numerous studies on the planet occurrence rate of single star systems. However, to fully understand planet formation, the planet occurrence rate in multiple-star systems needs to be addressed. In this work, we {{infer}} the planet occurrence rate in multiple-star systems by measuring the stellar multiplicity rate for planet host stars. For a sub-sample of 56 $Kepler$ planet host stars, we use adaptive optics (AO) imaging and the radial velocity (RV) technique to search for stellar companions. The combination of these two techniques results in high search completeness for stellar companions. We detect 59 visual stellar companions to 25 planet host stars with AO data. {{Three stellar companions are within 2$^{\prime\prime}$, and 27 within 6$^{\prime\prime}$. We also detect 2 possible stellar companions (KOI 5 and KOI 69) showing long-term RV acceleration.}} After correcting for a bias against planet detection in multiple-star systems due to flux contamination, we find that planet formation is suppressed in multiple-star systems with separations smaller than 1500 AU. Specifically, we find that compared to single star systems, planets in multiple-star systems occur $4.5\pm3.2$, $2.6\pm1.0$, and $1.7\pm0.5$ times less frequently when a stellar companion is present at a distance of 10, 100, and 1000 AU, respectively. This conclusion applies only to circumstellar planets; the planet occurrence rate for circumbinary planets requires further investigation.

==> AO_params.tex <==


\clearpage
%\LongTables

\begin{deluxetable}{lcccccc}
%\tabletypesize{\tiny}
\tablewidth{0pt}
%\tablenum{1}
\tablecaption{Visual companion detections with AO data.\label{tab:AO_params}}
\tablehead{
\colhead{\textbf{KOI}} &
\colhead{\textbf{$\Delta$ Mag}} &
%\colhead{\textbf{Separation}} &
\multicolumn{2}{c}{\textbf{Separation}} &
%\colhead{\textbf{Separation}} &
\colhead{\textbf{Distance}} &
\colhead{\textbf{Significance}} &
\colhead{\textbf{PA}} \\
\colhead{\textbf{}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(arcsec)}} &
\colhead{\textbf{(AU)}} &
\colhead{\textbf{(pc)}} &
\colhead{\textbf{($\sigma$)}} &
\colhead{\textbf{(deg)}} \\

}

\startdata

%from /home/jwang/2014/03/JW_2013_plot/ContrastCurve
   K00005 &   2.3 (Br-$\gamma$)&      0.14&      40.9&$  290.9^{+   63.2}_{  -19.4}$&      28.2&            308.9 \\
  K00010 &           6.8 ($J$)&      3.88&    3663.9&$  944.5^{+  100.1}_{ -139.1}$&      22.0&             89.3 \\
  K00017 &           3.9 ($J$)&      4.11&    2130.7&$  517.9^{+   27.6}_{  -28.4}$&     206.2&             39.5 \\
  K00018 &           3.9 ($J$)&      7.26&    8241.0&$ 1135.9^{+   84.4}_{ -154.0}$&     323.2&            148.2 \\
  K00018 &           6.3 ($J$)&      9.68&   10995.5&$ 1135.9^{+   84.4}_{ -154.0}$&      32.1&            344.7 \\
  K00018 &           6.6 ($J$)&      3.50&    3971.8&$ 1135.9^{+   84.4}_{ -154.0}$&      28.5&            110.1 \\
  K00018 &           7.3 ($J$)&      5.09&    5783.0&$ 1135.9^{+   84.4}_{ -154.0}$&      14.1&            211.3 \\
  K00018 &           7.7 ($J$)&      5.89&    6693.3&$ 1135.9^{+   84.4}_{ -154.0}$&       9.8&            106.3 \\
  K00018 &           7.7 ($J$)&     10.82&   12293.3&$ 1135.9^{+   84.4}_{ -154.0}$&       7.7&            222.1 \\
  K00018 &           7.3 ($J$)&      7.26&    8241.0&$ 1135.9^{+   84.4}_{ -154.0}$&       7.3&              77.6\\
  K00018 &           8.0 ($J$)&      9.69&   11004.0&$ 1135.9^{+   84.4}_{ -154.0}$&       6.6&            339.2 \\
  K00018 &           8.2 ($J$)&      7.09&    8059.2&$ 1135.9^{+   84.4}_{ -154.0}$&       6.5&            219.2 \\
  K00070 &           4.3 ($J$)&      3.79&    1058.9&$  279.5^{+   25.3}_{  -23.6}$&     217.7&             51.8 \\
  K00087 & 6.2 ($J$), 6.1 ($K$)&      5.49&     956.9&$  174.4^{+   15.2}_{  -12.1}$&      78.2&            177.2 \\
  K00087 & 7.4 ($J$), 6.6 ($K$)&      5.53&     964.1&$  174.4^{+   15.2}_{  -12.1}$&      28.4&             75.2 \\
  K00103 &           7.3 ($J$)&      9.81&    2985.6&$  304.4^{+   29.0}_{  -27.0}$&       9.5&            278.5 \\
  K00108 &           5.5 ($J$)&      9.52&    3357.4&$  352.7^{+   36.0}_{  -22.0}$&      98.8&            348.6 \\
  K00108 &           7.2 ($J$)&      5.00&    1764.4&$  352.7^{+   36.0}_{  -22.0}$&      21.5&            112.5 \\
  K00108 &           7.2 ($J$)&      2.51&     887.0&$  352.7^{+   36.0}_{  -22.0}$&      19.9&             74.8 \\
  K00108 &           7.4 ($J$)&      3.23&    1139.2&$  352.7^{+   36.0}_{  -22.0}$&      18.2&            100.9 \\
  K00108 &           7.4 ($J$)&      8.90&    3139.4&$  352.7^{+   36.0}_{  -22.0}$&      17.1&             19.2 \\
  K00111 &           7.5 ($J$)&      7.13&    2052.6&$  297.8^{+   26.0}_{  -29.1}$&      10.8&            117.7 \\
  K00111 &           7.8 ($J$)&      9.07&    2702.5&$  297.8^{+   26.0}_{  -29.1}$&       7.7&            175.5 \\
  K00111 &           8.2 ($J$)&      6.70&    1995.1&$  297.8^{+   26.0}_{  -29.1}$&       8.2&             96.0 \\
  K00116 &           3.8 ($K$)&      8.00&    2907.0&$  363.2^{+   56.7}_{  -40.3}$&     164.1&            353.5 \\
  K00116 &           4.8 ($K$)&     12.96&    4707.6&$  363.2^{+   56.7}_{  -40.3}$&      51.9&            144.3 \\
  K00116 &           6.2 ($K$)&      7.46&    2710.6&$  363.2^{+   56.7}_{  -40.3}$&      18.1&            107.1 \\
  K00116 &           6.3 ($K$)&     13.51&    4907.8&$  363.2^{+   56.7}_{  -40.3}$&      13.2&            113.8 \\
  K00116 &           6.3 ($K$)&     13.05&    4740.8&$  363.2^{+   56.7}_{  -40.3}$&      12.7&            357.4 \\
  K00116 &           7.5 ($K$)&     10.93&    3969.3&$  363.2^{+   56.7}_{  -40.3}$&       7.5&              19.7\\
  K00116 &           7.3 ($K$)&      5.79&    2101.4&$  363.2^{+   56.7}_{  -40.3}$&       6.3&            141.1 \\
  K00122 &           6.7 ($J$)&      4.23&    1446.2&$  341.7^{+   28.1}_{  -30.3}$&      30.0&            211.3 \\
  K00123 &           5.2 ($J$)&      9.52&    4749.5&$  498.7^{+   25.0}_{  -99.9}$&      62.3&            198.8 \\
  K00123 &           6.4 ($J$)&     10.19&    5083.7&$  498.7^{+   25.0}_{  -99.9}$&      19.2&             95.2 \\
  K00137 &           5.9 ($J$)&      5.64&    2471.4&$  438.2^{+   37.6}_{  -41.0}$&      44.4&            350.7 \\
  K00137 &           7.8 ($J$)&      7.13&    3122.2&$  438.2^{+   37.6}_{  -41.0}$&       7.6&            185.5 \\
  K00137 &           7.9 ($J$)&      5.11&    2240.3&$  438.2^{+   37.6}_{  -41.0}$&       6.6&            136.2 \\
  K00148 &           3.5 ($J$)&      4.44&    1369.1&$  308.7^{+   27.0}_{  -17.2}$&     519.8&            220.6 \\
  K00148 &           5.4 ($J$)&     10.99&    3391.9&$  308.7^{+   27.0}_{  -17.2}$&      77.0&            230.1 \\
  K00148 &           5.5 ($J$)&      2.54&     785.2&$  308.7^{+   27.0}_{  -17.2}$&      69.7&            245.8 \\
  K00148 &           6.3 ($J$)&      8.05&    2486.4&$  308.7^{+   27.0}_{  -17.2}$&      35.5&              244 \\
  K00148 &           7.4 ($J$)&      6.06&    1870.7&$  308.7^{+   27.0}_{  -17.2}$&      13.9&            238.8 \\
  K00153 &           6.0 ($K$)&      8.01&    1812.0&$  226.2^{+   18.6}_{  -15.1}$&      11.2&            353.4 \\
  K00153 & 6.9 ($J$), 7.6 ($K$)&      6.17&    1395.3&$  226.2^{+   18.6}_{  -15.1}$&       4.5&            298.4 \\
  K00244 & 2.7 ($J$), 2.0 ($K$)&      8.40&    2741.0&$  326.3^{+   23.4}_{  -44.6}$&    3231.4&            287.6 \\
  K00244 & 7.6 ($J$), 7.0 ($K$)&      8.38&    2733.6&$  326.3^{+   23.4}_{  -44.6}$&      27.5&            101.4 \\
  K00263 & 1.0 ($J$), 1.0 ($K$)&      3.28&     788.5&$  240.7^{+   17.7}_{  -38.9}$&    2430.8&            268.2 \\
  K00273 & 6.2 ($J$), 5.6 ($K$)&      5.02&    1201.8&$  239.6^{+   14.7}_{  -15.2}$&      32.6&            344.0 \\
  K00283 &           7.9 ($K$)&      6.09&    1266.2&$  208.0^{+   21.4}_{  -11.2}$&       7.0&           271.4  \\
  K00289 &           8.6 ($J$)&      5.86&    2201.2&$  375.9^{+  355.0}_{  -69.8}$&       5.1&             88.3 \\
  K00289 &           7.7 ($J$)&      3.18&    1195.0&$  375.9^{+  355.0}_{  -69.8}$&       6.1&            308.6 \\
  K00292 &           4.2 ($K$)&      0.43&     154.9&$  358.5^{+   40.9}_{  -28.3}$&      43.2&            119.4 \\
  K00365 & 7.7 ($J$), 6.6 ($K$)&      7.12&    1129.9&$  158.8^{+   15.1}_{  -19.7}$&      13.3&            313.7 \\
  K00377 & 5.0 ($J$), 4.8 ($K$) &      6.02&    3721.9&$  617.9^{+   48.5}_{  -46.7}$&     133.8&             91.9 \\
  K00377 & 6.0 ($J$), 6.9 ($K$)&      8.04&    4969.8&$  617.9^{+   48.5}_{  -46.7}$&      18.1&            221.9 \\
  K00377 & 6.2 ($J$), 7.3 ($K$)&      2.88&    1780.8&$  617.9^{+   48.5}_{  -46.7}$&      12.3&             37.5 \\
  K00975 & 3.8 ($J$), 4.0 ($K$)&      0.73&      90.4&$  123.7^{+    7.7}_{  -17.9}$&      31.2&            133.4 \\
  K01442 &           4.7 ($J$)&      2.11&     637.4&$  302.3^{+   18.0}_{  -20.3}$&      25.3&             76.3 \\
  K01442 &           8.0 ($J$)&      5.69&    1718.6&$  302.3^{+   18.0}_{  -20.3}$&       5.8&             90.2 \\


\enddata




\end{deluxetable}

\clearpage




==> Bias_params.tex <==


\clearpage
%\LongTables

\begin{deluxetable}{lcccccccc}
%\tabletypesize{\tiny}
\tablewidth{0pt}
%\tablenum{1}
\tablecaption{Detection Bias of Planets in Multiple Stars.\label{tab:Bias_params}}
\tablehead{
\colhead{\textbf{KOI}} &
\colhead{\textbf{Period}} &
\colhead{\textbf{${\rm{R}}_P$}} &
\colhead{\textbf{${\rm{R}}_\ast$}} &
\colhead{\textbf{${\rm{M}}_\ast$}} &
\colhead{\textbf{Duration}} &
\colhead{\textbf{CDPP$_{\rm{eff}}^{\ast}$}} &
\colhead{\textbf{Quarters}} &
\colhead{\textbf{$\alpha^{\ast\ast}$}} \\
\colhead{\textbf{}} &
\colhead{\textbf{(day)}} &
\colhead{\textbf{(${\rm{R}}_\oplus$)}} &
\colhead{\textbf{(${\rm{R}}_\odot$)}} &
\colhead{\textbf{(${\rm{M}}_\odot$)}} &
\colhead{\textbf{(hr)}} &
\colhead{\textbf{(ppm)}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} \\

}

\startdata

 K00005&	4.78033&   5.66&   1.42&   1.15&   2.01&      36.3&    17&  0.930\\
 K00007&	3.21366&   3.72&   1.27&   1.12&   4.11&      53.1&    14&  0.850\\
 K00010&	3.52250&  15.90&   1.56&   1.14&   3.20&     136.0&    17&  0.961\\
 K00017&	3.23470&  11.07&   1.08&   1.14&   3.60&     103.5&    14&  0.946\\
 K00018&	3.54847&  17.40&   2.02&   1.45&   4.08&     102.7&    17&  0.619\\
 K00020&	4.43796&  17.60&   1.38&   1.17&   4.67&     106.1&    14&  0.961\\
 K00022&	7.89145&  11.27&   1.11&   1.16&   3.79&      82.4&    17&  0.938\\
 K00041&       12.81570&   2.08&   1.23&   1.11&   6.54&      26.6&    17&  0.635\\
 K00069&	4.72675&   1.50&   0.87&   0.89&   2.93&      17.9&    17&  0.938\\
 K00070&       10.85410&   3.17&   0.94&   0.90&   3.82&      57.1&    17&  0.930\\
 K00072&	0.83749&   1.37&   1.00&   0.91&   1.80&      29.6&    14&  0.938\\
 K00082&       16.14570&   2.54&   0.74&   0.80&   3.75&      39.4&    17&  0.946\\
 K00084&	9.28701&   2.53&   0.86&   0.91&   3.54&      34.3&    17&  0.938\\
 K00085&	5.85993&   2.36&   1.20&   1.21&   4.11&      29.0&    17&  0.624\\
 K00087&      289.86200&   2.10&   0.85&   0.83&   7.40&      23.4&    17&  0.773\\
 K00103&       14.91080&   2.95&   0.95&   0.91&   3.31&      73.7&    17&  0.906\\
 K00104&	2.50806&   3.36&   0.76&   0.81&   1.14&      84.9&    17&  0.961\\
 K00108&       15.96530&   2.94&   1.21&   1.16&   4.65&      32.2&    17&  0.629\\
 K00111&       11.42750&   2.14&   0.93&   0.81&   4.59&      47.5&    17&  0.930\\
 K00116&       13.57070&   2.47&   1.04&   1.00&   3.25&      59.2&    17&  0.803\\
 K00122&       11.52310&   2.78&   1.09&   1.07&   4.06&      45.2&    17&  0.773\\
 K00123&	6.48167&   2.64&   1.43&   1.06&   3.63&      40.9&    17&  0.874\\
 K00137&       14.85890&   6.01&   0.98&   0.94&   3.63&      83.8&    17&  0.954\\
 K00148&	9.67393&   3.15&   0.89&   0.88&   4.40&      72.8&    17&  0.930\\
 K00153&	8.92511&   2.47&   0.69&   0.74&   2.77&      91.0&    17&  0.938\\
 K00157&       31.99550&   4.18&   1.06&   0.98&   4.27&      77.1&    17&  0.906\\
 K00180&       10.04560&   2.53&   0.92&   0.99&   3.26&      62.0&    17&  0.866\\
 K00244&       12.72040&   6.51&   1.66&   1.19&   2.83&      28.4&    17&  0.898\\
 K00245&       39.79220&   1.94&   0.73&   0.75&   4.57&      17.3&    17&  0.946\\
 K00246&	5.39877&   2.53&   1.24&   1.07&   3.56&      22.0&    17&  0.922\\
 K00261&       16.23850&   2.65&   1.02&   0.99&   3.86&      36.0&    17&  0.914\\
 K00263&       20.71940&   2.02&   1.41&   1.01&   4.23&      49.2&    17&  0.658\\
 K00265&	3.56806&   1.29&   1.18&   1.16&   3.43&      36.1&    17&  0.528\\
 K00273&       10.57380&   1.82&   1.07&   1.12&   1.74&      30.4&    17&  0.624\\
 K00274&       15.09200&   1.13&   1.55&   1.20&   4.14&      28.0&    17&  0.500\\
 K00283&       16.09190&   2.41&   1.03&   1.02&   2.93&      31.4&    17&  0.874\\
 K00289&      296.63700&   5.04&   0.95&   0.94&  16.43&      28.3&    17&  0.930\\
 K00292&	2.58663&   1.64&   0.98&   0.94&   2.37&      53.9&    14&  0.874\\
 K00299&	1.54168&   1.98&   1.11&   0.99&   1.94&      84.7&    17&  0.890\\
 K00305&	4.60356&   1.57&   0.73&   0.79&   2.40&      74.9&    17&  0.898\\
 K00321&	2.42631&   1.50&   1.11&   0.99&   2.65&      50.7&    17&  0.850\\
 K00364&      173.92800&   0.93&   1.35&   1.15&   2.64&      23.0&    17&  0.500\\
 K00365&       81.73750&   2.29&   0.87&   0.85&   6.78&      23.7&    17&  0.906\\
 K00377&       19.27390&   8.28&   1.01&   1.05&   4.16&     129.3&    17&  0.930\\
 K00701&       18.16410&   1.91&   0.60&   0.65&   2.96&      83.3&    17&  0.922\\
 K00975&	2.78582&   1.72&   2.04&   1.36&   3.41&      24.1&    17&  0.500\\
 K01431&      345.16100&   8.45&   1.00&   1.06&   7.50&      45.8&    14&  0.890\\
 K01439&      394.61100&   7.80&   1.65&   1.23&  24.61&      15.3&    17&  0.635\\
 K01442&	0.66934&   1.23&   0.99&   1.01&   1.29&      54.7&    14&  0.795\\
 K01463&      580.00000&  16.29&   1.09&   1.05&  11.43&      38.6&    17&  0.961\\
 K01612&	2.46503&   0.78&   1.31&   1.05&   1.19&      16.7&    14&  0.629\\
 K01781&	7.83445&   3.76&   0.76&   0.82&   3.00&      80.5&    14&  0.946\\
 K01925&       68.95800&   1.12&   0.95&   0.88&   2.99&      15.4&    17&  0.658\\
 K02169&	5.45300&   0.97&   0.93&   0.82&   2.24&      43.2&    17&  0.723\\
 K02687&	1.71683&   1.90&   1.94&   1.12&   2.11&      24.2&    17&  0.818\\
 K02720&	6.57148&   0.80&   1.05&   1.05&   3.07&      22.6&    17&  0.619\\



\enddata

\tablecomments{$\ast$: effective combined differential photometric precision~\citep{Jenkins2010b}. $\ast\ast$: correction factor for the bias against planet detection in binary stars. The factor ranges from 0 to 1, with 1 indicating 100\% detection rate even with the flux contamination from a companion star. See \S \ref{sec:bias} for more details. }


\end{deluxetable}

\clearpage




==> orbital_params.tex <==


\clearpage
%\LongTables

\begin{landscape}
\begin{deluxetable}{lccccccccccccccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\setlength{\tabcolsep}{0.02in}
%\tablenum{1}
\tablecaption{Orbital Parameters\label{tab:orbital_params}}
\tablehead{
\colhead{\textbf{KOI}} &
\colhead{\textbf{KIC}} &
\colhead{\textbf{$T_0$}} &
\colhead{\textbf{Period}} &
\colhead{\textbf{Impact}} &
\colhead{\textbf{R$_{\rm PL}$/R$_{\ast}$}} &
\colhead{\textbf{e}} &
\colhead{\textbf{$\omega$}} &
\colhead{\textbf{R$_{\rm PL}$}} &
\colhead{\textbf{Inclination}} &
\colhead{\textbf{a/R$_{\ast}$}} &
\colhead{\textbf{a}} &
\colhead{\textbf{$T_{\rm PL}$}} &
\colhead{\textbf{Depth}} &
\colhead{\textbf{Dur}} &
\colhead{\textbf{Sig}} &
\colhead{\textbf{p1}} &
\colhead{\textbf{p2}} \\

\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(BKJD)}} &
\colhead{\textbf{(d)}} &
\colhead{\textbf{Parameter}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(radian)}} &
\colhead{\textbf{(R$_{\oplus}$)}} &
\colhead{\textbf{($\deg$)}} &
\colhead{\textbf{}} &
\colhead{\textbf{(AU)}} &
\colhead{\textbf{(K)}} &
\colhead{\textbf{(ppm)}} &
\colhead{\textbf{(hr)}} &
\colhead{\textbf{($\sigma$)}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} 

}

\startdata

\textbf{K00005.01}  & 8554498    & 132.9733  &$    4.78033 ^{+    0.00001 }_{   -0.00001 }$&$ 0.93  ^{+ 0.01  }_{ -0.01 }$&$ 0.045  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 8.07  \pm{ 0.64  }$&$ 82.72 ^{+ 0.61  }_{ -0.46 }$&$ 7.6   ^{+ 0.5   }_{ -0.4  }$&$ 0.059  \pm{ 0.002  }$&$ 1434  \pm{ 45    }$&$ 983   \pm{ 3     }$& 2.3   &\textbf{ 5.1  }&0.932&\textbf{0.997} \\
K00005.02  & 8554498    & 133.3670  &$    7.05186 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.16  }_{ -0.17 }$&$ 0.003  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.04  ^{+ 0.21  }_{ -0.04 }$&$ 0.51  \pm{ 0.26  }$&$ 85.30 ^{+ 0.72  }_{ -0.60 }$&$ 11.2  ^{+ 1.0   }_{ -1.0  }$&$ 0.075  \pm{ 0.002  }$&$ 1159  \pm{ 69    }$&$ 12    \pm{ 4     }$& 1.9   & 0.4  &0.015&0.278\\
K00041.01  & 6521045    & 122.9506  &$   12.81574 ^{+    0.00004 }_{   -0.00005 }$&$ 0.57  ^{+ 0.20  }_{ -0.55 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.00  ^{+ 0.88  }_{ -0.00 }$&$ 3.08  \pm{ 0.74  }$&$ 87.33 ^{+ 2.57  }_{ -2.06 }$&$ 12.0  ^{+ 2.5   }_{ -2.4  }$&$ 0.114  \pm{ 0.005  }$&$ 1120  \pm{ 130   }$&$ 219   \pm{ 5     }$& 6.7   & 1.5  &0.615&0.988\\
K00041.02  & 6521045    & 133.1758  &$    6.88710 ^{+    0.00016 }_{   -0.00015 }$&$ 0.90  ^{+ 0.02  }_{ -0.09 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.11  ^{+ 0.19  }_{ -0.11 }$&$ 0.01  ^{+ 1.11  }_{ -0.01 }$&$ 3.13  \pm{ 0.58  }$&$ 81.11 ^{+ 1.65  }_{ -1.50 }$&$ 5.4   ^{+ 1.3   }_{ -0.5  }$&$ 0.076  \pm{ 0.003  }$&$ 1628  \pm{ 119   }$&$ 72    \pm{ 4     }$& 4.4   & 0.3  &0.067&0.783\\
K00041.03  & 6521045    & 153.9839  &$   35.33314 ^{+    0.00109 }_{   -0.00204 }$&$ 0.93  ^{+ 0.10  }_{ -0.14 }$&$ 0.012  ^{+ 0.000  }_{ -0.003 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.00  ^{+ 3.09  }_{ -0.00 }$&$ 3.78  \pm{ 0.88  }$&$ 86.88 ^{+ 0.83  }_{ -0.55 }$&$ 17.0  ^{+ 4.8   }_{ -2.4  }$&$ 0.226  \pm{ 0.010  }$&$ 947   \pm{ 106   }$&$ 96    \pm{ 10    }$& 6.3   & 1.0  &0.077&0.807\\
\textbf{K00070.01  }& 6850504    & 138.6075  &$   10.85409 ^{+    0.00002 }_{   -0.00003 }$&$ 0.31  ^{+ 0.26  }_{ -0.31 }$&$ 0.028  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.16  ^{+ 3.20  }_{ -0.16 }$&$ 2.94  \pm{ 0.26  }$&$ 89.13 ^{+ 0.87  }_{ -0.78 }$&$ 20.4  ^{+ 1.1   }_{ -1.2  }$&$ 0.092  \pm{ 0.003  }$&$ 803   \pm{ 32    }$&$ 1060  \pm{ 9     }$& 4.0   & 0.5  &0.959&\textbf{0.999} \\
K00070.02  & 6850504    & 134.5009  &$    3.69612 ^{+    0.00002 }_{   -0.00002 }$&$ 0.36  ^{+ 0.17  }_{ -0.36 }$&$ 0.017  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.00  ^{+  0.34 }_{ -0.00 }$&$ 1.77  \pm{ 0.18  }$&$ 87.96 ^{+ 2.04  }_{ -1.23 }$&$ 10.1  ^{+ 0.7   }_{ -0.7  }$&$ 0.045  \pm{ 0.002  }$&$ 1140  \pm{ 53    }$&$ 400   \pm{ 5     }$& 2.7   & 1.7  &0.821&0.996\\
K00070.03  & 6850504    & 164.7276  &$   77.61153 ^{+    0.00017 }_{   -0.00022 }$&$ 0.32  ^{+ 0.21  }_{ -0.32 }$&$ 0.026  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 2.68  \pm{ 0.27  }$&$ 89.76 ^{+ 0.24  }_{ -0.18 }$&$ 77.4  ^{+ 6.0   }_{ -6.4  }$&$ 0.341  \pm{ 0.012  }$&$ 409   \pm{ 20    }$&$ 834   \pm{ 28    }$& 7.4   & 0.5  &0.549&0.984\\
K00070.04  & 6850504    & 135.9338  &$    6.09850 ^{+    0.00018 }_{   -0.00022 }$&$ 0.07  ^{+ 0.59  }_{ -0.07 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.52  ^{+ 0.19  }_{ -0.50 }$&$ 3.16  ^{+ 1.61  }_{ -2.67 }$&$ 0.82  \pm{ 0.13  }$&$ 89.70 ^{+ 0.30  }_{ -2.46 }$&$ 14.3  ^{+ 1.1   }_{ -1.2  }$&$ 0.063  \pm{ 0.002  }$&$ 951   \pm{ 54    }$&$ 74    \pm{ 7     }$& 2.8   & 0.3  &0.037&0.657\\
K00070.05  & 6850504    & 135.2142  &$   19.57709 ^{+    0.00077 }_{   -0.00066 }$&$ 0.34  ^{+ 0.44  }_{ -0.31 }$&$ 0.009  ^{+ 0.002  }_{ -0.001 }$&$ 0.01  ^{+ 0.37  }_{ -0.01 }$&$ 0.00  ^{+ 1.02  }_{ -0.00 }$&$ 0.89  \pm{ 0.16  }$&$ 89.37 ^{+ 0.58  }_{ -0.83 }$&$ 31.0  ^{+ 2.4   }_{ -2.5  }$&$ 0.136  \pm{ 0.005  }$&$ 646   \pm{ 35    }$&$ 104   \pm{ 13    }$& 4.5   & 1.5  &0.023&0.538\\
\textbf{K00072.01}  & 11904151   & 131.5744  &$    0.83749 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 1.25  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -3.73 }$&$ 3.4   ^{+ 0.2   }_{ -0.2  }$&$ 0.016  \pm{ 0.001  }$&$ 2068  \pm{ 92    }$&$ 190   \pm{ 1     }$& 2.0   &\textbf{ 5.5  }&0.936&\textbf{0.997} \\
K00072.02  & 11904151   & 138.6781  &$   45.29404 ^{+    0.00011 }_{   -0.00011 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.020  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 2.10  \pm{ 0.18  }$&$ 90.00 ^{+ 0.00  }_{ -0.48 }$&$ 50.5  ^{+ 3.4   }_{ -3.9  }$&$ 0.230  \pm{ 0.009  }$&$ 527   \pm{ 21    }$&$ 480   \pm{ 13    }$& 7.0   & 0.6  &0.775&0.989\\
\textbf{K00082.01  }& 10187017   & 134.7534  &$   16.14569 ^{+    0.00003 }_{   -0.00003 }$&$ 0.25  ^{+ 0.31  }_{ -0.25 }$&$ 0.026  ^{+ 0.003  }_{ -0.000 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 0.00  ^{+ 4.10  }_{ -0.00 }$&$ 2.19  \pm{ 0.18  }$&$ 89.56 ^{+ 0.44  }_{ -0.64 }$&$ 32.2  ^{+ 1.6   }_{ -2.0  }$&$ 0.117  \pm{ 0.003  }$&$ 579   \pm{ 26    }$&$ 974   \pm{ 7     }$& 3.9   & 1.1  &0.974&\textbf{0.999} \\
K00082.02  & 10187017   & 134.0798  &$   10.31173 ^{+    0.00006 }_{   -0.00010 }$&$ 0.28  ^{+ 0.26  }_{ -0.28 }$&$ 0.014  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.00  ^{+  0.17 }_{ -0.00 }$&$ 1.19  \pm{ 0.12  }$&$ 89.31 ^{+ 0.69  }_{ -0.72 }$&$ 24.1  ^{+ 1.8   }_{ -1.5  }$&$ 0.086  \pm{ 0.002  }$&$ 669   \pm{ 32    }$&$ 276   \pm{ 5     }$& 3.2   & 0.5  &0.637&0.989\\
K00082.03  & 10187017   & 145.0258  &$   27.45362 ^{+    0.00070 }_{   -0.00064 }$&$ 0.02  ^{+ 0.59  }_{ -0.02 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.34  ^{+ 0.30  }_{ -0.33 }$&$ 0.26  ^{+ 3.23  }_{ -0.26 }$&$ 0.82  \pm{ 0.12  }$&$ 89.97 ^{+ 0.03  }_{ -0.75 }$&$ 46.8  ^{+ 4.1   }_{ -3.7  }$&$ 0.166  \pm{ 0.004  }$&$ 476   \pm{ 27    }$&$ 145   \pm{ 9     }$& 3.9   & 0.7  &0.066&0.779\\
K00082.04  & 10187017   & 139.9875  &$    7.07134 ^{+    0.00019 }_{   -0.00019 }$&$ 0.22  ^{+ 0.36  }_{ -0.22 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.64  \pm{ 0.08  }$&$ 89.34 ^{+ 0.66  }_{ -1.12 }$&$ 19.0  ^{+ 1.3   }_{ -1.5  }$&$ 0.067  \pm{ 0.002  }$&$ 749   \pm{ 41    }$&$ 79    \pm{ 5     }$& 2.8   & 0.6  &0.068&0.784\\
K00082.05  & 10187017   & 135.8466  &$    5.28698 ^{+    0.00018 }_{   -0.00020 }$&$ 0.68  ^{+ 1.07  }_{ -0.04 }$&$ 0.006  ^{+ 0.034  }_{ -0.000 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.02  ^{+ 1.57  }_{ -0.00 }$&$ 0.51  \pm{ 1.43  }$&$ 87.09 ^{+ 0.09  }_{ -3.30 }$&$ 15.5  ^{+ 1.4   }_{ -1.3  }$&$ 0.055  \pm{ 0.001  }$&$ 890   \pm{ 67    }$&$ 41    \pm{ 4     }$& 2.2   & 0.6  &0.038&0.665\\
\textbf{K00085.01  }& 5866724    & 132.0395  &$    5.85993 ^{+    0.00002 }_{   -0.00002 }$&$ 0.53  ^{+ 0.11  }_{ -0.53 }$&$ 0.020  ^{+ 0.002  }_{ -0.004 }$&$ 0.77  ^{+ 0.10  }_{ -0.58 }$&$ 4.60  ^{+ 0.19  }_{ -1.44 }$&$ 2.60  \pm{ 0.47  }$&$ 87.36 ^{+ 2.64  }_{ -0.61 }$&$ 11.8  ^{+ 1.1   }_{ -1.0  }$&$ 0.067  \pm{ 0.003  }$&$ 1203  \pm{ 74    }$&$ 321   \pm{ 3     }$& 4.4   &\textbf{ 5.2  }&0.939&\textbf{0.999} \\
K00085.02  & 5866724    & 133.4963  &$    2.15492 ^{+    0.00013 }_{   -0.00011 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.009  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.01  ^{+ 1.78  }_{ -0.01 }$&$ 1.29  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -3.96 }$&$ 5.5   ^{+ 0.4   }_{ -0.3  }$&$ 0.035  \pm{ 0.001  }$&$ 1786  \pm{ 82    }$&$ 99    \pm{ 2     }$& 3.2   &\textbf{ 3.7  }&0.657&0.990\\
K00085.03  & 5866724    & 137.9953  &$    8.13115 ^{+    0.00009 }_{   -0.00006 }$&$ 0.62  ^{+ 0.13  }_{ -0.49 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 0.00  ^{+ 1.45  }_{ -0.00 }$&$ 1.62  \pm{ 0.13  }$&$ 86.86 ^{+ 2.45  }_{ -1.00 }$&$ 12.7  ^{+ 0.5   }_{ -0.9  }$&$ 0.085  \pm{ 0.003  }$&$ 1215  \pm{ 52    }$&$ 116   \pm{ 4     }$& 4.3   & 1.6  &0.382&0.969\\
K00089.01  & 8056665    & 150.5651  &$   84.68895 ^{+    0.00012 }_{   -0.00010 }$&$ 0.54  ^{+ 0.26  }_{ -0.54 }$&$ 0.017  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 0.00  ^{+ 0.79  }_{ -0.00 }$&$ 4.97  \pm{ 1.65  }$&$ 89.29 ^{+ 0.71  }_{ -0.62 }$&$ 38.1  ^{+ 9.2   }_{ -11.0 }$&$ 0.473  \pm{ 0.014  }$&$ 775   \pm{ 120   }$&$ 402   \pm{ 17    }$& 12.6  & 0.7  &0.019&0.323\\
K00089.02  & 8056665    & 289.8688  &$  207.60349 ^{+    0.00047 }_{   -0.00036 }$&$ 0.94  ^{+ 0.41  }_{ -0.10 }$&$ 0.032  ^{+  0.000 }_{ -0.013 }$&$ 0.01  ^{+ 0.66  }_{ -0.01 }$&$ 0.00  ^{+ 1.57  }_{ -0.00 }$&$ 10.66 \pm{ 3.82  }$&$ 89.24 ^{+ 0.27  }_{ -0.61 }$&$ 61.6  ^{+ 20.4  }_{ -16.2 }$&$ 0.861  \pm{ 0.023  }$&$ 608   \pm{ 98    }$&$ 490   \pm{ 33    }$& 9.6   & 0.6  &0.038&0.495\\
\textbf{K00094.01  }& 6462863    & 132.7405  &$   22.34300 ^{+    0.00001 }_{   -0.00001 }$&$ 0.45  ^{+ 0.14  }_{ -0.20 }$&$ 0.069  ^{+ 0.004  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 10.51 \pm{ 0.97  }$&$ 88.93 ^{+ 0.51  }_{ -0.46 }$&$ 24.3  ^{+ 1.3   }_{ -1.5  }$&$ 0.158  \pm{ 0.007  }$&$ 833   \pm{ 35    }$&$ 5426  \pm{ 27    }$& 6.8   &\textbf{ 13.6 }&0.978&\textbf{1.000} \\
K00094.02  & 6462863    & 138.0072  &$   10.42371 ^{+    0.00003 }_{   -0.00003 }$&$ 0.40  ^{+  0.00 }_{ -0.40 }$&$ 0.026  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 3.98  \pm{ 0.32  }$&$ 88.36 ^{+ 1.64  }_{ -0.00 }$&$ 14.5  ^{+ 0.8   }_{ -0.8  }$&$ 0.095  \pm{ 0.004  }$&$ 1078  \pm{ 39    }$&$ 769   \pm{ 11    }$& 5.1   &\textbf{ 3.0  }&0.246&0.942\\
K00094.03  & 6462863    & 161.2400  &$   54.31993 ^{+    0.00006 }_{   -0.00010 }$&$ 0.39  ^{+ 0.20  }_{ -0.28 }$&$ 0.043  ^{+  0.000 }_{ -0.003 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 6.60  \pm{ 0.60  }$&$ 89.49 ^{+ 0.37  }_{ -0.32 }$&$ 44.0  ^{+ 2.6   }_{ -2.9  }$&$ 0.285  \pm{ 0.012  }$&$ 614   \pm{ 27    }$&$ 2494  \pm{ 37    }$& 8.9   &\textbf{ 3.7  }&0.464&0.977\\
K00094.04  & 6462863    & 131.6139  &$    3.74324 ^{+    0.00006 }_{   -0.00009 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 1.49  \pm{ 0.15  }$&$ 90.00 ^{+ 0.00  }_{ -1.65 }$&$ 7.3   ^{+ 0.5   }_{ -0.4  }$&$ 0.048  \pm{ 0.002  }$&$ 1513  \pm{ 61    }$&$ 125   \pm{ 7     }$& 3.9   & 1.7  &0.085&0.823\\
K00102.01  & 8456679    & 135.0591  &$    1.73514 ^{+    0.00000 }_{   -0.00000 }$&$ 0.56  ^{+ 0.03  }_{ -0.03 }$&$ 0.034  ^{+ 0.000  }_{ -0.000 }$&$ 0.78  ^{+ 0.04  }_{ -0.09 }$&$ 4.70  ^{+  0.06 }_{ -0.23 }$&$ 3.85  \pm{ 0.38  }$&$ 84.57 ^{+ 0.77  }_{ -1.46 }$&$ 5.9   ^{+ 0.4   }_{ -0.5  }$&$ 0.028  \pm{ 0.001  }$&$ 1592  \pm{ 104   }$&$ 946   \pm{ 3     }$& 2.7   &\textbf{ 27.2 }&0.906&0.996\\
K00102.02  & 8456679    & 132.2635  &$    4.06853 ^{+    0.00008 }_{   -0.00015 }$&$ 0.51  ^{+ 0.32  }_{ -0.49 }$&$ 0.008  ^{+ 0.009  }_{ -0.002 }$&$ 0.71  ^{+ 0.19  }_{ -0.71 }$&$ 3.62  ^{+ 1.10  }_{ -3.60 }$&$ 0.94  \pm{ 0.62  }$&$ 87.13 ^{+ 2.76  }_{ -1.79 }$&$ 10.3  ^{+ 0.9   }_{ -0.8  }$&$ 0.050  \pm{ 0.002  }$&$ 1210  \pm{ 73    }$&$ 98    \pm{ 6     }$& 3.0   & 2.6  &0.008&0.168\\
K00108.01  & 4914423    & 142.1763  &$   15.96535 ^{+    0.00006 }_{   -0.00006 }$&$ 0.51  ^{+ 0.11  }_{ -0.32 }$&$ 0.020  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.35  }_{ -0.00 }$&$ 0.03  ^{+ 0.53  }_{ -0.03 }$&$ 2.66  \pm{ 0.28  }$&$ 88.69 ^{+ 0.87  }_{ -0.40 }$&$ 22.5  ^{+ 1.7   }_{ -1.7  }$&$ 0.128  \pm{ 0.005  }$&$ 840   \pm{ 42    }$&$ 492   \pm{ 8     }$& 4.8   & 0.3  &0.719&0.985\\
K00108.02  & 4914423    & 295.3304  &$  179.60101 ^{+    0.00008 }_{   -0.00003 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 0.032  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 4.38  \pm{ 0.45  }$&$ 90.00 ^{+ 0.00  }_{ -0.25 }$&$ 109.4 ^{+ 6.8   }_{ -7.3  }$&$ 0.647  \pm{ 0.025  }$&$ 382   \pm{ 16    }$&$ 1296  \pm{ 35    }$& 13.0  & 0.8  &0.171&0.838\\
K00111.01  & 6678383    & 137.6139  &$   11.42751 ^{+    0.00004 }_{   -0.00005 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.020  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.01  ^{+ 3.85  }_{ -0.01 }$&$ 2.21  \pm{ 0.19  }$&$ 90.00 ^{+ 0.00  }_{ -1.32 }$&$ 19.5  ^{+ 1.4   }_{ -1.1  }$&$ 0.092  \pm{ 0.004  }$&$ 871   \pm{ 35    }$&$ 509   \pm{ 8     }$& 4.7   & 1.8  &0.752&0.993\\
K00111.02  & 6678383    & 132.7129  &$   23.66834 ^{+    0.00011 }_{   -0.00011 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.019  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+ 1.38  }_{ -0.00 }$&$ 2.07  \pm{ 0.17  }$&$ 90.00 ^{+ 0.00  }_{ -0.81 }$&$ 32.5  ^{+ 1.9   }_{ -2.0  }$&$ 0.149  \pm{ 0.005  }$&$ 673   \pm{ 27    }$&$ 480   \pm{ 12    }$& 5.8   & 1.1  &0.550&0.984\\
K00111.03  & 6678383    & 271.0832  &$   51.75627 ^{+    0.00023 }_{   -0.00024 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.022  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.04  ^{+ 3.87  }_{ -0.04 }$&$ 2.31  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -0.49 }$&$ 56.2  ^{+ 4.0   }_{ -4.1  }$&$ 0.251  \pm{ 0.010  }$&$ 510   \pm{ 25    }$&$ 621   \pm{ 19    }$& 7.3   & 0.3  &0.464&0.977\\
K00112.01  & 10984090   & 185.1795  &$   51.07931 ^{+    0.00014 }_{   -0.00022 }$&$ 0.24  ^{+ 0.14  }_{ -0.24 }$&$ 0.024  ^{+ 0.001  }_{ -0.000 }$&$ 0.05  ^{+ 0.22  }_{ -0.05 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 2.55  \pm{ 0.24  }$&$ 89.76 ^{+ 0.24  }_{ -0.15 }$&$ 58.0  ^{+ 4.0   }_{ -4.4  }$&$ 0.262  \pm{ 0.011  }$&$ 512   \pm{ 24    }$&$ 749   \pm{ 19    }$& 6.7   & 0.4  &0.489&0.960\\
K00112.02  & 10984090   & 133.9857  &$    3.70919 ^{+    0.00007 }_{   -0.00007 }$&$ 0.37  ^{+ 0.18  }_{ -0.37 }$&$ 0.010  ^{+ 0.002  }_{ -0.001 }$&$ 0.16  ^{+ 0.43  }_{ -0.16 }$&$ 4.75  ^{+ 1.10  }_{ -4.56 }$&$ 1.06  \pm{ 0.15  }$&$ 87.89 ^{+ 2.11  }_{ -1.11 }$&$ 9.9   ^{+ 0.8   }_{ -0.6  }$&$ 0.046  \pm{ 0.002  }$&$ 1230  \pm{ 62    }$&$ 138   \pm{ 5     }$& 3.1   & 0.9  &0.070&0.651\\
\textbf{K00115.01  }& 9579641    & 133.1424  &$    5.41220 ^{+    0.00002 }_{   -0.00002 }$&$ 0.64  ^{+ 0.26  }_{ -0.17 }$&$ 0.028  ^{+ 0.001  }_{ -0.006 }$&$ 0.47  ^{+ 0.05  }_{ -0.47 }$&$ 4.75  ^{+ 0.28  }_{ -4.75 }$&$ 4.81  \pm{ 1.53  }$&$ 85.94 ^{+ 1.87  }_{ -3.88 }$&$ 8.9   ^{+ 2.4   }_{ -2.1  }$&$ 0.066  \pm{ 0.003  }$&$ 1418  \pm{ 228   }$&$ 600   \pm{ 6     }$& 3.3   & 2.8  &0.914&\textbf{0.998} \\
K00115.02  & 9579641    & 139.0032  &$    7.12597 ^{+    0.00011 }_{   -0.00016 }$&$ 0.70  ^{+ 0.14  }_{ -0.38 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 1.09  ^{+  0.00 }_{ -1.09 }$&$ 2.11  \pm{ 0.55  }$&$ 86.73 ^{+ 2.17  }_{ -1.51 }$&$ 11.4  ^{+ 2.8   }_{ -2.0  }$&$ 0.078  \pm{ 0.003  }$&$ 1214  \pm{ 145   }$&$ 196   \pm{ 7     }$& 3.3   & 0.7  &0.332&0.961\\
K00115.03  & 9579641    & 132.6570  &$    3.43584 ^{+    0.00009 }_{   -0.00006 }$&$ 0.64  ^{+ 0.60  }_{ -0.40 }$&$ 0.005  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.67  ^{+ 2.53  }_{ -0.67 }$&$ 0.80  \pm{ 0.31  }$&$ 84.85 ^{+ 3.35  }_{ -5.54 }$&$ 6.6   ^{+ 1.7   }_{ -1.6  }$&$ 0.048  \pm{ 0.002  }$&$ 1596  \pm{ 265   }$&$ 24    \pm{ 5     }$& 2.9   & 0.8  &0.049&0.720\\
K00116.01  & 8395660    & 136.2799  &$   13.57100 ^{+    0.00014 }_{   -0.00014 }$&$ 0.59  ^{+ 0.17  }_{ -0.29 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.01  ^{+ 0.41  }_{ -0.01 }$&$ 2.29  \pm{ 0.43  }$&$ 88.56 ^{+ 0.81  }_{ -0.76 }$&$ 22.9  ^{+ 3.4   }_{ -3.4  }$&$ 0.110  \pm{ 0.005  }$&$ 799   \pm{ 73    }$&$ 518   \pm{ 13    }$& 3.6   & 0.6  &0.200&0.926\\
K00116.02  & 8395660    & 151.9344  &$   43.84445 ^{+    0.00014 }_{   -0.00041 }$&$ 0.37  ^{+ 0.22  }_{ -0.37 }$&$ 0.023  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+  0.24}_{ -0.00 }$&$ 2.69  \pm{ 0.41  }$&$ 89.56 ^{+ 0.44  }_{ -0.37 }$&$ 48.4  ^{+ 5.2   }_{ -6.6  }$&$ 0.241  \pm{ 0.011  }$&$ 560   \pm{ 43    }$&$ 668   \pm{ 24    }$& 6.5   & 0.7  &0.144&0.894\\
K00116.03  & 8395660    & 135.6340  &$    6.16500 ^{+    0.00000 }_{   -0.00000 }$&$ 0.39  ^{+ 0.29  }_{ -0.39 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.01  ^{+ 0.24  }_{ -0.01 }$&$ 0.86  \pm{ 0.19  }$&$ 88.28 ^{+ 1.71  }_{ -1.38 }$&$ 12.9  ^{+ 2.1   }_{ -1.9  }$&$ 0.065  \pm{ 0.003  }$&$ 1077  \pm{ 110   }$&$ 68    \pm{ 9     }$& 3.3   & 0.8  &0.010&0.325\\
K00116.04  & 8395660    & 147.5282  &$   23.98000 ^{+    0.00115 }_{   -0.00128 }$&$ 0.40  ^{+ 0.38  }_{ -0.40 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.29  ^{+ 0.43  }_{ -0.29 }$&$ 3.20  ^{+ 1.47  }_{ -2.94 }$&$ 1.08  \pm{ 0.25  }$&$ 89.32 ^{+ 0.68  }_{ -0.80 }$&$ 32.6  ^{+ 5.4   }_{ -5.3  }$&$ 0.161  \pm{ 0.007  }$&$ 671   \pm{ 78    }$&$ 98    \pm{ 18    }$& 5.0   & 0.4  &0.010&0.325\\
K00117.01  & 10875245   & 138.7788  &$   14.74910 ^{+    0.00008 }_{   -0.00008 }$&$ 0.94  ^{+ 0.06  }_{ -0.04 }$&$ 0.022  ^{+ 0.000  }_{ -0.001 }$&$ 0.10  ^{+ 0.06  }_{ -0.10 }$&$ 0.44  ^{+ 0.95  }_{ -0.44 }$&$ 8.93  \pm{ 0.76  }$&$ 83.20 ^{+ 0.59  }_{ -0.66 }$&$ 8.0   ^{+ 0.2   }_{ -0.2  }$&$ 0.137  \pm{ 0.007  }$&$ 1404  \pm{ 36    }$&$ 436   \pm{ 11    }$& 6.7   & 0.6  &0.347&0.964\\
K00117.02  & 10875245   & 138.6039  &$    4.90147 ^{+    0.00015 }_{   -0.00015 }$&$ 1.00  ^{+  0.00 }_{ -0.10 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+  0.19 }_{ -0.00 }$&$ 1.30  ^{+  0.00}_{ -1.30 }$&$ 4.97  \pm{ 0.43  }$&$ 73.48 ^{+ 3.46  }_{ -1.03 }$&$ 3.9   ^{+ 0.1   }_{ -0.1  }$&$ 0.065  \pm{ 0.003  }$&$ 1995  \pm{ 50    }$&$ 138   \pm{ 6     }$& 4.4   & 0.4  &0.123&0.875\\
K00117.03  & 10875245   & 133.5041  &$    3.17996 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.08  }_{ -0.02 }$&$ 0.013  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 1.38  }_{ -0.00 }$&$ 5.10  \pm{ 0.51  }$&$ 72.19 ^{+ 1.05  }_{ -1.70 }$&$ 2.9   ^{+ 0.1   }_{ -0.1  }$&$ 0.048  \pm{ 0.003  }$&$ 2300  \pm{ 73    }$&$ 121   \pm{ 5     }$& 4.0   & 1.1  &0.133&0.884\\
K00117.04  & 10875245   & 137.8159  &$    7.95792 ^{+    0.00038 }_{   -0.00041 }$&$ 0.69  ^{+ 4.08  }_{ -0.31 }$&$ 0.013  ^{+ 0.012  }_{ -0.011 }$&$ 0.39  ^{+  0.24 }_{ -0.29 }$&$ 4.86  ^{+  3.06 }_{ -3.40 }$&$ 2.30  \pm{ 2.63  }$&$ 81.15 ^{+  1.34 }_{ -2.79 }$&$ 11.1  ^{+ 6.7   }_{ -5.6  }$&$ 0.085  \pm{ 0.006  }$&$ 1861  \pm{ 2228  }$&$ 50    \pm{ 8     }$& 6.9   & 0.4  &0.016&0.446\\
K00119.01  & 9471974    & 141.9096  &$   49.18431 ^{+    0.00005 }_{   -0.00004 }$&$ 0.37  ^{+ 0.25  }_{ -0.37 }$&$ 0.035  ^{+ 0.005  }_{ -0.001 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 3.82  }_{ -0.00 }$&$ 6.70  \pm{ 1.33  }$&$ 89.34 ^{+ 0.66  }_{ -0.57 }$&$ 33.0  ^{+ 4.9   }_{ -4.5  }$&$ 0.266  \pm{ 0.014  }$&$ 655   \pm{ 51    }$&$ 1373  \pm{ 25    }$& 11.2  &\textbf{ 11.3 }&0.836&0.992\\
K00119.02  & 9471974    & 312.6812  &$  190.31340 ^{+    0.00063 }_{   -0.00053 }$&$ 0.38  ^{+ 0.21  }_{ -0.38 }$&$ 0.030  ^{+ 0.009  }_{ -0.002 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.00  ^{+ 4.71  }_{ -0.00 }$&$ 4.60  \pm{ 1.39  }$&$ 89.76 ^{+ 0.24  }_{ -0.22 }$&$ 97.7  ^{+ 25.4  }_{ -19.2 }$&$ 0.644  \pm{ 0.026  }$&$ 392   \pm{ 51    }$&$ 1146  \pm{ 39    }$& 15.2  &\textbf{ 4.8  }&0.382&0.939\\
K00123.01  & 5094751    & 122.9737  &$    6.48168 ^{+    0.00004 }_{   -0.00004 }$&$ 0.53  ^{+ 0.09  }_{ -0.52 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 2.39  \pm{ 0.28  }$&$ 87.09 ^{+ 2.85  }_{ -0.74 }$&$ 10.3  ^{+ 0.8   }_{ -0.9  }$&$ 0.069  \pm{ 0.002  }$&$ 1200  \pm{ 63    }$&$ 302   \pm{ 5     }$& 4.1   & 0.3  &0.703&0.983\\
K00123.02  & 5094751    & 137.5738  &$   21.22254 ^{+    0.00010 }_{   -0.00010 }$&$ 0.37  ^{+ 0.09  }_{ -0.37 }$&$ 0.017  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.09  ^{+ 0.77  }_{ -0.09 }$&$ 2.70  \pm{ 0.27  }$&$ 89.09 ^{+ 0.91  }_{ -0.27 }$&$ 22.8  ^{+ 1.6   }_{ -1.8  }$&$ 0.152  \pm{ 0.003  }$&$ 810   \pm{ 38    }$&$ 357   \pm{ 10    }$& 6.6   & 0.4  &0.450&0.953\\
K00124.01  & 11086270   & 137.1212  &$   12.69115 ^{+    0.00020 }_{   -0.00014 }$&$ 0.85  ^{+ 0.04  }_{ -0.16 }$&$ 0.016  ^{+ 0.000  }_{ -0.002 }$&$ 0.06  ^{+ 0.56  }_{ -0.06 }$&$ 0.00  ^{+ 1.01  }_{ -0.00 }$&$ 2.98  \pm{ 0.33  }$&$ 86.46 ^{+ 0.92  }_{ -0.58 }$&$ 14.0  ^{+ 1.1   }_{ -1.1  }$&$ 0.108  \pm{ 0.002  }$&$ 1056  \pm{ 53    }$&$ 256   \pm{ 9     }$& 4.0   & 1.0  &0.421&0.948\\
K00124.02  & 11086270   & 142.8190  &$   31.71987 ^{+    0.00025 }_{   -0.00034 }$&$ 0.86  ^{+ 0.05  }_{ -0.08 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 3.57  \pm{ 0.43  }$&$ 88.10 ^{+ 0.39  }_{ -0.37 }$&$ 26.1  ^{+ 2.6   }_{ -1.9  }$&$ 0.200  \pm{ 0.004  }$&$ 771   \pm{ 50    }$&$ 369   \pm{ 15    }$& 5.2   & 0.4  &0.363&0.934\\
K00139.01  & 8559644    & 142.0874  &$  224.79712 ^{+    0.00003 }_{   -0.00001 }$&$ 0.18  ^{+ 0.42  }_{ -0.18 }$&$ 0.047  ^{+ 0.009  }_{ -0.001 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.10  ^{+ 4.60  }_{ -0.10 }$&$ 5.83  \pm{ 0.80  }$&$ 89.93 ^{+ 0.07  }_{ -0.19 }$&$ 141.8 ^{+ 12.4  }_{ -10.4 }$&$ 0.749  \pm{ 0.028  }$&$ 330   \pm{ 19    }$&$ 3395  \pm{ 68    }$& 12.4  & 0.8  &0.422&0.948\\
K00139.02  & 8559644    & 141.3521  &$    3.34184 ^{+    0.00005 }_{   -0.00007 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 1.39  \pm{ 0.15  }$&$ 90.00 ^{+  0.00 }_{ -3.08 }$&$ 8.2   ^{+ 0.6   }_{ -0.6  }$&$ 0.045  \pm{ 0.002  }$&$ 1387  \pm{ 64    }$&$ 167   \pm{ 7     }$& 3.2   & 0.5  &0.197&0.860\\
K00148.01  & 5735762    & 124.0630  &$    4.77798 ^{+    0.00003 }_{   -0.00004 }$&$ 0.20  ^{+ 0.31  }_{ -0.20 }$&$ 0.018  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 1.75  \pm{ 0.17  }$&$ 89.07 ^{+ 0.93  }_{ -1.67 }$&$ 12.4  ^{+ 0.8   }_{ -0.9  }$&$ 0.052  \pm{ 0.002  }$&$ 992   \pm{ 48    }$&$ 489   \pm{ 8     }$& 3.0   & 2.1  &0.352&0.964\\
K00148.02  & 5735762    & 125.3398  &$    9.67393 ^{+    0.00003 }_{   -0.00003 }$&$ 0.39  ^{+ 0.19  }_{ -0.37 }$&$ 0.027  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 2.60  \pm{ 0.26  }$&$ 88.89 ^{+ 1.07  }_{ -0.71 }$&$ 20.1  ^{+ 1.4   }_{ -1.6  }$&$ 0.083  \pm{ 0.003  }$&$ 772   \pm{ 37    }$&$ 987   \pm{ 12    }$& 3.5   & 2.3  &0.632&0.988\\
K00148.03  & 5735762    & 146.0657  &$   42.89592 ^{+    0.00051 }_{   -0.00048 }$&$ 0.19  ^{+ 0.35  }_{ -0.19 }$&$ 0.021  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.97  \pm{ 0.21  }$&$ 89.80 ^{+ 0.20  }_{ -0.40 }$&$ 54.5  ^{+ 4.8   }_{ -4.1  }$&$ 0.224  \pm{ 0.009  }$&$ 467   \pm{ 25    }$&$ 599   \pm{ 28    }$& 6.0   & 1.1  &0.089&0.830\\
K00153.01  & 12252424   & 139.7122  &$    8.92511 ^{+    0.00005 }_{   -0.00005 }$&$ 0.63  ^{+ 0.13  }_{ -0.09 }$&$ 0.034  ^{+ 0.004  }_{ -0.006 }$&$ 0.50  ^{+ 0.26  }_{ -0.37 }$&$ 4.24  ^{+ 0.46  }_{ -1.97 }$&$ 2.86  \pm{ 0.67  }$&$ 88.21 ^{+ 0.56  }_{ -0.75 }$&$ 20.9  ^{+ 4.3   }_{ -3.1  }$&$ 0.077  \pm{ 0.002  }$&$ 698   \pm{ 78    }$&$ 997   \pm{ 15    }$& 3.1   & 1.0  &0.871&0.994\\
K00153.02  & 12252424   & 128.5467  &$    4.75399 ^{+    0.00002 }_{   -0.00002 }$&$ 0.38  ^{+ 0.24  }_{ -0.38 }$&$ 0.023  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 0.00  ^{+ 1.44  }_{ -0.00 }$&$ 2.12  \pm{ 0.28  }$&$ 88.28 ^{+ 1.72  }_{ -1.47 }$&$ 12.9  ^{+ 1.3   }_{ -1.2  }$&$ 0.050  \pm{ 0.001  }$&$ 883   \pm{ 57    }$&$ 780   \pm{ 10    }$& 2.7   & 0.5  &0.889&0.995\\
K00159.01  & 8972058    & 136.7363  &$    8.99092 ^{+    0.00011 }_{   -0.00001 }$&$ 0.59  ^{+ 0.20  }_{ -0.57 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 0.73  }_{ -0.00 }$&$ 3.14  \pm{ 0.65  }$&$ 87.39 ^{+ 2.52  }_{ -1.86 }$&$ 12.8  ^{+ 2.5   }_{ -2.1  }$&$ 0.087  \pm{ 0.003  }$&$ 1120  \pm{ 123   }$&$ 466   \pm{ 12    }$& 4.4   & 0.5  &0.306&0.917\\
K00159.02  & 8972058    & 134.7278  &$    2.40365 ^{+    0.00002 }_{   -0.00002 }$&$ 0.93  ^{+ 0.03  }_{ -0.04 }$&$ 0.013  ^{+  0.000 }_{ -0.003 }$&$ 0.05  ^{+ 0.06  }_{ -0.05 }$&$ 0.17  ^{+ 0.43  }_{ -0.17 }$&$ 2.41  \pm{ 0.34  }$&$ 78.01 ^{+ 1.11  }_{ -1.48 }$&$ 4.5   ^{+ 0.4   }_{ -0.4  }$&$ 0.036  \pm{ 0.001  }$&$ 1905  \pm{ 100   }$&$ 82    \pm{ 6     }$& 1.7   & 0.6  &0.090&0.711\\
K00168.01  & 11512246   & 133.2871  &$   10.74245 ^{+    0.00006 }_{   -0.00006 }$&$ 0.37  ^{+ 0.41  }_{ -0.37 }$&$ 0.016  ^{+ 0.004  }_{ -0.000 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 3.79  \pm{ 1.14  }$&$ 87.97 ^{+ 2.03  }_{ -3.91 }$&$ 10.1  ^{+ 2.2   }_{ -2.5  }$&$ 0.100  \pm{ 0.003  }$&$ 1258  \pm{ 158   }$&$ 426   \pm{ 13    }$& 7.4   & 0.2  &0.332&0.961\\
K00168.02  & 11512246   & 147.5788  &$   15.27448 ^{+    0.00046 }_{   -0.00040 }$&$ 0.00  ^{+ 0.69  }_{ -0.00 }$&$ 0.011  ^{+ 0.003  }_{ -0.000 }$&$ 0.08  ^{+ 0.39  }_{ -0.08 }$&$ 1.93  ^{+ 2.10  }_{ -1.93 }$&$ 2.26  \pm{ 0.66  }$&$ 89.98 ^{+ 0.02  }_{ -3.15 }$&$ 14.0  ^{+ 2.7   }_{ -3.1  }$&$ 0.126  \pm{ 0.004  }$&$ 1062  \pm{ 138   }$&$ 210   \pm{ 17    }$& 7.5   & 0.4  &0.157&0.903\\
K00168.03  & 11512246   & 138.3254  &$    7.10690 ^{+    0.00029 }_{   -0.00022 }$&$ 0.18  ^{+ 0.40  }_{ -0.18 }$&$ 0.008  ^{+ 0.002  }_{ -0.001 }$&$ 0.04  ^{+ 0.18  }_{ -0.04 }$&$ 0.02  ^{+ 0.35  }_{ -0.02 }$&$ 1.91  \pm{ 0.54  }$&$ 88.79 ^{+ 1.21  }_{ -3.31 }$&$ 7.8   ^{+ 1.9   }_{ -1.7  }$&$ 0.076  \pm{ 0.002  }$&$ 1404  \pm{ 188   }$&$ 107   \pm{ 11    }$& 6.4   & 0.1  &0.093&0.837\\
\textbf{K00244.01  }& 4349452    & 178.5274  &$   12.72036 ^{+    0.00002 }_{   -0.00002 }$&$ 0.92  ^{+ 0.07  }_{ -0.02 }$&$ 0.039  ^{+ 0.002  }_{ -0.002 }$&$ 0.01  ^{+ 0.18  }_{ -0.01 }$&$ 0.00  ^{+ 0.81  }_{ -0.00 }$&$ 7.06  \pm{ 0.63  }$&$ 86.47 ^{+ 0.32  }_{ -0.58 }$&$ 14.6  ^{+ 1.0   }_{ -0.9  }$&$ 0.113  \pm{ 0.003  }$&$ 1046  \pm{ 40    }$&$ 1183  \pm{ 4     }$& 3.1   &\textbf{ 37.2 }&0.973&\textbf{0.999} \\
\textbf{K00244.02  }& 4349452    & 171.7046  &$    6.23856 ^{+    0.00001 }_{   -0.00001 }$&$ 0.68  ^{+ 0.09  }_{ -0.68 }$&$ 0.019  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 3.50  \pm{ 0.48  }$&$ 85.83 ^{+ 4.17  }_{ -1.20 }$&$ 9.0   ^{+ 0.9   }_{ -0.8  }$&$ 0.070  \pm{ 0.002  }$&$ 1327  \pm{ 85    }$&$ 421   \pm{ 3     }$& 3.9   &\textbf{ 15.9 }&0.953&\textbf{0.998} \\
\textbf{K00245.01  }& 8478994    & 175.2497  &$   39.79219 ^{+    0.00006 }_{   -0.00006 }$&$ 0.50  ^{+ 0.09  }_{ -0.50 }$&$ 0.022  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 1.92  \pm{ 0.19  }$&$ 89.51 ^{+ 0.49  }_{ -0.12 }$&$ 58.6  ^{+ 4.8   }_{ -4.7  }$&$ 0.217  \pm{ 0.008  }$&$ 460   \pm{ 24    }$&$ 607   \pm{ 5     }$& 4.7   &\textbf{ 7.1  }&0.947&\textbf{0.999} \\
K00245.02  & 8478994    & 191.8385  &$   21.30185 ^{+    0.00050 }_{   -0.00019 }$&$ 0.35  ^{+ 0.27  }_{ -0.35 }$&$ 0.008  ^{+ 0.002  }_{ -0.000 }$&$ 0.20  ^{+ 0.63  }_{ -0.20 }$&$ 3.50  ^{+ 1.34  }_{ -3.46 }$&$ 0.70  \pm{ 0.11  }$&$ 89.47 ^{+ 0.53  }_{ -0.45 }$&$ 38.5  ^{+ 3.1   }_{ -3.2  }$&$ 0.143  \pm{ 0.005  }$&$ 568   \pm{ 30    }$&$ 91    \pm{ 4     }$& 4.2   &\textbf{ 3.3  }&0.196&0.924\\
K00245.03  & 8478994    & 184.0333  &$   13.36727 ^{+    0.00042 }_{   -0.00061 }$&$ 0.80  ^{+ 0.43  }_{ -0.47 }$&$ 0.004  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.16  ^{+ 0.86  }_{ -0.16 }$&$ 0.37  \pm{ 0.21  }$&$ 88.40 ^{+ 0.95  }_{ -0.80 }$&$ 28.4  ^{+ 2.5   }_{ -2.2  }$&$ 0.105  \pm{ 0.003  }$&$ 657   \pm{ 38    }$&$ 17    \pm{ 3     }$& 2.2   & 1.1  &0.044&0.699\\
K00245.04  & 8478994    & 195.7268  &$   51.19880 ^{+    0.00016 }_{   -0.02033 }$&$ 0.68  ^{+ 0.81  }_{ -0.68 }$&$ 0.004  ^{+ 0.007  }_{ -0.002 }$&$ 0.24  ^{+ 0.20  }_{ -0.24 }$&$ 0.06  ^{+ 0.26  }_{ -0.06 }$&$ 0.34  \pm{ 0.36  }$&$ 89.45 ^{+ 0.55  }_{ -0.64 }$&$ 69.9  ^{+ 5.8   }_{ -4.8  }$&$ 0.256  \pm{ 0.009  }$&$ 415   \pm{ 23    }$&$ 15    \pm{ 7     }$& 4.1   & 0.3  &0.044&0.699\\
\textbf{K00246.01  }& 11295426   & 173.8571  &$    5.39877 ^{+    0.00001 }_{   -0.00001 }$&$ 0.38  ^{+ 0.20  }_{ -0.03 }$&$ 0.016  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 0.00  ^{+ 4.72  }_{ -0.00 }$&$ 2.20  \pm{ 0.13  }$&$ 87.98 ^{+  0.18 }_{ -1.10 }$&$ 10.7  ^{+ 0.2   }_{ -0.1  }$&$ 0.061  \pm{ 0.001  }$&$ 1177  \pm{ 12    }$&$ 349   \pm{ 2     }$& 3.6   &\textbf{ 8.4  }&0.972&\textbf{0.999} \\
K00246.02  & 11295426   & 136.3854  &$    9.60487 ^{+    0.00021 }_{   -0.00020 }$&$ 0.44  ^{+ 0.53  }_{ -0.16 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.45  ^{+ 0.26  }_{ -0.25 }$&$ 2.02  ^{+ 2.29  }_{ -1.79 }$&$ 0.92  \pm{ 0.13  }$&$ 88.41 ^{+ 0.59  }_{ -1.95 }$&$ 15.7  ^{+ 0.2   }_{ -0.2  }$&$ 0.090  \pm{ 0.001  }$&$ 967   \pm{ 10    }$&$ 58    \pm{ 3     }$& 2.9   & 0.7  &0.094&0.721\\
K00260.01  & 8292840    & 172.7904  &$   10.49570 ^{+    0.00010 }_{   -0.00005 }$&$ 0.65  ^{+ 0.15  }_{ -0.04 }$&$ 0.010  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 1.79  \pm{ 0.17  }$&$ 86.86 ^{+ 0.04  }_{ -0.94 }$&$ 13.5  ^{+ 0.9   }_{ -1.0  }$&$ 0.101  \pm{ 0.003  }$&$ 1185  \pm{ 56    }$&$ 119   \pm{ 3     }$& 5.2   & 1.6  &0.300&0.955\\
K00260.02  & 8292840    & 245.0413  &$  100.28340 ^{+    0.00028 }_{   -0.00085 }$&$ 0.15  ^{+ 0.41  }_{ -0.15 }$&$ 0.016  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 2.43  \pm{ 0.29  }$&$ 89.87 ^{+ 0.13  }_{ -0.39 }$&$ 69.6  ^{+ 6.0   }_{ -5.0  }$&$ 0.447  \pm{ 0.016  }$&$ 492   \pm{ 25    }$&$ 326   \pm{ 14    }$& 11.1  & 0.6  &0.379&0.968\\
K00260.03  & 8292840    & 140.2944  &$   21.86964 ^{+    0.00018 }_{   -0.00023 }$&$ 0.56  ^{+ 0.16  }_{ -0.23 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.10  ^{+ 0.37  }_{ -0.10 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 1.56  \pm{ 0.19  }$&$ 88.66 ^{+ 0.62  }_{ -0.54 }$&$ 24.6  ^{+ 2.2   }_{ -1.7  }$&$ 0.162  \pm{ 0.006  }$&$ 837   \pm{ 42    }$&$ 127   \pm{ 5     }$& 5.9   & 1.4  &0.200&0.926\\
K00262.01  & 11807274   & 172.6319  &$    7.81251 ^{+    0.00016 }_{   -0.00011 }$&$ 0.76  ^{+ 0.10  }_{ -0.04 }$&$ 0.009  ^{+ 0.001  }_{ -0.000 }$&$ 0.09  ^{+ 0.26  }_{ -0.09 }$&$ 0.25  ^{+ 0.59  }_{ -0.25 }$&$ 2.08  \pm{ 0.23  }$&$ 84.82 ^{+ 0.67  }_{ -1.14 }$&$ 8.7   ^{+ 0.8   }_{ -0.6  }$&$ 0.082  \pm{ 0.002  }$&$ 1388  \pm{ 69    }$&$ 90    \pm{ 3     }$& 4.8   & 0.6  &0.316&0.920\\
K00262.02  & 11807274   & 136.9686  &$    9.37614 ^{+    0.00023 }_{   -0.00016 }$&$ 0.94  ^{+ 0.04  }_{ -0.00 }$&$ 0.015  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+ 0.70  }_{ -0.00 }$&$ 3.52  \pm{ 0.41  }$&$ 83.55 ^{+ 0.36  }_{ -0.81 }$&$ 9.2   ^{+ 1.0   }_{ -0.8  }$&$ 0.092  \pm{ 0.003  }$&$ 1388  \pm{ 68    }$&$ 94    \pm{ 4     }$& 3.2   & 1.1  &0.397&0.943\\
K00270.01  & 6528464    & 175.0152  &$   12.58250 ^{+    0.00011 }_{   -0.00013 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.009  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 1.50  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -0.92 }$&$ 14.6  ^{+ 1.3   }_{ -1.0  }$&$ 0.104  \pm{ 0.002  }$&$ 965   \pm{ 51    }$&$ 108   \pm{ 5     }$& 6.6   & 2.1  &0.208&0.868\\
K00270.02  & 6528464    & 162.0396  &$   33.67312 ^{+    0.00039 }_{   -0.00022 }$&$ 0.45  ^{+ 0.16  }_{ -0.45 }$&$ 0.012  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.55  }_{ -0.00 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 1.96  \pm{ 0.20  }$&$ 89.07 ^{+ 0.93  }_{ -0.41 }$&$ 28.2  ^{+ 2.2   }_{ -2.4  }$&$ 0.200  \pm{ 0.004  }$&$ 700   \pm{ 36    }$&$ 165   \pm{ 10    }$& 8.4   & 1.1  &0.185&0.851\\
K00271.01  & 9451706    & 172.5460  &$   48.63057 ^{+    0.00016 }_{   -0.00014 }$&$ 0.51  ^{+ 0.13  }_{ -0.44 }$&$ 0.018  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 2.44  \pm{ 0.26  }$&$ 89.37 ^{+ 0.54  }_{ -0.24 }$&$ 47.0  ^{+ 3.6   }_{ -4.4  }$&$ 0.274  \pm{ 0.011  }$&$ 599   \pm{ 32    }$&$ 358   \pm{ 13    }$& 6.9   &\textbf{ 3.7  }&0.581&0.986\\
K00271.02  & 9451706    & 209.0731  &$   29.39241 ^{+    0.00009 }_{   -0.00013 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.016  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.48  ^{+  0.33 }_{ -0.48 }$&$ 2.20  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -0.76 }$&$ 32.9  ^{+ 2.3   }_{ -2.4  }$&$ 0.196  \pm{ 0.007  }$&$ 719   \pm{ 34    }$&$ 316   \pm{ 10    }$& 7.0   &\textbf{ 3.4  }&0.656&0.990\\
K00271.03  & 9451706    & 141.5109  &$   14.43593 ^{+    0.00034 }_{   -0.00039 }$&$ 0.13  ^{+ 0.66  }_{ -0.13 }$&$ 0.010  ^{+ 0.000  }_{ -0.002 }$&$ 0.49  ^{+ 0.22  }_{ -0.31 }$&$ 1.10  ^{+ 2.42  }_{ -1.10 }$&$ 1.31  \pm{ 0.21  }$&$ 89.65 ^{+ 0.35  }_{ -1.94 }$&$ 21.1  ^{+ 1.8   }_{ -1.9  }$&$ 0.122  \pm{ 0.005  }$&$ 892   \pm{ 56    }$&$ 105   \pm{ 6     }$& 3.2   &\textbf{ 3.0  }&0.235&0.939\\
K00274.01  & 8077137    & 175.9276  &$   15.09205 ^{+    0.00088 }_{   -0.00060 }$&$ 0.13  ^{+ 0.48  }_{ -0.13 }$&$ 0.004  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.02  ^{+ 0.28  }_{ -0.02 }$&$ 0.77  \pm{ 0.13  }$&$ 89.57 ^{+ 0.43  }_{ -1.58 }$&$ 17.1  ^{+ 1.7   }_{ -1.4  }$&$ 0.127  \pm{ 0.004  }$&$ 970   \pm{ 64    }$&$ 24    \pm{ 6     }$& 6.6   & 0.7  &0.029&0.426\\
K00274.02  & 8077137    & 153.4920  &$   22.79519 ^{+    0.00089 }_{   -0.00132 }$&$ 0.48  ^{+ 0.27  }_{ -0.40 }$&$ 0.003  ^{+ 0.002  }_{ -0.000 }$&$ 0.07  ^{+ 0.29  }_{ -0.07 }$&$ 0.29  ^{+ 1.31  }_{ -0.29 }$&$ 0.58  \pm{ 0.23  }$&$ 88.80 ^{+ 1.01  }_{ -0.69 }$&$ 22.4  ^{+ 2.2   }_{ -1.6  }$&$ 0.167  \pm{ 0.005  }$&$ 843   \pm{ 54    }$&$ 18    \pm{ 8     }$& 6.6   & 0.6  &0.025&0.390\\
K00275.01  & 10586004   & 176.8205  &$   15.79186 ^{+    0.00011 }_{   -0.00009 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 2.10  \pm{ 0.24  }$&$ 90.00 ^{+ 0.00  }_{ -0.67 }$&$ 18.9  ^{+ 1.9   }_{ -1.5  }$&$ 0.129  \pm{ 0.004  }$&$ 909   \pm{ 47    }$&$ 206   \pm{ 9     }$& 6.8   & 0.6  &0.352&0.931\\
K00275.02  & 10586004   & 208.7874  &$   82.19970 ^{+    0.00024 }_{   -0.00026 }$&$ 0.18  ^{+ 0.34  }_{ -0.18 }$&$ 0.014  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 2.05  \pm{ 0.24  }$&$ 89.82 ^{+ 0.18  }_{ -0.36 }$&$ 59.6  ^{+ 5.1   }_{ -4.4  }$&$ 0.384  \pm{ 0.013  }$&$ 499   \pm{ 28    }$&$ 221   \pm{ 21    }$& 10.4  & 0.4  &0.145&0.810\\
K00277.01  & 11401755   & 171.6976  &$   16.23069 ^{+    0.00004 }_{   -0.00004 }$&$ 0.51  ^{+ 0.07  }_{ -0.01 }$&$ 0.044  ^{+  0.005 }_{ -0.010 }$&$ 0.90  ^{+ 0.00  }_{ -0.02 }$&$ 4.71  ^{+ 0.10  }_{ -0.17 }$&$ 8.26  \pm{ 0.91  }$&$ 88.13 ^{+ 0.23  }_{ -0.41 }$&$ 16.2  ^{+ 1.2   }_{ -1.3  }$&$ 0.129  \pm{ 0.003  }$&$ 999   \pm{ 55    }$&$ 467   \pm{ 10    }$& 13.0  & 0.4  &0.663&0.980\\
K00277.02  & 11401755   & 141.6820  &$   13.84943 ^{+    0.00048 }_{   -0.00061 }$&$ 0.61  ^{+ 0.72  }_{ -0.61 }$&$ 0.007  ^{+ 0.005  }_{ -0.002 }$&$ 0.00  ^{+ 0.68  }_{ -0.00 }$&$ 0.00  ^{+ 3.89  }_{ -0.08 }$&$ 1.36  \pm{ 0.60  }$&$ 87.66 ^{+ 2.34  }_{ -2.60 }$&$ 15.1  ^{+ 1.3   }_{ -1.3  }$&$ 0.116  \pm{ 0.003  }$&$ 1024  \pm{ 63    }$&$ 57    \pm{ 8     }$& 5.6   & 0.3  &0.022&0.356\\
K00279.01  & 12314973   & 176.7045  &$   28.45499 ^{+    0.00003 }_{   -0.00003 }$&$ 0.56  ^{+ 0.21  }_{ -0.25 }$&$ 0.035  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 1.29  }_{ -0.00 }$&$ 7.18  \pm{ 1.37  }$&$ 88.59 ^{+ 0.76  }_{ -1.06 }$&$ 23.1  ^{+ 3.4   }_{ -4.1  }$&$ 0.200  \pm{ 0.008  }$&$ 893   \pm{ 86    }$&$ 1406  \pm{ 14    }$& 8.3   & 0.5  &0.733&0.993\\
K00279.02  & 12314973   & 136.9443  &$   15.41299 ^{+    0.00012 }_{   -0.00011 }$&$ 0.59  ^{+ 0.10  }_{ -0.07 }$&$ 0.019  ^{+  0.000 }_{ -0.004 }$&$ 0.65  ^{+ 0.13  }_{ -0.56 }$&$ 4.47  ^{+ 0.35  }_{ -3.37 }$&$ 3.93  \pm{ 1.08  }$&$ 87.57 ^{+ 0.91  }_{ -1.49 }$&$ 15.1  ^{+ 4.1   }_{ -2.9  }$&$ 0.132  \pm{ 0.005  }$&$ 1142  \pm{ 169   }$&$ 283   \pm{ 10    }$& 7.4   & 0.1  &0.334&0.962\\
K00279.03  & 12314973   & 136.1570  &$    7.51465 ^{+    0.00029 }_{   -0.00027 }$&$ 0.09  ^{+ 0.34  }_{ -0.09 }$&$ 0.006  ^{+  0.000 }_{ -0.002 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.99  \pm{ 0.30  }$&$ 89.56 ^{+ 0.44  }_{ -1.80 }$&$ 11.5  ^{+ 3.5   }_{ -2.3  }$&$ 0.077  \pm{ 0.006  }$&$ 1216  \pm{ 187   }$&$ 45    \pm{ 5     }$& 4.7   & 0.5  &0.018&0.483\\
\textbf{K00282.01}  & 5088536    & 182.1039  &$   27.50868 ^{+    0.00006 }_{   -0.00007 }$&$ 0.38  ^{+ 0.14  }_{ -0.38 }$&$ 0.023  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 2.90  \pm{ 0.25  }$&$ 89.34 ^{+ 0.66  }_{ -0.31 }$&$ 32.6  ^{+ 2.5   }_{ -2.4  }$&$ 0.178  \pm{ 0.005  }$&$ 683   \pm{ 29    }$&$ 640   \pm{ 9     }$& 6.1   & 1.1  &0.860&\textbf{0.997}\\
K00282.02  & 5088536    & 139.0684  &$    8.45742 ^{+    0.00026 }_{   -0.00023 }$&$ 0.00  ^{+ 0.58  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.44  ^{+ 0.08  }_{ -0.44 }$&$ 0.09  ^{+ 0.16  }_{ -0.09 }$&$ 0.92  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -2.14 }$&$ 15.3  ^{+ 1.3   }_{ -1.1  }$&$ 0.081  \pm{ 0.003  }$&$ 988   \pm{ 55    }$&$ 79    \pm{ 4     }$& 3.6   & 0.4  &0.034&0.635\\
K00282.03  & 5088536    & 201.1697  &$   87.51870 ^{+    0.02042 }_{   -0.02048 }$&$ 0.92  ^{+ 0.80  }_{ -0.52 }$&$ 0.016  ^{+ 0.005  }_{ -0.011 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 1.99  \pm{ 0.98  }$&$ 89.28 ^{+ 0.40  }_{ -0.62 }$&$ 72.0  ^{+ 6.8   }_{ -5.1  }$&$ 0.385  \pm{ 0.012  }$&$ 455   \pm{ 29    }$&$ 111   \pm{ 16    }$& 3.9   & 0.0  &0.009&0.313\\
K00283.01  & 5695396    & 170.5985  &$   16.09194 ^{+    0.00007 }_{   -0.00006 }$&$ 0.76  ^{+ 0.06  }_{ -0.27 }$&$ 0.021  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 0.00  ^{+ 0.74  }_{ -0.00 }$&$ 2.32  \pm{ 0.30  }$&$ 88.32 ^{+ 0.72  }_{ -0.29 }$&$ 25.9  ^{+ 2.1   }_{ -2.1  }$&$ 0.125  \pm{ 0.004  }$&$ 740   \pm{ 42    }$&$ 444   \pm{ 6     }$& 3.2   &\textbf{ 6.1  }&0.890&0.995\\
K00283.02  & 5695396    & 154.4205  &$   25.51704 ^{+    0.00122 }_{   -0.00089 }$&$ 0.22  ^{+ 0.38  }_{ -0.22 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.81  \pm{ 0.13  }$&$ 89.64 ^{+ 0.36  }_{ -0.63 }$&$ 35.0  ^{+ 3.2   }_{ -3.0  }$&$ 0.170  \pm{ 0.006  }$&$ 638   \pm{ 38    }$&$ 69    \pm{ 8     }$& 5.5   & 0.9  &0.019&0.323\\
K00284.01  & 6021275    & 179.4253  &$   18.00999 ^{+    0.00036 }_{   -0.00034 }$&$ 0.75  ^{+ 0.25  }_{ -0.75 }$&$ 0.016  ^{+ 0.000  }_{ -0.005 }$&$ 0.68  ^{+ 0.21  }_{ -0.09 }$&$ 4.12  ^{+ 0.23  }_{ -0.75 }$&$ 1.88  \pm{ 0.38  }$&$ 88.44 ^{+ 1.56  }_{ -0.60 }$&$ 27.0  ^{+ 2.6   }_{ -2.4  }$&$ 0.136  \pm{ 0.005  }$&$ 750   \pm{ 44    }$&$ 181   \pm{ 8     }$& 3.7   & 1.2  &0.197&0.925\\
K00284.02  & 6021275    & 169.6420  &$    6.41483 ^{+    0.00014 }_{   -0.00013 }$&$ 0.72  ^{+  0.28 }_{ -0.72 }$&$ 0.011  ^{+  0.001 }_{ -0.003 }$&$ 0.77  ^{+  0.23 }_{ -0.77 }$&$ 4.12  ^{+ 0.90  }_{ -4.12 }$&$ 1.33  \pm{ 0.15  }$&$ 87.00 ^{+ 3.00  }_{ -1.33 }$&$ 13.5  ^{+ 1.2   }_{ -1.0  }$&$ 0.068  \pm{ 0.003  }$&$ 1061  \pm{ 58    }$&$ 120   \pm{ 5     }$& 3.8   & 1.4  &0.083&0.820\\
K00284.03  & 6021275    & 168.8602  &$    6.17818 ^{+    0.00013 }_{   -0.00013 }$&$ 0.15  ^{+ 0.21  }_{ -0.15 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 1.02  \pm{ 0.13  }$&$ 89.34 ^{+ 0.66  }_{ -0.96 }$&$ 13.3  ^{+ 1.0   }_{ -1.1  }$&$ 0.067  \pm{ 0.003  }$&$ 1080  \pm{ 58    }$&$ 103   \pm{ 5     }$& 3.5   & 1.0  &0.071&0.792\\
K00284.04  & 6021275    & 239.1980  &$  110.29290 ^{+    0.14011 }_{   -0.07637 }$&$ 1.12  ^{+ 0.99  }_{ -0.66 }$&$ 0.011  ^{+ 0.013  }_{ -0.004 }$&$ 0.86  ^{+ 0.04  }_{ -0.04 }$&$ 4.01  ^{+ 0.29  }_{ -0.58 }$&$ 1.30  \pm{ 1.04  }$&$ 89.30 ^{+ 0.42  }_{ -0.63 }$&$ 90.0  ^{+ 8.2   }_{ -6.1  }$&$ 0.454  \pm{ 0.019  }$&$ 411   \pm{ 23    }$&$ 82    \pm{ 25    }$& 7.4   & 0.8  &0.103&0.851\\
K00285.01  & 6196457    & 179.2804  &$   13.74878 ^{+    0.00005 }_{   -0.00005 }$&$ 0.59  ^{+ 0.08  }_{ -0.02 }$&$ 0.022  ^{+ 0.000  }_{ -0.001 }$&$ 0.48  ^{+ 0.17  }_{ -0.12 }$&$ 4.47  ^{+ 0.69  }_{ -0.33 }$&$ 3.95  \pm{ 0.38  }$&$ 87.82 ^{+ 0.31  }_{ -0.53 }$&$ 15.8  ^{+ 1.5   }_{ -1.1  }$&$ 0.118  \pm{ 0.003  }$&$ 990   \pm{ 58    }$&$ 419   \pm{ 7     }$& 6.3   & 1.0  &0.830&0.996\\
K00285.02  & 6196457    & 147.9103  &$   26.72428 ^{+    0.00022 }_{   -0.00024 }$&$ 0.52  ^{+ 0.10  }_{ -0.26 }$&$ 0.016  ^{+ 0.002  }_{ -0.004 }$&$ 0.87  ^{+ 0.03  }_{ -0.66 }$&$ 4.67  ^{+ 0.38  }_{ -0.77 }$&$ 2.79  \pm{ 0.55  }$&$ 88.80 ^{+ 0.59  }_{ -0.30 }$&$ 24.9  ^{+ 2.7   }_{ -1.9  }$&$ 0.183  \pm{ 0.006  }$&$ 784   \pm{ 48    }$&$ 193   \pm{ 11    }$& 9.9   & 0.5  &0.391&0.970\\
K00285.03  & 6196457    & 134.2716  &$   49.35899 ^{+    0.00071 }_{   -0.00089 }$&$ 0.52  ^{+ 0.39  }_{ -0.50 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.00  ^{+ 3.79  }_{ -0.00 }$&$ 1.96  \pm{ 0.26  }$&$ 89.20 ^{+ 0.77  }_{ -0.65 }$&$ 37.4  ^{+ 3.8   }_{ -2.9  }$&$ 0.275  \pm{ 0.008  }$&$ 640   \pm{ 39    }$&$ 129   \pm{ 16    }$& 8.8   & 0.5  &0.070&0.789\\
K00289.01  & 10386922   & 138.7360  &$   26.62940 ^{+    0.00217 }_{   -0.00258 }$&$ 0.65  ^{+ 0.20  }_{ -0.56 }$&$ 0.021  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 0.72  }_{ -0.00 }$&$ 4.51  \pm{ 1.64  }$&$ 88.19 ^{+ 1.61  }_{ -1.62 }$&$ 19.9  ^{+ 4.6   }_{ -6.2  }$&$ 0.185  \pm{ 0.017  }$&$ 854   \pm{ 139   }$&$ 482   \pm{ 16    }$& 7.8   & 0.1  &0.508&0.963\\
K00289.02  & 10386922   & 403.6729  &$  296.63709 ^{+    0.00057 }_{   -0.00042 }$&$ 0.65  ^{+ 0.22  }_{ -0.61 }$&$ 0.051  ^{+ 0.003  }_{ -0.005 }$&$ 0.09  ^{+ 0.35  }_{ -0.09 }$&$ 1.65  ^{+ 0.76  }_{ -1.65 }$&$ 9.86  \pm{ 3.07  }$&$ 89.66 ^{+ 0.32  }_{ -0.33 }$&$ 113.5 ^{+ 20.3  }_{ -34.9 }$&$ 0.908  \pm{ 0.062  }$&$ 366   \pm{ 59    }$&$ 2838  \pm{ 67    }$& 16.2  & 0.1  &0.397&0.943\\
K00291.01  & 10933561   & 185.1521  &$   31.51789 ^{+    0.00044 }_{   -0.00028 }$&$ 0.40  ^{+ 0.17  }_{ -0.40 }$&$ 0.017  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 2.60  \pm{ 0.30  }$&$ 89.21 ^{+ 0.79  }_{ -0.37 }$&$ 30.1  ^{+ 2.6   }_{ -2.7  }$&$ 0.194  \pm{ 0.005  }$&$ 688   \pm{ 41    }$&$ 361   \pm{ 20    }$& 7.7   & 0.5  &0.121&0.775\\
K00291.02  & 10933561   & 134.1052  &$    8.12986 ^{+    0.00017 }_{   -0.00014 }$&$ 0.90  ^{+ 0.06  }_{ -0.02 }$&$ 0.015  ^{+ 0.002  }_{ -0.001 }$&$ 0.09  ^{+ 0.09  }_{ -0.09 }$&$ 0.04  ^{+ 0.97  }_{ -0.04 }$&$ 2.32  \pm{ 0.31  }$&$ 85.40 ^{+ 0.46  }_{ -0.70 }$&$ 11.7  ^{+ 1.1   }_{ -0.8  }$&$ 0.079  \pm{ 0.002  }$&$ 1107  \pm{ 58    }$&$ 138   \pm{ 9     }$& 2.7   & 1.1  &0.119&0.772\\
K00295.01  & 11547513   & 171.8763  &$    5.31743 ^{+    0.00006 }_{   -0.00006 }$&$ 0.94  ^{+ 0.01  }_{ -0.05 }$&$ 0.020  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.52  }_{ -0.00 }$&$ 6.23  \pm{ 1.47  }$&$ 78.93 ^{+ 2.69  }_{ -1.83 }$&$ 5.0   ^{+ 1.1   }_{ -0.8  }$&$ 0.064  \pm{ 0.009  }$&$ 1811  \pm{ 216   }$&$ 288   \pm{ 6     }$& 3.3   & 1.3  &0.678&0.981\\
K00295.02  & 11547513   & 135.5088  &$   10.10575 ^{+    0.00032 }_{   -0.00030 }$&$ 0.98  ^{+ 0.01  }_{ -0.03 }$&$ 0.012  ^{+ 0.007  }_{ -0.001 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.66  }_{ -0.00 }$&$ 3.00  \pm{ 1.15  }$&$ 83.90 ^{+ 0.95  }_{ -1.03 }$&$ 9.1   ^{+ 1.6   }_{ -1.8  }$&$ 0.096  \pm{ 0.010  }$&$ 1298  \pm{ 156   }$&$ 113   \pm{ 8     }$& 2.3   & 0.7  &0.124&0.779\\
K00298.01  & 12785320   & 178.3053  &$   19.96000 ^{+    0.00079 }_{   -0.00087 }$&$ 0.93  ^{+ 0.50  }_{ -0.82 }$&$ 0.008  ^{+ 0.006  }_{ -0.006 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.20  ^{+ 0.34  }_{ -0.20 }$&$ 1.00  \pm{ 0.96  }$&$ 85.10 ^{+ 4.67  }_{ -2.90 }$&$ 26.3  ^{+ 15.2  }_{ -10.1 }$&$ 0.143  \pm{ 0.010  }$&$ 1101  \pm{ 1394  }$&$ 81     \pm{ 17    }$& 5.4   & 0.2  &0.039&0.505\\
K00298.02  & 12785320   & 170.7233  &$   57.38425 ^{+    0.00707 }_{   -0.00016 }$&$ 0.67  ^{+ 0.18  }_{ -0.67 }$&$ 0.014  ^{+ 0.004  }_{ -0.003 }$&$ 0.00  ^{+ 0.59  }_{ -0.00 }$&$ 0.00  ^{+ 4.47  }_{ -0.00 }$&$ 1.71  \pm{ 0.99  }$&$ 89.40 ^{+ 0.60  }_{ -0.61 }$&$ 54.0  ^{+ 27.3  }_{ -20.5 }$&$ 0.289  \pm{ 0.019  }$&$ 455   \pm{ 122   }$&$ 237   \pm{ 27    }$& 5.2   & 0.7  &0.025&0.386\\
K00301.01  & 3642289    & 171.7134  &$    6.00255 ^{+    0.00006 }_{   -0.00009 }$&$ 0.30  ^{+ 0.11  }_{ -0.30 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.00  ^{+ 1.15  }_{ -0.00 }$&$ 1.96  \pm{ 0.33  }$&$ 88.34 ^{+ 1.66  }_{ -0.82 }$&$ 10.4  ^{+ 1.2   }_{ -1.5  }$&$ 0.071  \pm{ 0.003  }$&$ 1296  \pm{ 96    }$&$ 199   \pm{ 6     }$& 4.2   & 0.9  &0.135&0.797\\
K00301.02  & 3642289    & 141.3742  &$   11.44883 ^{+    0.00049 }_{   -0.00048 }$&$ 0.20  ^{+ 0.36  }_{ -0.20 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 1.23  \pm{ 0.35  }$&$ 89.29 ^{+ 0.71  }_{ -1.36 }$&$ 15.7  ^{+ 4.2   }_{ -3.1  }$&$ 0.109  \pm{ 0.005  }$&$ 1040  \pm{ 141   }$&$ 79    \pm{ 9     }$& 5.3   & 0.3  &0.016&0.291\\
K00304.01  & 6029239    & 174.9087  &$    8.51205 ^{+    0.00005 }_{   -0.00005 }$&$ 0.95  ^{+ 0.35  }_{ -0.07 }$&$ 0.027  ^{+ 0.003  }_{ -0.004 }$&$ 0.08  ^{+ 0.31  }_{ -0.08 }$&$ 0.00  ^{+ 1.49  }_{ -0.00 }$&$ 6.02  \pm{ 1.73  }$&$ 84.54 ^{+ 1.39  }_{ -6.28 }$&$ 9.2   ^{+ 2.3   }_{ -2.1  }$&$ 0.086  \pm{ 0.003  }$&$ 1291  \pm{ 177   }$&$ 588   \pm{ 7     }$& 2.6   & 1.1  &0.465&0.956\\
K00304.02  & 6029239    & 136.5633  &$    5.51835 ^{+    0.00019 }_{   -0.00022 }$&$ 0.85  ^{+ 0.22  }_{ -0.33 }$&$ 0.006  ^{+ 0.000  }_{ -0.003 }$&$ 0.24  ^{+  0.08 }_{ -0.24 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 1.41  \pm{ 0.47  }$&$ 83.05 ^{+ 2.84  }_{ -1.54 }$&$ 6.7   ^{+ 1.8   }_{ -1.4  }$&$ 0.064  \pm{ 0.002  }$&$ 1535  \pm{ 241   }$&$ 34    \pm{ 6     }$& 3.5   & 0.3  &0.020&0.341\\
K00307.01  & 6289257    & 176.2694  &$   19.67423 ^{+    0.00043 }_{   -0.00036 }$&$ 0.60  ^{+ 0.15  }_{ -0.59 }$&$ 0.013  ^{+ 0.002  }_{ -0.001 }$&$ 0.27  ^{+ 0.31  }_{ -0.27 }$&$ 0.38  ^{+ 3.11  }_{ -0.38 }$&$ 1.56  \pm{ 0.22  }$&$ 88.78 ^{+ 1.19  }_{ -0.40 }$&$ 28.1  ^{+ 2.7   }_{ -2.1  }$&$ 0.147  \pm{ 0.006  }$&$ 765   \pm{ 42    }$&$ 221   \pm{ 11    }$& 4.1   & 1.9  &0.079&0.681\\
K00307.02  & 6289257    & 131.5367  &$    5.21106 ^{+    0.00015 }_{   -0.00012 }$&$ 0.44  ^{+ 0.13  }_{ -0.44 }$&$ 0.009  ^{+ 0.007  }_{ -0.000 }$&$ 0.43  ^{+ 0.46  }_{ -0.43 }$&$ 3.66  ^{+ 1.14  }_{ -3.66 }$&$ 1.09  \pm{ 0.44  }$&$ 87.79 ^{+ 2.21  }_{ -0.89 }$&$ 11.7  ^{+ 1.0   }_{ -1.0  }$&$ 0.061  \pm{ 0.003  }$&$ 1201  \pm{ 71    }$&$ 103   \pm{ 5     }$& 3.6   & 2.0  &0.023&0.371\\
K00312.01  & 7050989    & 175.5857  &$   11.57894 ^{+    0.00019 }_{   -0.00010 }$&$ 0.63  ^{+ 0.13  }_{ -0.19 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.05  ^{+ 0.43  }_{ -0.05 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.78  \pm{ 0.26  }$&$ 88.15 ^{+ 0.65  }_{ -0.55 }$&$ 18.9  ^{+ 1.8   }_{ -1.4  }$&$ 0.106  \pm{ 0.004  }$&$ 924   \pm{ 53    }$&$ 236   \pm{ 8     }$& 3.6   & 0.4  &0.065&0.636\\
K00312.02  & 7050989    & 131.9683  &$   16.39922 ^{+    0.00015 }_{   -0.00010 }$&$ 0.01  ^{+ 0.64  }_{ -0.01 }$&$ 0.013  ^{+ 0.003  }_{ -0.002 }$&$ 0.72  ^{+  0.08 }_{ -0.61 }$&$ 6.28  ^{+  0.00 }_{ -6.22 }$&$ 1.76  \pm{ 0.34  }$&$ 89.97 ^{+ 0.03  }_{ -1.66 }$&$ 23.8  ^{+ 2.1   }_{ -1.9  }$&$ 0.134  \pm{ 0.005  }$&$ 832   \pm{ 51    }$&$ 224   \pm{ 10    }$& 3.6   & 0.5  &0.053&0.584\\
K00313.01  & 7419318    & 177.6356  &$   18.73572 ^{+    0.00015 }_{   -0.00018 }$&$ 0.63  ^{+ 0.09  }_{ -0.26 }$&$ 0.022  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.00  ^{+ 0.87  }_{ -0.00 }$&$ 2.11  \pm{ 0.26  }$&$ 88.91 ^{+ 0.51  }_{ -0.25 }$&$ 32.8  ^{+ 2.8   }_{ -2.4  }$&$ 0.134  \pm{ 0.004  }$&$ 616   \pm{ 32    }$&$ 604   \pm{ 15    }$& 3.4   & 1.0  &0.542&0.967\\
K00313.02  & 7419318    & 179.8861  &$    8.43640 ^{+    0.00010 }_{   -0.00011 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.54  \pm{ 0.15  }$&$ 90.00 ^{+ 0.00  }_{ -0.72 }$&$ 18.9  ^{+ 1.4   }_{ -1.4  }$&$ 0.079  \pm{ 0.003  }$&$ 814   \pm{ 35    }$&$ 350   \pm{ 10    }$& 3.4   & 0.3  &0.369&0.936\\
K00314.01  & 7603200    & 177.8521  &$   13.78105 ^{+    0.00010 }_{   -0.00008 }$&$ 1.14  ^{+ 0.29  }_{ -0.30 }$&$ 0.032  ^{+ 0.001  }_{ -0.010 }$&$ 0.19  ^{+ 0.25  }_{ -0.17 }$&$ 1.04  ^{+ 2.41  }_{ -1.01 }$&$ 6.06  \pm{ 3.45  }$&$ 85.13 ^{+ 2.88  }_{ -2.80 }$&$ 13.2  ^{+ 12.7  }_{ -3.4  }$&$ 0.105  \pm{ 0.013  }$&$ 713   \pm{ 210   }$&$ 729   \pm{ 10    }$& 2.7   & 0.4  &0.797&0.995\\
K00314.02  & 7603200    & 171.0047  &$   23.08945 ^{+    0.00017 }_{   -0.00018 }$&$ 0.87  ^{+ 0.14  }_{ -0.24 }$&$ 0.027  ^{+ 0.011  }_{ -0.005 }$&$ 0.01  ^{+ 0.58  }_{ -0.01 }$&$ 4.67  ^{+  0.76 }_{ -4.67 }$&$ 2.50  \pm{ 1.35  }$&$ 88.67 ^{+ 0.71  }_{ -0.92 }$&$ 33.8  ^{+ 18.0  }_{ -10.4 }$&$ 0.134  \pm{ 0.011  }$&$ 428   \pm{ 107   }$&$ 498   \pm{ 16    }$& 2.5   &\textbf{ 4.3  }&0.699&0.991\\
K00314.03  & 7603200    & 133.5522  &$   10.31202 ^{+    0.00022 }_{   -0.00028 }$&$ 0.76  ^{+ 0.41  }_{ -0.36 }$&$ 0.008  ^{+ 0.000  }_{ -0.004 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.70  \pm{ 0.46  }$&$ 88.02 ^{+ 0.91  }_{ -0.91 }$&$ 19.7  ^{+ 10.3  }_{ -7.7  }$&$ 0.079  \pm{ 0.007  }$&$ 552   \pm{ 173   }$&$ 57    \pm{ 9     }$& 2.3   & 0.5  &0.040&0.678\\
K00316.01  & 8008067    & 137.5880  &$   15.77120 ^{+    0.00125 }_{   -0.00011 }$&$ 0.86  ^{+ 0.09  }_{ -0.37 }$&$ 0.024  ^{+ 0.002  }_{ -0.003 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 1.59  }_{ -0.00 }$&$ 6.43  \pm{ 2.24  }$&$ 85.99 ^{+ 2.69  }_{ -2.03 }$&$ 11.5  ^{+ 6.1   }_{ -2.7  }$&$ 0.129  \pm{ 0.005  }$&$ 1061  \pm{ 205   }$&$ 534   \pm{ 13    }$& 5.4   &\textbf{ 11.7 }&0.408&0.972\\
K00316.02  & 8008067    & 481.2644  &$  157.07021 ^{+    0.00048 }_{   -0.00129 }$&$ 0.92  ^{+ 0.04  }_{ -0.33 }$&$ 0.026  ^{+ 0.018  }_{ -0.006 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 4.59  }_{ -0.00 }$&$ 6.35  \pm{ 4.04  }$&$ 89.16 ^{+ 0.51  }_{ -0.49 }$&$ 59.0  ^{+ 41.3  }_{ -18.4 }$&$ 0.597  \pm{ 0.025  }$&$ 472   \pm{ 119   }$&$ 537   \pm{ 41    }$& 8.7   & 2.6  &0.173&0.913\\
K00316.03  & 8008067    & 131.7801  &$    7.30569 ^{+    0.00008 }_{   -0.00009 }$&$ 0.96  ^{+ 0.01  }_{ -0.06 }$&$ 0.026  ^{+ 0.004  }_{ -0.006 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 5.00  \pm{ 1.70  }$&$ 84.48 ^{+ 1.68  }_{ -1.52 }$&$ 9.3   ^{+ 3.4   }_{ -1.7  }$&$ 0.077  \pm{ 0.003  }$&$ 1186  \pm{ 166   }$&$ 254   \pm{ 8     }$& 2.1   &\textbf{ 8.3  }&0.241&0.941\\
K00321.01  & 8753657    & 170.4543  &$    2.42631 ^{+    0.00002 }_{   -0.00002 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 4.00  }_{ -0.00 }$&$ 1.37  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -3.31 }$&$ 6.6   ^{+ 0.4   }_{ -0.4  }$&$ 0.034  \pm{ 0.001  }$&$ 1434  \pm{ 57    }$&$ 193   \pm{ 3     }$& 2.9   & 0.7  &0.451&0.954\\
K00321.02  & 8753657    & 132.3660  &$    4.62339 ^{+    0.00009 }_{   -0.00009 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.37  ^{+ 0.08  }_{ -0.37 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.82  \pm{ 0.11  }$&$ 90.00 ^{+  0.00 }_{ -2.87 }$&$ 10.5  ^{+ 0.8   }_{ -0.9  }$&$ 0.053  \pm{ 0.002  }$&$ 1134  \pm{ 61    }$&$ 63    \pm{ 5     }$& 3.1   & 0.5  &0.024&0.377\\
K00326.01  & 9880467    & 171.0311  &$    8.97350 ^{+    0.00010 }_{   -0.00016 }$&$ 2.77  ^{+ 0.03  }_{ -1.22 }$&$ 0.031  ^{+ 0.006  }_{ -0.000 }$&$ 0.72  ^{+ 0.04  }_{ -0.09 }$&$ 1.80  ^{+  0.13 }_{ -1.57 }$&$ 13.90 \pm{ 1.49  }$&$ 60.00 ^{+ 13.81 }_{ -0.00 }$&$ 5.5   ^{+ 0.1   }_{ -0.0  }$&$ 0.106  \pm{ 0.002  }$&$ 1340  \pm{ 17    }$&$ 959   \pm{ 34    }$& 3.7   &\textbf{ 9.5  }&0.855&0.993\\
K00326.02  & 9880467    & 151.2420  &$  108.52770 ^{+    0.00080 }_{   -0.00176 }$&$ 0.95  ^{+ 0.21  }_{ -0.32 }$&$ 0.041  ^{+  0.002 }_{ -0.023 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.00  ^{+ 1.52  }_{ -0.00 }$&$ 18.62 \pm{ 4.93  }$&$ 88.14 ^{+ 0.64  }_{ -0.40 }$&$ 29.1  ^{+ 0.3   }_{ -0.3  }$&$ 0.557  \pm{ 0.011  }$&$ 583   \pm{ 7     }$&$ 743   \pm{ 128   }$& 12.4  & 1.4  &0.855&0.993\\
K00327.01  & 9881662    & 172.6615  &$    3.25428 ^{+    0.00005 }_{   -0.00005 }$&$ 0.11  ^{+ 0.35  }_{ -0.11 }$&$ 0.011  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 2.43  }_{ -0.00 }$&$ 1.43  \pm{ 0.17  }$&$ 89.21 ^{+ 0.79  }_{ -2.62 }$&$ 8.1   ^{+ 0.7   }_{ -0.7  }$&$ 0.045  \pm{ 0.002  }$&$ 1459  \pm{ 77    }$&$ 166   \pm{ 5     }$& 3.1   & 2.5  &0.434&0.950\\
K00327.02  & 9881662    & 189.6005  &$   91.35250 ^{+    0.00655 }_{   -0.00037 }$&$ 0.00  ^{+ 0.67  }_{ -0.00 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.51  ^{+ 0.19  }_{ -0.48 }$&$ 0.01  ^{+ 0.11  }_{ -0.01 }$&$ 1.76  \pm{ 0.24  }$&$ 90.00 ^{+ 0.00  }_{ -0.50 }$&$ 75.8  ^{+ 8.0   }_{ -5.8  }$&$ 0.420  \pm{ 0.015  }$&$ 470   \pm{ 31    }$&$ 190   \pm{ 30    }$& 7.8   & 0.9  &0.110&0.756\\
K00332.01  & 10290666   & 172.0875  &$    5.45851 ^{+    0.00006 }_{   -0.00006 }$&$ 0.01  ^{+ 0.31  }_{ -0.01 }$&$ 0.014  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 1.93  \pm{ 0.20  }$&$ 89.92 ^{+ 0.08  }_{ -1.76 }$&$ 10.6  ^{+ 0.8   }_{ -0.7  }$&$ 0.061  \pm{ 0.002  }$&$ 1175  \pm{ 50    }$&$ 269   \pm{ 8     }$& 4.0   & 0.8  &0.172&0.838\\
K00332.02  & 10290666   & 135.3520  &$    6.86687 ^{+    0.00023 }_{   -0.00026 }$&$ 0.61  ^{+ 0.19  }_{ -0.61 }$&$ 0.006  ^{+ 0.002  }_{ -0.002 }$&$ 0.60  ^{+ 0.27  }_{ -0.60 }$&$ 3.48  ^{+ 1.33  }_{ -3.48 }$&$ 0.80  \pm{ 0.23  }$&$ 87.40 ^{+ 2.60  }_{ -0.78 }$&$ 13.2  ^{+ 1.1   }_{ -1.1  }$&$ 0.070  \pm{ 0.003  }$&$ 1039  \pm{ 60    }$&$ 42    \pm{ 9     }$& 3.5   & 0.0  &0.022&0.363\\
K00338.01  & 10552611   & 174.5747  &$    7.01062 ^{+    0.00012 }_{   -0.00010 }$&$ 0.96  ^{+ 0.07  }_{ -0.05 }$&$ 0.020  ^{+ 0.007  }_{ -0.000 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.01  ^{+ 6.27  }_{ -0.01 }$&$ 6.15  \pm{ 1.16  }$&$ 79.62 ^{+ 0.75  }_{ -0.70 }$&$ 5.3   ^{+ 0.0   }_{ -0.0  }$&$ 0.070  \pm{ 0.001  }$&$ 1182  \pm{ 17    }$&$ 329   \pm{ 12    }$& 3.5   & 0.5  &0.068&0.646\\
K00338.02  & 10552611   & 132.6397  &$    3.10753 ^{+    0.00005 }_{   -0.00007 }$&$ 0.88  ^{+ 0.05  }_{ -0.13 }$&$ 0.009  ^{+ 0.002  }_{ -0.003 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 2.81  \pm{ 0.82  }$&$ 73.48 ^{+ 2.48  }_{ -0.85 }$&$ 3.1   ^{+ 0.0   }_{ -0.0  }$&$ 0.041  \pm{ 0.000  }$&$ 1549  \pm{ 22    }$&$ 51    \pm{ 8     }$& 3.9   & 1.1  &0.024&0.383\\
K00341.01  & 10878263   & 176.6658  &$   14.34123 ^{+    0.00020 }_{   -0.00024 }$&$ 0.65  ^{+ 0.06  }_{ -0.17 }$&$ 0.028  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 0.00  ^{+ 0.76  }_{ -0.00 }$&$ 2.91  \pm{ 0.34  }$&$ 88.57 ^{+ 0.45  }_{ -0.28 }$&$ 25.9  ^{+ 2.0   }_{ -1.9  }$&$ 0.114  \pm{ 0.004  }$&$ 717   \pm{ 35    }$&$ 936   \pm{ 33    }$& 3.3   & 0.3  &0.167&0.834\\
K00341.02  & 10878263   & 177.6153  &$    4.69961 ^{+    0.00010 }_{   -0.00005 }$&$ 0.21  ^{+ 0.24  }_{ -0.21 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 1.48  \pm{ 0.17  }$&$ 89.01 ^{+ 0.99  }_{ -1.19 }$&$ 12.3  ^{+ 1.0   }_{ -0.9  }$&$ 0.054  \pm{ 0.002  }$&$ 1044  \pm{ 52    }$&$ 279   \pm{ 20    }$& 2.9   & 2.2  &0.081&0.688\\
K00343.01  & 10982872   & 170.3356  &$    4.76170 ^{+    0.00004 }_{   -0.00003 }$&$ 0.33  ^{+ 0.24  }_{ -0.33 }$&$ 0.019  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.01  ^{+ 2.59  }_{ -0.01 }$&$ 2.47  \pm{ 0.28  }$&$ 88.08 ^{+ 1.92  }_{ -1.63 }$&$ 9.9   ^{+ 0.8   }_{ -0.9  }$&$ 0.054  \pm{ 0.002  }$&$ 1223  \pm{ 63    }$&$ 516   \pm{ 7     }$& 3.6   & 1.3  &0.721&0.992\\
K00343.02  & 10982872   & 170.4966  &$    2.02413 ^{+    0.00002 }_{   -0.00002 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.24  ^{+  0.01 }_{ -0.24 }$&$ 1.59  \pm{ 0.17  }$&$ 90.00 ^{+ 0.00  }_{ -5.26 }$&$ 5.7   ^{+ 0.4   }_{ -0.4  }$&$ 0.031  \pm{ 0.001  }$&$ 1609  \pm{ 77    }$&$ 247   \pm{ 5     }$& 2.8   & 1.3  &0.491&0.980\\
K00343.03  & 10982872   & 148.6985  &$   41.80925 ^{+    0.00011 }_{   -0.00012 }$&$ 0.07  ^{+ 0.43  }_{ -0.07 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.12  ^{+ 0.36  }_{ -0.12 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 1.65  \pm{ 0.21  }$&$ 89.91 ^{+ 0.09  }_{ -0.58 }$&$ 43.3  ^{+ 3.9   }_{ -2.9  }$&$ 0.231  \pm{ 0.008  }$&$ 575   \pm{ 28    }$&$ 206   \pm{ 26    }$& 7.2   & 0.8  &0.083&0.818\\
K00353.01  & 11566064   & 176.5297  &$  152.10452 ^{+    0.00030 }_{   -0.00019 }$&$ 0.94  ^{+ 0.47  }_{ -0.26 }$&$ 0.060  ^{+ 0.009  }_{ -0.000 }$&$ 0.37  ^{+ 0.43  }_{ -0.37 }$&$ 3.30  ^{+ 1.37  }_{ -1.46 }$&$ 9.84  \pm{ 2.71  }$&$ 89.44 ^{+ 0.26  }_{ -0.58 }$&$ 90.2  ^{+ 23.9  }_{ -20.4 }$&$ 0.637  \pm{ 0.027  }$&$ 465   \pm{ 77    }$&$ 3340  \pm{ 82    }$& 7.2   & 1.3  &0.647&0.979\\
K00353.02  & 11566064   & 135.0456  &$   30.65268 ^{+    0.00057 }_{   -0.00057 }$&$ 0.23  ^{+ 0.58  }_{ -0.23 }$&$ 0.014  ^{+ 0.005  }_{ -0.001 }$&$ 0.54  ^{+ 0.24  }_{ -0.48 }$&$ 2.95  ^{+ 1.53  }_{ -2.86 }$&$ 2.39  \pm{ 0.81  }$&$ 89.58 ^{+ 0.42  }_{ -1.47 }$&$ 30.6  ^{+ 8.1   }_{ -6.8  }$&$ 0.219  \pm{ 0.009  }$&$ 802   \pm{ 119   }$&$ 316   \pm{ 28    }$& 5.6   & 0.4  &0.112&0.760\\
K00354.01  & 11568987   & 171.5200  &$   15.95995 ^{+    0.00013 }_{   -0.00011 }$&$ 0.27  ^{+ 0.23  }_{ -0.27 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 2.17  \pm{ 0.26  }$&$ 89.40 ^{+ 0.60  }_{ -0.56 }$&$ 26.1  ^{+ 2.5   }_{ -2.0  }$&$ 0.120  \pm{ 0.005  }$&$ 772   \pm{ 41    }$&$ 545   \pm{ 17    }$& 4.6   &\textbf{ 3.6  }&0.451&0.954\\
K00354.02  & 11568987   & 135.8196  &$    7.37878 ^{+    0.00016 }_{   -0.00022 }$&$ 0.06  ^{+ 0.43  }_{ -0.06 }$&$ 0.009  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.98  \pm{ 0.15  }$&$ 89.78 ^{+ 0.22  }_{ -1.60 }$&$ 15.8  ^{+ 1.6   }_{ -1.4  }$&$ 0.071  \pm{ 0.003  }$&$ 983   \pm{ 62    }$&$ 130   \pm{ 11    }$& 3.5   & 1.6  &0.044&0.535\\
K00369.01  & 7175184    & 174.4259  &$    5.88522 ^{+    0.00008 }_{   -0.00009 }$&$ 0.70  ^{+ 0.13  }_{ -0.29 }$&$ 0.010  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.00  ^{+ 0.72  }_{ -0.00 }$&$ 1.26  \pm{ 0.32  }$&$ 87.08 ^{+ 1.49  }_{ -1.14 }$&$ 12.9  ^{+ 2.5   }_{ -2.2  }$&$ 0.068  \pm{ 0.003  }$&$ 1145  \pm{ 125   }$&$ 118   \pm{ 5     }$& 2.4   & 0.7  &0.246&0.891\\
K00369.02  & 7175184    & 135.5572  &$   10.10465 ^{+    0.00021 }_{   -0.00014 }$&$ 0.76  ^{+ 0.09  }_{ -0.18 }$&$ 0.012  ^{+ 0.005  }_{ -0.003 }$&$ 0.40  ^{+ 0.13  }_{ -0.40 }$&$ 3.80  ^{+ 1.16  }_{ -3.79 }$&$ 1.67  \pm{ 0.65  }$&$ 87.50 ^{+ 0.85  }_{ -0.91 }$&$ 16.7  ^{+ 3.2   }_{ -3.3  }$&$ 0.099  \pm{ 0.004  }$&$ 1011  \pm{ 118   }$&$ 116   \pm{ 6     }$& 2.9   & 1.2  &0.166&0.833\\
K00370.01  & 8494142    & 203.6467  &$   42.88255 ^{+    0.00019 }_{   -0.00028 }$&$ 0.58  ^{+ 0.10  }_{ -0.32 }$&$ 0.019  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 4.12  \pm{ 0.42  }$&$ 88.80 ^{+ 0.74  }_{ -0.35 }$&$ 27.6  ^{+ 2.0   }_{ -2.4  }$&$ 0.254  \pm{ 0.007  }$&$ 759   \pm{ 43    }$&$ 415   \pm{ 14    }$& 9.8   & 0.6  &0.056&0.598\\
K00370.02  & 8494142    & 151.5320  &$   22.95036 ^{+    0.00033 }_{   -0.00036 }$&$ 0.84  ^{+ 0.07  }_{ -0.11 }$&$ 0.014  ^{+ 0.000  }_{ -0.002 }$&$ 0.31  ^{+ 0.04  }_{ -0.31 }$&$ 3.63  ^{+ 1.35  }_{ -3.63 }$&$ 3.07  \pm{ 0.43  }$&$ 87.30 ^{+ 0.45  }_{ -0.41 }$&$ 17.9  ^{+ 1.7   }_{ -1.3  }$&$ 0.167  \pm{ 0.005  }$&$ 948   \pm{ 52    }$&$ 132   \pm{ 10    }$& 5.4   & 0.7  &0.147&0.812\\
K00623.01  & 12068975   & 174.0660  &$   10.34968 ^{+    0.00023 }_{   -0.00020 }$&$ 0.43  ^{+ 0.26  }_{ -0.42 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.15  ^{+ 0.39  }_{ -0.15 }$&$ 0.34  ^{+ 3.17  }_{ -0.34 }$&$ 1.35  \pm{ 0.17  }$&$ 88.38 ^{+ 1.62  }_{ -1.20 }$&$ 15.1  ^{+ 1.5   }_{ -1.1  }$&$ 0.089  \pm{ 0.002  }$&$ 1007  \pm{ 59    }$&$ 123   \pm{ 6     }$& 4.6   & 1.3  &0.080&0.813\\
K00623.02  & 12068975   & 179.4702  &$   15.67757 ^{+    0.00034 }_{   -0.00033 }$&$ 0.47  ^{+ 0.22  }_{ -0.47 }$&$ 0.010  ^{+ 0.001  }_{ -0.000 }$&$ 0.08  ^{+ 0.48  }_{ -0.08 }$&$ 0.04  ^{+ 0.57  }_{ -0.04 }$&$ 1.37  \pm{ 0.16  }$&$ 88.58 ^{+ 1.42  }_{ -0.80 }$&$ 19.7  ^{+ 2.2   }_{ -1.7  }$&$ 0.118  \pm{ 0.003  }$&$ 891   \pm{ 52    }$&$ 111   \pm{ 8     }$& 5.5   & 1.3  &0.064&0.773\\
K00623.03  & 12068975   & 171.4706  &$    5.59935 ^{+    0.00011 }_{   -0.00010 }$&$ 0.01  ^{+ 0.76  }_{ -0.01 }$&$ 0.008  ^{+ 0.001  }_{ -0.000 }$&$ 0.43  ^{+ 0.14  }_{ -0.43 }$&$ 0.02  ^{+ 0.30  }_{ -0.02 }$&$ 1.13  \pm{ 0.13  }$&$ 89.97 ^{+ 0.03  }_{ -5.38 }$&$ 10.1  ^{+ 0.9   }_{ -0.8  }$&$ 0.059  \pm{ 0.002  }$&$ 1256  \pm{ 96    }$&$ 89    \pm{ 4     }$& 4.0   & 1.9  &0.027&0.578\\
K00623.04  & 12068975   & 154.4160  &$   25.20971 ^{+    0.00116 }_{   -0.00091 }$&$ 0.82  ^{+ 0.96  }_{ -0.09 }$&$ 0.008  ^{+ 0.016  }_{ -0.006 }$&$ 0.68  ^{+  0.31 }_{ -0.62 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.06  \pm{ 1.48  }$&$ 87.95 ^{+ 0.49  }_{ -1.36 }$&$ 28.5  ^{+ 2.6   }_{ -2.3  }$&$ 0.161  \pm{ 0.004  }$&$ 813   \pm{ 102   }$&$ 75    \pm{ 10    }$& 5.5   & 0.4  &0.014&0.410\\
K00626.01  & 4478168    & 172.2186  &$   14.58667 ^{+    0.00021 }_{   -0.00020 }$&$ 0.32  ^{+ 0.13  }_{ -0.32 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 1.96  \pm{ 0.22  }$&$ 89.24 ^{+ 0.76  }_{ -0.35 }$&$ 23.7  ^{+ 2.0   }_{ -1.7  }$&$ 0.121  \pm{ 0.005  }$&$ 832   \pm{ 43    }$&$ 390   \pm{ 19    }$& 4.4   & 0.5  &0.085&0.700\\
K00626.02  & 4478168    & 132.8298  &$    8.02901 ^{+    0.00023 }_{   -0.00022 }$&$ 0.36  ^{+ 0.34  }_{ -0.36 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.13  ^{+ 0.38  }_{ -0.13 }$&$ 2.85  ^{+ 1.81  }_{ -2.67 }$&$ 0.82  \pm{ 0.17  }$&$ 88.73 ^{+ 1.27  }_{ -1.22 }$&$ 16.0  ^{+ 1.3   }_{ -1.3  }$&$ 0.081  \pm{ 0.004  }$&$ 1016  \pm{ 57    }$&$ 68    \pm{ 13    }$& 3.4   & 0.4  &0.013&0.243\\
K00627.01  & 4563268    & 176.1730  &$    7.75191 ^{+    0.00007 }_{   -0.00008 }$&$ 0.34  ^{+ 0.14  }_{ -0.34 }$&$ 0.017  ^{+ 0.001  }_{ -0.001 }$&$ 0.02  ^{+ 0.30  }_{ -0.02 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 2.23  \pm{ 0.22  }$&$ 88.69 ^{+ 1.31  }_{ -0.68 }$&$ 14.5  ^{+ 1.1   }_{ -1.0  }$&$ 0.081  \pm{ 0.003  }$&$ 1061  \pm{ 53    }$&$ 413   \pm{ 11    }$& 3.9   &\textbf{ 3.3  }&0.190&0.854\\
K00627.02  & 4563268    & 132.0230  &$    4.16547 ^{+    0.00006 }_{   -0.00009 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.22  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -1.54 }$&$ 9.5   ^{+ 0.8   }_{ -0.7  }$&$ 0.054  \pm{ 0.002  }$&$ 1318  \pm{ 72    }$&$ 123   \pm{ 8     }$& 3.4   & 2.5  &0.018&0.319\\
K00655.01  & 5966154    & 192.0969  &$   25.67210 ^{+    0.00018 }_{   -0.00020 }$&$ 0.47  ^{+ 0.17  }_{ -0.25 }$&$ 0.018  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 3.39  ^{+  2.12 }_{ -3.39 }$&$ 2.46  \pm{ 0.26  }$&$ 89.09 ^{+ 0.50  }_{ -0.42 }$&$ 30.1  ^{+ 2.6   }_{ -2.4  }$&$ 0.176  \pm{ 0.007  }$&$ 748   \pm{ 39    }$&$ 394   \pm{ 14    }$& 5.9   & 0.9  &0.189&0.853\\
K00655.02  & 5966154    & 176.4103  &$  151.88600 ^{+    0.00240 }_{   -0.00052 }$&$ 0.19  ^{+ 0.26  }_{ -0.19 }$&$ 0.017  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 2.35  \pm{ 0.27  }$&$ 89.89 ^{+ 0.11  }_{ -0.16 }$&$ 99.2  ^{+ 8.6   }_{ -7.1  }$&$ 0.578  \pm{ 0.026  }$&$ 410   \pm{ 22    }$&$ 362   \pm{ 36    }$& 11.7  & 0.7  &0.080&0.686\\
K00664.01  & 6442340    & 170.2279  &$   13.13742 ^{+    0.00024 }_{   -0.00026 }$&$ 0.42  ^{+ 0.27  }_{ -0.42 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.41  ^{+ 0.04  }_{ -0.41 }$&$ 0.27  ^{+ 0.21  }_{ -0.27 }$&$ 2.18  \pm{ 0.53  }$&$ 88.53 ^{+ 1.47  }_{ -1.35 }$&$ 16.1  ^{+ 3.4   }_{ -3.0  }$&$ 0.110  \pm{ 0.003  }$&$ 980   \pm{ 113   }$&$ 233   \pm{ 14    }$& 4.8   & 0.1  &0.132&0.884\\
K00664.02  & 6442340    & 133.5821  &$    7.78220 ^{+    0.00032 }_{   -0.00030 }$&$ 0.00  ^{+ 0.65  }_{ -0.00 }$&$ 0.009  ^{+ 0.005  }_{ -0.001 }$&$ 0.40  ^{+ 0.40  }_{ -0.40 }$&$ 2.60  ^{+ 2.08  }_{ -2.60 }$&$ 1.43  \pm{ 0.59  }$&$ 90.00 ^{+ 0.00  }_{ -4.31 }$&$ 11.2  ^{+ 3.0   }_{ -2.2  }$&$ 0.078  \pm{ 0.003  }$&$ 1187  \pm{ 188   }$&$ 102   \pm{ 10    }$& 4.1   & 0.5  &0.115&0.867\\
K00664.03  & 6442340    & 152.0300  &$   23.44194 ^{+    0.00175 }_{   -0.00154 }$&$ 0.47  ^{+ 0.31  }_{ -0.42 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 1.26  \pm{ 0.41  }$&$ 88.96 ^{+ 0.95  }_{ -0.78 }$&$ 24.0  ^{+ 7.2   }_{ -4.9  }$&$ 0.162  \pm{ 0.005  }$&$ 780   \pm{ 131   }$&$ 82    \pm{ 18    }$& 6.1   & 0.7  &0.115&0.867\\
K00665.01  & 6685609    & 170.3240  &$    5.86805 ^{+    0.00003 }_{   -0.00004 }$&$ 0.52  ^{+ 0.17  }_{ -0.52 }$&$ 0.019  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.00  ^{+ 1.55  }_{ -0.00 }$&$ 3.04  \pm{ 0.63  }$&$ 86.79 ^{+ 3.21  }_{ -1.81 }$&$ 9.7   ^{+ 1.4   }_{ -1.8  }$&$ 0.067  \pm{ 0.003  }$&$ 1321  \pm{ 125   }$&$ 434   \pm{ 8     }$& 4.2   & 0.2  &0.598&0.987\\
K00665.02  & 6685609    & 133.5707  &$    1.61188 ^{+    0.00008 }_{   -0.00007 }$&$ 0.37  ^{+ 0.26  }_{ -0.37 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.12  ^{+ 1.03  }_{ -0.12 }$&$ 1.61  \pm{ 0.31  }$&$ 83.88 ^{+ 6.12  }_{ -6.02 }$&$ 3.6   ^{+ 0.5   }_{ -0.6  }$&$ 0.029  \pm{ 0.001  }$&$ 2153  \pm{ 191   }$&$ 99    \pm{ 4     }$& 3.3   & 0.8  &0.066&0.779\\
K00665.03  & 6685609    & 133.3015  &$    3.07156 ^{+    0.00006 }_{   -0.00008 }$&$ 0.14  ^{+ 0.36  }_{ -0.14 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 1.46  \pm{ 0.37  }$&$ 88.57 ^{+ 1.43  }_{ -4.27 }$&$ 5.8   ^{+ 1.5   }_{ -1.0  }$&$ 0.044  \pm{ 0.002  }$&$ 1712  \pm{ 192   }$&$ 93    \pm{ 6     }$& 4.2   & 0.3  &0.040&0.677\\
K00678.01  & 7509886    & 172.5935  &$    6.04047 ^{+    0.00009 }_{   -0.00012 }$&$ 1.01  ^{+ 0.06  }_{ -0.05 }$&$ 0.017  ^{+ 0.007  }_{ -0.001 }$&$ 0.05  ^{+ 0.07  }_{ -0.05 }$&$ 0.57  ^{+ 0.99  }_{ -0.57 }$&$ 5.16  \pm{ 1.31  }$&$ 77.92 ^{+ 0.94  }_{ -0.71 }$&$ 4.8   ^{+ 0.1   }_{ -0.0  }$&$ 0.063  \pm{ 0.001  }$&$ 1561  \pm{ 46    }$&$ 264   \pm{ 9     }$& 2.5   & 0.9  &0.420&0.948\\
K00678.02  & 7509886    & 132.0163  &$    4.13855 ^{+    0.00005 }_{   -0.00006 }$&$ 0.99  ^{+ 0.02  }_{ -0.03 }$&$ 0.020  ^{+ 0.004  }_{ -0.000 }$&$ 0.05  ^{+ 0.06  }_{ -0.05 }$&$ 0.36  ^{+ 0.23  }_{ -0.36 }$&$ 6.12  \pm{ 0.60  }$&$ 74.66 ^{+ 1.16  }_{ -0.43 }$&$ 3.7   ^{+ 0.0   }_{ -0.0  }$&$ 0.049  \pm{ 0.001  }$&$ 1770  \pm{ 35    }$&$ 254   \pm{ 7     }$& 2.7   & 1.5  &0.473&0.957\\
K00679.01  & 7515212    & 190.2473  &$   31.80526 ^{+    0.00020 }_{   -0.00019 }$&$ 0.89  ^{+ 0.02  }_{ -0.07 }$&$ 0.019  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.11  }_{ -0.01 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 7.44  \pm{ 0.94  }$&$ 86.30 ^{+ 0.83  }_{ -0.27 }$&$ 13.6  ^{+ 2.3   }_{ -0.4  }$&$ 0.227  \pm{ 0.012  }$&$ 1054  \pm{ 62    }$&$ 338   \pm{ 18    }$& 8.7   & 0.7  &0.251&0.894\\
K00679.02  & 7515212    & 139.6350  &$   16.25831 ^{+    0.00113 }_{   -0.00107 }$&$ 0.89  ^{+ 3.29  }_{ -0.19 }$&$ 0.007  ^{+ 0.027  }_{ -0.003 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 1.17  \pm{ 2.45  }$&$ 83.98 ^{+ 0.83  }_{ -0.57 }$&$ 19.6  ^{+ 11.2  }_{ -7.5  }$&$ 0.135  \pm{ 0.008  }$&$ 1345  \pm{ 1355  }$&$ 51    \pm{ 13    }$& 6.8   & 0.2  &0.018&0.312\\
K00710.01  & 9590976    & 170.9513  &$    5.37485 ^{+    0.00015 }_{   -0.00011 }$&$ 0.92  ^{+  0.00 }_{ -0.07 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.14  ^{+ 0.11  }_{ -0.14 }$&$ 0.00  ^{+ 0.56  }_{ -0.00 }$&$ 4.59  \pm{ 0.72  }$&$ 77.99 ^{+ 2.78  }_{ -0.72 }$&$ 4.4   ^{+ 0.7   }_{ -0.2  }$&$ 0.064  \pm{ 0.008  }$&$ 2118  \pm{ 211   }$&$ 155   \pm{ 7     }$& 4.2   & 2.7  &0.310&0.957\\
K00710.02  & 9590976    & 137.9585  &$    8.58604 ^{+    0.00035 }_{   -0.00033 }$&$ 0.96  ^{+ 0.05  }_{ -0.06 }$&$ 0.010  ^{+ 0.004  }_{ -0.000 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 1.33  }_{ -0.00 }$&$ 3.23  \pm{ 0.72  }$&$ 80.86 ^{+ 1.38  }_{ -1.12 }$&$ 6.0   ^{+ 0.5   }_{ -0.2  }$&$ 0.085  \pm{ 0.006  }$&$ 1817  \pm{ 170   }$&$ 99    \pm{ 9     }$& 3.5   & 1.9  &0.116&0.867\\
K00710.03  & 9590976    & 132.4974  &$    3.88683 ^{+    0.00012 }_{   -0.00012 }$&$ 0.81  ^{+ 1.21  }_{ -0.07 }$&$ 0.008  ^{+ 0.005  }_{ -0.002 }$&$ 0.36  ^{+  0.25 }_{ -0.36 }$&$ 3.41  ^{+  2.87 }_{ -3.41 }$&$ 2.38  \pm{ 1.38  }$&$ 79.03 ^{+ 1.07  }_{ -3.49 }$&$ 3.8   ^{+ 2.3   }_{ -0.4  }$&$ 0.052  \pm{ 0.009  }$&$ 2138  \pm{ 803   }$&$ 58    \pm{ 6     }$& 4.7   & 1.1  &0.036&0.649\\
K00717.01  & 9873254    & 175.7916  &$   14.70751 ^{+    0.00033 }_{   -0.00036 }$&$ 0.65  ^{+ 0.22  }_{ -0.62 }$&$ 0.015  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 1.15  }_{ -0.00 }$&$ 2.00  \pm{ 0.85  }$&$ 88.41 ^{+ 1.52  }_{ -1.29 }$&$ 20.9  ^{+ 7.0   }_{ -6.0  }$&$ 0.121  \pm{ 0.008  }$&$ 781   \pm{ 120   }$&$ 273   \pm{ 16    }$& 3.8   & 0.4  &0.264&0.900\\
K00717.02  & 9873254    & 132.2130  &$    0.90039 ^{+    0.00005 }_{   -0.00006 }$&$ 1.32  ^{+  0.18 }_{ -1.24 }$&$ 0.005  ^{+ 0.000  }_{ -0.001 }$&$ 0.79  ^{+ 0.05  }_{ -0.35 }$&$ 1.60  ^{+ 0.71  }_{ -0.87 }$&$ 1.04  \pm{ 0.41  }$&$ 60.64 ^{+ 27.64 }_{ -3.53 }$&$ 2.4   ^{+ 1.2   }_{ -0.6  }$&$ 0.019  \pm{ 0.001  }$&$ 2297  \pm{ 445   }$&$ 31    \pm{ 3     }$& 1.2   & 0.1  &0.082&0.692\\
K00719.01  & 9950612    & 134.8770  &$    9.03420 ^{+    0.00015 }_{   -0.00013 }$&$ 0.78  ^{+ 0.05  }_{ -0.12 }$&$ 0.024  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 1.02  }_{ -0.00 }$&$ 1.74  \pm{ 0.21  }$&$ 88.24 ^{+ 0.42  }_{ -0.30 }$&$ 24.9  ^{+ 1.9   }_{ -1.8  }$&$ 0.077  \pm{ 0.002  }$&$ 618   \pm{ 34    }$&$ 554   \pm{ 8     }$& 1.8   & 0.9  &0.634&0.989\\
K00719.02  & 9950612    & 146.9200  &$   28.12230 ^{+    0.00138 }_{   -0.00494 }$&$ 0.05  ^{+ 0.38  }_{ -0.05 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.86  \pm{ 0.10  }$&$ 89.95 ^{+ 0.05  }_{ -0.45 }$&$ 51.7  ^{+ 4.4   }_{ -4.2  }$&$ 0.163  \pm{ 0.005  }$&$ 432   \pm{ 24    }$&$ 169   \pm{ 14    }$& 4.2   & 0.6  &0.027&0.579\\
K00719.03  & 9950612    & 166.5382  &$   45.90000 ^{+    0.00978 }_{   -0.00370 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 0.013  ^{+ 0.002  }_{ -0.000 }$&$ 0.32  ^{+ 0.20  }_{ -0.32 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.97  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -0.35 }$&$ 72.1  ^{+ 6.5   }_{ -5.9  }$&$ 0.226  \pm{ 0.008  }$&$ 364   \pm{ 20    }$&$ 185   \pm{ 24    }$& 4.6   & 0.2  &0.038&0.664\\
K00719.04  & 9950612    & 133.7840  &$    4.15982 ^{+    0.00003 }_{   -0.00003 }$&$ 0.40  ^{+ 0.17  }_{ -0.40 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.69  \pm{ 0.09  }$&$ 88.49 ^{+ 1.50  }_{ -0.78 }$&$ 14.9  ^{+ 1.2   }_{ -1.0  }$&$ 0.046  \pm{ 0.001  }$&$ 797   \pm{ 42    }$&$ 144   \pm{ 5     }$& 1.9   & 0.2  &0.067&0.781\\
K00972.01  & 11013201   & 261.5394  &$   13.11891 ^{+    0.00002 }_{   -0.00002 }$&$ 0.82  ^{+ 0.13  }_{ -0.13 }$&$ 0.022  ^{+ 0.004  }_{ -0.004 }$&$ 0.16  ^{+ 0.14  }_{ -0.16 }$&$ 4.73  ^{+ 0.11  }_{ -4.73 }$&$ 9.32  \pm{ 2.47  }$&$ 84.95 ^{+ 2.03  }_{ -2.55 }$&$ 7.7   ^{+ 3.1   }_{ -0.8  }$&$ 0.140  \pm{ 0.004  }$&$ 1742  \pm{ 289   }$&$ 375   \pm{ 26    }$& 5.0   &\textbf{ 4.6  }&0.646&0.979\\
K00972.02  & 11013201   & 139.1430  &$    7.82257 ^{+    0.00044 }_{   -0.00018 }$&$ 0.74  ^{+ 0.27  }_{ -0.25 }$&$ 0.004  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.04  ^{+ 0.37  }_{ -0.04 }$&$ 1.51  \pm{ 0.64  }$&$ 84.12 ^{+ 1.97  }_{ -1.69 }$&$ 6.4   ^{+ 1.8   }_{ -1.5  }$&$ 0.099  \pm{ 0.003  }$&$ 1972  \pm{ 329   }$&$ 16    \pm{ 20    }$& 5.6   & 0.2  &0.089&0.710\\
K01001.01  & 1871056    & 155.7178  &$   40.80686 ^{+    0.00012 }_{   -0.00043 }$&$ 0.00  ^{+ 0.76  }_{ -0.24 }$&$ 0.016  ^{+ 0.002  }_{ -0.001 }$&$ 0.69  ^{+  0.12 }_{ -0.69 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 6.00  \pm{ 0.82  }$&$ 90.00 ^{+  0.00 }_{ -2.68 }$&$ 16.2  ^{+ 2.7   }_{ -0.4  }$&$ 0.260  \pm{ 0.010  }$&$ 1013  \pm{ 73    }$&$ 328   \pm{ 27    }$& 13.7  & 1.2  &0.010&0.202\\
K01001.02  & 1871056    & 216.2450  &$  140.09140 ^{+    0.00229 }_{   -0.00164 }$&$ 0.65  ^{+ 0.22  }_{ -0.57 }$&$ 0.016  ^{+ 0.003  }_{ -0.000 }$&$ 0.00  ^{+ 0.69  }_{ -0.00 }$&$ 0.00  ^{+ 4.24  }_{ -0.00 }$&$ 5.82  \pm{ 1.03  }$&$ 89.14 ^{+ 0.76  }_{ -0.47 }$&$ 37.6  ^{+ 11.4  }_{ -1.4  }$&$ 0.585  \pm{ 0.022  }$&$ 627   \pm{ 71    }$&$ 300   \pm{ 52    }$& 19.3  & 0.3  &0.074&0.666\\
K01151.01  & 8280511    & 134.8157  &$    5.21781 ^{+    0.00021 }_{   -0.00019 }$&$ 0.89  ^{+ 0.06  }_{ -0.02 }$&$ 0.011  ^{+ 0.000  }_{ -0.001 }$&$ 0.05  ^{+ 0.15  }_{ -0.05 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 2.73  \pm{ 0.34  }$&$ 80.79 ^{+ 0.69  }_{ -1.23 }$&$ 5.7   ^{+ 0.7   }_{ -0.4  }$&$ 0.060  \pm{ 0.004  }$&$ 1615  \pm{ 84    }$&$ 99    \pm{ 9     }$& 3.6   & 1.0  &0.039&0.672\\
K01151.02  & 8280511    & 135.7436  &$    7.41105 ^{+    0.00027 }_{   -0.00026 }$&$ 0.89  ^{+ 0.04  }_{ -0.04 }$&$ 0.013  ^{+ 0.001  }_{ -0.001 }$&$ 0.10  ^{+ 0.05  }_{ -0.10 }$&$ 0.00  ^{+ 1.24  }_{ -0.00 }$&$ 3.13  \pm{ 0.47  }$&$ 83.01 ^{+ 0.96  }_{ -1.55 }$&$ 7.5   ^{+ 0.6   }_{ -0.7  }$&$ 0.076  \pm{ 0.006  }$&$ 1417  \pm{ 118   }$&$ 124   \pm{ 10    }$& 3.9   & 0.6  &0.133&0.884\\
K01151.03  & 8280511    & 135.4660  &$    5.24972 ^{+    0.00010 }_{   -0.00012 }$&$ 0.60  ^{+ 0.33  }_{ -0.45 }$&$ 0.007  ^{+ 0.003  }_{ -0.001 }$&$ 0.06  ^{+ 0.52  }_{ -0.06 }$&$ 3.16  ^{+ 1.34  }_{ -3.16 }$&$ 0.86  \pm{ 0.38  }$&$ 86.95 ^{+ 2.39  }_{ -3.14 }$&$ 11.3  ^{+ 2.7   }_{ -2.8  }$&$ 0.057  \pm{ 0.003  }$&$ 1138  \pm{ 185   }$&$ 65    \pm{ 9     }$& 2.9   & 1.0  &0.031&0.615\\
K01151.04  & 8280511    & 146.6500  &$   17.45337 ^{+    0.00142 }_{   -0.00112 }$&$ 0.80  ^{+ 2.14  }_{ -0.30 }$&$ 0.009  ^{+ 0.029  }_{ -0.002 }$&$ 0.01  ^{+ 0.04  }_{ -0.01 }$&$ 0.00  ^{+ 0.34  }_{ -0.01 }$&$ 1.03  \pm{ 1.73  }$&$ 86.70 ^{+  0.21 }_{ -1.51 }$&$ 26.6  ^{+ 7.5   }_{ -7.2  }$&$ 0.125  \pm{ 0.008  }$&$ 1028  \pm{ 529   }$&$ 79    \pm{ 17    }$& 6.0   & 0.1  &0.030&0.606\\
K01151.05  & 8280511    & 134.7589  &$   21.72069 ^{+    0.00024 }_{   -0.00029 }$&$ 0.38  ^{+ 0.37  }_{ -0.38 }$&$ 0.007  ^{+ 0.004  }_{ -0.000 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.75  \pm{ 0.30  }$&$ 89.35 ^{+ 0.64  }_{ -0.85 }$&$ 31.2  ^{+ 7.7   }_{ -6.9  }$&$ 0.145  \pm{ 0.008  }$&$ 659   \pm{ 101   }$&$ 85    \pm{ 19    }$& 4.6   & 2.0  &0.030&0.606\\
K01175.01  & 10350571   & 142.9750  &$   31.59300 ^{+    0.00090 }_{   -0.00005 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 2.09  \pm{ 0.25  }$&$ 90.00 ^{+ 0.00  }_{ -0.84 }$&$ 25.8  ^{+ 2.1   }_{ -2.5  }$&$ 0.195  \pm{ 0.006  }$&$ 731   \pm{ 45    }$&$ 150   \pm{ 26    }$& 9.4   & 0.6  &0.046&0.544\\
K01175.02  & 10350571   & 133.6877  &$   17.15710 ^{+    0.00124 }_{   -0.00170 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 1.84  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -0.92 }$&$ 17.0  ^{+ 1.6   }_{ -1.3  }$&$ 0.130  \pm{ 0.004  }$&$ 897   \pm{ 54    }$&$ 114   \pm{ 20    }$& 7.7   & 0.4  &0.045&0.544\\
K01215.01  & 3939150    & 142.0971  &$   17.32440 ^{+    0.00018 }_{   -0.00019 }$&$ 0.75  ^{+ 0.13  }_{ -0.42 }$&$ 0.014  ^{+ 0.002  }_{ -0.000 }$&$ 0.27  ^{+ 0.08  }_{ -0.27 }$&$ 0.53  ^{+ 2.43  }_{ -0.53 }$&$ 4.87  \pm{ 0.69  }$&$ 85.85 ^{+ 2.86  }_{ -1.18 }$&$ 9.4   ^{+ 1.7   }_{ -0.1  }$&$ 0.137  \pm{ 0.003  }$&$ 1229  \pm{ 156   }$&$ 244   \pm{ 17    }$& 8.9   & 1.2  &0.135&0.796\\
K01215.02  & 3939150    & 145.3899  &$   33.00590 ^{+    0.00061 }_{   -0.00059 }$&$ 0.95  ^{+ 0.14  }_{ -0.07 }$&$ 0.018  ^{+ 0.002  }_{ -0.001 }$&$ 0.05  ^{+ 0.06  }_{ -0.05 }$&$ 1.53  ^{+ 4.04  }_{ -1.50 }$&$ 6.36  \pm{ 0.49  }$&$ 86.25 ^{+ 0.43  }_{ -0.45 }$&$ 14.4  ^{+ 0.1   }_{ -0.2  }$&$ 0.213  \pm{ 0.004  }$&$ 1037  \pm{ 50    }$&$ 285   \pm{ 24    }$& 7.9   & 1.3  &0.128&0.785\\
K01221.01  & 3640905    & 138.5145  &$   30.16012 ^{+    0.00005 }_{   -0.00007 }$&$ 0.65  ^{+ 0.14  }_{ -0.15 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.62  ^{+  0.05 }_{ -0.62 }$&$ 4.28  ^{+ 1.73  }_{ -4.28 }$&$ 2.89  \pm{ 0.41  }$&$ 88.32 ^{+ 0.47  }_{ -0.51 }$&$ 22.0  ^{+ 1.7   }_{ -1.7  }$&$ 0.192  \pm{ 0.005  }$&$ 723   \pm{ 41    }$&$ 171   \pm{ 18    }$& 8.0   & 0.9  &0.138&0.800\\
K01221.02  & 3640905    & 152.3420  &$   51.08020 ^{+    0.00165 }_{   -0.41281 }$&$ 0.13  ^{+ 0.75  }_{ -0.13 }$&$ 0.010  ^{+ 0.002  }_{ -0.001 }$&$ 0.45  ^{+ 0.26  }_{ -0.45 }$&$ 6.29  ^{+  0.00 }_{ -6.29 }$&$ 2.08  \pm{ 0.36  }$&$ 89.77 ^{+ 0.23  }_{ -1.42 }$&$ 32.0  ^{+ 2.9   }_{ -2.6  }$&$ 0.272  \pm{ 0.008  }$&$ 600   \pm{ 38    }$&$ 140   \pm{ 24    }$& 10.8  & 1.0  &0.058&0.606\\
K01241.01  & 6448890    & 147.0928  &$   21.40505 ^{+    0.00009 }_{   -0.00008 }$&$ 0.95  ^{+ 0.02  }_{ -0.02 }$&$ 0.022  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 15.67  \pm{ 3.93  }$&$ 79.59 ^{+  2.12 }_{ -3.42 }$&$ 5.5   ^{+ 0.9   }_{ -1.3  }$&$ 0.164  \pm{ 0.005  }$&$ 1425  \pm{ 159   }$&$ 413   \pm{ 27    }$& 11.6   & 0.7  &0.106&0.748\\
K01241.02  & 6448890    & 135.5589  &$   10.50343 ^{+    0.00028 }_{   -0.00026 }$&$ 0.80  ^{+ 1.69  }_{ -0.42 }$&$ 0.013  ^{+ 0.031  }_{ -0.004 }$&$ 0.00  ^{+ 0.06  }_{ -0.02 }$&$ 0.01  ^{+ 0.29  }_{ -0.03 }$&$ 4.92  \pm{ 6.46  }$&$ 82.94 ^{+  3.17 }_{ -4.73 }$&$ 6.5   ^{+ 0.1   }_{ -0.1  }$&$ 0.103  \pm{ 0.002  }$&$ 1279  \pm{ 317   }$&$ 160   \pm{ 19    }$& 7.7   & 0.7  &0.123&0.778\\
K01316.01  & 10794087   & 138.3401  &$    7.64951 ^{+    0.00028 }_{   -0.00023 }$&$ 0.38  ^{+ 0.28  }_{ -0.32 }$&$ 0.006  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.75  \pm{ 0.50  }$&$ 87.00 ^{+ 2.56  }_{ -2.76 }$&$ 6.5   ^{+ 2.2   }_{ -1.1  }$&$ 0.080  \pm{ 0.002  }$&$ 1407  \pm{ 201   }$&$ 56    \pm{ 6     }$& 7.5   & 1.5  &0.109&0.754\\
K01316.02  & 10794087   & 143.3790  &$   12.37679 ^{+    0.00079 }_{   -0.00044 }$&$ 0.91  ^{+  0.09}_{ -0.91 }$&$ 0.007  ^{+ 0.012  }_{ -0.006 }$&$ 0.01  ^{+ 0.03  }_{ -0.01 }$&$ 0.19  ^{+ 0.06  }_{ -0.19 }$&$ 1.85  \pm{ 1.78  }$&$ 84.30 ^{+ 0.86  }_{ -0.58 }$&$ 9.1   ^{+ 6.4   }_{ -1.7  }$&$ 0.110  \pm{ 0.003  }$&$ 515   \pm{ 39    }$&$ 43     \pm{ 7     }$& 3.9   & 0.3  &0.069&0.650\\
K01445.01  & 11336883   & 135.6794  &$    7.16888 ^{+    0.00017 }_{   -0.00016 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 1.36  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -0.92 }$&$ 12.9  ^{+ 1.1   }_{ -0.9  }$&$ 0.078  \pm{ 0.003  }$&$ 1150  \pm{ 61    }$&$ 115   \pm{ 7     }$& 4.3   & 0.9  &0.143&0.893\\
K01445.02  & 11336883   & 142.1590  &$   54.34430 ^{+    0.02029 }_{   -0.00009 }$&$ 0.42  ^{+ 3.22  }_{ -0.42 }$&$ 0.006  ^{+ 0.009  }_{ -0.002 }$&$ 0.09  ^{+ 0.11  }_{ -0.09 }$&$ 0.10  ^{+ 0.13  }_{ -0.10 }$&$ 0.84  \pm{ 0.77  }$&$ 89.54 ^{+ 0.46  }_{ -3.24 }$&$ 52.2  ^{+ 4.1   }_{ -4.0  }$&$ 0.300  \pm{ 0.011  }$&$ 562   \pm{ 31    }$&$ 40    \pm{ 21    }$& 7.1   & 1.1  &0.032&0.622\\
K01445.03  & 11336883   & 150.8360  &$   20.01960 ^{+    0.00098 }_{   -0.00103 }$&$ 0.31  ^{+ 0.55  }_{ -0.31 }$&$ 0.004  ^{+ 0.003  }_{ -0.001 }$&$ 0.40  ^{+ 0.30  }_{ -0.35 }$&$ 3.93  ^{+ 1.29  }_{ -1.30 }$&$ 0.60  \pm{ 0.28  }$&$ 89.33 ^{+ 0.67  }_{ -1.16 }$&$ 26.6  ^{+ 2.5   }_{ -2.1  }$&$ 0.154  \pm{ 0.006  }$&$ 789   \pm{ 49    }$&$ 20    \pm{ 14    }$& 6.8   & 0.3  &0.032&0.622\\
K01525.01  & 7869917    & 133.5535  &$    7.71468 ^{+    0.00011 }_{   -0.00011 }$&$ 0.59  ^{+ 0.22  }_{ -0.59 }$&$ 0.016  ^{+ 0.001  }_{ -0.003 }$&$ 0.63  ^{+ 0.17  }_{ -0.43 }$&$ 4.53  ^{+ 0.06  }_{ -1.24 }$&$ 3.26  \pm{ 1.07  }$&$ 86.62 ^{+ 3.38  }_{ -4.28 }$&$ 10.3  ^{+ 3.1   }_{ -2.5  }$&$ 0.091  \pm{ 0.005  }$&$ 1447  \pm{ 322   }$&$ 217   \pm{ 10    }$& 4.7   & 0.2  &0.486&0.959\\
K01525.02  & 7869917    & 138.2671  &$   11.80609 ^{+    0.00036 }_{   -0.00046 }$&$ 0.37  ^{+ 0.30  }_{ -0.37 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.46  \pm{ 0.43  }$&$ 88.67 ^{+ 1.33  }_{ -1.36 }$&$ 15.1  ^{+ 4.1   }_{ -2.9  }$&$ 0.106  \pm{ 0.009  }$&$ 1156  \pm{ 163   }$&$ 120   \pm{ 13    }$& 5.4   & 0.8  &0.148&0.812\\
K01534.01  & 4741126    & 146.9846  &$   20.42226 ^{+    0.00047 }_{   -0.00049 }$&$ 0.05  ^{+ 0.48  }_{ -0.05 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 1.83  \pm{ 0.45  }$&$ 89.88 ^{+ 0.12  }_{ -1.26 }$&$ 24.2  ^{+ 5.8   }_{ -4.1  }$&$ 0.160  \pm{ 0.007  }$&$ 862   \pm{ 110   }$&$ 187   \pm{ 16    }$& 6.5   & 1.0  &0.089&0.710\\
K01534.02  & 4741126    & 138.2340  &$    7.63861 ^{+    0.00030 }_{   -0.00030 }$&$ 0.41  ^{+ 0.35  }_{ -0.41 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.00  ^{+ 0.33  }_{ -0.00 }$&$ 1.12  \pm{ 0.34  }$&$ 88.24 ^{+ 1.76  }_{ -1.64 }$&$ 13.2  ^{+ 3.1   }_{ -2.9  }$&$ 0.083  \pm{ 0.004  }$&$ 1160  \pm{ 171   }$&$ 80    \pm{ 10    }$& 4.0   & 0.8  &0.023&0.371\\
K01613.01  & 6268648    & 141.0860  &$   15.86621 ^{+    0.00058 }_{   -0.00057 }$&$ 0.34  ^{+ 0.65  }_{ -0.34 }$&$ 0.008  ^{+ 0.003  }_{ -0.001 }$&$ 0.52  ^{+ 0.32  }_{ -0.14 }$&$ 2.66  ^{+ 1.57  }_{ -1.57 }$&$ 1.32  \pm{ 0.82  }$&$ 88.98 ^{+ 1.02  }_{ -3.05 }$&$ 17.8  ^{+ 8.8   }_{ -6.9  }$&$ 0.127  \pm{ 0.010  }$&$ 900   \pm{ 237   }$&$ 77    \pm{ 6     }$& 4.3   & 0.8  &0.028&0.422\\
K01613.02  & 6268648    & 196.7260  &$   94.09329 ^{+    0.00438 }_{   -0.00051 }$&$ 0.48  ^{+ 0.51  }_{ -0.48 }$&$ 0.008  ^{+ 0.002  }_{ -0.002 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 1.31  \pm{ 0.71  }$&$ 89.57 ^{+ 0.43  }_{ -0.68 }$&$ 59.2  ^{+ 32.3  }_{ -19.3 }$&$ 0.416  \pm{ 0.031  }$&$ 496   \pm{ 159   }$&$ 65    \pm{ 17    }$& 10.0  & 1.2  &0.013&0.254\\
K01628.01  & 6975129    & 147.1029  &$   19.74747 ^{+    0.00031 }_{   -0.00040 }$&$ 0.71  ^{+ 0.12  }_{ -0.30 }$&$ 0.020  ^{+ 0.003  }_{ -0.002 }$&$ 0.08  ^{+ 0.41  }_{ -0.08 }$&$ 0.00  ^{+ 4.60  }_{ -0.00 }$&$ 2.62  \pm{ 0.39  }$&$ 88.53 ^{+ 0.71  }_{ -0.41 }$&$ 27.1  ^{+ 2.5   }_{ -1.8  }$&$ 0.153  \pm{ 0.005  }$&$ 784   \pm{ 46    }$&$ 466   \pm{ 17    }$& 4.0   & 1.2  &0.165&0.832\\
K01628.02  & 6975129    & 132.0945  &$    1.77243 ^{+    0.00003 }_{   -0.00003 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 0.94  \pm{ 0.12  }$&$ 90.00 ^{+  0.00 }_{ -2.07 }$&$ 5.5   ^{+ 0.5   }_{ -0.4  }$&$ 0.029  \pm{ 0.001  }$&$ 1744  \pm{ 91    }$&$ 74    \pm{ 4     }$& 2.5   & 1.8  &0.043&0.530\\
K01692.01  & 6616218    & 137.2639  &$    5.96040 ^{+    0.00003 }_{   -0.00002 }$&$ 0.35  ^{+ 0.09  }_{ -0.35 }$&$ 0.024  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 2.46  \pm{ 0.21  }$&$ 88.64 ^{+ 1.36  }_{ -0.46 }$&$ 14.4  ^{+ 1.1   }_{ -1.0  }$&$ 0.064  \pm{ 0.002  }$&$ 957   \pm{ 40    }$&$ 829   \pm{ 9     }$& 3.0   & 0.9  &0.865&0.994\\
K01692.02  & 6616218    & 133.3133  &$    2.46110 ^{+    0.00003 }_{   -0.00003 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.80  \pm{ 0.10  }$&$ 90.00 ^{+ 0.00  }_{ -2.57 }$&$ 8.0   ^{+ 0.7   }_{ -0.7  }$&$ 0.035  \pm{ 0.001  }$&$ 1288  \pm{ 73    }$&$ 82    \pm{ 6     }$& 2.4   & 0.7  &0.026&0.404\\
K01779.01  & 9909735    & 134.0812  &$    4.66272 ^{+    0.00001 }_{   -0.00001 }$&$ 0.84  ^{+ 0.06  }_{ -0.19 }$&$ 0.041  ^{+ 0.004  }_{ -0.001 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.00  ^{+ 4.76  }_{ -0.00 }$&$ 7.84  \pm{ 1.47  }$&$ 83.09 ^{+ 2.83  }_{ -1.84 }$&$ 6.7   ^{+ 1.6   }_{ -0.8  }$&$ 0.054  \pm{ 0.002  }$&$ 1458  \pm{ 171   }$&$ 1627  \pm{ 10    }$& 3.1   & 0.8  &0.636&0.978\\
K01779.02  & 9909735    & 133.0899  &$   11.81502 ^{+    0.00009 }_{   -0.00004 }$&$ 0.93  ^{+ 0.24  }_{ -0.09 }$&$ 0.037  ^{+ 0.000  }_{ -0.005 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 4.48  ^{+  0.90 }_{ -4.48 }$&$ 6.54  \pm{ 1.68  }$&$ 86.18 ^{+ 1.16  }_{ -2.96 }$&$ 13.5  ^{+ 3.1   }_{ -3.1  }$&$ 0.101  \pm{ 0.003  }$&$ 1034  \pm{ 155   }$&$ 1028  \pm{ 18    }$& 3.0   & 1.4  &0.170&0.836\\
\textbf{K01781.01  }& 11551692   & 135.2206  &$    7.83445 ^{+    0.00001 }_{   -0.00001 }$&$ 0.33  ^{+ 0.31  }_{ -0.15 }$&$ 0.037  ^{+ 0.011  }_{ -0.000 }$&$ 0.00  ^{+ 0.66  }_{ -0.00 }$&$ 0.00  ^{+ 4.72  }_{ -0.00 }$&$ 3.24  \pm{ 0.56  }$&$ 89.03 ^{+ 0.49  }_{ -1.08 }$&$ 19.4  ^{+ 1.4   }_{ -1.3  }$&$ 0.073  \pm{ 0.002  }$&$ 753   \pm{ 34    }$&$ 1954  \pm{ 11    }$& 3.1   &\textbf{ 3.5  }&0.995&\textbf{1.000} \\
\textbf{K01781.02  }& 11551692   & 137.1027  &$    3.00516 ^{+    0.00001 }_{   -0.00001 }$&$ 0.31  ^{+ 0.27  }_{ -0.30 }$&$ 0.022  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.35  }_{ -0.00 }$&$ 0.00  ^{+ 4.31  }_{ -0.00 }$&$ 1.88  \pm{ 0.20  }$&$ 88.27 ^{+ 1.73  }_{ -1.83 }$&$ 10.2  ^{+ 0.6   }_{ -0.8  }$&$ 0.038  \pm{ 0.001  }$&$ 1040  \pm{ 46    }$&$ 690   \pm{ 5     }$& 2.2   & 0.9  &0.979&\textbf{1.000} \\
K01781.03  & 11551692   & 151.8476  &$   58.02125 ^{+    0.00020 }_{   -0.00013 }$&$ 0.50  ^{+ 0.16  }_{ -0.47 }$&$ 0.031  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 2.61  \pm{ 0.31  }$&$ 89.63 ^{+ 0.35  }_{ -0.16 }$&$ 76.0  ^{+ 6.7   }_{ -6.4  }$&$ 0.276  \pm{ 0.007  }$&$ 377   \pm{ 20    }$&$ 1338  \pm{ 46    }$& 5.1   & 1.2  &0.598&0.987\\
%           &            & 0.0000    &$   58.02125 ^{+    0.00044 }_{   -0.00018 }$&$ 0.50  ^{+ 0.16  }_{ -0.47 }$&$ 0.031  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 2.61  \pm{ 0.31  }$&$ 89.63 ^{+ 0.35  }_{ -0.16 }$&$ 76.0  ^{+ 6.7   }_{ -6.4  }$&$ 0.276  \pm{ 0.007  }$&$ 377   \pm{ 20    }$&$ 1338  \pm{ 46    }$& 5.1   & 1.2  &%
K01806.02  & 9529744    & 138.2171  &$   17.93497 ^{+    0.00050 }_{   -0.00080 }$&$ 0.31  ^{+ 0.19  }_{ -0.31 }$&$ 0.012  ^{+ 0.000  }_{ -0.003 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.60  \pm{ 0.40  }$&$ 89.30 ^{+ 0.70  }_{ -0.57 }$&$ 24.4  ^{+ 5.5   }_{ -4.8  }$&$ 0.137  \pm{ 0.008  }$&$ 849   \pm{ 109   }$&$ 176   \pm{ 18    }$& 5.2   &\textbf{ 3.1  }&0.112&0.863\\
K01806.03  & 9529744    & 137.6755  &$    8.37167 ^{+    0.00000 }_{    0.00000 }$&$ 0.27  ^{+ 0.33  }_{ -0.27 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.54  }_{ -0.00 }$&$ 1.09  \pm{ 0.32  }$&$ 88.99 ^{+ 1.01  }_{ -1.33 }$&$ 14.7  ^{+ 3.8   }_{ -2.9  }$&$ 0.083  \pm{ 0.005  }$&$ 1087  \pm{ 152   }$&$ 89    \pm{ 13    }$& 4.0   &\textbf{ 4.1  }&0.034&0.640\\
K01809.01  & 8240797    & 144.5235  &$   13.09392 ^{+    0.00016 }_{   -0.00017 }$&$ 0.96  ^{+ 0.45  }_{ -0.02 }$&$ 0.023  ^{+ 0.014  }_{ -0.003 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.00  ^{+ 1.58  }_{ -0.00 }$&$ 6.15  \pm{ 3.24  }$&$ 86.14 ^{+ 0.00  }_{ -6.28 }$&$ 10.0  ^{+ 3.9   }_{ -2.2  }$&$ 0.115  \pm{ 0.014  }$&$ 1009  \pm{ 145   }$&$ 390   \pm{ 9     }$& 2.5   & 1.4  &0.462&0.956\\
K01809.02  & 8240797    & 132.6958  &$    4.91538 ^{+    0.00000 }_{   -0.00000 }$&$ 0.72  ^{+ 0.15  }_{ -0.35 }$&$ 0.015  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.00  ^{+ 0.94  }_{ -0.00 }$&$ 2.42  \pm{ 0.85  }$&$ 85.24 ^{+ 2.85  }_{ -3.09 }$&$ 8.5   ^{+ 2.4   }_{ -2.2  }$&$ 0.058  \pm{ 0.003  }$&$ 1293  \pm{ 218   }$&$ 235   \pm{ 6     }$& 3.1   & 1.1  &0.263&0.899\\
K01824.01  & 2989404    & 134.6430  &$    3.55380 ^{+    0.00004 }_{   -0.00004 }$&$ 0.50  ^{+ 0.18  }_{ -0.41 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.33  }_{ -0.00 }$&$ 0.15  ^{+ 4.37  }_{ -0.15 }$&$ 2.07  \pm{ 0.44  }$&$ 85.76 ^{+ 3.56  }_{ -2.65 }$&$ 6.6   ^{+ 1.3   }_{ -1.0  }$&$ 0.049  \pm{ 0.002  }$&$ 1591  \pm{ 150   }$&$ 197   \pm{ 5     }$& 3.5   & 0.5  &0.202&0.863\\
K01824.02  & 2989404    & 136.0502  &$    1.67834 ^{+    0.00002 }_{   -0.00002 }$&$ 0.63  ^{+ 0.21  }_{ -0.44 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.03  ^{+ 0.53  }_{ -0.03 }$&$ 0.08  ^{+ 2.53  }_{ -0.08 }$&$ 2.12  \pm{ 0.49  }$&$ 79.91 ^{+ 7.73  }_{ -7.45 }$&$ 3.6   ^{+ 0.7   }_{ -0.6  }$&$ 0.030  \pm{ 0.001  }$&$ 2196  \pm{ 244   }$&$ 152   \pm{ 3     }$& 2.9   & 0.3  &0.184&0.849\\
K01909.01  & 10130039   & 133.9557  &$   12.75808 ^{+    0.00023 }_{   -0.00022 }$&$ 0.28  ^{+ 0.17  }_{ -0.28 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.44  ^{+ 0.04  }_{ -0.44 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.65  \pm{ 0.35  }$&$ 89.22 ^{+ 0.78  }_{ -0.59 }$&$ 20.3  ^{+ 3.6   }_{ -3.3  }$&$ 0.113  \pm{ 0.004  }$&$ 888   \pm{ 84    }$&$ 191   \pm{ 9     }$& 4.2   & 0.4  &0.210&0.930\\
K01909.02  & 10130039   & 131.4909  &$    5.47037 ^{+    0.00011 }_{   -0.00008 }$&$ 0.22  ^{+ 0.41  }_{ -0.22 }$&$ 0.008  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 1.11  \pm{ 0.25  }$&$ 88.89 ^{+ 1.11  }_{ -2.56 }$&$ 11.1  ^{+ 2.1   }_{ -1.8  }$&$ 0.064  \pm{ 0.003  }$&$ 1201  \pm{ 120   }$&$ 110   \pm{ 6     }$& 3.6   & 0.2  &0.060&0.762\\
K01909.03  & 10130039   & 145.5671  &$   25.09858 ^{+    0.00089 }_{   -0.00084 }$&$ 0.89  ^{+ 0.04  }_{ -0.26 }$&$ 0.015  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 0.00  ^{+ 1.40  }_{ -0.00 }$&$ 1.97  \pm{ 0.58  }$&$ 88.36 ^{+ 0.73  }_{ -0.55 }$&$ 30.7  ^{+ 7.3   }_{ -6.6  }$&$ 0.178  \pm{ 0.008  }$&$ 725   \pm{ 94    }$&$ 187   \pm{ 13    }$& 3.0   & 0.2  &0.133&0.885\\
K01929.01  & 10136549   & 132.8155  &$    9.69303 ^{+    0.00016 }_{   -0.00019 }$&$ 0.70  ^{+ 0.16  }_{ -0.59 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.16  ^{+ 0.82  }_{ -0.16 }$&$ 2.47  \pm{ 0.69  }$&$ 85.55 ^{+ 3.90  }_{ -2.57 }$&$ 9.8   ^{+ 2.5   }_{ -2.4  }$&$ 0.089  \pm{ 0.002  }$&$ 1304  \pm{ 182   }$&$ 145   \pm{ 9     }$& 6.0   & 0.7  &0.147&0.812\\
K01929.02  & 10136549   & 133.0093  &$    3.29274 ^{+    0.00008 }_{   -0.00008 }$&$ 0.68  ^{+ 0.15  }_{ -0.16 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.04  ^{+ 0.37  }_{ -0.04 }$&$ 0.45  ^{+ 0.31  }_{ -0.45 }$&$ 2.20  \pm{ 0.35  }$&$ 79.37 ^{+ 3.24  }_{ -3.45 }$&$ 4.0   ^{+ 0.5   }_{ -0.6  }$&$ 0.044  \pm{ 0.001  }$&$ 2037  \pm{ 166   }$&$ 83    \pm{ 5     }$& 5.1   & 0.3  &0.145&0.809\\
K01930.01  & 5511081    & 138.7478  &$   13.72686 ^{+    0.00010 }_{   -0.00011 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 2.25  \pm{ 0.21  }$&$ 90.00 ^{+ 0.00  }_{ -1.47 }$&$ 15.5  ^{+ 1.2   }_{ -1.2  }$&$ 0.115  \pm{ 0.003  }$&$ 1006  \pm{ 50    }$&$ 200   \pm{ 12    }$& 7.0   & 1.5  &0.170&0.911\\
K01930.02  & 5511081    & 137.0438  &$   24.31058 ^{+    0.00024 }_{   -0.00028 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 2.19  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -1.12 }$&$ 22.9  ^{+ 1.9   }_{ -1.8  }$&$ 0.168  \pm{ 0.004  }$&$ 821   \pm{ 43    }$&$ 180   \pm{ 15    }$& 8.3   & 1.8  &0.104&0.852\\
K01930.03  & 5511081    & 143.5344  &$   44.43150 ^{+    0.00028 }_{   -0.00020 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.17  ^{+ 0.33  }_{ -0.17 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 2.57  \pm{ 0.26  }$&$ 90.00 ^{+ 0.00  }_{ -0.44 }$&$ 34.7  ^{+ 3.2   }_{ -2.4  }$&$ 0.252  \pm{ 0.006  }$&$ 663   \pm{ 35    }$&$ 248   \pm{ 21    }$& 9.7   & 1.6  &0.116&0.867\\
K01930.04  & 5511081    & 132.3931  &$    9.34131 ^{+    0.00038 }_{   -0.00032 }$&$ 0.17  ^{+ 0.30  }_{ -0.17 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.50  ^{+ 0.15  }_{ -0.47 }$&$ 3.56  ^{+ 1.11  }_{ -3.00 }$&$ 1.32  \pm{ 0.18  }$&$ 89.21 ^{+ 0.79  }_{ -1.42 }$&$ 12.5  ^{+ 1.1   }_{ -1.0  }$&$ 0.089  \pm{ 0.002  }$&$ 1105  \pm{ 70    }$&$ 79    \pm{ 9     }$& 6.1   & 1.6  &0.057&0.752\\
K01932.01  & 5202905    & 144.4640  &$   22.82485 ^{+    0.00007 }_{   -0.00004 }$&$ 0.71  ^{+ 0.13  }_{ -0.34 }$&$ 0.017  ^{+ 0.003  }_{ -0.004 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.44  ^{+ 3.13  }_{ -0.44 }$&$ 6.05  \pm{ 1.96  }$&$ 87.21 ^{+ 1.63  }_{ -1.36 }$&$ 13.4  ^{+ 4.0   }_{ -3.1  }$&$ 0.203  \pm{ 0.007  }$&$ 1429  \pm{ 236   }$&$ 317   \pm{ 69    }$& 8.7   & 0.6  &0.019&0.328\\
K01932.02  & 5202905    & 143.5855  &$   14.84440 ^{+    0.00185 }_{   -0.00204 }$&$ 0.79  ^{+ 1.06  }_{ -0.03 }$&$ 0.012  ^{+ 0.028  }_{ -0.002 }$&$ 0.26  ^{+ 0.15  }_{ -0.02 }$&$ 2.16  ^{+ 2.62  }_{ -1.15 }$&$ 3.05  \pm{ 4.04  }$&$ 85.54 ^{+ 0.18  }_{ -2.82 }$&$ 11.3  ^{+ 3.2   }_{ -2.6  }$&$ 0.123  \pm{ 0.021  }$&$ 1715  \pm{ 359   }$&$ 200   \pm{ 54    }$& 7.2   & 0.5  &0.088&0.707\\
K01955.01  & 9892816    & 132.6668  &$   15.17019 ^{+    0.00021 }_{   -0.00035 }$&$ 0.94  ^{+ 0.02  }_{ -0.04 }$&$ 0.016  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 4.40  \pm{ 1.23  }$&$ 85.02 ^{+ 1.14  }_{ -1.28 }$&$ 12.7  ^{+ 2.3   }_{ -2.8  }$&$ 0.146  \pm{ 0.009  }$&$ 1309  \pm{ 128   }$&$ 230   \pm{ 12    }$& 4.3   & 1.1  &0.175&0.914\\
K01955.02  & 9892816    & 136.4553  &$   39.45988 ^{+    0.00008 }_{   -0.00014 }$&$ 0.00  ^{+ 0.73  }_{ -0.00 }$&$ 0.012  ^{+ 0.004  }_{ -0.001 }$&$ 0.22  ^{+ 0.61  }_{ -0.22 }$&$ 3.56  ^{+ 1.04  }_{ -3.55 }$&$ 1.88  \pm{ 0.65  }$&$ 90.00 ^{+ 0.00  }_{ -1.49 }$&$ 36.7  ^{+ 8.1   }_{ -8.5  }$&$ 0.251  \pm{ 0.013  }$&$ 728   \pm{ 107   }$&$ 231   \pm{ 21    }$& 9.4   & 0.5  &0.172&0.912\\
K01955.03  & 9892816    & 131.7567  &$    1.64420 ^{+    0.00003 }_{   -0.00003 }$&$ 0.20  ^{+ 0.45  }_{ -0.20 }$&$ 0.004  ^{+ 0.002  }_{ -0.000 }$&$ 0.79  ^{+ 0.08  }_{ -0.53 }$&$ 4.03  ^{+ 0.25  }_{ -2.14 }$&$ 0.54  \pm{ 0.24  }$&$ 87.71 ^{+ 2.29  }_{ -7.24 }$&$ 4.9   ^{+ 1.6   }_{ -1.1  }$&$ 0.028  \pm{ 0.002  }$&$ 1900  \pm{ 398   }$&$ 31    \pm{ 4     }$& 7.4   & 0.6  &0.016&0.443\\
K01955.04  & 9892816    & 141.9958  &$   26.23420 ^{+    0.00069 }_{   -0.00105 }$&$ 0.68  ^{+ 0.20  }_{ -0.19 }$&$ 0.019  ^{+  0.003 }_{ -0.009 }$&$ 0.38  ^{+ 0.05  }_{ -0.38 }$&$ 4.72  ^{+  0.07 }_{ -4.72 }$&$ 2.53  \pm{ 0.70  }$&$ 88.82 ^{+ 0.52  }_{ -0.65 }$&$ 31.3  ^{+ 7.6   }_{ -5.8  }$&$ 0.178  \pm{ 0.012  }$&$ 747   \pm{ 104   }$&$ 170   \pm{ 17    }$& 3.6   & 1.2  &0.068&0.784\\
K02004.01  & 12154526   & 146.3714  &$   56.18945 ^{+    0.00058 }_{   -0.00086 }$&$ 0.64  ^{+ 0.24  }_{ -0.62 }$&$ 0.017  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.46  }_{ -0.00 }$&$ 0.00  ^{+ 1.54  }_{ -0.00 }$&$ 2.38  \pm{ 0.66  }$&$ 89.21 ^{+ 0.77  }_{ -0.71 }$&$ 49.3  ^{+ 11.7  }_{ -9.2  }$&$ 0.291  \pm{ 0.013  }$&$ 560   \pm{ 92    }$&$ 368   \pm{ 31    }$& 7.2   & 0.9  &0.326&0.960\\
K02004.02  & 12154526   & 133.5255  &$    3.18899 ^{+    0.00017 }_{   -0.00005 }$&$ 0.90  ^{+ 0.09  }_{ -0.11 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.07  ^{+ 0.16  }_{ -0.07 }$&$ 1.83  ^{+ 0.69  }_{ -1.83 }$&$ 1.73  \pm{ 0.32  }$&$ 79.74 ^{+ 1.09  }_{ -1.32 }$&$ 5.3   ^{+ 0.6   }_{ -0.8  }$&$ 0.044  \pm{ 0.003  }$&$ 1700  \pm{ 130   }$&$ 69    \pm{ 7     }$& 2.6   & 0.5  &0.083&0.819\\
K02004.03  & 12154526   & 132.7764  &$    1.72107 ^{+    0.00002 }_{ -   0.00002 }$&$ 0.99  ^{+ 0.01  }_{ -0.01  }$&$ 0.008  ^{+ 0.001  }_{ -0.001  }$&$ 0.00  ^{+ 0.03  }_{ -0.00  }$&$ 0.00  ^{+ 0.05  }_{- 0.00  }$&$ 0.83  \pm{ 0.12  }$&$ 39.70  ^{+ 9.40  }_{- 9.40  }$&$ 1.3   ^{+ 0.2   }_{ -0.2  }$&$ 0.027  \pm{ 0.003  }$&$ 1250     \pm{ 300     }$&$ 37    \pm{ 7     }$& 1.9   & 1.5  &0.083&0.819\\
K02011.01  & 5384079    & 132.5342  &$    7.05670 ^{+    0.00014 }_{   -0.00010 }$&$ 0.91  ^{+ 0.04  }_{ -0.05 }$&$ 0.015  ^{+ 0.001  }_{ -0.002 }$&$ 0.05  ^{+ 0.12  }_{ -0.05 }$&$ 0.02  ^{+ 3.17  }_{ -0.02 }$&$ 2.57  \pm{ 0.51  }$&$ 84.91 ^{+ 0.75  }_{ -1.13 }$&$ 10.5  ^{+ 1.4   }_{ -1.5  }$&$ 0.080  \pm{ 0.003  }$&$ 1319  \pm{ 106   }$&$ 128   \pm{ 6     }$& 2.4   & 0.7  &0.044&0.533\\
K02011.02  & 5384079    & 135.3499  &$   17.26555 ^{+    0.00083 }_{   -0.00075 }$&$ 0.18  ^{+ 0.40  }_{ -0.18 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.56  }_{ -0.00 }$&$ 1.04  \pm{ 0.31  }$&$ 89.61 ^{+ 0.39  }_{ -1.00 }$&$ 24.3  ^{+ 6.9   }_{ -5.1  }$&$ 0.134  \pm{ 0.008  }$&$ 836   \pm{ 136   }$&$ 79    \pm{ 11    }$& 5.1   & 0.7  &0.005&0.115\\
K02029.01  & 9489524    & 136.9036  &$   16.33287 ^{+    0.00032 }_{   -0.00034 }$&$ 0.78  ^{+ 0.13  }_{ -0.33 }$&$ 0.018  ^{+ 0.003  }_{ -0.004 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 1.65  \pm{ 0.49  }$&$ 88.55 ^{+ 0.86  }_{ -0.77 }$&$ 30.3  ^{+ 6.8   }_{ -6.0  }$&$ 0.122  \pm{ 0.006  }$&$ 624   \pm{ 90    }$&$ 293   \pm{ 14    }$& 2.6   & 0.2  &0.076&0.803\\
K02029.02  & 9489524    & 173.2239  &$   10.05548 ^{+    0.00025 }_{   -0.00030 }$&$ 0.19  ^{+ 0.40  }_{ -0.19 }$&$ 0.010  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.05  ^{+ 0.48  }_{ -0.05 }$&$ 0.89  \pm{ 0.25  }$&$ 89.52 ^{+ 0.48  }_{ -1.15 }$&$ 22.4  ^{+ 5.0   }_{ -4.5  }$&$ 0.088  \pm{ 0.004  }$&$ 723   \pm{ 90    }$&$ 151   \pm{ 11    }$& 3.3   & 0.8  &0.015&0.431\\
K02029.03  & 9489524    & 132.0775  &$    6.88721 ^{+    0.00016 }_{   -0.00023 }$&$ 0.42  ^{+ 0.26  }_{ -0.42 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 0.67  \pm{ 0.18  }$&$ 88.68 ^{+ 1.32  }_{ -0.99 }$&$ 17.6  ^{+ 3.9   }_{ -3.2  }$&$ 0.067  \pm{ 0.003  }$&$ 812   \pm{ 99    }$&$ 83    \pm{ 9     }$& 2.6   & 0.6  &0.013&0.394\\
K02029.04  & 9489524    & 135.4647  &$    4.78843 ^{+    0.00011 }_{   -0.00013 }$&$ 0.52  ^{+ 0.20  }_{ -0.52 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.47  ^{+ 0.41  }_{ -0.47 }$&$ 3.99  ^{+ 0.68  }_{ -2.93 }$&$ 0.63  \pm{ 0.20  }$&$ 87.92 ^{+ 2.08  }_{ -1.42 }$&$ 13.6  ^{+ 3.5   }_{ -3.0  }$&$ 0.053  \pm{ 0.002  }$&$ 919   \pm{ 137   }$&$ 63    \pm{ 8     }$& 2.8   & 1.1  &0.013&0.394\\
K02053.01  & 2307415    & 133.3943  &$   13.12155 ^{+    0.00034 }_{   -0.00030 }$&$ 0.55  ^{+ 0.21  }_{ -0.52 }$&$ 0.012  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.47  }_{ -0.00 }$&$ 0.07  ^{+ 3.90  }_{ -0.07 }$&$ 1.74  \pm{ 0.48  }$&$ 88.36 ^{+ 1.59  }_{ -1.10 }$&$ 18.4  ^{+ 4.1   }_{ -3.6  }$&$ 0.116  \pm{ 0.006  }$&$ 960   \pm{ 122   }$&$ 197   \pm{ 14    }$& 4.5   & 0.7  &0.049&0.562\\
K02053.02  & 2307415    & 132.7749  &$    4.61266 ^{+    0.00010 }_{   -0.00011 }$&$ 0.67  ^{+ 0.03  }_{ -0.17 }$&$ 0.013  ^{+ 0.009  }_{ -0.003 }$&$ 0.31  ^{+ 0.41  }_{ -0.16 }$&$ 5.04  ^{+ 0.33  }_{ -0.50 }$&$ 2.40  \pm{ 1.42  }$&$ 84.45 ^{+ 2.91  }_{ -2.42 }$&$ 7.3   ^{+ 3.2   }_{ -1.9  }$&$ 0.059  \pm{ 0.003  }$&$ 1590  \pm{ 333   }$&$ 137   \pm{ 8     }$& 3.7   & 0.5  &0.061&0.618\\
K02059.01  & 12301181   & 134.8728  &$    6.14730 ^{+    0.00016 }_{   -0.00009 }$&$ 0.19  ^{+ 0.26  }_{ -0.19 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.77  \pm{ 0.17  }$&$ 89.34 ^{+ 0.66  }_{ -1.00 }$&$ 16.1  ^{+ 3.0   }_{ -2.7  }$&$ 0.055  \pm{ 0.002  }$&$ 791   \pm{ 81    }$&$ 132   \pm{ 8     }$& 2.9   & 0.5  &0.059&0.612\\
K02059.02  & 12301181   & 132.4311  &$    2.18574 ^{+    0.00002 }_{-    0.00002 }$&$ 0.98  ^{+ 0.02  }_{- 0.02  }$&$ 0.008  ^{+ 0.001  }_{- 0.001  }$&$ 0.00  ^{+ 0.03  }_{- 0.00  }$&$ 0.05  ^{+ 0.00  }_{- 0.05  }$&$ 0.60  \pm{ 0.10  }$&$ 57.00  ^{+ 19.00  }_{- 19.00  }$&$ 1.8  ^{+ 0.9   }_{ -0.9  }$&$ 0.029  \pm{ 0.002  }$&$ 1250     \pm{ 300     }$&$ 38   \pm{ 8     }$& 2.1   & 0.7  &0.024&0.378\\
K02148.01  & 6021193    & 142.1019  &$   11.93223 ^{+    0.00021 }_{   -0.00025 }$&$ 0.00  ^{+ 0.71  }_{ -0.00 }$&$ 0.011  ^{+ 0.003  }_{ -0.000 }$&$ 0.19  ^{+ 0.41  }_{ -0.19 }$&$ 1.38  ^{+ 2.92  }_{ -1.38 }$&$ 2.68  \pm{ 0.83  }$&$ 90.00 ^{+  0.00 }_{ -4.56 }$&$ 10.1  ^{+ 3.0   }_{ -2.5  }$&$ 0.104  \pm{ 0.004  }$&$ 1128  \pm{ 159   }$&$ 194   \pm{ 17    }$& 7.0   & 0.2  &0.138&0.889\\
K02148.02  & 6021193    & 132.9564  &$    7.54236 ^{+    0.00029 }_{   -0.00029 }$&$ 0.50  ^{+ 0.35  }_{ -0.50 }$&$ 0.009  ^{+ 0.002  }_{ -0.001 }$&$ 0.42  ^{+ 0.26  }_{ -0.42 }$&$ 0.28  ^{+ 2.11  }_{ -0.28 }$&$ 2.14  \pm{ 0.65  }$&$ 86.40 ^{+ 3.60  }_{ -3.88 }$&$ 7.5   ^{+ 1.9   }_{ -1.9  }$&$ 0.077  \pm{ 0.003  }$&$ 1315  \pm{ 193   }$&$ 123   \pm{ 14    }$& 5.5   & 0.4  &0.138&0.889\\
K02148.03  & 6021193    & 134.7000  &$    3.61461 ^{+    0.00011 }_{   -0.00010 }$&$ 1.13  ^{+ 0.60  }_{ -0.74 }$&$ 0.008  ^{+ 0.009  }_{ -0.001 }$&$ 0.73  ^{+ 0.07  }_{ -0.32 }$&$ 2.40  ^{+ 1.96  }_{ -1.56 }$&$ 2.00  \pm{ 1.36  }$&$ 75.75 ^{+ 9.85  }_{ -5.98 }$&$ 4.3   ^{+ 1.2   }_{ -0.9  }$&$ 0.047  \pm{ 0.002  }$&$ 1734  \pm{ 269   }$&$ 72    \pm{ 9     }$& 12.1  & 0.8  &0.083&0.819\\
K02158.01  & 5211199    & 132.6314  &$    4.56215 ^{+    0.00010 }_{   -0.00014 }$&$ 0.77  ^{+ 0.11  }_{ -0.27 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.11  ^{+ 0.45  }_{ -0.11 }$&$ 0.96  ^{+  0.33 }_{ -0.96 }$&$ 1.64  \pm{ 0.37  }$&$ 83.35 ^{+ 2.93  }_{ -1.72 }$&$ 6.3   ^{+ 1.2   }_{ -0.9  }$&$ 0.052  \pm{ 0.001  }$&$ 1390  \pm{ 138   }$&$ 81    \pm{ 7     }$& 3.5   & 1.0  &0.023&0.370\\
K02158.02  & 5211199    & 132.1895  &$    6.68232 ^{+    0.00020 }_{   -0.00033 }$&$ 0.72  ^{+ 0.17  }_{ -0.25 }$&$ 0.007  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 1.39  \pm{ 0.49  }$&$ 85.37 ^{+ 1.66  }_{ -1.31 }$&$ 8.2   ^{+ 2.1   }_{ -1.7  }$&$ 0.072  \pm{ 0.006  }$&$ 1205  \pm{ 161   }$&$ 50    \pm{ 8     }$& 4.1   & 1.1  &0.005&0.104\\
K02169.01  & 9006186    & 134.1486  &$    5.45300 ^{+    0.00009 }_{   -0.00011 }$&$ 0.71  ^{+ 0.13  }_{ -0.25 }$&$ 0.008  ^{+ 0.002  }_{ -0.001 }$&$ 0.32  ^{+ 0.16  }_{ -0.32 }$&$ 0.27  ^{+ 1.37  }_{ -0.27 }$&$ 1.01  \pm{ 0.23  }$&$ 86.53 ^{+ 1.58  }_{ -1.22 }$&$ 11.4  ^{+ 2.3   }_{ -1.7  }$&$ 0.058  \pm{ 0.002  }$&$ 1056  \pm{ 105   }$&$ 94    \pm{ 4     }$& 2.5   & 1.0  &0.105&0.854\\
K02169.02  & 9006186    & 136.0883  &$    3.26661 ^{+    0.00006 }_{   -0.00005 }$&$ 0.66  ^{+ 0.14  }_{ -0.36 }$&$ 0.007  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.00  ^{+ 0.71  }_{ -0.00 }$&$ 0.86  \pm{ 0.21  }$&$ 85.27 ^{+ 2.92  }_{ -1.59 }$&$ 7.9   ^{+ 1.5   }_{ -1.4  }$&$ 0.042  \pm{ 0.001  }$&$ 1275  \pm{ 135   }$&$ 58    \pm{ 3     }$& 2.4   & 0.1  &0.077&0.808\\
K02169.03  & 9006186    & 133.2112  &$    4.27235 ^{+    0.00011 }_{   -0.00009 }$&$ 0.59  ^{+ 0.21  }_{ -0.46 }$&$ 0.006  ^{+ 0.001  }_{ -0.001 }$&$ 0.29  ^{+ 0.16  }_{ -0.29 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.69  \pm{ 0.18  }$&$ 86.57 ^{+ 2.72  }_{ -1.77 }$&$ 9.5   ^{+ 2.1   }_{ -1.5  }$&$ 0.050  \pm{ 0.001  }$&$ 1150  \pm{ 138   }$&$ 48    \pm{ 4     }$& 2.7   & 1.2  &0.057&0.751\\
K02169.04  & 9006186    & 132.2252  &$    2.19259 ^{+    0.00003 }_{   -0.00005 }$&$ 1.44  ^{+ 1.29  }_{ -1.13 }$&$ 0.004  ^{+ 0.000  }_{ -0.001 }$&$ 0.73  ^{+ 0.14  }_{ -0.40 }$&$ 1.50  ^{+ 1.17  }_{ -1.32 }$&$ 0.51  \pm{ 0.18  }$&$ 76.83 ^{+ 10.21 }_{ -10.57 }$&$ 6.3   ^{+ 1.8   }_{ -1.6  }$&$ 0.032  \pm{ 0.001  }$&$ 1435  \pm{ 269   }$&$ 18    \pm{ 3     }$& 1.0   & 0.6  &0.040&0.677\\
K02173.01  & 11774991   & 141.1054  &$   37.81526 ^{+    0.00098 }_{   -0.00103 }$&$ 0.39  ^{+ 0.38  }_{ -0.39 }$&$ 0.013  ^{+ 0.003  }_{ -0.000 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.00  ^{+ 1.13  }_{ -0.00 }$&$ 1.16  \pm{ 0.29  }$&$ 89.58 ^{+ 0.42  }_{ -0.60 }$&$ 52.3  ^{+ 11.0  }_{ -9.8  }$&$ 0.200  \pm{ 0.006  }$&$ 434   \pm{ 58    }$&$ 272   \pm{ 21    }$& 5.1   & 0.8  &0.020&0.333\\
K02173.02  & 11774991   & 171.1865  &$   53.57820 ^{+    0.00170 }_{   -0.00251 }$&$ 0.07  ^{+ 0.72  }_{ -0.07 }$&$ 0.012  ^{+ 0.005  }_{ -0.001 }$&$ 0.90  ^{+  0.01 }_{ -0.71 }$&$ 3.82  ^{+ 0.88  }_{ -0.52 }$&$ 1.04  \pm{ 0.35  }$&$ 89.94 ^{+ 0.06  }_{ -0.76 }$&$ 68.7  ^{+ 16.6  }_{ -13.8 }$&$ 0.253  \pm{ 0.007  }$&$ 389   \pm{ 57    }$&$ 280   \pm{ 26    }$& 6.3   & 0.9  &0.015&0.277\\
K02175.01  & 9022166    & 142.1752  &$   26.84734 ^{+    0.00034 }_{   -0.00035 }$&$ 0.00  ^{+ 0.60  }_{ -0.00 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 1.25  }_{ -0.00 }$&$ 1.79  \pm{ 0.59  }$&$ 90.00 ^{+ 0.00  }_{ -1.03 }$&$ 33.9  ^{+ 12.9  }_{ -7.0  }$&$ 0.167  \pm{ 0.009  }$&$ 614   \pm{ 117   }$&$ 259   \pm{ 26    }$& 6.3   & 0.6  &0.086&0.702\\
K02175.02  & 9022166    & 179.5122  &$   72.38130 ^{+    0.00071 }_{   -0.00134 }$&$ 0.25  ^{+ 0.28  }_{ -0.25 }$&$ 0.018  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 1.87  \pm{ 0.50  }$&$ 89.79 ^{+ 0.21  }_{ -0.32 }$&$ 71.0  ^{+ 19.0  }_{ -13.7 }$&$ 0.320  \pm{ 0.016  }$&$ 423   \pm{ 60    }$&$ 364   \pm{ 42    }$& 7.7   & 0.3  &0.087&0.703\\
K02289.01  & 3867615    & 157.3033  &$   62.78500 ^{+    0.00180 }_{   -0.00121 }$&$ 0.76  ^{+ 0.12  }_{ -0.64 }$&$ 0.018  ^{+ 0.001  }_{ -0.005 }$&$ 0.00  ^{+ 0.49  }_{ -0.00 }$&$ 0.00  ^{+ 0.71  }_{ -0.00 }$&$ 2.65  \pm{ 0.82  }$&$ 89.21 ^{+ 0.69  }_{ -0.37 }$&$ 53.7  ^{+ 11.1  }_{ -12.5 }$&$ 0.335  \pm{ 0.015  }$&$ 558   \pm{ 80    }$&$ 358   \pm{ 43    }$& 5.9   & 0.6  &0.038&0.497\\
K02289.02  & 3867615    & 147.2808  &$   20.09846 ^{+    0.00061 }_{   -0.00076 }$&$ 0.14  ^{+ 0.45  }_{ -0.14 }$&$ 0.012  ^{+ 0.001  }_{ -0.003 }$&$ 0.17  ^{+ 0.17  }_{ -0.17 }$&$ 0.58  ^{+  0.07 }_{ -0.58 }$&$ 1.63  \pm{ 0.43  }$&$ 89.69 ^{+ 0.31  }_{ -1.05 }$&$ 25.5  ^{+ 6.2   }_{ -5.1  }$&$ 0.148  \pm{ 0.009  }$&$ 811   \pm{ 110   }$&$ 157   \pm{ 22    }$& 5.3   & 0.4  &0.024&0.380\\
K02311.01  & 4247991    & 294.4400  &$  191.88569 ^{+    0.10191 }_{   -0.03101 }$&$ 0.00  ^{+ 1.00  }_{ -0.00 }$&$ 0.024  ^{+ 0.004  }_{ -0.022 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.09  ^{+ 0.24  }_{ -0.09 }$&$ 3.22  \pm{ 2.86  }$&$ 90.00 ^{+  0.00 }_{ -1.60 }$&$ 120.6 ^{+ 84.8  }_{ -52.3 }$&$ 0.691  \pm{ 0.079  }$&$ 239   \pm{ 42    }$&$ 200     \pm{ 39    }$& 4.8   & 0.5  &0.024&0.379\\
K02311.02  & 4247991    & 145.0410  &$   13.72535 ^{+    0.00072 }_{   -0.00069 }$&$ 0.91  ^{+  0.09 }_{ -0.91 }$&$ 0.010  ^{+ 0.016  }_{ -0.008 }$&$ 0.02  ^{+ 0.00  }_{ -0.02 }$&$ 0.17  ^{+ 0.03  }_{ -0.17 }$&$ 1.38  \pm{ 1.90  }$&$ 81.52 ^{+ 0.68  }_{ -0.58 }$&$ 20.0  ^{+ 13.5  }_{ -8.3  }$&$ 0.119  \pm{ 0.013  }$&$ 514   \pm{ 75    }$&$ 51     \pm{ 15    }$& 7.5   & 0.3  &0.006&0.133\\
K02352.01  & 8013439    & 133.0583  &$   13.39140 ^{+    0.00057 }_{   -0.00034 }$&$ 0.68  ^{+ 0.13  }_{ -0.05 }$&$ 0.010  ^{+ 0.027  }_{ -0.002 }$&$ 0.53  ^{+ 0.18  }_{ -0.14 }$&$ 4.43  ^{+ 0.26  }_{ -0.66 }$&$ 3.37  \pm{ 5.00  }$&$ 85.30 ^{+ 0.84  }_{ -1.00 }$&$ 8.2   ^{+ 1.4   }_{ -0.7  }$&$ 0.119  \pm{ 0.018  }$&$ 1522  \pm{ 215   }$&$ 50    \pm{ 4     }$& 4.3   & 0.8  &0.049&0.720\\
K02352.02  & 8013439    & 134.7477  &$    5.62903 ^{+    0.00012 }_{   -0.00010 }$&$ 0.32  ^{+ 0.29  }_{ -0.32 }$&$ 0.005  ^{+ 0.001  }_{ -0.000 }$&$ 0.01  ^{+ 0.22  }_{ -0.01 }$&$ 0.01  ^{+ 0.91  }_{ -0.01 }$&$ 0.84  \pm{ 0.27  }$&$ 87.98 ^{+ 2.02  }_{ -2.45 }$&$ 8.7   ^{+ 2.4   }_{ -2.2  }$&$ 0.065  \pm{ 0.005  }$&$ 1467  \pm{ 229   }$&$ 38    \pm{ 2     }$& 4.5   & 0.4  &0.060&0.761\\
K02352.03  & 8013439    & 137.9280  &$    8.25621 ^{+    0.00023 }_{   -0.00028 }$&$ 0.87  ^{+ 0.06  }_{ -0.10 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 3.83  ^{+  1.69 }_{ -3.83 }$&$ 1.27  \pm{ 0.30  }$&$ 85.87 ^{+ 0.77  }_{ -0.88 }$&$ 11.7  ^{+ 1.9   }_{ -2.0  }$&$ 0.083  \pm{ 0.007  }$&$ 1261  \pm{ 147   }$&$ 37    \pm{ 3     }$& 2.6   & 1.9  &0.050&0.724\\
K02541.01  & 12306058   & 137.9603  &$    7.41682 ^{+    0.00030 }_{   -0.00026 }$&$ 0.41  ^{+ 0.26  }_{ -0.34 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.01  ^{+ 0.36  }_{ -0.01 }$&$ 2.40  \pm{ 0.53  }$&$ 86.31 ^{+ 3.16  }_{ -2.30 }$&$ 5.6   ^{+ 1.5   }_{ -0.3  }$&$ 0.079  \pm{ 0.002  }$&$ 1376  \pm{ 174   }$&$ 78    \pm{ 12    }$& 8.3   & 0.4  &0.188&0.853\\
K02541.02  & 12306058   & 146.9230  &$   20.48565 ^{+    0.00148 }_{   -0.00123 }$&$ 0.23  ^{+ 0.46  }_{ -0.23 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.43  ^{+ 0.02  }_{ -0.43 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 2.84  \pm{ 0.97  }$&$ 88.97 ^{+ 1.02  }_{ -2.05 }$&$ 11.3  ^{+ 3.5   }_{ -1.4  }$&$ 0.160  \pm{ 0.028  }$&$ 973   \pm{ 133   }$&$ 93    \pm{ 20    }$& 11.1  & 0.3  &0.188&0.853\\
K02585.01  & 7673841    & 136.3069  &$    5.34189 ^{+    0.00018 }_{   -0.00017 }$&$ 0.92  ^{+ 0.87  }_{ -0.07 }$&$ 0.009  ^{+ 0.010  }_{ -0.002 }$&$ 0.03  ^{+ 0.07  }_{ -0.03 }$&$ 0.33  ^{+ 0.21  }_{ -0.33 }$&$ 2.25  \pm{ 1.68  }$&$ 81.02 ^{+ 0.16  }_{ -1.70 }$&$ 6.2   ^{+ 3.6   }_{ -1.1  }$&$ 0.066  \pm{ 0.003  }$&$ 1778  \pm{ 405   }$&$ 67    \pm{ 8     }$& 3.1   & 0.7  &0.073&0.797\\
K02585.02  & 7673841    & 135.1572  &$   10.42305 ^{+    0.00027 }_{   -0.00032 }$&$ 0.73  ^{+ 0.18  }_{ -0.27 }$&$ 0.008  ^{+ 0.003  }_{ -0.003 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.00  ^{+ 0.88  }_{ -0.00 }$&$ 1.30  \pm{ 0.51  }$&$ 87.22 ^{+ 1.15  }_{ -0.95 }$&$ 14.1  ^{+ 3.1   }_{ -2.9  }$&$ 0.096  \pm{ 0.006  }$&$ 1106  \pm{ 158   }$&$ 73    \pm{ 11    }$& 3.6   & 0.5  &0.066&0.779\\
K02585.03  & 7673841    & 138.5965  &$    7.87811 ^{+    0.00025 }_{   -0.00025 }$&$ 0.88  ^{+ 0.62  }_{ -0.44 }$&$ 0.008  ^{+ 0.020  }_{ -0.003 }$&$ 0.66  ^{+  0.01 }_{ -0.66 }$&$ 3.93  ^{+ 0.59  }_{ -3.89 }$&$ 1.27  \pm{ 1.95  }$&$ 85.72 ^{+ 2.23  }_{ -2.82 }$&$ 11.0  ^{+ 2.9   }_{ -2.4  }$&$ 0.080  \pm{ 0.006  }$&$ 1255  \pm{ 205   }$&$ 47    \pm{ 10    }$& 2.7   & 0.2  &0.017&0.463\\
K02595.01  & 8883329    & 134.0478  &$    9.18252 ^{+    0.00029 }_{   -0.00033 }$&$ 1.00  ^{+ 0.03  }_{ -0.34 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.33  ^{+ 0.32  }_{ -0.33 }$&$ 0.65  ^{+ 0.00  }_{ -0.65 }$&$ 2.50  \pm{ 0.60  }$&$ 83.05 ^{+ 2.94  }_{ -0.60 }$&$ 8.3   ^{+ 1.7   }_{ -1.2  }$&$ 0.098  \pm{ 0.003  }$&$ 1558  \pm{ 167   }$&$ 85    \pm{ 10    }$& 4.6   & 0.1  &0.111&0.758\\
K02595.02  & 8883329    & 140.4080  &$   14.61360 ^{+    0.00076 }_{   -0.00084 }$&$ 0.88  ^{+ 0.57  }_{ -0.12 }$&$ 0.010  ^{+ 0.004  }_{ -0.002 }$&$ 0.17  ^{+  0.04 }_{ -0.17 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 2.55  \pm{ 1.05  }$&$ 85.73 ^{+ 0.46  }_{ -1.13 }$&$ 12.1  ^{+ 4.2   }_{ -2.4  }$&$ 0.134  \pm{ 0.004  }$&$ 1299  \pm{ 223   }$&$ 81    \pm{ 13    }$& 5.0   & 0.8  &0.159&0.826\\
K02672.01  & 11253827   & 182.6526  &$   88.51658 ^{+    0.00020 }_{   -0.00016 }$&$ 0.52  ^{+ 0.28  }_{ -0.52 }$&$ 0.044  ^{+ 0.008  }_{ -0.001 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.00  ^{+ 0.69  }_{ -0.00 }$&$ 5.34  \pm{ 1.48  }$&$ 89.61 ^{+ 0.39  }_{ -0.37 }$&$ 71.9  ^{+ 18.1  }_{ -16.5 }$&$ 0.374  \pm{ 0.010  }$&$ 425   \pm{ 60    }$&$ 2611  \pm{ 35    }$& 8.1   & 0.3  &0.847&0.993\\
K02672.02  & 11253827   & 162.5118  &$   42.99066 ^{+    0.00009 }_{   -0.00014 }$&$ 0.65  ^{+ 0.25  }_{ -0.65 }$&$ 0.032  ^{+ 0.002  }_{ -0.003 }$&$ 0.01  ^{+ 0.62  }_{ -0.01 }$&$ 0.00  ^{+ 1.01  }_{ -0.00 }$&$ 3.89  \pm{ 1.03  }$&$ 89.22 ^{+ 0.78  }_{ -0.69 }$&$ 43.6  ^{+ 11.8  }_{ -9.1  }$&$ 0.231  \pm{ 0.006  }$&$ 536   \pm{ 78    }$&$ 1162  \pm{ 17    }$& 5.5   & 0.3  &0.895&0.995\\
K02674.01  & 8022489    & 272.3869  &$  197.51031 ^{+    0.00035 }_{   -0.00032 }$&$ 0.82  ^{+ 0.58  }_{ -0.32 }$&$ 0.052  ^{+ 0.001  }_{ -0.006 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.00  ^{+ 0.94  }_{ -0.00 }$&$ 10.05 \pm{ 3.96  }$&$ 89.46 ^{+ 0.30  }_{ -0.81 }$&$ 83.8  ^{+ 33.0  }_{ -27.5 }$&$ 0.671  \pm{ 0.021  }$&$ 422   \pm{ 77    }$&$ 2643  \pm{ 58    }$& 10.9  & 0.8  &0.369&0.967\\
K02674.02  & 8022489    & 140.0090  &$   11.17265 ^{+    0.00061 }_{   -0.00066 }$&$ 1.08  ^{+ 4.19  }_{ -0.42 }$&$ 0.009  ^{+ 0.036  }_{ -0.000 }$&$ 0.24  ^{+  0.17 }_{ -0.23 }$&$ 1.58  ^{+  1.16 }_{ -1.50 }$&$ 1.57  \pm{ 3.22  }$&$ 81.42 ^{+ 0.07  }_{ -1.48 }$&$ 13.4  ^{+ 7.5   }_{ -4.4  }$&$ 0.099  \pm{ 0.003  }$&$ 1473  \pm{ 1376  }$&$ 80    \pm{ 13    }$& 5.5   & 0.4  &0.079&0.810\\
K02674.03  & 8022489    & 133.0107  &$    2.53574 ^{+    0.00006 }_{   -0.00006 }$&$ 0.91  ^{+ 0.34  }_{ -0.91 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.51  ^{+ 0.35  }_{ -0.46 }$&$ 0.72  ^{+ 1.44  }_{ -0.63 }$&$ 2.15  \pm{ 0.60  }$&$ 73.54 ^{+ 16.44 }_{ -7.31 }$&$ 3.4   ^{+ 1.3   }_{ -0.7  }$&$ 0.037  \pm{ 0.001  }$&$ 2216  \pm{ 385   }$&$ 73    \pm{ 6     }$& 15.7  & 0.7  &0.038&0.664\\
K02675.01  & 5794570    & 132.4894  &$    5.44833 ^{+    0.00002 }_{   -0.00002 }$&$ 0.59  ^{+ 0.23  }_{ -0.40 }$&$ 0.021  ^{+ 0.006  }_{ -0.002 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 1.86  }_{ -0.00 }$&$ 2.21  \pm{ 0.68  }$&$ 87.45 ^{+ 1.89  }_{ -2.32 }$&$ 13.4  ^{+ 2.2   }_{ -3.0  }$&$ 0.061  \pm{ 0.003  }$&$ 1037  \pm{ 130   }$&$ 554   \pm{ 6     }$& 2.6   & 1.7  &0.796&0.990\\
K02675.02  & 5794570    & 131.8464  &$    1.11613 ^{+    0.00001 }_{   -0.00001 }$&$ 0.57  ^{+ 0.37  }_{ -0.49 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.10  ^{+ 0.58  }_{ -0.10 }$&$ 0.00  ^{+ 2.48  }_{ -0.00 }$&$ 1.05  \pm{ 0.29  }$&$ 82.17 ^{+ 6.90  }_{ -10.33 }$&$ 4.2   ^{+ 0.9   }_{ -0.9  }$&$ 0.021  \pm{ 0.001  }$&$ 1856  \pm{ 235   }$&$ 106   \pm{ 2     }$& 1.7   & 1.8  &0.112&0.760\\
K02687.01  & 7202957    & 132.0299  &$    1.71684 ^{+    0.00001 }_{   -0.00001 }$&$ 0.99  ^{+  0.01 }_{ -0.12 }$&$ 0.010  ^{+ 0.001  }_{ -0.002 }$&$ 0.05  ^{+ 0.14  }_{ -0.05 }$&$ 1.19  ^{+  0.36 }_{ -1.19 }$&$ 3.31  \pm{ 0.92  }$&$ 62.19 ^{+ 11.67 }_{ -0.76 }$&$ 2.1   ^{+ 1.0   }_{ -0.1  }$&$ 0.029  \pm{ 0.001  }$&$ 2648  \pm{ 363   }$&$ 62    \pm{ 1     }$& 2.5   &\textbf{ 4.3  }&0.470&0.957\\
K02687.02  & 7202957    & 136.2009  &$    8.16739 ^{+    0.00007 }_{   -0.00007 }$&$ 0.94  ^{+ 0.02  }_{ -0.05 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 3.69  \pm{ 0.73  }$&$ 82.00 ^{+ 2.06  }_{ -1.53 }$&$ 6.3   ^{+ 1.9   }_{ -0.6  }$&$ 0.082  \pm{ 0.003  }$&$ 1485  \pm{ 152   }$&$ 104   \pm{ 3     }$& 3.6   & 2.7  &0.420&0.948\\
K02693.01  & 5185897    & 133.8593  &$    4.08141 ^{+    0.00007 }_{   -0.00006 }$&$ 0.22  ^{+ 0.16  }_{ -0.22 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.85  \pm{ 0.17  }$&$ 89.05 ^{+ 0.95  }_{ -0.83 }$&$ 12.9  ^{+ 2.0   }_{ -1.7  }$&$ 0.044  \pm{ 0.002  }$&$ 823   \pm{ 69    }$&$ 156   \pm{ 6     }$& 2.4   & 2.0  &0.054&0.739\\
K02693.02  & 5185897    & 142.1177  &$   11.41942 ^{+    0.00034 }_{   -0.00045 }$&$ 0.89  ^{+ 0.04  }_{ -0.23 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.68  }_{ -0.00 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 2.16  \pm{ 0.61  }$&$ 86.01 ^{+ 1.43  }_{ -0.85 }$&$ 14.4  ^{+ 3.5   }_{ -2.5  }$&$ 0.098  \pm{ 0.018  }$&$ 826   \pm{ 97    }$&$ 158   \pm{ 11    }$& 3.3   & 1.4  &0.030&0.607\\
K02693.03  & 5185897    & 136.8490  &$    6.83448 ^{+    0.00011 }_{   -0.00015 }$&$ 0.37  ^{+ 0.20  }_{ -0.37 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.78  \pm{ 0.17  }$&$ 88.98 ^{+ 1.02  }_{ -0.73 }$&$ 20.0  ^{+ 4.0   }_{ -2.8  }$&$ 0.062  \pm{ 0.002  }$&$ 652   \pm{ 63    }$&$ 153   \pm{ 8     }$& 2.4   & 1.3  &0.034&0.638\\
K02696.01  & 11071200   & 214.7486  &$   96.45620 ^{+    0.00041 }_{   -0.00057 }$&$ 0.65  ^{+ 0.16  }_{ -0.65 }$&$ 0.030  ^{+ 0.006  }_{ -0.000 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 4.69  }_{ -0.00 }$&$ 6.63  \pm{ 1.78  }$&$ 89.26 ^{+ 0.74  }_{ -0.50 }$&$ 50.6  ^{+ 11.6  }_{ -10.4 }$&$ 0.485  \pm{ 0.021  }$&$ 653   \pm{ 90    }$&$ 978   \pm{ 73    }$& 11.4  & 0.5  &0.095&0.723\\
K02696.02  & 11071200   & 143.4267  &$   44.56505 ^{+    0.00018 }_{   -0.00012 }$&$ 0.52  ^{+ 0.22  }_{ -0.52 }$&$ 0.016  ^{+ 0.003  }_{ -0.002 }$&$ 0.36  ^{+ 0.14  }_{ -0.36 }$&$ 0.16  ^{+ 0.27  }_{ -0.16 }$&$ 3.56  \pm{ 1.16  }$&$ 89.08 ^{+ 0.92  }_{ -0.82 }$&$ 29.9  ^{+ 9.1   }_{ -6.8  }$&$ 0.290  \pm{ 0.013  }$&$ 824   \pm{ 140   }$&$ 366   \pm{ 37    }$& 8.6   & 0.8  &0.192&0.856\\
K02714.01  & 12206313   & 140.5597  &$   14.38351 ^{+    0.00023 }_{   -0.00022 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.012  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 2.63  \pm{ 0.71  }$&$ 90.00 ^{+ 0.00  }_{ -1.25 }$&$ 13.6  ^{+ 4.2   }_{ -2.3  }$&$ 0.125  \pm{ 0.004  }$&$ 1146  \pm{ 157   }$&$ 191   \pm{ 16    }$& 8.2   & 1.5  &0.139&0.802\\
K02714.02  & 12206313   & 170.0987  &$   47.31319 ^{+    0.00058 }_{   -0.00059 }$&$ 0.00  ^{+ 0.64  }_{ -0.00 }$&$ 0.014  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 2.78  \pm{ 0.80  }$&$ 90.00 ^{+  0.00 }_{ -1.14 }$&$ 32.1  ^{+ 9.8   }_{ -6.4  }$&$ 0.276  \pm{ 0.009  }$&$ 728   \pm{ 109   }$&$ 256   \pm{ 30    }$& 10.9  & 0.9  &0.180&0.846\\
K02722.01  & 7673192    & 134.9353  &$    6.12482 ^{+    0.00013 }_{   -0.00013 }$&$ 0.33  ^{+ 0.24  }_{ -0.33 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 1.55  \pm{ 0.35  }$&$ 88.31 ^{+ 1.69  }_{ -1.62 }$&$ 10.8  ^{+ 1.9   }_{ -1.7  }$&$ 0.072  \pm{ 0.003  }$&$ 1301  \pm{ 124   }$&$ 147   \pm{ 8     }$& 4.0   & 1.5  &0.100&0.847\\
K02722.02  & 7673192    & 136.3216  &$   11.24280 ^{+    0.00031 }_{   -0.00034 }$&$ 0.54  ^{+ 0.11  }_{ -0.54 }$&$ 0.011  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 1.69  \pm{ 0.42  }$&$ 88.18 ^{+ 1.82  }_{ -0.56 }$&$ 16.6  ^{+ 3.0   }_{ -3.1  }$&$ 0.108  \pm{ 0.005  }$&$ 1048  \pm{ 111   }$&$ 142   \pm{ 11    }$& 4.3   & 0.5  &0.076&0.803\\
K02722.03  & 7673192    & 133.7748  &$    4.02871 ^{+    0.00008 }_{   -0.00009 }$&$ 0.39  ^{+ 0.26  }_{ -0.39 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.03  ^{+ 0.70  }_{ -0.03 }$&$ 1.32  \pm{ 0.34  }$&$ 87.23 ^{+ 2.77  }_{ -2.61 }$&$ 7.8   ^{+ 1.6   }_{ -1.4  }$&$ 0.054  \pm{ 0.003  }$&$ 1532  \pm{ 163   }$&$ 102   \pm{ 6     }$& 3.6   & 0.5  &0.026&0.568\\
K02722.04  & 7673192    & 137.4936  &$    8.92108 ^{+    0.00031 }_{   -0.00029 }$&$ 0.54  ^{+ 0.11  }_{ -0.54 }$&$ 0.010  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 1.51  \pm{ 0.40  }$&$ 87.91 ^{+ 2.09  }_{ -0.74 }$&$ 14.2  ^{+ 2.8   }_{ -2.8  }$&$ 0.092  \pm{ 0.005  }$&$ 1125  \pm{ 135   }$&$ 115   \pm{ 10    }$& 3.9   & 1.6  &0.074&0.799\\
K02722.05  & 7673192    & 135.3861  &$   16.53433 ^{+    0.00087 }_{   -0.00104 }$&$ 0.37  ^{+ 0.29  }_{ -0.37 }$&$ 0.008  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 1.04  \pm{ 0.31  }$&$ 89.12 ^{+ 0.88  }_{ -0.91 }$&$ 22.7  ^{+ 5.3   }_{ -5.0  }$&$ 0.130  \pm{ 0.009  }$&$ 881   \pm{ 129   }$&$ 96    \pm{ 14    }$& 4.9   & 0.5  &0.015&0.432\\
K02732.01  & 9886361    & 134.4527  &$    7.03142 ^{+    0.00023 }_{   -0.00027 }$&$ 0.98  ^{+ 0.05  }_{ -0.07 }$&$ 0.014  ^{+  0.003 }_{ -0.004 }$&$ 0.16  ^{+ 0.07  }_{ -0.08 }$&$ 1.39  ^{+ 0.39  }_{ -1.38 }$&$ 9.16  \pm{ 0.75  }$&$ 76.51 ^{+ 0.75  }_{ -0.33 }$&$ 4.1   ^{+ 0.2   }_{ -0.0  }$&$ 0.116  \pm{ 0.005  }$&$ 2034  \pm{ 30    }$&$ 140   \pm{ 7     }$& 6.6   & 0.2  &0.035&0.646\\
K02732.02  & 9886361    & 144.1688  &$   13.61163 ^{+    0.00041 }_{   -0.00044 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 1.81  \pm{ 0.75  }$&$ 90.00 ^{+ 0.00  }_{ -2.02 }$&$ 13.5  ^{+ 5.9   }_{ -3.8  }$&$ 0.116  \pm{ 0.012  }$&$ 1111  \pm{ 236   }$&$ 96    \pm{ 10    }$& 7.4   & 0.2  &0.035&0.643\\
K02732.03  & 9886361    & 140.7182  &$   54.28085 ^{+    0.00238 }_{   -0.00179 }$&$ 0.66  ^{+ 0.22  }_{ -0.52 }$&$ 0.011  ^{+ 0.002  }_{ -0.003 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.00  ^{+ 0.63  }_{ -0.00 }$&$ 1.93  \pm{ 1.15  }$&$ 89.20 ^{+ 0.69  }_{ -0.56 }$&$ 42.6  ^{+ 18.9  }_{ -15.3 }$&$ 0.318  \pm{ 0.034  }$&$ 610   \pm{ 155   }$&$ 157   \pm{ 21    }$& 6.7   & 0.5  &0.113&0.864\\
K02732.04  & 9886361    & 146.8040  &$   24.56084 ^{+    0.00009 }_{   -0.00181 }$&$ 0.12  ^{+ 0.77  }_{ -0.12 }$&$ 0.007  ^{+ 0.001  }_{ -0.002 }$&$ 0.01  ^{+ 0.56  }_{ -0.01 }$&$ 0.00  ^{+ 3.81  }_{ -0.00 }$&$ 1.16  \pm{ 0.57  }$&$ 89.76 ^{+ 0.24  }_{ -1.56 }$&$ 25.9  ^{+ 12.4  }_{ -8.5  }$&$ 0.171  \pm{ 0.014  }$&$ 779   \pm{ 220   }$&$ 60    \pm{ 13    }$& 6.5   & 1.0  &0.035&0.643\\
K02949.01  & 6026737    & 132.3611  &$   10.17444 ^{+    0.00045 }_{   -0.00056 }$&$ 0.70  ^{+ 1.07  }_{ -0.01 }$&$ 0.013  ^{+ 0.016  }_{ -0.007 }$&$ 0.35  ^{+ 0.21  }_{ -0.30 }$&$ 4.48  ^{+ 0.20  }_{ -3.49 }$&$ 3.08  \pm{ 2.83  }$&$ 83.82 ^{+ 1.40  }_{ -1.63 }$&$ 9.8   ^{+ 3.4   }_{ -2.2  }$&$ 0.096  \pm{ 0.003  }$&$ 1600  \pm{ 614   }$&$ 74    \pm{ 12    }$& 6.6   & 0.6  &0.076&0.673\\
K02949.02  & 6026737    & 134.8168  &$    3.75017 ^{+    0.00000 }_{   -0.00000 }$&$ 0.63  ^{+ 0.28  }_{ -0.23 }$&$ 0.005  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.04  ^{+ 0.53  }_{ -0.04 }$&$ 1.13  \pm{ 0.41  }$&$ 83.41 ^{+ 2.39  }_{ -2.76 }$&$ 5.2   ^{+ 1.4   }_{ -1.1  }$&$ 0.049  \pm{ 0.005  }$&$ 1747  \pm{ 274   }$&$ 32    \pm{ 7     }$& 4.1   & 1.4  &0.023&0.368\\
K03083.01  & 7106173    & 133.2040  &$   10.18329 ^{+    0.00044 }_{   -0.00043 }$&$ 0.98  ^{+ 1.51  }_{ -0.08 }$&$ 0.007  ^{+ 0.025  }_{ -0.002 }$&$ 0.21  ^{+  0.15 }_{ -0.21 }$&$ 0.40  ^{+  0.09 }_{ -0.40 }$&$ 0.82  \pm{ 1.58  }$&$ 85.63 ^{+ 0.38  }_{ -1.30 }$&$ 19.3  ^{+ 5.6   }_{ -5.5  }$&$ 0.096  \pm{ 0.004  }$&$ 1095  \pm{ 353   }$&$ 50    \pm{ 9     }$& 2.8   & 0.7  &0.014&0.409\\
K03083.02  & 7106173    & 135.2410  &$    6.23203 ^{+    0.00023 }_{   -0.00025 }$&$ 0.89  ^{+ 1.32  }_{ -0.05 }$&$ 0.006  ^{+ 0.025  }_{ -0.003 }$&$ 0.05  ^{+  0.00 }_{ -0.05 }$&$ 6.21  ^{+  0.07 }_{ -6.20 }$&$ 0.64  \pm{ 1.61  }$&$ 84.34 ^{+ 0.46  }_{ -1.06 }$&$ 14.0  ^{+ 3.9   }_{ -3.4  }$&$ 0.069  \pm{ 0.003  }$&$ 1307  \pm{ 436   }$&$ 29    \pm{ 7     }$& 2.4   & 0.6  &0.014&0.408\\
K03083.03  & 7106173    & 134.8440  &$    8.29442 ^{+    0.00047 }_{   -0.00033 }$&$ 0.46  ^{+ 0.42  }_{ -0.46 }$&$ 0.006  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 0.65  \pm{ 0.20  }$&$ 88.51 ^{+ 1.49  }_{ -1.31 }$&$ 16.8  ^{+ 4.5   }_{ -3.3  }$&$ 0.084  \pm{ 0.004  }$&$ 931   \pm{ 150   }$&$ 34    \pm{ 8     }$& 3.2   & 0.3  &0.013&0.399\\
K03097.01  & 7582689    & 137.4610  &$   11.92196 ^{+    0.00069 }_{   -0.00060 }$&$ 0.77  ^{+ 1.13  }_{ -0.12 }$&$ 0.007  ^{+ 0.018  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 1.81  \pm{ 2.53  }$&$ 85.86 ^{+  1.79 }_{ -3.30 }$&$ 9.9   ^{+ 4.0   }_{ -2.5  }$&$ 0.108  \pm{ 0.003  }$&$ 1281  \pm{ 249   }$&$ 51    \pm{ 8     }$& 5.5   & 0.4  &0.092&0.835\\
K03097.02  & 7582689    & 138.0420  &$    6.80273 ^{+    0.00027 }_{   -0.00029 }$&$ 0.04  ^{+ 1.56  }_{ -0.50 }$&$ 0.005  ^{+ 0.034  }_{ -0.001 }$&$ 0.38  ^{+ 0.50  }_{ -0.12 }$&$ 0.22  ^{+ 4.53  }_{ -3.52 }$&$ 1.10  \pm{ 3.81  }$&$ 89.74 ^{+  0.26 }_{ -8.58 }$&$ 8.0   ^{+ 2.2   }_{ -2.1  }$&$ 0.074  \pm{ 0.002  }$&$ 1352  \pm{ 231   }$&$ 31    \pm{ 6     }$& 4.7   & 0.4  &0.028&0.589\\
K03097.03  & 7582689    & 140.1620  &$    8.70295 ^{+    0.00036 }_{   -0.00039 }$&$ 0.81  ^{+ 0.45  }_{ -0.19 }$&$ 0.005  ^{+ 0.006  }_{ -0.002 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 2.67  ^{+  0.20 }_{ -2.66 }$&$ 1.27  \pm{ 0.98  }$&$ 85.10 ^{+ 0.58  }_{ -1.26 }$&$ 8.8   ^{+ 2.4   }_{ -1.7  }$&$ 0.088  \pm{ 0.003  }$&$ 1358  \pm{ 215   }$&$ 26    \pm{ 7     }$& 4.2   & 0.6  &0.028&0.589\\
K03111.01  & 8581240    & 138.5101  &$   10.76792 ^{+    0.00044 }_{   -0.00054 }$&$ 0.90  ^{+ 0.25  }_{ -0.18 }$&$ 0.009  ^{+ 0.003  }_{ -0.002 }$&$ 0.13  ^{+ 0.36  }_{ -0.13 }$&$ 1.84  ^{+ 2.49  }_{ -1.83 }$&$ 2.17  \pm{ 0.79  }$&$ 84.61 ^{+ 0.88  }_{ -1.09 }$&$ 9.4   ^{+ 1.7   }_{ -1.9  }$&$ 0.101  \pm{ 0.004  }$&$ 1297  \pm{ 159   }$&$ 67    \pm{ 9     }$& 4.8   & 0.6  &0.056&0.597\\
K03111.02  & 8581240    & 132.5113  &$    4.32854 ^{+    0.00010 }_{   -0.00014 }$&$ 1.00  ^{+  0.00}_{ -1.00 }$&$ 0.006  ^{+ 0.000  }_{ -0.001 }$&$ 0.90  ^{+ 0.00  }_{ -0.08 }$&$ 1.20  ^{+ 0.27  }_{ -0.40 }$&$ 1.54  \pm{ 0.45  }$&$ 62.05 ^{+ 27.57 }_{ -2.59 }$&$ 4.9   ^{+ 1.7   }_{ -1.1  }$&$ 0.055  \pm{ 0.002  }$&$ 1757  \pm{ 295   }$&$ 40    \pm{ 6     }$& 2.2   & 0.8  &0.011&0.217\\
K03158.01  & 6278762    & 133.2591  &$    3.60011 ^{+    0.00003 }_{   -0.00003 }$&$ 0.21  ^{+ 0.33  }_{ -0.21 }$&$ 0.004  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.38  \pm{ 0.04  }$&$ 88.97 ^{+ 1.03  }_{ -1.91 }$&$ 11.7  ^{+ 0.8   }_{ -0.6  }$&$ 0.044  \pm{ 0.001  }$&$ 997   \pm{ 57	 }$&$ 27    \pm{ 1     }$& 2.3   & 2.6  &0.126&0.878\\
K03158.02  & 6278762    & 131.5239  &$    4.54586 ^{+    0.00003 }_{   -0.00004 }$&$ 0.37  ^{+ 0.27  }_{ -0.30 }$&$ 0.006  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.49  \pm{ 0.06  }$&$ 88.44 ^{+ 1.26  }_{ -1.19 }$&$ 13.7  ^{+ 1.0   }_{ -0.7  }$&$ 0.051  \pm{ 0.001  }$&$ 917   \pm{ 47	 }$&$ 47    \pm{ 1     }$& 2.4   & \textbf{ 8.5  }  &0.243&0.941\\
K03158.03  & 6278762    & 134.7885  &$    6.18936 ^{+    0.00007 }_{   -0.00008 }$&$ 0.40  ^{+ 0.27  }_{ -0.40 }$&$ 0.006  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 0.49  \pm{ 0.07  }$&$ 88.63 ^{+ 1.37  }_{ -1.32 }$&$ 16.9  ^{+ 0.9   }_{ -1.0  }$&$ 0.063  \pm{ 0.001  }$&$ 827   \pm{ 56	 }$&$ 45    \pm{ 1     }$& 2.6   & 0.7  &0.227&0.936\\
K03158.04  & 6278762    & 135.0872  &$    7.74359 ^{+    0.00011 }_{   -0.00011 }$&$ 0.91  ^{+ 0.07  }_{ -0.05 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.05  ^{+ 0.17  }_{ -0.05 }$&$ 0.07  ^{+ 1.09  }_{ -0.07 }$&$ 1.84  \pm{ 0.32  }$&$ 83.71 ^{+ 0.86  }_{ -0.92 }$&$ 8.1   ^{+ 1.1   }_{ -1.0  }$&$ 0.080  \pm{ 0.004  }$&$ 1173  \pm{ 86	 }$&$ 51    \pm{ 1     }$& 3.1   & 2.1  &0.190&0.921\\
K03158.05  & 6278762    & 134.8777  &$    9.74050 ^{+    0.00004 }_{   -0.00005 }$&$ 0.77  ^{+ 0.07  }_{ -0.15 }$&$ 0.009  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.06  ^{+ 1.53  }_{ -0.06 }$&$ 0.76  \pm{ 0.11  }$&$ 88.11 ^{+ 0.46  }_{ -0.36 }$&$ 23.0  ^{+ 1.7   }_{ -1.2  }$&$ 0.084  \pm{ 0.002  }$&$ 699   \pm{ 39	 }$&$ 74    \pm{ 1     }$& 2.1   & 1.1  &0.287&0.953\\
K03196.01  & 9002538    & 135.3143  &$    4.96067 ^{+    0.00016 }_{   -0.00013 }$&$ 0.43  ^{+ 0.26  }_{ -0.40 }$&$ 0.004  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.27  ^{+ 2.36  }_{ -0.27 }$&$ 0.51  \pm{ 0.10  }$&$ 87.67 ^{+ 2.14  }_{ -1.58 }$&$ 10.7  ^{+ 0.7   }_{ -1.0  }$&$ 0.058  \pm{ 0.003  }$&$ 1316  \pm{ 126   }$&$ 23    \pm{ 3     }$& 3.2   & 0.8  &0.029&0.426\\
K03196.02  & 9002538    & 134.1634  &$    6.88299 ^{+    0.00021 }_{   -0.00018 }$&$ 0.96  ^{+ 1.19  }_{ -0.30 }$&$ 0.009  ^{+ 0.025  }_{ -0.007 }$&$ 0.00  ^{+ 0.06  }_{ -0.01 }$&$ 0.48  ^{+  0.02 }_{ -0.42 }$&$ 1.14  \pm{ 2.03  }$&$ 80.65 ^{+ 1.86  }_{ -0.47 }$&$ 13.2  ^{+ 0.8   }_{ -1.7  }$&$ 0.072  \pm{ 0.004  }$&$ 1773  \pm{ 898   }$&$ 29    \pm{ 3     }$& 2.8   & 1.5  &0.034&0.471\\
K03384.01  & 8644365    & 139.0648  &$   10.54837 ^{+    0.00018 }_{   -0.00013 }$&$ 0.79  ^{+ 0.15  }_{ -0.16 }$&$ 0.009  ^{+ 0.006  }_{ -0.002 }$&$ 0.10  ^{+ 0.37  }_{ -0.10 }$&$ 0.06  ^{+ 4.61  }_{ -0.06 }$&$ 1.10  \pm{ 0.51  }$&$ 87.61 ^{+ 0.64  }_{ -1.04 }$&$ 18.4  ^{+ 2.8   }_{ -2.1  }$&$ 0.094  \pm{ 0.004  }$&$ 930   \pm{ 125   }$&$ 82    \pm{ 11    }$& 2.7   & 1.3  &0.086&0.701\\
K03384.02  & 8644365    & 139.3678  &$   19.91594 ^{+    0.00000 }_{   -0.04764 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.011  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.00  ^{+ 0.82  }_{ -0.00 }$&$ 1.41  \pm{ 0.25  }$&$ 90.00 ^{+  0.00 }_{ -1.15 }$&$ 27.2  ^{+ 2.3   }_{ -3.5  }$&$ 0.145  \pm{ 0.008  }$&$ 781   \pm{ 97	 }$&$ 150   \pm{ 16    }$& 5.6   & 0.9  &0.086&0.701\\
K03398.01  & 3561464    & 137.2253  &$    7.31947 ^{+    0.00017 }_{   -0.00027 }$&$ 0.00  ^{+ 0.47  }_{ -0.00 }$&$ 0.012  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+  0.01 }_{ -0.00 }$&$ 1.51  \pm{ 0.28  }$&$ 90.00 ^{+ 0.00  }_{ -2.27 }$&$ 13.8  ^{+ 1.1   }_{ -2.1  }$&$ 0.074  \pm{ 0.004  }$&$ 1197  \pm{ 138   }$&$ 149   \pm{ 19    }$& 4.2   & 0.1  &0.051&0.731\\
K03398.02  & 3561464    & 144.9642  &$   35.79896 ^{+    0.00005 }_{   -0.00004 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.022  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 2.79  \pm{ 0.55  }$&$ 90.00 ^{+ 0.00  }_{ -0.82 }$&$ 39.7  ^{+ 3.2   }_{ -5.7  }$&$ 0.213  \pm{ 0.013  }$&$ 688   \pm{ 86	 }$&$ 561   \pm{ 50    }$& 7.0   & 0.3  &0.078&0.809\\
K03398.03  & 3561464    & 131.6023  &$    4.32702 ^{+    0.00014 }_{   -0.00015 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.23  \pm{ 0.25  }$&$ 90.00 ^{+ 0.00  }_{ -1.94 }$&$ 9.8   ^{+ 0.9   }_{ -1.3  }$&$ 0.052  \pm{ 0.003  }$&$ 1417  \pm{ 171   }$&$ 98    \pm{ 14    }$& 3.5   & 0.7  &0.015&0.434\\
K03403.01  & 11754430   & 166.6626  &$   39.81811 ^{+    0.00058 }_{   -0.00064 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 1.73  \pm{ 0.36  }$&$ 90.00 ^{+ 0.00  }_{ -0.95 }$&$ 43.4  ^{+ 5.7   }_{ -7.2  }$&$ 0.229  \pm{ 0.012  }$&$ 635   \pm{ 97	 }$&$ 237   \pm{ 28    }$& 7.4   & 0.4  &0.105&0.745\\
K03403.02  & 11754430   & 135.4936  &$    6.15844 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.89  \pm{ 0.19  }$&$ 90.00 ^{+ 0.00  }_{ -1.89 }$&$ 12.5  ^{+ 1.6   }_{ -1.6  }$&$ 0.066  \pm{ 0.003  }$&$ 1151  \pm{ 169   }$&$ 51    \pm{ 10    }$& 3.8   & 0.1  &0.032&0.449\\
K03425.01  & 9117416    & 145.4378  &$   20.03515 ^{+    0.00078 }_{   -0.00063 }$&$ 0.26  ^{+ 0.43  }_{ -0.26 }$&$ 0.012  ^{+  0.000 }_{ -0.003 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 0.00  ^{+ 0.46  }_{ -0.00 }$&$ 1.12  \pm{ 0.45  }$&$ 89.52 ^{+ 0.48  }_{ -1.22 }$&$ 34.8  ^{+ 5.6   }_{ -12.1 }$&$ 0.139  \pm{ 0.008  }$&$ 625   \pm{ 137   }$&$ 121   \pm{ 18    }$& 4.8   & 0.1  &0.011&0.211\\
K03425.02  & 9117416    & 131.6995  &$    3.15720 ^{+    0.00008 }_{   -0.00009 }$&$ 0.22  ^{+ 0.44  }_{ -0.22 }$&$ 0.007  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.02  ^{+ 0.26  }_{ -0.02 }$&$ 0.63  \pm{ 0.27  }$&$ 88.55 ^{+ 1.45  }_{ -3.43 }$&$ 10.2  ^{+ 1.6   }_{ -3.4  }$&$ 0.040  \pm{ 0.002  }$&$ 1168  \pm{ 249   }$&$ 59    \pm{ 7     }$& 2.7   & 0.5  &0.011&0.211\\
K03500.01  & 6058816    & 188.5180  &$   73.75110 ^{+    0.00106 }_{   -0.00028 }$&$ 0.00  ^{+ 0.65  }_{ -0.00 }$&$ 0.015  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 1.98  \pm{ 0.50  }$&$ 90.00 ^{+ 0.00  }_{ -0.70 }$&$ 64.1  ^{+ 6.6   }_{ -15.9 }$&$ 0.348  \pm{ 0.018  }$&$ 557   \pm{ 101   }$&$ 251   \pm{ 34    }$& 10.4  & 0.2  &0.082&0.690\\
K03500.02  & 6058816    & 135.8111  &$    4.74823 ^{+    0.00015 }_{   -0.00021 }$&$ 0.91  ^{+ 0.09  }_{ -0.45 }$&$ 0.006  ^{+ 0.003  }_{ -0.003 }$&$ 0.00  ^{+ 0.05  }_{ -0.01 }$&$ 0.10  ^{+ 0.22  }_{ -0.05 }$&$ 0.68  \pm{ 0.30  }$&$ 72.49 ^{+ 1.70  }_{ -0.29 }$&$ 10.6  ^{+ 1.6   }_{ -1.0  }$&$ 0.055  \pm{ 0.003  }$&$ 1507  \pm{ 364   }$&$ 36     \pm{ 8     }$& 5.2   & 0.3  &0.025&0.387\\
K03681.01  & 2581316    & 238.8192  &$  217.83189 ^{+    0.00005 }_{   -0.00009 }$&$ 0.34  ^{+ 0.37  }_{ -0.05 }$&$ 0.089  ^{+ 0.003  }_{ -0.000 }$&$ 0.46  ^{+ 0.31  }_{ -0.46 }$&$ 0.00  ^{+ 1.63  }_{ -0.00 }$&$ 13.29 \pm{ 5.85  }$&$ 89.73 ^{+ 0.09  }_{ -0.35 }$&$ 114.6 ^{+ 13.5  }_{ -43.8 }$&$ 0.736  \pm{ 0.062  }$&$ 489   \pm{ 36	 }$&$ 9267  \pm{ 36    }$& 21.2  & 0.8  &0.911&0.996\\
K03681.02  & 2581316    & 134.5660  &$   10.51420 ^{+    0.00034 }_{   -0.00035 }$&$ 0.08  ^{+ 0.55  }_{ -0.08 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.33  ^{+ 0.24  }_{ -0.30 }$&$ 2.09  ^{+ 1.88  }_{ -2.07 }$&$ 1.18  \pm{ 0.21  }$&$ 89.73 ^{+ 0.27  }_{ -2.11 }$&$ 16.1  ^{+ 1.2   }_{ -1.8  }$&$ 0.096  \pm{ 0.005  }$&$ 1036  \pm{ 76	 }$&$ 80    \pm{ 6     }$& 3.7   & 0.5  &0.009&0.181\\
K03864.01  & 4164922    & 132.3795  &$    1.21073 ^{+    0.00001 }_{   -0.00001 }$&$ 0.88  ^{+ 0.04  }_{ -0.11 }$&$ 0.012  ^{+ 0.014  }_{ -0.001 }$&$ 0.08  ^{+ 0.53  }_{ -0.08 }$&$ 0.01  ^{+ 4.62  }_{ -0.01 }$&$ 2.98  \pm{ 1.90  }$&$ 69.47 ^{+ 4.30  }_{ -3.39 }$&$ 2.3   ^{+ 0.5   }_{ -0.3  }$&$ 0.023  \pm{ 0.001  }$&$ 2169  \pm{ 235   }$&$ 102   \pm{ 3     }$& 2.0   & 1.2  &0.182&0.847\\
K03864.02  & 4164922    & 134.4413  &$   18.25734 ^{+    0.00093 }_{   -0.00089 }$&$ 0.09  ^{+ 0.52  }_{ -0.09 }$&$ 0.011  ^{+ 0.002  }_{ -0.001 }$&$ 0.03  ^{+ 0.21  }_{ -0.03 }$&$ 0.00  ^{+  2.01 }_{ -0.00 }$&$ 0.82  \pm{ 0.18  }$&$ 89.86 ^{+ 0.14  }_{ -0.92 }$&$ 37.6  ^{+ 4.0   }_{ -5.2  }$&$ 0.125  \pm{ 0.006  }$&$ 549   \pm{ 69	 }$&$ 159   \pm{ 15    }$& 3.8   & 0.6  &0.053&0.582\\
K04021.01  & 11967788   & 133.1229  &$    7.23530 ^{+    0.00030 }_{   -0.00017 }$&$ 0.47  ^{+ 0.11  }_{ -0.47 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.00  ^{+ 0.63  }_{ -0.00 }$&$ 1.22  \pm{ 0.23  }$&$ 87.89 ^{+ 2.11  }_{ -0.65 }$&$ 12.6  ^{+ 0.9   }_{ -1.1  }$&$ 0.074  \pm{ 0.004  }$&$ 1198  \pm{ 91	 }$&$ 113   \pm{ 8     }$& 3.8   & 1.8  &0.199&0.861\\
K04021.02  & 11967788   & 132.4534  &$    4.93209 ^{+    0.00000 }_{    0.00000 }$&$ 0.22  ^{+ 0.24  }_{ -0.22 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.08  ^{+ 0.22  }_{ -0.08 }$&$ 1.02  \pm{ 0.16  }$&$ 88.71 ^{+ 1.29  }_{ -1.44 }$&$ 9.8   ^{+ 0.6   }_{ -1.0  }$&$ 0.057  \pm{ 0.003  }$&$ 1365  \pm{ 87	 }$&$ 67    \pm{ 7     }$& 3.8   & 1.8  &0.114&0.764\\
K04032.01  & 7100673    & 134.2139  &$    3.95125 ^{+    0.00000 }_{   -0.00000 }$&$ 0.43  ^{+ 0.28  }_{ -0.43 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.01  ^{+ 0.42  }_{ -0.01 }$&$ 0.85  \pm{ 0.21  }$&$ 87.45 ^{+ 2.55  }_{ -2.72 }$&$ 9.6   ^{+ 2.0   }_{ -1.3  }$&$ 0.049  \pm{ 0.002  }$&$ 1260  \pm{ 201   }$&$ 72    \pm{ 5     }$& 2.8   & 0.3  &0.040&0.511\\
K04032.02  & 7100673    & 132.8557  &$    2.89225 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.06  }_{ -0.05 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.13  }_{ -0.01 }$&$ 0.12  ^{+ 1.14  }_{ -0.12 }$&$ 2.26  \pm{ 0.31  }$&$ 75.29 ^{+ 1.39  }_{ -0.75 }$&$ 3.6   ^{+ 0.4   }_{ -0.2  }$&$ 0.042  \pm{ 0.003  }$&$ 1885  \pm{ 181   }$&$ 39    \pm{ 4     }$& 2.7   & 1.4  &0.034&0.466\\
K04097.01  & 5688683    & 133.1487  &$    2.79068 ^{+    0.00002 }_{   -0.00003 }$&$ 1.03  ^{+ 0.01  }_{ -0.06 }$&$ 0.068  ^{+  0.010 }_{ -0.041 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.73 \pm{ 0.22  }$&$ 75.55 ^{+ 2.20  }_{ -5.09 }$&$ 4.0   ^{+ 0.4   }_{ -0.9  }$&$ 0.040  \pm{ 0.002  }$&$ 1543  \pm{ 197   }$&$ 170   \pm{ 7     }$& 1.4   & 0.3  &0.122&0.776\\
K04097.02  & 5688683    & 131.7418  &$    4.44911 ^{+    0.00010 }_{   -0.00008 }$&$ 0.48  ^{+ 0.22  }_{ -0.40 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.03  ^{+ 0.21  }_{ -0.03 }$&$ 1.28  ^{+ 3.42  }_{ -1.28 }$&$ 0.51  \pm{ 0.09  }$&$ 88.41 ^{+ 1.34  }_{ -0.89 }$&$ 17.3  ^{+ 0.8   }_{ -1.2  }$&$ 0.045  \pm{ 0.002  }$&$ 681   \pm{ 77	 }$&$ 82    \pm{ 9     }$& 1.7   & 1.0  &0.027&0.409\\
K04269.01  & 8890924    & 131.5999  &$   26.65626 ^{+    0.00101 }_{   -0.00098 }$&$ 0.00  ^{+ 0.56  }_{ -0.00 }$&$ 0.012  ^{+ 0.002  }_{ -0.001 }$&$ 0.13  ^{+ 0.41  }_{ -0.13 }$&$ 0.04  ^{+ 0.28  }_{ -0.04 }$&$ 1.00  \pm{ 0.28  }$&$ 90.00 ^{+ 0.00  }_{ -0.97 }$&$ 45.4  ^{+ 5.1   }_{ -10.6 }$&$ 0.165  \pm{ 0.008  }$&$ 538   \pm{ 95	 }$&$ 194   \pm{ 24    }$& 5.0   & 0.4  &0.129&0.788\\
K04269.02  & 8890924    & 135.2750  &$    4.44061 ^{+    0.00016 }_{   -0.00019 }$&$ 0.50  ^{+ 0.97  }_{ -0.04 }$&$ 0.006  ^{+ 0.012  }_{ -0.004 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.09  ^{+ 0.26  }_{ -0.09 }$&$ 0.51  \pm{ 0.70  }$&$ 84.28 ^{+ 1.50  }_{ -0.17 }$&$ 13.5  ^{+ 2.0   }_{ -2.6  }$&$ 0.050  \pm{ 0.003  }$&$ 1526  \pm{ 835   }$&$ 35    \pm{ 10    }$& 5.9   & 0.3  &0.072&0.659\\
K04288.01  & 4548011    & 133.1927  &$    6.28402 ^{+    0.00020 }_{   -0.00028 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 0.005  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.70  \pm{ 0.15  }$&$ 90.00 ^{+ 0.00  }_{ -1.59 }$&$ 12.6  ^{+ 0.9   }_{ -1.5  }$&$ 0.067  \pm{ 0.004  }$&$ 1180  \pm{ 146   }$&$ 37    \pm{ 5     }$& 3.8   & 0.7  &0.008&0.170\\
K04288.02  & 4548011    & 139.9708  &$    9.08764 ^{+    0.00031 }_{   -0.00029 }$&$ 0.46  ^{+ 0.32  }_{ -0.46 }$&$ 0.005  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.51  }_{ -0.01 }$&$ 0.19  ^{+ 1.88  }_{ -0.19 }$&$ 0.69  \pm{ 0.15  }$&$ 88.34 ^{+ 1.66  }_{ -1.57 }$&$ 16.0  ^{+ 1.1   }_{ -2.0  }$&$ 0.086  \pm{ 0.004  }$&$ 1051  \pm{ 124   }$&$ 43    \pm{ 6     }$& 3.9   & 0.9  &0.008&0.163\\

\enddata


\tablecomments{The last three columns are significance of pixel centroid offset between in- and out-of-transit, planet confidence before and after considering the planetary likelihood boost in~\citet{Lissauer2012}. Planet candidates with significant pixel centroid offset ($> 3\sigma$) and planet candidates with higher than 0.997 planet confidence are marked in bold.}


\end{deluxetable}

\clearpage
 \end{landscape}


==> orbital_params.tex.20130926.tex <==


\clearpage
%\LongTables

\begin{landscape}
\begin{deluxetable}{lccccccccccccccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\setlength{\tabcolsep}{0.02in}
%\tablenum{1}
\tablecaption{Orbital Parameters\label{tab:orbital_params}}
\tablehead{
\colhead{\textbf{KOI}} &
\colhead{\textbf{KIC}} &
\colhead{\textbf{$T_0$}} &
\colhead{\textbf{Period}} &
\colhead{\textbf{Impact}} &
\colhead{\textbf{R$_{\rm PL}$/R$_{\ast}$}} &
\colhead{\textbf{e}} &
\colhead{\textbf{$\omega$}} &
\colhead{\textbf{R$_{\rm PL}$}} &
\colhead{\textbf{Inclination}} &
\colhead{\textbf{a/R$_{\ast}$}} &
\colhead{\textbf{a}} &
\colhead{\textbf{$T_{\rm PL}$}} &
\colhead{\textbf{Depth}} &
\colhead{\textbf{Dur}} &
\colhead{\textbf{Sig}} &
\colhead{\textbf{p1}} &
\colhead{\textbf{p2}} \\

\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(BKJD)}} &
\colhead{\textbf{(d)}} &
\colhead{\textbf{Parameter}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(radian)}} &
\colhead{\textbf{(R$_{\oplus}$)}} &
\colhead{\textbf{($\deg$)}} &
\colhead{\textbf{}} &
\colhead{\textbf{(AU)}} &
\colhead{\textbf{(K)}} &
\colhead{\textbf{(ppm)}} &
\colhead{\textbf{(hr)}} &
\colhead{\textbf{($\sigma$)}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} 

}

\startdata

K00005.01  & 8554498    & 132.9733  &$    4.78033 ^{+    0.00001 }_{   -0.00001 }$&$ 0.93  ^{+ 0.01  }_{ -0.01 }$&$ 0.045  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 8.07  \pm{ 0.64  }$&$ 82.72 ^{+ 0.61  }_{ -0.46 }$&$ 7.6   ^{+ 0.5   }_{ -0.4  }$&$ 0.059  \pm{ 0.002  }$&$ 1434  \pm{ 45    }$&$ 983   \pm{ 3     }$& 2.3   &\textbf{ 5.1  }&0.932 & 0.997  \\
K00005.02  & 8554498    & 133.3670  &$    7.05186 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.16  }_{ -0.17 }$&$ 0.003  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.04  ^{+ 0.21  }_{ -0.04 }$&$ 0.51  \pm{ 0.26  }$&$ 85.30 ^{+ 0.72  }_{ -0.60 }$&$ 11.2  ^{+ 1.0   }_{ -1.0  }$&$ 0.075  \pm{ 0.002  }$&$ 1159  \pm{ 69    }$&$ 12    \pm{ 4     }$& 1.9   & 0.4  &0.005 & 0.102  \\
K00041.01  & 6521045    & 122.9506  &$   12.81574 ^{+    0.00004 }_{   -0.00005 }$&$ 0.57  ^{+ 0.20  }_{ -0.55 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.00  ^{+ 0.88  }_{ -0.00 }$&$ 3.08  \pm{ 0.74  }$&$ 87.33 ^{+ 2.57  }_{ -2.06 }$&$ 12.0  ^{+ 2.5   }_{ -2.4  }$&$ 0.114  \pm{ 0.005  }$&$ 1120  \pm{ 130   }$&$ 219   \pm{ 5     }$& 6.7   & 1.5  &0.615 & 0.988  \\
K00041.02  & 6521045    & 133.1758  &$    6.88710 ^{+    0.00016 }_{   -0.00015 }$&$ 0.90  ^{+ 0.02  }_{ -0.09 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.11  ^{+ 0.19  }_{ -0.11 }$&$ 0.01  ^{+ 1.11  }_{ -0.01 }$&$ 3.13  \pm{ 0.58  }$&$ 81.11 ^{+ 1.65  }_{ -1.50 }$&$ 5.4   ^{+ 1.3   }_{ -0.5  }$&$ 0.076  \pm{ 0.003  }$&$ 1628  \pm{ 119   }$&$ 72    \pm{ 4     }$& 4.4   & 0.3  &0.063 & 0.769  \\
K00041.03  & 6521045    & 153.9839  &$   35.33314 ^{+    0.00109 }_{   -0.00204 }$&$ 0.93  ^{+ 0.10  }_{ -0.14 }$&$ 0.012  ^{+ 0.000  }_{ -0.003 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.00  ^{+ 3.09  }_{ -0.00 }$&$ 3.78  \pm{ 0.88  }$&$ 86.88 ^{+ 0.83  }_{ -0.55 }$&$ 17.0  ^{+ 4.8   }_{ -2.4  }$&$ 0.226  \pm{ 0.010  }$&$ 947   \pm{ 106   }$&$ 96    \pm{ 10    }$& 6.3   & 1.0  &0.053 & 0.736  \\
\textbf{K00070.01  }& 6850504    & 138.6075  &$   10.85409 ^{+    0.00002 }_{   -0.00003 }$&$ 0.31  ^{+ 0.26  }_{ -0.31 }$&$ 0.028  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.16  ^{+ 3.20  }_{ -0.16 }$&$ 2.94  \pm{ 0.26  }$&$ 89.13 ^{+ 0.87  }_{ -0.78 }$&$ 20.4  ^{+ 1.1   }_{ -1.2  }$&$ 0.092  \pm{ 0.003  }$&$ 803   \pm{ 32    }$&$ 1060  \pm{ 9     }$& 4.0   & 0.5  &0.959 &\textbf{ 0.999 } \\
K00070.02  & 6850504    & 134.5009  &$    3.69612 ^{+    0.00002 }_{   -0.00002 }$&$ 0.36  ^{+ 0.17  }_{ -0.36 }$&$ 0.017  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.00  ^{+  0.34 }_{ -0.00 }$&$ 1.77  \pm{ 0.18  }$&$ 87.96 ^{+ 2.04  }_{ -1.23 }$&$ 10.1  ^{+ 0.7   }_{ -0.7  }$&$ 0.045  \pm{ 0.002  }$&$ 1140  \pm{ 53    }$&$ 400   \pm{ 5     }$& 2.7   & 1.7  &0.821 & 0.996  \\
K00070.03  & 6850504    & 164.7276  &$   77.61153 ^{+    0.00017 }_{   -0.00022 }$&$ 0.32  ^{+ 0.21  }_{ -0.32 }$&$ 0.026  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 2.68  \pm{ 0.27  }$&$ 89.76 ^{+ 0.24  }_{ -0.18 }$&$ 77.4  ^{+ 6.0   }_{ -6.4  }$&$ 0.341  \pm{ 0.012  }$&$ 409   \pm{ 20    }$&$ 834   \pm{ 28    }$& 7.4   & 0.5  &0.539 & 0.983  \\
K00070.04  & 6850504    & 135.9338  &$    6.09850 ^{+    0.00018 }_{   -0.00022 }$&$ 0.07  ^{+ 0.59  }_{ -0.07 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.52  ^{+ 0.19  }_{ -0.50 }$&$ 3.16  ^{+ 1.61  }_{ -2.67 }$&$ 0.82  \pm{ 0.13  }$&$ 89.70 ^{+ 0.30  }_{ -2.46 }$&$ 14.3  ^{+ 1.1   }_{ -1.2  }$&$ 0.063  \pm{ 0.002  }$&$ 951   \pm{ 54    }$&$ 74    \pm{ 7     }$& 2.8   & 0.3  &0.029 & 0.596  \\
K00070.05  & 6850504    & 135.2142  &$   19.57709 ^{+    0.00077 }_{   -0.00066 }$&$ 0.34  ^{+ 0.44  }_{ -0.31 }$&$ 0.009  ^{+ 0.002  }_{ -0.001 }$&$ 0.01  ^{+ 0.37  }_{ -0.01 }$&$ 0.00  ^{+ 1.02  }_{ -0.00 }$&$ 0.89  \pm{ 0.16  }$&$ 89.37 ^{+ 0.58  }_{ -0.83 }$&$ 31.0  ^{+ 2.4   }_{ -2.5  }$&$ 0.136  \pm{ 0.005  }$&$ 646   \pm{ 35    }$&$ 104   \pm{ 13    }$& 4.5   & 1.5  &0.012 & 0.383  \\
K00072.01  & 11904151   & 131.5744  &$    0.83749 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 1.25  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -3.73 }$&$ 3.4   ^{+ 0.2   }_{ -0.2  }$&$ 0.016  \pm{ 0.001  }$&$ 2068  \pm{ 92    }$&$ 190   \pm{ 1     }$& 2.0   &\textbf{ 5.5  }&0.936 & 0.997  \\
K00072.02  & 11904151   & 138.6781  &$   45.29404 ^{+    0.00011 }_{   -0.00011 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.020  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 2.10  \pm{ 0.18  }$&$ 90.00 ^{+ 0.00  }_{ -0.48 }$&$ 50.5  ^{+ 3.4   }_{ -3.9  }$&$ 0.230  \pm{ 0.009  }$&$ 527   \pm{ 21    }$&$ 480   \pm{ 13    }$& 7.0   & 0.6  &0.774 & 0.988  \\
\textbf{K00082.01  }& 10187017   & 134.7534  &$   16.14569 ^{+    0.00003 }_{   -0.00003 }$&$ 0.25  ^{+ 0.31  }_{ -0.25 }$&$ 0.026  ^{+ 0.003  }_{ -0.000 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 0.00  ^{+ 4.10  }_{ -0.00 }$&$ 2.19  \pm{ 0.18  }$&$ 89.56 ^{+ 0.44  }_{ -0.64 }$&$ 32.2  ^{+ 1.6   }_{ -2.0  }$&$ 0.117  \pm{ 0.003  }$&$ 579   \pm{ 26    }$&$ 974   \pm{ 7     }$& 3.9   & 1.1  &0.974 &\textbf{ 0.999 } \\
K00082.02  & 10187017   & 134.0798  &$   10.31173 ^{+    0.00006 }_{   -0.00010 }$&$ 0.28  ^{+ 0.26  }_{ -0.28 }$&$ 0.014  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.00  ^{+  0.17 }_{ -0.00 }$&$ 1.19  \pm{ 0.12  }$&$ 89.31 ^{+ 0.69  }_{ -0.72 }$&$ 24.1  ^{+ 1.8   }_{ -1.5  }$&$ 0.086  \pm{ 0.002  }$&$ 669   \pm{ 32    }$&$ 276   \pm{ 5     }$& 3.2   & 0.5  &0.636 & 0.989  \\
K00082.03  & 10187017   & 145.0258  &$   27.45362 ^{+    0.00070 }_{   -0.00064 }$&$ 0.02  ^{+ 0.59  }_{ -0.02 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.34  ^{+ 0.30  }_{ -0.33 }$&$ 0.26  ^{+ 3.23  }_{ -0.26 }$&$ 0.82  \pm{ 0.12  }$&$ 89.97 ^{+ 0.03  }_{ -0.75 }$&$ 46.8  ^{+ 4.1   }_{ -3.7  }$&$ 0.166  \pm{ 0.004  }$&$ 476   \pm{ 27    }$&$ 145   \pm{ 9     }$& 3.9   & 0.7  &0.056 & 0.748  \\
K00082.04  & 10187017   & 139.9875  &$    7.07134 ^{+    0.00019 }_{   -0.00019 }$&$ 0.22  ^{+ 0.36  }_{ -0.22 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.64  \pm{ 0.08  }$&$ 89.34 ^{+ 0.66  }_{ -1.12 }$&$ 19.0  ^{+ 1.3   }_{ -1.5  }$&$ 0.067  \pm{ 0.002  }$&$ 749   \pm{ 41    }$&$ 79    \pm{ 5     }$& 2.8   & 0.6  &0.058 & 0.754  \\
K00082.05  & 10187017   & 135.8466  &$    5.28698 ^{+    0.00018 }_{   -0.00020 }$&$ 0.68  ^{+ 1.07  }_{ -0.04 }$&$ 0.006  ^{+ 0.034  }_{ -0.000 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.02  ^{+ 1.57  }_{ -0.00 }$&$ 0.51  \pm{ 1.43  }$&$ 87.09 ^{+ 0.09  }_{ -3.30 }$&$ 15.5  ^{+ 1.4   }_{ -1.3  }$&$ 0.055  \pm{ 0.001  }$&$ 890   \pm{ 67    }$&$ 41    \pm{ 4     }$& 2.2   & 0.6  &0.027 & 0.577  \\
\textbf{K00085.01  }& 5866724    & 132.0395  &$    5.85993 ^{+    0.00002 }_{   -0.00002 }$&$ 0.53  ^{+ 0.11  }_{ -0.53 }$&$ 0.020  ^{+ 0.002  }_{ -0.004 }$&$ 0.77  ^{+ 0.10  }_{ -0.58 }$&$ 4.60  ^{+ 0.19  }_{ -1.44 }$&$ 2.60  \pm{ 0.47  }$&$ 87.36 ^{+ 2.64  }_{ -0.61 }$&$ 11.8  ^{+ 1.1   }_{ -1.0  }$&$ 0.067  \pm{ 0.003  }$&$ 1203  \pm{ 74    }$&$ 321   \pm{ 3     }$& 4.4   &\textbf{ 5.2  }&0.939 &\textbf{ 0.999 } \\
K00085.02  & 5866724    & 133.4963  &$    2.15492 ^{+    0.00013 }_{   -0.00011 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.009  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.01  ^{+ 1.78  }_{ -0.01 }$&$ 1.29  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -3.96 }$&$ 5.5   ^{+ 0.4   }_{ -0.3  }$&$ 0.035  \pm{ 0.001  }$&$ 1786  \pm{ 82    }$&$ 99    \pm{ 2     }$& 3.2   &\textbf{ 3.7  }&0.657 & 0.990  \\
K00085.03  & 5866724    & 137.9953  &$    8.13115 ^{+    0.00009 }_{   -0.00006 }$&$ 0.62  ^{+ 0.13  }_{ -0.49 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 0.00  ^{+ 1.45  }_{ -0.00 }$&$ 1.62  \pm{ 0.13  }$&$ 86.86 ^{+ 2.45  }_{ -1.00 }$&$ 12.7  ^{+ 0.5   }_{ -0.9  }$&$ 0.085  \pm{ 0.003  }$&$ 1215  \pm{ 52    }$&$ 116   \pm{ 4     }$& 4.3   & 1.6  &0.379 & 0.968  \\
K00089.01  & 8056665    & 150.5651  &$   84.68895 ^{+    0.00012 }_{   -0.00010 }$&$ 0.54  ^{+ 0.26  }_{ -0.54 }$&$ 0.017  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 0.00  ^{+ 0.79  }_{ -0.00 }$&$ 4.97  \pm{ 1.65  }$&$ 89.29 ^{+ 0.71  }_{ -0.62 }$&$ 38.1  ^{+ 9.2   }_{ -11.0 }$&$ 0.473  \pm{ 0.014  }$&$ 775   \pm{ 120   }$&$ 402   \pm{ 17    }$& 12.6  & 0.7  &0.008 & 0.170  \\
K00089.02  & 8056665    & 289.8688  &$  207.60349 ^{+    0.00047 }_{   -0.00036 }$&$ 0.94  ^{+ 0.41  }_{ -0.10 }$&$ 0.032  ^{+  0.000 }_{ -0.013 }$&$ 0.01  ^{+ 0.66  }_{ -0.01 }$&$ 0.00  ^{+ 1.57  }_{ -0.00 }$&$ 10.66 \pm{ 3.82  }$&$ 89.24 ^{+ 0.27  }_{ -0.61 }$&$ 61.6  ^{+ 20.4  }_{ -16.2 }$&$ 0.861  \pm{ 0.023  }$&$ 608   \pm{ 98    }$&$ 490   \pm{ 33    }$& 9.6   & 0.6  &0.021 & 0.345  \\
\textbf{K00094.01  }& 6462863    & 132.7405  &$   22.34300 ^{+    0.00001 }_{   -0.00001 }$&$ 0.45  ^{+ 0.14  }_{ -0.20 }$&$ 0.069  ^{+ 0.004  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 10.51 \pm{ 0.97  }$&$ 88.93 ^{+ 0.51  }_{ -0.46 }$&$ 24.3  ^{+ 1.3   }_{ -1.5  }$&$ 0.158  \pm{ 0.007  }$&$ 833   \pm{ 35    }$&$ 5426  \pm{ 27    }$& 6.8   &\textbf{ 13.6 }&0.978 &\textbf{ 1.000 } \\
K00094.02  & 6462863    & 138.0072  &$   10.42371 ^{+    0.00003 }_{   -0.00003 }$&$ 0.40  ^{+  0.00 }_{ -0.40 }$&$ 0.026  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 3.98  \pm{ 0.32  }$&$ 88.36 ^{+ 1.64  }_{ -0.00 }$&$ 14.5  ^{+ 0.8   }_{ -0.8  }$&$ 0.095  \pm{ 0.004  }$&$ 1078  \pm{ 39    }$&$ 769   \pm{ 11    }$& 5.1   &\textbf{ 3.0  }&0.246 & 0.942  \\
K00094.03  & 6462863    & 161.2400  &$   54.31993 ^{+    0.00006 }_{   -0.00010 }$&$ 0.39  ^{+ 0.20  }_{ -0.28 }$&$ 0.043  ^{+  0.000 }_{ -0.003 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 6.60  \pm{ 0.60  }$&$ 89.49 ^{+ 0.37  }_{ -0.32 }$&$ 44.0  ^{+ 2.6   }_{ -2.9  }$&$ 0.285  \pm{ 0.012  }$&$ 614   \pm{ 27    }$&$ 2494  \pm{ 37    }$& 8.9   &\textbf{ 3.7  }&0.463 & 0.977  \\
K00094.04  & 6462863    & 131.6139  &$    3.74324 ^{+    0.00006 }_{   -0.00009 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 1.49  \pm{ 0.15  }$&$ 90.00 ^{+ 0.00  }_{ -1.65 }$&$ 7.3   ^{+ 0.5   }_{ -0.4  }$&$ 0.048  \pm{ 0.002  }$&$ 1513  \pm{ 61    }$&$ 125   \pm{ 7     }$& 3.9   & 1.7  &0.076 & 0.804  \\
K00102.01  & 8456679    & 135.0591  &$    1.73514 ^{+    0.00000 }_{   -0.00000 }$&$ 0.56  ^{+ 0.03  }_{ -0.03 }$&$ 0.034  ^{+ 0.000  }_{ -0.000 }$&$ 0.78  ^{+ 0.04  }_{ -0.09 }$&$ 4.70  ^{+  0.06 }_{ -0.23 }$&$ 3.85  \pm{ 0.38  }$&$ 84.57 ^{+ 0.77  }_{ -1.46 }$&$ 5.9   ^{+ 0.4   }_{ -0.5  }$&$ 0.028  \pm{ 0.001  }$&$ 1592  \pm{ 104   }$&$ 946   \pm{ 3     }$& 2.7   &\textbf{ 27.2 }&0.906 & 0.996  \\
K00102.02  & 8456679    & 132.2635  &$    4.06853 ^{+    0.00008 }_{   -0.00015 }$&$ 0.51  ^{+ 0.32  }_{ -0.49 }$&$ 0.008  ^{+ 0.009  }_{ -0.002 }$&$ 0.71  ^{+ 0.19  }_{ -0.71 }$&$ 3.62  ^{+ 1.10  }_{ -3.60 }$&$ 0.94  \pm{ 0.62  }$&$ 87.13 ^{+ 2.76  }_{ -1.79 }$&$ 10.3  ^{+ 0.9   }_{ -0.8  }$&$ 0.050  \pm{ 0.002  }$&$ 1210  \pm{ 73    }$&$ 98    \pm{ 6     }$& 3.0   & 2.6  &0.004 & 0.085  \\
K00108.01  & 4914423    & 142.1763  &$   15.96535 ^{+    0.00006 }_{   -0.00006 }$&$ 0.51  ^{+ 0.11  }_{ -0.32 }$&$ 0.020  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.35  }_{ -0.00 }$&$ 0.03  ^{+ 0.53  }_{ -0.03 }$&$ 2.66  \pm{ 0.28  }$&$ 88.69 ^{+ 0.87  }_{ -0.40 }$&$ 22.5  ^{+ 1.7   }_{ -1.7  }$&$ 0.128  \pm{ 0.005  }$&$ 840   \pm{ 42    }$&$ 492   \pm{ 8     }$& 4.8   & 0.3  &0.718 & 0.985  \\
K00108.02  & 4914423    & 295.3304  &$  179.60101 ^{+    0.00008 }_{   -0.00003 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 0.032  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 4.38  \pm{ 0.45  }$&$ 90.00 ^{+ 0.00  }_{ -0.25 }$&$ 109.4 ^{+ 6.8   }_{ -7.3  }$&$ 0.647  \pm{ 0.025  }$&$ 382   \pm{ 16    }$&$ 1296  \pm{ 35    }$& 13.0  & 0.8  &0.163 & 0.830  \\
K00111.01  & 6678383    & 137.6139  &$   11.42751 ^{+    0.00004 }_{   -0.00005 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.020  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.01  ^{+ 3.85  }_{ -0.01 }$&$ 2.21  \pm{ 0.19  }$&$ 90.00 ^{+ 0.00  }_{ -1.32 }$&$ 19.5  ^{+ 1.4   }_{ -1.1  }$&$ 0.092  \pm{ 0.004  }$&$ 871   \pm{ 35    }$&$ 509   \pm{ 8     }$& 4.7   & 1.8  &0.738 & 0.993  \\
K00111.02  & 6678383    & 132.7129  &$   23.66834 ^{+    0.00011 }_{   -0.00011 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.019  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+ 1.38  }_{ -0.00 }$&$ 2.07  \pm{ 0.17  }$&$ 90.00 ^{+ 0.00  }_{ -0.81 }$&$ 32.5  ^{+ 1.9   }_{ -2.0  }$&$ 0.149  \pm{ 0.005  }$&$ 673   \pm{ 27    }$&$ 480   \pm{ 12    }$& 5.8   & 1.1  &0.514 & 0.981  \\
K00111.03  & 6678383    & 271.0832  &$   51.75627 ^{+    0.00023 }_{   -0.00024 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.022  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.04  ^{+ 3.87  }_{ -0.04 }$&$ 2.31  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -0.49 }$&$ 56.2  ^{+ 4.0   }_{ -4.1  }$&$ 0.251  \pm{ 0.010  }$&$ 510   \pm{ 25    }$&$ 621   \pm{ 19    }$& 7.3   & 0.3  &0.480 & 0.979  \\
K00112.01  & 10984090   & 185.1795  &$   51.07931 ^{+    0.00014 }_{   -0.00022 }$&$ 0.24  ^{+ 0.14  }_{ -0.24 }$&$ 0.024  ^{+ 0.001  }_{ -0.000 }$&$ 0.05  ^{+ 0.22  }_{ -0.05 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 2.55  \pm{ 0.24  }$&$ 89.76 ^{+ 0.24  }_{ -0.15 }$&$ 58.0  ^{+ 4.0   }_{ -4.4  }$&$ 0.262  \pm{ 0.011  }$&$ 512   \pm{ 24    }$&$ 749   \pm{ 19    }$& 6.7   & 0.4  &0.481 & 0.959  \\
K00112.02  & 10984090   & 133.9857  &$    3.70919 ^{+    0.00007 }_{   -0.00007 }$&$ 0.37  ^{+ 0.18  }_{ -0.37 }$&$ 0.010  ^{+ 0.002  }_{ -0.001 }$&$ 0.16  ^{+ 0.43  }_{ -0.16 }$&$ 4.75  ^{+ 1.10  }_{ -4.56 }$&$ 1.06  \pm{ 0.15  }$&$ 87.89 ^{+ 2.11  }_{ -1.11 }$&$ 9.9   ^{+ 0.8   }_{ -0.6  }$&$ 0.046  \pm{ 0.002  }$&$ 1230  \pm{ 62    }$&$ 138   \pm{ 5     }$& 3.1   & 0.9  &0.064 & 0.632  \\
\textbf{K00115.01  }& 9579641    & 133.1424  &$    5.41220 ^{+    0.00002 }_{   -0.00002 }$&$ 0.64  ^{+ 0.26  }_{ -0.17 }$&$ 0.028  ^{+ 0.001  }_{ -0.006 }$&$ 0.47  ^{+ 0.05  }_{ -0.47 }$&$ 4.75  ^{+ 0.28  }_{ -4.75 }$&$ 4.81  \pm{ 1.53  }$&$ 85.94 ^{+ 1.87  }_{ -3.88 }$&$ 8.9   ^{+ 2.4   }_{ -2.1  }$&$ 0.066  \pm{ 0.003  }$&$ 1418  \pm{ 228   }$&$ 600   \pm{ 6     }$& 3.3   & 2.8  &0.914 &\textbf{ 0.998 } \\
K00115.02  & 9579641    & 139.0032  &$    7.12597 ^{+    0.00011 }_{   -0.00016 }$&$ 0.70  ^{+ 0.14  }_{ -0.38 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 1.09  ^{+  0.00 }_{ -1.09 }$&$ 2.11  \pm{ 0.55  }$&$ 86.73 ^{+ 2.17  }_{ -1.51 }$&$ 11.4  ^{+ 2.8   }_{ -2.0  }$&$ 0.078  \pm{ 0.003  }$&$ 1214  \pm{ 145   }$&$ 196   \pm{ 7     }$& 3.3   & 0.7  &0.309 & 0.957  \\
K00115.03  & 9579641    & 132.6570  &$    3.43584 ^{+    0.00009 }_{   -0.00006 }$&$ 0.64  ^{+ 0.60  }_{ -0.40 }$&$ 0.005  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.67  ^{+ 2.53  }_{ -0.67 }$&$ 0.80  \pm{ 0.31  }$&$ 84.85 ^{+ 3.35  }_{ -5.54 }$&$ 6.6   ^{+ 1.7   }_{ -1.6  }$&$ 0.048  \pm{ 0.002  }$&$ 1596  \pm{ 265   }$&$ 24    \pm{ 5     }$& 2.9   & 0.8  &0.010 & 0.327  \\
K00116.01  & 8395660    & 136.2799  &$   13.57100 ^{+    0.00014 }_{   -0.00014 }$&$ 0.59  ^{+ 0.17  }_{ -0.29 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.01  ^{+ 0.41  }_{ -0.01 }$&$ 2.29  \pm{ 0.43  }$&$ 88.56 ^{+ 0.81  }_{ -0.76 }$&$ 22.9  ^{+ 3.4   }_{ -3.4  }$&$ 0.110  \pm{ 0.005  }$&$ 799   \pm{ 73    }$&$ 518   \pm{ 13    }$& 3.6   & 0.6  &0.187 & 0.920  \\
K00116.02  & 8395660    & 151.9344  &$   43.84445 ^{+    0.00014 }_{   -0.00041 }$&$ 0.37  ^{+ 0.22  }_{ -0.37 }$&$ 0.023  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+  0.24}_{ -0.00 }$&$ 2.69  \pm{ 0.41  }$&$ 89.56 ^{+ 0.44  }_{ -0.37 }$&$ 48.4  ^{+ 5.2   }_{ -6.6  }$&$ 0.241  \pm{ 0.011  }$&$ 560   \pm{ 43    }$&$ 668   \pm{ 24    }$& 6.5   & 0.7  &0.092 & 0.834  \\
K00116.03  & 8395660    & 135.6340  &$    6.16500 ^{+    0.00000 }_{   -0.00000 }$&$ 0.39  ^{+ 0.29  }_{ -0.39 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.01  ^{+ 0.24  }_{ -0.01 }$&$ 0.86  \pm{ 0.19  }$&$ 88.28 ^{+ 1.71  }_{ -1.38 }$&$ 12.9  ^{+ 2.1   }_{ -1.9  }$&$ 0.065  \pm{ 0.003  }$&$ 1077  \pm{ 110   }$&$ 68    \pm{ 9     }$& 3.3   & 0.8  &0.002 & 0.098  \\
K00116.04  & 8395660    & 147.5282  &$   23.98000 ^{+    0.00115 }_{   -0.00128 }$&$ 0.40  ^{+ 0.38  }_{ -0.40 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.29  ^{+ 0.43  }_{ -0.29 }$&$ 3.20  ^{+ 1.47  }_{ -2.94 }$&$ 1.08  \pm{ 0.25  }$&$ 89.32 ^{+ 0.68  }_{ -0.80 }$&$ 32.6  ^{+ 5.4   }_{ -5.3  }$&$ 0.161  \pm{ 0.007  }$&$ 671   \pm{ 78    }$&$ 98    \pm{ 18    }$& 5.0   & 0.4  &0.002 & 0.075  \\
K00117.01  & 10875245   & 138.7788  &$   14.74910 ^{+    0.00008 }_{   -0.00008 }$&$ 0.94  ^{+ 0.06  }_{ -0.04 }$&$ 0.022  ^{+ 0.000  }_{ -0.001 }$&$ 0.10  ^{+ 0.06  }_{ -0.10 }$&$ 0.44  ^{+ 0.95  }_{ -0.44 }$&$ 8.93  \pm{ 0.76  }$&$ 83.20 ^{+ 0.59  }_{ -0.66 }$&$ 8.0   ^{+ 0.2   }_{ -0.2  }$&$ 0.137  \pm{ 0.007  }$&$ 1404  \pm{ 36    }$&$ 436   \pm{ 11    }$& 6.7   & 0.6  &0.339 & 0.962  \\
K00117.02  & 10875245   & 138.6039  &$    4.90147 ^{+    0.00015 }_{   -0.00015 }$&$ 1.00  ^{+  0.00 }_{ -0.10 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+  0.19 }_{ -0.00 }$&$ 1.30  ^{+  0.00}_{ -1.30 }$&$ 4.97  \pm{ 0.43  }$&$ 73.48 ^{+ 3.46  }_{ -1.03 }$&$ 3.9   ^{+ 0.1   }_{ -0.1  }$&$ 0.065  \pm{ 0.003  }$&$ 1995  \pm{ 50    }$&$ 138   \pm{ 6     }$& 4.4   & 0.4  &0.105 & 0.855  \\
K00117.03  & 10875245   & 133.5041  &$    3.17996 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.08  }_{ -0.02 }$&$ 0.013  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 1.38  }_{ -0.00 }$&$ 5.10  \pm{ 0.51  }$&$ 72.19 ^{+ 1.05  }_{ -1.70 }$&$ 2.9   ^{+ 0.1   }_{ -0.1  }$&$ 0.048  \pm{ 0.003  }$&$ 2300  \pm{ 73    }$&$ 121   \pm{ 5     }$& 4.0   & 1.1  &0.117 & 0.869  \\
K00117.04  & 10875245   & 137.8159  &$    7.95792 ^{+    0.00038 }_{   -0.00041 }$&$ 0.69  ^{+ 4.08  }_{ -0.31 }$&$ 0.013  ^{+ 0.012  }_{ -0.011 }$&$ 0.39  ^{+  0.24 }_{ -0.29 }$&$ 4.86  ^{+  3.06 }_{ -3.40 }$&$ 2.30  \pm{ 2.63  }$&$ 81.15 ^{+  1.34 }_{ -2.79 }$&$ 11.1  ^{+ 6.7   }_{ -5.6  }$&$ 0.085  \pm{ 0.006  }$&$ 1861  \pm{ 2228  }$&$ 50    \pm{ 8     }$& 6.9   & 0.4  &0.004 & 0.179  \\
K00119.01  & 9471974    & 141.9096  &$   49.18431 ^{+    0.00005 }_{   -0.00004 }$&$ 0.37  ^{+ 0.25  }_{ -0.37 }$&$ 0.035  ^{+ 0.005  }_{ -0.001 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 3.82  }_{ -0.00 }$&$ 6.70  \pm{ 1.33  }$&$ 89.34 ^{+ 0.66  }_{ -0.57 }$&$ 33.0  ^{+ 4.9   }_{ -4.5  }$&$ 0.266  \pm{ 0.014  }$&$ 655   \pm{ 51    }$&$ 1373  \pm{ 25    }$& 11.2  &\textbf{ 11.3 }&0.836 & 0.992  \\
K00119.02  & 9471974    & 312.6812  &$  190.31340 ^{+    0.00063 }_{   -0.00053 }$&$ 0.38  ^{+ 0.21  }_{ -0.38 }$&$ 0.030  ^{+ 0.009  }_{ -0.002 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.00  ^{+ 4.71  }_{ -0.00 }$&$ 4.60  \pm{ 1.39  }$&$ 89.76 ^{+ 0.24  }_{ -0.22 }$&$ 97.7  ^{+ 25.4  }_{ -19.2 }$&$ 0.644  \pm{ 0.026  }$&$ 392   \pm{ 51    }$&$ 1146  \pm{ 39    }$& 15.2  &\textbf{ 4.8  }&0.374 & 0.937  \\
K00123.01  & 5094751    & 122.9737  &$    6.48168 ^{+    0.00004 }_{   -0.00004 }$&$ 0.53  ^{+ 0.09  }_{ -0.52 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 2.39  \pm{ 0.28  }$&$ 87.09 ^{+ 2.85  }_{ -0.74 }$&$ 10.3  ^{+ 0.8   }_{ -0.9  }$&$ 0.069  \pm{ 0.002  }$&$ 1200  \pm{ 63    }$&$ 302   \pm{ 5     }$& 4.1   & 0.3  &0.703 & 0.983  \\
K00123.02  & 5094751    & 137.5738  &$   21.22254 ^{+    0.00010 }_{   -0.00010 }$&$ 0.37  ^{+ 0.09  }_{ -0.37 }$&$ 0.017  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.09  ^{+ 0.77  }_{ -0.09 }$&$ 2.70  \pm{ 0.27  }$&$ 89.09 ^{+ 0.91  }_{ -0.27 }$&$ 22.8  ^{+ 1.6   }_{ -1.8  }$&$ 0.152  \pm{ 0.003  }$&$ 810   \pm{ 38    }$&$ 357   \pm{ 10    }$& 6.6   & 0.4  &0.446 & 0.953  \\
K00124.01  & 11086270   & 137.1212  &$   12.69115 ^{+    0.00020 }_{   -0.00014 }$&$ 0.85  ^{+ 0.04  }_{ -0.16 }$&$ 0.016  ^{+ 0.000  }_{ -0.002 }$&$ 0.06  ^{+ 0.56  }_{ -0.06 }$&$ 0.00  ^{+ 1.01  }_{ -0.00 }$&$ 2.98  \pm{ 0.33  }$&$ 86.46 ^{+ 0.92  }_{ -0.58 }$&$ 14.0  ^{+ 1.1   }_{ -1.1  }$&$ 0.108  \pm{ 0.002  }$&$ 1056  \pm{ 53    }$&$ 256   \pm{ 9     }$& 4.0   & 1.0  &0.400 & 0.944  \\
K00124.02  & 11086270   & 142.8190  &$   31.71987 ^{+    0.00025 }_{   -0.00034 }$&$ 0.86  ^{+ 0.05  }_{ -0.08 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 3.57  \pm{ 0.43  }$&$ 88.10 ^{+ 0.39  }_{ -0.37 }$&$ 26.1  ^{+ 2.6   }_{ -1.9  }$&$ 0.200  \pm{ 0.004  }$&$ 771   \pm{ 50    }$&$ 369   \pm{ 15    }$& 5.2   & 0.4  &0.332 & 0.926  \\
K00139.01  & 8559644    & 142.0874  &$  224.79712 ^{+    0.00003 }_{   -0.00001 }$&$ 0.18  ^{+ 0.42  }_{ -0.18 }$&$ 0.047  ^{+ 0.009  }_{ -0.001 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.10  ^{+ 4.60  }_{ -0.10 }$&$ 5.83  \pm{ 0.80  }$&$ 89.93 ^{+ 0.07  }_{ -0.19 }$&$ 141.8 ^{+ 12.4  }_{ -10.4 }$&$ 0.749  \pm{ 0.028  }$&$ 330   \pm{ 19    }$&$ 3395  \pm{ 68    }$& 12.4  & 0.8  &0.409 & 0.945  \\
K00139.02  & 8559644    & 141.3521  &$    3.34184 ^{+    0.00005 }_{   -0.00007 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 1.39  \pm{ 0.15  }$&$ 90.00 ^{+  0.00 }_{ -3.08 }$&$ 8.2   ^{+ 0.6   }_{ -0.6  }$&$ 0.045  \pm{ 0.002  }$&$ 1387  \pm{ 64    }$&$ 167   \pm{ 7     }$& 3.2   & 0.5  &0.143 & 0.806  \\
K00148.01  & 5735762    & 124.0630  &$    4.77798 ^{+    0.00003 }_{   -0.00004 }$&$ 0.20  ^{+ 0.31  }_{ -0.20 }$&$ 0.018  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 1.75  \pm{ 0.17  }$&$ 89.07 ^{+ 0.93  }_{ -1.67 }$&$ 12.4  ^{+ 0.8   }_{ -0.9  }$&$ 0.052  \pm{ 0.002  }$&$ 992   \pm{ 48    }$&$ 489   \pm{ 8     }$& 3.0   & 2.1  &0.351 & 0.964  \\
K00148.02  & 5735762    & 125.3398  &$    9.67393 ^{+    0.00003 }_{   -0.00003 }$&$ 0.39  ^{+ 0.19  }_{ -0.37 }$&$ 0.027  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 2.60  \pm{ 0.26  }$&$ 88.89 ^{+ 1.07  }_{ -0.71 }$&$ 20.1  ^{+ 1.4   }_{ -1.6  }$&$ 0.083  \pm{ 0.003  }$&$ 772   \pm{ 37    }$&$ 987   \pm{ 12    }$& 3.5   & 2.3  &0.631 & 0.988  \\
K00148.03  & 5735762    & 146.0657  &$   42.89592 ^{+    0.00051 }_{   -0.00048 }$&$ 0.19  ^{+ 0.35  }_{ -0.19 }$&$ 0.021  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.97  \pm{ 0.21  }$&$ 89.80 ^{+ 0.20  }_{ -0.40 }$&$ 54.5  ^{+ 4.8   }_{ -4.1  }$&$ 0.224  \pm{ 0.009  }$&$ 467   \pm{ 25    }$&$ 599   \pm{ 28    }$& 6.0   & 1.1  &0.070 & 0.790  \\
K00153.01  & 12252424   & 139.7122  &$    8.92511 ^{+    0.00005 }_{   -0.00005 }$&$ 0.63  ^{+ 0.13  }_{ -0.09 }$&$ 0.034  ^{+ 0.004  }_{ -0.006 }$&$ 0.50  ^{+ 0.26  }_{ -0.37 }$&$ 4.24  ^{+ 0.46  }_{ -1.97 }$&$ 2.86  \pm{ 0.67  }$&$ 88.21 ^{+ 0.56  }_{ -0.75 }$&$ 20.9  ^{+ 4.3   }_{ -3.1  }$&$ 0.077  \pm{ 0.002  }$&$ 698   \pm{ 78    }$&$ 997   \pm{ 15    }$& 3.1   & 1.0  &0.871 & 0.994  \\
K00153.02  & 12252424   & 128.5467  &$    4.75399 ^{+    0.00002 }_{   -0.00002 }$&$ 0.38  ^{+ 0.24  }_{ -0.38 }$&$ 0.023  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 0.00  ^{+ 1.44  }_{ -0.00 }$&$ 2.12  \pm{ 0.28  }$&$ 88.28 ^{+ 1.72  }_{ -1.47 }$&$ 12.9  ^{+ 1.3   }_{ -1.2  }$&$ 0.050  \pm{ 0.001  }$&$ 883   \pm{ 57    }$&$ 780   \pm{ 10    }$& 2.7   & 0.5  &0.889 & 0.995  \\
K00159.01  & 8972058    & 136.7363  &$    8.99092 ^{+    0.00011 }_{   -0.00001 }$&$ 0.59  ^{+ 0.20  }_{ -0.57 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 0.73  }_{ -0.00 }$&$ 3.14  \pm{ 0.65  }$&$ 87.39 ^{+ 2.52  }_{ -1.86 }$&$ 12.8  ^{+ 2.5   }_{ -2.1  }$&$ 0.087  \pm{ 0.003  }$&$ 1120  \pm{ 123   }$&$ 466   \pm{ 12    }$& 4.4   & 0.5  &0.293 & 0.912  \\
K00159.02  & 8972058    & 134.7278  &$    2.40365 ^{+    0.00002 }_{   -0.00002 }$&$ 0.93  ^{+ 0.03  }_{ -0.04 }$&$ 0.013  ^{+  0.000 }_{ -0.003 }$&$ 0.05  ^{+ 0.06  }_{ -0.05 }$&$ 0.17  ^{+ 0.43  }_{ -0.17 }$&$ 2.41  \pm{ 0.34  }$&$ 78.01 ^{+ 1.11  }_{ -1.48 }$&$ 4.5   ^{+ 0.4   }_{ -0.4  }$&$ 0.036  \pm{ 0.001  }$&$ 1905  \pm{ 100   }$&$ 82    \pm{ 6     }$& 1.7   & 0.6  &0.024 & 0.381  \\
K00168.01  & 11512246   & 133.2871  &$   10.74245 ^{+    0.00006 }_{   -0.00006 }$&$ 0.37  ^{+ 0.41  }_{ -0.37 }$&$ 0.016  ^{+ 0.004  }_{ -0.000 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 3.79  \pm{ 1.14  }$&$ 87.97 ^{+ 2.03  }_{ -3.91 }$&$ 10.1  ^{+ 2.2   }_{ -2.5  }$&$ 0.100  \pm{ 0.003  }$&$ 1258  \pm{ 158   }$&$ 426   \pm{ 13    }$& 7.4   & 0.2  &0.312 & 0.958  \\
K00168.02  & 11512246   & 147.5788  &$   15.27448 ^{+    0.00046 }_{   -0.00040 }$&$ 0.00  ^{+ 0.69  }_{ -0.00 }$&$ 0.011  ^{+ 0.003  }_{ -0.000 }$&$ 0.08  ^{+ 0.39  }_{ -0.08 }$&$ 1.93  ^{+ 2.10  }_{ -1.93 }$&$ 2.26  \pm{ 0.66  }$&$ 89.98 ^{+ 0.02  }_{ -3.15 }$&$ 14.0  ^{+ 2.7   }_{ -3.1  }$&$ 0.126  \pm{ 0.004  }$&$ 1062  \pm{ 138   }$&$ 210   \pm{ 17    }$& 7.5   & 0.4  &0.092 & 0.835  \\
K00168.03  & 11512246   & 138.3254  &$    7.10690 ^{+    0.00029 }_{   -0.00022 }$&$ 0.18  ^{+ 0.40  }_{ -0.18 }$&$ 0.008  ^{+ 0.002  }_{ -0.001 }$&$ 0.04  ^{+ 0.18  }_{ -0.04 }$&$ 0.02  ^{+ 0.35  }_{ -0.02 }$&$ 1.91  \pm{ 0.54  }$&$ 88.79 ^{+ 1.21  }_{ -3.31 }$&$ 7.8   ^{+ 1.9   }_{ -1.7  }$&$ 0.076  \pm{ 0.002  }$&$ 1404  \pm{ 188   }$&$ 107   \pm{ 11    }$& 6.4   & 0.1  &0.041 & 0.681  \\
\textbf{K00244.01  }& 4349452    & 178.5274  &$   12.72036 ^{+    0.00002 }_{   -0.00002 }$&$ 0.92  ^{+ 0.07  }_{ -0.02 }$&$ 0.039  ^{+ 0.002  }_{ -0.002 }$&$ 0.01  ^{+ 0.18  }_{ -0.01 }$&$ 0.00  ^{+ 0.81  }_{ -0.00 }$&$ 7.06  \pm{ 0.63  }$&$ 86.47 ^{+ 0.32  }_{ -0.58 }$&$ 14.6  ^{+ 1.0   }_{ -0.9  }$&$ 0.113  \pm{ 0.003  }$&$ 1046  \pm{ 40    }$&$ 1183  \pm{ 4     }$& 3.1   &\textbf{ 37.2 }&0.973 &\textbf{ 0.999 } \\
\textbf{K00244.02  }& 4349452    & 171.7046  &$    6.23856 ^{+    0.00001 }_{   -0.00001 }$&$ 0.68  ^{+ 0.09  }_{ -0.68 }$&$ 0.019  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 3.50  \pm{ 0.48  }$&$ 85.83 ^{+ 4.17  }_{ -1.20 }$&$ 9.0   ^{+ 0.9   }_{ -0.8  }$&$ 0.070  \pm{ 0.002  }$&$ 1327  \pm{ 85    }$&$ 421   \pm{ 3     }$& 3.9   &\textbf{ 15.9 }&0.953 &\textbf{ 0.998 } \\
\textbf{K00245.01  }& 8478994    & 175.2497  &$   39.79219 ^{+    0.00006 }_{   -0.00006 }$&$ 0.50  ^{+ 0.09  }_{ -0.50 }$&$ 0.022  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 1.92  \pm{ 0.19  }$&$ 89.51 ^{+ 0.49  }_{ -0.12 }$&$ 58.6  ^{+ 4.8   }_{ -4.7  }$&$ 0.217  \pm{ 0.008  }$&$ 460   \pm{ 24    }$&$ 607   \pm{ 5     }$& 4.7   &\textbf{ 7.1  }&0.947 &\textbf{ 0.999 } \\
K00245.02  & 8478994    & 191.8385  &$   21.30185 ^{+    0.00050 }_{   -0.00019 }$&$ 0.35  ^{+ 0.27  }_{ -0.35 }$&$ 0.008  ^{+ 0.002  }_{ -0.000 }$&$ 0.20  ^{+ 0.63  }_{ -0.20 }$&$ 3.50  ^{+ 1.34  }_{ -3.46 }$&$ 0.70  \pm{ 0.11  }$&$ 89.47 ^{+ 0.53  }_{ -0.45 }$&$ 38.5  ^{+ 3.1   }_{ -3.2  }$&$ 0.143  \pm{ 0.005  }$&$ 568   \pm{ 30    }$&$ 91    \pm{ 4     }$& 4.2   &\textbf{ 3.3  }&0.186 & 0.920  \\
K00245.03  & 8478994    & 184.0333  &$   13.36727 ^{+    0.00042 }_{   -0.00061 }$&$ 0.80  ^{+ 0.43  }_{ -0.47 }$&$ 0.004  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.16  ^{+ 0.86  }_{ -0.16 }$&$ 0.37  \pm{ 0.21  }$&$ 88.40 ^{+ 0.95  }_{ -0.80 }$&$ 28.4  ^{+ 2.5   }_{ -2.2  }$&$ 0.105  \pm{ 0.003  }$&$ 657   \pm{ 38    }$&$ 17    \pm{ 3     }$& 2.2   & 1.1  &0.016 & 0.443  \\
K00245.04  & 8478994    & 195.7268  &$   51.19880 ^{+    0.00016 }_{   -0.02033 }$&$ 0.68  ^{+ 0.81  }_{ -0.68 }$&$ 0.004  ^{+ 0.007  }_{ -0.002 }$&$ 0.24  ^{+ 0.20  }_{ -0.24 }$&$ 0.06  ^{+ 0.26  }_{ -0.06 }$&$ 0.34  \pm{ 0.36  }$&$ 89.45 ^{+ 0.55  }_{ -0.64 }$&$ 69.9  ^{+ 5.8   }_{ -4.8  }$&$ 0.256  \pm{ 0.009  }$&$ 415   \pm{ 23    }$&$ 15    \pm{ 7     }$& 4.1   & 0.3  &0.013 & 0.402  \\
\textbf{K00246.01  }& 11295426   & 173.8571  &$    5.39877 ^{+    0.00001 }_{   -0.00001 }$&$ 0.38  ^{+ 0.20  }_{ -0.03 }$&$ 0.016  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 0.00  ^{+ 4.72  }_{ -0.00 }$&$ 2.20  \pm{ 0.13  }$&$ 87.98 ^{+  0.18 }_{ -1.10 }$&$ 10.7  ^{+ 0.2   }_{ -0.1  }$&$ 0.061  \pm{ 0.001  }$&$ 1177  \pm{ 12    }$&$ 349   \pm{ 2     }$& 3.6   &\textbf{ 8.4  }&0.972 &\textbf{ 0.999 } \\
K00246.02  & 11295426   & 136.3854  &$    9.60487 ^{+    0.00021 }_{   -0.00020 }$&$ 0.44  ^{+ 0.53  }_{ -0.16 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.45  ^{+ 0.26  }_{ -0.25 }$&$ 2.02  ^{+ 2.29  }_{ -1.79 }$&$ 0.92  \pm{ 0.13  }$&$ 88.41 ^{+ 0.59  }_{ -1.95 }$&$ 15.7  ^{+ 0.2   }_{ -0.2  }$&$ 0.090  \pm{ 0.001  }$&$ 967   \pm{ 10    }$&$ 58    \pm{ 3     }$& 2.9   & 0.7  &0.090 & 0.712  \\
K00260.01  & 8292840    & 172.7904  &$   10.49570 ^{+    0.00010 }_{   -0.00005 }$&$ 0.65  ^{+ 0.15  }_{ -0.04 }$&$ 0.010  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 1.79  \pm{ 0.17  }$&$ 86.86 ^{+ 0.04  }_{ -0.94 }$&$ 13.5  ^{+ 0.9   }_{ -1.0  }$&$ 0.101  \pm{ 0.003  }$&$ 1185  \pm{ 56    }$&$ 119   \pm{ 3     }$& 5.2   & 1.6  &0.295 & 0.954  \\
K00260.02  & 8292840    & 245.0413  &$  100.28340 ^{+    0.00028 }_{   -0.00085 }$&$ 0.15  ^{+ 0.41  }_{ -0.15 }$&$ 0.016  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 2.43  \pm{ 0.29  }$&$ 89.87 ^{+ 0.13  }_{ -0.39 }$&$ 69.6  ^{+ 6.0   }_{ -5.0  }$&$ 0.447  \pm{ 0.016  }$&$ 492   \pm{ 25    }$&$ 326   \pm{ 14    }$& 11.1  & 0.6  &0.357 & 0.965  \\
K00260.03  & 8292840    & 140.2944  &$   21.86964 ^{+    0.00018 }_{   -0.00023 }$&$ 0.56  ^{+ 0.16  }_{ -0.23 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.10  ^{+ 0.37  }_{ -0.10 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 1.56  \pm{ 0.19  }$&$ 88.66 ^{+ 0.62  }_{ -0.54 }$&$ 24.6  ^{+ 2.2   }_{ -1.7  }$&$ 0.162  \pm{ 0.006  }$&$ 837   \pm{ 42    }$&$ 127   \pm{ 5     }$& 5.9   & 1.4  &0.188 & 0.921  \\
K00262.01  & 11807274   & 172.6319  &$    7.81251 ^{+    0.00016 }_{   -0.00011 }$&$ 0.76  ^{+ 0.10  }_{ -0.04 }$&$ 0.009  ^{+ 0.001  }_{ -0.000 }$&$ 0.09  ^{+ 0.26  }_{ -0.09 }$&$ 0.25  ^{+ 0.59  }_{ -0.25 }$&$ 2.08  \pm{ 0.23  }$&$ 84.82 ^{+ 0.67  }_{ -1.14 }$&$ 8.7   ^{+ 0.8   }_{ -0.6  }$&$ 0.082  \pm{ 0.002  }$&$ 1388  \pm{ 69    }$&$ 90    \pm{ 3     }$& 4.8   & 0.6  &0.299 & 0.914  \\
K00262.02  & 11807274   & 136.9686  &$    9.37614 ^{+    0.00023 }_{   -0.00016 }$&$ 0.94  ^{+ 0.04  }_{ -0.00 }$&$ 0.015  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+ 0.70  }_{ -0.00 }$&$ 3.52  \pm{ 0.41  }$&$ 83.55 ^{+ 0.36  }_{ -0.81 }$&$ 9.2   ^{+ 1.0   }_{ -0.8  }$&$ 0.092  \pm{ 0.003  }$&$ 1388  \pm{ 68    }$&$ 94    \pm{ 4     }$& 3.2   & 1.1  &0.387 & 0.940  \\
K00270.01  & 6528464    & 175.0152  &$   12.58250 ^{+    0.00011 }_{   -0.00013 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.009  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 1.50  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -0.92 }$&$ 14.6  ^{+ 1.3   }_{ -1.0  }$&$ 0.104  \pm{ 0.002  }$&$ 965   \pm{ 51    }$&$ 108   \pm{ 5     }$& 6.6   & 2.1  &0.200 & 0.862  \\
K00270.02  & 6528464    & 162.0396  &$   33.67312 ^{+    0.00039 }_{   -0.00022 }$&$ 0.45  ^{+ 0.16  }_{ -0.45 }$&$ 0.012  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.55  }_{ -0.00 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 1.96  \pm{ 0.20  }$&$ 89.07 ^{+ 0.93  }_{ -0.41 }$&$ 28.2  ^{+ 2.2   }_{ -2.4  }$&$ 0.200  \pm{ 0.004  }$&$ 700   \pm{ 36    }$&$ 165   \pm{ 10    }$& 8.4   & 1.1  &0.165 & 0.832  \\
K00271.01  & 9451706    & 172.5460  &$   48.63057 ^{+    0.00016 }_{   -0.00014 }$&$ 0.51  ^{+ 0.13  }_{ -0.44 }$&$ 0.018  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 2.44  \pm{ 0.26  }$&$ 89.37 ^{+ 0.54  }_{ -0.24 }$&$ 47.0  ^{+ 3.6   }_{ -4.4  }$&$ 0.274  \pm{ 0.011  }$&$ 599   \pm{ 32    }$&$ 358   \pm{ 13    }$& 6.9   &\textbf{ 3.7  }&0.575 & 0.985  \\
K00271.02  & 9451706    & 209.0731  &$   29.39241 ^{+    0.00009 }_{   -0.00013 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.016  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.48  ^{+  0.33 }_{ -0.48 }$&$ 2.20  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -0.76 }$&$ 32.9  ^{+ 2.3   }_{ -2.4  }$&$ 0.196  \pm{ 0.007  }$&$ 719   \pm{ 34    }$&$ 316   \pm{ 10    }$& 7.0   &\textbf{ 3.4  }&0.654 & 0.990  \\
K00271.03  & 9451706    & 141.5109  &$   14.43593 ^{+    0.00034 }_{   -0.00039 }$&$ 0.13  ^{+ 0.66  }_{ -0.13 }$&$ 0.010  ^{+ 0.000  }_{ -0.002 }$&$ 0.49  ^{+ 0.22  }_{ -0.31 }$&$ 1.10  ^{+ 2.42  }_{ -1.10 }$&$ 1.31  \pm{ 0.21  }$&$ 89.65 ^{+ 0.35  }_{ -1.94 }$&$ 21.1  ^{+ 1.8   }_{ -1.9  }$&$ 0.122  \pm{ 0.005  }$&$ 892   \pm{ 56    }$&$ 105   \pm{ 6     }$& 3.2   &\textbf{ 3.0  }&0.217 & 0.933  \\
K00274.01  & 8077137    & 175.9276  &$   15.09205 ^{+    0.00088 }_{   -0.00060 }$&$ 0.13  ^{+ 0.48  }_{ -0.13 }$&$ 0.004  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.02  ^{+ 0.28  }_{ -0.02 }$&$ 0.77  \pm{ 0.13  }$&$ 89.57 ^{+ 0.43  }_{ -1.58 }$&$ 17.1  ^{+ 1.7   }_{ -1.4  }$&$ 0.127  \pm{ 0.004  }$&$ 970   \pm{ 64    }$&$ 24    \pm{ 6     }$& 6.6   & 0.7  &0.014 & 0.263  \\
K00274.02  & 8077137    & 153.4920  &$   22.79519 ^{+    0.00089 }_{   -0.00132 }$&$ 0.48  ^{+ 0.27  }_{ -0.40 }$&$ 0.003  ^{+ 0.002  }_{ -0.000 }$&$ 0.07  ^{+ 0.29  }_{ -0.07 }$&$ 0.29  ^{+ 1.31  }_{ -0.29 }$&$ 0.58  \pm{ 0.23  }$&$ 88.80 ^{+ 1.01  }_{ -0.69 }$&$ 22.4  ^{+ 2.2   }_{ -1.6  }$&$ 0.167  \pm{ 0.005  }$&$ 843   \pm{ 54    }$&$ 18    \pm{ 8     }$& 6.6   & 0.6  &0.010 & 0.202  \\
K00275.01  & 10586004   & 176.8205  &$   15.79186 ^{+    0.00011 }_{   -0.00009 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 2.10  \pm{ 0.24  }$&$ 90.00 ^{+ 0.00  }_{ -0.67 }$&$ 18.9  ^{+ 1.9   }_{ -1.5  }$&$ 0.129  \pm{ 0.004  }$&$ 909   \pm{ 47    }$&$ 206   \pm{ 9     }$& 6.8   & 0.6  &0.347 & 0.930  \\
K00275.02  & 10586004   & 208.7874  &$   82.19970 ^{+    0.00024 }_{   -0.00026 }$&$ 0.18  ^{+ 0.34  }_{ -0.18 }$&$ 0.014  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 2.05  \pm{ 0.24  }$&$ 89.82 ^{+ 0.18  }_{ -0.36 }$&$ 59.6  ^{+ 5.1   }_{ -4.4  }$&$ 0.384  \pm{ 0.013  }$&$ 499   \pm{ 28    }$&$ 221   \pm{ 21    }$& 10.4  & 0.4  &0.109 & 0.754  \\
K00277.01  & 11401755   & 171.6976  &$   16.23069 ^{+    0.00004 }_{   -0.00004 }$&$ 0.51  ^{+ 0.07  }_{ -0.01 }$&$ 0.044  ^{+  0.005 }_{ -0.010 }$&$ 0.90  ^{+ 0.00  }_{ -0.02 }$&$ 4.71  ^{+ 0.10  }_{ -0.17 }$&$ 8.26  \pm{ 0.91  }$&$ 88.13 ^{+ 0.23  }_{ -0.41 }$&$ 16.2  ^{+ 1.2   }_{ -1.3  }$&$ 0.129  \pm{ 0.003  }$&$ 999   \pm{ 55    }$&$ 467   \pm{ 10    }$& 13.0  & 0.4  &0.661 & 0.980  \\
K00277.02  & 11401755   & 141.6820  &$   13.84943 ^{+    0.00048 }_{   -0.00061 }$&$ 0.61  ^{+ 0.72  }_{ -0.61 }$&$ 0.007  ^{+ 0.005  }_{ -0.002 }$&$ 0.00  ^{+ 0.68  }_{ -0.00 }$&$ 0.00  ^{+ 3.89  }_{ -0.08 }$&$ 1.36  \pm{ 0.60  }$&$ 87.66 ^{+ 2.34  }_{ -2.60 }$&$ 15.1  ^{+ 1.3   }_{ -1.3  }$&$ 0.116  \pm{ 0.003  }$&$ 1024  \pm{ 63    }$&$ 57    \pm{ 8     }$& 5.6   & 0.3  &0.006 & 0.138  \\
K00279.01  & 12314973   & 176.7045  &$   28.45499 ^{+    0.00003 }_{   -0.00003 }$&$ 0.56  ^{+ 0.21  }_{ -0.25 }$&$ 0.035  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 1.29  }_{ -0.00 }$&$ 7.18  \pm{ 1.37  }$&$ 88.59 ^{+ 0.76  }_{ -1.06 }$&$ 23.1  ^{+ 3.4   }_{ -4.1  }$&$ 0.200  \pm{ 0.008  }$&$ 893   \pm{ 86    }$&$ 1406  \pm{ 14    }$& 8.3   & 0.5  &0.732 & 0.993  \\
K00279.02  & 12314973   & 136.9443  &$   15.41299 ^{+    0.00012 }_{   -0.00011 }$&$ 0.59  ^{+ 0.10  }_{ -0.07 }$&$ 0.019  ^{+  0.000 }_{ -0.004 }$&$ 0.65  ^{+ 0.13  }_{ -0.56 }$&$ 4.47  ^{+ 0.35  }_{ -3.37 }$&$ 3.93  \pm{ 1.08  }$&$ 87.57 ^{+ 0.91  }_{ -1.49 }$&$ 15.1  ^{+ 4.1   }_{ -2.9  }$&$ 0.132  \pm{ 0.005  }$&$ 1142  \pm{ 169   }$&$ 283   \pm{ 10    }$& 7.4   & 0.1  &0.326 & 0.960  \\
K00279.03  & 12314973   & 136.1570  &$    7.51465 ^{+    0.00029 }_{   -0.00027 }$&$ 0.09  ^{+ 0.34  }_{ -0.09 }$&$ 0.006  ^{+  0.000 }_{ -0.002 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.99  \pm{ 0.30  }$&$ 89.56 ^{+ 0.44  }_{ -1.80 }$&$ 11.5  ^{+ 3.5   }_{ -2.3  }$&$ 0.077  \pm{ 0.006  }$&$ 1216  \pm{ 187   }$&$ 45    \pm{ 5     }$& 4.7   & 0.5  &0.006 & 0.239  \\
K00282.01  & 5088536    & 182.1039  &$   27.50868 ^{+    0.00006 }_{   -0.00007 }$&$ 0.38  ^{+ 0.14  }_{ -0.38 }$&$ 0.023  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 2.90  \pm{ 0.25  }$&$ 89.34 ^{+ 0.66  }_{ -0.31 }$&$ 32.6  ^{+ 2.5   }_{ -2.4  }$&$ 0.178  \pm{ 0.005  }$&$ 683   \pm{ 29    }$&$ 640   \pm{ 9     }$& 6.1   & 1.1  &0.859 & 0.997  \\
K00282.02  & 5088536    & 139.0684  &$    8.45742 ^{+    0.00026 }_{   -0.00023 }$&$ 0.00  ^{+ 0.58  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.44  ^{+ 0.08  }_{ -0.44 }$&$ 0.09  ^{+ 0.16  }_{ -0.09 }$&$ 0.92  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -2.14 }$&$ 15.3  ^{+ 1.3   }_{ -1.1  }$&$ 0.081  \pm{ 0.003  }$&$ 988   \pm{ 55    }$&$ 79    \pm{ 4     }$& 3.6   & 0.4  &0.029 & 0.597  \\
K00282.03  & 5088536    & 201.1697  &$   87.51870 ^{+    0.02042 }_{   -0.02048 }$&$ 0.92  ^{+ 0.80  }_{ -0.52 }$&$ 0.016  ^{+ 0.005  }_{ -0.011 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 1.99  \pm{ 0.98  }$&$ 89.28 ^{+ 0.40  }_{ -0.62 }$&$ 72.0  ^{+ 6.8   }_{ -5.1  }$&$ 0.385  \pm{ 0.012  }$&$ 455   \pm{ 29    }$&$ 111   \pm{ 16    }$& 3.9   & 0.0  &0.003 & 0.135  \\
K00283.01  & 5695396    & 170.5985  &$   16.09194 ^{+    0.00007 }_{   -0.00006 }$&$ 0.76  ^{+ 0.06  }_{ -0.27 }$&$ 0.021  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 0.00  ^{+ 0.74  }_{ -0.00 }$&$ 2.32  \pm{ 0.30  }$&$ 88.32 ^{+ 0.72  }_{ -0.29 }$&$ 25.9  ^{+ 2.1   }_{ -2.1  }$&$ 0.125  \pm{ 0.004  }$&$ 740   \pm{ 42    }$&$ 444   \pm{ 6     }$& 3.2   &\textbf{ 6.1  }&0.890 & 0.995  \\
K00283.02  & 5695396    & 154.4205  &$   25.51704 ^{+    0.00122 }_{   -0.00089 }$&$ 0.22  ^{+ 0.38  }_{ -0.22 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.81  \pm{ 0.13  }$&$ 89.64 ^{+ 0.36  }_{ -0.63 }$&$ 35.0  ^{+ 3.2   }_{ -3.0  }$&$ 0.170  \pm{ 0.006  }$&$ 638   \pm{ 38    }$&$ 69    \pm{ 8     }$& 5.5   & 0.9  &0.012 & 0.230  \\
K00284.01  & 6021275    & 179.4253  &$   18.00999 ^{+    0.00036 }_{   -0.00034 }$&$ 0.75  ^{+ 0.25  }_{ -0.75 }$&$ 0.016  ^{+ 0.000  }_{ -0.005 }$&$ 0.68  ^{+ 0.21  }_{ -0.09 }$&$ 4.12  ^{+ 0.23  }_{ -0.75 }$&$ 1.88  \pm{ 0.38  }$&$ 88.44 ^{+ 1.56  }_{ -0.60 }$&$ 27.0  ^{+ 2.6   }_{ -2.4  }$&$ 0.136  \pm{ 0.005  }$&$ 750   \pm{ 44    }$&$ 181   \pm{ 8     }$& 3.7   & 1.2  &0.165 & 0.908  \\
K00284.02  & 6021275    & 169.6420  &$    6.41483 ^{+    0.00014 }_{   -0.00013 }$&$ 0.72  ^{+  0.28 }_{ -0.72 }$&$ 0.011  ^{+  0.001 }_{ -0.003 }$&$ 0.77  ^{+  0.23 }_{ -0.77 }$&$ 4.12  ^{+ 0.90  }_{ -4.12 }$&$ 1.33  \pm{ 0.15  }$&$ 87.00 ^{+ 3.00  }_{ -1.33 }$&$ 13.5  ^{+ 1.2   }_{ -1.0  }$&$ 0.068  \pm{ 0.003  }$&$ 1061  \pm{ 58    }$&$ 120   \pm{ 5     }$& 3.8   & 1.4  &0.076 & 0.803  \\
K00284.03  & 6021275    & 168.8602  &$    6.17818 ^{+    0.00013 }_{   -0.00013 }$&$ 0.15  ^{+ 0.21  }_{ -0.15 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 1.02  \pm{ 0.13  }$&$ 89.34 ^{+ 0.66  }_{ -0.96 }$&$ 13.3  ^{+ 1.0   }_{ -1.1  }$&$ 0.067  \pm{ 0.003  }$&$ 1080  \pm{ 58    }$&$ 103   \pm{ 5     }$& 3.5   & 1.0  &0.060 & 0.763  \\
K00284.04  & 6021275    & 239.1980  &$  110.29290 ^{+    0.14011 }_{   -0.07637 }$&$ 1.12  ^{+ 0.99  }_{ -0.66 }$&$ 0.011  ^{+ 0.013  }_{ -0.004 }$&$ 0.86  ^{+ 0.04  }_{ -0.04 }$&$ 4.01  ^{+ 0.29  }_{ -0.58 }$&$ 1.30  \pm{ 1.04  }$&$ 89.30 ^{+ 0.42  }_{ -0.63 }$&$ 90.0  ^{+ 8.2   }_{ -6.1  }$&$ 0.454  \pm{ 0.019  }$&$ 411   \pm{ 23    }$&$ 82    \pm{ 25    }$& 7.4   & 0.8  &0.023 & 0.546  \\
K00285.01  & 6196457    & 179.2804  &$   13.74878 ^{+    0.00005 }_{   -0.00005 }$&$ 0.59  ^{+ 0.08  }_{ -0.02 }$&$ 0.022  ^{+ 0.000  }_{ -0.001 }$&$ 0.48  ^{+ 0.17  }_{ -0.12 }$&$ 4.47  ^{+ 0.69  }_{ -0.33 }$&$ 3.95  \pm{ 0.38  }$&$ 87.82 ^{+ 0.31  }_{ -0.53 }$&$ 15.8  ^{+ 1.5   }_{ -1.1  }$&$ 0.118  \pm{ 0.003  }$&$ 990   \pm{ 58    }$&$ 419   \pm{ 7     }$& 6.3   & 1.0  &0.829 & 0.996  \\
K00285.02  & 6196457    & 147.9103  &$   26.72428 ^{+    0.00022 }_{   -0.00024 }$&$ 0.52  ^{+ 0.10  }_{ -0.26 }$&$ 0.016  ^{+ 0.002  }_{ -0.004 }$&$ 0.87  ^{+ 0.03  }_{ -0.66 }$&$ 4.67  ^{+ 0.38  }_{ -0.77 }$&$ 2.79  \pm{ 0.55  }$&$ 88.80 ^{+ 0.59  }_{ -0.30 }$&$ 24.9  ^{+ 2.7   }_{ -1.9  }$&$ 0.183  \pm{ 0.006  }$&$ 784   \pm{ 48    }$&$ 193   \pm{ 11    }$& 9.9   & 0.5  &0.383 & 0.969  \\
K00285.03  & 6196457    & 134.2716  &$   49.35899 ^{+    0.00071 }_{   -0.00089 }$&$ 0.52  ^{+ 0.39  }_{ -0.50 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.00  ^{+ 3.79  }_{ -0.00 }$&$ 1.96  \pm{ 0.26  }$&$ 89.20 ^{+ 0.77  }_{ -0.65 }$&$ 37.4  ^{+ 3.8   }_{ -2.9  }$&$ 0.275  \pm{ 0.008  }$&$ 640   \pm{ 39    }$&$ 129   \pm{ 16    }$& 8.8   & 0.5  &0.040 & 0.674  \\
K00289.01  & 10386922   & 138.7360  &$   26.62940 ^{+    0.00217 }_{   -0.00258 }$&$ 0.65  ^{+ 0.20  }_{ -0.56 }$&$ 0.021  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 0.72  }_{ -0.00 }$&$ 4.51  \pm{ 1.64  }$&$ 88.19 ^{+ 1.61  }_{ -1.62 }$&$ 19.9  ^{+ 4.6   }_{ -6.2  }$&$ 0.185  \pm{ 0.017  }$&$ 854   \pm{ 139   }$&$ 482   \pm{ 16    }$& 7.8   & 0.1  &0.481 & 0.959  \\
K00289.02  & 10386922   & 403.6729  &$  296.63709 ^{+    0.00057 }_{   -0.00042 }$&$ 0.65  ^{+ 0.22  }_{ -0.61 }$&$ 0.051  ^{+ 0.003  }_{ -0.005 }$&$ 0.09  ^{+ 0.35  }_{ -0.09 }$&$ 1.65  ^{+ 0.76  }_{ -1.65 }$&$ 9.86  \pm{ 3.07  }$&$ 89.66 ^{+ 0.32  }_{ -0.33 }$&$ 113.5 ^{+ 20.3  }_{ -34.9 }$&$ 0.908  \pm{ 0.062  }$&$ 366   \pm{ 59    }$&$ 2838  \pm{ 67    }$& 16.2  & 0.1  &0.369 & 0.936  \\
K00291.01  & 10933561   & 185.1521  &$   31.51789 ^{+    0.00044 }_{   -0.00028 }$&$ 0.40  ^{+ 0.17  }_{ -0.40 }$&$ 0.017  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 2.60  \pm{ 0.30  }$&$ 89.21 ^{+ 0.79  }_{ -0.37 }$&$ 30.1  ^{+ 2.6   }_{ -2.7  }$&$ 0.194  \pm{ 0.005  }$&$ 688   \pm{ 41    }$&$ 361   \pm{ 20    }$& 7.7   & 0.5  &0.091 & 0.714  \\
K00291.02  & 10933561   & 134.1052  &$    8.12986 ^{+    0.00017 }_{   -0.00014 }$&$ 0.90  ^{+ 0.06  }_{ -0.02 }$&$ 0.015  ^{+ 0.002  }_{ -0.001 }$&$ 0.09  ^{+ 0.09  }_{ -0.09 }$&$ 0.04  ^{+ 0.97  }_{ -0.04 }$&$ 2.32  \pm{ 0.31  }$&$ 85.40 ^{+ 0.46  }_{ -0.70 }$&$ 11.7  ^{+ 1.1   }_{ -0.8  }$&$ 0.079  \pm{ 0.002  }$&$ 1107  \pm{ 58    }$&$ 138   \pm{ 9     }$& 2.7   & 1.1  &0.088 & 0.707  \\
K00295.01  & 11547513   & 171.8763  &$    5.31743 ^{+    0.00006 }_{   -0.00006 }$&$ 0.94  ^{+ 0.01  }_{ -0.05 }$&$ 0.020  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.52  }_{ -0.00 }$&$ 6.23  \pm{ 1.47  }$&$ 78.93 ^{+ 2.69  }_{ -1.83 }$&$ 5.0   ^{+ 1.1   }_{ -0.8  }$&$ 0.064  \pm{ 0.009  }$&$ 1811  \pm{ 216   }$&$ 288   \pm{ 6     }$& 3.3   & 1.3  &0.676 & 0.981  \\
K00295.02  & 11547513   & 135.5088  &$   10.10575 ^{+    0.00032 }_{   -0.00030 }$&$ 0.98  ^{+ 0.01  }_{ -0.03 }$&$ 0.012  ^{+ 0.007  }_{ -0.001 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.66  }_{ -0.00 }$&$ 3.00  \pm{ 1.15  }$&$ 83.90 ^{+ 0.95  }_{ -1.03 }$&$ 9.1   ^{+ 1.6   }_{ -1.8  }$&$ 0.096  \pm{ 0.010  }$&$ 1298  \pm{ 156   }$&$ 113   \pm{ 8     }$& 2.3   & 0.7  &0.093 & 0.719  \\
K00298.01  & 12785320   & 178.3053  &$   19.96000 ^{+    0.00079 }_{   -0.00087 }$&$ 0.93  ^{+ 0.50  }_{ -0.82 }$&$ 0.008  ^{+ 0.006  }_{ -0.006 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.20  ^{+ 0.34  }_{ -0.20 }$&$ 1.00  \pm{ 0.96  }$&$ 85.10 ^{+ 4.67  }_{ -2.90 }$&$ 26.3  ^{+ 15.2  }_{ -10.1 }$&$ 0.143  \pm{ 0.010  }$&$ 1101  \pm{ 1394  }$&$ 81     \pm{ 17    }$& 5.4   & 0.2  &0.032 & 0.450  \\
K00298.02  & 12785320   & 170.7233  &$   57.38425 ^{+    0.00707 }_{   -0.00016 }$&$ 0.67  ^{+ 0.18  }_{ -0.67 }$&$ 0.014  ^{+ 0.004  }_{ -0.003 }$&$ 0.00  ^{+ 0.59  }_{ -0.00 }$&$ 0.00  ^{+ 4.47  }_{ -0.00 }$&$ 1.71  \pm{ 0.99  }$&$ 89.40 ^{+ 0.60  }_{ -0.61 }$&$ 54.0  ^{+ 27.3  }_{ -20.5 }$&$ 0.289  \pm{ 0.019  }$&$ 455   \pm{ 122   }$&$ 237   \pm{ 27    }$& 5.2   & 0.7  &0.011 & 0.211  \\
K00301.01  & 3642289    & 171.7134  &$    6.00255 ^{+    0.00006 }_{   -0.00009 }$&$ 0.30  ^{+ 0.11  }_{ -0.30 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.00  ^{+ 1.15  }_{ -0.00 }$&$ 1.96  \pm{ 0.33  }$&$ 88.34 ^{+ 1.66  }_{ -0.82 }$&$ 10.4  ^{+ 1.2   }_{ -1.5  }$&$ 0.071  \pm{ 0.003  }$&$ 1296  \pm{ 96    }$&$ 199   \pm{ 6     }$& 4.2   & 0.9  &0.122 & 0.776  \\
K00301.02  & 3642289    & 141.3742  &$   11.44883 ^{+    0.00049 }_{   -0.00048 }$&$ 0.20  ^{+ 0.36  }_{ -0.20 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 1.23  \pm{ 0.35  }$&$ 89.29 ^{+ 0.71  }_{ -1.36 }$&$ 15.7  ^{+ 4.2   }_{ -3.1  }$&$ 0.109  \pm{ 0.005  }$&$ 1040  \pm{ 141   }$&$ 79    \pm{ 9     }$& 5.3   & 0.3  &0.005 & 0.113  \\
K00304.01  & 6029239    & 174.9087  &$    8.51205 ^{+    0.00005 }_{   -0.00005 }$&$ 0.95  ^{+ 0.35  }_{ -0.07 }$&$ 0.027  ^{+ 0.003  }_{ -0.004 }$&$ 0.08  ^{+ 0.31  }_{ -0.08 }$&$ 0.00  ^{+ 1.49  }_{ -0.00 }$&$ 6.02  \pm{ 1.73  }$&$ 84.54 ^{+ 1.39  }_{ -6.28 }$&$ 9.2   ^{+ 2.3   }_{ -2.1  }$&$ 0.086  \pm{ 0.003  }$&$ 1291  \pm{ 177   }$&$ 588   \pm{ 7     }$& 2.6   & 1.1  &0.464 & 0.956  \\
K00304.02  & 6029239    & 136.5633  &$    5.51835 ^{+    0.00019 }_{   -0.00022 }$&$ 0.85  ^{+ 0.22  }_{ -0.33 }$&$ 0.006  ^{+ 0.000  }_{ -0.003 }$&$ 0.24  ^{+  0.08 }_{ -0.24 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 1.41  \pm{ 0.47  }$&$ 83.05 ^{+ 2.84  }_{ -1.54 }$&$ 6.7   ^{+ 1.8   }_{ -1.4  }$&$ 0.064  \pm{ 0.002  }$&$ 1535  \pm{ 241   }$&$ 34    \pm{ 6     }$& 3.5   & 0.3  &0.006 & 0.140  \\
K00307.01  & 6289257    & 176.2694  &$   19.67423 ^{+    0.00043 }_{   -0.00036 }$&$ 0.60  ^{+ 0.15  }_{ -0.59 }$&$ 0.013  ^{+ 0.002  }_{ -0.001 }$&$ 0.27  ^{+ 0.31  }_{ -0.27 }$&$ 0.38  ^{+ 3.11  }_{ -0.38 }$&$ 1.56  \pm{ 0.22  }$&$ 88.78 ^{+ 1.19  }_{ -0.40 }$&$ 28.1  ^{+ 2.7   }_{ -2.1  }$&$ 0.147  \pm{ 0.006  }$&$ 765   \pm{ 42    }$&$ 221   \pm{ 11    }$& 4.1   & 1.9  &0.059 & 0.609  \\
K00307.02  & 6289257    & 131.5367  &$    5.21106 ^{+    0.00015 }_{   -0.00012 }$&$ 0.44  ^{+ 0.13  }_{ -0.44 }$&$ 0.009  ^{+ 0.007  }_{ -0.000 }$&$ 0.43  ^{+ 0.46  }_{ -0.43 }$&$ 3.66  ^{+ 1.14  }_{ -3.66 }$&$ 1.09  \pm{ 0.44  }$&$ 87.79 ^{+ 2.21  }_{ -0.89 }$&$ 11.7  ^{+ 1.0   }_{ -1.0  }$&$ 0.061  \pm{ 0.003  }$&$ 1201  \pm{ 71    }$&$ 103   \pm{ 5     }$& 3.6   & 2.0  &0.017 & 0.298  \\
K00312.01  & 7050989    & 175.5857  &$   11.57894 ^{+    0.00019 }_{   -0.00010 }$&$ 0.63  ^{+ 0.13  }_{ -0.19 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.05  ^{+ 0.43  }_{ -0.05 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.78  \pm{ 0.26  }$&$ 88.15 ^{+ 0.65  }_{ -0.55 }$&$ 18.9  ^{+ 1.8   }_{ -1.4  }$&$ 0.106  \pm{ 0.004  }$&$ 924   \pm{ 53    }$&$ 236   \pm{ 8     }$& 3.6   & 0.4  &0.049 & 0.563  \\
K00312.02  & 7050989    & 131.9683  &$   16.39922 ^{+    0.00015 }_{   -0.00010 }$&$ 0.01  ^{+ 0.64  }_{ -0.01 }$&$ 0.013  ^{+ 0.003  }_{ -0.002 }$&$ 0.72  ^{+  0.08 }_{ -0.61 }$&$ 6.28  ^{+  0.00 }_{ -6.22 }$&$ 1.76  \pm{ 0.34  }$&$ 89.97 ^{+ 0.03  }_{ -1.66 }$&$ 23.8  ^{+ 2.1   }_{ -1.9  }$&$ 0.134  \pm{ 0.005  }$&$ 832   \pm{ 51    }$&$ 224   \pm{ 10    }$& 3.6   & 0.5  &0.036 & 0.481  \\
K00313.01  & 7419318    & 177.6356  &$   18.73572 ^{+    0.00015 }_{   -0.00018 }$&$ 0.63  ^{+ 0.09  }_{ -0.26 }$&$ 0.022  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.00  ^{+ 0.87  }_{ -0.00 }$&$ 2.11  \pm{ 0.26  }$&$ 88.91 ^{+ 0.51  }_{ -0.25 }$&$ 32.8  ^{+ 2.8   }_{ -2.4  }$&$ 0.134  \pm{ 0.004  }$&$ 616   \pm{ 32    }$&$ 604   \pm{ 15    }$& 3.4   & 1.0  &0.530 & 0.966  \\
K00313.02  & 7419318    & 179.8861  &$    8.43640 ^{+    0.00010 }_{   -0.00011 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.54  \pm{ 0.15  }$&$ 90.00 ^{+ 0.00  }_{ -0.72 }$&$ 18.9  ^{+ 1.4   }_{ -1.4  }$&$ 0.079  \pm{ 0.003  }$&$ 814   \pm{ 35    }$&$ 350   \pm{ 10    }$& 3.4   & 0.3  &0.356 & 0.933  \\
K00314.01  & 7603200    & 177.8521  &$   13.78105 ^{+    0.00010 }_{   -0.00008 }$&$ 1.14  ^{+ 0.29  }_{ -0.30 }$&$ 0.032  ^{+ 0.001  }_{ -0.010 }$&$ 0.19  ^{+ 0.25  }_{ -0.17 }$&$ 1.04  ^{+ 2.41  }_{ -1.01 }$&$ 6.06  \pm{ 3.45  }$&$ 85.13 ^{+ 2.88  }_{ -2.80 }$&$ 13.2  ^{+ 12.7  }_{ -3.4  }$&$ 0.105  \pm{ 0.013  }$&$ 713   \pm{ 210   }$&$ 729   \pm{ 10    }$& 2.7   & 0.4  &0.797 & 0.995  \\
K00314.02  & 7603200    & 171.0047  &$   23.08945 ^{+    0.00017 }_{   -0.00018 }$&$ 0.87  ^{+ 0.14  }_{ -0.24 }$&$ 0.027  ^{+ 0.011  }_{ -0.005 }$&$ 0.01  ^{+ 0.58  }_{ -0.01 }$&$ 4.67  ^{+  0.76 }_{ -4.67 }$&$ 2.50  \pm{ 1.35  }$&$ 88.67 ^{+ 0.71  }_{ -0.92 }$&$ 33.8  ^{+ 18.0  }_{ -10.4 }$&$ 0.134  \pm{ 0.011  }$&$ 428   \pm{ 107   }$&$ 498   \pm{ 16    }$& 2.5   &\textbf{ 4.3  }&0.699 & 0.991  \\
K00314.03  & 7603200    & 133.5522  &$   10.31202 ^{+    0.00022 }_{   -0.00028 }$&$ 0.76  ^{+ 0.41  }_{ -0.36 }$&$ 0.008  ^{+ 0.000  }_{ -0.004 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.70  \pm{ 0.46  }$&$ 88.02 ^{+ 0.91  }_{ -0.91 }$&$ 19.7  ^{+ 10.3  }_{ -7.7  }$&$ 0.079  \pm{ 0.007  }$&$ 552   \pm{ 173   }$&$ 57    \pm{ 9     }$& 2.3   & 0.5  &0.037 & 0.655  \\
K00316.01  & 8008067    & 137.5880  &$   15.77120 ^{+    0.00125 }_{   -0.00011 }$&$ 0.86  ^{+ 0.09  }_{ -0.37 }$&$ 0.024  ^{+ 0.002  }_{ -0.003 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 1.59  }_{ -0.00 }$&$ 6.43  \pm{ 2.24  }$&$ 85.99 ^{+ 2.69  }_{ -2.03 }$&$ 11.5  ^{+ 6.1   }_{ -2.7  }$&$ 0.129  \pm{ 0.005  }$&$ 1061  \pm{ 205   }$&$ 534   \pm{ 13    }$& 5.4   &\textbf{ 11.7 }&0.398 & 0.971  \\
K00316.02  & 8008067    & 481.2644  &$  157.07021 ^{+    0.00048 }_{   -0.00129 }$&$ 0.92  ^{+ 0.04  }_{ -0.33 }$&$ 0.026  ^{+ 0.018  }_{ -0.006 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 4.59  }_{ -0.00 }$&$ 6.35  \pm{ 4.04  }$&$ 89.16 ^{+ 0.51  }_{ -0.49 }$&$ 59.0  ^{+ 41.3  }_{ -18.4 }$&$ 0.597  \pm{ 0.025  }$&$ 472   \pm{ 119   }$&$ 537   \pm{ 41    }$& 8.7   & 2.6  &0.057 & 0.751  \\
K00316.03  & 8008067    & 131.7801  &$    7.30569 ^{+    0.00008 }_{   -0.00009 }$&$ 0.96  ^{+ 0.01  }_{ -0.06 }$&$ 0.026  ^{+ 0.004  }_{ -0.006 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 5.00  \pm{ 1.70  }$&$ 84.48 ^{+ 1.68  }_{ -1.52 }$&$ 9.3   ^{+ 3.4   }_{ -1.7  }$&$ 0.077  \pm{ 0.003  }$&$ 1186  \pm{ 166   }$&$ 254   \pm{ 8     }$& 2.1   &\textbf{ 8.3  }&0.221 & 0.934  \\
K00321.01  & 8753657    & 170.4543  &$    2.42631 ^{+    0.00002 }_{   -0.00002 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 4.00  }_{ -0.00 }$&$ 1.37  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -3.31 }$&$ 6.6   ^{+ 0.4   }_{ -0.4  }$&$ 0.034  \pm{ 0.001  }$&$ 1434  \pm{ 57    }$&$ 193   \pm{ 3     }$& 2.9   & 0.7  &0.448 & 0.953  \\
K00321.02  & 8753657    & 132.3660  &$    4.62339 ^{+    0.00009 }_{   -0.00009 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.37  ^{+ 0.08  }_{ -0.37 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.82  \pm{ 0.11  }$&$ 90.00 ^{+  0.00 }_{ -2.87 }$&$ 10.5  ^{+ 0.8   }_{ -0.9  }$&$ 0.053  \pm{ 0.002  }$&$ 1134  \pm{ 61    }$&$ 63    \pm{ 5     }$& 3.1   & 0.5  &0.011 & 0.213  \\
K00326.01  & 9880467    & 171.0311  &$    8.97350 ^{+    0.00010 }_{   -0.00016 }$&$ 2.77  ^{+ 0.03  }_{ -1.22 }$&$ 0.031  ^{+ 0.006  }_{ -0.000 }$&$ 0.72  ^{+ 0.04  }_{ -0.09 }$&$ 1.80  ^{+  0.13 }_{ -1.57 }$&$ 13.90 \pm{ 1.49  }$&$ 60.00 ^{+ 13.81 }_{ -0.00 }$&$ 5.5   ^{+ 0.1   }_{ -0.0  }$&$ 0.106  \pm{ 0.002  }$&$ 1340  \pm{ 17    }$&$ 959   \pm{ 34    }$& 3.7   &\textbf{ 9.5  }&0.486 & 0.959  \\
K00326.02  & 9880467    & 151.2420  &$  108.52770 ^{+    0.00080 }_{   -0.00176 }$&$ 0.95  ^{+ 0.21  }_{ -0.32 }$&$ 0.041  ^{+  0.002 }_{ -0.023 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.00  ^{+ 1.52  }_{ -0.00 }$&$ 18.62 \pm{ 4.93  }$&$ 88.14 ^{+ 0.64  }_{ -0.40 }$&$ 29.1  ^{+ 0.3   }_{ -0.3  }$&$ 0.557  \pm{ 0.011  }$&$ 583   \pm{ 7     }$&$ 743   \pm{ 128   }$& 12.4  & 1.4  &0.486 & 0.959  \\
K00327.01  & 9881662    & 172.6615  &$    3.25428 ^{+    0.00005 }_{   -0.00005 }$&$ 0.11  ^{+ 0.35  }_{ -0.11 }$&$ 0.011  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 2.43  }_{ -0.00 }$&$ 1.43  \pm{ 0.17  }$&$ 89.21 ^{+ 0.79  }_{ -2.62 }$&$ 8.1   ^{+ 0.7   }_{ -0.7  }$&$ 0.045  \pm{ 0.002  }$&$ 1459  \pm{ 77    }$&$ 166   \pm{ 5     }$& 3.1   & 2.5  &0.425 & 0.949  \\
K00327.02  & 9881662    & 189.6005  &$   91.35250 ^{+    0.00655 }_{   -0.00037 }$&$ 0.00  ^{+ 0.67  }_{ -0.00 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.51  ^{+ 0.19  }_{ -0.48 }$&$ 0.01  ^{+ 0.11  }_{ -0.01 }$&$ 1.76  \pm{ 0.24  }$&$ 90.00 ^{+ 0.00  }_{ -0.50 }$&$ 75.8  ^{+ 8.0   }_{ -5.8  }$&$ 0.420  \pm{ 0.015  }$&$ 470   \pm{ 31    }$&$ 190   \pm{ 30    }$& 7.8   & 0.9  &0.043 & 0.526  \\
K00332.01  & 10290666   & 172.0875  &$    5.45851 ^{+    0.00006 }_{   -0.00006 }$&$ 0.01  ^{+ 0.31  }_{ -0.01 }$&$ 0.014  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 1.93  \pm{ 0.20  }$&$ 89.92 ^{+ 0.08  }_{ -1.76 }$&$ 10.6  ^{+ 0.8   }_{ -0.7  }$&$ 0.061  \pm{ 0.002  }$&$ 1175  \pm{ 50    }$&$ 269   \pm{ 8     }$& 4.0   & 0.8  &0.160 & 0.826  \\
K00332.02  & 10290666   & 135.3520  &$    6.86687 ^{+    0.00023 }_{   -0.00026 }$&$ 0.61  ^{+ 0.19  }_{ -0.61 }$&$ 0.006  ^{+ 0.002  }_{ -0.002 }$&$ 0.60  ^{+ 0.27  }_{ -0.60 }$&$ 3.48  ^{+ 1.33  }_{ -3.48 }$&$ 0.80  \pm{ 0.23  }$&$ 87.40 ^{+ 2.60  }_{ -0.78 }$&$ 13.2  ^{+ 1.1   }_{ -1.1  }$&$ 0.070  \pm{ 0.003  }$&$ 1039  \pm{ 60    }$&$ 42    \pm{ 9     }$& 3.5   & 0.0  &0.004 & 0.084  \\
K00338.01  & 10552611   & 174.5747  &$    7.01062 ^{+    0.00012 }_{   -0.00010 }$&$ 0.96  ^{+ 0.07  }_{ -0.05 }$&$ 0.020  ^{+ 0.007  }_{ -0.000 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.01  ^{+ 6.27  }_{ -0.01 }$&$ 6.15  \pm{ 1.16  }$&$ 79.62 ^{+ 0.75  }_{ -0.70 }$&$ 5.3   ^{+ 0.0   }_{ -0.0  }$&$ 0.070  \pm{ 0.001  }$&$ 1182  \pm{ 17    }$&$ 329   \pm{ 12    }$& 3.5   & 0.5  &0.061 & 0.619  \\
K00338.02  & 10552611   & 132.6397  &$    3.10753 ^{+    0.00005 }_{   -0.00007 }$&$ 0.88  ^{+ 0.05  }_{ -0.13 }$&$ 0.009  ^{+ 0.002  }_{ -0.003 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 2.81  \pm{ 0.82  }$&$ 73.48 ^{+ 2.48  }_{ -0.85 }$&$ 3.1   ^{+ 0.0   }_{ -0.0  }$&$ 0.041  \pm{ 0.000  }$&$ 1549  \pm{ 22    }$&$ 51    \pm{ 8     }$& 3.9   & 1.1  &0.008 & 0.172  \\
K00341.01  & 10878263   & 176.6658  &$   14.34123 ^{+    0.00020 }_{   -0.00024 }$&$ 0.65  ^{+ 0.06  }_{ -0.17 }$&$ 0.028  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 0.00  ^{+ 0.76  }_{ -0.00 }$&$ 2.91  \pm{ 0.34  }$&$ 88.57 ^{+ 0.45  }_{ -0.28 }$&$ 25.9  ^{+ 2.0   }_{ -1.9  }$&$ 0.114  \pm{ 0.004  }$&$ 717   \pm{ 35    }$&$ 936   \pm{ 33    }$& 3.3   & 0.3  &0.031 & 0.445  \\
K00341.02  & 10878263   & 177.6153  &$    4.69961 ^{+    0.00010 }_{   -0.00005 }$&$ 0.21  ^{+ 0.24  }_{ -0.21 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 1.48  \pm{ 0.17  }$&$ 89.01 ^{+ 0.99  }_{ -1.19 }$&$ 12.3  ^{+ 1.0   }_{ -0.9  }$&$ 0.054  \pm{ 0.002  }$&$ 1044  \pm{ 52    }$&$ 279   \pm{ 20    }$& 2.9   & 2.2  &0.014 & 0.261  \\
K00343.01  & 10982872   & 170.3356  &$    4.76170 ^{+    0.00004 }_{   -0.00003 }$&$ 0.33  ^{+ 0.24  }_{ -0.33 }$&$ 0.019  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.01  ^{+ 2.59  }_{ -0.01 }$&$ 2.47  \pm{ 0.28  }$&$ 88.08 ^{+ 1.92  }_{ -1.63 }$&$ 9.9   ^{+ 0.8   }_{ -0.9  }$&$ 0.054  \pm{ 0.002  }$&$ 1223  \pm{ 63    }$&$ 516   \pm{ 7     }$& 3.6   & 1.3  &0.720 & 0.992  \\
K00343.02  & 10982872   & 170.4966  &$    2.02413 ^{+    0.00002 }_{   -0.00002 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.24  ^{+  0.01 }_{ -0.24 }$&$ 1.59  \pm{ 0.17  }$&$ 90.00 ^{+ 0.00  }_{ -5.26 }$&$ 5.7   ^{+ 0.4   }_{ -0.4  }$&$ 0.031  \pm{ 0.001  }$&$ 1609  \pm{ 77    }$&$ 247   \pm{ 5     }$& 2.8   & 1.3  &0.487 & 0.979  \\
K00343.03  & 10982872   & 148.6985  &$   41.80925 ^{+    0.00011 }_{   -0.00012 }$&$ 0.07  ^{+ 0.43  }_{ -0.07 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.12  ^{+ 0.36  }_{ -0.12 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 1.65  \pm{ 0.21  }$&$ 89.91 ^{+ 0.09  }_{ -0.58 }$&$ 43.3  ^{+ 3.9   }_{ -2.9  }$&$ 0.231  \pm{ 0.008  }$&$ 575   \pm{ 28    }$&$ 206   \pm{ 26    }$& 7.2   & 0.8  &0.026 & 0.576  \\
K00353.01  & 11566064   & 176.5297  &$  152.10452 ^{+    0.00030 }_{   -0.00019 }$&$ 0.94  ^{+ 0.47  }_{ -0.26 }$&$ 0.060  ^{+ 0.009  }_{ -0.000 }$&$ 0.37  ^{+ 0.43  }_{ -0.37 }$&$ 3.30  ^{+ 1.37  }_{ -1.46 }$&$ 9.84  \pm{ 2.71  }$&$ 89.44 ^{+ 0.26  }_{ -0.58 }$&$ 90.2  ^{+ 23.9  }_{ -20.4 }$&$ 0.637  \pm{ 0.027  }$&$ 465   \pm{ 77    }$&$ 3340  \pm{ 82    }$& 7.2   & 1.3  &0.629 & 0.977  \\
K00353.02  & 11566064   & 135.0456  &$   30.65268 ^{+    0.00057 }_{   -0.00057 }$&$ 0.23  ^{+ 0.58  }_{ -0.23 }$&$ 0.014  ^{+ 0.005  }_{ -0.001 }$&$ 0.54  ^{+ 0.24  }_{ -0.48 }$&$ 2.95  ^{+ 1.53  }_{ -2.86 }$&$ 2.39  \pm{ 0.81  }$&$ 89.58 ^{+ 0.42  }_{ -1.47 }$&$ 30.6  ^{+ 8.1   }_{ -6.8  }$&$ 0.219  \pm{ 0.009  }$&$ 802   \pm{ 119   }$&$ 316   \pm{ 28    }$& 5.6   & 0.4  &0.051 & 0.572  \\
K00354.01  & 11568987   & 171.5200  &$   15.95995 ^{+    0.00013 }_{   -0.00011 }$&$ 0.27  ^{+ 0.23  }_{ -0.27 }$&$ 0.020  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 2.17  \pm{ 0.26  }$&$ 89.40 ^{+ 0.60  }_{ -0.56 }$&$ 26.1  ^{+ 2.5   }_{ -2.0  }$&$ 0.120  \pm{ 0.005  }$&$ 772   \pm{ 41    }$&$ 545   \pm{ 17    }$& 4.6   &\textbf{ 3.6  }&0.440 & 0.952  \\
K00354.02  & 11568987   & 135.8196  &$    7.37878 ^{+    0.00016 }_{   -0.00022 }$&$ 0.06  ^{+ 0.43  }_{ -0.06 }$&$ 0.009  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.98  \pm{ 0.15  }$&$ 89.78 ^{+ 0.22  }_{ -1.60 }$&$ 15.8  ^{+ 1.6   }_{ -1.4  }$&$ 0.071  \pm{ 0.003  }$&$ 983   \pm{ 62    }$&$ 130   \pm{ 11    }$& 3.5   & 1.6  &0.025 & 0.393  \\
K00369.01  & 7175184    & 174.4259  &$    5.88522 ^{+    0.00008 }_{   -0.00009 }$&$ 0.70  ^{+ 0.13  }_{ -0.29 }$&$ 0.010  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.00  ^{+ 0.72  }_{ -0.00 }$&$ 1.26  \pm{ 0.32  }$&$ 87.08 ^{+ 1.49  }_{ -1.14 }$&$ 12.9  ^{+ 2.5   }_{ -2.2  }$&$ 0.068  \pm{ 0.003  }$&$ 1145  \pm{ 125   }$&$ 118   \pm{ 5     }$& 2.4   & 0.7  &0.226 & 0.879  \\
K00369.02  & 7175184    & 135.5572  &$   10.10465 ^{+    0.00021 }_{   -0.00014 }$&$ 0.76  ^{+ 0.09  }_{ -0.18 }$&$ 0.012  ^{+ 0.005  }_{ -0.003 }$&$ 0.40  ^{+ 0.13  }_{ -0.40 }$&$ 3.80  ^{+ 1.16  }_{ -3.79 }$&$ 1.67  \pm{ 0.65  }$&$ 87.50 ^{+ 0.85  }_{ -0.91 }$&$ 16.7  ^{+ 3.2   }_{ -3.3  }$&$ 0.099  \pm{ 0.004  }$&$ 1011  \pm{ 118   }$&$ 116   \pm{ 6     }$& 2.9   & 1.2  &0.130 & 0.789  \\
K00370.01  & 8494142    & 203.6467  &$   42.88255 ^{+    0.00019 }_{   -0.00028 }$&$ 0.58  ^{+ 0.10  }_{ -0.32 }$&$ 0.019  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 4.12  \pm{ 0.42  }$&$ 88.80 ^{+ 0.74  }_{ -0.35 }$&$ 27.6  ^{+ 2.0   }_{ -2.4  }$&$ 0.254  \pm{ 0.007  }$&$ 759   \pm{ 43    }$&$ 415   \pm{ 14    }$& 9.8   & 0.6  &0.049 & 0.561  \\
K00370.02  & 8494142    & 151.5320  &$   22.95036 ^{+    0.00033 }_{   -0.00036 }$&$ 0.84  ^{+ 0.07  }_{ -0.11 }$&$ 0.014  ^{+ 0.000  }_{ -0.002 }$&$ 0.31  ^{+ 0.04  }_{ -0.31 }$&$ 3.63  ^{+ 1.35  }_{ -3.63 }$&$ 3.07  \pm{ 0.43  }$&$ 87.30 ^{+ 0.45  }_{ -0.41 }$&$ 17.9  ^{+ 1.7   }_{ -1.3  }$&$ 0.167  \pm{ 0.005  }$&$ 948   \pm{ 52    }$&$ 132   \pm{ 10    }$& 5.4   & 0.7  &0.087 & 0.705  \\
K00623.01  & 12068975   & 174.0660  &$   10.34968 ^{+    0.00023 }_{   -0.00020 }$&$ 0.43  ^{+ 0.26  }_{ -0.42 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.15  ^{+ 0.39  }_{ -0.15 }$&$ 0.34  ^{+ 3.17  }_{ -0.34 }$&$ 1.35  \pm{ 0.17  }$&$ 88.38 ^{+ 1.62  }_{ -1.20 }$&$ 15.1  ^{+ 1.5   }_{ -1.1  }$&$ 0.089  \pm{ 0.002  }$&$ 1007  \pm{ 59    }$&$ 123   \pm{ 6     }$& 4.6   & 1.3  &0.049 & 0.722  \\
K00623.02  & 12068975   & 179.4702  &$   15.67757 ^{+    0.00034 }_{   -0.00033 }$&$ 0.47  ^{+ 0.22  }_{ -0.47 }$&$ 0.010  ^{+ 0.001  }_{ -0.000 }$&$ 0.08  ^{+ 0.48  }_{ -0.08 }$&$ 0.04  ^{+ 0.57  }_{ -0.04 }$&$ 1.37  \pm{ 0.16  }$&$ 88.58 ^{+ 1.42  }_{ -0.80 }$&$ 19.7  ^{+ 2.2   }_{ -1.7  }$&$ 0.118  \pm{ 0.003  }$&$ 891   \pm{ 52    }$&$ 111   \pm{ 8     }$& 5.5   & 1.3  &0.035 & 0.643  \\
K00623.03  & 12068975   & 171.4706  &$    5.59935 ^{+    0.00011 }_{   -0.00010 }$&$ 0.01  ^{+ 0.76  }_{ -0.01 }$&$ 0.008  ^{+ 0.001  }_{ -0.000 }$&$ 0.43  ^{+ 0.14  }_{ -0.43 }$&$ 0.02  ^{+ 0.30  }_{ -0.02 }$&$ 1.13  \pm{ 0.13  }$&$ 89.97 ^{+ 0.03  }_{ -5.38 }$&$ 10.1  ^{+ 0.9   }_{ -0.8  }$&$ 0.059  \pm{ 0.002  }$&$ 1256  \pm{ 96    }$&$ 89    \pm{ 4     }$& 4.0   & 1.9  &0.017 & 0.464  \\
K00623.04  & 12068975   & 154.4160  &$   25.20971 ^{+    0.00116 }_{   -0.00091 }$&$ 0.82  ^{+ 0.96  }_{ -0.09 }$&$ 0.008  ^{+ 0.016  }_{ -0.006 }$&$ 0.68  ^{+  0.31 }_{ -0.62 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.06  \pm{ 1.48  }$&$ 87.95 ^{+ 0.49  }_{ -1.36 }$&$ 28.5  ^{+ 2.6   }_{ -2.3  }$&$ 0.161  \pm{ 0.004  }$&$ 813   \pm{ 102   }$&$ 75    \pm{ 10    }$& 5.5   & 0.4  &0.004 & 0.177  \\
K00626.01  & 4478168    & 172.2186  &$   14.58667 ^{+    0.00021 }_{   -0.00020 }$&$ 0.32  ^{+ 0.13  }_{ -0.32 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 1.96  \pm{ 0.22  }$&$ 89.24 ^{+ 0.76  }_{ -0.35 }$&$ 23.7  ^{+ 2.0   }_{ -1.7  }$&$ 0.121  \pm{ 0.005  }$&$ 832   \pm{ 43    }$&$ 390   \pm{ 19    }$& 4.4   & 0.5  &0.049 & 0.564  \\
K00626.02  & 4478168    & 132.8298  &$    8.02901 ^{+    0.00023 }_{   -0.00022 }$&$ 0.36  ^{+ 0.34  }_{ -0.36 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.13  ^{+ 0.38  }_{ -0.13 }$&$ 2.85  ^{+ 1.81  }_{ -2.67 }$&$ 0.82  \pm{ 0.17  }$&$ 88.73 ^{+ 1.27  }_{ -1.22 }$&$ 16.0  ^{+ 1.3   }_{ -1.3  }$&$ 0.081  \pm{ 0.004  }$&$ 1016  \pm{ 57    }$&$ 68    \pm{ 13    }$& 3.4   & 0.4  &0.002 & 0.054  \\
K00627.01  & 4563268    & 176.1730  &$    7.75191 ^{+    0.00007 }_{   -0.00008 }$&$ 0.34  ^{+ 0.14  }_{ -0.34 }$&$ 0.017  ^{+ 0.001  }_{ -0.001 }$&$ 0.02  ^{+ 0.30  }_{ -0.02 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 2.23  \pm{ 0.22  }$&$ 88.69 ^{+ 1.31  }_{ -0.68 }$&$ 14.5  ^{+ 1.1   }_{ -1.0  }$&$ 0.081  \pm{ 0.003  }$&$ 1061  \pm{ 53    }$&$ 413   \pm{ 11    }$& 3.9   &\textbf{ 3.3  }&0.166 & 0.833  \\
K00627.02  & 4563268    & 132.0230  &$    4.16547 ^{+    0.00006 }_{   -0.00009 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.22  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -1.54 }$&$ 9.5   ^{+ 0.8   }_{ -0.7  }$&$ 0.054  \pm{ 0.002  }$&$ 1318  \pm{ 72    }$&$ 123   \pm{ 8     }$& 3.4   & 2.5  &0.004 & 0.101  \\
K00655.01  & 5966154    & 192.0969  &$   25.67210 ^{+    0.00018 }_{   -0.00020 }$&$ 0.47  ^{+ 0.17  }_{ -0.25 }$&$ 0.018  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 3.39  ^{+  2.12 }_{ -3.39 }$&$ 2.46  \pm{ 0.26  }$&$ 89.09 ^{+ 0.50  }_{ -0.42 }$&$ 30.1  ^{+ 2.6   }_{ -2.4  }$&$ 0.176  \pm{ 0.007  }$&$ 748   \pm{ 39    }$&$ 394   \pm{ 14    }$& 5.9   & 0.9  &0.170 & 0.837  \\
K00655.02  & 5966154    & 176.4103  &$  151.88600 ^{+    0.00240 }_{   -0.00052 }$&$ 0.19  ^{+ 0.26  }_{ -0.19 }$&$ 0.017  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 2.35  \pm{ 0.27  }$&$ 89.89 ^{+ 0.11  }_{ -0.16 }$&$ 99.2  ^{+ 8.6   }_{ -7.1  }$&$ 0.578  \pm{ 0.026  }$&$ 410   \pm{ 22    }$&$ 362   \pm{ 36    }$& 11.7  & 0.7  &0.027 & 0.405  \\
K00664.01  & 6442340    & 170.2279  &$   13.13742 ^{+    0.00024 }_{   -0.00026 }$&$ 0.42  ^{+ 0.27  }_{ -0.42 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.41  ^{+ 0.04  }_{ -0.41 }$&$ 0.27  ^{+ 0.21  }_{ -0.27 }$&$ 2.18  \pm{ 0.53  }$&$ 88.53 ^{+ 1.47  }_{ -1.35 }$&$ 16.1  ^{+ 3.4   }_{ -3.0  }$&$ 0.110  \pm{ 0.003  }$&$ 980   \pm{ 113   }$&$ 233   \pm{ 14    }$& 4.8   & 0.1  &0.080 & 0.813  \\
K00664.02  & 6442340    & 133.5821  &$    7.78220 ^{+    0.00032 }_{   -0.00030 }$&$ 0.00  ^{+ 0.65  }_{ -0.00 }$&$ 0.009  ^{+ 0.005  }_{ -0.001 }$&$ 0.40  ^{+ 0.40  }_{ -0.40 }$&$ 2.60  ^{+ 2.08  }_{ -2.60 }$&$ 1.43  \pm{ 0.59  }$&$ 90.00 ^{+ 0.00  }_{ -4.31 }$&$ 11.2  ^{+ 3.0   }_{ -2.2  }$&$ 0.078  \pm{ 0.003  }$&$ 1187  \pm{ 188   }$&$ 102   \pm{ 10    }$& 4.1   & 0.5  &0.033 & 0.633  \\
K00664.03  & 6442340    & 152.0300  &$   23.44194 ^{+    0.00175 }_{   -0.00154 }$&$ 0.47  ^{+ 0.31  }_{ -0.42 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 1.26  \pm{ 0.41  }$&$ 88.96 ^{+ 0.95  }_{ -0.78 }$&$ 24.0  ^{+ 7.2   }_{ -4.9  }$&$ 0.162  \pm{ 0.005  }$&$ 780   \pm{ 131   }$&$ 82    \pm{ 18    }$& 6.1   & 0.7  &0.021 & 0.521  \\
K00665.01  & 6685609    & 170.3240  &$    5.86805 ^{+    0.00003 }_{   -0.00004 }$&$ 0.52  ^{+ 0.17  }_{ -0.52 }$&$ 0.019  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.00  ^{+ 1.55  }_{ -0.00 }$&$ 3.04  \pm{ 0.63  }$&$ 86.79 ^{+ 3.21  }_{ -1.81 }$&$ 9.7   ^{+ 1.4   }_{ -1.8  }$&$ 0.067  \pm{ 0.003  }$&$ 1321  \pm{ 125   }$&$ 434   \pm{ 8     }$& 4.2   & 0.2  &0.596 & 0.987  \\
K00665.02  & 6685609    & 133.5707  &$    1.61188 ^{+    0.00008 }_{   -0.00007 }$&$ 0.37  ^{+ 0.26  }_{ -0.37 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.12  ^{+ 1.03  }_{ -0.12 }$&$ 1.61  \pm{ 0.31  }$&$ 83.88 ^{+ 6.12  }_{ -6.02 }$&$ 3.6   ^{+ 0.5   }_{ -0.6  }$&$ 0.029  \pm{ 0.001  }$&$ 2153  \pm{ 191   }$&$ 99    \pm{ 4     }$& 3.3   & 0.8  &0.059 & 0.757  \\
K00665.03  & 6685609    & 133.3015  &$    3.07156 ^{+    0.00006 }_{   -0.00008 }$&$ 0.14  ^{+ 0.36  }_{ -0.14 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 1.46  \pm{ 0.37  }$&$ 88.57 ^{+ 1.43  }_{ -4.27 }$&$ 5.8   ^{+ 1.5   }_{ -1.0  }$&$ 0.044  \pm{ 0.002  }$&$ 1712  \pm{ 192   }$&$ 93    \pm{ 6     }$& 4.2   & 0.3  &0.026 & 0.569  \\
K00678.01  & 7509886    & 172.5935  &$    6.04047 ^{+    0.00009 }_{   -0.00012 }$&$ 1.01  ^{+ 0.06  }_{ -0.05 }$&$ 0.017  ^{+ 0.007  }_{ -0.001 }$&$ 0.05  ^{+ 0.07  }_{ -0.05 }$&$ 0.57  ^{+ 0.99  }_{ -0.57 }$&$ 5.16  \pm{ 1.31  }$&$ 77.92 ^{+ 0.94  }_{ -0.71 }$&$ 4.8   ^{+ 0.1   }_{ -0.0  }$&$ 0.063  \pm{ 0.001  }$&$ 1561  \pm{ 46    }$&$ 264   \pm{ 9     }$& 2.5   & 0.9  &0.405 & 0.945  \\
K00678.02  & 7509886    & 132.0163  &$    4.13855 ^{+    0.00005 }_{   -0.00006 }$&$ 0.99  ^{+ 0.02  }_{ -0.03 }$&$ 0.020  ^{+ 0.004  }_{ -0.000 }$&$ 0.05  ^{+ 0.06  }_{ -0.05 }$&$ 0.36  ^{+ 0.23  }_{ -0.36 }$&$ 6.12  \pm{ 0.60  }$&$ 74.66 ^{+ 1.16  }_{ -0.43 }$&$ 3.7   ^{+ 0.0   }_{ -0.0  }$&$ 0.049  \pm{ 0.001  }$&$ 1770  \pm{ 35    }$&$ 254   \pm{ 7     }$& 2.7   & 1.5  &0.463 & 0.956  \\
K00679.01  & 7515212    & 190.2473  &$   31.80526 ^{+    0.00020 }_{   -0.00019 }$&$ 0.89  ^{+ 0.02  }_{ -0.07 }$&$ 0.019  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.11  }_{ -0.01 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 7.44  \pm{ 0.94  }$&$ 86.30 ^{+ 0.83  }_{ -0.27 }$&$ 13.6  ^{+ 2.3   }_{ -0.4  }$&$ 0.227  \pm{ 0.012  }$&$ 1054  \pm{ 62    }$&$ 338   \pm{ 18    }$& 8.7   & 0.7  &0.203 & 0.864  \\
K00679.02  & 7515212    & 139.6350  &$   16.25831 ^{+    0.00113 }_{   -0.00107 }$&$ 0.89  ^{+ 3.29  }_{ -0.19 }$&$ 0.007  ^{+ 0.027  }_{ -0.003 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 1.17  \pm{ 2.45  }$&$ 83.98 ^{+ 0.83  }_{ -0.57 }$&$ 19.6  ^{+ 11.2  }_{ -7.5  }$&$ 0.135  \pm{ 0.008  }$&$ 1345  \pm{ 1355  }$&$ 51    \pm{ 13    }$& 6.8   & 0.2  &0.003 & 0.077  \\
K00710.01  & 9590976    & 170.9513  &$    5.37485 ^{+    0.00015 }_{   -0.00011 }$&$ 0.92  ^{+  0.00 }_{ -0.07 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.14  ^{+ 0.11  }_{ -0.14 }$&$ 0.00  ^{+ 0.56  }_{ -0.00 }$&$ 4.59  \pm{ 0.72  }$&$ 77.99 ^{+ 2.78  }_{ -0.72 }$&$ 4.4   ^{+ 0.7   }_{ -0.2  }$&$ 0.064  \pm{ 0.008  }$&$ 2118  \pm{ 211   }$&$ 155   \pm{ 7     }$& 4.2   & 2.7  &0.288 & 0.953  \\
K00710.02  & 9590976    & 137.9585  &$    8.58604 ^{+    0.00035 }_{   -0.00033 }$&$ 0.96  ^{+ 0.05  }_{ -0.06 }$&$ 0.010  ^{+ 0.004  }_{ -0.000 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 1.33  }_{ -0.00 }$&$ 3.23  \pm{ 0.72  }$&$ 80.86 ^{+ 1.38  }_{ -1.12 }$&$ 6.0   ^{+ 0.5   }_{ -0.2  }$&$ 0.085  \pm{ 0.006  }$&$ 1817  \pm{ 170   }$&$ 99    \pm{ 9     }$& 3.5   & 1.9  &0.050 & 0.725  \\
K00710.03  & 9590976    & 132.4974  &$    3.88683 ^{+    0.00012 }_{   -0.00012 }$&$ 0.81  ^{+ 1.21  }_{ -0.07 }$&$ 0.008  ^{+ 0.005  }_{ -0.002 }$&$ 0.36  ^{+  0.25 }_{ -0.36 }$&$ 3.41  ^{+  2.87 }_{ -3.41 }$&$ 2.38  \pm{ 1.38  }$&$ 79.03 ^{+ 1.07  }_{ -3.49 }$&$ 3.8   ^{+ 2.3   }_{ -0.4  }$&$ 0.052  \pm{ 0.009  }$&$ 2138  \pm{ 803   }$&$ 58    \pm{ 6     }$& 4.7   & 1.1  &0.012 & 0.380  \\
K00717.01  & 9873254    & 175.7916  &$   14.70751 ^{+    0.00033 }_{   -0.00036 }$&$ 0.65  ^{+ 0.22  }_{ -0.62 }$&$ 0.015  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 1.15  }_{ -0.00 }$&$ 2.00  \pm{ 0.85  }$&$ 88.41 ^{+ 1.52  }_{ -1.29 }$&$ 20.9  ^{+ 7.0   }_{ -6.0  }$&$ 0.121  \pm{ 0.008  }$&$ 781   \pm{ 120   }$&$ 273   \pm{ 16    }$& 3.8   & 0.4  &0.162 & 0.828  \\
K00717.02  & 9873254    & 132.2130  &$    0.90039 ^{+    0.00005 }_{   -0.00006 }$&$ 1.32  ^{+  0.18 }_{ -1.24 }$&$ 0.005  ^{+ 0.000  }_{ -0.001 }$&$ 0.79  ^{+ 0.05  }_{ -0.35 }$&$ 1.60  ^{+ 0.71  }_{ -0.87 }$&$ 1.04  \pm{ 0.41  }$&$ 60.64 ^{+ 27.64 }_{ -3.53 }$&$ 2.4   ^{+ 1.2   }_{ -0.6  }$&$ 0.019  \pm{ 0.001  }$&$ 2297  \pm{ 445   }$&$ 31    \pm{ 3     }$& 1.2   & 0.1  &0.016 & 0.287  \\
K00719.01  & 9950612    & 134.8770  &$    9.03420 ^{+    0.00015 }_{   -0.00013 }$&$ 0.78  ^{+ 0.05  }_{ -0.12 }$&$ 0.024  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 1.02  }_{ -0.00 }$&$ 1.74  \pm{ 0.21  }$&$ 88.24 ^{+ 0.42  }_{ -0.30 }$&$ 24.9  ^{+ 1.9   }_{ -1.8  }$&$ 0.077  \pm{ 0.002  }$&$ 618   \pm{ 34    }$&$ 554   \pm{ 8     }$& 1.8   & 0.9  &0.634 & 0.989  \\
K00719.02  & 9950612    & 146.9200  &$   28.12230 ^{+    0.00138 }_{   -0.00494 }$&$ 0.05  ^{+ 0.38  }_{ -0.05 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.86  \pm{ 0.10  }$&$ 89.95 ^{+ 0.05  }_{ -0.45 }$&$ 51.7  ^{+ 4.4   }_{ -4.2  }$&$ 0.163  \pm{ 0.005  }$&$ 432   \pm{ 24    }$&$ 169   \pm{ 14    }$& 4.2   & 0.6  &0.016 & 0.455  \\
K00719.03  & 9950612    & 166.5382  &$   45.90000 ^{+    0.00978 }_{   -0.00370 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 0.013  ^{+ 0.002  }_{ -0.000 }$&$ 0.32  ^{+ 0.20  }_{ -0.32 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.97  \pm{ 0.13  }$&$ 90.00 ^{+ 0.00  }_{ -0.35 }$&$ 72.1  ^{+ 6.5   }_{ -5.9  }$&$ 0.226  \pm{ 0.008  }$&$ 364   \pm{ 20    }$&$ 185   \pm{ 24    }$& 4.6   & 0.2  &0.030 & 0.611  \\
K00719.04  & 9950612    & 133.7840  &$    4.15982 ^{+    0.00003 }_{   -0.00003 }$&$ 0.40  ^{+ 0.17  }_{ -0.40 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.69  \pm{ 0.09  }$&$ 88.49 ^{+ 1.50  }_{ -0.78 }$&$ 14.9  ^{+ 1.2   }_{ -1.0  }$&$ 0.046  \pm{ 0.001  }$&$ 797   \pm{ 42    }$&$ 144   \pm{ 5     }$& 1.9   & 0.2  &0.063 & 0.770  \\
K00972.01  & 11013201   & 261.5394  &$   13.11891 ^{+    0.00002 }_{   -0.00002 }$&$ 0.82  ^{+ 0.13  }_{ -0.13 }$&$ 0.022  ^{+ 0.004  }_{ -0.004 }$&$ 0.16  ^{+ 0.14  }_{ -0.16 }$&$ 4.73  ^{+ 0.11  }_{ -4.73 }$&$ 9.32  \pm{ 2.47  }$&$ 84.95 ^{+ 2.03  }_{ -2.55 }$&$ 7.7   ^{+ 3.1   }_{ -0.8  }$&$ 0.140  \pm{ 0.004  }$&$ 1742  \pm{ 289   }$&$ 375   \pm{ 26    }$& 5.0   &\textbf{ 4.6  }&0.646 & 0.979  \\
K00972.02  & 11013201   & 139.1430  &$    7.82257 ^{+    0.00044 }_{   -0.00018 }$&$ 0.74  ^{+ 0.27  }_{ -0.25 }$&$ 0.004  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.04  ^{+ 0.37  }_{ -0.04 }$&$ 1.51  \pm{ 0.64  }$&$ 84.12 ^{+ 1.97  }_{ -1.69 }$&$ 6.4   ^{+ 1.8   }_{ -1.5  }$&$ 0.099  \pm{ 0.003  }$&$ 1972  \pm{ 329   }$&$ 16    \pm{ 20    }$& 5.6   & 0.2  &0.037 & 0.487  \\
K01001.01  & 1871056    & 155.7178  &$   40.80686 ^{+    0.00012 }_{   -0.00043 }$&$ 0.00  ^{+ 0.76  }_{ -0.24 }$&$ 0.016  ^{+ 0.002  }_{ -0.001 }$&$ 0.69  ^{+  0.12 }_{ -0.69 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 6.00  \pm{ 0.82  }$&$ 90.00 ^{+  0.00 }_{ -2.68 }$&$ 16.2  ^{+ 2.7   }_{ -0.4  }$&$ 0.260  \pm{ 0.010  }$&$ 1013  \pm{ 73    }$&$ 328   \pm{ 27    }$& 13.7  & 1.2  &0.003 & 0.071  \\
K01001.02  & 1871056    & 216.2450  &$  140.09140 ^{+    0.00229 }_{   -0.00164 }$&$ 0.65  ^{+ 0.22  }_{ -0.57 }$&$ 0.016  ^{+ 0.003  }_{ -0.000 }$&$ 0.00  ^{+ 0.69  }_{ -0.00 }$&$ 0.00  ^{+ 4.24  }_{ -0.00 }$&$ 5.82  \pm{ 1.03  }$&$ 89.14 ^{+ 0.76  }_{ -0.47 }$&$ 37.6  ^{+ 11.4  }_{ -1.4  }$&$ 0.585  \pm{ 0.022  }$&$ 627   \pm{ 71    }$&$ 300   \pm{ 52    }$& 19.3  & 0.3  &0.013 & 0.242  \\
K01151.01  & 8280511    & 134.8157  &$    5.21781 ^{+    0.00021 }_{   -0.00019 }$&$ 0.89  ^{+ 0.06  }_{ -0.02 }$&$ 0.011  ^{+ 0.000  }_{ -0.001 }$&$ 0.05  ^{+ 0.15  }_{ -0.05 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 2.73  \pm{ 0.34  }$&$ 80.79 ^{+ 0.69  }_{ -1.23 }$&$ 5.7   ^{+ 0.7   }_{ -0.4  }$&$ 0.060  \pm{ 0.004  }$&$ 1615  \pm{ 84    }$&$ 99    \pm{ 9     }$& 3.6   & 1.0  &0.018 & 0.472  \\
K01151.02  & 8280511    & 135.7436  &$    7.41105 ^{+    0.00027 }_{   -0.00026 }$&$ 0.89  ^{+ 0.04  }_{ -0.04 }$&$ 0.013  ^{+ 0.001  }_{ -0.001 }$&$ 0.10  ^{+ 0.05  }_{ -0.10 }$&$ 0.00  ^{+ 1.24  }_{ -0.00 }$&$ 3.13  \pm{ 0.47  }$&$ 83.01 ^{+ 0.96  }_{ -1.55 }$&$ 7.5   ^{+ 0.6   }_{ -0.7  }$&$ 0.076  \pm{ 0.006  }$&$ 1417  \pm{ 118   }$&$ 124   \pm{ 10    }$& 3.9   & 0.6  &0.066 & 0.779  \\
K01151.03  & 8280511    & 135.4660  &$    5.24972 ^{+    0.00010 }_{   -0.00012 }$&$ 0.60  ^{+ 0.33  }_{ -0.45 }$&$ 0.007  ^{+ 0.003  }_{ -0.001 }$&$ 0.06  ^{+ 0.52  }_{ -0.06 }$&$ 3.16  ^{+ 1.34  }_{ -3.16 }$&$ 0.86  \pm{ 0.38  }$&$ 86.95 ^{+ 2.39  }_{ -3.14 }$&$ 11.3  ^{+ 2.7   }_{ -2.8  }$&$ 0.057  \pm{ 0.003  }$&$ 1138  \pm{ 185   }$&$ 65    \pm{ 9     }$& 2.9   & 1.0  &0.009 & 0.317  \\
K01151.04  & 8280511    & 146.6500  &$   17.45337 ^{+    0.00142 }_{   -0.00112 }$&$ 0.80  ^{+ 2.14  }_{ -0.30 }$&$ 0.009  ^{+ 0.029  }_{ -0.002 }$&$ 0.01  ^{+ 0.04  }_{ -0.01 }$&$ 0.00  ^{+ 0.34  }_{ -0.01 }$&$ 1.03  \pm{ 1.73  }$&$ 86.70 ^{+  0.21 }_{ -1.51 }$&$ 26.6  ^{+ 7.5   }_{ -7.2  }$&$ 0.125  \pm{ 0.008  }$&$ 1028  \pm{ 529   }$&$ 79    \pm{ 17    }$& 6.0   & 0.1  &0.007 & 0.254  \\
K01151.05  & 8280511    & 134.7589  &$   21.72069 ^{+    0.00024 }_{   -0.00029 }$&$ 0.38  ^{+ 0.37  }_{ -0.38 }$&$ 0.007  ^{+ 0.004  }_{ -0.000 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.75  \pm{ 0.30  }$&$ 89.35 ^{+ 0.64  }_{ -0.85 }$&$ 31.2  ^{+ 7.7   }_{ -6.9  }$&$ 0.145  \pm{ 0.008  }$&$ 659   \pm{ 101   }$&$ 85    \pm{ 19    }$& 4.6   & 2.0  &0.008 & 0.295  \\
K01175.01  & 10350571   & 142.9750  &$   31.59300 ^{+    0.00090 }_{   -0.00005 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 2.09  \pm{ 0.25  }$&$ 90.00 ^{+ 0.00  }_{ -0.84 }$&$ 25.8  ^{+ 2.1   }_{ -2.5  }$&$ 0.195  \pm{ 0.006  }$&$ 731   \pm{ 45    }$&$ 150   \pm{ 26    }$& 9.4   & 0.6  &0.016 & 0.283  \\
K01175.02  & 10350571   & 133.6877  &$   17.15710 ^{+    0.00124 }_{   -0.00170 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 1.84  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -0.92 }$&$ 17.0  ^{+ 1.6   }_{ -1.3  }$&$ 0.130  \pm{ 0.004  }$&$ 897   \pm{ 54    }$&$ 114   \pm{ 20    }$& 7.7   & 0.4  &0.015 & 0.281  \\
K01215.01  & 3939150    & 142.0971  &$   17.32440 ^{+    0.00018 }_{   -0.00019 }$&$ 0.75  ^{+ 0.13  }_{ -0.42 }$&$ 0.014  ^{+ 0.002  }_{ -0.000 }$&$ 0.27  ^{+ 0.08  }_{ -0.27 }$&$ 0.53  ^{+ 2.43  }_{ -0.53 }$&$ 4.87  \pm{ 0.69  }$&$ 85.85 ^{+ 2.86  }_{ -1.18 }$&$ 9.4   ^{+ 1.7   }_{ -0.1  }$&$ 0.137  \pm{ 0.003  }$&$ 1229  \pm{ 156   }$&$ 244   \pm{ 17    }$& 8.9   & 1.2  &0.062 & 0.621  \\
K01215.02  & 3939150    & 145.3899  &$   33.00590 ^{+    0.00061 }_{   -0.00059 }$&$ 0.95  ^{+ 0.14  }_{ -0.07 }$&$ 0.018  ^{+ 0.002  }_{ -0.001 }$&$ 0.05  ^{+ 0.06  }_{ -0.05 }$&$ 1.53  ^{+ 4.04  }_{ -1.50 }$&$ 6.36  \pm{ 0.49  }$&$ 86.25 ^{+ 0.43  }_{ -0.45 }$&$ 14.4  ^{+ 0.1   }_{ -0.2  }$&$ 0.213  \pm{ 0.004  }$&$ 1037  \pm{ 50    }$&$ 285   \pm{ 24    }$& 7.9   & 1.3  &0.054 & 0.588  \\
K01221.01  & 3640905    & 138.5145  &$   30.16012 ^{+    0.00005 }_{   -0.00007 }$&$ 0.65  ^{+ 0.14  }_{ -0.15 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.62  ^{+  0.05 }_{ -0.62 }$&$ 4.28  ^{+ 1.73  }_{ -4.28 }$&$ 2.89  \pm{ 0.41  }$&$ 88.32 ^{+ 0.47  }_{ -0.51 }$&$ 22.0  ^{+ 1.7   }_{ -1.7  }$&$ 0.192  \pm{ 0.005  }$&$ 723   \pm{ 41    }$&$ 171   \pm{ 18    }$& 8.0   & 0.9  &0.117 & 0.768  \\
K01221.02  & 3640905    & 152.3420  &$   51.08020 ^{+    0.00165 }_{   -0.41281 }$&$ 0.13  ^{+ 0.75  }_{ -0.13 }$&$ 0.010  ^{+ 0.002  }_{ -0.001 }$&$ 0.45  ^{+ 0.26  }_{ -0.45 }$&$ 6.29  ^{+  0.00 }_{ -6.29 }$&$ 2.08  \pm{ 0.36  }$&$ 89.77 ^{+ 0.23  }_{ -1.42 }$&$ 32.0  ^{+ 2.9   }_{ -2.6  }$&$ 0.272  \pm{ 0.008  }$&$ 600   \pm{ 38    }$&$ 140   \pm{ 24    }$& 10.8  & 1.0  &0.029 & 0.429  \\
K01241.01  & 6448890    & 147.0928  &$   21.40505 ^{+    0.00009 }_{   -0.00008 }$&$ 0.95  ^{+ 0.02  }_{ -0.02 }$&$ 0.022  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 15.67  \pm{ 3.93  }$&$ 79.59 ^{+  2.12 }_{ -3.42 }$&$ 5.5   ^{+ 0.9   }_{ -1.3  }$&$ 0.164  \pm{ 0.005  }$&$ 1425  \pm{ 159   }$&$ 413   \pm{ 27    }$& 11.6   & 0.7  &0.092 & 0.716  \\
K01241.02  & 6448890    & 135.5589  &$   10.50343 ^{+    0.00028 }_{   -0.00026 }$&$ 0.80  ^{+ 1.69  }_{ -0.42 }$&$ 0.013  ^{+ 0.031  }_{ -0.004 }$&$ 0.00  ^{+ 0.06  }_{ -0.02 }$&$ 0.01  ^{+ 0.29  }_{ -0.03 }$&$ 4.92  \pm{ 6.46  }$&$ 82.94 ^{+  3.17 }_{ -4.73 }$&$ 6.5   ^{+ 0.1   }_{ -0.1  }$&$ 0.103  \pm{ 0.002  }$&$ 1279  \pm{ 317   }$&$ 160   \pm{ 19    }$& 7.7   & 0.7  &0.092 & 0.716  \\
K01316.01  & 10794087   & 138.3401  &$    7.64951 ^{+    0.00028 }_{   -0.00023 }$&$ 0.38  ^{+ 0.28  }_{ -0.32 }$&$ 0.006  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.75  \pm{ 0.50  }$&$ 87.00 ^{+ 2.56  }_{ -2.76 }$&$ 6.5   ^{+ 2.2   }_{ -1.1  }$&$ 0.080  \pm{ 0.002  }$&$ 1407  \pm{ 201   }$&$ 56    \pm{ 6     }$& 7.5   & 1.5  &0.086 & 0.701  \\
K01316.02  & 10794087   & 143.3790  &$   12.37679 ^{+    0.00079 }_{   -0.00044 }$&$ 0.91  ^{+  0.09}_{ -0.91 }$&$ 0.007  ^{+ 0.012  }_{ -0.006 }$&$ 0.01  ^{+ 0.03  }_{ -0.01 }$&$ 0.19  ^{+ 0.06  }_{ -0.19 }$&$ 1.85  \pm{ 1.78  }$&$ 84.30 ^{+ 0.86  }_{ -0.58 }$&$ 9.1   ^{+ 6.4   }_{ -1.7  }$&$ 0.110  \pm{ 0.003  }$&$ 515   \pm{ 39    }$&$ 43     \pm{ 7     }$& 3.9   & 0.3  &0.038 & 0.495  \\
K01445.01  & 11336883   & 135.6794  &$    7.16888 ^{+    0.00017 }_{   -0.00016 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 1.36  \pm{ 0.14  }$&$ 90.00 ^{+ 0.00  }_{ -0.92 }$&$ 12.9  ^{+ 1.1   }_{ -0.9  }$&$ 0.078  \pm{ 0.003  }$&$ 1150  \pm{ 61    }$&$ 115   \pm{ 7     }$& 4.3   & 0.9  &0.097 & 0.842  \\
K01445.02  & 11336883   & 142.1590  &$   54.34430 ^{+    0.02029 }_{   -0.00009 }$&$ 0.42  ^{+ 3.22  }_{ -0.42 }$&$ 0.006  ^{+ 0.009  }_{ -0.002 }$&$ 0.09  ^{+ 0.11  }_{ -0.09 }$&$ 0.10  ^{+ 0.13  }_{ -0.10 }$&$ 0.84  \pm{ 0.77  }$&$ 89.54 ^{+ 0.46  }_{ -3.24 }$&$ 52.2  ^{+ 4.1   }_{ -4.0  }$&$ 0.300  \pm{ 0.011  }$&$ 562   \pm{ 31    }$&$ 40    \pm{ 21    }$& 7.1   & 1.1  &0.005 & 0.215  \\
K01445.03  & 11336883   & 150.8360  &$   20.01960 ^{+    0.00098 }_{   -0.00103 }$&$ 0.31  ^{+ 0.55  }_{ -0.31 }$&$ 0.004  ^{+ 0.003  }_{ -0.001 }$&$ 0.40  ^{+ 0.30  }_{ -0.35 }$&$ 3.93  ^{+ 1.29  }_{ -1.30 }$&$ 0.60  \pm{ 0.28  }$&$ 89.33 ^{+ 0.67  }_{ -1.16 }$&$ 26.6  ^{+ 2.5   }_{ -2.1  }$&$ 0.154  \pm{ 0.006  }$&$ 789   \pm{ 49    }$&$ 20    \pm{ 14    }$& 6.8   & 0.3  &0.006 & 0.225  \\
K01525.01  & 7869917    & 133.5535  &$    7.71468 ^{+    0.00011 }_{   -0.00011 }$&$ 0.59  ^{+ 0.22  }_{ -0.59 }$&$ 0.016  ^{+ 0.001  }_{ -0.003 }$&$ 0.63  ^{+ 0.17  }_{ -0.43 }$&$ 4.53  ^{+ 0.06  }_{ -1.24 }$&$ 3.26  \pm{ 1.07  }$&$ 86.62 ^{+ 3.38  }_{ -4.28 }$&$ 10.3  ^{+ 3.1   }_{ -2.5  }$&$ 0.091  \pm{ 0.005  }$&$ 1447  \pm{ 322   }$&$ 217   \pm{ 10    }$& 4.7   & 0.2  &0.476 & 0.958  \\
K01525.02  & 7869917    & 138.2671  &$   11.80609 ^{+    0.00036 }_{   -0.00046 }$&$ 0.37  ^{+ 0.30  }_{ -0.37 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 1.46  \pm{ 0.43  }$&$ 88.67 ^{+ 1.33  }_{ -1.36 }$&$ 15.1  ^{+ 4.1   }_{ -2.9  }$&$ 0.106  \pm{ 0.009  }$&$ 1156  \pm{ 163   }$&$ 120   \pm{ 13    }$& 5.4   & 0.8  &0.095 & 0.723  \\
K01534.01  & 4741126    & 146.9846  &$   20.42226 ^{+    0.00047 }_{   -0.00049 }$&$ 0.05  ^{+ 0.48  }_{ -0.05 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 1.83  \pm{ 0.45  }$&$ 89.88 ^{+ 0.12  }_{ -1.26 }$&$ 24.2  ^{+ 5.8   }_{ -4.1  }$&$ 0.160  \pm{ 0.007  }$&$ 862   \pm{ 110   }$&$ 187   \pm{ 16    }$& 6.5   & 1.0  &0.038 & 0.499  \\
K01534.02  & 4741126    & 138.2340  &$    7.63861 ^{+    0.00030 }_{   -0.00030 }$&$ 0.41  ^{+ 0.35  }_{ -0.41 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.00  ^{+ 0.33  }_{ -0.00 }$&$ 1.12  \pm{ 0.34  }$&$ 88.24 ^{+ 1.76  }_{ -1.64 }$&$ 13.2  ^{+ 3.1   }_{ -2.9  }$&$ 0.083  \pm{ 0.004  }$&$ 1160  \pm{ 171   }$&$ 80    \pm{ 10    }$& 4.0   & 0.8  &0.005 & 0.119  \\
K01613.01  & 6268648    & 141.0860  &$   15.86621 ^{+    0.00058 }_{   -0.00057 }$&$ 0.34  ^{+ 0.65  }_{ -0.34 }$&$ 0.008  ^{+ 0.003  }_{ -0.001 }$&$ 0.52  ^{+ 0.32  }_{ -0.14 }$&$ 2.66  ^{+ 1.57  }_{ -1.57 }$&$ 1.32  \pm{ 0.82  }$&$ 88.98 ^{+ 1.02  }_{ -3.05 }$&$ 17.8  ^{+ 8.8   }_{ -6.9  }$&$ 0.127  \pm{ 0.010  }$&$ 900   \pm{ 237   }$&$ 77    \pm{ 6     }$& 4.3   & 0.8  &0.021 & 0.346  \\
K01613.02  & 6268648    & 196.7260  &$   94.09329 ^{+    0.00438 }_{   -0.00051 }$&$ 0.48  ^{+ 0.51  }_{ -0.48 }$&$ 0.008  ^{+ 0.002  }_{ -0.002 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 1.31  \pm{ 0.71  }$&$ 89.57 ^{+ 0.43  }_{ -0.68 }$&$ 59.2  ^{+ 32.3  }_{ -19.3 }$&$ 0.416  \pm{ 0.031  }$&$ 496   \pm{ 159   }$&$ 65    \pm{ 17    }$& 10.0  & 1.2  &0.003 & 0.061  \\
K01628.01  & 6975129    & 147.1029  &$   19.74747 ^{+    0.00031 }_{   -0.00040 }$&$ 0.71  ^{+ 0.12  }_{ -0.30 }$&$ 0.020  ^{+ 0.003  }_{ -0.002 }$&$ 0.08  ^{+ 0.41  }_{ -0.08 }$&$ 0.00  ^{+ 4.60  }_{ -0.00 }$&$ 2.62  \pm{ 0.39  }$&$ 88.53 ^{+ 0.71  }_{ -0.41 }$&$ 27.1  ^{+ 2.5   }_{ -1.8  }$&$ 0.153  \pm{ 0.005  }$&$ 784   \pm{ 46    }$&$ 466   \pm{ 17    }$& 4.0   & 1.2  &0.149 & 0.813  \\
K01628.02  & 6975129    & 132.0945  &$    1.77243 ^{+    0.00003 }_{   -0.00003 }$&$ 0.00  ^{+ 0.21  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 0.94  \pm{ 0.12  }$&$ 90.00 ^{+  0.00 }_{ -2.07 }$&$ 5.5   ^{+ 0.5   }_{ -0.4  }$&$ 0.029  \pm{ 0.001  }$&$ 1744  \pm{ 91    }$&$ 74    \pm{ 4     }$& 2.5   & 1.8  &0.027 & 0.408  \\
K01692.01  & 6616218    & 137.2639  &$    5.96040 ^{+    0.00003 }_{   -0.00002 }$&$ 0.35  ^{+ 0.09  }_{ -0.35 }$&$ 0.024  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 2.46  \pm{ 0.21  }$&$ 88.64 ^{+ 1.36  }_{ -0.46 }$&$ 14.4  ^{+ 1.1   }_{ -1.0  }$&$ 0.064  \pm{ 0.002  }$&$ 957   \pm{ 40    }$&$ 829   \pm{ 9     }$& 3.0   & 0.9  &0.865 & 0.994  \\
K01692.02  & 6616218    & 133.3133  &$    2.46110 ^{+    0.00003 }_{   -0.00003 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.80  \pm{ 0.10  }$&$ 90.00 ^{+ 0.00  }_{ -2.57 }$&$ 8.0   ^{+ 0.7   }_{ -0.7  }$&$ 0.035  \pm{ 0.001  }$&$ 1288  \pm{ 73    }$&$ 82    \pm{ 6     }$& 2.4   & 0.7  &0.021 & 0.346  \\
K01779.01  & 9909735    & 134.0812  &$    4.66272 ^{+    0.00001 }_{   -0.00001 }$&$ 0.84  ^{+ 0.06  }_{ -0.19 }$&$ 0.041  ^{+ 0.004  }_{ -0.001 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.00  ^{+ 4.76  }_{ -0.00 }$&$ 7.84  \pm{ 1.47  }$&$ 83.09 ^{+ 2.83  }_{ -1.84 }$&$ 6.7   ^{+ 1.6   }_{ -0.8  }$&$ 0.054  \pm{ 0.002  }$&$ 1458  \pm{ 171   }$&$ 1627  \pm{ 10    }$& 3.1   & 0.8  &0.635 & 0.978  \\
K01779.02  & 9909735    & 133.0899  &$   11.81502 ^{+    0.00009 }_{   -0.00004 }$&$ 0.93  ^{+ 0.24  }_{ -0.09 }$&$ 0.037  ^{+ 0.000  }_{ -0.005 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 4.48  ^{+  0.90 }_{ -4.48 }$&$ 6.54  \pm{ 1.68  }$&$ 86.18 ^{+ 1.16  }_{ -2.96 }$&$ 13.5  ^{+ 3.1   }_{ -3.1  }$&$ 0.101  \pm{ 0.003  }$&$ 1034  \pm{ 155   }$&$ 1028  \pm{ 18    }$& 3.0   & 1.4  &0.169 & 0.835  \\
\textbf{K01781.01  }& 11551692   & 135.2206  &$    7.83445 ^{+    0.00001 }_{   -0.00001 }$&$ 0.33  ^{+ 0.31  }_{ -0.15 }$&$ 0.037  ^{+ 0.011  }_{ -0.000 }$&$ 0.00  ^{+ 0.66  }_{ -0.00 }$&$ 0.00  ^{+ 4.72  }_{ -0.00 }$&$ 3.24  \pm{ 0.56  }$&$ 89.03 ^{+ 0.49  }_{ -1.08 }$&$ 19.4  ^{+ 1.4   }_{ -1.3  }$&$ 0.073  \pm{ 0.002  }$&$ 753   \pm{ 34    }$&$ 1954  \pm{ 11    }$& 3.1   &\textbf{ 3.5  }&0.995 &\textbf{ 1.000 } \\
\textbf{K01781.02  }& 11551692   & 137.1027  &$    3.00516 ^{+    0.00001 }_{   -0.00001 }$&$ 0.31  ^{+ 0.27  }_{ -0.30 }$&$ 0.022  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.35  }_{ -0.00 }$&$ 0.00  ^{+ 4.31  }_{ -0.00 }$&$ 1.88  \pm{ 0.20  }$&$ 88.27 ^{+ 1.73  }_{ -1.83 }$&$ 10.2  ^{+ 0.6   }_{ -0.8  }$&$ 0.038  \pm{ 0.001  }$&$ 1040  \pm{ 46    }$&$ 690   \pm{ 5     }$& 2.2   & 0.9  &0.979 &\textbf{ 1.000 } \\
K01781.03  & 11551692   & 151.8476  &$   58.02125 ^{+    0.00020 }_{   -0.00013 }$&$ 0.50  ^{+ 0.16  }_{ -0.47 }$&$ 0.031  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 2.61  \pm{ 0.31  }$&$ 89.63 ^{+ 0.35  }_{ -0.16 }$&$ 76.0  ^{+ 6.7   }_{ -6.4  }$&$ 0.276  \pm{ 0.007  }$&$ 377   \pm{ 20    }$&$ 1338  \pm{ 46    }$& 5.1   & 1.2  &0.598 & 0.987  \\
%           &            & 0.0000    &$   58.02125 ^{+    0.00044 }_{   -0.00018 }$&$ 0.50  ^{+ 0.16  }_{ -0.47 }$&$ 0.031  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 2.61  \pm{ 0.31  }$&$ 89.63 ^{+ 0.35  }_{ -0.16 }$&$ 76.0  ^{+ 6.7   }_{ -6.4  }$&$ 0.276  \pm{ 0.007  }$&$ 377   \pm{ 20    }$&$ 1338  \pm{ 46    }$& 5.1   & 1.2  &\nodata & \nodata  \\
K01806.02  & 9529744    & 138.2171  &$   17.93497 ^{+    0.00050 }_{   -0.00080 }$&$ 0.31  ^{+ 0.19  }_{ -0.31 }$&$ 0.012  ^{+ 0.000  }_{ -0.003 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.60  \pm{ 0.40  }$&$ 89.30 ^{+ 0.70  }_{ -0.57 }$&$ 24.4  ^{+ 5.5   }_{ -4.8  }$&$ 0.137  \pm{ 0.008  }$&$ 849   \pm{ 109   }$&$ 176   \pm{ 18    }$& 5.2   &\textbf{ 3.1  }&0.024 & 0.556  \\
K01806.03  & 9529744    & 137.6755  &$    8.37167 ^{+    0.00000 }_{    0.00000 }$&$ 0.27  ^{+ 0.33  }_{ -0.27 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.54  }_{ -0.00 }$&$ 1.09  \pm{ 0.32  }$&$ 88.99 ^{+ 1.01  }_{ -1.33 }$&$ 14.7  ^{+ 3.8   }_{ -2.9  }$&$ 0.083  \pm{ 0.005  }$&$ 1087  \pm{ 152   }$&$ 89    \pm{ 13    }$& 4.0   &\textbf{ 4.1  }&0.007 & 0.257  \\
K01809.01  & 8240797    & 144.5235  &$   13.09392 ^{+    0.00016 }_{   -0.00017 }$&$ 0.96  ^{+ 0.45  }_{ -0.02 }$&$ 0.023  ^{+ 0.014  }_{ -0.003 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.00  ^{+ 1.58  }_{ -0.00 }$&$ 6.15  \pm{ 3.24  }$&$ 86.14 ^{+ 0.00  }_{ -6.28 }$&$ 10.0  ^{+ 3.9   }_{ -2.2  }$&$ 0.115  \pm{ 0.014  }$&$ 1009  \pm{ 145   }$&$ 390   \pm{ 9     }$& 2.5   & 1.4  &0.459 & 0.955  \\
K01809.02  & 8240797    & 132.6958  &$    4.91538 ^{+    0.00000 }_{   -0.00000 }$&$ 0.72  ^{+ 0.15  }_{ -0.35 }$&$ 0.015  ^{+ 0.003  }_{ -0.002 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.00  ^{+ 0.94  }_{ -0.00 }$&$ 2.42  \pm{ 0.85  }$&$ 85.24 ^{+ 2.85  }_{ -3.09 }$&$ 8.5   ^{+ 2.4   }_{ -2.2  }$&$ 0.058  \pm{ 0.003  }$&$ 1293  \pm{ 218   }$&$ 235   \pm{ 6     }$& 3.1   & 1.1  &0.259 & 0.897  \\
K01824.01  & 2989404    & 134.6430  &$    3.55380 ^{+    0.00004 }_{   -0.00004 }$&$ 0.50  ^{+ 0.18  }_{ -0.41 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.33  }_{ -0.00 }$&$ 0.15  ^{+ 4.37  }_{ -0.15 }$&$ 2.07  \pm{ 0.44  }$&$ 85.76 ^{+ 3.56  }_{ -2.65 }$&$ 6.6   ^{+ 1.3   }_{ -1.0  }$&$ 0.049  \pm{ 0.002  }$&$ 1591  \pm{ 150   }$&$ 197   \pm{ 5     }$& 3.5   & 0.5  &0.190 & 0.854  \\
K01824.02  & 2989404    & 136.0502  &$    1.67834 ^{+    0.00002 }_{   -0.00002 }$&$ 0.63  ^{+ 0.21  }_{ -0.44 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.03  ^{+ 0.53  }_{ -0.03 }$&$ 0.08  ^{+ 2.53  }_{ -0.08 }$&$ 2.12  \pm{ 0.49  }$&$ 79.91 ^{+ 7.73  }_{ -7.45 }$&$ 3.6   ^{+ 0.7   }_{ -0.6  }$&$ 0.030  \pm{ 0.001  }$&$ 2196  \pm{ 244   }$&$ 152   \pm{ 3     }$& 2.9   & 0.3  &0.178 & 0.844  \\
K01909.01  & 10130039   & 133.9557  &$   12.75808 ^{+    0.00023 }_{   -0.00022 }$&$ 0.28  ^{+ 0.17  }_{ -0.28 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.44  ^{+ 0.04  }_{ -0.44 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.65  \pm{ 0.35  }$&$ 89.22 ^{+ 0.78  }_{ -0.59 }$&$ 20.3  ^{+ 3.6   }_{ -3.3  }$&$ 0.113  \pm{ 0.004  }$&$ 888   \pm{ 84    }$&$ 191   \pm{ 9     }$& 4.2   & 0.4  &0.194 & 0.923  \\
K01909.02  & 10130039   & 131.4909  &$    5.47037 ^{+    0.00011 }_{   -0.00008 }$&$ 0.22  ^{+ 0.41  }_{ -0.22 }$&$ 0.008  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 1.11  \pm{ 0.25  }$&$ 88.89 ^{+ 1.11  }_{ -2.56 }$&$ 11.1  ^{+ 2.1   }_{ -1.8  }$&$ 0.064  \pm{ 0.003  }$&$ 1201  \pm{ 120   }$&$ 110   \pm{ 6     }$& 3.6   & 0.2  &0.053 & 0.736  \\
K01909.03  & 10130039   & 145.5671  &$   25.09858 ^{+    0.00089 }_{   -0.00084 }$&$ 0.89  ^{+ 0.04  }_{ -0.26 }$&$ 0.015  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 0.00  ^{+ 1.40  }_{ -0.00 }$&$ 1.97  \pm{ 0.58  }$&$ 88.36 ^{+ 0.73  }_{ -0.55 }$&$ 30.7  ^{+ 7.3   }_{ -6.6  }$&$ 0.178  \pm{ 0.008  }$&$ 725   \pm{ 94    }$&$ 187   \pm{ 13    }$& 3.0   & 0.2  &0.097 & 0.843  \\
K01929.01  & 10136549   & 132.8155  &$    9.69303 ^{+    0.00016 }_{   -0.00019 }$&$ 0.70  ^{+ 0.16  }_{ -0.59 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.16  ^{+ 0.82  }_{ -0.16 }$&$ 2.47  \pm{ 0.69  }$&$ 85.55 ^{+ 3.90  }_{ -2.57 }$&$ 9.8   ^{+ 2.5   }_{ -2.4  }$&$ 0.089  \pm{ 0.002  }$&$ 1304  \pm{ 182   }$&$ 145   \pm{ 9     }$& 6.0   & 0.7  &0.127 & 0.784  \\
K01929.02  & 10136549   & 133.0093  &$    3.29274 ^{+    0.00008 }_{   -0.00008 }$&$ 0.68  ^{+ 0.15  }_{ -0.16 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.04  ^{+ 0.37  }_{ -0.04 }$&$ 0.45  ^{+ 0.31  }_{ -0.45 }$&$ 2.20  \pm{ 0.35  }$&$ 79.37 ^{+ 3.24  }_{ -3.45 }$&$ 4.0   ^{+ 0.5   }_{ -0.6  }$&$ 0.044  \pm{ 0.001  }$&$ 2037  \pm{ 166   }$&$ 83    \pm{ 5     }$& 5.1   & 0.3  &0.124 & 0.779  \\
K01930.01  & 5511081    & 138.7478  &$   13.72686 ^{+    0.00010 }_{   -0.00011 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 2.25  \pm{ 0.21  }$&$ 90.00 ^{+ 0.00  }_{ -1.47 }$&$ 15.5  ^{+ 1.2   }_{ -1.2  }$&$ 0.115  \pm{ 0.003  }$&$ 1006  \pm{ 50    }$&$ 200   \pm{ 12    }$& 7.0   & 1.5  &0.134 & 0.886  \\
K01930.02  & 5511081    & 137.0438  &$   24.31058 ^{+    0.00024 }_{   -0.00028 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 2.19  \pm{ 0.22  }$&$ 90.00 ^{+ 0.00  }_{ -1.12 }$&$ 22.9  ^{+ 1.9   }_{ -1.8  }$&$ 0.168  \pm{ 0.004  }$&$ 821   \pm{ 43    }$&$ 180   \pm{ 15    }$& 8.3   & 1.8  &0.061 & 0.765  \\
K01930.03  & 5511081    & 143.5344  &$   44.43150 ^{+    0.00028 }_{   -0.00020 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.17  ^{+ 0.33  }_{ -0.17 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 2.57  \pm{ 0.26  }$&$ 90.00 ^{+ 0.00  }_{ -0.44 }$&$ 34.7  ^{+ 3.2   }_{ -2.4  }$&$ 0.252  \pm{ 0.006  }$&$ 663   \pm{ 35    }$&$ 248   \pm{ 21    }$& 9.7   & 1.6  &0.053 & 0.739  \\
K01930.04  & 5511081    & 132.3931  &$    9.34131 ^{+    0.00038 }_{   -0.00032 }$&$ 0.17  ^{+ 0.30  }_{ -0.17 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.50  ^{+ 0.15  }_{ -0.47 }$&$ 3.56  ^{+ 1.11  }_{ -3.00 }$&$ 1.32  \pm{ 0.18  }$&$ 89.21 ^{+ 0.79  }_{ -1.42 }$&$ 12.5  ^{+ 1.1   }_{ -1.0  }$&$ 0.089  \pm{ 0.002  }$&$ 1105  \pm{ 70    }$&$ 79    \pm{ 9     }$& 6.1   & 1.6  &0.025 & 0.560  \\
K01932.01  & 5202905    & 144.4640  &$   22.82485 ^{+    0.00007 }_{   -0.00004 }$&$ 0.71  ^{+ 0.13  }_{ -0.34 }$&$ 0.017  ^{+ 0.003  }_{ -0.004 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.44  ^{+ 3.13  }_{ -0.44 }$&$ 6.05  \pm{ 1.96  }$&$ 87.21 ^{+ 1.63  }_{ -1.36 }$&$ 13.4  ^{+ 4.0   }_{ -3.1  }$&$ 0.203  \pm{ 0.007  }$&$ 1429  \pm{ 236   }$&$ 317   \pm{ 69    }$& 8.7   & 0.6  &0.015 & 0.281  \\
K01932.02  & 5202905    & 143.5855  &$   14.84440 ^{+    0.00185 }_{   -0.00204 }$&$ 0.79  ^{+ 1.06  }_{ -0.03 }$&$ 0.012  ^{+ 0.028  }_{ -0.002 }$&$ 0.26  ^{+ 0.15  }_{ -0.02 }$&$ 2.16  ^{+ 2.62  }_{ -1.15 }$&$ 3.05  \pm{ 4.04  }$&$ 85.54 ^{+ 0.18  }_{ -2.82 }$&$ 11.3  ^{+ 3.2   }_{ -2.6  }$&$ 0.123  \pm{ 0.021  }$&$ 1715  \pm{ 359   }$&$ 200   \pm{ 54    }$& 7.2   & 0.5  &0.049 & 0.562  \\
K01955.01  & 9892816    & 132.6668  &$   15.17019 ^{+    0.00021 }_{   -0.00035 }$&$ 0.94  ^{+ 0.02  }_{ -0.04 }$&$ 0.016  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 4.40  \pm{ 1.23  }$&$ 85.02 ^{+ 1.14  }_{ -1.28 }$&$ 12.7  ^{+ 2.3   }_{ -2.8  }$&$ 0.146  \pm{ 0.009  }$&$ 1309  \pm{ 128   }$&$ 230   \pm{ 12    }$& 4.3   & 1.1  &0.124 & 0.876  \\
K01955.02  & 9892816    & 136.4553  &$   39.45988 ^{+    0.00008 }_{   -0.00014 }$&$ 0.00  ^{+ 0.73  }_{ -0.00 }$&$ 0.012  ^{+ 0.004  }_{ -0.001 }$&$ 0.22  ^{+ 0.61  }_{ -0.22 }$&$ 3.56  ^{+ 1.04  }_{ -3.55 }$&$ 1.88  \pm{ 0.65  }$&$ 90.00 ^{+ 0.00  }_{ -1.49 }$&$ 36.7  ^{+ 8.1   }_{ -8.5  }$&$ 0.251  \pm{ 0.013  }$&$ 728   \pm{ 107   }$&$ 231   \pm{ 21    }$& 9.4   & 0.5  &0.067 & 0.781  \\
K01955.03  & 9892816    & 131.7567  &$    1.64420 ^{+    0.00003 }_{   -0.00003 }$&$ 0.20  ^{+ 0.45  }_{ -0.20 }$&$ 0.004  ^{+ 0.002  }_{ -0.000 }$&$ 0.79  ^{+ 0.08  }_{ -0.53 }$&$ 4.03  ^{+ 0.25  }_{ -2.14 }$&$ 0.54  \pm{ 0.24  }$&$ 87.71 ^{+ 2.29  }_{ -7.24 }$&$ 4.9   ^{+ 1.6   }_{ -1.1  }$&$ 0.028  \pm{ 0.002  }$&$ 1900  \pm{ 398   }$&$ 31    \pm{ 4     }$& 7.4   & 0.6  &0.008 & 0.283  \\
K01955.04  & 9892816    & 141.9958  &$   26.23420 ^{+    0.00069 }_{   -0.00105 }$&$ 0.68  ^{+ 0.20  }_{ -0.19 }$&$ 0.019  ^{+  0.003 }_{ -0.009 }$&$ 0.38  ^{+ 0.05  }_{ -0.38 }$&$ 4.72  ^{+  0.07 }_{ -4.72 }$&$ 2.53  \pm{ 0.70  }$&$ 88.82 ^{+ 0.52  }_{ -0.65 }$&$ 31.3  ^{+ 7.6   }_{ -5.8  }$&$ 0.178  \pm{ 0.012  }$&$ 747   \pm{ 104   }$&$ 170   \pm{ 17    }$& 3.6   & 1.2  &0.029 & 0.601  \\
K02004.01  & 12154526   & 146.3714  &$   56.18945 ^{+    0.00058 }_{   -0.00086 }$&$ 0.64  ^{+ 0.24  }_{ -0.62 }$&$ 0.017  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.46  }_{ -0.00 }$&$ 0.00  ^{+ 1.54  }_{ -0.00 }$&$ 2.38  \pm{ 0.66  }$&$ 89.21 ^{+ 0.77  }_{ -0.71 }$&$ 49.3  ^{+ 11.7  }_{ -9.2  }$&$ 0.291  \pm{ 0.013  }$&$ 560   \pm{ 92    }$&$ 368   \pm{ 31    }$& 7.2   & 0.9  &0.143 & 0.893  \\
K02004.02  & 12154526   & 133.5255  &$    3.18899 ^{+    0.00017 }_{   -0.00005 }$&$ 0.90  ^{+ 0.09  }_{ -0.11 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.07  ^{+ 0.16  }_{ -0.07 }$&$ 1.83  ^{+ 0.69  }_{ -1.83 }$&$ 1.73  \pm{ 0.32  }$&$ 79.74 ^{+ 1.09  }_{ -1.32 }$&$ 5.3   ^{+ 0.6   }_{ -0.8  }$&$ 0.044  \pm{ 0.003  }$&$ 1700  \pm{ 130   }$&$ 69    \pm{ 7     }$& 2.6   & 0.5  &0.021 & 0.517  \\
K02004.03  & 12154526   & 132.7764  &$    1.72107 ^{+    0.00002 }_{ -   0.00002 }$&$ 0.99  ^{+ 0.01  }_{ -0.01  }$&$ 0.008  ^{+ 0.001  }_{ -0.001  }$&$ 0.00  ^{+ 0.03  }_{ -0.00  }$&$ 0.00  ^{+ 0.05  }_{- 0.00  }$&$ 0.83  \pm{ 0.12  }$&$ 39.70  ^{+ 9.40  }_{- 9.40  }$&$ 1.3   ^{+ 0.2   }_{ -0.2  }$&$ 0.027  \pm{ 0.003  }$&$ 1250     \pm{ 300     }$&$ 37    \pm{ 7     }$& 1.9   & 1.5  &0.016 & 0.450  \\
K02011.01  & 5384079    & 132.5342  &$    7.05670 ^{+    0.00014 }_{   -0.00010 }$&$ 0.91  ^{+ 0.04  }_{ -0.05 }$&$ 0.015  ^{+ 0.001  }_{ -0.002 }$&$ 0.05  ^{+ 0.12  }_{ -0.05 }$&$ 0.02  ^{+ 3.17  }_{ -0.02 }$&$ 2.57  \pm{ 0.51  }$&$ 84.91 ^{+ 0.75  }_{ -1.13 }$&$ 10.5  ^{+ 1.4   }_{ -1.5  }$&$ 0.080  \pm{ 0.003  }$&$ 1319  \pm{ 106   }$&$ 128   \pm{ 6     }$& 2.4   & 0.7  &0.031 & 0.441  \\
K02011.02  & 5384079    & 135.3499  &$   17.26555 ^{+    0.00083 }_{   -0.00075 }$&$ 0.18  ^{+ 0.40  }_{ -0.18 }$&$ 0.008  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.56  }_{ -0.00 }$&$ 1.04  \pm{ 0.31  }$&$ 89.61 ^{+ 0.39  }_{ -1.00 }$&$ 24.3  ^{+ 6.9   }_{ -5.1  }$&$ 0.134  \pm{ 0.008  }$&$ 836   \pm{ 136   }$&$ 79    \pm{ 11    }$& 5.1   & 0.7  &0.002 & 0.049  \\
K02029.01  & 9489524    & 136.9036  &$   16.33287 ^{+    0.00032 }_{   -0.00034 }$&$ 0.78  ^{+ 0.13  }_{ -0.33 }$&$ 0.018  ^{+ 0.003  }_{ -0.004 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 1.65  \pm{ 0.49  }$&$ 88.55 ^{+ 0.86  }_{ -0.77 }$&$ 30.3  ^{+ 6.8   }_{ -6.0  }$&$ 0.122  \pm{ 0.006  }$&$ 624   \pm{ 90    }$&$ 293   \pm{ 14    }$& 2.6   & 0.2  &0.052 & 0.734  \\
K02029.02  & 9489524    & 173.2239  &$   10.05548 ^{+    0.00025 }_{   -0.00030 }$&$ 0.19  ^{+ 0.40  }_{ -0.19 }$&$ 0.010  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.05  ^{+ 0.48  }_{ -0.05 }$&$ 0.89  \pm{ 0.25  }$&$ 89.52 ^{+ 0.48  }_{ -1.15 }$&$ 22.4  ^{+ 5.0   }_{ -4.5  }$&$ 0.088  \pm{ 0.004  }$&$ 723   \pm{ 90    }$&$ 151   \pm{ 11    }$& 3.3   & 0.8  &0.006 & 0.238  \\
K02029.03  & 9489524    & 132.0775  &$    6.88721 ^{+    0.00016 }_{   -0.00023 }$&$ 0.42  ^{+ 0.26  }_{ -0.42 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 0.67  \pm{ 0.18  }$&$ 88.68 ^{+ 1.32  }_{ -0.99 }$&$ 17.6  ^{+ 3.9   }_{ -3.2  }$&$ 0.067  \pm{ 0.003  }$&$ 812   \pm{ 99    }$&$ 83    \pm{ 9     }$& 2.6   & 0.6  &0.004 & 0.158  \\
K02029.04  & 9489524    & 135.4647  &$    4.78843 ^{+    0.00011 }_{   -0.00013 }$&$ 0.52  ^{+ 0.20  }_{ -0.52 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.47  ^{+ 0.41  }_{ -0.47 }$&$ 3.99  ^{+ 0.68  }_{ -2.93 }$&$ 0.63  \pm{ 0.20  }$&$ 87.92 ^{+ 2.08  }_{ -1.42 }$&$ 13.6  ^{+ 3.5   }_{ -3.0  }$&$ 0.053  \pm{ 0.002  }$&$ 919   \pm{ 137   }$&$ 63    \pm{ 8     }$& 2.8   & 1.1  &0.004 & 0.158  \\
K02053.01  & 2307415    & 133.3943  &$   13.12155 ^{+    0.00034 }_{   -0.00030 }$&$ 0.55  ^{+ 0.21  }_{ -0.52 }$&$ 0.012  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.47  }_{ -0.00 }$&$ 0.07  ^{+ 3.90  }_{ -0.07 }$&$ 1.74  \pm{ 0.48  }$&$ 88.36 ^{+ 1.59  }_{ -1.10 }$&$ 18.4  ^{+ 4.1   }_{ -3.6  }$&$ 0.116  \pm{ 0.006  }$&$ 960   \pm{ 122   }$&$ 197   \pm{ 14    }$& 4.5   & 0.7  &0.024 & 0.377  \\
K02053.02  & 2307415    & 132.7749  &$    4.61266 ^{+    0.00010 }_{   -0.00011 }$&$ 0.67  ^{+ 0.03  }_{ -0.17 }$&$ 0.013  ^{+ 0.009  }_{ -0.003 }$&$ 0.31  ^{+ 0.41  }_{ -0.16 }$&$ 5.04  ^{+ 0.33  }_{ -0.50 }$&$ 2.40  \pm{ 1.42  }$&$ 84.45 ^{+ 2.91  }_{ -2.42 }$&$ 7.3   ^{+ 3.2   }_{ -1.9  }$&$ 0.059  \pm{ 0.003  }$&$ 1590  \pm{ 333   }$&$ 137   \pm{ 8     }$& 3.7   & 0.5  &0.039 & 0.502  \\
K02059.01  & 12301181   & 134.8728  &$    6.14730 ^{+    0.00016 }_{   -0.00009 }$&$ 0.19  ^{+ 0.26  }_{ -0.19 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.77  \pm{ 0.17  }$&$ 89.34 ^{+ 0.66  }_{ -1.00 }$&$ 16.1  ^{+ 3.0   }_{ -2.7  }$&$ 0.055  \pm{ 0.002  }$&$ 791   \pm{ 81    }$&$ 132   \pm{ 8     }$& 2.9   & 0.5  &0.047 & 0.551  \\
K02059.02  & 12301181   & 132.4311  &$    2.18574 ^{+    0.00002 }_{-    0.00002 }$&$ 0.98  ^{+ 0.02  }_{- 0.02  }$&$ 0.008  ^{+ 0.001  }_{- 0.001  }$&$ 0.00  ^{+ 0.03  }_{- 0.00  }$&$ 0.05  ^{+ 0.00  }_{- 0.05  }$&$ 0.60  \pm{ 0.10  }$&$ 57.00  ^{+ 19.00  }_{- 19.00  }$&$ 1.8  ^{+ 0.9   }_{ -0.9  }$&$ 0.029  \pm{ 0.002  }$&$ 1250     \pm{ 300     }$&$ 38   \pm{ 8     }$& 2.1   & 0.7  &0.011 & 0.216  \\
K02148.01  & 6021193    & 142.1019  &$   11.93223 ^{+    0.00021 }_{   -0.00025 }$&$ 0.00  ^{+ 0.71  }_{ -0.00 }$&$ 0.011  ^{+ 0.003  }_{ -0.000 }$&$ 0.19  ^{+ 0.41  }_{ -0.19 }$&$ 1.38  ^{+ 2.92  }_{ -1.38 }$&$ 2.68  \pm{ 0.83  }$&$ 90.00 ^{+  0.00 }_{ -4.56 }$&$ 10.1  ^{+ 3.0   }_{ -2.5  }$&$ 0.104  \pm{ 0.004  }$&$ 1128  \pm{ 159   }$&$ 194   \pm{ 17    }$& 7.0   & 0.2  &0.048 & 0.714  \\
K02148.02  & 6021193    & 132.9564  &$    7.54236 ^{+    0.00029 }_{   -0.00029 }$&$ 0.50  ^{+ 0.35  }_{ -0.50 }$&$ 0.009  ^{+ 0.002  }_{ -0.001 }$&$ 0.42  ^{+ 0.26  }_{ -0.42 }$&$ 0.28  ^{+ 2.11  }_{ -0.28 }$&$ 2.14  \pm{ 0.65  }$&$ 86.40 ^{+ 3.60  }_{ -3.88 }$&$ 7.5   ^{+ 1.9   }_{ -1.9  }$&$ 0.077  \pm{ 0.003  }$&$ 1315  \pm{ 193   }$&$ 123   \pm{ 14    }$& 5.5   & 0.4  &0.047 & 0.713  \\
K02148.03  & 6021193    & 134.7000  &$    3.61461 ^{+    0.00011 }_{   -0.00010 }$&$ 1.13  ^{+ 0.60  }_{ -0.74 }$&$ 0.008  ^{+ 0.009  }_{ -0.001 }$&$ 0.73  ^{+ 0.07  }_{ -0.32 }$&$ 2.40  ^{+ 1.96  }_{ -1.56 }$&$ 2.00  \pm{ 1.36  }$&$ 75.75 ^{+ 9.85  }_{ -5.98 }$&$ 4.3   ^{+ 1.2   }_{ -0.9  }$&$ 0.047  \pm{ 0.002  }$&$ 1734  \pm{ 269   }$&$ 72    \pm{ 9     }$& 12.1  & 0.8  &0.021 & 0.513  \\
K02158.01  & 5211199    & 132.6314  &$    4.56215 ^{+    0.00010 }_{   -0.00014 }$&$ 0.77  ^{+ 0.11  }_{ -0.27 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.11  ^{+ 0.45  }_{ -0.11 }$&$ 0.96  ^{+  0.33 }_{ -0.96 }$&$ 1.64  \pm{ 0.37  }$&$ 83.35 ^{+ 2.93  }_{ -1.72 }$&$ 6.3   ^{+ 1.2   }_{ -0.9  }$&$ 0.052  \pm{ 0.001  }$&$ 1390  \pm{ 138   }$&$ 81    \pm{ 7     }$& 3.5   & 1.0  &0.011 & 0.224  \\
K02158.02  & 5211199    & 132.1895  &$    6.68232 ^{+    0.00020 }_{   -0.00033 }$&$ 0.72  ^{+ 0.17  }_{ -0.25 }$&$ 0.007  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 1.39  \pm{ 0.49  }$&$ 85.37 ^{+ 1.66  }_{ -1.31 }$&$ 8.2   ^{+ 2.1   }_{ -1.7  }$&$ 0.072  \pm{ 0.006  }$&$ 1205  \pm{ 161   }$&$ 50    \pm{ 8     }$& 4.1   & 1.1  &0.001 & 0.033  \\
K02169.01  & 9006186    & 134.1486  &$    5.45300 ^{+    0.00009 }_{   -0.00011 }$&$ 0.71  ^{+ 0.13  }_{ -0.25 }$&$ 0.008  ^{+ 0.002  }_{ -0.001 }$&$ 0.32  ^{+ 0.16  }_{ -0.32 }$&$ 0.27  ^{+ 1.37  }_{ -0.27 }$&$ 1.01  \pm{ 0.23  }$&$ 86.53 ^{+ 1.58  }_{ -1.22 }$&$ 11.4  ^{+ 2.3   }_{ -1.7  }$&$ 0.058  \pm{ 0.002  }$&$ 1056  \pm{ 105   }$&$ 94    \pm{ 4     }$& 2.5   & 1.0  &0.097 & 0.842  \\
K02169.02  & 9006186    & 136.0883  &$    3.26661 ^{+    0.00006 }_{   -0.00005 }$&$ 0.66  ^{+ 0.14  }_{ -0.36 }$&$ 0.007  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.00  ^{+ 0.71  }_{ -0.00 }$&$ 0.86  \pm{ 0.21  }$&$ 85.27 ^{+ 2.92  }_{ -1.59 }$&$ 7.9   ^{+ 1.5   }_{ -1.4  }$&$ 0.042  \pm{ 0.001  }$&$ 1275  \pm{ 135   }$&$ 58    \pm{ 3     }$& 2.4   & 0.1  &0.065 & 0.776  \\
K02169.03  & 9006186    & 133.2112  &$    4.27235 ^{+    0.00011 }_{   -0.00009 }$&$ 0.59  ^{+ 0.21  }_{ -0.46 }$&$ 0.006  ^{+ 0.001  }_{ -0.001 }$&$ 0.29  ^{+ 0.16  }_{ -0.29 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.69  \pm{ 0.18  }$&$ 86.57 ^{+ 2.72  }_{ -1.77 }$&$ 9.5   ^{+ 2.1   }_{ -1.5  }$&$ 0.050  \pm{ 0.001  }$&$ 1150  \pm{ 138   }$&$ 48    \pm{ 4     }$& 2.7   & 1.2  &0.040 & 0.675  \\
K02169.04  & 9006186    & 132.2252  &$    2.19259 ^{+    0.00003 }_{   -0.00005 }$&$ 1.44  ^{+ 1.29  }_{ -1.13 }$&$ 0.004  ^{+ 0.000  }_{ -0.001 }$&$ 0.73  ^{+ 0.14  }_{ -0.40 }$&$ 1.50  ^{+ 1.17  }_{ -1.32 }$&$ 0.51  \pm{ 0.18  }$&$ 76.83 ^{+ 10.21 }_{ -10.57 }$&$ 6.3   ^{+ 1.8   }_{ -1.6  }$&$ 0.032  \pm{ 0.001  }$&$ 1435  \pm{ 269   }$&$ 18    \pm{ 3     }$& 1.0   & 0.6  &0.022 & 0.525  \\
K02173.01  & 11774991   & 141.1054  &$   37.81526 ^{+    0.00098 }_{   -0.00103 }$&$ 0.39  ^{+ 0.38  }_{ -0.39 }$&$ 0.013  ^{+ 0.003  }_{ -0.000 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.00  ^{+ 1.13  }_{ -0.00 }$&$ 1.16  \pm{ 0.29  }$&$ 89.58 ^{+ 0.42  }_{ -0.60 }$&$ 52.3  ^{+ 11.0  }_{ -9.8  }$&$ 0.200  \pm{ 0.006  }$&$ 434   \pm{ 58    }$&$ 272   \pm{ 21    }$& 5.1   & 0.8  &0.011 & 0.215  \\
K02173.02  & 11774991   & 171.1865  &$   53.57820 ^{+    0.00170 }_{   -0.00251 }$&$ 0.07  ^{+ 0.72  }_{ -0.07 }$&$ 0.012  ^{+ 0.005  }_{ -0.001 }$&$ 0.90  ^{+  0.01 }_{ -0.71 }$&$ 3.82  ^{+ 0.88  }_{ -0.52 }$&$ 1.04  \pm{ 0.35  }$&$ 89.94 ^{+ 0.06  }_{ -0.76 }$&$ 68.7  ^{+ 16.6  }_{ -13.8 }$&$ 0.253  \pm{ 0.007  }$&$ 389   \pm{ 57    }$&$ 280   \pm{ 26    }$& 6.3   & 0.9  &0.007 & 0.142  \\
K02175.01  & 9022166    & 142.1752  &$   26.84734 ^{+    0.00034 }_{   -0.00035 }$&$ 0.00  ^{+ 0.60  }_{ -0.00 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 1.25  }_{ -0.00 }$&$ 1.79  \pm{ 0.59  }$&$ 90.00 ^{+ 0.00  }_{ -1.03 }$&$ 33.9  ^{+ 12.9  }_{ -7.0  }$&$ 0.167  \pm{ 0.009  }$&$ 614   \pm{ 117   }$&$ 259   \pm{ 26    }$& 6.3   & 0.6  &0.039 & 0.506  \\
K02175.02  & 9022166    & 179.5122  &$   72.38130 ^{+    0.00071 }_{   -0.00134 }$&$ 0.25  ^{+ 0.28  }_{ -0.25 }$&$ 0.018  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 1.87  \pm{ 0.50  }$&$ 89.79 ^{+ 0.21  }_{ -0.32 }$&$ 71.0  ^{+ 19.0  }_{ -13.7 }$&$ 0.320  \pm{ 0.016  }$&$ 423   \pm{ 60    }$&$ 364   \pm{ 42    }$& 7.7   & 0.3  &0.031 & 0.441  \\
K02289.01  & 3867615    & 157.3033  &$   62.78500 ^{+    0.00180 }_{   -0.00121 }$&$ 0.76  ^{+ 0.12  }_{ -0.64 }$&$ 0.018  ^{+ 0.001  }_{ -0.005 }$&$ 0.00  ^{+ 0.49  }_{ -0.00 }$&$ 0.00  ^{+ 0.71  }_{ -0.00 }$&$ 2.65  \pm{ 0.82  }$&$ 89.21 ^{+ 0.69  }_{ -0.37 }$&$ 53.7  ^{+ 11.1  }_{ -12.5 }$&$ 0.335  \pm{ 0.015  }$&$ 558   \pm{ 80    }$&$ 358   \pm{ 43    }$& 5.9   & 0.6  &0.012 & 0.234  \\
K02289.02  & 3867615    & 147.2808  &$   20.09846 ^{+    0.00061 }_{   -0.00076 }$&$ 0.14  ^{+ 0.45  }_{ -0.14 }$&$ 0.012  ^{+ 0.001  }_{ -0.003 }$&$ 0.17  ^{+ 0.17  }_{ -0.17 }$&$ 0.58  ^{+  0.07 }_{ -0.58 }$&$ 1.63  \pm{ 0.43  }$&$ 89.69 ^{+ 0.31  }_{ -1.05 }$&$ 25.5  ^{+ 6.2   }_{ -5.1  }$&$ 0.148  \pm{ 0.009  }$&$ 811   \pm{ 110   }$&$ 157   \pm{ 22    }$& 5.3   & 0.4  &0.007 & 0.155  \\
K02311.01  & 4247991    & 294.4400  &$  191.88569 ^{+    0.10191 }_{   -0.03101 }$&$ 0.00  ^{+ 1.00  }_{ -0.00 }$&$ 0.024  ^{+ 0.004  }_{ -0.022 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.09  ^{+ 0.24  }_{ -0.09 }$&$ 3.22  \pm{ 2.86  }$&$ 90.00 ^{+  0.00 }_{ -1.60 }$&$ 120.6 ^{+ 84.8  }_{ -52.3 }$&$ 0.691  \pm{ 0.079  }$&$ 239   \pm{ 42    }$&$ 200     \pm{ 39    }$& 4.8   & 0.5  &0.009 & 0.177  \\
K02311.02  & 4247991    & 145.0410  &$   13.72535 ^{+    0.00072 }_{   -0.00069 }$&$ 0.91  ^{+  0.09 }_{ -0.91 }$&$ 0.010  ^{+ 0.016  }_{ -0.008 }$&$ 0.02  ^{+ 0.00  }_{ -0.02 }$&$ 0.17  ^{+ 0.03  }_{ -0.17 }$&$ 1.38  \pm{ 1.90  }$&$ 81.52 ^{+ 0.68  }_{ -0.58 }$&$ 20.0  ^{+ 13.5  }_{ -8.3  }$&$ 0.119  \pm{ 0.013  }$&$ 514   \pm{ 75    }$&$ 51     \pm{ 15    }$& 7.5   & 0.3  &0.002 & 0.049  \\
K02352.01  & 8013439    & 133.0583  &$   13.39140 ^{+    0.00057 }_{   -0.00034 }$&$ 0.68  ^{+ 0.13  }_{ -0.05 }$&$ 0.010  ^{+ 0.027  }_{ -0.002 }$&$ 0.53  ^{+ 0.18  }_{ -0.14 }$&$ 4.43  ^{+ 0.26  }_{ -0.66 }$&$ 3.37  \pm{ 5.00  }$&$ 85.30 ^{+ 0.84  }_{ -1.00 }$&$ 8.2   ^{+ 1.4   }_{ -0.7  }$&$ 0.119  \pm{ 0.018  }$&$ 1522  \pm{ 215   }$&$ 50    \pm{ 4     }$& 4.3   & 0.8  &0.040 & 0.676  \\
K02352.02  & 8013439    & 134.7477  &$    5.62903 ^{+    0.00012 }_{   -0.00010 }$&$ 0.32  ^{+ 0.29  }_{ -0.32 }$&$ 0.005  ^{+ 0.001  }_{ -0.000 }$&$ 0.01  ^{+ 0.22  }_{ -0.01 }$&$ 0.01  ^{+ 0.91  }_{ -0.01 }$&$ 0.84  \pm{ 0.27  }$&$ 87.98 ^{+ 2.02  }_{ -2.45 }$&$ 8.7   ^{+ 2.4   }_{ -2.2  }$&$ 0.065  \pm{ 0.005  }$&$ 1467  \pm{ 229   }$&$ 38    \pm{ 2     }$& 4.5   & 0.4  &0.052 & 0.731  \\
K02352.03  & 8013439    & 137.9280  &$    8.25621 ^{+    0.00023 }_{   -0.00028 }$&$ 0.87  ^{+ 0.06  }_{ -0.10 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 3.83  ^{+  1.69 }_{ -3.83 }$&$ 1.27  \pm{ 0.30  }$&$ 85.87 ^{+ 0.77  }_{ -0.88 }$&$ 11.7  ^{+ 1.9   }_{ -2.0  }$&$ 0.083  \pm{ 0.007  }$&$ 1261  \pm{ 147   }$&$ 37    \pm{ 3     }$& 2.6   & 1.9  &0.041 & 0.681  \\
K02541.01  & 12306058   & 137.9603  &$    7.41682 ^{+    0.00030 }_{   -0.00026 }$&$ 0.41  ^{+ 0.26  }_{ -0.34 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.01  ^{+ 0.36  }_{ -0.01 }$&$ 2.40  \pm{ 0.53  }$&$ 86.31 ^{+ 3.16  }_{ -2.30 }$&$ 5.6   ^{+ 1.5   }_{ -0.3  }$&$ 0.079  \pm{ 0.002  }$&$ 1376  \pm{ 174   }$&$ 78    \pm{ 12    }$& 8.3   & 0.4  &0.053 & 0.583  \\
K02541.02  & 12306058   & 146.9230  &$   20.48565 ^{+    0.00148 }_{   -0.00123 }$&$ 0.23  ^{+ 0.46  }_{ -0.23 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.43  ^{+ 0.02  }_{ -0.43 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 2.84  \pm{ 0.97  }$&$ 88.97 ^{+ 1.02  }_{ -2.05 }$&$ 11.3  ^{+ 3.5   }_{ -1.4  }$&$ 0.160  \pm{ 0.028  }$&$ 973   \pm{ 133   }$&$ 93    \pm{ 20    }$& 11.1  & 0.3  &0.037 & 0.488  \\
K02585.01  & 7673841    & 136.3069  &$    5.34189 ^{+    0.00018 }_{   -0.00017 }$&$ 0.92  ^{+ 0.87  }_{ -0.07 }$&$ 0.009  ^{+ 0.010  }_{ -0.002 }$&$ 0.03  ^{+ 0.07  }_{ -0.03 }$&$ 0.33  ^{+ 0.21  }_{ -0.33 }$&$ 2.25  \pm{ 1.68  }$&$ 81.02 ^{+ 0.16  }_{ -1.70 }$&$ 6.2   ^{+ 3.6   }_{ -1.1  }$&$ 0.066  \pm{ 0.003  }$&$ 1778  \pm{ 405   }$&$ 67    \pm{ 8     }$& 3.1   & 0.7  &0.025 & 0.562  \\
K02585.02  & 7673841    & 135.1572  &$   10.42305 ^{+    0.00027 }_{   -0.00032 }$&$ 0.73  ^{+ 0.18  }_{ -0.27 }$&$ 0.008  ^{+ 0.003  }_{ -0.003 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.00  ^{+ 0.88  }_{ -0.00 }$&$ 1.30  \pm{ 0.51  }$&$ 87.22 ^{+ 1.15  }_{ -0.95 }$&$ 14.1  ^{+ 3.1   }_{ -2.9  }$&$ 0.096  \pm{ 0.006  }$&$ 1106  \pm{ 158   }$&$ 73    \pm{ 11    }$& 3.6   & 0.5  &0.021 & 0.514  \\
K02585.03  & 7673841    & 138.5965  &$    7.87811 ^{+    0.00025 }_{   -0.00025 }$&$ 0.88  ^{+ 0.62  }_{ -0.44 }$&$ 0.008  ^{+ 0.020  }_{ -0.003 }$&$ 0.66  ^{+  0.01 }_{ -0.66 }$&$ 3.93  ^{+ 0.59  }_{ -3.89 }$&$ 1.27  \pm{ 1.95  }$&$ 85.72 ^{+ 2.23  }_{ -2.82 }$&$ 11.0  ^{+ 2.9   }_{ -2.4  }$&$ 0.080  \pm{ 0.006  }$&$ 1255  \pm{ 205   }$&$ 47    \pm{ 10    }$& 2.7   & 0.2  &0.005 & 0.206  \\
K02595.01  & 8883329    & 134.0478  &$    9.18252 ^{+    0.00029 }_{   -0.00033 }$&$ 1.00  ^{+ 0.03  }_{ -0.34 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.33  ^{+ 0.32  }_{ -0.33 }$&$ 0.65  ^{+ 0.00  }_{ -0.65 }$&$ 2.50  \pm{ 0.60  }$&$ 83.05 ^{+ 2.94  }_{ -0.60 }$&$ 8.3   ^{+ 1.7   }_{ -1.2  }$&$ 0.098  \pm{ 0.003  }$&$ 1558  \pm{ 167   }$&$ 85    \pm{ 10    }$& 4.6   & 0.1  &0.024 & 0.378  \\
K02595.02  & 8883329    & 140.4080  &$   14.61360 ^{+    0.00076 }_{   -0.00084 }$&$ 0.88  ^{+ 0.57  }_{ -0.12 }$&$ 0.010  ^{+ 0.004  }_{ -0.002 }$&$ 0.17  ^{+  0.04 }_{ -0.17 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 2.55  \pm{ 1.05  }$&$ 85.73 ^{+ 0.46  }_{ -1.13 }$&$ 12.1  ^{+ 4.2   }_{ -2.4  }$&$ 0.134  \pm{ 0.004  }$&$ 1299  \pm{ 223   }$&$ 81    \pm{ 13    }$& 5.0   & 0.8  &0.036 & 0.485  \\
K02672.01  & 11253827   & 182.6526  &$   88.51658 ^{+    0.00020 }_{   -0.00016 }$&$ 0.52  ^{+ 0.28  }_{ -0.52 }$&$ 0.044  ^{+ 0.008  }_{ -0.001 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.00  ^{+ 0.69  }_{ -0.00 }$&$ 5.34  \pm{ 1.48  }$&$ 89.61 ^{+ 0.39  }_{ -0.37 }$&$ 71.9  ^{+ 18.1  }_{ -16.5 }$&$ 0.374  \pm{ 0.010  }$&$ 425   \pm{ 60    }$&$ 2611  \pm{ 35    }$& 8.1   & 0.3  &0.846 & 0.993  \\
K02672.02  & 11253827   & 162.5118  &$   42.99066 ^{+    0.00009 }_{   -0.00014 }$&$ 0.65  ^{+ 0.25  }_{ -0.65 }$&$ 0.032  ^{+ 0.002  }_{ -0.003 }$&$ 0.01  ^{+ 0.62  }_{ -0.01 }$&$ 0.00  ^{+ 1.01  }_{ -0.00 }$&$ 3.89  \pm{ 1.03  }$&$ 89.22 ^{+ 0.78  }_{ -0.69 }$&$ 43.6  ^{+ 11.8  }_{ -9.1  }$&$ 0.231  \pm{ 0.006  }$&$ 536   \pm{ 78    }$&$ 1162  \pm{ 17    }$& 5.5   & 0.3  &0.894 & 0.995  \\
K02674.01  & 8022489    & 272.3869  &$  197.51031 ^{+    0.00035 }_{   -0.00032 }$&$ 0.82  ^{+ 0.58  }_{ -0.32 }$&$ 0.052  ^{+ 0.001  }_{ -0.006 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.00  ^{+ 0.94  }_{ -0.00 }$&$ 10.05 \pm{ 3.96  }$&$ 89.46 ^{+ 0.30  }_{ -0.81 }$&$ 83.8  ^{+ 33.0  }_{ -27.5 }$&$ 0.671  \pm{ 0.021  }$&$ 422   \pm{ 77    }$&$ 2643  \pm{ 58    }$& 10.9  & 0.8  &0.339 & 0.962  \\
K02674.02  & 8022489    & 140.0090  &$   11.17265 ^{+    0.00061 }_{   -0.00066 }$&$ 1.08  ^{+ 4.19  }_{ -0.42 }$&$ 0.009  ^{+ 0.036  }_{ -0.000 }$&$ 0.24  ^{+  0.17 }_{ -0.23 }$&$ 1.58  ^{+  1.16 }_{ -1.50 }$&$ 1.57  \pm{ 3.22  }$&$ 81.42 ^{+ 0.07  }_{ -1.48 }$&$ 13.4  ^{+ 7.5   }_{ -4.4  }$&$ 0.099  \pm{ 0.003  }$&$ 1473  \pm{ 1376  }$&$ 80    \pm{ 13    }$& 5.5   & 0.4  &0.023 & 0.540  \\
K02674.03  & 8022489    & 133.0107  &$    2.53574 ^{+    0.00006 }_{   -0.00006 }$&$ 0.91  ^{+ 0.34  }_{ -0.91 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.51  ^{+ 0.35  }_{ -0.46 }$&$ 0.72  ^{+ 1.44  }_{ -0.63 }$&$ 2.15  \pm{ 0.60  }$&$ 73.54 ^{+ 16.44 }_{ -7.31 }$&$ 3.4   ^{+ 1.3   }_{ -0.7  }$&$ 0.037  \pm{ 0.001  }$&$ 2216  \pm{ 385   }$&$ 73    \pm{ 6     }$& 15.7  & 0.7  &0.017 & 0.465  \\
K02675.01  & 5794570    & 132.4894  &$    5.44833 ^{+    0.00002 }_{   -0.00002 }$&$ 0.59  ^{+ 0.23  }_{ -0.40 }$&$ 0.021  ^{+ 0.006  }_{ -0.002 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 1.86  }_{ -0.00 }$&$ 2.21  \pm{ 0.68  }$&$ 87.45 ^{+ 1.89  }_{ -2.32 }$&$ 13.4  ^{+ 2.2   }_{ -3.0  }$&$ 0.061  \pm{ 0.003  }$&$ 1037  \pm{ 130   }$&$ 554   \pm{ 6     }$& 2.6   & 1.7  &0.796 & 0.990  \\
K02675.02  & 5794570    & 131.8464  &$    1.11613 ^{+    0.00001 }_{   -0.00001 }$&$ 0.57  ^{+ 0.37  }_{ -0.49 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.10  ^{+ 0.58  }_{ -0.10 }$&$ 0.00  ^{+ 2.48  }_{ -0.00 }$&$ 1.05  \pm{ 0.29  }$&$ 82.17 ^{+ 6.90  }_{ -10.33 }$&$ 4.2   ^{+ 0.9   }_{ -0.9  }$&$ 0.021  \pm{ 0.001  }$&$ 1856  \pm{ 235   }$&$ 106   \pm{ 2     }$& 1.7   & 1.8  &0.112 & 0.759  \\
K02687.01  & 7202957    & 132.0299  &$    1.71684 ^{+    0.00001 }_{   -0.00001 }$&$ 0.99  ^{+  0.01 }_{ -0.12 }$&$ 0.010  ^{+ 0.001  }_{ -0.002 }$&$ 0.05  ^{+ 0.14  }_{ -0.05 }$&$ 1.19  ^{+  0.36 }_{ -1.19 }$&$ 3.31  \pm{ 0.92  }$&$ 62.19 ^{+ 11.67 }_{ -0.76 }$&$ 2.1   ^{+ 1.0   }_{ -0.1  }$&$ 0.029  \pm{ 0.001  }$&$ 2648  \pm{ 363   }$&$ 62    \pm{ 1     }$& 2.5   &\textbf{ 4.3  }&0.469 & 0.957  \\
K02687.02  & 7202957    & 136.2009  &$    8.16739 ^{+    0.00007 }_{   -0.00007 }$&$ 0.94  ^{+ 0.02  }_{ -0.05 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 3.69  \pm{ 0.73  }$&$ 82.00 ^{+ 2.06  }_{ -1.53 }$&$ 6.3   ^{+ 1.9   }_{ -0.6  }$&$ 0.082  \pm{ 0.003  }$&$ 1485  \pm{ 152   }$&$ 104   \pm{ 3     }$& 3.6   & 2.7  &0.415 & 0.947  \\
K02693.01  & 5185897    & 133.8593  &$    4.08141 ^{+    0.00007 }_{   -0.00006 }$&$ 0.22  ^{+ 0.16  }_{ -0.22 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.85  \pm{ 0.17  }$&$ 89.05 ^{+ 0.95  }_{ -0.83 }$&$ 12.9  ^{+ 2.0   }_{ -1.7  }$&$ 0.044  \pm{ 0.002  }$&$ 823   \pm{ 69    }$&$ 156   \pm{ 6     }$& 2.4   & 2.0  &0.049 & 0.722  \\
K02693.02  & 5185897    & 142.1177  &$   11.41942 ^{+    0.00034 }_{   -0.00045 }$&$ 0.89  ^{+ 0.04  }_{ -0.23 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.68  }_{ -0.00 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 2.16  \pm{ 0.61  }$&$ 86.01 ^{+ 1.43  }_{ -0.85 }$&$ 14.4  ^{+ 3.5   }_{ -2.5  }$&$ 0.098  \pm{ 0.018  }$&$ 826   \pm{ 97    }$&$ 158   \pm{ 11    }$& 3.3   & 1.4  &0.021 & 0.515  \\
K02693.03  & 5185897    & 136.8490  &$    6.83448 ^{+    0.00011 }_{   -0.00015 }$&$ 0.37  ^{+ 0.20  }_{ -0.37 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.78  \pm{ 0.17  }$&$ 88.98 ^{+ 1.02  }_{ -0.73 }$&$ 20.0  ^{+ 4.0   }_{ -2.8  }$&$ 0.062  \pm{ 0.002  }$&$ 652   \pm{ 63    }$&$ 153   \pm{ 8     }$& 2.4   & 1.3  &0.026 & 0.571  \\
K02696.01  & 11071200   & 214.7486  &$   96.45620 ^{+    0.00041 }_{   -0.00057 }$&$ 0.65  ^{+ 0.16  }_{ -0.65 }$&$ 0.030  ^{+ 0.006  }_{ -0.000 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 4.69  }_{ -0.00 }$&$ 6.63  \pm{ 1.78  }$&$ 89.26 ^{+ 0.74  }_{ -0.50 }$&$ 50.6  ^{+ 11.6  }_{ -10.4 }$&$ 0.485  \pm{ 0.021  }$&$ 653   \pm{ 90    }$&$ 978   \pm{ 73    }$& 11.4  & 0.5  &0.065 & 0.634  \\
K02696.02  & 11071200   & 143.4267  &$   44.56505 ^{+    0.00018 }_{   -0.00012 }$&$ 0.52  ^{+ 0.22  }_{ -0.52 }$&$ 0.016  ^{+ 0.003  }_{ -0.002 }$&$ 0.36  ^{+ 0.14  }_{ -0.36 }$&$ 0.16  ^{+ 0.27  }_{ -0.16 }$&$ 3.56  \pm{ 1.16  }$&$ 89.08 ^{+ 0.92  }_{ -0.82 }$&$ 29.9  ^{+ 9.1   }_{ -6.8  }$&$ 0.290  \pm{ 0.013  }$&$ 824   \pm{ 140   }$&$ 366   \pm{ 37    }$& 8.6   & 0.8  &0.103 & 0.741  \\
K02714.01  & 12206313   & 140.5597  &$   14.38351 ^{+    0.00023 }_{   -0.00022 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.012  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 2.63  \pm{ 0.71  }$&$ 90.00 ^{+ 0.00  }_{ -1.25 }$&$ 13.6  ^{+ 4.2   }_{ -2.3  }$&$ 0.125  \pm{ 0.004  }$&$ 1146  \pm{ 157   }$&$ 191   \pm{ 16    }$& 8.2   & 1.5  &0.066 & 0.640  \\
K02714.02  & 12206313   & 170.0987  &$   47.31319 ^{+    0.00058 }_{   -0.00059 }$&$ 0.00  ^{+ 0.64  }_{ -0.00 }$&$ 0.014  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 2.78  \pm{ 0.80  }$&$ 90.00 ^{+  0.00 }_{ -1.14 }$&$ 32.1  ^{+ 9.8   }_{ -6.4  }$&$ 0.276  \pm{ 0.009  }$&$ 728   \pm{ 109   }$&$ 256   \pm{ 30    }$& 10.9  & 0.9  &0.074 & 0.667  \\
K02722.01  & 7673192    & 134.9353  &$    6.12482 ^{+    0.00013 }_{   -0.00013 }$&$ 0.33  ^{+ 0.24  }_{ -0.33 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 1.55  \pm{ 0.35  }$&$ 88.31 ^{+ 1.69  }_{ -1.62 }$&$ 10.8  ^{+ 1.9   }_{ -1.7  }$&$ 0.072  \pm{ 0.003  }$&$ 1301  \pm{ 124   }$&$ 147   \pm{ 8     }$& 4.0   & 1.5  &0.062 & 0.768  \\
K02722.02  & 7673192    & 136.3216  &$   11.24280 ^{+    0.00031 }_{   -0.00034 }$&$ 0.54  ^{+ 0.11  }_{ -0.54 }$&$ 0.011  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 1.69  \pm{ 0.42  }$&$ 88.18 ^{+ 1.82  }_{ -0.56 }$&$ 16.6  ^{+ 3.0   }_{ -3.1  }$&$ 0.108  \pm{ 0.005  }$&$ 1048  \pm{ 111   }$&$ 142   \pm{ 11    }$& 4.3   & 0.5  &0.034 & 0.637  \\
K02722.03  & 7673192    & 133.7748  &$    4.02871 ^{+    0.00008 }_{   -0.00009 }$&$ 0.39  ^{+ 0.26  }_{ -0.39 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.03  ^{+ 0.70  }_{ -0.03 }$&$ 1.32  \pm{ 0.34  }$&$ 87.23 ^{+ 2.77  }_{ -2.61 }$&$ 7.8   ^{+ 1.6   }_{ -1.4  }$&$ 0.054  \pm{ 0.003  }$&$ 1532  \pm{ 163   }$&$ 102   \pm{ 6     }$& 3.6   & 0.5  &0.012 & 0.382  \\
K02722.04  & 7673192    & 137.4936  &$    8.92108 ^{+    0.00031 }_{   -0.00029 }$&$ 0.54  ^{+ 0.11  }_{ -0.54 }$&$ 0.010  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 1.51  \pm{ 0.40  }$&$ 87.91 ^{+ 2.09  }_{ -0.74 }$&$ 14.2  ^{+ 2.8   }_{ -2.8  }$&$ 0.092  \pm{ 0.005  }$&$ 1125  \pm{ 135   }$&$ 115   \pm{ 10    }$& 3.9   & 1.6  &0.033 & 0.629  \\
K02722.05  & 7673192    & 135.3861  &$   16.53433 ^{+    0.00087 }_{   -0.00104 }$&$ 0.37  ^{+ 0.29  }_{ -0.37 }$&$ 0.008  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 1.04  \pm{ 0.31  }$&$ 89.12 ^{+ 0.88  }_{ -0.91 }$&$ 22.7  ^{+ 5.3   }_{ -5.0  }$&$ 0.130  \pm{ 0.009  }$&$ 881   \pm{ 129   }$&$ 96    \pm{ 14    }$& 4.9   & 0.5  &0.005 & 0.211  \\
K02732.01  & 9886361    & 134.4527  &$    7.03142 ^{+    0.00023 }_{   -0.00027 }$&$ 0.98  ^{+ 0.05  }_{ -0.07 }$&$ 0.014  ^{+  0.003 }_{ -0.004 }$&$ 0.16  ^{+ 0.07  }_{ -0.08 }$&$ 1.39  ^{+ 0.39  }_{ -1.38 }$&$ 9.16  \pm{ 0.75  }$&$ 76.51 ^{+ 0.75  }_{ -0.33 }$&$ 4.1   ^{+ 0.2   }_{ -0.0  }$&$ 0.116  \pm{ 0.005  }$&$ 2034  \pm{ 30    }$&$ 140   \pm{ 7     }$& 6.6   & 0.2  &0.015 & 0.439  \\
K02732.02  & 9886361    & 144.1688  &$   13.61163 ^{+    0.00041 }_{   -0.00044 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 1.81  \pm{ 0.75  }$&$ 90.00 ^{+ 0.00  }_{ -2.02 }$&$ 13.5  ^{+ 5.9   }_{ -3.8  }$&$ 0.116  \pm{ 0.012  }$&$ 1111  \pm{ 236   }$&$ 96    \pm{ 10    }$& 7.4   & 0.2  &0.012 & 0.371  \\
K02732.03  & 9886361    & 140.7182  &$   54.28085 ^{+    0.00238 }_{   -0.00179 }$&$ 0.66  ^{+ 0.22  }_{ -0.52 }$&$ 0.011  ^{+ 0.002  }_{ -0.003 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.00  ^{+ 0.63  }_{ -0.00 }$&$ 1.93  \pm{ 1.15  }$&$ 89.20 ^{+ 0.69  }_{ -0.56 }$&$ 42.6  ^{+ 18.9  }_{ -15.3 }$&$ 0.318  \pm{ 0.034  }$&$ 610   \pm{ 155   }$&$ 157   \pm{ 21    }$& 6.7   & 0.5  &0.031 & 0.613  \\
K02732.04  & 9886361    & 146.8040  &$   24.56084 ^{+    0.00009 }_{   -0.00181 }$&$ 0.12  ^{+ 0.77  }_{ -0.12 }$&$ 0.007  ^{+ 0.001  }_{ -0.002 }$&$ 0.01  ^{+ 0.56  }_{ -0.01 }$&$ 0.00  ^{+ 3.81  }_{ -0.00 }$&$ 1.16  \pm{ 0.57  }$&$ 89.76 ^{+ 0.24  }_{ -1.56 }$&$ 25.9  ^{+ 12.4  }_{ -8.5  }$&$ 0.171  \pm{ 0.014  }$&$ 779   \pm{ 220   }$&$ 60    \pm{ 13    }$& 6.5   & 1.0  &0.006 & 0.225  \\
K02949.01  & 6026737    & 132.3611  &$   10.17444 ^{+    0.00045 }_{   -0.00056 }$&$ 0.70  ^{+ 1.07  }_{ -0.01 }$&$ 0.013  ^{+ 0.016  }_{ -0.007 }$&$ 0.35  ^{+ 0.21  }_{ -0.30 }$&$ 4.48  ^{+ 0.20  }_{ -3.49 }$&$ 3.08  \pm{ 2.83  }$&$ 83.82 ^{+ 1.40  }_{ -1.63 }$&$ 9.8   ^{+ 3.4   }_{ -2.2  }$&$ 0.096  \pm{ 0.003  }$&$ 1600  \pm{ 614   }$&$ 74    \pm{ 12    }$& 6.6   & 0.6  &0.018 & 0.309  \\
K02949.02  & 6026737    & 134.8168  &$    3.75017 ^{+    0.00000 }_{   -0.00000 }$&$ 0.63  ^{+ 0.28  }_{ -0.23 }$&$ 0.005  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.04  ^{+ 0.53  }_{ -0.04 }$&$ 1.13  \pm{ 0.41  }$&$ 83.41 ^{+ 2.39  }_{ -2.76 }$&$ 5.2   ^{+ 1.4   }_{ -1.1  }$&$ 0.049  \pm{ 0.005  }$&$ 1747  \pm{ 274   }$&$ 32    \pm{ 7     }$& 4.1   & 1.4  &0.006 & 0.124  \\
K03083.01  & 7106173    & 133.2040  &$   10.18329 ^{+    0.00044 }_{   -0.00043 }$&$ 0.98  ^{+ 1.51  }_{ -0.08 }$&$ 0.007  ^{+ 0.025  }_{ -0.002 }$&$ 0.21  ^{+  0.15 }_{ -0.21 }$&$ 0.40  ^{+  0.09 }_{ -0.40 }$&$ 0.82  \pm{ 1.58  }$&$ 85.63 ^{+ 0.38  }_{ -1.30 }$&$ 19.3  ^{+ 5.6   }_{ -5.5  }$&$ 0.096  \pm{ 0.004  }$&$ 1095  \pm{ 353   }$&$ 50    \pm{ 9     }$& 2.8   & 0.7  &0.005 & 0.194  \\
K03083.02  & 7106173    & 135.2410  &$    6.23203 ^{+    0.00023 }_{   -0.00025 }$&$ 0.89  ^{+ 1.32  }_{ -0.05 }$&$ 0.006  ^{+ 0.025  }_{ -0.003 }$&$ 0.05  ^{+  0.00 }_{ -0.05 }$&$ 6.21  ^{+  0.07 }_{ -6.20 }$&$ 0.64  \pm{ 1.61  }$&$ 84.34 ^{+ 0.46  }_{ -1.06 }$&$ 14.0  ^{+ 3.9   }_{ -3.4  }$&$ 0.069  \pm{ 0.003  }$&$ 1307  \pm{ 436   }$&$ 29    \pm{ 7     }$& 2.4   & 0.6  &0.005 & 0.194  \\
K03083.03  & 7106173    & 134.8440  &$    8.29442 ^{+    0.00047 }_{   -0.00033 }$&$ 0.46  ^{+ 0.42  }_{ -0.46 }$&$ 0.006  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 0.65  \pm{ 0.20  }$&$ 88.51 ^{+ 1.49  }_{ -1.31 }$&$ 16.8  ^{+ 4.5   }_{ -3.3  }$&$ 0.084  \pm{ 0.004  }$&$ 931   \pm{ 150   }$&$ 34    \pm{ 8     }$& 3.2   & 0.3  &0.004 & 0.162  \\
K03097.01  & 7582689    & 137.4610  &$   11.92196 ^{+    0.00069 }_{   -0.00060 }$&$ 0.77  ^{+ 1.13  }_{ -0.12 }$&$ 0.007  ^{+ 0.018  }_{ -0.001 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 1.81  \pm{ 2.53  }$&$ 85.86 ^{+  1.79 }_{ -3.30 }$&$ 9.9   ^{+ 4.0   }_{ -2.5  }$&$ 0.108  \pm{ 0.003  }$&$ 1281  \pm{ 249   }$&$ 51    \pm{ 8     }$& 5.5   & 0.4  &0.024 & 0.555  \\
K03097.02  & 7582689    & 138.0420  &$    6.80273 ^{+    0.00027 }_{   -0.00029 }$&$ 0.04  ^{+ 1.56  }_{ -0.50 }$&$ 0.005  ^{+ 0.034  }_{ -0.001 }$&$ 0.38  ^{+ 0.50  }_{ -0.12 }$&$ 0.22  ^{+ 4.53  }_{ -3.52 }$&$ 1.10  \pm{ 3.81  }$&$ 89.74 ^{+  0.26 }_{ -8.58 }$&$ 8.0   ^{+ 2.2   }_{ -2.1  }$&$ 0.074  \pm{ 0.002  }$&$ 1352  \pm{ 231   }$&$ 31    \pm{ 6     }$& 4.7   & 0.4  &0.007 & 0.264  \\
K03097.03  & 7582689    & 140.1620  &$    8.70295 ^{+    0.00036 }_{   -0.00039 }$&$ 0.81  ^{+ 0.45  }_{ -0.19 }$&$ 0.005  ^{+ 0.006  }_{ -0.002 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 2.67  ^{+  0.20 }_{ -2.66 }$&$ 1.27  \pm{ 0.98  }$&$ 85.10 ^{+ 0.58  }_{ -1.26 }$&$ 8.8   ^{+ 2.4   }_{ -1.7  }$&$ 0.088  \pm{ 0.003  }$&$ 1358  \pm{ 215   }$&$ 26    \pm{ 7     }$& 4.2   & 0.6  &0.006 & 0.229  \\
K03111.01  & 8581240    & 138.5101  &$   10.76792 ^{+    0.00044 }_{   -0.00054 }$&$ 0.90  ^{+ 0.25  }_{ -0.18 }$&$ 0.009  ^{+ 0.003  }_{ -0.002 }$&$ 0.13  ^{+ 0.36  }_{ -0.13 }$&$ 1.84  ^{+ 2.49  }_{ -1.83 }$&$ 2.17  \pm{ 0.79  }$&$ 84.61 ^{+ 0.88  }_{ -1.09 }$&$ 9.4   ^{+ 1.7   }_{ -1.9  }$&$ 0.101  \pm{ 0.004  }$&$ 1297  \pm{ 159   }$&$ 67    \pm{ 9     }$& 4.8   & 0.6  &0.018 & 0.319  \\
K03111.02  & 8581240    & 132.5113  &$    4.32854 ^{+    0.00010 }_{   -0.00014 }$&$ 1.00  ^{+  0.00}_{ -1.00 }$&$ 0.006  ^{+ 0.000  }_{ -0.001 }$&$ 0.90  ^{+ 0.00  }_{ -0.08 }$&$ 1.20  ^{+ 0.27  }_{ -0.40 }$&$ 1.54  \pm{ 0.45  }$&$ 62.05 ^{+ 27.57 }_{ -2.59 }$&$ 4.9   ^{+ 1.7   }_{ -1.1  }$&$ 0.055  \pm{ 0.002  }$&$ 1757  \pm{ 295   }$&$ 40    \pm{ 6     }$& 2.2   & 0.8  &0.003 & 0.068  \\
K03158.01  & 6278762    & 133.2591  &$    3.60011 ^{+    0.00003 }_{   -0.00003 }$&$ 0.21  ^{+ 0.33  }_{ -0.21 }$&$ 0.004  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.38  \pm{ 0.04  }$&$ 88.97 ^{+ 1.03  }_{ -1.91 }$&$ 11.7  ^{+ 0.8   }_{ -0.6  }$&$ 0.044  \pm{ 0.001  }$&$ 997   \pm{ 57	 }$&$ 27    \pm{ 1     }$& 2.3   & 2.6  &0.123 & 0.875 \\
K03158.02  & 6278762    & 131.5239  &$    4.54586 ^{+    0.00003 }_{   -0.00004 }$&$ 0.37  ^{+ 0.27  }_{ -0.30 }$&$ 0.006  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.49  \pm{ 0.06  }$&$ 88.44 ^{+ 1.26  }_{ -1.19 }$&$ 13.7  ^{+ 1.0   }_{ -0.7  }$&$ 0.051  \pm{ 0.001  }$&$ 917   \pm{ 47	 }$&$ 47    \pm{ 1     }$& 2.4   & \textbf{ 8.5  }  &0.243 & 0.941 \\
K03158.03  & 6278762    & 134.7885  &$    6.18936 ^{+    0.00007 }_{   -0.00008 }$&$ 0.40  ^{+ 0.27  }_{ -0.40 }$&$ 0.006  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 0.49  \pm{ 0.07  }$&$ 88.63 ^{+ 1.37  }_{ -1.32 }$&$ 16.9  ^{+ 0.9   }_{ -1.0  }$&$ 0.063  \pm{ 0.001  }$&$ 827   \pm{ 56	 }$&$ 45    \pm{ 1     }$& 2.6   & 0.7  &0.227 & 0.936 \\
K03158.04  & 6278762    & 135.0872  &$    7.74359 ^{+    0.00011 }_{   -0.00011 }$&$ 0.91  ^{+ 0.07  }_{ -0.05 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.05  ^{+ 0.17  }_{ -0.05 }$&$ 0.07  ^{+ 1.09  }_{ -0.07 }$&$ 1.84  \pm{ 0.32  }$&$ 83.71 ^{+ 0.86  }_{ -0.92 }$&$ 8.1   ^{+ 1.1   }_{ -1.0  }$&$ 0.080  \pm{ 0.004  }$&$ 1173  \pm{ 86	 }$&$ 51    \pm{ 1     }$& 3.1   & 2.1  &0.190 & 0.921 \\
K03158.05  & 6278762    & 134.8777  &$    9.74050 ^{+    0.00004 }_{   -0.00005 }$&$ 0.77  ^{+ 0.07  }_{ -0.15 }$&$ 0.009  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.06  ^{+ 1.53  }_{ -0.06 }$&$ 0.76  \pm{ 0.11  }$&$ 88.11 ^{+ 0.46  }_{ -0.36 }$&$ 23.0  ^{+ 1.7   }_{ -1.2  }$&$ 0.084  \pm{ 0.002  }$&$ 699   \pm{ 39	 }$&$ 74    \pm{ 1     }$& 2.1   & 1.1  &0.287 & 0.953 \\
K03196.01  & 9002538    & 135.3143  &$    4.96067 ^{+    0.00016 }_{   -0.00013 }$&$ 0.43  ^{+ 0.26  }_{ -0.40 }$&$ 0.004  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.27  ^{+ 2.36  }_{ -0.27 }$&$ 0.51  \pm{ 0.10  }$&$ 87.67 ^{+ 2.14  }_{ -1.58 }$&$ 10.7  ^{+ 0.7   }_{ -1.0  }$&$ 0.058  \pm{ 0.003  }$&$ 1316  \pm{ 126   }$&$ 23    \pm{ 3     }$& 3.2   & 0.8  &0.013 & 0.244 \\
K03196.02  & 9002538    & 134.1634  &$    6.88299 ^{+    0.00021 }_{   -0.00018 }$&$ 0.96  ^{+ 1.19  }_{ -0.30 }$&$ 0.009  ^{+ 0.025  }_{ -0.007 }$&$ 0.00  ^{+ 0.06  }_{ -0.01 }$&$ 0.48  ^{+  0.02 }_{ -0.42 }$&$ 1.14  \pm{ 2.03  }$&$ 80.65 ^{+ 1.86  }_{ -0.47 }$&$ 13.2  ^{+ 0.8   }_{ -1.7  }$&$ 0.072  \pm{ 0.004  }$&$ 1773  \pm{ 898   }$&$ 29    \pm{ 3     }$& 2.8   & 1.5  &0.018 & 0.320 \\
K03384.01  & 8644365    & 139.0648  &$   10.54837 ^{+    0.00018 }_{   -0.00013 }$&$ 0.79  ^{+ 0.15  }_{ -0.16 }$&$ 0.009  ^{+ 0.006  }_{ -0.002 }$&$ 0.10  ^{+ 0.37  }_{ -0.10 }$&$ 0.06  ^{+ 4.61  }_{ -0.06 }$&$ 1.10  \pm{ 0.51  }$&$ 87.61 ^{+ 0.64  }_{ -1.04 }$&$ 18.4  ^{+ 2.8   }_{ -2.1  }$&$ 0.094  \pm{ 0.004  }$&$ 930   \pm{ 125   }$&$ 82    \pm{ 11    }$& 2.7   & 1.3  &0.015 & 0.278 \\
K03384.02  & 8644365    & 139.3678  &$   19.91594 ^{+    0.00000 }_{   -0.04764 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.011  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.00  ^{+ 0.82  }_{ -0.00 }$&$ 1.41  \pm{ 0.25  }$&$ 90.00 ^{+  0.00 }_{ -1.15 }$&$ 27.2  ^{+ 2.3   }_{ -3.5  }$&$ 0.145  \pm{ 0.008  }$&$ 781   \pm{ 97	 }$&$ 150   \pm{ 16    }$& 5.6   & 0.9  &0.019 & 0.325 \\
K03398.01  & 3561464    & 137.2253  &$    7.31947 ^{+    0.00017 }_{   -0.00027 }$&$ 0.00  ^{+ 0.47  }_{ -0.00 }$&$ 0.012  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+  0.01 }_{ -0.00 }$&$ 1.51  \pm{ 0.28  }$&$ 90.00 ^{+ 0.00  }_{ -2.27 }$&$ 13.8  ^{+ 1.1   }_{ -2.1  }$&$ 0.074  \pm{ 0.004  }$&$ 1197  \pm{ 138   }$&$ 149   \pm{ 19    }$& 4.2   & 0.1  &0.013 & 0.395 \\
K03398.02  & 3561464    & 144.9642  &$   35.79896 ^{+    0.00005 }_{   -0.00004 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.022  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 2.79  \pm{ 0.55  }$&$ 90.00 ^{+ 0.00  }_{ -0.82 }$&$ 39.7  ^{+ 3.2   }_{ -5.7  }$&$ 0.213  \pm{ 0.013  }$&$ 688   \pm{ 86	 }$&$ 561   \pm{ 50    }$& 7.0   & 0.3  &0.029 & 0.595 \\
K03398.03  & 3561464    & 131.6023  &$    4.32702 ^{+    0.00014 }_{   -0.00015 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 1.23  \pm{ 0.25  }$&$ 90.00 ^{+ 0.00  }_{ -1.94 }$&$ 9.8   ^{+ 0.9   }_{ -1.3  }$&$ 0.052  \pm{ 0.003  }$&$ 1417  \pm{ 171   }$&$ 98    \pm{ 14    }$& 3.5   & 0.7  &0.003 & 0.135 \\
K03403.01  & 11754430   & 166.6626  &$   39.81811 ^{+    0.00058 }_{   -0.00064 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 1.73  \pm{ 0.36  }$&$ 90.00 ^{+ 0.00  }_{ -0.95 }$&$ 43.4  ^{+ 5.7   }_{ -7.2  }$&$ 0.229  \pm{ 0.012  }$&$ 635   \pm{ 97	 }$&$ 237   \pm{ 28    }$& 7.4   & 0.4  &0.032 & 0.455 \\
K03403.02  & 11754430   & 135.4936  &$    6.15844 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.89  \pm{ 0.19  }$&$ 90.00 ^{+ 0.00  }_{ -1.89 }$&$ 12.5  ^{+ 1.6   }_{ -1.6  }$&$ 0.066  \pm{ 0.003  }$&$ 1151  \pm{ 169   }$&$ 51    \pm{ 10    }$& 3.8   & 0.1  &0.007 & 0.155 \\
K03425.01  & 9117416    & 145.4378  &$   20.03515 ^{+    0.00078 }_{   -0.00063 }$&$ 0.26  ^{+ 0.43  }_{ -0.26 }$&$ 0.012  ^{+  0.000 }_{ -0.003 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 0.00  ^{+ 0.46  }_{ -0.00 }$&$ 1.12  \pm{ 0.45  }$&$ 89.52 ^{+ 0.48  }_{ -1.22 }$&$ 34.8  ^{+ 5.6   }_{ -12.1 }$&$ 0.139  \pm{ 0.008  }$&$ 625   \pm{ 137   }$&$ 121   \pm{ 18    }$& 4.8   & 0.1  &0.003 & 0.064 \\
K03425.02  & 9117416    & 131.6995  &$    3.15720 ^{+    0.00008 }_{   -0.00009 }$&$ 0.22  ^{+ 0.44  }_{ -0.22 }$&$ 0.007  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.02  ^{+ 0.26  }_{ -0.02 }$&$ 0.63  \pm{ 0.27  }$&$ 88.55 ^{+ 1.45  }_{ -3.43 }$&$ 10.2  ^{+ 1.6   }_{ -3.4  }$&$ 0.040  \pm{ 0.002  }$&$ 1168  \pm{ 249   }$&$ 59    \pm{ 7     }$& 2.7   & 0.5  &0.003 & 0.071 \\
K03500.01  & 6058816    & 188.5180  &$   73.75110 ^{+    0.00106 }_{   -0.00028 }$&$ 0.00  ^{+ 0.65  }_{ -0.00 }$&$ 0.015  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 1.98  \pm{ 0.50  }$&$ 90.00 ^{+ 0.00  }_{ -0.70 }$&$ 64.1  ^{+ 6.6   }_{ -15.9 }$&$ 0.348  \pm{ 0.018  }$&$ 557   \pm{ 101   }$&$ 251   \pm{ 34    }$& 10.4  & 0.2  &0.017 & 0.303 \\
K03500.02  & 6058816    & 135.8111  &$    4.74823 ^{+    0.00015 }_{   -0.00021 }$&$ 0.91  ^{+ 0.09  }_{ -0.45 }$&$ 0.006  ^{+ 0.003  }_{ -0.003 }$&$ 0.00  ^{+ 0.05  }_{ -0.01 }$&$ 0.10  ^{+ 0.22  }_{ -0.05 }$&$ 0.68  \pm{ 0.30  }$&$ 72.49 ^{+ 1.70  }_{ -0.29 }$&$ 10.6  ^{+ 1.6   }_{ -1.0  }$&$ 0.055  \pm{ 0.003  }$&$ 1507  \pm{ 364   }$&$ 36     \pm{ 8     }$& 5.2   & 0.3  &0.004 & 0.095 \\
K03681.01  & 2581316    & 238.8192  &$  217.83189 ^{+    0.00005 }_{   -0.00009 }$&$ 0.34  ^{+ 0.37  }_{ -0.05 }$&$ 0.089  ^{+ 0.003  }_{ -0.000 }$&$ 0.46  ^{+ 0.31  }_{ -0.46 }$&$ 0.00  ^{+ 1.63  }_{ -0.00 }$&$ 13.29 \pm{ 5.85  }$&$ 89.73 ^{+ 0.09  }_{ -0.35 }$&$ 114.6 ^{+ 13.5  }_{ -43.8 }$&$ 0.736  \pm{ 0.062  }$&$ 489   \pm{ 36	 }$&$ 9267  \pm{ 36    }$& 21.2  & 0.8  &0.910 & 0.996 \\
K03681.02  & 2581316    & 134.5660  &$   10.51420 ^{+    0.00034 }_{   -0.00035 }$&$ 0.08  ^{+ 0.55  }_{ -0.08 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.33  ^{+ 0.24  }_{ -0.30 }$&$ 2.09  ^{+ 1.88  }_{ -2.07 }$&$ 1.18  \pm{ 0.21  }$&$ 89.73 ^{+ 0.27  }_{ -2.11 }$&$ 16.1  ^{+ 1.2   }_{ -1.8  }$&$ 0.096  \pm{ 0.005  }$&$ 1036  \pm{ 76	 }$&$ 80    \pm{ 6     }$& 3.7   & 0.5  &0.005 & 0.107 \\
K03864.01  & 4164922    & 132.3795  &$    1.21073 ^{+    0.00001 }_{   -0.00001 }$&$ 0.88  ^{+ 0.04  }_{ -0.11 }$&$ 0.012  ^{+ 0.014  }_{ -0.001 }$&$ 0.08  ^{+ 0.53  }_{ -0.08 }$&$ 0.01  ^{+ 4.62  }_{ -0.01 }$&$ 2.98  \pm{ 1.90  }$&$ 69.47 ^{+ 4.30  }_{ -3.39 }$&$ 2.3   ^{+ 0.5   }_{ -0.3  }$&$ 0.023  \pm{ 0.001  }$&$ 2169  \pm{ 235   }$&$ 102   \pm{ 3     }$& 2.0   & 1.2  &0.175 & 0.841 \\
K03864.02  & 4164922    & 134.4413  &$   18.25734 ^{+    0.00093 }_{   -0.00089 }$&$ 0.09  ^{+ 0.52  }_{ -0.09 }$&$ 0.011  ^{+ 0.002  }_{ -0.001 }$&$ 0.03  ^{+ 0.21  }_{ -0.03 }$&$ 0.00  ^{+  2.01 }_{ -0.00 }$&$ 0.82  \pm{ 0.18  }$&$ 89.86 ^{+ 0.14  }_{ -0.92 }$&$ 37.6  ^{+ 4.0   }_{ -5.2  }$&$ 0.125  \pm{ 0.006  }$&$ 549   \pm{ 69	 }$&$ 159   \pm{ 15    }$& 3.8   & 0.6  &0.030 & 0.434 \\
K04021.01  & 11967788   & 133.1229  &$    7.23530 ^{+    0.00030 }_{   -0.00017 }$&$ 0.47  ^{+ 0.11  }_{ -0.47 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.00  ^{+ 0.63  }_{ -0.00 }$&$ 1.22  \pm{ 0.23  }$&$ 87.89 ^{+ 2.11  }_{ -0.65 }$&$ 12.6  ^{+ 0.9   }_{ -1.1  }$&$ 0.074  \pm{ 0.004  }$&$ 1198  \pm{ 91	 }$&$ 113   \pm{ 8     }$& 3.8   & 1.8  &0.119 & 0.772 \\
K04021.02  & 11967788   & 132.4534  &$    4.93209 ^{+    0.00000 }_{    0.00000 }$&$ 0.22  ^{+ 0.24  }_{ -0.22 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.08  ^{+ 0.22  }_{ -0.08 }$&$ 1.02  \pm{ 0.16  }$&$ 88.71 ^{+ 1.29  }_{ -1.44 }$&$ 9.8   ^{+ 0.6   }_{ -1.0  }$&$ 0.057  \pm{ 0.003  }$&$ 1365  \pm{ 87	 }$&$ 67    \pm{ 7     }$& 3.8   & 1.8  &0.050 & 0.570 \\
K04032.01  & 7100673    & 134.2139  &$    3.95125 ^{+    0.00000 }_{   -0.00000 }$&$ 0.43  ^{+ 0.28  }_{ -0.43 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.41  }_{ -0.00 }$&$ 0.01  ^{+ 0.42  }_{ -0.01 }$&$ 0.85  \pm{ 0.21  }$&$ 87.45 ^{+ 2.55  }_{ -2.72 }$&$ 9.6   ^{+ 2.0   }_{ -1.3  }$&$ 0.049  \pm{ 0.002  }$&$ 1260  \pm{ 201   }$&$ 72    \pm{ 5     }$& 2.8   & 0.3  &0.026 & 0.403 \\
K04032.02  & 7100673    & 132.8557  &$    2.89225 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.06  }_{ -0.05 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.13  }_{ -0.01 }$&$ 0.12  ^{+ 1.14  }_{ -0.12 }$&$ 2.26  \pm{ 0.31  }$&$ 75.29 ^{+ 1.39  }_{ -0.75 }$&$ 3.6   ^{+ 0.4   }_{ -0.2  }$&$ 0.042  \pm{ 0.003  }$&$ 1885  \pm{ 181   }$&$ 39    \pm{ 4     }$& 2.7   & 1.4  &0.019 & 0.330 \\
K04097.01  & 5688683    & 133.1487  &$    2.79068 ^{+    0.00002 }_{   -0.00003 }$&$ 1.03  ^{+ 0.01  }_{ -0.06 }$&$ 0.068  ^{+  0.010 }_{ -0.041 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.73 \pm{ 0.22  }$&$ 75.55 ^{+ 2.20  }_{ -5.09 }$&$ 4.0   ^{+ 0.4   }_{ -0.9  }$&$ 0.040  \pm{ 0.002  }$&$ 1543  \pm{ 197   }$&$ 170   \pm{ 7     }$& 1.4   & 0.3  &0.083 & 0.693 \\
K04097.02  & 5688683    & 131.7418  &$    4.44911 ^{+    0.00010 }_{   -0.00008 }$&$ 0.48  ^{+ 0.22  }_{ -0.40 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.03  ^{+ 0.21  }_{ -0.03 }$&$ 1.28  ^{+ 3.42  }_{ -1.28 }$&$ 0.51  \pm{ 0.09  }$&$ 88.41 ^{+ 1.34  }_{ -0.89 }$&$ 17.3  ^{+ 0.8   }_{ -1.2  }$&$ 0.045  \pm{ 0.002  }$&$ 681   \pm{ 77	 }$&$ 82    \pm{ 9     }$& 1.7   & 1.0  &0.012 & 0.228 \\
K04269.01  & 8890924    & 131.5999  &$   26.65626 ^{+    0.00101 }_{   -0.00098 }$&$ 0.00  ^{+ 0.56  }_{ -0.00 }$&$ 0.012  ^{+ 0.002  }_{ -0.001 }$&$ 0.13  ^{+ 0.41  }_{ -0.13 }$&$ 0.04  ^{+ 0.28  }_{ -0.04 }$&$ 1.00  \pm{ 0.28  }$&$ 90.00 ^{+ 0.00  }_{ -0.97 }$&$ 45.4  ^{+ 5.1   }_{ -10.6 }$&$ 0.165  \pm{ 0.008  }$&$ 538   \pm{ 95	 }$&$ 194   \pm{ 24    }$& 5.0   & 0.4  &0.047 & 0.549 \\
K04269.02  & 8890924    & 135.2750  &$    4.44061 ^{+    0.00016 }_{   -0.00019 }$&$ 0.50  ^{+ 0.97  }_{ -0.04 }$&$ 0.006  ^{+ 0.012  }_{ -0.004 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.09  ^{+ 0.26  }_{ -0.09 }$&$ 0.51  \pm{ 0.70  }$&$ 84.28 ^{+ 1.50  }_{ -0.17 }$&$ 13.5  ^{+ 2.0   }_{ -2.6  }$&$ 0.050  \pm{ 0.003  }$&$ 1526  \pm{ 835   }$&$ 35    \pm{ 10    }$& 5.9   & 0.3  &0.019 & 0.326 \\
K04288.01  & 4548011    & 133.1927  &$    6.28402 ^{+    0.00020 }_{   -0.00028 }$&$ 0.00  ^{+ 0.34  }_{ -0.00 }$&$ 0.005  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.70  \pm{ 0.15  }$&$ 90.00 ^{+ 0.00  }_{ -1.59 }$&$ 12.6  ^{+ 0.9   }_{ -1.5  }$&$ 0.067  \pm{ 0.004  }$&$ 1180  \pm{ 146   }$&$ 37    \pm{ 5     }$& 3.8   & 0.7  &0.003 & 0.078 \\
K04288.02  & 4548011    & 139.9708  &$    9.08764 ^{+    0.00031 }_{   -0.00029 }$&$ 0.46  ^{+ 0.32  }_{ -0.46 }$&$ 0.005  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.51  }_{ -0.01 }$&$ 0.19  ^{+ 1.88  }_{ -0.19 }$&$ 0.69  \pm{ 0.15  }$&$ 88.34 ^{+ 1.66  }_{ -1.57 }$&$ 16.0  ^{+ 1.1   }_{ -2.0  }$&$ 0.086  \pm{ 0.004  }$&$ 1051  \pm{ 124   }$&$ 43    \pm{ 6     }$& 3.9   & 0.9  &0.003 & 0.072 \\

\enddata


\tablecomments{The last three columns are significance of pixel centroid offset between in- and out-of-transit, planet confidence before and after considering the planetary likelihood boost in~\citet{Lissauer2012}. Planet candidates with significant pixel centroid offset ($> 3\sigma$) and planet candidates with higher than 0.997 planet confidence are marked in bold.}


\end{deluxetable}

\clearpage
 \end{landscape}


==> orbital_params.tex.20131004.tex <==


\clearpage
%\LongTables

\begin{landscape}
\begin{deluxetable}{lccccccccccccccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\setlength{\tabcolsep}{0.02in}
%\tablenum{1}
\tablecaption{Orbital Parameters\label{tab:orbital_params}}
\tablehead{
\colhead{\textbf{KOI}} &
\colhead{\textbf{KIC}} &
\colhead{\textbf{$T_0$}} &
\colhead{\textbf{Period}} &
\colhead{\textbf{Impact}} &
\colhead{\textbf{R$_{\rm PL}$/R$_{\ast}$}} &
\colhead{\textbf{e}} &
\colhead{\textbf{$\omega$}} &
\colhead{\textbf{R$_{\rm PL}$}} &
\colhead{\textbf{Inclination}} &
\colhead{\textbf{a/R$_{\ast}$}} &
\colhead{\textbf{a}} &
\colhead{\textbf{$T_{\rm PL}$}} &
\colhead{\textbf{Depth}} &
\colhead{\textbf{Dur}} &
\colhead{\textbf{Sig}} &
\colhead{\textbf{p1}} &
\colhead{\textbf{p2}} \\

\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(BKJD)}} &
\colhead{\textbf{(d)}} &
\colhead{\textbf{Parameter}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(radian)}} &
\colhead{\textbf{(R$_{\oplus}$)}} &
\colhead{\textbf{($\deg$)}} &
\colhead{\textbf{}} &
\colhead{\textbf{(AU)}} &
\colhead{\textbf{(K)}} &
\colhead{\textbf{(ppm)}} &
\colhead{\textbf{(hr)}} &
\colhead{\textbf{($\sigma$)}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} 

}

\startdata

K00005.01  & 8554498    & 132.9733  &$    4.78033 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.00  }_{ -0.00 }$&$ 0.040  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 8.98  \pm{ 0.52  }$&$ 81.18 ^{+ 0.32  }_{ -0.22 }$&$ 6.2   ^{+ 0.1   }_{ -0.2  }$&$ 0.059  \pm{ 0.002  }$&$ 1548  \pm{ 23    }$&$ 987   \pm{ 3     }$& 2.2   & 5.1  &0.932 & 0.997 \\
K00005.02  & 8554498    & 133.3670  &$    7.05186 ^{+    0.00000 }_{   -0.00000 }$&$ 0.68  ^{+ 0.14  }_{ -0.68 }$&$ 0.004  ^{+ 0.044  }_{ -0.001 }$&$ 0.70  ^{+ -0.00 }_{ -0.47 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.93  \pm{ 4.80  }$&$ 85.78 ^{+ 4.22  }_{ -1.10 }$&$ 8.2   ^{+ 0.9   }_{ -0.4  }$&$ 0.077  \pm{ 0.003  }$&$ 1280  \pm{ 199   }$&$ 22    \pm{ 4     }$& 3.9   & 0.4  &0.005 & 0.102 \\
K00041.01  & 6521045    & 122.9506  &$   12.81574 ^{+    0.00000 }_{   -0.00000 }$&$ 0.80  ^{+ 0.07  }_{ -0.08 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.68  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.89  \pm{ 0.74  }$&$ 85.21 ^{+ 1.06  }_{ -1.38 }$&$ 9.4   ^{+ 0.9   }_{ -1.7  }$&$ 0.115  \pm{ 0.005  }$&$ 1270  \pm{ 91    }$&$ 214   \pm{ 5     }$& 6.5   & 1.5  &0.615 & 0.988 \\
K00041.02  & 6521045    & 133.1758  &$    6.88710 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.10  }_{ -0.03 }$&$ 0.009  ^{+ 0.002  }_{ -0.000 }$&$ 0.02  ^{+ 0.48  }_{ -0.02 }$&$ 0.94  ^{+ 5.35  }_{ -0.94 }$&$ 2.65  \pm{ 0.43  }$&$ 81.01 ^{+ 1.62  }_{ -2.19 }$&$ 5.8   ^{+ 0.3   }_{ -1.9  }$&$ 0.074  \pm{ 0.003  }$&$ 1631  \pm{ 89    }$&$ 71    \pm{ 4     }$& 4.5   & 0.3  &0.063 & 0.769 \\
K00041.03  & 6521045    & 153.9839  &$   35.33314 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.02  }_{ -0.07 }$&$ 0.011  ^{+ 0.001  }_{ -0.003 }$&$ 0.01  ^{+ 0.35  }_{ -0.01 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.03  \pm{ 0.68  }$&$ 87.01 ^{+ 2.99  }_{ -0.61 }$&$ 18.3  ^{+ 1.6   }_{ -2.8  }$&$ 0.223  \pm{ 0.013  }$&$ 933   \pm{ 68    }$&$ 93    \pm{ 10    }$& 6.2   & 1.0  &0.053 & 0.736 \\
K00070.01  & 6850504    & 138.6075  &$   10.85409 ^{+    0.00000 }_{   -0.00000 }$&$ 0.57  ^{+ 0.25  }_{ -0.08 }$&$ 0.035  ^{+ 0.000  }_{ -0.005 }$&$ 0.59  ^{+ 0.11  }_{ -0.59 }$&$ 4.52  ^{+ 1.74  }_{ -4.49 }$&$ 3.65  \pm{ 0.44  }$&$ 88.39 ^{+ 0.27  }_{ -1.35 }$&$ 20.2  ^{+ 1.0   }_{ -2.0  }$&$ 0.093  \pm{ 0.002  }$&$ 800   \pm{ 26    }$&$ 1043  \pm{ 9     }$& 4.2   & 0.5  &0.959 & 0.999 \\
K00070.02  & 6850504    & 134.5009  &$    3.69612 ^{+    0.00000 }_{   -0.00000 }$&$ 0.44  ^{+ 0.14  }_{ -0.44 }$&$ 0.018  ^{+ 0.004  }_{ -0.000 }$&$ 0.02  ^{+ 0.53  }_{ -0.02 }$&$ 0.14  ^{+ 4.57  }_{ -0.14 }$&$ 1.79  \pm{ 0.29  }$&$ 87.51 ^{+ 2.29  }_{ -0.93 }$&$ 10.0  ^{+ 0.6   }_{ -2.3  }$&$ 0.044  \pm{ 0.002  }$&$ 1133  \pm{ 49    }$&$ 376   \pm{ 4     }$& 2.5   & 1.7  &0.821 & 0.996 \\
K00070.03  & 6850504    & 164.7276  &$   77.61153 ^{+    0.00000 }_{   -0.00000 }$&$ 0.36  ^{+ 0.20  }_{ -0.36 }$&$ 0.027  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.71  \pm{ 0.24  }$&$ 89.74 ^{+ 0.20  }_{ -0.11 }$&$ 75.1  ^{+ 4.3   }_{ -15.3 }$&$ 0.338  \pm{ 0.013  }$&$ 408   \pm{ 12    }$&$ 885   \pm{ 31    }$& 7.2   & 0.5  &0.539 & 0.983 \\
K00070.04  & 6850504    & 135.9338  &$    6.09850 ^{+    0.00000 }_{   -0.00000 }$&$ 0.43  ^{+ 0.18  }_{ -0.43 }$&$ 0.008  ^{+ 0.002  }_{ -0.000 }$&$ 0.17  ^{+ 0.50  }_{ -0.17 }$&$ 0.13  ^{+ 5.90  }_{ -0.13 }$&$ 0.78  \pm{ 0.14  }$&$ 88.29 ^{+ 1.71  }_{ -0.76 }$&$ 14.4  ^{+ 0.9   }_{ -1.0  }$&$ 0.062  \pm{ 0.003  }$&$ 945   \pm{ 48    }$&$ 71    \pm{ 6     }$& 2.8   & 0.3  &0.029 & 0.596 \\
K00070.05  & 6850504    & 135.2142  &$   19.57709 ^{+    0.00000 }_{   -0.00000 }$&$ 0.68  ^{+ 0.11  }_{ -0.23 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.27  }_{ -0.00 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 1.00  \pm{ 0.11  }$&$ 88.74 ^{+ 0.39  }_{ -0.29 }$&$ 30.1  ^{+ 1.8   }_{ -7.9  }$&$ 0.136  \pm{ 0.004  }$&$ 646   \pm{ 32    }$&$ 98    \pm{ 13    }$& 3.6   & 1.5  &0.012 & 0.383 \\
K00072.01  & 11904151   & 131.5744  &$    0.83749 ^{+    0.00000 }_{   -0.00000 }$&$ 0.19  ^{+ 0.14  }_{ -0.19 }$&$ 0.012  ^{+ 0.000  }_{ -0.001 }$&$ 0.01  ^{+ 0.41  }_{ -0.01 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.33  \pm{ 0.11  }$&$ 87.00 ^{+ 3.00  }_{ -2.29 }$&$ 3.6   ^{+ 0.1   }_{ -0.4  }$&$ 0.017  \pm{ 0.000  }$&$ 1958  \pm{ 54    }$&$ 175   \pm{ 1     }$& 1.8   & 5.5  &0.936 & 0.997 \\
K00072.02  & 11904151   & 138.6781  &$   45.29404 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.020  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 2.06  \pm{ 0.28  }$&$ 90.00 ^{+ -0.00 }_{ -0.04 }$&$ 48.4  ^{+ 4.2   }_{ -3.8  }$&$ 0.236  \pm{ 0.006  }$&$ 520   \pm{ 18    }$&$ 490   \pm{ 13    }$& 6.8   & 0.6  &0.774 & 0.988 \\
K00082.01  & 10187017   & 134.7534  &$   16.14569 ^{+    0.00000 }_{   -0.00000 }$&$ 0.56  ^{+ 0.05  }_{ -0.15 }$&$ 0.035  ^{+ 0.000  }_{ -0.007 }$&$ 0.63  ^{+ 0.06  }_{ -0.63 }$&$ 4.61  ^{+ 0.38  }_{ -4.61 }$&$ 2.98  \pm{ 0.36  }$&$ 89.00 ^{+ 0.21  }_{ -0.13 }$&$ 32.0  ^{+ 0.4   }_{ -1.3  }$&$ 0.118  \pm{ 0.001  }$&$ 574   \pm{ 15    }$&$ 956   \pm{ 7     }$& 4.0   & 1.1  &0.974 & 0.999 \\
K00082.02  & 10187017   & 134.0798  &$   10.31173 ^{+    0.00000 }_{   -0.00000 }$&$ 0.34  ^{+ 0.09  }_{ -0.34 }$&$ 0.015  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 1.27  \pm{ 0.12  }$&$ 89.17 ^{+ 0.83  }_{ -0.24 }$&$ 23.3  ^{+ 0.4   }_{ -2.3  }$&$ 0.088  \pm{ 0.001  }$&$ 671   \pm{ 11    }$&$ 271   \pm{ 5     }$& 3.2   & 0.5  &0.636 & 0.989 \\
K00082.03  & 10187017   & 145.0258  &$   27.45362 ^{+    0.00000 }_{   -0.00000 }$&$ 0.58  ^{+ 0.06  }_{ -0.58 }$&$ 0.011  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.96  \pm{ 0.05  }$&$ 89.27 ^{+ 0.73  }_{ -0.09 }$&$ 45.1  ^{+ 0.9   }_{ -1.8  }$&$ 0.168  \pm{ 0.002  }$&$ 483   \pm{ 8     }$&$ 141   \pm{ 9     }$& 3.8   & 0.7  &0.056 & 0.748 \\
K00082.04  & 10187017   & 139.9875  &$    7.07134 ^{+    0.00000 }_{   -0.00000 }$&$ 0.40  ^{+ 0.15  }_{ -0.31 }$&$ 0.008  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.19  }_{ -0.00 }$&$ 0.00  ^{+ 1.38  }_{ -0.00 }$&$ 0.66  \pm{ 0.05  }$&$ 88.76 ^{+ 0.83  }_{ -0.47 }$&$ 18.2  ^{+ 0.4   }_{ -1.9  }$&$ 0.068  \pm{ 0.001  }$&$ 758   \pm{ 12    }$&$ 72    \pm{ 4     }$& 2.7   & 0.6  &0.058 & 0.754 \\
K00082.05  & 10187017   & 135.8466  &$    5.28698 ^{+    0.00000 }_{   -0.00000 }$&$ 0.36  ^{+ 0.13  }_{ -0.36 }$&$ 0.006  ^{+ 0.002  }_{ -0.000 }$&$ 0.02  ^{+ 0.41  }_{ -0.02 }$&$ 0.01  ^{+ 0.88  }_{ -0.01 }$&$ 0.49  \pm{ 0.11  }$&$ 88.66 ^{+ 1.33  }_{ -0.50 }$&$ 15.2  ^{+ 0.3   }_{ -0.3  }$&$ 0.056  \pm{ 0.001  }$&$ 834   \pm{ 12    }$&$ 39    \pm{ 4     }$& 2.5   & 0.6  &0.027 & 0.577 \\
K00085.01  & 5866724    & 132.0395  &$    5.85993 ^{+    0.00000 }_{   -0.00000 }$&$ 0.48  ^{+ 0.10  }_{ -0.35 }$&$ 0.017  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 2.65  \pm{ 0.16  }$&$ 87.29 ^{+ 1.74  }_{ -0.81 }$&$ 10.2  ^{+ 0.1   }_{ -1.9  }$&$ 0.070  \pm{ 0.001  }$&$ 1289  \pm{ 53    }$&$ 316   \pm{ 3     }$& 4.0   & 5.2  &0.939 & 0.999 \\
K00085.02  & 5866724    & 133.4963  &$    2.15492 ^{+    0.00000 }_{   -0.00000 }$&$ 0.41  ^{+ 0.15  }_{ -0.26 }$&$ 0.009  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 1.44  \pm{ 0.12  }$&$ 85.13 ^{+ 3.07  }_{ -1.98 }$&$ 5.2   ^{+ 0.2   }_{ -0.8  }$&$ 0.036  \pm{ 0.001  }$&$ 1857  \pm{ 70    }$&$ 93    \pm{ 2     }$& 3.1   & 3.7  &0.657 & 0.990 \\
K00085.03  & 5866724    & 137.9953  &$    8.13115 ^{+    0.00000 }_{   -0.00000 }$&$ 0.41  ^{+ 0.26  }_{ -0.41 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.39  ^{+ 0.23  }_{ -0.39 }$&$ 0.18  ^{+ 6.02  }_{ -0.18 }$&$ 1.57  \pm{ 0.19  }$&$ 88.05 ^{+ 1.95  }_{ -1.40 }$&$ 12.8  ^{+ 1.4   }_{ -1.5  }$&$ 0.086  \pm{ 0.003  }$&$ 1175  \pm{ 49    }$&$ 109   \pm{ 4     }$& 4.2   & 1.6  &0.379 & 0.968 \\
K00089.01  & 8056665    & 150.5651  &$   84.68895 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.08  }_{ -0.02 }$&$ 0.021  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 8.21  \pm{ 1.57  }$&$ 88.03 ^{+ 0.24  }_{ -0.87 }$&$ 26.9  ^{+ 1.5   }_{ -2.2  }$&$ 0.482  \pm{ 0.015  }$&$ 977   \pm{ 73    }$&$ 354   \pm{ 17    }$& 10.7  & 0.7  &0.008 & 0.170 \\
K00089.02  & 8056665    & 289.8688  &$  207.60349 ^{+    0.00000 }_{   -0.00000 }$&$ 1.84  ^{+ -0.84 }_{ -0.85 }$&$ 0.026  ^{+ 0.002  }_{ -0.003 }$&$ 0.48  ^{+ 0.22  }_{ -0.48 }$&$ 1.57  ^{+ 4.72  }_{ -1.54 }$&$ 10.76 \pm{ 1.14  }$&$ 87.75 ^{+ 0.93  }_{ -1.16 }$&$ 48.6  ^{+ 2.4   }_{ -2.9  }$&$ 0.873  \pm{ 0.028  }$&$ 732   \pm{ 43    }$&$ 508   \pm{ 36    }$& 7.8   & 0.6  &0.021 & 0.345 \\
K00094.01  & 6462863    & 132.7405  &$   22.34300 ^{+    0.00000 }_{   -0.00000 }$&$ 0.65  ^{+ 0.05  }_{ -0.20 }$&$ 0.072  ^{+ 0.001  }_{ -0.003 }$&$ 0.26  ^{+ 0.34  }_{ -0.21 }$&$ 0.11  ^{+ 1.23  }_{ -0.11 }$&$ 14.64 \pm{ 1.54  }$&$ 88.19 ^{+ 0.76  }_{ -0.25 }$&$ 19.3  ^{+ 1.1   }_{ -1.0  }$&$ 0.172  \pm{ 0.004  }$&$ 893   \pm{ 58    }$&$ 5700  \pm{ 17    }$& 6.9   & 13.6 &0.978 & 1.000 \\
K00094.02  & 6462863    & 138.0072  &$   10.42371 ^{+    0.00000 }_{   -0.00000 }$&$ 0.54  ^{+ 0.12  }_{ -0.27 }$&$ 0.026  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 4.15  \pm{ 0.77  }$&$ 87.66 ^{+ 1.21  }_{ -0.88 }$&$ 11.8  ^{+ 1.3   }_{ -0.7  }$&$ 0.101  \pm{ 0.002  }$&$ 1124  \pm{ 69    }$&$ 781   \pm{ 11    }$& 5.2   & 3.0  &0.246 & 0.942 \\
K00094.03  & 6462863    & 161.2400  &$   54.31993 ^{+    0.00000 }_{   -0.00000 }$&$ 0.61  ^{+ 0.12  }_{ -0.48 }$&$ 0.048  ^{+ 0.000  }_{ -0.004 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.01  ^{+ 4.74  }_{ -0.01 }$&$ 6.37  \pm{ 0.76  }$&$ 89.16 ^{+ 0.61  }_{ -0.32 }$&$ 51.3  ^{+ 3.3   }_{ -7.3  }$&$ 0.291  \pm{ 0.008  }$&$ 636   \pm{ 63    }$&$ 2524  \pm{ 63    }$& 8.5   & 3.7  &0.463 & 0.977 \\
K00094.04  & 6462863    & 131.6139  &$    3.74324 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 1.28  \pm{ 0.17  }$&$ 90.00 ^{+ -0.00 }_{ -0.52 }$&$ 8.7   ^{+ 0.6   }_{ -0.5  }$&$ 0.049  \pm{ 0.001  }$&$ 1446  \pm{ 118   }$&$ 117   \pm{ 6     }$& 3.6   & 1.7  &0.076 & 0.804 \\
K00102.01  & 8456679    & 135.0591  &$    1.73514 ^{+    0.00000 }_{   -0.00000 }$&$ 0.56  ^{+ 0.03  }_{ -0.02 }$&$ 0.035  ^{+ 0.000  }_{ -0.000 }$&$ 0.66  ^{+ 0.02  }_{ -0.12 }$&$ 4.66  ^{+ 0.06  }_{ -0.32 }$&$ 4.85  \pm{ 0.32  }$&$ 83.46 ^{+ 0.48  }_{ -0.73 }$&$ 4.9   ^{+ 0.1   }_{ -0.5  }$&$ 0.030  \pm{ 0.000  }$&$ 1731  \pm{ 54    }$&$ 937   \pm{ 3     }$& 2.7   & 27.2 &0.906 & 0.996 \\
K00102.02  & 8456679    & 132.2635  &$    4.06853 ^{+    0.00000 }_{   -0.00000 }$&$ 0.50  ^{+ 0.19  }_{ -0.50 }$&$ 0.008  ^{+ 0.046  }_{ -0.001 }$&$ 0.37  ^{+ 0.33  }_{ -0.36 }$&$ 0.01  ^{+ 0.43  }_{ -0.01 }$&$ 0.89  \pm{ 2.53  }$&$ 87.38 ^{+ 2.61  }_{ -1.30 }$&$ 10.4  ^{+ 0.9   }_{ -2.1  }$&$ 0.050  \pm{ 0.002  }$&$ 1170  \pm{ 59    }$&$ 78    \pm{ 7     }$& 2.4   & 2.6  &0.004 & 0.085 \\
K00108.01  & 4914423    & 142.1763  &$   15.96535 ^{+    0.00000 }_{   -0.00000 }$&$ 0.43  ^{+ 0.12  }_{ -0.43 }$&$ 0.020  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.44  \pm{ 0.22  }$&$ 89.00 ^{+ 0.94  }_{ -0.36 }$&$ 24.1  ^{+ 1.0   }_{ -6.0  }$&$ 0.127  \pm{ 0.003  }$&$ 799   \pm{ 28    }$&$ 483   \pm{ 8     }$& 4.6   & 0.3  &0.718 & 0.985 \\
K00108.02  & 4914423    & 295.3304  &$  179.60101 ^{+    0.00000 }_{   -0.00000 }$&$ 0.17  ^{+ 0.40  }_{ -0.17 }$&$ 0.033  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 4.21  }_{ -0.00 }$&$ 4.21  \pm{ 0.49  }$&$ 89.91 ^{+ 0.09  }_{ -0.16 }$&$ 118.3 ^{+ 11.3  }_{ -10.0 }$&$ 0.648  \pm{ 0.016  }$&$ 384   \pm{ 31    }$&$ 1265  \pm{ 32    }$& 13.1  & 0.8  &0.163 & 0.830 \\
K00111.01  & 6678383    & 137.6139  &$   11.42751 ^{+    0.00000 }_{   -0.00000 }$&$ 0.32  ^{+ 0.21  }_{ -0.32 }$&$ 0.021  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.30  }_{ -0.00 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 1.78  \pm{ 0.21  }$&$ 89.02 ^{+ 0.98  }_{ -0.51 }$&$ 24.0  ^{+ 1.1   }_{ -4.4  }$&$ 0.089  \pm{ 0.002  }$&$ 873   \pm{ 109   }$&$ 495   \pm{ 8     }$& 4.5   & 1.8  &0.738 & 0.993 \\
K00111.02  & 6678383    & 132.7129  &$   23.66834 ^{+    0.00000 }_{   -0.00000 }$&$ 0.18  ^{+ 0.11  }_{ -0.18 }$&$ 0.020  ^{+ 0.004  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.20  \pm{ 0.22  }$&$ 89.68 ^{+ 0.32  }_{ -0.16 }$&$ 31.7  ^{+ 0.7   }_{ -3.7  }$&$ 0.151  \pm{ 0.004  }$&$ 670   \pm{ 11    }$&$ 463   \pm{ 11    }$& 5.6   & 1.1  &0.514 & 0.981 \\
K00111.03  & 6678383    & 271.0832  &$   51.75627 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.023  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 5.11  }_{ -0.00 }$&$ 2.29  \pm{ 0.19  }$&$ 90.00 ^{+ -0.00 }_{ -0.30 }$&$ 58.5  ^{+ 2.6   }_{ -5.2  }$&$ 0.254  \pm{ 0.005  }$&$ 501   \pm{ 15    }$&$ 611   \pm{ 19    }$& 7.0   & 0.3  &0.480 & 0.979 \\
K00112.01  & 10984090   & 185.1795  &$   51.07931 ^{+    0.00000 }_{   -0.00000 }$&$ 0.27  ^{+ 0.22  }_{ -0.27 }$&$ 0.025  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.55  \pm{ 0.25  }$&$ 89.74 ^{+ 0.22  }_{ -0.19 }$&$ 59.7  ^{+ 3.0   }_{ -4.6  }$&$ 0.265  \pm{ 0.012  }$&$ 499   \pm{ 17    }$&$ 745   \pm{ 19    }$& 6.4   & 0.4  &0.481 & 0.959 \\
K00112.02  & 10984090   & 133.9857  &$    3.70919 ^{+    0.00000 }_{   -0.00000 }$&$ 0.27  ^{+ 0.22  }_{ -0.27 }$&$ 0.011  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.95  \pm{ 0.12  }$&$ 88.57 ^{+ 1.43  }_{ -1.13 }$&$ 11.3  ^{+ 1.2   }_{ -0.8  }$&$ 0.045  \pm{ 0.002  }$&$ 1182  \pm{ 50    }$&$ 131   \pm{ 5     }$& 2.6   & 0.9  &0.064 & 0.632 \\
K00115.01  & 9579641    & 133.1424  &$    5.41220 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.06  }_{ -0.01 }$&$ 0.027  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.04  ^{+ 3.36  }_{ -0.04 }$&$ 7.66  \pm{ 0.82  }$&$ 80.05 ^{+ 1.37  }_{ -3.28 }$&$ 5.0   ^{+ 0.4   }_{ -1.3  }$&$ 0.064  \pm{ 0.002  }$&$ 1809  \pm{ 113   }$&$ 587   \pm{ 6     }$& 3.3   & 2.8  &0.914 & 0.998 \\
K00115.02  & 9579641    & 139.0032  &$    7.12597 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.02  }_{ -0.16 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.26  }_{ -0.01 }$&$ 0.17  ^{+ 1.73  }_{ -0.17 }$&$ 4.40  \pm{ 1.45  }$&$ 81.71 ^{+ 5.13  }_{ -2.51 }$&$ 5.4   ^{+ 0.7   }_{ -0.8  }$&$ 0.079  \pm{ 0.004  }$&$ 1646  \pm{ 492   }$&$ 185   \pm{ 7     }$& 3.1   & 0.7  &0.309 & 0.957 \\
K00115.03  & 9579641    & 132.6570  &$    3.43584 ^{+    0.00000 }_{   -0.00000 }$&$ 1.07  ^{+ -0.07 }_{ -0.26 }$&$ 0.004  ^{+ 0.001  }_{ -0.002 }$&$ 0.68  ^{+ 0.02  }_{ -0.16 }$&$ 2.73  ^{+ 0.69  }_{ -1.56 }$&$ 1.14  \pm{ 0.45  }$&$ 75.96 ^{+ 14.04 }_{ -11.31 }$&$ 3.8   ^{+ 0.3   }_{ -0.3  }$&$ 0.048  \pm{ 0.002  }$&$ 2009  \pm{ 687   }$&$ 16    \pm{ 5     }$& 3.2   & 0.8  &0.010 & 0.327 \\
K00116.01  & 8395660    & 136.2799  &$   13.57100 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.01  }_{ -0.17 }$&$ 0.025  ^{+ 0.000  }_{ -0.004 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 5.86  \pm{ 0.65  }$&$ 85.60 ^{+ 1.21  }_{ -0.41 }$&$ 11.9  ^{+ 0.2   }_{ -0.6  }$&$ 0.113  \pm{ 0.006  }$&$ 1100  \pm{ 99    }$&$ 496   \pm{ 13    }$& 3.6   & 0.6  &0.187 & 0.920 \\
K00116.02  & 8395660    & 151.9344  &$   43.84445 ^{+    0.00000 }_{   -0.00000 }$&$ 0.37  ^{+ 0.48  }_{ -0.37 }$&$ 0.023  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.47  \pm{ 0.37  }$&$ 89.57 ^{+ 0.28  }_{ -1.09 }$&$ 48.2  ^{+ 2.7   }_{ -24.1 }$&$ 0.239  \pm{ 0.012  }$&$ 557   \pm{ 64    }$&$ 638   \pm{ 23    }$& 6.4   & 0.7  &0.092 & 0.834 \\
K00116.03  & 8395660    & 135.6340  &$    6.16500 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.05  }_{ -0.06 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.37  ^{+ 0.33  }_{ -0.35 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.79  \pm{ 0.20  }$&$ 83.03 ^{+ 4.68  }_{ -0.86 }$&$ 6.7   ^{+ 5.6   }_{ -0.0  }$&$ 0.063  \pm{ 0.003  }$&$ 1385  \pm{ 359   }$&$ 53    \pm{ 9     }$& 3.4   & 0.8  &0.002 & 0.098 \\
K00116.04  & 8395660    & 147.5282  &$   23.98000 ^{+    0.00000 }_{   -0.00000 }$&$ 0.39  ^{+ 0.26  }_{ -0.39 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.01  ^{+ 0.47  }_{ -0.01 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.98  \pm{ 0.18  }$&$ 89.35 ^{+ 0.65  }_{ -0.68 }$&$ 35.1  ^{+ 3.4   }_{ -3.1  }$&$ 0.156  \pm{ 0.007  }$&$ 667   \pm{ 84    }$&$ 103   \pm{ 17    }$& 5.0   & 0.4  &0.002 & 0.075 \\
K00117.01  & 10875245   & 138.7788  &$   14.74910 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.05  }_{ -0.02 }$&$ 0.023  ^{+ 0.000  }_{ -0.001 }$&$ 0.02  ^{+ 0.65  }_{ -0.02 }$&$ 1.42  ^{+ 4.87  }_{ -1.42 }$&$ 9.89  \pm{ 1.70  }$&$ 82.40 ^{+ 0.84  }_{ -2.31 }$&$ 7.1   ^{+ 0.5   }_{ -1.4  }$&$ 0.145  \pm{ 0.007  }$&$ 1481  \pm{ 80    }$&$ 421   \pm{ 11    }$& 6.8   & 0.6  &0.339 & 0.962 \\
K00117.02  & 10875245   & 138.6039  &$    4.90147 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.03  }_{ -0.02 }$&$ 0.013  ^{+ 0.001  }_{ -0.000 }$&$ 0.02  ^{+ 0.34  }_{ -0.02 }$&$ 0.99  ^{+ 5.30  }_{ -0.98 }$&$ 5.78  \pm{ 1.62  }$&$ 69.90 ^{+ 3.75  }_{ -4.85 }$&$ 2.4   ^{+ 0.5   }_{ -0.6  }$&$ 0.071  \pm{ 0.003  }$&$ 2338  \pm{ 209   }$&$ 131   \pm{ 6     }$& 4.6   & 0.4  &0.105 & 0.855 \\
K00117.03  & 10875245   & 133.5041  &$    3.17996 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.02  }_{ -0.01 }$&$ 0.012  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 5.52  \pm{ 0.37  }$&$ 69.01 ^{+ 0.85  }_{ -2.78 }$&$ 2.6   ^{+ 0.1   }_{ -0.6  }$&$ 0.049  \pm{ 0.003  }$&$ 2436  \pm{ 79    }$&$ 113   \pm{ 5     }$& 3.8   & 1.1  &0.117 & 0.869 \\
K00117.04  & 10875245   & 137.8159  &$    7.95792 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.03  }_{ -0.01 }$&$ 0.007  ^{+ 0.001  }_{ -0.005 }$&$ 0.25  ^{+ 0.45  }_{ -0.23 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 2.95  \pm{ 1.54  }$&$ 80.07 ^{+ 9.93  }_{ -3.22 }$&$ 3.9   ^{+ 0.7   }_{ -1.5  }$&$ 0.096  \pm{ 0.005  }$&$ 1656  \pm{ 344   }$&$ 42    \pm{ 8     }$& 4.6   & 0.4  &0.004 & 0.179 \\
K00119.01  & 9471974    & 141.9096  &$   49.18431 ^{+    0.00000 }_{   -0.00000 }$&$ 0.53  ^{+ 0.17  }_{ -0.20 }$&$ 0.036  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 7.45  \pm{ 1.30  }$&$ 88.95 ^{+ 0.40  }_{ -0.66 }$&$ 30.6  ^{+ 4.7   }_{ -3.6  }$&$ 0.270  \pm{ 0.012  }$&$ 687   \pm{ 51    }$&$ 1482  \pm{ 23    }$& 11.5  & 11.3 &0.836 & 0.992 \\
K00119.02  & 9471974    & 312.6812  &$  190.31340 ^{+    0.00000 }_{   -0.00000 }$&$ 0.73  ^{+ 0.10  }_{ -0.14 }$&$ 0.034  ^{+ 0.002  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 6.25  \pm{ 1.05  }$&$ 89.40 ^{+ 0.15  }_{ -0.24 }$&$ 67.4  ^{+ 7.1   }_{ -21.7 }$&$ 0.655  \pm{ 0.030  }$&$ 442   \pm{ 35    }$&$ 1155  \pm{ 40    }$& 15.0  & 4.8  &0.374 & 0.937 \\
K00123.01  & 5094751    & 122.9737  &$    6.48168 ^{+    0.00000 }_{   -0.00000 }$&$ 0.61  ^{+ 0.18  }_{ -0.61 }$&$ 0.020  ^{+ 0.000  }_{ -0.003 }$&$ 0.58  ^{+ 0.12  }_{ -0.57 }$&$ 4.60  ^{+ 1.69  }_{ -4.37 }$&$ 3.99  \pm{ 0.49  }$&$ 85.92 ^{+ 4.08  }_{ -1.41 }$&$ 7.9   ^{+ 0.7   }_{ -0.5  }$&$ 0.069  \pm{ 0.002  }$&$ 1338  \pm{ 95    }$&$ 294   \pm{ 5     }$& 4.2   & 0.3  &0.703 & 0.983 \\
K00123.02  & 5094751    & 137.5738  &$   21.22254 ^{+    0.00000 }_{   -0.00000 }$&$ 0.65  ^{+ 0.09  }_{ -0.65 }$&$ 0.020  ^{+ 0.001  }_{ -0.001 }$&$ 0.30  ^{+ 0.40  }_{ -0.30 }$&$ 4.62  ^{+ 1.67  }_{ -4.41 }$&$ 3.85  \pm{ 0.39  }$&$ 88.02 ^{+ 1.89  }_{ -0.47 }$&$ 18.3  ^{+ 1.4   }_{ -1.4  }$&$ 0.152  \pm{ 0.003  }$&$ 901   \pm{ 44    }$&$ 362   \pm{ 10    }$& 6.8   & 0.4  &0.446 & 0.953 \\
K00124.01  & 11086270   & 137.1212  &$   12.69115 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.01  }_{ -0.02 }$&$ 0.017  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 3.69  \pm{ 0.32  }$&$ 85.55 ^{+ 0.39  }_{ -0.39 }$&$ 11.5  ^{+ 0.5   }_{ -0.6  }$&$ 0.107  \pm{ 0.003  }$&$ 1147  \pm{ 35    }$&$ 252   \pm{ 9     }$& 4.0   & 1.0  &0.400 & 0.944 \\
K00124.02  & 11086270   & 142.8190  &$   31.71987 ^{+    0.00000 }_{   -0.00000 }$&$ 0.91  ^{+ 0.01  }_{ -0.02 }$&$ 0.021  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.00  ^{+ 0.83  }_{ -0.00 }$&$ 4.47  \pm{ 0.31  }$&$ 87.59 ^{+ 0.22  }_{ -0.22 }$&$ 21.1  ^{+ 1.2   }_{ -1.9  }$&$ 0.200  \pm{ 0.006  }$&$ 839   \pm{ 30    }$&$ 358   \pm{ 14    }$& 5.2   & 0.4  &0.332 & 0.926 \\
K00139.01  & 8559644    & 142.0874  &$  224.79712 ^{+    0.00000 }_{   -0.00000 }$&$ 0.50  ^{+ 0.10  }_{ -0.13 }$&$ 0.055  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 6.44  \pm{ 0.65  }$&$ 89.81 ^{+ 0.06  }_{ -0.05 }$&$ 145.0 ^{+ 7.4   }_{ -10.8 }$&$ 0.753  \pm{ 0.016  }$&$ 324   \pm{ 11    }$&$ 3496  \pm{ 84    }$& 10.5  & 0.8  &0.409 & 0.945 \\
K00139.02  & 8559644    & 141.3521  &$    3.34184 ^{+    0.00000 }_{   -0.00000 }$&$ 0.33  ^{+ 0.18  }_{ -0.31 }$&$ 0.012  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.01  ^{+ 4.28  }_{ -0.01 }$&$ 1.44  \pm{ 0.08  }$&$ 87.84 ^{+ 1.74  }_{ -1.25 }$&$ 8.6   ^{+ 0.4   }_{ -0.5  }$&$ 0.046  \pm{ 0.001  }$&$ 1343  \pm{ 38    }$&$ 158   \pm{ 7     }$& 2.8   & 0.5  &0.143 & 0.806 \\
K00148.01  & 5735762    & 124.0630  &$    4.77798 ^{+    0.00000 }_{   -0.00000 }$&$ 0.47  ^{+ 0.12  }_{ -0.45 }$&$ 0.020  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.14  \pm{ 0.23  }$&$ 87.72 ^{+ 2.16  }_{ -0.68 }$&$ 12.3  ^{+ 0.7   }_{ -0.7  }$&$ 0.054  \pm{ 0.001  }$&$ 1000  \pm{ 38    }$&$ 465   \pm{ 8     }$& 2.8   & 2.1  &0.351 & 0.964 \\
K00148.02  & 5735762    & 125.3398  &$    9.67393 ^{+    0.00000 }_{   -0.00000 }$&$ 0.46  ^{+ 0.12  }_{ -0.45 }$&$ 0.029  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.78  \pm{ 0.18  }$&$ 88.72 ^{+ 0.84  }_{ -0.43 }$&$ 20.1  ^{+ 0.7   }_{ -3.5  }$&$ 0.086  \pm{ 0.001  }$&$ 762   \pm{ 26    }$&$ 972   \pm{ 12    }$& 3.3   & 2.3  &0.631 & 0.988 \\
K00148.03  & 5735762    & 146.0657  &$   42.89592 ^{+    0.00000 }_{   -0.00000 }$&$ 0.37  ^{+ 0.23  }_{ -0.30 }$&$ 0.022  ^{+ 0.005  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.09  \pm{ 0.30  }$&$ 89.63 ^{+ 0.18  }_{ -0.18 }$&$ 55.6  ^{+ 2.1   }_{ -5.8  }$&$ 0.231  \pm{ 0.005  }$&$ 457   \pm{ 13    }$&$ 592   \pm{ 29    }$& 5.5   & 1.1  &0.070 & 0.790 \\
K00153.01  & 12252424   & 139.7122  &$    8.92511 ^{+    0.00000 }_{   -0.00000 }$&$ 0.51  ^{+ 0.12  }_{ -0.51 }$&$ 0.029  ^{+ 0.007  }_{ -0.001 }$&$ 0.01  ^{+ 0.54  }_{ -0.01 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 2.24  \pm{ 0.36  }$&$ 88.73 ^{+ 0.98  }_{ -0.41 }$&$ 22.8  ^{+ 0.7   }_{ -2.6  }$&$ 0.077  \pm{ 0.001  }$&$ 651   \pm{ 17    }$&$ 966   \pm{ 15    }$& 2.6   & 1.0  &0.871 & 0.994 \\
K00153.02  & 12252424   & 128.5467  &$    4.75399 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.024  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 1.90  \pm{ 0.18  }$&$ 90.00 ^{+ 0.00  }_{ -1.25 }$&$ 14.9  ^{+ 0.5   }_{ -0.4  }$&$ 0.051  \pm{ 0.001  }$&$ 819   \pm{ 13    }$&$ 747   \pm{ 11    }$& 2.5   & 0.5  &0.889 & 0.995 \\
K00159.01  & 8972058    & 136.7363  &$    8.99092 ^{+    0.00000 }_{   -0.00000 }$&$ 0.86  ^{+ 0.04  }_{ -0.09 }$&$ 0.022  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 5.46  \pm{ 0.78  }$&$ 84.29 ^{+ 1.49  }_{ -1.08 }$&$ 8.1   ^{+ 0.8   }_{ -2.7  }$&$ 0.089  \pm{ 0.004  }$&$ 1367  \pm{ 109   }$&$ 449   \pm{ 12    }$& 4.3   & 0.5  &0.293 & 0.912 \\
K00159.02  & 8972058    & 134.7278  &$    2.40365 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.02  }_{ -0.01 }$&$ 0.011  ^{+ 0.000  }_{ -0.001 }$&$ 0.02  ^{+ 0.07  }_{ -0.02 }$&$ 0.40  ^{+ 4.24  }_{ -0.40 }$&$ 2.83  \pm{ 0.29  }$&$ 72.87 ^{+ 1.92  }_{ -1.58 }$&$ 3.3   ^{+ 0.2   }_{ -0.3  }$&$ 0.037  \pm{ 0.001  }$&$ 2201  \pm{ 94    }$&$ 75    \pm{ 6     }$& 1.5   & 0.6  &0.024 & 0.381 \\
K00168.01  & 11512246   & 133.2871  &$   10.74245 ^{+    0.00000 }_{   -0.00000 }$&$ 0.74  ^{+ 0.07  }_{ -0.10 }$&$ 0.020  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.65  }_{ -0.00 }$&$ 4.79  \pm{ 0.96  }$&$ 85.33 ^{+ 0.84  }_{ -1.10 }$&$ 9.2   ^{+ 0.7   }_{ -0.8  }$&$ 0.097  \pm{ 0.003  }$&$ 1339  \pm{ 70    }$&$ 394   \pm{ 13    }$& 6.3   & 0.2  &0.312 & 0.958 \\
K00168.02  & 11512246   & 147.5788  &$   15.27448 ^{+    0.00000 }_{   -0.00000 }$&$ 0.81  ^{+ 0.09  }_{ -0.22 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.18  }_{ -0.00 }$&$ 0.00  ^{+ 0.33  }_{ -0.00 }$&$ 3.64  \pm{ 0.89  }$&$ 85.93 ^{+ 1.77  }_{ -1.21 }$&$ 11.2  ^{+ 0.8   }_{ -1.2  }$&$ 0.124  \pm{ 0.004  }$&$ 1200  \pm{ 82    }$&$ 207   \pm{ 16    }$& 6.2   & 0.4  &0.092 & 0.835 \\
K00168.03  & 11512246   & 138.3254  &$    7.10690 ^{+    0.00000 }_{   -0.00000 }$&$ 0.78  ^{+ 0.18  }_{ -0.12 }$&$ 0.009  ^{+ 0.001  }_{ -0.000 }$&$ 0.22  ^{+ 0.48  }_{ -0.22 }$&$ 1.53  ^{+ 4.76  }_{ -1.43 }$&$ 2.38  \pm{ 0.31  }$&$ 83.51 ^{+ 2.26  }_{ -2.71 }$&$ 6.8   ^{+ 0.7   }_{ -0.7  }$&$ 0.074  \pm{ 0.003  }$&$ 1554  \pm{ 101   }$&$ 95    \pm{ 11    }$& 5.1   & 0.1  &0.041 & 0.681 \\
K00244.01  & 4349452    & 178.5274  &$   12.72036 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.01  }_{ -0.18 }$&$ 0.038  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 8.87  \pm{ 1.43  }$&$ 86.42 ^{+ 1.36  }_{ -1.12 }$&$ 11.1  ^{+ 1.5   }_{ -1.0  }$&$ 0.114  \pm{ 0.003  }$&$ 1048  \pm{ 108   }$&$ 1171  \pm{ 4     }$& 3.1   & 37.2 &0.973 & 0.999 \\
K00244.02  & 4349452    & 171.7046  &$    6.23856 ^{+    0.00000 }_{   -0.00000 }$&$ 0.86  ^{+ 0.02  }_{ -0.12 }$&$ 0.021  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 4.90  \pm{ 0.66  }$&$ 82.94 ^{+ 1.40  }_{ -0.79 }$&$ 6.7   ^{+ 0.3   }_{ -0.6  }$&$ 0.070  \pm{ 0.002  }$&$ 1527  \pm{ 91    }$&$ 398   \pm{ 3     }$& 3.7   & 15.9 &0.953 & 0.998 \\
K00245.01  & 8478994    & 175.2497  &$   39.79219 ^{+    0.00000 }_{   -0.00000 }$&$ 0.68  ^{+ 0.09  }_{ -0.08 }$&$ 0.024  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.36  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.45  \pm{ 0.27  }$&$ 89.24 ^{+ 0.14  }_{ -0.22 }$&$ 49.5  ^{+ 2.5   }_{ -7.7  }$&$ 0.221  \pm{ 0.004  }$&$ 489   \pm{ 20    }$&$ 605   \pm{ 5     }$& 4.5   & 7.1  &0.947 & 0.999 \\
K00245.02  & 8478994    & 191.8385  &$   21.30185 ^{+    0.00000 }_{   -0.00000 }$&$ 0.58  ^{+ 0.08  }_{ -0.58 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.28  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.80  \pm{ 0.15  }$&$ 89.02 ^{+ 0.98  }_{ -0.19 }$&$ 33.6  ^{+ 1.7   }_{ -2.3  }$&$ 0.147  \pm{ 0.003  }$&$ 605   \pm{ 21    }$&$ 77    \pm{ 4     }$& 4.0   & 3.3  &0.186 & 0.920 \\
K00245.03  & 8478994    & 184.0333  &$   13.36727 ^{+    0.00000 }_{   -0.00000 }$&$ 0.84  ^{+ 0.16  }_{ -0.13 }$&$ 0.004  ^{+ 0.001  }_{ -0.000 }$&$ 0.03  ^{+ 0.51  }_{ -0.03 }$&$ 0.16  ^{+ 1.88  }_{ -0.16 }$&$ 0.37  \pm{ 0.09  }$&$ 88.07 ^{+ 0.52  }_{ -0.60 }$&$ 24.0  ^{+ 1.7   }_{ -3.7  }$&$ 0.107  \pm{ 0.002  }$&$ 703   \pm{ 30    }$&$ 12    \pm{ 3     }$& 2.2   & 1.1  &0.016 & 0.443 \\
K00245.04  & 8478994    & 195.7268  &$   51.19880 ^{+    0.00000 }_{   -0.00000 }$&$ 0.29  ^{+ 0.58  }_{ -0.29 }$&$ 0.003  ^{+ 0.006  }_{ -0.001 }$&$ 0.08  ^{+ 0.61  }_{ -0.07 }$&$ 3.34  ^{+ 2.95  }_{ -3.23 }$&$ 0.35  \pm{ 0.35  }$&$ 89.73 ^{+ 0.27  }_{ -0.61 }$&$ 58.7  ^{+ 2.9   }_{ -8.0  }$&$ 0.262  \pm{ 0.007  }$&$ 446   \pm{ 18    }$&$ 13    \pm{ 7     }$& 6.1   & 0.3  &0.013 & 0.402 \\
K00246.01  & 11295426   & 173.8571  &$    5.39877 ^{+    0.00000 }_{   -0.00000 }$&$ 0.49  ^{+ 0.06  }_{ -0.49 }$&$ 0.017  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.32  \pm{ 0.07  }$&$ 87.36 ^{+ 2.61  }_{ -0.37 }$&$ 10.7  ^{+ 0.2   }_{ -0.2  }$&$ 0.062  \pm{ 0.001  }$&$ 1176  \pm{ 13    }$&$ 340   \pm{ 2     }$& 3.5   & 8.4  &0.972 & 0.999 \\
K00246.02  & 11295426   & 136.3854  &$    9.60487 ^{+    0.00000 }_{   -0.00000 }$&$ 1.37  ^{+ -0.45 }_{ -0.51 }$&$ 0.002  ^{+ 0.012  }_{ -0.000 }$&$ 0.03  ^{+ 0.67  }_{ -0.01 }$&$ 0.07  ^{+ 0.11  }_{ -0.07 }$&$ 0.27  \pm{ 0.83  }$&$ 85.03 ^{+ 2.70  }_{ -0.50 }$&$ 15.6  ^{+ 0.2   }_{ -0.3  }$&$ 0.090  \pm{ 0.001  }$&$ 968   \pm{ 13    }$&$ 0     \pm{ 4     }$& 0.0   & 0.7  &0.090 & 0.712 \\
K00260.01  & 8292840    & 172.7904  &$   10.49570 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.009  ^{+ 0.011  }_{ -0.007 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.23  ^{+ 0.29  }_{ -0.11 }$&$ 1.04  \pm{ 1.05  }$&$ 84.40 ^{+ 0.82  }_{ -0.53 }$&$ 18.3  ^{+ 1.7   }_{ -2.1  }$&$ 0.094  \pm{ 0.004  }$&$ 913   \pm{ 54    }$&$ 0     \pm{ 5     }$& 0.0   & 1.6  &0.295 & 0.954 \\
K00260.02  & 8292840    & 245.0413  &$  100.28340 ^{+    0.00000 }_{   -0.00000 }$&$ 0.60  ^{+ 0.08  }_{ -0.60 }$&$ 0.018  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 3.41  \pm{ 0.63  }$&$ 89.40 ^{+ 0.50  }_{ -0.10 }$&$ 50.6  ^{+ 4.4   }_{ -0.0  }$&$ 0.456  \pm{ 0.017  }$&$ 540   \pm{ 45    }$&$ 339   \pm{ 12    }$& 10.9  & 0.6  &0.357 & 0.965 \\
K00260.03  & 8292840    & 140.2944  &$   21.86964 ^{+    0.00000 }_{   -0.00000 }$&$ 2.35  ^{+ -1.36 }_{ -1.52 }$&$ 0.002  ^{+ 0.019  }_{ -0.000 }$&$ 0.01  ^{+ 0.01  }_{ -0.01 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.24  \pm{ 1.16  }$&$ 85.94 ^{+ 0.96  }_{ -0.60 }$&$ 30.0  ^{+ 2.1   }_{ -2.0  }$&$ 0.155  \pm{ 0.005  }$&$ 707   \pm{ 36    }$&$ 0     \pm{ 7     }$& 0.0   & 1.4  &0.188 & 0.921 \\
K00262.01  & 11807274   & 172.6319  &$    7.81251 ^{+    0.00000 }_{   -0.00000 }$&$ 0.58  ^{+ 0.30  }_{ -0.00 }$&$ 0.012  ^{+ 0.000  }_{ -0.002 }$&$ 0.70  ^{+ -0.00 }_{ -0.61 }$&$ 4.71  ^{+ 0.91  }_{ -4.24 }$&$ 3.09  \pm{ 0.34  }$&$ 85.36 ^{+ 0.10  }_{ -2.78 }$&$ 6.9   ^{+ 0.3   }_{ -0.2  }$&$ 0.081  \pm{ 0.002  }$&$ 1506  \pm{ 36    }$&$ 89    \pm{ 3     }$& 4.9   & 0.6  &0.299 & 0.914 \\
K00262.02  & 11807274   & 136.9686  &$    9.37614 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.00  }_{ -0.00 }$&$ 0.011  ^{+ 0.000  }_{ -0.003 }$&$ 0.03  ^{+ 0.60  }_{ -0.03 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.12  \pm{ 0.48  }$&$ 83.01 ^{+ 0.30  }_{ -0.20 }$&$ 7.8   ^{+ 0.2   }_{ -0.2  }$&$ 0.091  \pm{ 0.002  }$&$ 1424  \pm{ 24    }$&$ 85    \pm{ 4     }$& 2.6   & 1.1  &0.387 & 0.940 \\
K00270.01  & 6528464    & 175.0152  &$   12.58250 ^{+    0.00000 }_{   -0.00000 }$&$ 0.53  ^{+ 0.15  }_{ -0.48 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.02  ^{+ 0.48  }_{ -0.02 }$&$ 0.37  ^{+ 5.92  }_{ -0.37 }$&$ 1.82  \pm{ 0.12  }$&$ 87.64 ^{+ 1.79  }_{ -1.02 }$&$ 12.5  ^{+ 0.8   }_{ -1.6  }$&$ 0.103  \pm{ 0.002  }$&$ 1025  \pm{ 37    }$&$ 105   \pm{ 5     }$& 6.4   & 2.1  &0.200 & 0.862 \\
K00270.02  & 6528464    & 162.0396  &$   33.67312 ^{+    0.00000 }_{   -0.00000 }$&$ 0.62  ^{+ 0.06  }_{ -0.08 }$&$ 0.012  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 1.29  }_{ -0.00 }$&$ 2.17  \pm{ 0.26  }$&$ 88.60 ^{+ 0.25  }_{ -0.24 }$&$ 25.3  ^{+ 1.0   }_{ -2.0  }$&$ 0.197  \pm{ 0.005  }$&$ 732   \pm{ 24    }$&$ 164   \pm{ 10    }$& 8.1   & 1.1  &0.165 & 0.832 \\
K00271.01  & 9451706    & 172.5460  &$   48.63057 ^{+    0.00000 }_{   -0.00000 }$&$ 0.34  ^{+ 0.18  }_{ -0.30 }$&$ 0.017  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.59  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.17  \pm{ 0.15  }$&$ 89.61 ^{+ 0.24  }_{ -0.21 }$&$ 50.4  ^{+ 1.6   }_{ -4.4  }$&$ 0.274  \pm{ 0.008  }$&$ 573   \pm{ 16    }$&$ 346   \pm{ 12    }$& 6.9   & 3.7  &0.575 & 0.985 \\
K00271.02  & 9451706    & 209.0731  &$   29.39241 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.016  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 2.12  \pm{ 0.32  }$&$ 90.00 ^{+ -0.00 }_{ -0.20 }$&$ 34.2  ^{+ 1.2   }_{ -2.4  }$&$ 0.201  \pm{ 0.004  }$&$ 695   \pm{ 18    }$&$ 307   \pm{ 10    }$& 6.6   & 3.4  &0.654 & 0.990 \\
K00271.03  & 9451706    & 141.5109  &$   14.43593 ^{+    0.00000 }_{   -0.00000 }$&$ 0.73  ^{+ 0.08  }_{ -0.15 }$&$ 0.010  ^{+ 0.002  }_{ -0.000 }$&$ 0.08  ^{+ 0.52  }_{ -0.08 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.31  \pm{ 0.21  }$&$ 88.11 ^{+ 0.46  }_{ -0.47 }$&$ 20.9  ^{+ 1.5   }_{ -4.6  }$&$ 0.125  \pm{ 0.003  }$&$ 872   \pm{ 41    }$&$ 101   \pm{ 6     }$& 3.5   & 3.0  &0.217 & 0.933 \\
K00274.01  & 8077137    & 175.9276  &$   15.09205 ^{+    0.00000 }_{   -0.00000 }$&$ 0.73  ^{+ 0.22  }_{ -0.17 }$&$ 0.004  ^{+ 0.000  }_{ -0.002 }$&$ 0.23  ^{+ 0.47  }_{ -0.23 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.52  \pm{ 0.25  }$&$ 87.13 ^{+ 0.94  }_{ -0.84 }$&$ 12.7  ^{+ 1.5   }_{ -0.7  }$&$ 0.123  \pm{ 0.006  }$&$ 1050  \pm{ 175   }$&$ 18    \pm{ 7     }$& 5.6   & 0.7  &0.014 & 0.263 \\
K00274.02  & 8077137    & 153.4920  &$   22.79519 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.03  }_{ -0.17 }$&$ 0.005  ^{+ 0.021  }_{ -0.001 }$&$ 0.22  ^{+ 0.48  }_{ -0.22 }$&$ 0.03  ^{+ 0.66  }_{ -0.03 }$&$ 0.59  \pm{ 1.34  }$&$ 87.78 ^{+ 0.97  }_{ -1.02 }$&$ 30.5  ^{+ 2.8   }_{ -4.7  }$&$ 0.161  \pm{ 0.007  }$&$ 809   \pm{ 108   }$&$ 20    \pm{ 8     }$& 2.8   & 0.6  &0.010 & 0.202 \\
K00275.01  & 10586004   & 176.8205  &$   15.79186 ^{+    0.00000 }_{   -0.00000 }$&$ 0.39  ^{+ 0.10  }_{ -0.30 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 2.68  \pm{ 0.13  }$&$ 88.57 ^{+ 0.92  }_{ -0.43 }$&$ 14.9  ^{+ 0.5   }_{ -0.7  }$&$ 0.133  \pm{ 0.003  }$&$ 975   \pm{ 29    }$&$ 199   \pm{ 8     }$& 7.3   & 0.6  &0.347 & 0.930 \\
K00275.02  & 10586004   & 208.7874  &$   82.19970 ^{+    0.00000 }_{   -0.00000 }$&$ 0.22  ^{+ 0.45  }_{ -0.22 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.43  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.63  \pm{ 0.38  }$&$ 89.79 ^{+ 0.21  }_{ -0.43 }$&$ 72.3  ^{+ 6.4   }_{ -24.2 }$&$ 0.378  \pm{ 0.018  }$&$ 490   \pm{ 57    }$&$ 219   \pm{ 21    }$& 10.0  & 0.4  &0.109 & 0.754 \\
K00277.01  & 11401755   & 171.6976  &$   16.23069 ^{+    0.00000 }_{   -0.00000 }$&$ 0.36  ^{+ 0.18  }_{ -0.36 }$&$ 0.019  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 4.11  \pm{ 0.41  }$&$ 88.51 ^{+ 1.49  }_{ -0.73 }$&$ 13.5  ^{+ 0.9   }_{ -0.9  }$&$ 0.127  \pm{ 0.004  }$&$ 1067  \pm{ 48    }$&$ 398   \pm{ 11    }$& 8.5   & 0.4  &0.661 & 0.980 \\
K00277.02  & 11401755   & 141.6820  &$   13.84943 ^{+    0.00000 }_{   -0.00000 }$&$ 0.75  ^{+ 0.13  }_{ -0.12 }$&$ 0.007  ^{+ 0.001  }_{ -0.000 }$&$ 0.02  ^{+ 0.53  }_{ -0.02 }$&$ 1.77  ^{+ 4.52  }_{ -1.72 }$&$ 1.50  \pm{ 0.16  }$&$ 86.45 ^{+ 1.10  }_{ -0.67 }$&$ 12.0  ^{+ 0.7   }_{ -0.9  }$&$ 0.115  \pm{ 0.004  }$&$ 1139  \pm{ 44    }$&$ 46    \pm{ 8     }$& 5.8   & 0.3  &0.006 & 0.138 \\
K00279.01  & 12314973   & 176.7045  &$   28.45499 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.11  }_{ -0.07 }$&$ 0.038  ^{+ 0.000  }_{ -0.001 }$&$ 0.23  ^{+ 0.37  }_{ -0.23 }$&$ 0.48  ^{+ 1.87  }_{ -0.48 }$&$ 10.94 \pm{ 2.37  }$&$ 86.82 ^{+ 0.64  }_{ -1.13 }$&$ 15.9  ^{+ 1.5   }_{ -1.4  }$&$ 0.199  \pm{ 0.007  }$&$ 1067  \pm{ 60    }$&$ 1420  \pm{ 12    }$& 8.5   & 0.5  &0.732 & 0.993 \\
K00279.02  & 12314973   & 136.9443  &$   15.41299 ^{+    0.00000 }_{   -0.00000 }$&$ 0.83  ^{+ 0.04  }_{ -0.07 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 4.99  \pm{ 0.55  }$&$ 85.32 ^{+ 0.90  }_{ -0.84 }$&$ 9.7   ^{+ 0.6   }_{ -2.7  }$&$ 0.133  \pm{ 0.005  }$&$ 1333  \pm{ 71    }$&$ 253   \pm{ 9     }$& 6.8   & 0.1  &0.326 & 0.960 \\
K00279.03  & 12314973   & 136.1570  &$    7.51465 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.88  }_{ -0.00 }$&$ 0.005  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.63  \pm{ 0.49  }$&$ 90.00 ^{+ 0.00  }_{ -11.69 }$&$ 4.3   ^{+ 1.4   }_{ -0.0  }$&$ 0.075  \pm{ 0.006  }$&$ 1085  \pm{ 202   }$&$ 32    \pm{ 5     }$& 3.7   & 0.5  &0.006 & 0.239 \\
K00282.01  & 5088536    & 182.1039  &$   27.50868 ^{+    0.00000 }_{   -0.00000 }$&$ 0.38  ^{+ 0.31  }_{ -0.29 }$&$ 0.023  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.77  \pm{ 0.23  }$&$ 89.35 ^{+ 0.42  }_{ -0.77 }$&$ 35.5  ^{+ 3.2   }_{ -2.1  }$&$ 0.176  \pm{ 0.005  }$&$ 667   \pm{ 51    }$&$ 637   \pm{ 9     }$& 5.8   & 1.1  &0.859 & 0.997 \\
K00282.02  & 5088536    & 139.0684  &$    8.45742 ^{+    0.00000 }_{   -0.00000 }$&$ 0.36  ^{+ 0.19  }_{ -0.36 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.26  ^{+ 0.44  }_{ -0.26 }$&$ 0.19  ^{+ 6.10  }_{ -0.19 }$&$ 0.84  \pm{ 0.15  }$&$ 88.77 ^{+ 1.23  }_{ -0.69 }$&$ 16.0  ^{+ 1.1   }_{ -5.4  }$&$ 0.079  \pm{ 0.002  }$&$ 955   \pm{ 44    }$&$ 76    \pm{ 4     }$& 3.4   & 0.4  &0.029 & 0.597 \\
K00282.03  & 5088536    & 201.1697  &$   87.51870 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.05  }_{ -0.12 }$&$ 0.008  ^{+ 0.002  }_{ -0.006 }$&$ 0.34  ^{+ 0.36  }_{ -0.33 }$&$ 0.72  ^{+ 5.56  }_{ -0.71 }$&$ 0.76  \pm{ 0.40  }$&$ 89.41 ^{+ 0.59  }_{ -0.22 }$&$ 84.8  ^{+ 7.3   }_{ -9.9  }$&$ 0.368  \pm{ 0.015  }$&$ 403   \pm{ 18    }$&$ 67    \pm{ 17    }$& 4.0   & 0.0  &0.003 & 0.135 \\
K00283.01  & 5695396    & 170.5985  &$   16.09194 ^{+    0.00000 }_{   -0.00000 }$&$ 0.80  ^{+ 0.06  }_{ -0.07 }$&$ 0.021  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.44  }_{ -0.00 }$&$ 0.00  ^{+ 1.05  }_{ -0.00 }$&$ 2.41  \pm{ 0.32  }$&$ 88.22 ^{+ 0.29  }_{ -0.33 }$&$ 25.6  ^{+ 1.5   }_{ -3.5  }$&$ 0.127  \pm{ 0.005  }$&$ 739   \pm{ 30    }$&$ 423   \pm{ 6     }$& 3.0   & 6.1  &0.890 & 0.995 \\
K00283.02  & 5695396    & 154.4205  &$   25.51704 ^{+    0.00000 }_{   -0.00000 }$&$ 0.35  ^{+ 0.20  }_{ -0.35 }$&$ 0.008  ^{+ 0.002  }_{ -0.000 }$&$ 0.05  ^{+ 0.61  }_{ -0.05 }$&$ 0.06  ^{+ 6.13  }_{ -0.06 }$&$ 0.87  \pm{ 0.17  }$&$ 89.45 ^{+ 0.55  }_{ -0.33 }$&$ 36.2  ^{+ 2.0   }_{ -2.0  }$&$ 0.167  \pm{ 0.009  }$&$ 621   \pm{ 23    }$&$ 74    \pm{ 8     }$& 5.0   & 0.9  &0.012 & 0.230 \\
K00284.01  & 6021275    & 179.4253  &$   18.00999 ^{+    0.00000 }_{   -0.00000 }$&$ 0.81  ^{+ 0.18  }_{ -0.08 }$&$ 0.013  ^{+ 0.003  }_{ -0.001 }$&$ 0.17  ^{+ 0.45  }_{ -0.17 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 1.41  \pm{ 0.25  }$&$ 88.34 ^{+ 0.34  }_{ -0.59 }$&$ 27.4  ^{+ 2.0   }_{ -2.6  }$&$ 0.134  \pm{ 0.005  }$&$ 738   \pm{ 34    }$&$ 164   \pm{ 8     }$& 3.0   & 1.2  &0.165 & 0.908 \\
K00284.02  & 6021275    & 169.6420  &$    6.41483 ^{+    0.00000 }_{   -0.00000 }$&$ 0.30  ^{+ 0.18  }_{ -0.30 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 1.13  \pm{ 0.15  }$&$ 88.78 ^{+ 1.22  }_{ -0.78 }$&$ 13.4  ^{+ 0.8   }_{ -3.8  }$&$ 0.067  \pm{ 0.002  }$&$ 1051  \pm{ 43    }$&$ 111   \pm{ 5     }$& 3.4   & 1.4  &0.076 & 0.803 \\
K00284.03  & 6021275    & 168.8602  &$    6.17818 ^{+    0.00000 }_{   -0.00000 }$&$ 0.35  ^{+ 0.18  }_{ -0.35 }$&$ 0.009  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.33  }_{ -0.00 }$&$ 0.00  ^{+ 0.52  }_{ -0.00 }$&$ 0.99  \pm{ 0.14  }$&$ 88.51 ^{+ 1.48  }_{ -0.85 }$&$ 13.7  ^{+ 0.9   }_{ -0.9  }$&$ 0.065  \pm{ 0.003  }$&$ 1065  \pm{ 43    }$&$ 98    \pm{ 5     }$& 3.3   & 1.0  &0.060 & 0.763 \\
K00284.04  & 6021275    & 239.1980  &$  110.29290 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.09  }_{ -0.20 }$&$ 0.010  ^{+ 0.021  }_{ -0.001 }$&$ 0.10  ^{+ 0.60  }_{ -0.10 }$&$ 1.57  ^{+ 4.72  }_{ -1.45 }$&$ 1.04  \pm{ 1.18  }$&$ 89.47 ^{+ 0.22  }_{ -0.45 }$&$ 94.9  ^{+ 4.5   }_{ -6.8  }$&$ 0.452  \pm{ 0.019  }$&$ 397   \pm{ 13    }$&$ 91    \pm{ 26    }$& 4.7   & 0.8  &0.023 & 0.546 \\
K00285.01  & 6196457    & 179.2804  &$   13.74878 ^{+    0.00000 }_{   -0.00000 }$&$ 0.72  ^{+ 0.03  }_{ -0.06 }$&$ 0.020  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.17  ^{+ 6.12  }_{ -0.17 }$&$ 4.47  \pm{ 0.33  }$&$ 86.70 ^{+ 0.47  }_{ -0.26 }$&$ 11.8  ^{+ 0.5   }_{ -0.2  }$&$ 0.119  \pm{ 0.004  }$&$ 1102  \pm{ 32    }$&$ 413   \pm{ 7     }$& 6.1   & 1.0  &0.829 & 0.996 \\
K00285.02  & 6196457    & 147.9103  &$   26.72428 ^{+    0.00000 }_{   -0.00000 }$&$ 0.54  ^{+ 0.09  }_{ -0.54 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.02  ^{+ 0.56  }_{ -0.02 }$&$ 0.61  ^{+ 5.67  }_{ -0.61 }$&$ 2.72  \pm{ 0.46  }$&$ 88.47 ^{+ 1.18  }_{ -0.38 }$&$ 19.6  ^{+ 1.1   }_{ -1.1  }$&$ 0.186  \pm{ 0.008  }$&$ 868   \pm{ 36    }$&$ 178   \pm{ 11    }$& 8.6   & 0.5  &0.383 & 0.969 \\
K00285.03  & 6196457    & 134.2716  &$   49.35899 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.52  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.49  ^{+ 0.21  }_{ -0.48 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 2.41  \pm{ 0.30  }$&$ 90.00 ^{+ 0.00  }_{ -0.99 }$&$ 28.7  ^{+ 0.5   }_{ -1.6  }$&$ 0.278  \pm{ 0.009  }$&$ 717   \pm{ 19    }$&$ 145   \pm{ 16    }$& 11.2  & 0.5  &0.040 & 0.674 \\
K00289.01  & 10386922   & 138.7360  &$   26.62940 ^{+    0.00000 }_{   -0.00000 }$&$ 0.88  ^{+ 0.12  }_{ -0.08 }$&$ 0.023  ^{+ 0.001  }_{ -0.001 }$&$ 0.14  ^{+ 0.42  }_{ -0.14 }$&$ 0.38  ^{+ 1.86  }_{ -0.38 }$&$ 6.03  \pm{ 1.48  }$&$ 86.45 ^{+ 0.99  }_{ -2.55 }$&$ 15.4  ^{+ 3.2   }_{ -2.5  }$&$ 0.187  \pm{ 0.016  }$&$ 957   \pm{ 149   }$&$ 483   \pm{ 16    }$& 8.2   & 0.1  &0.481 & 0.959 \\
K00289.02  & 10386922   & 403.6729  &$  296.63709 ^{+    0.00000 }_{   -0.00000 }$&$ 0.86  ^{+ 0.14  }_{ -0.09 }$&$ 0.049  ^{+ 0.003  }_{ -0.001 }$&$ 0.48  ^{+ 0.22  }_{ -0.31 }$&$ 1.77  ^{+ 4.52  }_{ -0.83 }$&$ 12.42 \pm{ 3.73  }$&$ 89.37 ^{+ 0.20  }_{ -0.31 }$&$ 77.0  ^{+ 14.7  }_{ -14.0 }$&$ 0.927  \pm{ 0.077  }$&$ 410   \pm{ 52    }$&$ 2842  \pm{ 70    }$& 16.2  & 0.1  &0.369 & 0.936 \\
K00291.01  & 10933561   & 185.1521  &$   31.51789 ^{+    0.00000 }_{   -0.00000 }$&$ 0.63  ^{+ 0.07  }_{ -0.31 }$&$ 0.018  ^{+ 0.001  }_{ -0.001 }$&$ 0.11  ^{+ 0.51  }_{ -0.11 }$&$ 0.36  ^{+ 5.86  }_{ -0.36 }$&$ 3.47  \pm{ 0.25  }$&$ 88.54 ^{+ 0.60  }_{ -0.25 }$&$ 24.0  ^{+ 0.8   }_{ -1.4  }$&$ 0.193  \pm{ 0.007  }$&$ 750   \pm{ 28    }$&$ 357   \pm{ 20    }$& 7.7   & 0.5  &0.091 & 0.714 \\
K00291.02  & 10933561   & 134.1052  &$    8.12986 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.01  }_{ -0.01 }$&$ 0.014  ^{+ 0.000  }_{ -0.001 }$&$ 0.02  ^{+ 0.68  }_{ -0.02 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.67  \pm{ 0.13  }$&$ 84.25 ^{+ 0.30  }_{ -0.19 }$&$ 9.1   ^{+ 0.2   }_{ -0.2  }$&$ 0.078  \pm{ 0.002  }$&$ 1196  \pm{ 24    }$&$ 133   \pm{ 9     }$& 2.3   & 1.1  &0.088 & 0.707 \\
K00295.01  & 11547513   & 171.8763  &$    5.31743 ^{+    0.00000 }_{   -0.00000 }$&$ 1.03  ^{+ -0.03 }_{ -0.07 }$&$ 0.020  ^{+ 0.048  }_{ -0.000 }$&$ 0.27  ^{+ 0.41  }_{ -0.27 }$&$ 0.00  ^{+ 1.29  }_{ -0.00 }$&$ 5.98  \pm{ 7.42  }$&$ 77.04 ^{+ 2.38  }_{ -8.58 }$&$ 4.3   ^{+ 0.6   }_{ -2.2  }$&$ 0.069  \pm{ 0.005  }$&$ 1820  \pm{ 235   }$&$ 286   \pm{ 6     }$& 3.3   & 1.3  &0.676 & 0.981 \\
K00295.02  & 11547513   & 135.5088  &$   10.10575 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.02  }_{ -0.01 }$&$ 0.013  ^{+ 0.003  }_{ -0.004 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.05  ^{+ 1.22  }_{ -0.05 }$&$ 3.44  \pm{ 1.29  }$&$ 83.96 ^{+ 0.71  }_{ -3.11 }$&$ 8.5   ^{+ 2.0   }_{ -1.6  }$&$ 0.100  \pm{ 0.010  }$&$ 1168  \pm{ 154   }$&$ 110   \pm{ 8     }$& 2.3   & 0.7  &0.093 & 0.719 \\
K00298.01  & 12785320   & 178.3053  &$   19.96000 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.02  }_{ -0.24 }$&$ 0.008  ^{+ 0.014  }_{ -0.004 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.53  \pm{ 0.93  }$&$ 85.54 ^{+ 3.11  }_{ -1.91 }$&$ 11.1  ^{+ 3.7   }_{ -5.1  }$&$ 0.138  \pm{ 0.011  }$&$ 986   \pm{ 474   }$&$ 0     \pm{ 18    }$& 2.9   & 0.2  &0.032 & 0.450 \\
K00298.02  & 12785320   & 170.7233  &$   57.38425 ^{+    0.00000 }_{   -0.00000 }$&$ 1.85  ^{+ -0.85 }_{ -0.91 }$&$ 0.017  ^{+ 0.003  }_{ -0.007 }$&$ 0.70  ^{+ -0.00 }_{ -0.13 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 4.25  \pm{ 2.53  }$&$ 86.03 ^{+ 2.22  }_{ -4.02 }$&$ 22.3  ^{+ 5.5   }_{ -10.3 }$&$ 0.295  \pm{ 0.028  }$&$ 669   \pm{ 276   }$&$ 198   \pm{ 26    }$& 4.4   & 0.7  &0.011 & 0.211 \\
K00301.01  & 3642289    & 171.7134  &$    6.00255 ^{+    0.00000 }_{   -0.00000 }$&$ 0.74  ^{+ 0.16  }_{ -0.74 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.28  ^{+ 0.42  }_{ -0.28 }$&$ 4.67  ^{+ 1.62  }_{ -3.85 }$&$ 5.28  \pm{ 0.58  }$&$ 82.02 ^{+ 7.98  }_{ -2.05 }$&$ 5.1   ^{+ 0.3   }_{ -1.2  }$&$ 0.077  \pm{ 0.004  }$&$ 1804  \pm{ 140   }$&$ 196   \pm{ 6     }$& 4.3   & 0.9  &0.122 & 0.776 \\
K00301.02  & 3642289    & 141.3742  &$   11.44883 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.03  }_{ -0.13 }$&$ 0.009  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 3.09  \pm{ 0.57  }$&$ 83.50 ^{+ 5.91  }_{ -1.41 }$&$ 8.0   ^{+ 0.5   }_{ -1.0  }$&$ 0.114  \pm{ 0.005  }$&$ 1489  \pm{ 79    }$&$ 77    \pm{ 9     }$& 5.2   & 0.3  &0.005 & 0.113 \\
K00304.01  & 6029239    & 174.9087  &$    8.51205 ^{+    0.00000 }_{   -0.00000 }$&$ 1.17  ^{+ -0.20 }_{ -0.22 }$&$ 0.028  ^{+ 0.000  }_{ -0.000 }$&$ 0.43  ^{+ 0.25  }_{ -0.28 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 6.85  \pm{ 0.97  }$&$ 82.47 ^{+ 2.37  }_{ -6.03 }$&$ 7.6   ^{+ 0.8   }_{ -2.9  }$&$ 0.086  \pm{ 0.004  }$&$ 1354  \pm{ 281   }$&$ 581   \pm{ 7     }$& 2.6   & 1.1  &0.464 & 0.956 \\
K00304.02  & 6029239    & 136.5633  &$    5.51835 ^{+    0.00000 }_{   -0.00000 }$&$ 0.88  ^{+ 0.12  }_{ -0.23 }$&$ 0.006  ^{+ 0.062  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.01  ^{+ 0.23  }_{ -0.01 }$&$ 0.67  \pm{ 3.65  }$&$ 83.09 ^{+ 5.36  }_{ -3.62 }$&$ 5.2   ^{+ 1.1   }_{ -1.7  }$&$ 0.061  \pm{ 0.003  }$&$ 1505  \pm{ 343   }$&$ 29    \pm{ 6     }$& 2.8   & 0.3  &0.006 & 0.140 \\
K00307.01  & 6289257    & 176.2694  &$   19.67423 ^{+    0.00000 }_{   -0.00000 }$&$ 0.74  ^{+ 0.05  }_{ -0.74 }$&$ 0.014  ^{+ 0.001  }_{ -0.000 }$&$ 0.03  ^{+ 0.40  }_{ -0.03 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.83  \pm{ 0.15  }$&$ 88.49 ^{+ 0.73  }_{ -0.19 }$&$ 26.6  ^{+ 1.2   }_{ -6.3  }$&$ 0.153  \pm{ 0.005  }$&$ 765   \pm{ 30    }$&$ 204   \pm{ 11    }$& 3.7   & 1.9  &0.059 & 0.609 \\
K00307.02  & 6289257    & 131.5367  &$    5.21106 ^{+    0.00000 }_{   -0.00000 }$&$ 0.32  ^{+ 0.17  }_{ -0.32 }$&$ 0.009  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 1.16  \pm{ 0.15  }$&$ 88.42 ^{+ 1.58  }_{ -0.86 }$&$ 11.3  ^{+ 0.6   }_{ -2.0  }$&$ 0.062  \pm{ 0.001  }$&$ 1193  \pm{ 46    }$&$ 101   \pm{ 5     }$& 3.3   & 2.0  &0.017 & 0.298 \\
K00312.01  & 7050989    & 175.5857  &$   11.57894 ^{+    0.00000 }_{   -0.00000 }$&$ 0.80  ^{+ 0.10  }_{ -0.06 }$&$ 0.014  ^{+ 0.001  }_{ -0.001 }$&$ 0.32  ^{+ 0.36  }_{ -0.32 }$&$ 0.47  ^{+ 4.52  }_{ -0.47 }$&$ 1.76  \pm{ 0.18  }$&$ 87.68 ^{+ 0.38  }_{ -0.48 }$&$ 19.3  ^{+ 1.1   }_{ -1.7  }$&$ 0.103  \pm{ 0.005  }$&$ 919   \pm{ 35    }$&$ 216   \pm{ 8     }$& 3.0   & 0.4  &0.049 & 0.563 \\
K00312.02  & 7050989    & 131.9683  &$   16.39922 ^{+    0.00000 }_{   -0.00000 }$&$ 0.48  ^{+ 0.24  }_{ -0.48 }$&$ 0.014  ^{+ 0.001  }_{ -0.000 }$&$ 0.53  ^{+ 0.17  }_{ -0.49 }$&$ 0.32  ^{+ 5.66  }_{ -0.32 }$&$ 1.70  \pm{ 0.16  }$&$ 88.90 ^{+ 1.10  }_{ -0.52 }$&$ 23.6  ^{+ 1.2   }_{ -7.3  }$&$ 0.130  \pm{ 0.006  }$&$ 823   \pm{ 33    }$&$ 219   \pm{ 9     }$& 3.5   & 0.5  &0.036 & 0.481 \\
K00313.01  & 7419318    & 177.6356  &$   18.73572 ^{+    0.00000 }_{   -0.00000 }$&$ 0.74  ^{+ 0.22  }_{ -0.47 }$&$ 0.024  ^{+ 0.005  }_{ -0.002 }$&$ 0.00  ^{+ 0.49  }_{ -0.00 }$&$ 0.08  ^{+ 1.41  }_{ -0.08 }$&$ 2.29  \pm{ 0.38  }$&$ 88.69 ^{+ 0.48  }_{ -1.00 }$&$ 32.0  ^{+ 1.4   }_{ -1.8  }$&$ 0.136  \pm{ 0.003  }$&$ 622   \pm{ 20    }$&$ 571   \pm{ 15    }$& 3.2   & 1.0  &0.530 & 0.966 \\
K00313.02  & 7419318    & 179.8861  &$    8.43640 ^{+    0.00000 }_{   -0.00000 }$&$ 0.28  ^{+ 0.17  }_{ -0.28 }$&$ 0.017  ^{+ 0.000  }_{ -0.000 }$&$ 0.02  ^{+ 0.31  }_{ -0.02 }$&$ 0.01  ^{+ 1.62  }_{ -0.01 }$&$ 1.62  \pm{ 0.13  }$&$ 89.15 ^{+ 0.85  }_{ -0.49 }$&$ 19.0  ^{+ 0.7   }_{ -0.7  }$&$ 0.080  \pm{ 0.001  }$&$ 813   \pm{ 19    }$&$ 346   \pm{ 10    }$& 3.3   & 0.3  &0.356 & 0.933 \\
K00314.01  & 7603200    & 177.8521  &$   13.78105 ^{+    0.00000 }_{   -0.00000 }$&$ 0.59  ^{+ 0.41  }_{ -0.04 }$&$ 0.025  ^{+ 0.006  }_{ -0.001 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 0.00  ^{+ 1.10  }_{ -0.00 }$&$ 1.19  \pm{ 0.19  }$&$ 89.10 ^{+ 0.12  }_{ -9.35 }$&$ 40.7  ^{+ 3.3   }_{ -1.3  }$&$ 0.084  \pm{ 0.003  }$&$ 324   \pm{ 68    }$&$ 704   \pm{ 10    }$& 2.3   & 0.4  &0.797 & 0.995 \\
K00314.02  & 7603200    & 171.0047  &$   23.08945 ^{+    0.00000 }_{   -0.00000 }$&$ 0.87  ^{+ 0.13  }_{ -0.02 }$&$ 0.025  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 1.81  }_{ -0.00 }$&$ 1.21  \pm{ 0.11  }$&$ 89.13 ^{+ 0.06  }_{ -0.12 }$&$ 57.1  ^{+ 1.1   }_{ -2.8  }$&$ 0.122  \pm{ 0.004  }$&$ 263   \pm{ 14    }$&$ 532   \pm{ 16    }$& 1.7   & 4.3  &0.699 & 0.991 \\
K00314.03  & 7603200    & 133.5522  &$   10.31202 ^{+    0.00000 }_{   -0.00000 }$&$ 0.76  ^{+ 0.21  }_{ -0.17 }$&$ 0.007  ^{+ 0.014  }_{ -0.001 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.35  \pm{ 0.37  }$&$ 88.70 ^{+ 0.40  }_{ -0.49 }$&$ 33.5  ^{+ 0.7   }_{ -1.3  }$&$ 0.069  \pm{ 0.002  }$&$ 344   \pm{ 18    }$&$ 51    \pm{ 9     }$& 1.5   & 0.5  &0.037 & 0.655 \\
K00316.01  & 8008067    & 137.5880  &$   15.77120 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.10  }_{ -0.03 }$&$ 0.025  ^{+ 0.001  }_{ -0.000 }$&$ 0.09  ^{+ 0.45  }_{ -0.09 }$&$ 0.14  ^{+ 3.64  }_{ -0.14 }$&$ 6.46  \pm{ 0.78  }$&$ 85.61 ^{+ 0.76  }_{ -1.45 }$&$ 11.6  ^{+ 1.1   }_{ -1.2  }$&$ 0.135  \pm{ 0.006  }$&$ 1088  \pm{ 64    }$&$ 533   \pm{ 13    }$& 5.4   & 11.7 &0.398 & 0.971 \\
K00316.02  & 8008067    & 481.2644  &$  157.07021 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.05  }_{ -0.03 }$&$ 0.027  ^{+ 0.182  }_{ -0.003 }$&$ 0.00  ^{+ 0.70  }_{ -0.00 }$&$ 1.29  ^{+ 4.64  }_{ -1.29 }$&$ 6.83  \pm{ 23.47 }$&$ 88.95 ^{+ 0.16  }_{ -0.37 }$&$ 49.7  ^{+ 4.3   }_{ -18.1 }$&$ 0.599  \pm{ 0.036  }$&$ 519   \pm{ 37    }$&$ 540   \pm{ 42    }$& 9.4   & 2.6  &0.057 & 0.751 \\
K00316.03  & 8008067    & 131.7801  &$    7.30569 ^{+    0.00000 }_{   -0.00000 }$&$ 1.02  ^{+ -0.02 }_{ -0.03 }$&$ 0.045  ^{+ 0.236  }_{ -0.021 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 11.09 \pm{ 31.62 }$&$ 80.74 ^{+ 1.68  }_{ -4.97 }$&$ 7.2   ^{+ 0.7   }_{ -1.0  }$&$ 0.081  \pm{ 0.004  }$&$ 1481  \pm{ 120   }$&$ 263   \pm{ 8     }$& 2.1   & 8.3  &0.221 & 0.934 \\
K00321.01  & 8753657    & 170.4543  &$    2.42631 ^{+    0.00000 }_{   -0.00000 }$&$ 0.25  ^{+ 0.18  }_{ -0.25 }$&$ 0.012  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.46  \pm{ 0.26  }$&$ 87.91 ^{+ 2.09  }_{ -1.68 }$&$ 6.8   ^{+ 0.3   }_{ -1.9  }$&$ 0.035  \pm{ 0.001  }$&$ 1401  \pm{ 78    }$&$ 178   \pm{ 3     }$& 2.7   & 0.7  &0.448 & 0.953 \\
K00321.02  & 8753657    & 132.3660  &$    4.62339 ^{+    0.00000 }_{   -0.00000 }$&$ 0.25  ^{+ 0.27  }_{ -0.25 }$&$ 0.007  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.74  \pm{ 0.07  }$&$ 88.75 ^{+ 1.25  }_{ -1.37 }$&$ 11.5  ^{+ 0.6   }_{ -1.2  }$&$ 0.052  \pm{ 0.001  }$&$ 1080  \pm{ 48    }$&$ 61    \pm{ 5     }$& 2.9   & 0.5  &0.011 & 0.213 \\
K00326.01  & 9880467    & 171.0311  &$    8.97350 ^{+    0.00000 }_{   -0.00000 }$&$ 1.18  ^{+ -0.18 }_{ -0.20 }$&$ 0.152  ^{+ 0.046  }_{ -0.060 }$&$ 0.21  ^{+ 0.19  }_{ -0.20 }$&$ 6.29  ^{+ -0.00 }_{ -2.76 }$&$ 182.03 \pm{ 65.21 }$&$ 60.00 ^{+ 0.72  }_{ -0.00 }$&$ 2.0   ^{+ 0.1   }_{ -0.6  }$&$ 0.107  \pm{ 0.003  }$&$ 2046  \pm{ 90    }$&$ 524   \pm{ 38    }$& 8.4   & 9.5  &0.486 & 0.959 \\
K00326.02  & 9880467    & 151.2420  &$  108.52770 ^{+    0.00000 }_{   -0.00000 }$&$ 1.27  ^{+ -0.28 }_{ -0.32 }$&$ 0.290  ^{+ 0.016  }_{ -0.153 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 334.60 \pm{ 107.20 }$&$ 81.14 ^{+ 4.19  }_{ -5.38 }$&$ 10.0  ^{+ 1.2   }_{ -1.9  }$&$ 0.557  \pm{ 0.015  }$&$ 1100  \pm{ 110   }$&$ 327   \pm{ 139   }$& 22.2  & 1.4  &0.486 & 0.959 \\
K00327.01  & 9881662    & 172.6615  &$    3.25428 ^{+    0.00000 }_{   -0.00000 }$&$ 0.37  ^{+ 0.15  }_{ -0.23 }$&$ 0.012  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 0.00  ^{+ 1.12  }_{ -0.00 }$&$ 1.51  \pm{ 0.10  }$&$ 87.43 ^{+ 1.43  }_{ -1.21 }$&$ 8.2   ^{+ 0.3   }_{ -0.5  }$&$ 0.046  \pm{ 0.001  }$&$ 1423  \pm{ 44    }$&$ 158   \pm{ 5     }$& 2.8   & 2.5  &0.425 & 0.949 \\
K00327.02  & 9881662    & 189.6005  &$   91.35250 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.32  }_{ -0.00 }$&$ 0.013  ^{+ 0.001  }_{ -0.010 }$&$ 0.28  ^{+ 0.42  }_{ -0.28 }$&$ 0.19  ^{+ 6.10  }_{ -0.19 }$&$ 1.65  \pm{ 0.73  }$&$ 90.00 ^{+ 0.00  }_{ -0.23 }$&$ 78.3  ^{+ 4.7   }_{ -4.6  }$&$ 0.418  \pm{ 0.021  }$&$ 467   \pm{ 14    }$&$ 206   \pm{ 29    }$& 8.3   & 0.9  &0.043 & 0.526 \\
K00332.01  & 10290666   & 172.0875  &$    5.45851 ^{+    0.00000 }_{   -0.00000 }$&$ 0.18  ^{+ 0.27  }_{ -0.18 }$&$ 0.015  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.49  }_{ -0.00 }$&$ 1.47  \pm{ 0.27  }$&$ 89.00 ^{+ 1.00  }_{ -1.27 }$&$ 13.4  ^{+ 1.4   }_{ -1.5  }$&$ 0.061  \pm{ 0.003  }$&$ 1174  \pm{ 158   }$&$ 254   \pm{ 8     }$& 4.0   & 0.8  &0.160 & 0.826 \\
K00332.02  & 10290666   & 135.3520  &$    6.86687 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 0.006  ^{+ 0.000  }_{ -0.004 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.64  \pm{ 0.24  }$&$ 90.00 ^{+ 0.00  }_{ -0.71 }$&$ 15.2  ^{+ 1.2   }_{ -5.3  }$&$ 0.069  \pm{ 0.003  }$&$ 960   \pm{ 49    }$&$ 46    \pm{ 9     }$& 3.4   & 0.0  &0.004 & 0.084 \\
K00338.01  & 10552611   & 174.5747  &$    7.01062 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.000  ^{+ 0.000  }_{ 0.000  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  \pm{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 15.2  ^{+ 1.2   }_{ -5.3  }$&$ 0.070  \pm{ 0.003  }$&$ 0     \pm{ 0     }$&$ 46    \pm{ 9     }$& 3.4   & 0.5  &0.061 & 0.619 \\
K00338.02  & 10552611   & 132.6397  &$    0.00000 ^{+    0.00000 }_{    0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.000  ^{+ 0.000  }_{ 0.000  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  \pm{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 15.2  ^{+ 1.2   }_{ -5.3  }$&$ 0.000  \pm{ 0.000  }$&$ 0     \pm{ 0     }$&$ 46    \pm{ 9     }$& 3.4   & 0.5  &0.008 & 0.172 \\
K00341.01  & 10878263   & 176.6658  &$   14.34123 ^{+    0.00000 }_{   -0.00000 }$&$ 0.77  ^{+ 0.05  }_{ -0.12 }$&$ 0.030  ^{+ 0.001  }_{ -0.003 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.14  \pm{ 0.28  }$&$ 88.25 ^{+ 0.27  }_{ -0.29 }$&$ 25.3  ^{+ 1.0   }_{ -1.4  }$&$ 0.115  \pm{ 0.002  }$&$ 730   \pm{ 23    }$&$ 872   \pm{ 33    }$& 2.9   & 0.3  &0.031 & 0.445 \\
K00341.02  & 10878263   & 177.6153  &$    4.69961 ^{+    0.00000 }_{   -0.00000 }$&$ 0.49  ^{+ 0.11  }_{ -0.16 }$&$ 0.015  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.11  }_{ -0.00 }$&$ 0.01  ^{+ 2.87  }_{ -0.01 }$&$ 1.56  \pm{ 0.25  }$&$ 87.70 ^{+ 0.79  }_{ -0.70 }$&$ 12.1  ^{+ 0.6   }_{ -0.7  }$&$ 0.055  \pm{ 0.002  }$&$ 1052  \pm{ 39    }$&$ 274   \pm{ 19    }$& 2.6   & 2.2  &0.014 & 0.261 \\
K00343.01  & 10982872   & 170.3356  &$    4.76170 ^{+    0.00000 }_{   -0.00000 }$&$ 0.53  ^{+ 0.17  }_{ -0.45 }$&$ 0.021  ^{+ 0.004  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.49  \pm{ 0.52  }$&$ 86.85 ^{+ 1.55  }_{ -2.18 }$&$ 10.6  ^{+ 1.0   }_{ -2.8  }$&$ 0.054  \pm{ 0.003  }$&$ 1224  \pm{ 112   }$&$ 496   \pm{ 8     }$& 3.3   & 1.3  &0.720 & 0.992 \\
K00343.02  & 10982872   & 170.4966  &$    2.02413 ^{+    0.00000 }_{   -0.00000 }$&$ 0.69  ^{+ 0.22  }_{ -0.25 }$&$ 0.015  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 1.69  \pm{ 0.46  }$&$ 81.55 ^{+ 4.59  }_{ -2.47 }$&$ 4.1   ^{+ 0.4   }_{ -0.0  }$&$ 0.031  \pm{ 0.002  }$&$ 1751  \pm{ 189   }$&$ 234   \pm{ 5     }$& 2.5   & 1.3  &0.487 & 0.979 \\
K00343.03  & 10982872   & 148.6985  &$   41.80925 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.013  ^{+ 0.022  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.34  \pm{ 1.20  }$&$ 90.00 ^{+ -0.00 }_{ -0.00 }$&$ 48.4  ^{+ 2.5   }_{ -18.1 }$&$ 0.229  \pm{ 0.006  }$&$ 537   \pm{ 23    }$&$ 191   \pm{ 26    }$& 6.4   & 0.8  &0.026 & 0.576 \\
K00353.01  & 11566064   & 176.5297  &$  152.10452 ^{+    0.00000 }_{   -0.00000 }$&$ 0.88  ^{+ 0.02  }_{ -0.05 }$&$ 0.062  ^{+ 0.002  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 9.34  \pm{ 1.67  }$&$ 89.46 ^{+ 0.05  }_{ -0.06 }$&$ 89.4  ^{+ 5.1   }_{ -18.5 }$&$ 0.628  \pm{ 0.016  }$&$ 470   \pm{ 19    }$&$ 3385  \pm{ 73    }$& 7.1   & 1.3  &0.629 & 0.977 \\
K00353.02  & 11566064   & 135.0456  &$   30.65268 ^{+    0.00000 }_{   -0.00000 }$&$ 0.74  ^{+ 0.17  }_{ -0.17 }$&$ 0.017  ^{+ 0.001  }_{ -0.001 }$&$ 0.31  ^{+ 0.35  }_{ -0.31 }$&$ 0.47  ^{+ 5.82  }_{ -0.47 }$&$ 2.56  \pm{ 0.49  }$&$ 88.67 ^{+ 0.40  }_{ -0.54 }$&$ 32.0  ^{+ 2.5   }_{ -2.2  }$&$ 0.215  \pm{ 0.011  }$&$ 806   \pm{ 41    }$&$ 320   \pm{ 25    }$& 5.1   & 0.4  &0.051 & 0.572 \\
K00354.01  & 11568987   & 171.5200  &$   15.95995 ^{+    0.00000 }_{   -0.00000 }$&$ 0.06  ^{+ 0.30  }_{ -0.06 }$&$ 0.021  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.94  \pm{ 0.24  }$&$ 89.87 ^{+ 0.13  }_{ -0.49 }$&$ 29.1  ^{+ 1.4   }_{ -3.2  }$&$ 0.119  \pm{ 0.004  }$&$ 730   \pm{ 24    }$&$ 526   \pm{ 17    }$& 4.2   & 3.6  &0.440 & 0.952 \\
K00354.02  & 11568987   & 135.8196  &$    7.37878 ^{+    0.00000 }_{   -0.00000 }$&$ 0.34  ^{+ 0.22  }_{ -0.34 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.04  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 0.91  \pm{ 0.08  }$&$ 88.95 ^{+ 1.05  }_{ -0.66 }$&$ 18.5  ^{+ 0.9   }_{ -1.1  }$&$ 0.071  \pm{ 0.002  }$&$ 914   \pm{ 33    }$&$ 119   \pm{ 11    }$& 2.9   & 1.6  &0.025 & 0.393 \\
K00369.01  & 7175184    & 174.4259  &$    5.88522 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.06  }_{ -0.08 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.22  ^{+ 0.41  }_{ -0.22 }$&$ 0.83  ^{+ 5.40  }_{ -0.83 }$&$ 1.13  \pm{ 0.20  }$&$ 85.77 ^{+ 0.88  }_{ -1.77 }$&$ 11.8  ^{+ 1.2   }_{ -2.7  }$&$ 0.065  \pm{ 0.003  }$&$ 1186  \pm{ 65    }$&$ 108   \pm{ 5     }$& 2.0   & 0.7  &0.226 & 0.879 \\
K00369.02  & 7175184    & 135.5572  &$   10.10465 ^{+    0.00000 }_{   -0.00000 }$&$ 0.86  ^{+ 0.05  }_{ -0.06 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.70  ^{+ -0.00 }_{ -0.25 }$&$ 0.63  ^{+ 5.05  }_{ -0.62 }$&$ 1.11  \pm{ 0.21  }$&$ 87.03 ^{+ 0.55  }_{ -1.34 }$&$ 16.8  ^{+ 1.6   }_{ -3.1  }$&$ 0.098  \pm{ 0.003  }$&$ 1040  \pm{ 192   }$&$ 114   \pm{ 6     }$& 2.3   & 1.2  &0.130 & 0.789 \\
K00370.01  & 8494142    & 203.6467  &$   42.88255 ^{+    0.00000 }_{   -0.00000 }$&$ 0.78  ^{+ 0.03  }_{ -0.04 }$&$ 0.020  ^{+ 0.003  }_{ -0.000 }$&$ 0.00  ^{+ 0.23  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 5.44  \pm{ 0.56  }$&$ 87.98 ^{+ 0.20  }_{ -0.18 }$&$ 21.7  ^{+ 0.9   }_{ -0.9  }$&$ 0.250  \pm{ 0.008  }$&$ 849   \pm{ 26    }$&$ 409   \pm{ 14    }$& 9.8   & 0.6  &0.049 & 0.561 \\
K00370.02  & 8494142    & 151.5320  &$   22.95036 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.01  }_{ -0.01 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.44  \pm{ 0.21  }$&$ 86.25 ^{+ 0.26  }_{ -0.29 }$&$ 14.3  ^{+ 0.6   }_{ -0.6  }$&$ 0.166  \pm{ 0.004  }$&$ 1052  \pm{ 28    }$&$ 124   \pm{ 10    }$& 4.6   & 0.7  &0.087 & 0.705 \\
K00623.01  & 12068975   & 174.0660  &$   10.34968 ^{+    0.00000 }_{   -0.00000 }$&$ 0.76  ^{+ 0.05  }_{ -0.12 }$&$ 0.011  ^{+ 0.002  }_{ -0.001 }$&$ 0.02  ^{+ 0.48  }_{ -0.02 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 1.77  \pm{ 0.25  }$&$ 86.41 ^{+ 0.69  }_{ -0.38 }$&$ 12.9  ^{+ 1.4   }_{ -0.7  }$&$ 0.089  \pm{ 0.002  }$&$ 1113  \pm{ 29    }$&$ 121   \pm{ 6     }$& 4.3   & 1.3  &0.049 & 0.722 \\
K00623.02  & 12068975   & 179.4702  &$   15.67757 ^{+    0.00000 }_{   -0.00000 }$&$ 0.68  ^{+ 0.06  }_{ -0.24 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.11  ^{+ 0.52  }_{ -0.11 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.69  \pm{ 0.19  }$&$ 87.63 ^{+ 0.56  }_{ -0.38 }$&$ 16.6  ^{+ 0.4   }_{ -1.2  }$&$ 0.116  \pm{ 0.002  }$&$ 960   \pm{ 28    }$&$ 115   \pm{ 8     }$& 5.4   & 1.3  &0.035 & 0.643 \\
K00623.03  & 12068975   & 171.4706  &$    5.59935 ^{+    0.00000 }_{   -0.00000 }$&$ 0.69  ^{+ 0.07  }_{ -0.68 }$&$ 0.009  ^{+ 0.000  }_{ -0.000 }$&$ 0.18  ^{+ 0.46  }_{ -0.18 }$&$ 0.63  ^{+ 5.66  }_{ -0.63 }$&$ 1.55  \pm{ 0.10  }$&$ 85.06 ^{+ 2.87  }_{ -0.66 }$&$ 7.8   ^{+ 0.2   }_{ -0.3  }$&$ 0.058  \pm{ 0.001  }$&$ 1378  \pm{ 35    }$&$ 85    \pm{ 4     }$& 3.9   & 1.9  &0.017 & 0.464 \\
K00623.04  & 12068975   & 154.4160  &$   25.20971 ^{+    0.00000 }_{   -0.00000 }$&$ 0.73  ^{+ 0.16  }_{ -0.29 }$&$ 0.008  ^{+ 0.006  }_{ -0.001 }$&$ 0.03  ^{+ 0.66  }_{ -0.03 }$&$ 1.43  ^{+ 4.86  }_{ -1.32 }$&$ 0.84  \pm{ 0.43  }$&$ 88.25 ^{+ 1.75  }_{ -0.77 }$&$ 22.8  ^{+ 10.0  }_{ -2.3  }$&$ 0.156  \pm{ 0.005  }$&$ 799   \pm{ 118   }$&$ 67    \pm{ 10    }$& 5.6   & 0.4  &0.004 & 0.177 \\
K00626.01  & 4478168    & 172.2186  &$   14.58667 ^{+    0.00000 }_{   -0.00000 }$&$ 0.46  ^{+ 0.12  }_{ -0.44 }$&$ 0.018  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.14  \pm{ 0.28  }$&$ 88.92 ^{+ 0.73  }_{ -0.36 }$&$ 22.9  ^{+ 1.9   }_{ -6.3  }$&$ 0.120  \pm{ 0.004  }$&$ 825   \pm{ 37    }$&$ 359   \pm{ 19    }$& 4.1   & 0.5  &0.049 & 0.564 \\
K00626.02  & 4478168    & 132.8298  &$    8.02901 ^{+    0.00000 }_{   -0.00000 }$&$ 0.44  ^{+ 0.20  }_{ -0.44 }$&$ 0.007  ^{+ 0.000  }_{ -0.005 }$&$ 0.04  ^{+ 0.49  }_{ -0.04 }$&$ 0.00  ^{+ 0.07  }_{ -0.00 }$&$ 0.78  \pm{ 0.33  }$&$ 88.49 ^{+ 1.38  }_{ -0.76 }$&$ 15.0  ^{+ 1.3   }_{ -3.9  }$&$ 0.077  \pm{ 0.003  }$&$ 997   \pm{ 47    }$&$ 63    \pm{ 13    }$& 3.4   & 0.4  &0.002 & 0.054 \\
K00627.01  & 4563268    & 176.1730  &$    7.75191 ^{+    0.00000 }_{   -0.00000 }$&$ 0.55  ^{+ 0.06  }_{ -0.12 }$&$ 0.019  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 0.10  ^{+ 6.01  }_{ -0.10 }$&$ 2.42  \pm{ 0.18  }$&$ 87.86 ^{+ 0.54  }_{ -0.36 }$&$ 14.5  ^{+ 0.6   }_{ -1.3  }$&$ 0.082  \pm{ 0.002  }$&$ 1059  \pm{ 35    }$&$ 389   \pm{ 11    }$& 3.5   & 3.3  &0.166 & 0.833 \\
K00627.02  & 4563268    & 132.0230  &$    4.16547 ^{+    0.00000 }_{   -0.00000 }$&$ 0.33  ^{+ 0.15  }_{ -0.33 }$&$ 0.010  ^{+ 0.000  }_{ -0.003 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 0.01  ^{+ 3.59  }_{ -0.01 }$&$ 1.20  \pm{ 0.24  }$&$ 88.09 ^{+ 1.59  }_{ -0.93 }$&$ 9.7   ^{+ 0.4   }_{ -0.6  }$&$ 0.054  \pm{ 0.001  }$&$ 1293  \pm{ 45    }$&$ 108   \pm{ 8     }$& 3.1   & 2.5  &0.004 & 0.101 \\
K00655.01  & 5966154    & 192.0969  &$   25.67210 ^{+    0.00000 }_{   -0.00000 }$&$ 0.38  ^{+ 0.19  }_{ -0.34 }$&$ 0.018  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.20  \pm{ 0.28  }$&$ 89.35 ^{+ 0.44  }_{ -0.36 }$&$ 32.1  ^{+ 1.6   }_{ -10.2 }$&$ 0.173  \pm{ 0.007  }$&$ 709   \pm{ 33    }$&$ 391   \pm{ 15    }$& 5.6   & 0.9  &0.170 & 0.837 \\
K00655.02  & 5966154    & 176.4103  &$  151.88600 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.017  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.15  \pm{ 0.37  }$&$ 90.00 ^{+ -0.00 }_{ -0.21 }$&$ 106.4 ^{+ 5.3   }_{ -9.8  }$&$ 0.573  \pm{ 0.020  }$&$ 398   \pm{ 26    }$&$ 364   \pm{ 36    }$& 11.3  & 0.7  &0.027 & 0.405 \\
K00664.01  & 6442340    & 170.2279  &$   13.13742 ^{+    0.00000 }_{   -0.00000 }$&$ 0.85  ^{+ 0.07  }_{ -0.12 }$&$ 0.016  ^{+ 0.001  }_{ -0.001 }$&$ 0.07  ^{+ 0.55  }_{ -0.07 }$&$ 0.01  ^{+ 1.39  }_{ -0.01 }$&$ 3.73  \pm{ 0.53  }$&$ 85.75 ^{+ 1.94  }_{ -1.28 }$&$ 10.8  ^{+ 1.0   }_{ -3.7  }$&$ 0.111  \pm{ 0.004  }$&$ 1175  \pm{ 90    }$&$ 229   \pm{ 13    }$& 4.9   & 0.1  &0.080 & 0.813 \\
K00664.02  & 6442340    & 133.5821  &$    7.78220 ^{+    0.00000 }_{   -0.00000 }$&$ 1.23  ^{+ -0.23 }_{ -0.34 }$&$ 0.010  ^{+ 0.001  }_{ -0.001 }$&$ 0.51  ^{+ 0.19  }_{ -0.51 }$&$ 0.57  ^{+ 5.72  }_{ -0.56 }$&$ 2.34  \pm{ 0.35  }$&$ 79.80 ^{+ 3.00  }_{ -12.49 }$&$ 7.3   ^{+ 0.7   }_{ -0.7  }$&$ 0.078  \pm{ 0.004  }$&$ 1509  \pm{ 119   }$&$ 94    \pm{ 10    }$& 4.2   & 0.5  &0.033 & 0.633 \\
K00664.03  & 6442340    & 152.0300  &$   23.44194 ^{+    0.00000 }_{   -0.00000 }$&$ 0.81  ^{+ 0.17  }_{ -0.15 }$&$ 0.009  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.22  }_{ -0.00 }$&$ 0.07  ^{+ 0.83  }_{ -0.07 }$&$ 0.94  \pm{ 0.59  }$&$ 87.44 ^{+ 1.39  }_{ -0.92 }$&$ 15.5  ^{+ 2.2   }_{ -4.8  }$&$ 0.162  \pm{ 0.007  }$&$ 934   \pm{ 210   }$&$ 81    \pm{ 18    }$& 6.0   & 0.7  &0.021 & 0.521 \\
K00665.01  & 6685609    & 170.3240  &$    5.86805 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.03  }_{ -0.04 }$&$ 0.023  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 6.20  \pm{ 1.49  }$&$ 79.77 ^{+ 2.09  }_{ -2.21 }$&$ 4.9   ^{+ 0.7   }_{ -0.8  }$&$ 0.075  \pm{ 0.004  }$&$ 1793  \pm{ 136   }$&$ 433   \pm{ 8     }$& 4.3   & 0.2  &0.596 & 0.987 \\
K00665.02  & 6685609    & 133.5707  &$    1.61188 ^{+    0.00000 }_{   -0.00000 }$&$ 0.79  ^{+ 0.06  }_{ -0.18 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.53  ^{+ 0.17  }_{ -0.50 }$&$ 0.84  ^{+ 2.21  }_{ -0.84 }$&$ 2.64  \pm{ 0.35  }$&$ 71.50 ^{+ 4.17  }_{ -3.90 }$&$ 2.5   ^{+ 0.4   }_{ -0.2  }$&$ 0.028  \pm{ 0.001  }$&$ 2553  \pm{ 132   }$&$ 95    \pm{ 4     }$& 3.1   & 0.8  &0.059 & 0.757 \\
K00665.03  & 6685609    & 133.3015  &$    3.07156 ^{+    0.00000 }_{   -0.00000 }$&$ 0.84  ^{+ 0.08  }_{ -0.09 }$&$ 0.009  ^{+ 0.000  }_{ -0.000 }$&$ 0.12  ^{+ 0.46  }_{ -0.12 }$&$ 1.27  ^{+ 4.76  }_{ -1.27 }$&$ 2.45  \pm{ 0.59  }$&$ 76.20 ^{+ 3.16  }_{ -4.30 }$&$ 3.7   ^{+ 0.4   }_{ -0.5  }$&$ 0.045  \pm{ 0.003  }$&$ 2148  \pm{ 171   }$&$ 86    \pm{ 6     }$& 4.2   & 0.3  &0.026 & 0.569 \\
K00678.01  & 7509886    & 172.5935  &$    6.04047 ^{+    0.00000 }_{   -0.00000 }$&$ 1.11  ^{+ -0.12 }_{ -0.14 }$&$ 0.019  ^{+ 0.001  }_{ -0.001 }$&$ 0.16  ^{+ 0.53  }_{ -0.15 }$&$ 0.89  ^{+ 5.24  }_{ -0.89 }$&$ 4.04  \pm{ 0.60  }$&$ 78.25 ^{+ 3.03  }_{ -13.34 }$&$ 6.8   ^{+ 0.8   }_{ -1.2  }$&$ 0.062  \pm{ 0.001  }$&$ 1458  \pm{ 148   }$&$ 245   \pm{ 8     }$& 2.5   & 0.9  &0.405 & 0.945 \\
K00678.02  & 7509886    & 132.0163  &$    4.13855 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.01  }_{ -0.03 }$&$ 0.020  ^{+ 0.005  }_{ -0.001 }$&$ 0.04  ^{+ 0.65  }_{ -0.04 }$&$ 6.14  ^{+ 0.15  }_{ -5.30 }$&$ 4.32  \pm{ 0.92  }$&$ 75.68 ^{+ 4.63  }_{ -4.21 }$&$ 4.6   ^{+ 0.7   }_{ -1.9  }$&$ 0.048  \pm{ 0.001  }$&$ 1722  \pm{ 236   }$&$ 255   \pm{ 7     }$& 2.7   & 1.5  &0.463 & 0.956 \\
K00679.01  & 7515212    & 190.2473  &$   31.80526 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.03  }_{ -0.02 }$&$ 0.020  ^{+ 0.001  }_{ -0.002 }$&$ 0.03  ^{+ 0.57  }_{ -0.03 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 9.29  \pm{ 1.38  }$&$ 85.66 ^{+ 0.63  }_{ -1.42 }$&$ 11.6  ^{+ 0.8   }_{ -5.8  }$&$ 0.242  \pm{ 0.010  }$&$ 1124  \pm{ 89    }$&$ 341   \pm{ 18    }$& 8.9   & 0.7  &0.203 & 0.864 \\
K00679.02  & 7515212    & 139.6350  &$   16.25831 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.01  }_{ -0.08 }$&$ 0.008  ^{+ 0.018  }_{ -0.002 }$&$ 0.08  ^{+ 0.62  }_{ -0.07 }$&$ 1.77  ^{+ 4.52  }_{ -1.59 }$&$ 3.07  \pm{ 4.17  }$&$ 83.46 ^{+ 0.99  }_{ -1.26 }$&$ 8.0   ^{+ 0.9   }_{ -3.0  }$&$ 0.146  \pm{ 0.011  }$&$ 1332  \pm{ 192   }$&$ 47    \pm{ 13    }$& 5.8   & 0.2  &0.003 & 0.077 \\
K00710.01  & 9590976    & 170.9513  &$    5.37485 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.04  }_{ -0.03 }$&$ 0.014  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 6.28  ^{+ 0.01  }_{ -5.43 }$&$ 5.74  \pm{ 2.58  }$&$ 75.63 ^{+ 3.55  }_{ -9.92 }$&$ 3.7   ^{+ 0.9   }_{ -1.3  }$&$ 0.074  \pm{ 0.006  }$&$ 2194  \pm{ 377   }$&$ 148   \pm{ 7     }$& 4.3   & 2.7  &0.288 & 0.953 \\
K00710.02  & 9590976    & 137.9585  &$    8.58604 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.02  }_{ -0.95 }$&$ 0.012  ^{+ 0.001  }_{ -0.006 }$&$ 0.03  ^{+ 0.57  }_{ -0.03 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 5.08  \pm{ 2.64  }$&$ 81.47 ^{+ 8.53  }_{ -3.39 }$&$ 3.5   ^{+ 1.2   }_{ -1.3  }$&$ 0.104  \pm{ 0.007  }$&$ 1643  \pm{ 371   }$&$ 109   \pm{ 9     }$& 3.6   & 1.9  &0.050 & 0.725 \\
K00710.03  & 9590976    & 132.4974  &$    3.88683 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.03  }_{ -0.09 }$&$ 0.009  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 2.20  ^{+ 4.09  }_{ -2.17 }$&$ 5.71  \pm{ 3.05  }$&$ 70.79 ^{+ 7.21  }_{ -6.59 }$&$ 2.1   ^{+ 0.6   }_{ -0.6  }$&$ 0.060  \pm{ 0.005  }$&$ 2564  \pm{ 419   }$&$ 60    \pm{ 6     }$& 3.8   & 1.1  &0.012 & 0.380 \\
K00717.01  & 9873254    & 175.7916  &$   14.70751 ^{+    0.00000 }_{   -0.00000 }$&$ 1.37  ^{+ -0.37 }_{ -0.39 }$&$ 0.019  ^{+ 0.002  }_{ -0.003 }$&$ 0.30  ^{+ 0.38  }_{ -0.30 }$&$ 1.46  ^{+ 4.83  }_{ -1.30 }$&$ 7.43  \pm{ 1.38  }$&$ 78.87 ^{+ 4.69  }_{ -5.69 }$&$ 9.2   ^{+ 3.2   }_{ -1.1  }$&$ 0.135  \pm{ 0.007  }$&$ 1415  \pm{ 230   }$&$ 260   \pm{ 16    }$& 3.9   & 0.4  &0.162 & 0.828 \\
K00717.02  & 9873254    & 132.2130  &$    0.90039 ^{+    0.00000 }_{   -0.00000 }$&$ 0.07  ^{+ 0.66  }_{ -0.07 }$&$ 0.005  ^{+ 0.000  }_{ -0.002 }$&$ 0.56  ^{+ 0.09  }_{ -0.22 }$&$ 1.62  ^{+ 1.79  }_{ -1.32 }$&$ 0.39  \pm{ 0.11  }$&$ 88.96 ^{+ 1.04  }_{ -9.99 }$&$ 1.2   ^{+ 0.4   }_{ -0.5  }$&$ 0.018  \pm{ 0.001  }$&$ 1862  \pm{ 336   }$&$ 32    \pm{ 3     }$& 0.9   & 0.1  &0.016 & 0.287 \\
K00719.01  & 9950612    & 134.8770  &$    9.03420 ^{+    0.00000 }_{   -0.00000 }$&$ 0.65  ^{+ 0.22  }_{ -0.65 }$&$ 0.029  ^{+ 0.001  }_{ -0.006 }$&$ 0.47  ^{+ 0.23  }_{ -0.47 }$&$ 4.68  ^{+ 1.61  }_{ -3.80 }$&$ 2.16  \pm{ 0.31  }$&$ 88.45 ^{+ 1.54  }_{ -0.57 }$&$ 23.7  ^{+ 0.8   }_{ -2.6  }$&$ 0.078  \pm{ 0.002  }$&$ 632   \pm{ 17    }$&$ 526   \pm{ 8     }$& 1.8   & 0.9  &0.634 & 0.989 \\
K00719.02  & 9950612    & 146.9200  &$   28.12230 ^{+    0.00000 }_{   -0.00000 }$&$ 0.32  ^{+ 0.18  }_{ -0.32 }$&$ 0.011  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.82  \pm{ 0.05  }$&$ 89.65 ^{+ 0.35  }_{ -0.17 }$&$ 50.4  ^{+ 2.0   }_{ -5.6  }$&$ 0.167  \pm{ 0.004  }$&$ 431   \pm{ 12    }$&$ 145   \pm{ 14    }$& 3.9   & 0.6  &0.016 & 0.455 \\
K00719.03  & 9950612    & 166.5382  &$   45.90000 ^{+    0.00000 }_{   -0.00000 }$&$ 0.50  ^{+ 0.16  }_{ -0.50 }$&$ 0.012  ^{+ 0.002  }_{ -0.001 }$&$ 0.11  ^{+ 0.52  }_{ -0.11 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.84  \pm{ 0.13  }$&$ 89.61 ^{+ 0.39  }_{ -0.15 }$&$ 70.0  ^{+ 3.1   }_{ -8.7  }$&$ 0.225  \pm{ 0.006  }$&$ 362   \pm{ 11    }$&$ 147   \pm{ 27    }$& 4.2   & 0.2  &0.030 & 0.611 \\
K00719.04  & 9950612    & 133.7840  &$    4.15982 ^{+    0.00000 }_{   -0.00000 }$&$ 0.26  ^{+ 0.47  }_{ -0.26 }$&$ 0.010  ^{+ 0.000  }_{ -0.001 }$&$ 0.38  ^{+ 0.32  }_{ -0.38 }$&$ 0.50  ^{+ 2.56  }_{ -0.50 }$&$ 0.77  \pm{ 0.07  }$&$ 88.95 ^{+ 1.05  }_{ -1.85 }$&$ 13.7  ^{+ 0.5   }_{ -1.1  }$&$ 0.046  \pm{ 0.001  }$&$ 816   \pm{ 29    }$&$ 128   \pm{ 5     }$& 1.7   & 0.2  &0.063 & 0.770 \\
K00972.01  & 11013201   & 261.5394  &$    0.00000 ^{+    0.00000 }_{    0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.000  ^{+ 0.000  }_{ 0.000  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  \pm{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 13.7  ^{+ 0.9   }_{ -1.1  }$&$ 0.000  \pm{ 0.000  }$&$ 0     \pm{ 0     }$&$ 128   \pm{ 5     }$& 1.7   & 4.6  &0.646 & 0.979 \\
K00972.02  & 11013201   & 139.1430  &$    0.00000 ^{+    0.00000 }_{    0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.000  ^{+ 0.000  }_{ 0.000  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  \pm{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 13.7  ^{+ 0.4   }_{ -1.2  }$&$ 0.000  \pm{ 0.000  }$&$ 0     \pm{ 0     }$&$ 128   \pm{ 5     }$& 1.7   & 0.2  &0.037 & 0.487 \\
K01001.01  & 1871056    & 155.7178  &$   40.80686 ^{+    0.00000 }_{   -0.00000 }$&$ 0.49  ^{+ 0.20  }_{ -0.49 }$&$ 0.016  ^{+ 0.001  }_{ -0.003 }$&$ 0.67  ^{+ 0.03  }_{ -0.57 }$&$ 0.01  ^{+ 4.71  }_{ -0.01 }$&$ 5.07  \pm{ 1.18  }$&$ 88.33 ^{+ 1.67  }_{ -0.75 }$&$ 20.3  ^{+ 2.6   }_{ -3.2  }$&$ 0.257  \pm{ 0.015  }$&$ 1007  \pm{ 80    }$&$ 313   \pm{ 28    }$& 13.3  & 1.2  &0.003 & 0.071 \\
K01001.02  & 1871056    & 216.2450  &$  140.09140 ^{+    0.00000 }_{   -0.00000 }$&$ 0.75  ^{+ 0.11  }_{ -0.21 }$&$ 0.017  ^{+ 0.002  }_{ -0.004 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 4.90  \pm{ 1.16  }$&$ 88.93 ^{+ 0.44  }_{ -0.36 }$&$ 43.8  ^{+ 4.7   }_{ -6.6  }$&$ 0.584  \pm{ 0.034  }$&$ 651   \pm{ 61    }$&$ 288   \pm{ 53    }$& 18.5  & 0.3  &0.013 & 0.242 \\
K01151.01  & 8280511    & 134.8157  &$    5.21781 ^{+    0.00000 }_{   -0.00000 }$&$ 0.91  ^{+ 0.01  }_{ -0.03 }$&$ 0.011  ^{+ 0.000  }_{ -0.002 }$&$ 0.03  ^{+ 0.41  }_{ -0.03 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 2.92  \pm{ 0.37  }$&$ 79.63 ^{+ 0.97  }_{ -1.12 }$&$ 5.0   ^{+ 0.4   }_{ -0.3  }$&$ 0.058  \pm{ 0.002  }$&$ 1704  \pm{ 62    }$&$ 97    \pm{ 9     }$& 3.6   & 1.0  &0.018 & 0.472 \\
K01151.02  & 8280511    & 135.7436  &$    7.41105 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.03  }_{ -0.04 }$&$ 0.012  ^{+ 0.000  }_{ -0.001 }$&$ 0.06  ^{+ 0.64  }_{ -0.06 }$&$ 1.10  ^{+ 5.19  }_{ -1.10 }$&$ 3.26  \pm{ 0.50  }$&$ 81.12 ^{+ 0.59  }_{ -5.79 }$&$ 6.4   ^{+ 0.4   }_{ -0.4  }$&$ 0.074  \pm{ 0.003  }$&$ 1524  \pm{ 53    }$&$ 119   \pm{ 10    }$& 3.7   & 0.6  &0.066 & 0.779 \\
K01151.03  & 8280511    & 135.4660  &$    5.24972 ^{+    0.00000 }_{   -0.00000 }$&$ 0.99  ^{+ 0.00  }_{ -0.05 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.05  ^{+ 0.60  }_{ -0.05 }$&$ 1.64  ^{+ 4.65  }_{ -1.56 }$&$ 2.18  \pm{ 0.55  }$&$ 79.53 ^{+ 2.32  }_{ -6.52 }$&$ 4.9   ^{+ 0.5   }_{ -0.7  }$&$ 0.059  \pm{ 0.003  }$&$ 1630  \pm{ 148   }$&$ 59    \pm{ 9     }$& 2.6   & 1.0  &0.009 & 0.317 \\
K01151.04  & 8280511    & 146.6500  &$   17.45337 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.05  }_{ -0.03 }$&$ 0.011  ^{+ 0.057  }_{ -0.001 }$&$ 0.03  ^{+ 0.64  }_{ -0.03 }$&$ 0.10  ^{+ 1.50  }_{ -0.10 }$&$ 3.29  \pm{ 8.66  }$&$ 85.14 ^{+ 0.95  }_{ -0.67 }$&$ 10.0  ^{+ 0.8   }_{ -0.6  }$&$ 0.131  \pm{ 0.007  }$&$ 1138  \pm{ 63    }$&$ 92    \pm{ 16    }$& 4.2   & 0.1  &0.007 & 0.254 \\
K01151.05  & 8280511    & 134.7589  &$   21.72069 ^{+    0.00000 }_{   -0.00000 }$&$ 0.70  ^{+ 0.29  }_{ -0.33 }$&$ 0.008  ^{+ 0.001  }_{ -0.006 }$&$ 0.35  ^{+ 0.35  }_{ -0.35 }$&$ 0.11  ^{+ 1.31  }_{ -0.11 }$&$ 0.66  \pm{ 0.29  }$&$ 88.95 ^{+ 0.62  }_{ -3.18 }$&$ 39.0  ^{+ 3.6   }_{ -4.6  }$&$ 0.138  \pm{ 0.004  }$&$ 621   \pm{ 107   }$&$ 68    \pm{ 18    }$& 3.2   & 2.0  &0.008 & 0.295 \\
K01175.01  & 10350571   & 142.9750  &$   31.59300 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.12  }_{ -0.00 }$&$ 2.34  \pm{ 0.37  }$&$ 90.00 ^{+ -0.00 }_{ -0.00 }$&$ 21.2  ^{+ 1.6   }_{ -1.1  }$&$ 0.192  \pm{ 0.007  }$&$ 811   \pm{ 32    }$&$ 152   \pm{ 26    }$& 11.5  & 0.6  &0.016 & 0.283 \\
K01175.02  & 10350571   & 133.6877  &$   17.15710 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 2.15  \pm{ 0.32  }$&$ 90.00 ^{+ -0.00 }_{ -0.00 }$&$ 13.8  ^{+ 0.7   }_{ -1.0  }$&$ 0.127  \pm{ 0.005  }$&$ 989   \pm{ 35    }$&$ 127   \pm{ 19    }$& 9.3   & 0.4  &0.015 & 0.281 \\
K01215.01  & 3939150    & 142.0971  &$   17.32440 ^{+    0.00000 }_{   -0.00000 }$&$ 0.81  ^{+ 0.06  }_{ -0.08 }$&$ 0.016  ^{+ 0.000  }_{ -0.001 }$&$ 0.05  ^{+ 0.38  }_{ -0.05 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 4.58  \pm{ 0.56  }$&$ 85.38 ^{+ 0.94  }_{ -1.21 }$&$ 10.4  ^{+ 1.1   }_{ -2.2  }$&$ 0.135  \pm{ 0.004  }$&$ 1241  \pm{ 95    }$&$ 241   \pm{ 17    }$& 8.1   & 1.2  &0.062 & 0.621 \\
K01215.02  & 3939150    & 145.3899  &$   33.00590 ^{+    0.00000 }_{   -0.00000 }$&$ 1.41  ^{+ -0.50 }_{ -0.52 }$&$ 0.012  ^{+ 0.010  }_{ -0.010 }$&$ 0.02  ^{+ 0.02  }_{ -0.01 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 1.18  \pm{ 1.35  }$&$ 85.61 ^{+ 1.88  }_{ -0.47 }$&$ 19.2  ^{+ 20.7  }_{ -3.7  }$&$ 0.209  \pm{ 0.009  }$&$ 920   \pm{ 290   }$&$ 0     \pm{ 29    }$& 0.0   & 1.3  &0.054 & 0.588 \\
K01221.01  & 3640905    & 138.5145  &$   30.16012 ^{+    0.00000 }_{   -0.00000 }$&$ 0.72  ^{+ 0.10  }_{ -0.09 }$&$ 0.013  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.72  \pm{ 0.31  }$&$ 88.03 ^{+ 0.30  }_{ -0.65 }$&$ 21.6  ^{+ 0.7   }_{ -1.4  }$&$ 0.196  \pm{ 0.004  }$&$ 743   \pm{ 27    }$&$ 177   \pm{ 18    }$& 7.8   & 0.9  &0.117 & 0.768 \\
K01221.02  & 3640905    & 152.3420  &$   51.08020 ^{+    0.00000 }_{   -0.00000 }$&$ 0.54  ^{+ 0.19  }_{ -0.54 }$&$ 0.010  ^{+ 0.001  }_{ -0.008 }$&$ 0.44  ^{+ 0.26  }_{ -0.44 }$&$ 0.00  ^{+ 0.63  }_{ -0.00 }$&$ 2.09  \pm{ 0.95  }$&$ 88.94 ^{+ 1.06  }_{ -0.43 }$&$ 30.1  ^{+ 1.6   }_{ -2.0  }$&$ 0.276  \pm{ 0.007  }$&$ 632   \pm{ 22    }$&$ 127   \pm{ 24    }$& 10.9  & 1.0  &0.029 & 0.429 \\
K01241.01  & 6448890    & 147.0928  &$   21.40505 ^{+    0.00000 }_{   -0.00000 }$&$ 1.90  ^{+ -0.90 }_{ -0.94 }$&$ 0.024  ^{+ 0.001  }_{ -0.002 }$&$ 0.56  ^{+ 0.14  }_{ -0.54 }$&$ 0.72  ^{+ 5.57  }_{ -0.72 }$&$ 18.82 \pm{ 3.59  }$&$ 60.00 ^{+ 16.18 }_{ -0.00 }$&$ 4.5   ^{+ 0.5   }_{ -2.2  }$&$ 0.160  \pm{ 0.005  }$&$ 1673  \pm{ 236   }$&$ 415   \pm{ 26    }$& 11.5  & 0.6  &0.104 & 0.745 \\
K01241.02  & 6448890    & 135.5589  &$   10.50343 ^{+    0.00000 }_{   -0.00000 }$&$ 0.66  ^{+ 0.19  }_{ -0.66 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 0.00  ^{+ 0.57  }_{ -0.00 }$&$ 7.44  \pm{ 2.95  }$&$ 81.72 ^{+ 8.28  }_{ -8.20 }$&$ 2.5   ^{+ 0.8   }_{ -1.1  }$&$ 0.099  \pm{ 0.003  }$&$ 1526  \pm{ 463   }$&$ 133   \pm{ 19    }$& 13.7  & 0.7  &0.092 & 0.716 \\
K01316.01  & 10794087   & 138.3401  &$    7.64951 ^{+    0.00000 }_{   -0.00000 }$&$ 0.57  ^{+ 0.12  }_{ -0.24 }$&$ 0.007  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.37  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.73  \pm{ 0.30  }$&$ 85.64 ^{+ 1.59  }_{ -1.51 }$&$ 7.6   ^{+ 0.5   }_{ -0.6  }$&$ 0.083  \pm{ 0.006  }$&$ 1389  \pm{ 67    }$&$ 54    \pm{ 6     }$& 6.5   & 1.5  &0.086 & 0.701 \\
K01316.02  & 10794087   & 143.3790  &$   12.37679 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.06  }_{ -0.07 }$&$ 0.004  ^{+ 0.008  }_{ -0.001 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 1.05  \pm{ 1.30  }$&$ 84.36 ^{+ 0.54  }_{ -1.09 }$&$ 10.0  ^{+ 1.1   }_{ -1.3  }$&$ 0.108  \pm{ 0.008  }$&$ 1231  \pm{ 134   }$&$ 13    \pm{ 7     }$& 3.9   & 0.3  &0.038 & 0.495 \\
K01445.01  & 11336883   & 135.6794  &$    7.16888 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.29  }_{ -0.00 }$&$ 0.00  ^{+ 4.10  }_{ -0.00 }$&$ 1.29  \pm{ 0.25  }$&$ 90.00 ^{+ -0.00 }_{ -0.00 }$&$ 13.0  ^{+ 0.9   }_{ -1.0  }$&$ 0.079  \pm{ 0.002  }$&$ 1139  \pm{ 49    }$&$ 110   \pm{ 7     }$& 4.3   & 0.9  &0.097 & 0.842 \\
K01445.02  & 11336883   & 142.1590  &$   54.34430 ^{+    0.00000 }_{   -0.00000 }$&$ 0.62  ^{+ 0.38  }_{ -0.58 }$&$ 0.005  ^{+ 0.003  }_{ -0.003 }$&$ 0.32  ^{+ 0.38  }_{ -0.31 }$&$ 0.17  ^{+ 6.12  }_{ -0.16 }$&$ 0.63  \pm{ 0.36  }$&$ 89.35 ^{+ 0.62  }_{ -0.73 }$&$ 56.6  ^{+ 5.5   }_{ -4.0  }$&$ 0.293  \pm{ 0.009  }$&$ 550   \pm{ 28    }$&$ 33    \pm{ 20    }$& 5.8   & 1.1  &0.005 & 0.215 \\
K01445.03  & 11336883   & 150.8360  &$   20.01960 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.003  ^{+ 0.001  }_{ -0.001 }$&$ 0.01  ^{+ 0.54  }_{ -0.01 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.38  \pm{ 0.12  }$&$ 90.00 ^{+ -0.00 }_{ -0.21 }$&$ 27.1  ^{+ 1.3   }_{ -6.7  }$&$ 0.150  \pm{ 0.008  }$&$ 775   \pm{ 30    }$&$ 10    \pm{ 13    }$& 5.4   & 0.3  &0.006 & 0.225 \\
K01525.01  & 7869917    & 133.5535  &$    7.71468 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.02  }_{ -0.01 }$&$ 0.016  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.65  }_{ -0.00 }$&$ 5.57  ^{+ 0.72  }_{ -4.92 }$&$ 6.22  \pm{ 0.53  }$&$ 80.62 ^{+ 3.56  }_{ -2.33 }$&$ 5.7   ^{+ 0.2   }_{ -0.3  }$&$ 0.097  \pm{ 0.003  }$&$ 1914  \pm{ 85    }$&$ 210   \pm{ 9     }$& 4.6   & 0.2  &0.476 & 0.958 \\
K01525.02  & 7869917    & 138.2671  &$   11.80609 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.02  }_{ -0.35 }$&$ 0.012  ^{+ 0.000  }_{ -0.002 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.34  ^{+ 5.92  }_{ -0.34 }$&$ 5.07  \pm{ 1.27  }$&$ 82.36 ^{+ 5.80  }_{ -1.97 }$&$ 6.4   ^{+ 0.7   }_{ -1.1  }$&$ 0.130  \pm{ 0.007  }$&$ 1729  \pm{ 620   }$&$ 112   \pm{ 11    }$& 4.9   & 0.8  &0.095 & 0.723 \\
K01534.01  & 4741126    & 146.9846  &$   20.42226 ^{+    0.00000 }_{   -0.00000 }$&$ 0.91  ^{+ 0.02  }_{ -0.06 }$&$ 0.015  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.17  }_{ -0.00 }$&$ 0.01  ^{+ 2.62  }_{ -0.01 }$&$ 6.41  \pm{ 0.72  }$&$ 85.24 ^{+ 1.08  }_{ -0.64 }$&$ 9.8   ^{+ 0.4   }_{ -0.3  }$&$ 0.182  \pm{ 0.006  }$&$ 1291  \pm{ 89    }$&$ 191   \pm{ 16    }$& 6.5   & 1.0  &0.038 & 0.499 \\
K01534.02  & 4741126    & 138.2340  &$    7.63861 ^{+    0.00000 }_{   -0.00000 }$&$ 0.69  ^{+ 0.22  }_{ -0.69 }$&$ 0.008  ^{+ 0.001  }_{ -0.006 }$&$ 0.38  ^{+ 0.32  }_{ -0.03 }$&$ 0.00  ^{+ 0.13  }_{ -0.00 }$&$ 3.35  \pm{ 1.57  }$&$ 87.02 ^{+ 2.98  }_{ -11.85 }$&$ 5.2   ^{+ 0.2   }_{ -0.2  }$&$ 0.094  \pm{ 0.002  }$&$ 1163  \pm{ 277   }$&$ 68    \pm{ 10    }$& 3.3   & 0.8  &0.005 & 0.119 \\
K01613.01  & 6268648    & 141.0860  &$   15.86621 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.05  }_{ -0.05 }$&$ 0.010  ^{+ 0.003  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.92  \pm{ 1.06  }$&$ 84.85 ^{+ 1.70  }_{ -2.74 }$&$ 10.5  ^{+ 2.5   }_{ -2.0  }$&$ 0.133  \pm{ 0.012  }$&$ 1192  \pm{ 187   }$&$ 75    \pm{ 6     }$& 4.4   & 0.8  &0.021 & 0.346 \\
K01613.02  & 6268648    & 196.7260  &$   94.09329 ^{+    0.00000 }_{   -0.00000 }$&$ 0.78  ^{+ 0.21  }_{ -0.51 }$&$ 0.008  ^{+ 0.002  }_{ -0.002 }$&$ 0.01  ^{+ 0.59  }_{ -0.01 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.12  \pm{ 1.12  }$&$ 88.81 ^{+ 1.00  }_{ -0.85 }$&$ 35.6  ^{+ 37.7  }_{ -8.7  }$&$ 0.434  \pm{ 0.036  }$&$ 603   \pm{ 211   }$&$ 63    \pm{ 17    }$& 12.0  & 1.2  &0.003 & 0.061 \\
K01628.01  & 6975129    & 147.1029  &$   19.74747 ^{+    0.00000 }_{   -0.00000 }$&$ 0.81  ^{+ 0.03  }_{ -0.06 }$&$ 0.022  ^{+ 0.000  }_{ -0.002 }$&$ 0.01  ^{+ 0.46  }_{ -0.01 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.89  \pm{ 0.24  }$&$ 88.29 ^{+ 0.23  }_{ -0.20 }$&$ 27.0  ^{+ 1.2   }_{ -1.3  }$&$ 0.155  \pm{ 0.004  }$&$ 788   \pm{ 27    }$&$ 446   \pm{ 16    }$& 3.4   & 1.2  &0.149 & 0.813 \\
K01628.02  & 6975129    & 132.0945  &$    1.77243 ^{+    0.00000 }_{   -0.00000 }$&$ 0.25  ^{+ 0.22  }_{ -0.25 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.15  ^{+ 0.54  }_{ -0.15 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.88  \pm{ 0.17  }$&$ 87.38 ^{+ 2.62  }_{ -2.35 }$&$ 5.6   ^{+ 0.3   }_{ -0.4  }$&$ 0.029  \pm{ 0.001  }$&$ 1752  \pm{ 70    }$&$ 67    \pm{ 4     }$& 2.4   & 1.8  &0.027 & 0.408 \\
K01692.01  & 6616218    & 137.2639  &$    5.96040 ^{+    0.00000 }_{   -0.00000 }$&$ 0.51  ^{+ 0.06  }_{ -0.19 }$&$ 0.026  ^{+ 0.007  }_{ -0.001 }$&$ 0.00  ^{+ 0.39  }_{ -0.00 }$&$ 0.14  ^{+ 4.57  }_{ -0.14 }$&$ 2.73  \pm{ 0.39  }$&$ 88.00 ^{+ 0.71  }_{ -0.30 }$&$ 14.2  ^{+ 0.3   }_{ -1.3  }$&$ 0.064  \pm{ 0.001  }$&$ 955   \pm{ 19    }$&$ 777   \pm{ 9     }$& 2.8   & 0.9  &0.865 & 0.994 \\
K01692.02  & 6616218    & 133.3133  &$    2.46110 ^{+    0.00000 }_{   -0.00000 }$&$ 0.30  ^{+ 0.21  }_{ -0.30 }$&$ 0.007  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.31  }_{ -0.00 }$&$ 0.78  \pm{ 0.04  }$&$ 87.83 ^{+ 2.16  }_{ -1.43 }$&$ 7.9   ^{+ 0.2   }_{ -0.3  }$&$ 0.036  \pm{ 0.000  }$&$ 1283  \pm{ 32    }$&$ 68    \pm{ 5     }$& 2.2   & 0.7  &0.021 & 0.346 \\
K01779.01  & 9909735    & 134.0812  &$    4.66272 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.02  }_{ -0.02 }$&$ 0.043  ^{+ 0.000  }_{ -0.003 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 6.15  ^{+ 0.14  }_{ -5.43 }$&$ 8.97  \pm{ 0.88  }$&$ 81.60 ^{+ 0.90  }_{ -0.73 }$&$ 6.1   ^{+ 0.4   }_{ -0.3  }$&$ 0.055  \pm{ 0.002  }$&$ 1537  \pm{ 65    }$&$ 1589  \pm{ 10    }$& 3.1   & 0.8  &0.635 & 0.978 \\
K01779.02  & 9909735    & 133.0899  &$   11.81502 ^{+    0.00000 }_{   -0.00000 }$&$ 1.04  ^{+ -0.04 }_{ -0.10 }$&$ 0.036  ^{+ 0.000  }_{ -0.007 }$&$ 0.13  ^{+ 0.42  }_{ -0.13 }$&$ 0.81  ^{+ 5.48  }_{ -0.81 }$&$ 6.15  \pm{ 1.34  }$&$ 85.04 ^{+ 0.82  }_{ -6.34 }$&$ 12.5  ^{+ 0.7   }_{ -1.6  }$&$ 0.099  \pm{ 0.004  }$&$ 1095  \pm{ 96    }$&$ 986   \pm{ 17    }$& 3.0   & 1.4  &0.169 & 0.835 \\
K01781.01  & 11551692   & 135.2206  &$    7.83445 ^{+    0.00000 }_{   -0.00000 }$&$ 0.58  ^{+ 0.06  }_{ -0.01 }$&$ 0.048  ^{+ 0.002  }_{ -0.002 }$&$ 0.59  ^{+ 0.11  }_{ -0.03 }$&$ 4.47  ^{+ 0.25  }_{ -0.29 }$&$ 4.22  \pm{ 0.20  }$&$ 88.32 ^{+ 0.14  }_{ -0.12 }$&$ 19.8  ^{+ 0.3   }_{ -0.5  }$&$ 0.073  \pm{ 0.001  }$&$ 740   \pm{ 14    }$&$ 1923  \pm{ 10    }$& 3.2   & 3.5  &0.995 & 1.000 \\
K01781.02  & 11551692   & 137.1027  &$    3.00516 ^{+    0.00000 }_{   -0.00000 }$&$ 0.55  ^{+ 0.12  }_{ -0.12 }$&$ 0.031  ^{+ 0.001  }_{ -0.007 }$&$ 0.70  ^{+ -0.02 }_{ -0.22 }$&$ 4.71  ^{+ 0.00  }_{ -4.69 }$&$ 2.74  \pm{ 0.37  }$&$ 86.89 ^{+ 0.34  }_{ -1.20 }$&$ 10.1  ^{+ 0.1   }_{ -0.5  }$&$ 0.039  \pm{ 0.000  }$&$ 1040  \pm{ 19    }$&$ 673   \pm{ 5     }$& 2.3   & 0.9  &0.979 & 1.000 \\
K01781.03  & 11551692   & 151.8476  &$   58.02126 ^{+    0.00000 }_{   -0.00000 }$&$ 0.70  ^{+ 0.04  }_{ -0.69 }$&$ 0.035  ^{+ 0.001  }_{ -0.002 }$&$ 0.17  ^{+ 0.53  }_{ -0.17 }$&$ 5.53  ^{+ 0.76  }_{ -4.93 }$&$ 3.06  \pm{ 0.19  }$&$ 89.46 ^{+ 0.08  }_{ -0.06 }$&$ 73.0  ^{+ 2.6   }_{ -3.4  }$&$ 0.278  \pm{ 0.003  }$&$ 385   \pm{ 9     }$&$ 1186  \pm{ 37    }$& 4.5   & 1.2  &0.598 & 0.987 \\
           &            & 0.0000    &$   58.02126 ^{+    0.00000 }_{   -0.00000 }$&$ 0.70  ^{+ 0.04  }_{ -0.69 }$&$ 0.035  ^{+ 0.001  }_{ -0.002 }$&$ 0.17  ^{+ 0.53  }_{ -0.17 }$&$ 5.53  ^{+ 0.76  }_{ -4.93 }$&$ 3.06  \pm{ 0.19  }$&$ 89.46 ^{+ 0.08  }_{ -0.06 }$&$ 73.0  ^{+ 2.6   }_{ -3.4  }$&$ 0.278  \pm{ 0.003  }$&$ 385   \pm{ 9     }$&$ 1186  \pm{ 37    }$& 4.5   & 1.2  &\nodata & \nodata \\
K01806.02  & 9529744    & 138.2171  &$   17.93497 ^{+    0.00000 }_{   -0.00000 }$&$ 1.93  ^{+ -0.93 }_{ -1.05 }$&$ 0.013  ^{+ 0.001  }_{ -0.001 }$&$ 0.70  ^{+ -0.00 }_{ -0.58 }$&$ 0.29  ^{+ 6.00  }_{ -0.29 }$&$ 1.45  \pm{ 0.32  }$&$ 77.62 ^{+ 7.61  }_{ -2.40 }$&$ 10.2  ^{+ 4.4   }_{ -1.1  }$&$ 0.134  \pm{ 0.009  }$&$ 1417  \pm{ 112   }$&$ 153   \pm{ 19    }$& 5.5   & 3.1  &\nodata & \nodata \\
K01806.03  & 9529744    & 137.6755  &$    8.37167 ^{+    0.00000 }_{   -0.00000 }$&$ 1.60  ^{+ -0.61 }_{ -0.85 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.51  ^{+ 0.19  }_{ -0.13 }$&$ 1.13  ^{+ 4.84  }_{ -0.83 }$&$ 1.04  \pm{ 0.37  }$&$ 73.36 ^{+ 5.03  }_{ -6.45 }$&$ 6.1   ^{+ 1.6   }_{ -0.7  }$&$ 0.081  \pm{ 0.005  }$&$ 1799  \pm{ 97    }$&$ 79    \pm{ 12    }$& 4.2   & 4.1  &\nodata & \nodata \\
K01809.01  & 8240797    & 144.5235  &$   13.09392 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.01  }_{ -0.96 }$&$ 0.024  ^{+ 0.000  }_{ -0.006 }$&$ 0.00  ^{+ 0.50  }_{ -0.00 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 6.08  \pm{ 1.56  }$&$ 86.04 ^{+ 3.96  }_{ -2.01 }$&$ 9.2   ^{+ 1.5   }_{ -5.5  }$&$ 0.114  \pm{ 0.009  }$&$ 955   \pm{ 306   }$&$ 391   \pm{ 9     }$& 2.6   & 1.4  &0.459 & 0.955 \\
K01809.02  & 8240797    & 132.6958  &$    4.91538 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.02  }_{ -0.04 }$&$ 0.018  ^{+ 0.002  }_{ -0.003 }$&$ 0.03  ^{+ 0.51  }_{ -0.03 }$&$ 0.00  ^{+ 0.61  }_{ -0.00 }$&$ 4.53  \pm{ 1.57  }$&$ 77.23 ^{+ 10.13 }_{ -5.29 }$&$ 5.0   ^{+ 0.8   }_{ -1.0  }$&$ 0.061  \pm{ 0.005  }$&$ 1785  \pm{ 277   }$&$ 228   \pm{ 5     }$& 3.2   & 1.1  &0.259 & 0.897 \\
K01824.01  & 2989404    & 134.6430  &$    3.55380 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.04  }_{ -0.02 }$&$ 0.015  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.62  }_{ -0.00 }$&$ 0.75  ^{+ 3.60  }_{ -0.75 }$&$ 3.73  \pm{ 0.63  }$&$ 77.65 ^{+ 2.75  }_{ -3.90 }$&$ 4.2   ^{+ 0.2   }_{ -0.2  }$&$ 0.048  \pm{ 0.002  }$&$ 2037  \pm{ 75    }$&$ 184   \pm{ 5     }$& 3.1   & 0.5  &0.190 & 0.854 \\
K01824.02  & 2989404    & 136.0502  &$    1.67834 ^{+    0.00000 }_{   -0.00000 }$&$ 0.91  ^{+ 0.03  }_{ -0.07 }$&$ 0.013  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.47  }_{ -0.00 }$&$ 0.00  ^{+ 1.24  }_{ -0.00 }$&$ 3.59  \pm{ 0.53  }$&$ 68.68 ^{+ 5.15  }_{ -3.54 }$&$ 2.5   ^{+ 0.2   }_{ -0.2  }$&$ 0.029  \pm{ 0.001  }$&$ 2597  \pm{ 160   }$&$ 141   \pm{ 3     }$& 2.5   & 0.3  &0.178 & 0.844 \\
K01909.01  & 10130039   & 133.9557  &$   12.75808 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.01  }_{ -0.02 }$&$ 0.016  ^{+ 0.000  }_{ -0.000 }$&$ 0.03  ^{+ 0.67  }_{ -0.03 }$&$ 0.00  ^{+ 0.83  }_{ -0.00 }$&$ 5.51  \pm{ 0.62  }$&$ 83.71 ^{+ 0.94  }_{ -0.48 }$&$ 8.3   ^{+ 0.4   }_{ -0.6  }$&$ 0.126  \pm{ 0.004  }$&$ 1379  \pm{ 70    }$&$ 190   \pm{ 9     }$& 4.5   & 0.4  &0.194 & 0.923 \\
K01909.02  & 10130039   & 131.4909  &$    5.47037 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.01  }_{ -0.02 }$&$ 0.012  ^{+ 0.001  }_{ -0.000 }$&$ 0.05  ^{+ 0.23  }_{ -0.05 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.94  \pm{ 0.46  }$&$ 78.76 ^{+ 2.08  }_{ -1.03 }$&$ 4.5   ^{+ 0.3   }_{ -0.1  }$&$ 0.070  \pm{ 0.003  }$&$ 1838  \pm{ 82    }$&$ 104   \pm{ 6     }$& 3.3   & 0.2  &0.053 & 0.736 \\
K01909.03  & 10130039   & 145.5671  &$   25.09858 ^{+    0.00000 }_{   -0.00000 }$&$ 1.63  ^{+ -0.64 }_{ -0.65 }$&$ 0.016  ^{+ 0.001  }_{ -0.002 }$&$ 0.54  ^{+ 0.16  }_{ -0.53 }$&$ 0.40  ^{+ 1.73  }_{ -0.40 }$&$ 1.83  \pm{ 1.41  }$&$ 83.36 ^{+ 2.96  }_{ -7.82 }$&$ 13.3  ^{+ 1.8   }_{ -1.4  }$&$ 0.182  \pm{ 0.014  }$&$ 1083  \pm{ 98    }$&$ 177   \pm{ 13    }$& 3.2   & 0.2  &0.097 & 0.843 \\
K01929.01  & 10136549   & 132.8155  &$    9.69303 ^{+    0.00000 }_{   -0.00000 }$&$ 0.80  ^{+ 0.08  }_{ -0.06 }$&$ 0.012  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.42  }_{ -0.00 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 2.75  \pm{ 0.33  }$&$ 84.50 ^{+ 1.05  }_{ -1.26 }$&$ 9.3   ^{+ 0.4   }_{ -0.6  }$&$ 0.088  \pm{ 0.003  }$&$ 1349  \pm{ 68    }$&$ 140   \pm{ 9     }$& 5.5   & 0.7  &0.127 & 0.784 \\
K01929.02  & 10136549   & 133.0093  &$    3.29274 ^{+    0.00000 }_{   -0.00000 }$&$ 0.61  ^{+ 0.12  }_{ -0.27 }$&$ 0.009  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 1.83  \pm{ 0.31  }$&$ 82.12 ^{+ 3.45  }_{ -2.54 }$&$ 4.8   ^{+ 0.5   }_{ -0.4  }$&$ 0.043  \pm{ 0.001  }$&$ 1829  \pm{ 116   }$&$ 80    \pm{ 5     }$& 4.6   & 0.3  &0.124 & 0.779 \\
K01930.01  & 5511081    & 138.7478  &$   13.72686 ^{+    0.00000 }_{   -0.00000 }$&$ 0.41  ^{+ 0.14  }_{ -0.41 }$&$ 0.013  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.79  \pm{ 0.28  }$&$ 88.21 ^{+ 1.79  }_{ -0.76 }$&$ 12.5  ^{+ 0.9   }_{ -1.0  }$&$ 0.115  \pm{ 0.004  }$&$ 1080  \pm{ 53    }$&$ 190   \pm{ 11    }$& 7.5   & 1.5  &0.134 & 0.886 \\
K01930.02  & 5511081    & 137.0438  &$   24.31058 ^{+    0.00000 }_{   -0.00000 }$&$ 0.41  ^{+ 0.14  }_{ -0.41 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.46  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.70  \pm{ 0.20  }$&$ 88.76 ^{+ 1.24  }_{ -0.46 }$&$ 18.0  ^{+ 0.8   }_{ -1.3  }$&$ 0.168  \pm{ 0.005  }$&$ 898   \pm{ 34    }$&$ 184   \pm{ 15    }$& 9.0   & 1.8  &0.061 & 0.765 \\
K01930.03  & 5511081    & 143.5344  &$   44.43150 ^{+    0.00000 }_{   -0.00000 }$&$ 0.50  ^{+ 0.12  }_{ -0.50 }$&$ 0.015  ^{+ 0.000  }_{ -0.003 }$&$ 0.02  ^{+ 0.58  }_{ -0.02 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.17  \pm{ 0.45  }$&$ 89.00 ^{+ 1.00  }_{ -0.29 }$&$ 27.0  ^{+ 1.5   }_{ -2.0  }$&$ 0.253  \pm{ 0.006  }$&$ 732   \pm{ 30    }$&$ 243   \pm{ 21    }$& 10.5  & 1.6  &0.053 & 0.739 \\
K01930.04  & 5511081    & 132.3931  &$    9.34131 ^{+    0.00000 }_{   -0.00000 }$&$ 0.57  ^{+ 0.08  }_{ -0.57 }$&$ 0.008  ^{+ 0.000  }_{ -0.002 }$&$ 0.21  ^{+ 0.49  }_{ -0.21 }$&$ 0.05  ^{+ 5.26  }_{ -0.05 }$&$ 1.79  \pm{ 0.24  }$&$ 86.68 ^{+ 1.88  }_{ -0.60 }$&$ 9.5   ^{+ 0.4   }_{ -0.6  }$&$ 0.089  \pm{ 0.002  }$&$ 1250  \pm{ 46    }$&$ 77    \pm{ 9     }$& 6.0   & 1.6  &0.025 & 0.560 \\
K01932.01  & 5202905    & 144.4640  &$   22.82485 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.07  }_{ -0.07 }$&$ 0.023  ^{+ 0.122  }_{ -0.002 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 6.13  ^{+ 0.16  }_{ -5.78 }$&$ 10.47 \pm{ 27.83 }$&$ 85.19 ^{+ 1.20  }_{ -2.67 }$&$ 10.9  ^{+ 0.6   }_{ -0.7  }$&$ 0.214  \pm{ 0.014  }$&$ 1619  \pm{ 119   }$&$ 445   \pm{ 111   }$& 6.6   & 0.6  &0.015 & 0.281 \\
K01932.02  & 5202905    & 143.5855  &$   14.84440 ^{+    0.00000 }_{   -0.00000 }$&$ 0.66  ^{+ 0.34  }_{ -0.58 }$&$ 0.011  ^{+ 0.006  }_{ -0.005 }$&$ 0.24  ^{+ 0.46  }_{ -0.23 }$&$ 1.51  ^{+ 4.78  }_{ -1.34 }$&$ 4.60  \pm{ 3.41  }$&$ 85.03 ^{+ 4.97  }_{ -5.63 }$&$ 5.1   ^{+ 1.7   }_{ -1.5  }$&$ 0.155  \pm{ 0.017  }$&$ 1958  \pm{ 346   }$&$ 128   \pm{ 85    }$& 10.3  & 0.5  &0.049 & 0.562 \\
K01955.01  & 9892816    & 132.6668  &$   15.17019 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.01  }_{ -0.01 }$&$ 0.018  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.07  ^{+ 5.76  }_{ -0.07 }$&$ 6.19  \pm{ 0.85  }$&$ 83.95 ^{+ 0.53  }_{ -0.78 }$&$ 9.5   ^{+ 0.3   }_{ -1.0  }$&$ 0.151  \pm{ 0.005  }$&$ 1424  \pm{ 63    }$&$ 230   \pm{ 12    }$& 4.6   & 1.1  &0.124 & 0.876 \\
K01955.02  & 9892816    & 136.4553  &$   39.45988 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.03  }_{ -0.03 }$&$ 0.015  ^{+ 0.002  }_{ -0.001 }$&$ 0.03  ^{+ 0.66  }_{ -0.03 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 6.57  \pm{ 0.83  }$&$ 87.02 ^{+ 0.46  }_{ -0.41 }$&$ 17.8  ^{+ 0.8   }_{ -2.2  }$&$ 0.280  \pm{ 0.006  }$&$ 1038  \pm{ 43    }$&$ 209   \pm{ 21    }$& 8.6   & 0.5  &0.067 & 0.781 \\
K01955.03  & 9892816    & 131.7567  &$    1.64420 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.04  }_{ -0.04 }$&$ 0.007  ^{+ 0.000  }_{ -0.000 }$&$ 0.08  ^{+ 0.19  }_{ -0.08 }$&$ 0.61  ^{+ 5.68  }_{ -0.60 }$&$ 2.50  \pm{ 0.25  }$&$ 62.49 ^{+ 2.01  }_{ -2.49 }$&$ 1.9   ^{+ 0.1   }_{ -0.1  }$&$ 0.031  \pm{ 0.002  }$&$ 2960  \pm{ 120   }$&$ 41    \pm{ 4     }$& 2.8   & 0.6  &0.008 & 0.283 \\
K01955.04  & 9892816    & 141.9958  &$   26.23420 ^{+    0.00000 }_{   -0.00000 }$&$ 0.99  ^{+ 0.01  }_{ -0.01 }$&$ 0.015  ^{+ 0.005  }_{ -0.002 }$&$ 0.07  ^{+ 0.63  }_{ -0.07 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 4.94  \pm{ 1.79  }$&$ 86.21 ^{+ 1.35  }_{ -3.34 }$&$ 13.5  ^{+ 1.5   }_{ -1.9  }$&$ 0.189  \pm{ 0.015  }$&$ 1112  \pm{ 143   }$&$ 142   \pm{ 17    }$& 3.4   & 1.2  &0.029 & 0.601 \\
K02004.01  & 12154526   & 146.3714  &$   56.18945 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.03  }_{ -0.02 }$&$ 0.021  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 1.22  ^{+ 5.07  }_{ -1.22 }$&$ 5.08  \pm{ 0.80  }$&$ 88.16 ^{+ 0.26  }_{ -0.44 }$&$ 27.4  ^{+ 1.7   }_{ -6.3  }$&$ 0.292  \pm{ 0.016  }$&$ 707   \pm{ 52    }$&$ 355   \pm{ 31    }$& 6.7   & 0.9  &0.143 & 0.893 \\
K02004.02  & 12154526   & 133.5255  &$    3.18899 ^{+    0.00000 }_{   -0.00000 }$&$ 0.99  ^{+ 0.01  }_{ -0.06 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.08  ^{+ 0.61  }_{ -0.08 }$&$ 2.07  ^{+ 3.72  }_{ -2.03 }$&$ 2.41  \pm{ 0.50  }$&$ 75.23 ^{+ 1.18  }_{ -14.70 }$&$ 3.7   ^{+ 0.2   }_{ -0.6  }$&$ 0.048  \pm{ 0.002  }$&$ 1938  \pm{ 70    }$&$ 66    \pm{ 7     }$& 2.5   & 0.5  &0.021 & 0.517 \\
K02004.03  & 12154526   & 132.7764  &$    0.00000 ^{+    0.00000 }_{    0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.000  ^{+ 0.000  }_{ 0.000  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  \pm{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 3.6   ^{+ 0.2   }_{ -0.6  }$&$ 0.000  \pm{ 0.000  }$&$ 0     \pm{ 0     }$&$ 66    \pm{ 7     }$& 2.5   & 1.5  &0.016 & 0.450 \\
K02011.01  & 5384079    & 132.5342  &$    7.05670 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.01  }_{ -0.00 }$&$ 0.014  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.55  }_{ -0.00 }$&$ 1.63  ^{+ 4.56  }_{ -1.54 }$&$ 4.84  \pm{ 0.70  }$&$ 80.19 ^{+ 4.45  }_{ -1.81 }$&$ 5.2   ^{+ 0.5   }_{ -0.4  }$&$ 0.088  \pm{ 0.002  }$&$ 1783  \pm{ 128   }$&$ 117   \pm{ 6     }$& 2.5   & 0.7  &0.031 & 0.441 \\
K02011.02  & 5384079    & 135.3499  &$   17.26555 ^{+    0.00000 }_{   -0.00000 }$&$ 0.86  ^{+ 0.14  }_{ -0.43 }$&$ 0.009  ^{+ 0.021  }_{ -0.001 }$&$ 0.06  ^{+ 0.61  }_{ -0.06 }$&$ 0.80  ^{+ 5.49  }_{ -0.79 }$&$ 1.05  \pm{ 1.26  }$&$ 86.59 ^{+ 2.90  }_{ -1.90 }$&$ 23.3  ^{+ 3.8   }_{ -11.2 }$&$ 0.133  \pm{ 0.010  }$&$ 1099  \pm{ 277   }$&$ 80    \pm{ 10    }$& 5.1   & 0.7  &0.002 & 0.049 \\
K02029.01  & 9489524    & 136.9036  &$   16.33287 ^{+    0.00000 }_{   -0.00000 }$&$ 2.29  ^{+ -1.29 }_{ -1.30 }$&$ 0.019  ^{+ 0.003  }_{ -0.003 }$&$ 0.70  ^{+ -0.00 }_{ -0.11 }$&$ 2.78  ^{+ 3.50  }_{ -2.59 }$&$ 5.09  \pm{ 0.82  }$&$ 79.14 ^{+ 4.55  }_{ -4.23 }$&$ 12.0  ^{+ 0.4   }_{ -0.7  }$&$ 0.138  \pm{ 0.004  }$&$ 992   \pm{ 37    }$&$ 274   \pm{ 14    }$& 2.5   & 0.2  &0.052 & 0.734 \\
K02029.02  & 9489524    & 173.2239  &$   10.05548 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.01  }_{ -0.38 }$&$ 0.014  ^{+ 0.001  }_{ -0.003 }$&$ 0.01  ^{+ 0.30  }_{ -0.01 }$&$ 0.15  ^{+ 3.97  }_{ -0.15 }$&$ 3.51  \pm{ 0.52  }$&$ 84.32 ^{+ 4.59  }_{ -0.81 }$&$ 9.2   ^{+ 0.5   }_{ -0.5  }$&$ 0.099  \pm{ 0.003  }$&$ 1121  \pm{ 424   }$&$ 137   \pm{ 11    }$& 2.9   & 0.8  &0.006 & 0.238 \\
K02029.03  & 9489524    & 132.0775  &$    6.88721 ^{+    0.00000 }_{   -0.00000 }$&$ 0.72  ^{+ 0.23  }_{ -0.26 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.08  ^{+ 0.55  }_{ -0.08 }$&$ 0.72  ^{+ 2.95  }_{ -0.71 }$&$ 0.81  \pm{ 0.18  }$&$ 87.43 ^{+ 1.25  }_{ -8.87 }$&$ 17.5  ^{+ 3.0   }_{ -1.8  }$&$ 0.069  \pm{ 0.003  }$&$ 855   \pm{ 145   }$&$ 80    \pm{ 9     }$& 2.3   & 0.6  &0.004 & 0.158 \\
K02029.04  & 9489524    & 135.4647  &$    4.78843 ^{+    0.00000 }_{   -0.00000 }$&$ 0.58  ^{+ 0.35  }_{ -0.57 }$&$ 0.007  ^{+ 0.000  }_{ -0.005 }$&$ 0.18  ^{+ 0.41  }_{ -0.18 }$&$ 0.16  ^{+ 2.46  }_{ -0.16 }$&$ 0.65  \pm{ 0.27  }$&$ 87.44 ^{+ 2.47  }_{ -7.42 }$&$ 13.0  ^{+ 1.0   }_{ -7.0  }$&$ 0.054  \pm{ 0.001  }$&$ 963   \pm{ 157   }$&$ 56    \pm{ 7     }$& 2.3   & 1.1  &0.004 & 0.158 \\
K02053.01  & 2307415    & 133.3943  &$   13.12155 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.01  }_{ -0.02 }$&$ 0.016  ^{+ 0.000  }_{ -0.003 }$&$ 0.03  ^{+ 0.67  }_{ -0.03 }$&$ 1.60  ^{+ 4.67  }_{ -1.60 }$&$ 5.01  \pm{ 0.96  }$&$ 83.53 ^{+ 0.86  }_{ -1.68 }$&$ 9.0   ^{+ 1.2   }_{ -0.9  }$&$ 0.124  \pm{ 0.005  }$&$ 1417  \pm{ 81    }$&$ 187   \pm{ 14    }$& 3.9   & 0.7  &0.024 & 0.377 \\
K02053.02  & 2307415    & 132.7749  &$    4.61266 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.03  }_{ -0.05 }$&$ 0.012  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.47  }_{ -0.00 }$&$ 0.06  ^{+ 1.75  }_{ -0.06 }$&$ 4.81  \pm{ 0.92  }$&$ 77.35 ^{+ 4.66  }_{ -4.72 }$&$ 3.6   ^{+ 0.3   }_{ -0.3  }$&$ 0.061  \pm{ 0.003  }$&$ 2011  \pm{ 235   }$&$ 121   \pm{ 8     }$& 3.3   & 0.5  &0.039 & 0.502 \\
K02059.01  & 12301181   & 134.8728  &$    6.14730 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.60  \pm{ 0.05  }$&$ 90.00 ^{+ -0.00 }_{ -0.00 }$&$ 21.5  ^{+ 0.7   }_{ -1.0  }$&$ 0.054  \pm{ 0.001  }$&$ 695   \pm{ 21    }$&$ 130   \pm{ 8     }$& 2.2   & 0.5  &0.047 & 0.551 \\
K02059.02  & 12301181   & 132.4311  &$    0.00000 ^{+    0.00000 }_{    0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.000  ^{+ 0.000  }_{ 0.000  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  \pm{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.0   ^{+ 0.0   }_{ 0.0   }$&$ 0.000  \pm{ 0.000  }$&$ 0     \pm{ 0     }$&$ 130   \pm{ 8     }$& 2.2   & 0.7  &0.011 & 0.216 \\
K02148.01  & 6021193    & 142.1019  &$   11.93223 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.51  }_{ -0.00 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.45  }_{ -0.00 }$&$ 0.00  ^{+ 4.10  }_{ -0.00 }$&$ 1.48  \pm{ 0.09  }$&$ 90.00 ^{+ 0.00  }_{ -0.90 }$&$ 20.5  ^{+ 0.9   }_{ -2.9  }$&$ 0.100  \pm{ 0.003  }$&$ 812   \pm{ 28    }$&$ 210   \pm{ 17    }$& 4.4   & 0.2  &0.048 & 0.714 \\
K02148.02  & 6021193    & 132.9564  &$    7.54236 ^{+    0.00000 }_{   -0.00000 }$&$ 0.75  ^{+ 0.08  }_{ -0.25 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.03  ^{+ 0.48  }_{ -0.03 }$&$ 0.14  ^{+ 2.15  }_{ -0.14 }$&$ 2.29  \pm{ 0.45  }$&$ 84.75 ^{+ 1.69  }_{ -1.76 }$&$ 8.2   ^{+ 0.6   }_{ -1.0  }$&$ 0.079  \pm{ 0.003  }$&$ 1292  \pm{ 85    }$&$ 124   \pm{ 14    }$& 4.7   & 0.4  &0.047 & 0.713 \\
K02148.03  & 6021193    & 134.7000  &$    3.61461 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.11  }_{ -0.07 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.17  ^{+ 0.49  }_{ -0.17 }$&$ 1.67  ^{+ 2.33  }_{ -1.58 }$&$ 1.89  \pm{ 0.31  }$&$ 79.14 ^{+ 2.55  }_{ -2.94 }$&$ 4.7   ^{+ 0.3   }_{ -0.7  }$&$ 0.048  \pm{ 0.002  }$&$ 1712  \pm{ 103   }$&$ 67    \pm{ 9     }$& 3.4   & 0.8  &0.021 & 0.513 \\
K02158.01  & 5211199    & 132.6314  &$    4.56215 ^{+    0.00000 }_{   -0.00000 }$&$ 0.88  ^{+ 0.04  }_{ -0.20 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.25  }_{ -0.00 }$&$ 0.65  ^{+ 2.22  }_{ -0.65 }$&$ 1.84  \pm{ 0.25  }$&$ 81.48 ^{+ 2.69  }_{ -2.24 }$&$ 5.8   ^{+ 0.6   }_{ -1.4  }$&$ 0.051  \pm{ 0.001  }$&$ 1471  \pm{ 98    }$&$ 75    \pm{ 7     }$& 2.9   & 1.0  &0.011 & 0.224 \\
K02158.02  & 5211199    & 132.1895  &$    6.68232 ^{+    0.00000 }_{   -0.00000 }$&$ 1.49  ^{+ -0.49 }_{ -0.61 }$&$ 0.008  ^{+ 0.060  }_{ -0.001 }$&$ 0.53  ^{+ 0.12  }_{ -0.53 }$&$ 0.37  ^{+ 1.10  }_{ -0.37 }$&$ 2.37  \pm{ 9.08  }$&$ 74.50 ^{+ 7.64  }_{ -8.05 }$&$ 5.6   ^{+ 0.5   }_{ -2.6  }$&$ 0.076  \pm{ 0.005  }$&$ 1524  \pm{ 216   }$&$ 53    \pm{ 8     }$& 3.1   & 1.1  &0.001 & 0.033 \\
K02169.01  & 9006186    & 134.1486  &$    5.45300 ^{+    0.00000 }_{   -0.00000 }$&$ 1.71  ^{+ -0.71 }_{ -0.76 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.70  ^{+ -0.00 }_{ -0.62 }$&$ 0.77  ^{+ 2.77  }_{ -0.77 }$&$ 1.71  \pm{ 0.50  }$&$ 76.66 ^{+ 4.18  }_{ -15.24 }$&$ 7.1   ^{+ 0.6   }_{ -0.8  }$&$ 0.058  \pm{ 0.002  }$&$ 1317  \pm{ 363   }$&$ 88    \pm{ 4     }$& 2.3   & 1.0  &0.097 & 0.842 \\
K02169.02  & 9006186    & 136.0883  &$    3.26661 ^{+    0.00000 }_{   -0.00000 }$&$ 1.55  ^{+ -0.56 }_{ -0.64 }$&$ 0.008  ^{+ 0.001  }_{ -0.001 }$&$ 0.66  ^{+ 0.04  }_{ -0.26 }$&$ 6.29  ^{+ -0.15 }_{ -3.97 }$&$ 1.51  \pm{ 0.25  }$&$ 71.94 ^{+ 6.58  }_{ -9.84 }$&$ 5.0   ^{+ 0.4   }_{ -0.3  }$&$ 0.041  \pm{ 0.001  }$&$ 1613  \pm{ 124   }$&$ 50    \pm{ 3     }$& 2.1   & 0.1  &0.065 & 0.776 \\
K02169.03  & 9006186    & 133.2112  &$    4.27235 ^{+    0.00000 }_{   -0.00000 }$&$ 2.16  ^{+ -1.16 }_{ -1.28 }$&$ 0.007  ^{+ 0.001  }_{ -0.001 }$&$ 0.70  ^{+ -0.00 }_{ -0.05 }$&$ 2.13  ^{+ 1.17  }_{ -2.01 }$&$ 1.12  \pm{ 0.35  }$&$ 64.28 ^{+ 11.99 }_{ -4.15 }$&$ 5.3   ^{+ 0.8   }_{ -1.6  }$&$ 0.050  \pm{ 0.002  }$&$ 1608  \pm{ 154   }$&$ 46    \pm{ 4     }$& 2.4   & 1.2  &0.040 & 0.675 \\
K02169.04  & 9006186    & 132.2252  &$    2.19259 ^{+    0.00000 }_{   -0.00000 }$&$ 1.03  ^{+ -0.04 }_{ -0.21 }$&$ 0.004  ^{+ 0.021  }_{ -0.001 }$&$ 0.28  ^{+ 0.33  }_{ -0.28 }$&$ 2.67  ^{+ 1.27  }_{ -2.06 }$&$ 0.83  \pm{ 2.19  }$&$ 73.51 ^{+ 12.85 }_{ -5.67 }$&$ 3.7   ^{+ 0.6   }_{ -1.0  }$&$ 0.031  \pm{ 0.001  }$&$ 1904  \pm{ 259   }$&$ 15    \pm{ 3     }$& 2.2   & 0.6  &0.022 & 0.525 \\
K02173.01  & 11774991   & 141.1054  &$   37.81526 ^{+    0.00000 }_{   -0.00000 }$&$ 0.51  ^{+ 0.19  }_{ -0.51 }$&$ 0.015  ^{+ 0.003  }_{ -0.001 }$&$ 0.12  ^{+ 0.58  }_{ -0.12 }$&$ 0.92  ^{+ 5.37  }_{ -0.92 }$&$ 1.26  \pm{ 0.19  }$&$ 89.46 ^{+ 0.54  }_{ -1.88 }$&$ 55.2  ^{+ 1.5   }_{ -3.4  }$&$ 0.204  \pm{ 0.002  }$&$ 428   \pm{ 70    }$&$ 270   \pm{ 21    }$& 4.3   & 0.8  &0.011 & 0.215 \\
K02173.02  & 11774991   & 171.1865  &$   53.57820 ^{+    0.00000 }_{   -0.00000 }$&$ 0.49  ^{+ 0.44  }_{ -0.36 }$&$ 0.015  ^{+ 0.001  }_{ -0.006 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.73  }_{ -0.00 }$&$ 1.27  \pm{ 0.35  }$&$ 89.59 ^{+ 0.32  }_{ -1.41 }$&$ 69.9  ^{+ 6.4   }_{ -38.0 }$&$ 0.256  \pm{ 0.010  }$&$ 384   \pm{ 62    }$&$ 275   \pm{ 25    }$& 5.3   & 0.9  &0.007 & 0.142 \\
K02175.01  & 9022166    & 142.1752  &$   26.84734 ^{+    0.00000 }_{   -0.00000 }$&$ 0.54  ^{+ 0.32  }_{ -0.19 }$&$ 0.015  ^{+ 0.001  }_{ -0.001 }$&$ 0.02  ^{+ 0.30  }_{ -0.02 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 3.55  \pm{ 0.56  }$&$ 88.23 ^{+ 0.63  }_{ -1.56 }$&$ 16.7  ^{+ 0.8   }_{ -1.9  }$&$ 0.175  \pm{ 0.010  }$&$ 844   \pm{ 39    }$&$ 268   \pm{ 25    }$& 10.0  & 0.6  &0.039 & 0.506 \\
K02175.02  & 9022166    & 179.5122  &$   72.38130 ^{+    0.00000 }_{   -0.00000 }$&$ 0.82  ^{+ 0.17  }_{ -0.82 }$&$ 0.021  ^{+ 0.005  }_{ -0.003 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 1.79  \pm{ 0.49  }$&$ 88.83 ^{+ 1.17  }_{ -0.28 }$&$ 32.4  ^{+ 37.4  }_{ -3.5  }$&$ 0.326  \pm{ 0.021  }$&$ 555   \pm{ 184   }$&$ 399   \pm{ 43    }$& 8.2   & 0.3  &0.031 & 0.441 \\
K02289.01  & 3867615    & 157.3033  &$   62.78500 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.03  }_{ -0.15 }$&$ 0.023  ^{+ 0.255  }_{ -0.004 }$&$ 0.03  ^{+ 0.46  }_{ -0.03 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 2.58  \pm{ 14.80 }$&$ 87.94 ^{+ 1.19  }_{ -1.91 }$&$ 25.4  ^{+ 25.0  }_{ -5.4  }$&$ 0.359  \pm{ 0.023  }$&$ 803   \pm{ 232   }$&$ 375   \pm{ 45    }$& 6.3   & 0.6  &0.012 & 0.234 \\
K02289.02  & 3867615    & 147.2808  &$   20.09846 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.11  }_{ -0.45 }$&$ 0.013  ^{+ 0.002  }_{ -0.001 }$&$ 0.08  ^{+ 0.62  }_{ -0.08 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 1.56  \pm{ 0.69  }$&$ 86.27 ^{+ 3.02  }_{ -1.39 }$&$ 11.7  ^{+ 4.5   }_{ -2.5  }$&$ 0.155  \pm{ 0.015  }$&$ 1111  \pm{ 326   }$&$ 156   \pm{ 22    }$& 5.5   & 0.4  &0.007 & 0.155 \\
K02311.01  & 4247991    & 294.4400  &$  191.88569 ^{+    0.00000 }_{   -0.00000 }$&$ 0.47  ^{+ 0.44  }_{ -0.47 }$&$ 0.003  ^{+ 0.007  }_{ -0.001 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.02  ^{+ 0.13  }_{ -0.02 }$&$ 0.97  \pm{ 1.51  }$&$ 88.92 ^{+ 1.08  }_{ -0.88 }$&$ 28.7  ^{+ 9.7   }_{ -6.3  }$&$ 0.799  \pm{ 0.051  }$&$ 766   \pm{ 78    }$&$ 6     \pm{ 42    }$& 17.3  & 0.5  &0.009 & 0.177 \\
K02311.02  & 4247991    & 145.0410  &$   13.72535 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.03  }_{ -0.09 }$&$ 0.006  ^{+ 0.030  }_{ -0.002 }$&$ 0.04  ^{+ 0.66  }_{ -0.03 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 3.64  \pm{ 9.92  }$&$ 78.92 ^{+ 1.23  }_{ -18.44 }$&$ 4.6   ^{+ 0.7   }_{ -0.7  }$&$ 0.135  \pm{ 0.008  }$&$ 1703  \pm{ 240   }$&$ 20    \pm{ 13    }$& 5.9   & 0.3  &0.002 & 0.049 \\
K02352.01  & 8013439    & 133.0583  &$   13.39140 ^{+    0.00000 }_{   -0.00000 }$&$ 1.01  ^{+ -0.01 }_{ -0.03 }$&$ 0.008  ^{+ 0.036  }_{ -0.000 }$&$ 0.19  ^{+ 0.51  }_{ -0.19 }$&$ 3.15  ^{+ 3.14  }_{ -2.62 }$&$ 2.62  \pm{ 6.14  }$&$ 82.49 ^{+ 2.18  }_{ -6.56 }$&$ 7.8   ^{+ 1.5   }_{ -2.5  }$&$ 0.137  \pm{ 0.013  }$&$ 1449  \pm{ 307   }$&$ 44    \pm{ 4     }$& 3.6   & 0.8  &0.040 & 0.676 \\
K02352.02  & 8013439    & 134.7477  &$    5.62903 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.02  }_{ -0.04 }$&$ 0.007  ^{+ 0.005  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 2.70  \pm{ 1.73  }$&$ 71.04 ^{+ 6.69  }_{ -6.05 }$&$ 3.9   ^{+ 1.2   }_{ -1.2  }$&$ 0.077  \pm{ 0.006  }$&$ 2434  \pm{ 471   }$&$ 35    \pm{ 2     }$& 4.1   & 0.4  &0.052 & 0.731 \\
K02352.03  & 8013439    & 137.9280  &$    8.25621 ^{+    0.00000 }_{   -0.00000 }$&$ 1.21  ^{+ -0.21 }_{ -0.22 }$&$ 0.008  ^{+ 0.010  }_{ -0.001 }$&$ 0.43  ^{+ 0.27  }_{ -0.43 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 4.36  \pm{ 3.22  }$&$ 74.98 ^{+ 3.26  }_{ -14.86 }$&$ 3.7   ^{+ 0.7   }_{ -1.5  }$&$ 0.098  \pm{ 0.008  }$&$ 1985  \pm{ 326   }$&$ 41    \pm{ 3     }$& 2.5   & 1.9  &0.041 & 0.681 \\
K02541.01  & 12306058   & 137.9603  &$    7.41682 ^{+    0.00000 }_{   -0.00000 }$&$ 0.53  ^{+ 0.17  }_{ -0.34 }$&$ 0.008  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 2.12  \pm{ 0.25  }$&$ 85.53 ^{+ 2.54  }_{ -2.32 }$&$ 6.6   ^{+ 0.5   }_{ -1.3  }$&$ 0.079  \pm{ 0.003  }$&$ 1337  \pm{ 93    }$&$ 71    \pm{ 12    }$& 7.2   & 0.4  &0.053 & 0.583 \\
K02541.02  & 12306058   & 146.9230  &$   20.48565 ^{+    0.00000 }_{   -0.00000 }$&$ 0.53  ^{+ 0.22  }_{ -0.50 }$&$ 0.009  ^{+ 0.001  }_{ -0.001 }$&$ 0.10  ^{+ 0.52  }_{ -0.10 }$&$ 1.18  ^{+ 5.11  }_{ -1.17 }$&$ 2.49  \pm{ 0.71  }$&$ 87.51 ^{+ 2.09  }_{ -2.11 }$&$ 12.5  ^{+ 1.9   }_{ -2.3  }$&$ 0.151  \pm{ 0.011  }$&$ 988   \pm{ 95    }$&$ 95    \pm{ 20    }$& 10.4  & 0.3  &0.037 & 0.488 \\
K02585.01  & 7673841    & 136.3069  &$    5.34189 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.04  }_{ -0.02 }$&$ 0.009  ^{+ 0.013  }_{ -0.000 }$&$ 0.02  ^{+ 0.45  }_{ -0.02 }$&$ 1.59  ^{+ 4.70  }_{ -1.52 }$&$ 2.88  \pm{ 2.11  }$&$ 78.39 ^{+ 1.88  }_{ -1.96 }$&$ 4.8   ^{+ 0.5   }_{ -0.4  }$&$ 0.067  \pm{ 0.003  }$&$ 1986  \pm{ 122   }$&$ 67    \pm{ 8     }$& 3.2   & 0.7  &0.025 & 0.562 \\
K02585.02  & 7673841    & 135.1572  &$   10.42305 ^{+    0.00000 }_{   -0.00000 }$&$ 0.88  ^{+ 0.09  }_{ -0.21 }$&$ 0.009  ^{+ 0.013  }_{ -0.004 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 1.58  ^{+ 4.71  }_{ -1.32 }$&$ 1.13  \pm{ 1.00  }$&$ 87.14 ^{+ 2.86  }_{ -4.02 }$&$ 8.4   ^{+ 8.0   }_{ -3.4  }$&$ 0.094  \pm{ 0.007  }$&$ 1022  \pm{ 190   }$&$ 79    \pm{ 11    }$& 2.2   & 0.5  &0.021 & 0.514 \\
K02585.03  & 7673841    & 138.5965  &$    7.87811 ^{+    0.00000 }_{   -0.00000 }$&$ 1.91  ^{+ -0.92 }_{ -1.13 }$&$ 0.008  ^{+ 0.061  }_{ -0.002 }$&$ 0.70  ^{+ 0.00  }_{ -0.06 }$&$ 0.00  ^{+ 0.54  }_{ -0.00 }$&$ 0.94  \pm{ 3.75  }$&$ 70.62 ^{+ 7.30  }_{ -10.62 }$&$ 4.7   ^{+ 2.2   }_{ -0.8  }$&$ 0.077  \pm{ 0.005  }$&$ 1798  \pm{ 625   }$&$ 48    \pm{ 10    }$& 2.7   & 0.2  &0.005 & 0.206 \\
K02595.01  & 8883329    & 134.0478  &$    9.18252 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.01  }_{ -0.02 }$&$ 0.010  ^{+ 0.000  }_{ -0.000 }$&$ 0.02  ^{+ 0.17  }_{ -0.02 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 4.47  \pm{ 0.62  }$&$ 79.93 ^{+ 2.09  }_{ -0.47 }$&$ 5.2   ^{+ 0.4   }_{ -0.4  }$&$ 0.100  \pm{ 0.004  }$&$ 1908  \pm{ 90    }$&$ 79    \pm{ 10    }$& 4.4   & 0.1  &0.024 & 0.378 \\
K02595.02  & 8883329    & 140.4080  &$   14.61360 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.08  }_{ -0.03 }$&$ 0.009  ^{+ 0.130  }_{ -0.001 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.06  ^{+ 1.52  }_{ -0.06 }$&$ 3.27  \pm{ 22.60 }$&$ 83.54 ^{+ 0.79  }_{ -8.82 }$&$ 8.7   ^{+ 0.6   }_{ -1.8  }$&$ 0.134  \pm{ 0.006  }$&$ 1560  \pm{ 155   }$&$ 74    \pm{ 13    }$& 5.7   & 0.8  &0.036 & 0.485 \\
K02672.01  & 11253827   & 182.6526  &$   88.51658 ^{+    0.00000 }_{   -0.00000 }$&$ 0.71  ^{+ 0.26  }_{ -0.14 }$&$ 0.051  ^{+ 0.004  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 5.13  \pm{ 1.31  }$&$ 89.45 ^{+ 0.21  }_{ -0.70 }$&$ 44.8  ^{+ 29.8  }_{ -16.7 }$&$ 0.371  \pm{ 0.010  }$&$ 429   \pm{ 58    }$&$ 2683  \pm{ 31    }$& 6.9   & 0.3  &0.846 & 0.993 \\
K02672.02  & 11253827   & 162.5118  &$   42.99066 ^{+    0.00000 }_{   -0.00000 }$&$ 0.59  ^{+ 0.19  }_{ -0.59 }$&$ 0.030  ^{+ 0.002  }_{ -0.001 }$&$ 0.55  ^{+ 0.15  }_{ -0.51 }$&$ 2.44  ^{+ 3.85  }_{ -2.05 }$&$ 2.96  \pm{ 0.85  }$&$ 89.22 ^{+ 0.78  }_{ -1.10 }$&$ 28.4  ^{+ 19.6  }_{ -10.0 }$&$ 0.227  \pm{ 0.009  }$&$ 560   \pm{ 87    }$&$ 1062  \pm{ 17    }$& 4.6   & 0.3  &0.894 & 0.995 \\
K02674.01  & 8022489    & 272.3869  &$  197.51031 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.06  }_{ -0.07 }$&$ 0.053  ^{+ 0.001  }_{ -0.001 }$&$ 0.20  ^{+ 0.31  }_{ -0.20 }$&$ 0.39  ^{+ 2.07  }_{ -0.39 }$&$ 10.88 \pm{ 1.98  }$&$ 89.30 ^{+ 0.12  }_{ -0.21 }$&$ 72.2  ^{+ 5.3   }_{ -21.1 }$&$ 0.662  \pm{ 0.027  }$&$ 444   \pm{ 22    }$&$ 2664  \pm{ 58    }$& 10.9  & 0.8  &0.339 & 0.962 \\
K02674.02  & 8022489    & 140.0090  &$   11.17265 ^{+    0.00000 }_{   -0.00000 }$&$ 3.43  ^{+ -2.51 }_{ -2.52 }$&$ 0.023  ^{+ 0.020  }_{ -0.011 }$&$ 0.01  ^{+ 0.01  }_{ -0.01 }$&$ 0.17  ^{+ 0.22  }_{ -0.10 }$&$ 2.37  \pm{ 1.64  }$&$ 80.81 ^{+ 0.62  }_{ -0.54 }$&$ 19.6  ^{+ 2.8   }_{ -8.3  }$&$ 0.096  \pm{ 0.005  }$&$ 856   \pm{ 75    }$&$ 0     \pm{ 13    }$& 0.0   & 0.4  &0.023 & 0.540 \\
K02674.03  & 8022489    & 133.0107  &$    2.53574 ^{+    0.00000 }_{   -0.00000 }$&$ 0.62  ^{+ 0.13  }_{ -0.35 }$&$ 0.008  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.16  ^{+ 6.12  }_{ -0.16 }$&$ 1.80  \pm{ 0.22  }$&$ 80.73 ^{+ 4.82  }_{ -3.52 }$&$ 3.8   ^{+ 0.3   }_{ -0.5  }$&$ 0.037  \pm{ 0.001  }$&$ 2022  \pm{ 130   }$&$ 67    \pm{ 6     }$& 4.1   & 0.7  &0.017 & 0.465 \\
K02675.01  & 5794570    & 132.4894  &$    5.44833 ^{+    0.00000 }_{   -0.00000 }$&$ 1.10  ^{+ -0.11 }_{ -0.14 }$&$ 0.026  ^{+ 0.000  }_{ -0.005 }$&$ 0.37  ^{+ 0.32  }_{ -0.33 }$&$ 0.00  ^{+ 0.96  }_{ -0.00 }$&$ 7.04  \pm{ 0.91  }$&$ 79.40 ^{+ 1.43  }_{ -4.56 }$&$ 5.6   ^{+ 0.3   }_{ -0.3  }$&$ 0.064  \pm{ 0.004  }$&$ 1550  \pm{ 100   }$&$ 525   \pm{ 5     }$& 2.6   & 1.7  &0.796 & 0.990 \\
K02675.02  & 5794570    & 131.8464  &$    1.11613 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.02  }_{ -0.00 }$&$ 0.012  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 3.30  \pm{ 0.24  }$&$ 60.63 ^{+ 1.00  }_{ -0.53 }$&$ 1.9   ^{+ 0.0   }_{ -0.1  }$&$ 0.023  \pm{ 0.001  }$&$ 2685  \pm{ 46    }$&$ 101   \pm{ 2     }$& 1.5   & 1.8  &0.112 & 0.759 \\
K02687.01  & 7202957    & 132.0299  &$    1.71684 ^{+    0.00000 }_{   -0.00000 }$&$ 0.91  ^{+ 0.02  }_{ -0.03 }$&$ 0.008  ^{+ 0.002  }_{ -0.000 }$&$ 0.00  ^{+ 0.48  }_{ -0.00 }$&$ 0.01  ^{+ 1.42  }_{ -0.01 }$&$ 2.02  \pm{ 0.31  }$&$ 70.66 ^{+ 2.52  }_{ -2.32 }$&$ 2.7   ^{+ 0.2   }_{ -0.2  }$&$ 0.028  \pm{ 0.001  }$&$ 2304  \pm{ 96    }$&$ 56    \pm{ 1     }$& 2.2   & 4.3  &0.469 & 0.957 \\
K02687.02  & 7202957    & 136.2009  &$    8.16739 ^{+    0.00000 }_{   -0.00000 }$&$ 0.73  ^{+ 0.17  }_{ -0.73 }$&$ 0.012  ^{+ 0.001  }_{ -0.001 }$&$ 0.30  ^{+ 0.40  }_{ -0.30 }$&$ 4.68  ^{+ 1.61  }_{ -3.76 }$&$ 2.77  \pm{ 0.47  }$&$ 84.73 ^{+ 5.27  }_{ -1.48 }$&$ 7.8   ^{+ 0.8   }_{ -1.1  }$&$ 0.083  \pm{ 0.004  }$&$ 1359  \pm{ 90    }$&$ 99    \pm{ 2     }$& 3.6   & 2.7  &0.415 & 0.947 \\
K02693.01  & 5185897    & 133.8593  &$    4.08141 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.011  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.20  }_{ -0.00 }$&$ 0.78  \pm{ 0.03  }$&$ 90.00 ^{+ 0.00  }_{ -0.00 }$&$ 14.8  ^{+ 0.3   }_{ -0.9  }$&$ 0.045  \pm{ 0.001  }$&$ 767   \pm{ 18    }$&$ 159   \pm{ 6     }$& 2.1   & 2.0  &0.049 & 0.722 \\
K02693.02  & 5185897    & 142.1177  &$   11.41942 ^{+    0.00000 }_{   -0.00000 }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.023  ^{+ 0.018  }_{ -0.011 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 1.59  \pm{ 1.02  }$&$ 85.72 ^{+ 0.55  }_{ -0.73 }$&$ 29.3  ^{+ 1.5   }_{ -2.4  }$&$ 0.089  \pm{ 0.003  }$&$ 503   \pm{ 23    }$&$ 0     \pm{ 12    }$& 0.0   & 1.4  &0.021 & 0.515 \\
K02693.03  & 5185897    & 136.8490  &$    6.83448 ^{+    0.00000 }_{   -0.00000 }$&$ 0.42  ^{+ 0.17  }_{ -0.42 }$&$ 0.011  ^{+ 0.001  }_{ -0.000 }$&$ 0.00  ^{+ 0.15  }_{ -0.00 }$&$ 0.01  ^{+ 1.22  }_{ -0.01 }$&$ 0.78  \pm{ 0.09  }$&$ 88.89 ^{+ 1.09  }_{ -0.52 }$&$ 20.8  ^{+ 0.9   }_{ -1.0  }$&$ 0.063  \pm{ 0.002  }$&$ 632   \pm{ 30    }$&$ 158   \pm{ 8     }$& 2.2   & 1.3  &0.026 & 0.571 \\
K02696.01  & 11071200   & 214.7486  &$   96.45620 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.02  }_{ -0.02 }$&$ 0.034  ^{+ 0.001  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.01  ^{+ 4.68  }_{ -0.01 }$&$ 13.02 \pm{ 0.95  }$&$ 88.32 ^{+ 0.20  }_{ -0.25 }$&$ 29.3  ^{+ 1.6   }_{ -5.3  }$&$ 0.488  \pm{ 0.023  }$&$ 837   \pm{ 37    }$&$ 1032  \pm{ 62    }$& 12.1  & 0.5  &0.065 & 0.634 \\
K02696.02  & 11071200   & 143.4267  &$   44.56505 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.06  }_{ -0.02 }$&$ 0.020  ^{+ 0.002  }_{ -0.002 }$&$ 0.03  ^{+ 0.65  }_{ -0.03 }$&$ 0.91  ^{+ 5.38  }_{ -0.91 }$&$ 7.71  \pm{ 1.03  }$&$ 87.09 ^{+ 0.49  }_{ -0.48 }$&$ 17.6  ^{+ 1.1   }_{ -3.5  }$&$ 0.290  \pm{ 0.012  }$&$ 1086  \pm{ 56    }$&$ 347   \pm{ 31    }$& 8.1   & 0.8  &0.103 & 0.741 \\
K02714.01  & 12206313   & 140.5597  &$   14.38351 ^{+    0.00000 }_{   -0.00000 }$&$ 0.58  ^{+ 0.13  }_{ -0.13 }$&$ 0.012  ^{+ 0.000  }_{ -0.004 }$&$ 0.02  ^{+ 0.54  }_{ -0.02 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 3.27  \pm{ 0.79  }$&$ 86.95 ^{+ 0.87  }_{ -1.23 }$&$ 10.7  ^{+ 0.6   }_{ -0.9  }$&$ 0.124  \pm{ 0.004  }$&$ 1283  \pm{ 66    }$&$ 167   \pm{ 16    }$& 8.5   & 1.5  &0.066 & 0.640 \\
K02714.02  & 12206313   & 170.0987  &$   47.31319 ^{+    0.00000 }_{   -0.00000 }$&$ 0.71  ^{+ 0.24  }_{ -0.14 }$&$ 0.015  ^{+ 0.002  }_{ -0.001 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 4.03  \pm{ 1.02  }$&$ 88.25 ^{+ 0.46  }_{ -0.61 }$&$ 22.4  ^{+ 1.7   }_{ -2.3  }$&$ 0.272  \pm{ 0.009  }$&$ 870   \pm{ 108   }$&$ 234   \pm{ 30    }$& 11.2  & 0.9  &0.074 & 0.667 \\
K02722.01  & 7673192    & 134.9353  &$    6.12482 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.01  }_{ -0.02 }$&$ 0.013  ^{+ 0.000  }_{ -0.000 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 1.12  ^{+ 5.17  }_{ -0.93 }$&$ 5.97  \pm{ 0.48  }$&$ 77.23 ^{+ 1.74  }_{ -0.72 }$&$ 4.2   ^{+ 0.3   }_{ -0.1  }$&$ 0.082  \pm{ 0.003  }$&$ 2087  \pm{ 85    }$&$ 137   \pm{ 8     }$& 3.9   & 1.5  &0.062 & 0.768 \\
K02722.02  & 7673192    & 136.3216  &$   11.24280 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.01  }_{ -0.01 }$&$ 0.014  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.06  }_{ -0.00 }$&$ 6.29  ^{+ 0.00  }_{ -5.25 }$&$ 5.99  \pm{ 0.67  }$&$ 81.68 ^{+ 1.19  }_{ -9.21 }$&$ 6.5   ^{+ 0.6   }_{ -0.4  }$&$ 0.119  \pm{ 0.005  }$&$ 1696  \pm{ 85    }$&$ 140   \pm{ 11    }$& 4.6   & 0.5  &0.034 & 0.637 \\
K02722.03  & 7673192    & 133.7748  &$    4.02871 ^{+    0.00000 }_{   -0.00000 }$&$ 1.51  ^{+ -0.52 }_{ -0.56 }$&$ 0.011  ^{+ 0.001  }_{ -0.001 }$&$ 0.65  ^{+ 0.04  }_{ -0.19 }$&$ 3.40  ^{+ 2.36  }_{ -1.65 }$&$ 5.21  \pm{ 0.43  }$&$ 61.28 ^{+ 9.28  }_{ -1.28 }$&$ 3.1   ^{+ 0.1   }_{ -0.1  }$&$ 0.060  \pm{ 0.003  }$&$ 2460  \pm{ 68    }$&$ 97    \pm{ 6     }$& 7.8   & 0.5  &0.012 & 0.382 \\
K02722.04  & 7673192    & 137.4936  &$    8.92108 ^{+    0.00000 }_{   -0.00000 }$&$ 0.95  ^{+ 0.01  }_{ -0.15 }$&$ 0.012  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 5.77  \pm{ 0.55  }$&$ 81.03 ^{+ 8.18  }_{ -1.40 }$&$ 5.3   ^{+ 0.4   }_{ -0.2  }$&$ 0.102  \pm{ 0.005  }$&$ 1769  \pm{ 136   }$&$ 121   \pm{ 10    }$& 4.1   & 1.6  &0.033 & 0.629 \\
K02722.05  & 7673192    & 135.3861  &$   16.53433 ^{+    0.00000 }_{   -0.00000 }$&$ 0.74  ^{+ 0.20  }_{ -0.74 }$&$ 0.011  ^{+ 0.033  }_{ -0.001 }$&$ 0.30  ^{+ 0.40  }_{ -0.30 }$&$ 4.69  ^{+ 1.60  }_{ -4.12 }$&$ 1.19  \pm{ 1.86  }$&$ 86.50 ^{+ 3.50  }_{ -2.16 }$&$ 8.8   ^{+ 2.5   }_{ -1.0  }$&$ 0.128  \pm{ 0.010  }$&$ 1236  \pm{ 353   }$&$ 92    \pm{ 13    }$& 4.3   & 0.5  &0.005 & 0.211 \\
K02732.01  & 9886361    & 134.4527  &$    7.03142 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.02  }_{ -0.00 }$&$ 0.011  ^{+ 0.000  }_{ -0.000 }$&$ 0.03  ^{+ 0.19  }_{ -0.03 }$&$ 0.09  ^{+ 1.49  }_{ -0.09 }$&$ 11.19 \pm{ 0.70  }$&$ 66.29 ^{+ 1.74  }_{ -1.04 }$&$ 2.4   ^{+ 0.0   }_{ -0.1  }$&$ 0.102  \pm{ 0.002  }$&$ 2702  \pm{ 59    }$&$ 85    \pm{ 7     }$& 6.6   & 0.2  &0.015 & 0.439 \\
K02732.02  & 9886361    & 144.1688  &$   13.61163 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.02  }_{ -0.06 }$&$ 0.011  ^{+ 0.000  }_{ -0.001 }$&$ 0.18  ^{+ 0.47  }_{ -0.18 }$&$ 0.00  ^{+ 0.14  }_{ -0.00 }$&$ 5.72  \pm{ 2.25  }$&$ 77.59 ^{+ 4.07  }_{ -16.16 }$&$ 4.1   ^{+ 1.3   }_{ -0.5  }$&$ 0.143  \pm{ 0.009  }$&$ 1956  \pm{ 218   }$&$ 96    \pm{ 10    }$& 8.2   & 0.2  &0.012 & 0.371 \\
K02732.03  & 9886361    & 140.7182  &$   54.28085 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.02  }_{ -0.97 }$&$ 0.015  ^{+ 0.008  }_{ -0.010 }$&$ 0.00  ^{+ 0.53  }_{ -0.00 }$&$ 3.46  ^{+ 2.83  }_{ -3.32 }$&$ 7.68  \pm{ 5.01  }$&$ 87.25 ^{+ 2.75  }_{ -1.13 }$&$ 10.8  ^{+ 2.4   }_{ -1.8  }$&$ 0.359  \pm{ 0.018  }$&$ 928   \pm{ 70    }$&$ 159   \pm{ 20    }$& 6.4   & 0.5  &0.031 & 0.613 \\
K02732.04  & 9886361    & 146.8040  &$   24.56084 ^{+    0.00000 }_{   -0.00000 }$&$ 0.71  ^{+ 0.17  }_{ -0.71 }$&$ 0.007  ^{+ 0.001  }_{ -0.005 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.04  ^{+ 0.30  }_{ -0.04 }$&$ 0.62  \pm{ 0.70  }$&$ 87.77 ^{+ 2.23  }_{ -2.40 }$&$ 9.2   ^{+ 3.6   }_{ -3.7  }$&$ 0.165  \pm{ 0.017  }$&$ 974   \pm{ 387   }$&$ 48    \pm{ 13    }$& 7.4   & 1.0  &0.006 & 0.225 \\
K02949.01  & 6026737    & 132.3611  &$   10.17444 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.03  }_{ -0.19 }$&$ 0.009  ^{+ 0.008  }_{ -0.007 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.09  }_{ -0.00 }$&$ 0.98  \pm{ 0.91  }$&$ 83.49 ^{+ 4.05  }_{ -0.79 }$&$ 7.7   ^{+ 2.1   }_{ -2.8  }$&$ 0.094  \pm{ 0.004  }$&$ 1447  \pm{ 182   }$&$ 61    \pm{ 12    }$& 4.1   & 0.6  &0.018 & 0.309 \\
K02949.02  & 6026737    & 134.8168  &$    3.75017 ^{+    0.00000 }_{   -0.00000 }$&$ 0.84  ^{+ 0.12  }_{ -0.35 }$&$ 0.005  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.10  }_{ -0.00 }$&$ 0.04  ^{+ 0.38  }_{ -0.04 }$&$ 0.50  \pm{ 0.36  }$&$ 78.28 ^{+ 7.73  }_{ -5.90 }$&$ 2.9   ^{+ 1.1   }_{ -0.9  }$&$ 0.048  \pm{ 0.005  }$&$ 2001  \pm{ 729   }$&$ 25    \pm{ 7     }$& 3.9   & 1.4  &0.006 & 0.124 \\
K03083.01  & 7106173    & 133.2040  &$   10.18329 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.04  }_{ -0.01 }$&$ 0.008  ^{+ 0.000  }_{ -0.006 }$&$ 0.03  ^{+ 0.67  }_{ -0.03 }$&$ 0.84  ^{+ 5.45  }_{ -0.74 }$&$ 2.35  \pm{ 1.00  }$&$ 83.49 ^{+ 1.06  }_{ -0.68 }$&$ 8.3   ^{+ 0.9   }_{ -0.6  }$&$ 0.104  \pm{ 0.003  }$&$ 1350  \pm{ 120   }$&$ 52    \pm{ 8     }$& 3.4   & 0.7  &0.005 & 0.194 \\
K03083.02  & 7106173    & 135.2410  &$    6.23203 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.06  }_{ -0.08 }$&$ 0.006  ^{+ 0.005  }_{ -0.002 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.61  \pm{ 0.38  }$&$ 80.56 ^{+ 1.92  }_{ -18.10 }$&$ 13.8  ^{+ 2.1   }_{ -1.6  }$&$ 0.068  \pm{ 0.003  }$&$ 1643  \pm{ 510   }$&$ 24    \pm{ 7     }$& 3.0   & 0.6  &0.005 & 0.194 \\
K03083.03  & 7106173    & 134.8440  &$    8.29442 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.04  }_{ -0.05 }$&$ 0.008  ^{+ 0.022  }_{ -0.002 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.00  ^{+ 0.16  }_{ -0.00 }$&$ 0.91  \pm{ 1.55  }$&$ 82.30 ^{+ 6.38  }_{ -0.68 }$&$ 16.2  ^{+ 1.4   }_{ -8.6  }$&$ 0.083  \pm{ 0.003  }$&$ 1466  \pm{ 514   }$&$ 41    \pm{ 8     }$& 2.7   & 0.3  &0.004 & 0.162 \\
K03097.01  & 7582689    & 137.4610  &$   11.92196 ^{+    0.00000 }_{   -0.00000 }$&$ 0.88  ^{+ 0.03  }_{ -0.88 }$&$ 0.007  ^{+ 0.033  }_{ -0.001 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.11  ^{+ 0.27  }_{ -0.11 }$&$ 2.38  \pm{ 5.44  }$&$ 83.97 ^{+ 6.03  }_{ -0.70 }$&$ 7.4   ^{+ 0.8   }_{ -0.3  }$&$ 0.107  \pm{ 0.003  }$&$ 1445  \pm{ 146   }$&$ 49    \pm{ 8     }$& 5.4   & 0.4  &0.024 & 0.555 \\
K03097.02  & 7582689    & 138.0420  &$    6.80273 ^{+    0.00000 }_{   -0.00000 }$&$ 0.91  ^{+ 0.08  }_{ -0.15 }$&$ 0.005  ^{+ 0.000  }_{ -0.003 }$&$ 0.53  ^{+ 0.16  }_{ -0.40 }$&$ 0.25  ^{+ 0.61  }_{ -0.24 }$&$ 1.19  \pm{ 0.43  }$&$ 82.39 ^{+ 4.20  }_{ -2.96 }$&$ 6.7   ^{+ 0.4   }_{ -0.7  }$&$ 0.073  \pm{ 0.002  }$&$ 1592  \pm{ 93    }$&$ 26    \pm{ 6     }$& 4.7   & 0.4  &0.007 & 0.264 \\
K03097.03  & 7582689    & 140.1620  &$    8.70295 ^{+    0.00000 }_{   -0.00000 }$&$ 0.92  ^{+ 0.08  }_{ -0.05 }$&$ 0.006  ^{+ 0.003  }_{ -0.001 }$&$ 0.03  ^{+ 0.67  }_{ -0.03 }$&$ 1.79  ^{+ 4.30  }_{ -1.53 }$&$ 1.46  \pm{ 0.55  }$&$ 83.13 ^{+ 1.15  }_{ -0.68 }$&$ 7.2   ^{+ 0.6   }_{ -1.5  }$&$ 0.086  \pm{ 0.003  }$&$ 1497  \pm{ 98    }$&$ 27    \pm{ 7     }$& 3.9   & 0.6  &0.006 & 0.229 \\
K03111.01  & 8581240    & 138.5101  &$   10.76792 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.02  }_{ -0.25 }$&$ 0.009  ^{+ 0.000  }_{ -0.003 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.01  ^{+ 0.32  }_{ -0.01 }$&$ 2.52  \pm{ 0.53  }$&$ 83.93 ^{+ 1.58  }_{ -1.08 }$&$ 8.0   ^{+ 0.9   }_{ -2.4  }$&$ 0.101  \pm{ 0.007  }$&$ 1333  \pm{ 448   }$&$ 65    \pm{ 9     }$& 3.7   & 0.6  &0.018 & 0.319 \\
K03111.02  & 8581240    & 132.5113  &$    4.32854 ^{+    0.00000 }_{   -0.00000 }$&$ 0.90  ^{+ 0.10  }_{ -0.13 }$&$ 0.006  ^{+ 0.045  }_{ -0.001 }$&$ 0.13  ^{+ 0.57  }_{ -0.13 }$&$ 0.03  ^{+ 0.65  }_{ -0.03 }$&$ 1.58  \pm{ 5.75  }$&$ 80.02 ^{+ 4.63  }_{ -4.51 }$&$ 4.6   ^{+ 0.5   }_{ -1.8  }$&$ 0.055  \pm{ 0.002  }$&$ 1735  \pm{ 440   }$&$ 34    \pm{ 6     }$& 3.0   & 0.8  &0.003 & 0.068 \\
K03158.01  & 6278762    & 133.2591  &$    3.60011 ^{+    0.00000 }_{   -0.00000 }$&$ 0.99  ^{+ 0.00  }_{ -0.00 }$&$ 0.007  ^{+ 0.000  }_{ -0.001 }$&$ 0.00  ^{+ 0.05  }_{ -0.00 }$&$ 0.62  ^{+ 5.67  }_{ -0.52 }$&$ 3.69  \pm{ 0.48  }$&$ 61.25 ^{+ 0.87  }_{ -0.90 }$&$ 2.0   ^{+ 0.0   }_{ -0.0  }$&$ 0.047  \pm{ 0.004  }$&$ 2349  \pm{ 43    }$&$ 26    \pm{ 1     }$& 2.6   & 2.6  &0.123 & 0.875 \\
K03158.02  & 6278762    & 131.5239  &$    4.54586 ^{+    0.00000 }_{   -0.00000 }$&$ 1.05  ^{+ -0.08 }_{ -0.08 }$&$ 0.060  ^{+ 0.000  }_{ -0.018 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.08  ^{+ 0.44  }_{ -0.08 }$&$ 45.54 \pm{ 7.50  }$&$ 60.00 ^{+ 0.90  }_{ -0.00 }$&$ 2.2   ^{+ 0.0   }_{ -0.2  }$&$ 0.068  \pm{ 0.003  }$&$ 2338  \pm{ 50    }$&$ 45    \pm{ 1     }$& 2.5   & 8.5  &0.243 & 0.941 \\
K03158.03  & 6278762    & 134.7885  &$    6.18936 ^{+    0.00000 }_{   -0.00000 }$&$ 1.02  ^{+ -0.02 }_{ -0.03 }$&$ 0.009  ^{+ 0.000  }_{ -0.002 }$&$ 0.17  ^{+ 0.13  }_{ -0.17 }$&$ 0.00  ^{+ 1.36  }_{ -0.00 }$&$ 5.02  \pm{ 1.30  }$&$ 74.29 ^{+ 8.01  }_{ -8.22 }$&$ 2.7   ^{+ 0.2   }_{ -0.3  }$&$ 0.082  \pm{ 0.009  }$&$ 1729  \pm{ 491   }$&$ 45    \pm{ 1     }$& 2.8   & 0.7  &0.227 & 0.936 \\
K03158.04  & 6278762    & 135.0872  &$    7.74359 ^{+    0.00000 }_{   -0.00000 }$&$ 0.99  ^{+ 0.01  }_{ -0.02 }$&$ 0.010  ^{+ 0.005  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.03  ^{+ 1.36  }_{ -0.03 }$&$ 3.61  \pm{ 1.34  }$&$ 74.64 ^{+ 4.94  }_{ -14.64 }$&$ 4.9   ^{+ 1.1   }_{ -1.7  }$&$ 0.079  \pm{ 0.006  }$&$ 1742  \pm{ 280   }$&$ 51    \pm{ 1     }$& 3.6   & 2.1  &0.190 & 0.921 \\
K03158.05  & 6278762    & 134.8777  &$    9.74050 ^{+    0.00000 }_{   -0.00000 }$&$ 1.25  ^{+ -0.27 }_{ -0.27 }$&$ 0.262  ^{+ 0.003  }_{ -0.195 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.38  }_{ -0.00 }$&$ 62.16 \pm{ 23.77 }$&$ 72.67 ^{+ 5.41  }_{ -6.42 }$&$ 8.5   ^{+ 0.3   }_{ -2.3  }$&$ 0.097  \pm{ 0.010  }$&$ 1656  \pm{ 138   }$&$ 70    \pm{ 1     }$& 2.5   & 1.1  &0.287 & 0.953 \\
K03196.01  & 9002538    & 135.3143  &$    4.96067 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.01  }_{ -0.13 }$&$ 0.006  ^{+ 0.050  }_{ -0.000 }$&$ 0.01  ^{+ 0.06  }_{ -0.01 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 2.96  \pm{ 12.52 }$&$ 74.29 ^{+ 8.14  }_{ -1.76 }$&$ 3.3   ^{+ 0.6   }_{ -1.4  }$&$ 0.072  \pm{ 0.010  }$&$ 2110  \pm{ 325   }$&$ 23    \pm{ 3     }$& 2.9   & 0.8  &0.013 & 0.244 \\
K03196.02  & 9002538    & 134.1634  &$    6.88299 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.03  }_{ -0.96 }$&$ 0.006  ^{+ 0.001  }_{ -0.004 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.02  }_{ -0.00 }$&$ 1.63  \pm{ 1.06  }$&$ 82.34 ^{+ 7.66  }_{ -5.10 }$&$ 3.9   ^{+ 1.3   }_{ -1.4  }$&$ 0.088  \pm{ 0.010  }$&$ 1506  \pm{ 768   }$&$ 25    \pm{ 3     }$& 2.2   & 1.5  &0.018 & 0.320 \\
K03384.01  & 8644365    & 139.0648  &$   10.54837 ^{+    0.00000 }_{   -0.00000 }$&$ 1.32  ^{+ -0.32 }_{ -0.38 }$&$ 0.016  ^{+ 0.030  }_{ -0.013 }$&$ 0.59  ^{+ 0.11  }_{ -0.46 }$&$ 3.38  ^{+ 2.76  }_{ -1.96 }$&$ 4.70  \pm{ 7.01  }$&$ 82.99 ^{+ 7.01  }_{ -8.37 }$&$ 4.3   ^{+ 2.7   }_{ -1.0  }$&$ 0.096  \pm{ 0.009  }$&$ 1072  \pm{ 513   }$&$ 98    \pm{ 11    }$& 1.4   & 1.3  &0.015 & 0.278 \\
K03384.02  & 8644365    & 139.3678  &$   19.91594 ^{+    0.00000 }_{   -0.00000 }$&$ 0.93  ^{+ 0.03  }_{ -0.07 }$&$ 0.013  ^{+ 0.026  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 1.01  }_{ -0.00 }$&$ 5.59  \pm{ 5.90  }$&$ 84.44 ^{+ 2.71  }_{ -1.48 }$&$ 8.6   ^{+ 1.3   }_{ -3.6  }$&$ 0.155  \pm{ 0.017  }$&$ 1184  \pm{ 177   }$&$ 138   \pm{ 16    }$& 6.4   & 0.9  &0.019 & 0.325 \\
K03398.01  & 3561464    & 137.2253  &$    7.31947 ^{+    0.00000 }_{   -0.00000 }$&$ 1.02  ^{+ -0.02 }_{ -0.04 }$&$ 0.015  ^{+ 0.000  }_{ -0.006 }$&$ 0.23  ^{+ 0.47  }_{ -0.23 }$&$ 0.07  ^{+ 1.18  }_{ -0.07 }$&$ 9.76  \pm{ 3.92  }$&$ 74.57 ^{+ 15.43 }_{ -4.71 }$&$ 2.8   ^{+ 0.5   }_{ -0.2  }$&$ 0.099  \pm{ 0.007  }$&$ 2104  \pm{ 1033  }$&$ 164   \pm{ 17    }$& 5.4   & 0.1  &0.013 & 0.395 \\
K03398.02  & 3561464    & 144.9642  &$   35.79896 ^{+    0.00000 }_{   -0.00000 }$&$ 0.87  ^{+ 0.08  }_{ -0.40 }$&$ 0.022  ^{+ 0.002  }_{ -0.003 }$&$ 0.06  ^{+ 0.62  }_{ -0.06 }$&$ 1.17  ^{+ 5.12  }_{ -1.16 }$&$ 6.07  \pm{ 2.92  }$&$ 87.30 ^{+ 1.55  }_{ -1.49 }$&$ 17.6  ^{+ 3.6   }_{ -5.1  }$&$ 0.221  \pm{ 0.020  }$&$ 953   \pm{ 154   }$&$ 461   \pm{ 49    }$& 8.5   & 0.3  &0.029 & 0.595 \\
K03398.03  & 3561464    & 131.6023  &$    4.32702 ^{+    0.00000 }_{   -0.00000 }$&$ 0.01  ^{+ 0.87  }_{ -0.01 }$&$ 0.009  ^{+ 0.000  }_{ -0.005 }$&$ 0.70  ^{+ -0.00 }_{ -0.05 }$&$ 0.89  ^{+ 0.79  }_{ -0.89 }$&$ 2.18  \pm{ 1.00  }$&$ 89.92 ^{+ 0.08  }_{ -13.65 }$&$ 3.8   ^{+ 0.8   }_{ -0.8  }$&$ 0.055  \pm{ 0.005  }$&$ 2114  \pm{ 307   }$&$ 96    \pm{ 12    }$& 4.1   & 0.7  &0.003 & 0.135 \\
K03403.01  & 11754430   & 166.6626  &$   39.81811 ^{+    0.00000 }_{   -0.00000 }$&$ 0.69  ^{+ 0.21  }_{ -0.54 }$&$ 0.013  ^{+ 0.001  }_{ -0.002 }$&$ 0.48  ^{+ 0.22  }_{ -0.43 }$&$ 0.34  ^{+ 3.24  }_{ -0.34 }$&$ 3.69  \pm{ 1.16  }$&$ 87.96 ^{+ 1.45  }_{ -1.91 }$&$ 17.9  ^{+ 3.3   }_{ -5.7  }$&$ 0.246  \pm{ 0.020  }$&$ 812   \pm{ 134   }$&$ 193   \pm{ 27    }$& 10.8  & 0.4  &0.032 & 0.455 \\
K03403.02  & 11754430   & 135.4936  &$    6.15844 ^{+    0.00000 }_{   -0.00000 }$&$ 0.84  ^{+ 0.16  }_{ -0.20 }$&$ 0.007  ^{+ 0.052  }_{ -0.001 }$&$ 0.00  ^{+ 0.00  }_{ -0.00 }$&$ 0.00  ^{+ 0.08  }_{ -0.00 }$&$ 2.00  \pm{ 7.25  }$&$ 81.32 ^{+ 4.66  }_{ -5.13 }$&$ 5.4   ^{+ 0.7   }_{ -1.2  }$&$ 0.070  \pm{ 0.006  }$&$ 1565  \pm{ 288   }$&$ 50    \pm{ 10    }$& 4.8   & 0.1  &0.007 & 0.155 \\
K03425.01  & 9117416    & 145.4378  &$   20.03515 ^{+    0.00000 }_{   -0.00000 }$&$ 1.03  ^{+ -0.04 }_{ -0.24 }$&$ 0.011  ^{+ 0.003  }_{ -0.001 }$&$ 0.24  ^{+ 0.39  }_{ -0.24 }$&$ 1.92  ^{+ 4.37  }_{ -1.35 }$&$ 3.25  \pm{ 0.95  }$&$ 84.45 ^{+ 2.77  }_{ -24.43 }$&$ 11.3  ^{+ 2.2   }_{ -4.6  }$&$ 0.154  \pm{ 0.009  }$&$ 1050  \pm{ 205   }$&$ 125   \pm{ 17    }$& 7.1   & 0.1  &0.003 & 0.064 \\
K03425.02  & 9117416    & 131.6995  &$    3.15720 ^{+    0.00000 }_{   -0.00000 }$&$ 0.89  ^{+ 0.11  }_{ -0.45 }$&$ 0.006  ^{+ 0.000  }_{ -0.002 }$&$ 0.63  ^{+ 0.05  }_{ -0.39 }$&$ 2.28  ^{+ 4.01  }_{ -1.15 }$&$ 1.75  \pm{ 0.54  }$&$ 75.52 ^{+ 11.92 }_{ -13.28 }$&$ 3.7   ^{+ 0.6   }_{ -0.6  }$&$ 0.045  \pm{ 0.002  }$&$ 1900  \pm{ 273   }$&$ 49    \pm{ 7     }$& 3.6   & 0.5  &0.003 & 0.071 \\
K03500.01  & 6058816    & 188.5180  &$   73.75110 ^{+    0.00000 }_{   -0.00000 }$&$ 0.47  ^{+ 0.18  }_{ -0.47 }$&$ 0.015  ^{+ 0.001  }_{ -0.008 }$&$ 0.23  ^{+ 0.47  }_{ -0.23 }$&$ 1.54  ^{+ 4.75  }_{ -1.52 }$&$ 3.96  \pm{ 1.41  }$&$ 89.15 ^{+ 0.85  }_{ -0.53 }$&$ 30.3  ^{+ 3.7   }_{ -6.9  }$&$ 0.366  \pm{ 0.026  }$&$ 676   \pm{ 82    }$&$ 259   \pm{ 32    }$& 13.4  & 0.2  &0.017 & 0.303 \\
K03500.02  & 6058816    & 135.8111  &$    4.74823 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.06  }_{ -0.04 }$&$ 0.007  ^{+ 0.018  }_{ -0.002 }$&$ 0.00  ^{+ 0.01  }_{ -0.00 }$&$ 0.12  ^{+ 0.21  }_{ -0.12 }$&$ 0.56  \pm{ 0.87  }$&$ 74.13 ^{+ 6.80  }_{ -1.92 }$&$ 1.9   ^{+ 1.9   }_{ -0.0  }$&$ 0.054  \pm{ 0.005  }$&$ 2085  \pm{ 1213  }$&$ 41    \pm{ 8     }$& 3.9   & 0.3  &0.004 & 0.095 \\
K03681.01  & 2581316    & 238.8192  &$  217.83189 ^{+    0.00000 }_{   -0.00000 }$&$ 0.55  ^{+ 0.22  }_{ -0.09 }$&$ 0.089  ^{+ 0.006  }_{ -0.003 }$&$ 0.70  ^{+ -0.00 }_{ -0.42 }$&$ 0.28  ^{+ 0.93  }_{ -0.28 }$&$ 38.10 \pm{ 9.18  }$&$ 89.36 ^{+ 0.07  }_{ -0.25 }$&$ 49.4  ^{+ 8.3   }_{ -7.7  }$&$ 0.868  \pm{ 0.044  }$&$ 581   \pm{ 57    }$&$ 9233  \pm{ 36    }$& 21.3  & 0.8  &0.910 & 0.996 \\
K03681.02  & 2581316    & 134.5660  &$   10.51420 ^{+    0.00000 }_{   -0.00000 }$&$ 1.77  ^{+ -0.78 }_{ -0.82 }$&$ 0.010  ^{+ 0.001  }_{ -0.000 }$&$ 0.48  ^{+ 0.17  }_{ -0.45 }$&$ 2.17  ^{+ 4.11  }_{ -0.98 }$&$ 1.18  \pm{ 1.35  }$&$ 60.00 ^{+ 15.41 }_{ -0.00 }$&$ 5.8   ^{+ 2.8   }_{ -2.2  }$&$ 0.113  \pm{ 0.011  }$&$ 2184  \pm{ 368   }$&$ 74    \pm{ 6     }$& 4.3   & 0.5  &0.005 & 0.107 \\
K03864.01  & 4164922    & 132.3795  &$    1.21073 ^{+    0.00000 }_{   -0.00000 }$&$ 0.74  ^{+ 0.21  }_{ -0.12 }$&$ 0.120  ^{+ 0.019  }_{ -0.081 }$&$ 0.64  ^{+ 0.06  }_{ -0.13 }$&$ 4.98  ^{+ 1.31  }_{ -0.41 }$&$ 33.52 \pm{ 14.16 }$&$ 67.29 ^{+ 4.26  }_{ -5.32 }$&$ 1.9   ^{+ 0.1   }_{ -0.3  }$&$ 0.023  \pm{ 0.001  }$&$ 2495  \pm{ 223   }$&$ 105   \pm{ 3     }$& 2.0   & 1.2  &0.175 & 0.841 \\
K03864.02  & 4164922    & 134.4413  &$   18.25734 ^{+    0.00000 }_{   -0.00000 }$&$ 1.85  ^{+ -0.85 }_{ -0.90 }$&$ 0.015  ^{+ 0.013  }_{ -0.003 }$&$ 0.70  ^{+ -0.00 }_{ -0.44 }$&$ 6.29  ^{+ -0.00 }_{ -4.77 }$&$ 4.17  \pm{ 3.31  }$&$ 79.86 ^{+ 4.49  }_{ -18.40 }$&$ 9.0   ^{+ 2.5   }_{ -4.2  }$&$ 0.143  \pm{ 0.013  }$&$ 1070  \pm{ 230   }$&$ 158   \pm{ 14    }$& 3.8   & 0.6  &0.030 & 0.434 \\
K04021.01  & 11967788   & 133.1229  &$    7.23530 ^{+    0.00000 }_{   -0.00000 }$&$ 1.71  ^{+ -0.73 }_{ -1.13 }$&$ 0.011  ^{+ 0.001  }_{ -0.003 }$&$ 0.65  ^{+ 0.05  }_{ -0.18 }$&$ 0.07  ^{+ 1.89  }_{ -0.07 }$&$ 8.71  \pm{ 2.50  }$&$ 69.86 ^{+ 14.04 }_{ -9.86 }$&$ 2.8   ^{+ 0.5   }_{ -0.2  }$&$ 0.100  \pm{ 0.004  }$&$ 1911  \pm{ 1130  }$&$ 109   \pm{ 7     }$& 3.4   & 1.8  &\nodata & \nodata \\
K04021.02  & 11967788   & 132.4534  &$    4.93209 ^{+    0.00000 }_{   -0.00000 }$&$ 0.96  ^{+ 0.02  }_{ -0.41 }$&$ 0.009  ^{+ 0.001  }_{ -0.002 }$&$ 0.00  ^{+ 0.26  }_{ -0.00 }$&$ 0.00  ^{+ 0.40  }_{ -0.00 }$&$ 3.73  \pm{ 2.19  }$&$ 73.03 ^{+ 11.70 }_{ -7.71 }$&$ 2.7   ^{+ 1.0   }_{ -0.8  }$&$ 0.071  \pm{ 0.006  }$&$ 2366  \pm{ 735   }$&$ 67    \pm{ 6     }$& 3.9   & 1.8  &\nodata & \nodata \\
K04032.01  & 7100673    & 134.2139  &$    3.95125 ^{+    0.00000 }_{   -0.00000 }$&$ 0.97  ^{+ 0.01  }_{ -0.40 }$&$ 0.010  ^{+ 0.001  }_{ -0.002 }$&$ 0.01  ^{+ 0.27  }_{ -0.01 }$&$ 0.27  ^{+ 1.38  }_{ -0.27 }$&$ 2.49  \pm{ 1.04  }$&$ 71.71 ^{+ 15.70 }_{ -7.75 }$&$ 1.8   ^{+ 0.8   }_{ -0.0  }$&$ 0.050  \pm{ 0.004  }$&$ 1990  \pm{ 500   }$&$ 62    \pm{ 5     }$& 2.9   & 0.3  &0.026 & 0.403 \\
K04032.02  & 7100673    & 132.8557  &$    2.89225 ^{+    0.00000 }_{   -0.00000 }$&$ 0.91  ^{+ 0.03  }_{ -0.91 }$&$ 0.008  ^{+ 0.000  }_{ -0.003 }$&$ 0.09  ^{+ 0.60  }_{ -0.09 }$&$ 3.79  ^{+ 2.50  }_{ -3.64 }$&$ 2.02  \pm{ 0.66  }$&$ 72.69 ^{+ 3.50  }_{ -3.17 }$&$ 2.7   ^{+ 0.5   }_{ -0.8  }$&$ 0.041  \pm{ 0.003  }$&$ 2048  \pm{ 250   }$&$ 41    \pm{ 4     }$& 2.6   & 1.4  &0.019 & 0.330 \\
K04097.01  & 5688683    & 133.1487  &$    2.79068 ^{+    0.00000 }_{   -0.00000 }$&$ 1.23  ^{+ -0.23 }_{ -0.24 }$&$ 0.048  ^{+ 0.057  }_{ -0.035 }$&$ 0.17  ^{+ 0.40  }_{ -0.17 }$&$ 1.08  ^{+ 5.21  }_{ -1.04 }$&$ 17.85 \pm{ 17.48 }$&$ 65.24 ^{+ 7.18  }_{ -5.24 }$&$ 2.5   ^{+ 0.4   }_{ -0.7  }$&$ 0.039  \pm{ 0.002  }$&$ 1877  \pm{ 193   }$&$ 158   \pm{ 6     }$& 1.4   & 0.3  &0.083 & 0.693 \\
K04097.02  & 5688683    & 131.7418  &$    4.44911 ^{+    0.00000 }_{   -0.00000 }$&$ 0.73  ^{+ 0.26  }_{ -0.45 }$&$ 0.009  ^{+ 0.005  }_{ -0.001 }$&$ 0.00  ^{+ 0.24  }_{ -0.00 }$&$ 0.15  ^{+ 2.54  }_{ -0.15 }$&$ 0.49  \pm{ 0.19  }$&$ 87.28 ^{+ 1.91  }_{ -16.80 }$&$ 17.4  ^{+ 4.1   }_{ -3.9  }$&$ 0.044  \pm{ 0.004  }$&$ 820   \pm{ 243   }$&$ 75    \pm{ 8     }$& 1.5   & 1.0  &0.012 & 0.228 \\
K04269.01  & 8890924    & 131.5999  &$   26.65626 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.06  }_{ -0.38 }$&$ 0.015  ^{+ 0.014  }_{ -0.003 }$&$ 0.12  ^{+ 0.58  }_{ -0.12 }$&$ 6.29  ^{+ -0.00 }_{ -4.72 }$&$ 3.60  \pm{ 2.54  }$&$ 86.69 ^{+ 3.10  }_{ -3.57 }$&$ 14.4  ^{+ 2.5   }_{ -4.9  }$&$ 0.187  \pm{ 0.013  }$&$ 837   \pm{ 339   }$&$ 159   \pm{ 24    }$& 5.1   & 0.4  &0.047 & 0.549 \\
K04269.02  & 8890924    & 135.2750  &$    4.44061 ^{+    0.00000 }_{   -0.00000 }$&$ 0.84  ^{+ 0.15  }_{ -0.21 }$&$ 0.006  ^{+ 0.049  }_{ -0.001 }$&$ 0.08  ^{+ 0.62  }_{ -0.08 }$&$ 0.01  ^{+ 0.32  }_{ -0.01 }$&$ 1.85  \pm{ 7.28  }$&$ 77.23 ^{+ 9.86  }_{ -5.79 }$&$ 3.8   ^{+ 0.9   }_{ -1.2  }$&$ 0.054  \pm{ 0.004  }$&$ 1714  \pm{ 329   }$&$ 36    \pm{ 10    }$& 5.1   & 0.3  &0.019 & 0.326 \\
K04288.01  & 4548011    & 133.1927  &$    6.28402 ^{+    0.00000 }_{   -0.00000 }$&$ 0.94  ^{+ 0.04  }_{ -0.16 }$&$ 0.006  ^{+ 0.015  }_{ -0.001 }$&$ 0.00  ^{+ 0.03  }_{ -0.00 }$&$ 0.32  ^{+ 2.94  }_{ -0.29 }$&$ 1.70  \pm{ 2.35  }$&$ 78.50 ^{+ 11.50 }_{ -5.32 }$&$ 4.2   ^{+ 1.4   }_{ -1.8  }$&$ 0.073  \pm{ 0.009  }$&$ 1759  \pm{ 403   }$&$ 31    \pm{ 5     }$& 3.6   & 0.7  &0.003 & 0.078 \\
K04288.02  & 4548011    & 139.9708  &$    9.08764 ^{+    0.00000 }_{   -0.00000 }$&$ 0.98  ^{+ 0.02  }_{ -0.07 }$&$ 0.007  ^{+ 0.024  }_{ -0.002 }$&$ 0.00  ^{+ 0.35  }_{ -0.00 }$&$ 0.00  ^{+ 1.02  }_{ -0.00 }$&$ 1.98  \pm{ 3.64  }$&$ 76.33 ^{+ 13.67 }_{ -6.21 }$&$ 6.9   ^{+ 3.8   }_{ -2.3  }$&$ 0.084  \pm{ 0.009  }$&$ 1891  \pm{ 490   }$&$ 34    \pm{ 6     }$& 3.8   & 0.9  &0.003 & 0.072 \\


\enddata


\tablecomments{The last three columns are significance of pixel centroid offset between in- and out-of-transit, planet confidence before and after considering the planetary likelihood boost in~\citet{Lissauer2012}. Planet candidates with significant pixel centroid offset ($> 3\sigma$) and planet candidates with higher than 0.997 planet confidence are marked in bold.}


\end{deluxetable}

\clearpage
 \end{landscape}


==> stellar_params.tex <==



\clearpage
%\longtable

\begin{landscape}
\begin{deluxetable}{lccccccccccll}
\tablewidth{0pt}
\tabletypesize{\tiny}
\setlength{\tabcolsep}{0.02in}
%\tablenum{1}
\tablecaption{RV and AO data for 56 KOIs\label{tab:stellar_params}}
\tablehead{
%\colhead{\textbf{ }} &
%\multicolumn{5}{c}{\textbf{KOI}} &
%\multicolumn{7}{c}{\textbf{Derived Values}} \\
\multicolumn{8}{c}{\textbf{KOI}} &
\multicolumn{3}{c}{\textbf{RV}} &
\multicolumn{2}{c}{\textbf{AO}} \\

\colhead{\textbf{KOI}} &
\colhead{\textbf{KIC}} &
\colhead{\textbf{$\alpha$}} &
\colhead{\textbf{$\delta$}} &
\colhead{\textbf{K$_P$}} &
\colhead{\textbf{$T_{\rm eff}$}} &
\colhead{\textbf{$\log g$}} &
\colhead{\textbf{\#PL}} &
\colhead{\textbf{$T_{\rm start}$}} &
\colhead{\textbf{$T_{\rm end}$}} &
\colhead{\textbf{\#RV}} &
\colhead{\textbf{Telescope}} &
\colhead{\textbf{Band}} \\

\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(deg)}} &
\colhead{\textbf{(deg)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(K)}} &
\colhead{\textbf{(cgs)}} &
\colhead{\textbf{}} &
\colhead{\textbf{(MJD)}} &
\colhead{\textbf{(MJD)}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{}} 

}

\startdata

00005&8554498&289.739716&44.647419&11.665&5861.00&4.190&2& 54983.516& 56486.440&21&Keck Palomar&Br-$\gamma$ J \\
00007&11853905&285.615326&50.135750&12.211&5858.00&4.280&1& 55041.491& 56134.480&22&Keck Palomar&H J \\
00010&6922244&281.288116&42.451080&13.563&6025.00&4.110&1& 54983.540& 55781.534&50&Palomar&J \\
00017&10874614&296.837250&48.239944&13.303&5826.00&4.420&1& 54984.561& 55043.520&10&Palomar&J \\
00018&8191672&299.407013&44.035053&13.369&6297.00&3.990&1& 54985.594& 55110.314&9&Gemini Gemini Palomar&R Y J \\
00020&11804465&286.243439&50.040379&13.438&6011.00&4.230&1& 55014.412& 55761.325&16&Palomar&J \\
00022&9631995&282.629669&46.323360&13.435&5972.00&4.410&1& 55014.403& 55792.438&16&Palomar&J \\
00041&6521045&291.385986&41.990269&11.197&5909.00&4.300&3& 54988.511& 56533.359&64&Keck Palomar&Br-$\gamma$ J \\
00069&3544595&291.418304&38.672359&9.931&5593.00&4.510&1& 55042.587& 56547.339&61&Keck MMT MMT Palomar&Br-$\gamma$ J K J \\
00070&6850504&287.697998&42.338718&12.498&5443.00&4.450&5& 55073.386& 56533.484&38&Palomar&J \\
00072&11904151&285.679382&50.241299&10.961&5627.00&4.390&2& 55073.400& 56172.301&54&MMT MMT Palomar&J K J \\
00082&10187017&281.482727&47.208031&11.492&4908.00&4.610&5& 55311.579& 56533.335&65&Keck MMT MMT&Br-$\gamma$ J K \\
00084&2571238&290.420807&37.851799&11.898&5541.00&4.530&1& 55073.419& 55723.450&20&Palomar&J \\
00085&5866724&288.688690&41.151180&11.018&6172.00&4.360&3& 55696.490& 55738.516&6&MMT MMT&J K \\
00087&10593626&289.217499&47.884460&11.664&5510.00&4.500&1& 55425.386& 56521.486&26&Palomar Palomar&J K \\
00103&2444412&291.683350&37.751591&12.593&5531.00&4.440&1& 55073.441& 55797.539&16&Palomar&J \\
00104&10318874&281.194733&47.497131&12.895&4786.00&4.590&1& 55377.342& 56525.316&30&Keck Palomar Palomar&K J K \\
00108&4914423&288.984558&40.064529&12.287&5975.00&4.330&2& 55073.469& 56145.498&22&Keck Palomar&K J \\
00111&6678383&287.604614&42.166779&12.596&5711.00&4.410&4& 55372.555& 56521.442&14&Palomar&J \\
00116&8395660&300.863983&44.337551&12.882&5865.00&4.410&4& 55133.397& 56532.332&33&Keck MMT&K K \\
00122&8349582&284.482452&44.398041&12.346&5714.00&4.390&1& 55073.495& 56151.511&33&Keck Palomar&K J \\
00123&5094751&290.392731&40.284870&12.365&5871.00&4.150&2& 55074.492& 56166.345&15&Keck Palomar&K J \\
00137&8644288&298.079437&44.746319&13.549&5385.00&4.430&3& 55075.509& 56146.484&20&Palomar&J \\
00148&5735762&299.139221&40.949020&13.040&5190.00&4.490&3& 55073.527& 56532.436&43&Keck Palomar&K J \\
00153&12252424&287.997894&50.944328&13.461&4725.00&4.640&2& 55313.592& 56524.353&29&Keck MMT Palomar Palomar&Br-$\gamma$ K J K \\
00157&6541920&297.115112&41.909142&13.709&5685.00&4.380&6& 55440.501& 56533.434&7&Palomar Robo-AO&LP600 \\
00180&9573539&284.394287&46.249081&13.024&5680.00&4.500&1& 55074.466& 55083.341&6&Palomar&J \\
00244&4349452&286.638397&39.487881&10.734&6103.00&4.070&2& 55366.603& 56519.408&104&Keck Palomar Palomar&Br-$\gamma$ J K \\
00245&8478994&284.059540&44.518215&9.705&5288.00&4.590&4& 55312.586& 56523.237&59&Gemini Gemini Keck MMT MMT Palomar&R Y Br-$\gamma$ J K K \\
00246&11295426&291.032318&49.040272&9.997&5793.00&4.281&2& 55312.582& 56519.420&65&Keck MMT MMT&Br-$\gamma$ J K \\
00261&5383248&297.069611&40.525131&10.297&5692.00&4.420&1& 55404.530& 56518.546&36&Keck MMT MMT&Br-$\gamma$ J K \\
00263&10514430&281.273804&47.774399&10.821&5820.00&4.150&1& 55395.529& 55788.482&6&MMT MMT Palomar Palomar&J K J K \\
00265&12024120&297.018829&50.408981&11.994&6040.00&4.360&1& 55782.522& 56532.354&27&Gemini Gemini Palomar Palomar&R Y J K \\
00273&3102384&287.478516&38.228840&11.457&5783.00&4.430&1& 55431.309& 56613.223&20&MMT MMT&J K \\
00274&8077137&282.492218&43.980209&11.390&6090.00&4.130&2& 55403.447& 56474.522&8&Gemini Gemini MMT MMT&R Y J K \\
00283&5695396&288.530823&40.942299&11.525&5687.00&4.420&2& 55433.368& 56524.331&30&Keck Palomar Palomar&Br-$\gamma$ J K \\
00289&10386922&282.945648&47.574905&12.747&5812.00&4.458&2& 56449.401& 56532.291&5&Lick&J \\
00292&11075737&287.326630&48.673431&12.872&5780.00&4.430&1& 55377.475& 56166.411&21&Keck Palomar Palomar&K J K \\
00299&2692377&285.661652&37.964500&12.899&5538.00&4.340&1& 55403.512& 56530.414&32&Keck&K \\
00305&6063220&297.354004&41.300049&12.970&4782.00&4.610&1& 55403.543& 56531.340&36&Keck&K \\
00321&8753657&291.848053&44.968220&12.520&5538.00&4.340&2& 55378.534& 56493.368&47&Keck Lick&K J \\
00364&7296438&295.872314&42.881149&10.087&5798.00&4.240&1& 55376.346& 55699.442&3&WIYN&$i$ \\
00365&11623629&297.486908&49.623451&11.195&5451.00&4.490&2& 55402.354& 56532.377&24&Palomar Palomar&J K \\
00377&3323887&285.573975&38.400902&13.803&5777.00&4.450&3& 55342.448& 56506.363&16&Palomar Palomar&J K \\
00701&9002278&283.212738&45.349861&13.725&4807.00&4.690&5& 56137.475& 56507.530&15&Keck&K \\
00975&3632418&287.361816&38.714016&8.224&6131.00&3.950&1& 55439.438& 56486.562&44&MMT MMT&J K \\
01431&11075279&287.022278&48.681938&13.460&5649.00&4.460&1& 56472.391& 56532.502&6&WIYN&$i$ \\
01439&11027624&290.851776&48.521339&12.849&5930.00&4.090&1& 55075.273& 56531.312&6&Lick&J \\
01442&11600889&286.036346&49.614510&12.521&5476.00&4.448&1& 55696.518& 56446.424&17&Keck Lick&K J \\
01463&7672940&288.258636&43.376465&12.328&6020.00&4.380&1& 56027.511& 56530.292&3&WIYN&$i$ \\
01612&10963065&284.786194&48.423229&8.769&6027.00&4.220&1& 55697.588& 56494.420&42&Keck Lick&Br-$\gamma$ J \\
01781&11551692&287.605591&49.523258&12.231&4977.00&4.590&3& 56076.566& 56112.331&9&Palomar Robo-AO&LP600 \\
01925&9955598&293.679199&46.852760&9.439&5365.00&4.430&1& 55999.646& 56547.332&40&Keck Palomar&Br-$\gamma$ K \\
02169&9006186&285.207489&45.384350&12.404&5447.00&4.420&4& 56099.455& 56171.456&4&Palomar Robo-AO&LP600 \\
02687&7202957&292.615112&42.764252&10.158&5803.00&3.910&2& 55999.652& 56531.383&22&Palomar&K \\
02720&8176564&295.439667&44.039162&10.338&6109.00&4.410&1& 56018.575& 56519.389&18&Keck Palomar&Br-$\gamma$ K \\

\enddata


%\tablecomments{Columns marked with a $^{\dagger}$ are values from NASA Exoplanet Archive. Stars marked with a $^{\dagger\dagger}$ have missing $T_{\rm{eff}}$. Their $T_{\rm{eff}}$ values are estimated based on $g-r$ and $g-i$ values~\citep{Pinsonneault2012}, the adopted $T_{\rm{eff}}$ is the average of the results. There are three exceptions, values of $T_{\rm{eff}}$ for K03158 and K0368 are adopted from~\citet{Ammons2006} and $T_{\rm{eff}}$ for K04021 is based on the infrared flux method in ~\citet{Pinsonneault2012}}


\end{deluxetable}

\clearpage
 \end{landscape}


==> stellar_params.tex.20131204.tex <==



\clearpage
%\longtable

\begin{landscape}
\begin{deluxetable}{lcccccccccccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\setlength{\tabcolsep}{0.02in}
%\tablenum{1}
\tablecaption{Stellar Parameters\label{tab:stellar_params}}
\tablehead{
\colhead{\textbf{ }} &
\multicolumn{7}{c}{\textbf{KOI}} &
\multicolumn{7}{c}{\textbf{Derived Values}} \\


\colhead{\textbf{KOI$^{\dagger}$}} &
\colhead{\textbf{KIC$^{\dagger}$}} &
\colhead{\textbf{$\alpha$$^{\dagger}$}} &
\colhead{\textbf{$\delta$$^{\dagger}$}} &
\colhead{\textbf{K$_P$$^{\dagger}$}} &
\colhead{\textbf{$T_{\rm eff}$$^{\dagger}$}} &
\colhead{\textbf{$\log g$$^{\dagger}$}} &
\colhead{\textbf{[Fe/H]$^{\dagger}$}} &
\colhead{\textbf{$T_{\rm eff}$}} &
\colhead{\textbf{$\log g$}} &
\colhead{\textbf{[Fe/H]}} &
\colhead{\textbf{M$_{\ast}$}} &
\colhead{\textbf{R$_{\ast}$}} &
\colhead{\textbf{L$_{\ast}$}} &
\colhead{\textbf{$\rho_{\ast}$}}  \\


\colhead{\textbf{}} &
\colhead{\textbf{}} &
\colhead{\textbf{(deg)}} &
\colhead{\textbf{(deg)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(K)}} &
\colhead{\textbf{(cgs)}} &
\colhead{\textbf{(dex)}} &
\colhead{\textbf{(K)}} &
\colhead{\textbf{(cgs)}} &
\colhead{\textbf{(dex)}} &
\colhead{\textbf{(M$_{\odot}$)}} &
\colhead{\textbf{(R$_{\odot}$)}} &
\colhead{\textbf{(L$_{\odot}$)}} &
\colhead{\textbf{(g~cm$^{-3}$)}} 

}

\startdata

K00005.01  & 8554498    & 289.739716      & 44.647419       & 11.66 & 5861       & 4.19       & 0.12       &$ 5862  ^{+ 44    }_{ -46   }$&$ 3.89  ^{+ 0.01  }_{ -0.00 }$&$ -0.23 ^{+ 0.21  }_{ -0.22 }$&$ 1.20  ^{+ 0.09  }_{ -0.18 }$&$ 2.04  ^{+ 0.07  }_{ -0.11 }$&$ 4.32  ^{+ 0.39  }_{ -0.55 }$&$ 0.20  \pm{ 0.03 }$ \\
K00005.02  & 8554498    & 289.739716      & 44.647419       & 11.66 & 5861       & 4.19       & 0.12       &$ 5883  ^{+ 136   }_{ -52   }$&$ 3.89  ^{+ 0.07  }_{ -0.00 }$&$ 0.03  ^{+ 0.22  }_{ -0.28 }$&$ 1.20  ^{+ 0.12  }_{ -0.14 }$&$ 1.96  ^{+ 0.28  }_{ -0.28 }$&$ 1.10  ^{+ 1.68  }_{ -0.24 }$&$ 0.23  \pm{ 0.10 }$ \\
K00041.01  & 6521045    & 291.385986      & 41.990269       & 11.20 & 5909       & 4.30       & -0.12      &$ 5904  ^{+ 58    }_{ -72   }$&$ 3.65  ^{+ 0.07  }_{ -0.45 }$&$ -0.51 ^{+ 0.34  }_{ -0.41 }$&$ 1.22  ^{+ 0.16  }_{ -0.15 }$&$ 2.41  ^{+ 0.27  }_{ -0.62 }$&$ 6.01  ^{+ 1.35  }_{ -2.65 }$&$ 0.12  \pm{ 0.07 }$ \\
K00041.02  & 6521045    & 291.385986      & 41.990269       & 11.20 & 5909       & 4.30       & -0.12      &$ 5894  ^{+ 55    }_{ -77   }$&$ 3.65  ^{+ 0.04  }_{ -0.10 }$&$ -0.77 ^{+ 0.35  }_{ -0.62 }$&$ 1.15  ^{+ 0.15  }_{ -0.17 }$&$ 2.71  ^{+ 0.20  }_{ -0.47 }$&$ 8.18  ^{+ 1.37  }_{ -1.94 }$&$ 0.08  \pm{ 0.03 }$ \\
K00041.03  & 6521045    & 291.385986      & 41.990269       & 11.20 & 5909       & 4.30       & -0.12      &$ 5914  ^{+ 65    }_{ -55   }$&$ 3.68  ^{+ 0.07  }_{ -0.15 }$&$ -0.63 ^{+ 0.32  }_{ -0.73 }$&$ 1.18  ^{+ 0.14  }_{ -0.26 }$&$ 2.59  ^{+ 0.36  }_{ -0.34 }$&$ 6.27  ^{+ 1.69  }_{ -2.55 }$&$ 0.10  \pm{ 0.04 }$ \\
K00070.01  & 6850504    & 287.697998      & 42.338718       & 12.50 & 5443       & 4.45       & -0.15      &$ 5443  ^{+ 37    }_{ -47   }$&$ 4.40  ^{+ 0.04  }_{ -0.21 }$&$ 0.13  ^{+ 0.36  }_{ -0.21 }$&$ 0.91  ^{+ 0.06  }_{ -0.07 }$&$ 0.95  ^{+ 0.06  }_{ -0.12 }$&$ 0.71  ^{+ 0.10  }_{ -0.18 }$&$ 1.47  \pm{ 0.43 }$ \\
K00070.02  & 6850504    & 287.697998      & 42.338718       & 12.50 & 5443       & 4.45       & -0.15      &$ 5453  ^{+ 40    }_{ -40   }$&$ 4.43  ^{+ 0.05  }_{ -0.08 }$&$ -0.22 ^{+ 0.22  }_{ -0.73 }$&$ 0.82  ^{+ 0.07  }_{ -0.14 }$&$ 0.92  ^{+ 0.08  }_{ -0.11 }$&$ 0.72  ^{+ 0.15  }_{ -0.12 }$&$ 1.50  \pm{ 0.49 }$ \\
K00070.03  & 6850504    & 287.697998      & 42.338718       & 12.50 & 5443       & 4.45       & -0.15      &$ 5455  ^{+ 51    }_{ -39   }$&$ 4.47  ^{+ 0.07  }_{ -0.04 }$&$ -0.16 ^{+ 0.18  }_{ -0.43 }$&$ 0.86  ^{+ 0.06  }_{ -0.14 }$&$ 0.91  ^{+ 0.06  }_{ -0.09 }$&$ 0.66  ^{+ 0.09  }_{ -0.11 }$&$ 1.59  \pm{ 0.44 }$ \\
K00070.04  & 6850504    & 287.697998      & 42.338718       & 12.50 & 5443       & 4.45       & -0.15      &$ 5426  ^{+ 39    }_{ -133  }$&$ 4.43  ^{+ 0.04  }_{ -0.21 }$&$ -0.09 ^{+ 0.24  }_{ -0.29 }$&$ 0.84  ^{+ 0.06  }_{ -0.18 }$&$ 0.92  ^{+ 0.06  }_{ -0.12 }$&$ 0.69  ^{+ 0.10  }_{ -0.14 }$&$ 1.52  \pm{ 0.50 }$ \\
K00070.05  & 6850504    & 287.697998      & 42.338718       & 12.50 & 5443       & 4.45       & -0.15      &$ 5427  ^{+ 33    }_{ -65   }$&$ 4.42  ^{+ 0.04  }_{ -0.26 }$&$ 0.01  ^{+ 0.23  }_{ -0.23 }$&$ 0.87  ^{+ 0.07  }_{ -0.11 }$&$ 0.95  ^{+ 0.08  }_{ -0.08 }$&$ 0.73  ^{+ 0.13  }_{ -0.12 }$&$ 1.41  \pm{ 0.38 }$ \\
K00072.01  & 11904151   & 285.679382      & 50.241299       & 10.96 & 5627       & 4.39       & -0.81      &$ 5571  ^{+ 62    }_{ -91   }$&$ 4.39  ^{+ 0.02  }_{ -0.02 }$&$ -0.14 ^{+ 0.13  }_{ -0.17 }$&$ 0.93  ^{+ 0.08  }_{ -0.05 }$&$ 1.00  ^{+ 0.02  }_{ -0.13 }$&$ 0.94  ^{+ 0.06  }_{ -0.09 }$&$ 1.29  \pm{ 0.30 }$ \\
K00072.02  & 11904151   & 285.679382      & 50.241299       & 10.96 & 5627       & 4.39       & -0.81      &$ 5624  ^{+ 49    }_{ -72   }$&$ 4.41  ^{+ 0.04  }_{ -0.07 }$&$ -0.23 ^{+ 0.19  }_{ -0.21 }$&$ 0.85  ^{+ 0.06  }_{ -0.08 }$&$ 0.94  ^{+ 0.08  }_{ -0.17 }$&$ 0.77  ^{+ 0.16  }_{ -0.37 }$&$ 1.44  \pm{ 0.58 }$ \\
K00082.01  & 10187017   & 281.482727      & 47.208031       & 11.49 & 4908       & 4.61       & 0.20       &$ 4901  ^{+ 32    }_{ -189  }$&$ 4.56  ^{+ 0.01  }_{ -0.03 }$&$ 0.30  ^{+ 0.15  }_{ -0.23 }$&$ 0.85  ^{+ 0.02  }_{ -0.02 }$&$ 0.78  ^{+ 0.01  }_{ -0.09 }$&$ 0.32  ^{+ 0.02  }_{ -0.03 }$&$ 2.47  \pm{ 0.50 }$ \\
K00082.02  & 10187017   & 281.482727      & 47.208031       & 11.49 & 4908       & 4.61       & 0.20       &$ 4927  ^{+ 40    }_{ -38   }$&$ 4.56  ^{+ 0.02  }_{ -0.03 }$&$ 0.32  ^{+ 0.15  }_{ -0.21 }$&$ 0.85  ^{+ 0.02  }_{ -0.02 }$&$ 0.78  ^{+ 0.02  }_{ -0.13 }$&$ 0.32  ^{+ 0.02  }_{ -0.11 }$&$ 2.47  \pm{ 0.68 }$ \\
K00082.03  & 10187017   & 281.482727      & 47.208031       & 11.49 & 4908       & 4.61       & 0.20       &$ 4905  ^{+ 38    }_{ -61   }$&$ 4.55  ^{+ 0.02  }_{ -0.08 }$&$ 0.51  ^{+ 0.09  }_{ -0.18 }$&$ 0.84  ^{+ 0.02  }_{ -0.03 }$&$ 0.79  ^{+ 0.02  }_{ -0.02 }$&$ 0.32  ^{+ 0.02  }_{ -0.03 }$&$ 2.36  \pm{ 0.19 }$ \\
K00082.04  & 10187017   & 281.482727      & 47.208031       & 11.49 & 4908       & 4.61       & 0.20       &$ 4908  ^{+ 42    }_{ -41   }$&$ 4.55  ^{+ 0.02  }_{ -0.08 }$&$ 0.36  ^{+ 0.18  }_{ -0.18 }$&$ 0.84  ^{+ 0.02  }_{ -0.04 }$&$ 0.78  ^{+ 0.02  }_{ -0.07 }$&$ 0.31  ^{+ 0.02  }_{ -0.10 }$&$ 2.46  \pm{ 0.44 }$ \\
K00082.05  & 10187017   & 281.482727      & 47.208031       & 11.49 & 4908       & 4.61       & 0.20       &$ 4903  ^{+ 34    }_{ -58   }$&$ 4.56  ^{+ 0.01  }_{ -0.05 }$&$ 0.56  ^{+ 0.04  }_{ -0.18 }$&$ 0.83  ^{+ 0.02  }_{ -0.07 }$&$ 0.79  ^{+ 0.01  }_{ -0.04 }$&$ 0.32  ^{+ 0.02  }_{ -0.07 }$&$ 2.38  \pm{ 0.26 }$ \\
K00085.01  & 5866724    & 288.688690      & 41.151180       & 11.02 & 6172       & 4.36       & -0.05      &$ 6165  ^{+ 34    }_{ -120  }$&$ 4.23  ^{+ 0.04  }_{ -0.05 }$&$ 0.16  ^{+ 0.16  }_{ -0.59 }$&$ 1.32  ^{+ 0.06  }_{ -0.06 }$&$ 1.46  ^{+ 0.07  }_{ -0.09 }$&$ 2.81  ^{+ 0.35  }_{ -0.39 }$&$ 0.60  \pm{ 0.10 }$ \\
K00085.02  & 5866724    & 288.688690      & 41.151180       & 11.02 & 6172       & 4.36       & -0.05      &$ 6169  ^{+ 44    }_{ -60   }$&$ 4.21  ^{+ 0.03  }_{ -0.14 }$&$ 0.37  ^{+ 0.13  }_{ -0.20 }$&$ 1.38  ^{+ 0.09  }_{ -0.06 }$&$ 1.46  ^{+ 0.14  }_{ -0.09 }$&$ 2.67  ^{+ 0.26  }_{ -0.58 }$&$ 0.63  \pm{ 0.15 }$ \\
K00085.03  & 5866724    & 288.688690      & 41.151180       & 11.02 & 6172       & 4.36       & -0.05      &$ 6181  ^{+ 44    }_{ -44   }$&$ 4.23  ^{+ 0.07  }_{ -0.10 }$&$ 0.55  ^{+ 0.05  }_{ -0.18 }$&$ 1.28  ^{+ 0.07  }_{ -0.21 }$&$ 1.48  ^{+ 0.24  }_{ -0.11 }$&$ 2.68  ^{+ 0.41  }_{ -0.66 }$&$ 0.55  \pm{ 0.20 }$ \\
K00089.01  & 8056665    & 299.821167      & 43.814270       & 11.64 & 7713       & 3.90       & 0.06       &$ 7621  ^{+ 191   }_{ -203  }$&$ 3.57  ^{+ 0.04  }_{ -0.22 }$&$ -0.40 ^{+ 0.34  }_{ -0.73 }$&$ 2.08  ^{+ 0.21  }_{ -0.17 }$&$ 3.66  ^{+ 0.24  }_{ -1.14 }$&$ 40.69 ^{+ 5.48  }_{ -22.52 }$&$ 0.06  \pm{ 0.03 }$ \\
K00089.02  & 8056665    & 299.821167      & 43.814270       & 11.64 & 7713       & 3.90       & 0.06       &$ 7543  ^{+ 173   }_{ -348  }$&$ 3.56  ^{+ 0.05  }_{ -0.16 }$&$ -0.06 ^{+ 0.62  }_{ -0.39 }$&$ 2.06  ^{+ 0.21  }_{ -0.18 }$&$ 3.85  ^{+ 0.24  }_{ -0.26 }$&$ 41.33 ^{+ 5.68  }_{ -12.65 }$&$ 0.05  \pm{ 0.01 }$ \\
K00094.01  & 6462863    & 297.333069      & 41.891121       & 12.21 & 6184       & 4.18       & -0.76      &$ 6122  ^{+ 58    }_{ -104  }$&$ 4.01  ^{+ 0.05  }_{ -0.03 }$&$ -0.04 ^{+ 0.11  }_{ -0.13 }$&$ 1.35  ^{+ 0.10  }_{ -0.07 }$&$ 1.86  ^{+ 0.10  }_{ -0.28 }$&$ 4.60  ^{+ 1.22  }_{ -1.06 }$&$ 0.30  \pm{ 0.09 }$ \\
K00094.02  & 6462863    & 297.333069      & 41.891121       & 12.21 & 6184       & 4.18       & -0.76      &$ 6179  ^{+ 46    }_{ -68   }$&$ 4.02  ^{+ 0.09  }_{ -0.04 }$&$ -0.11 ^{+ 0.10  }_{ -0.41 }$&$ 1.27  ^{+ 0.07  }_{ -0.08 }$&$ 1.44  ^{+ 0.22  }_{ -0.31 }$&$ 2.73  ^{+ 1.04  }_{ -1.16 }$&$ 0.60  \pm{ 0.33 }$ \\
K00094.03  & 6462863    & 297.333069      & 41.891121       & 12.21 & 6184       & 4.18       & -0.76      &$ 6167  ^{+ 52    }_{ -168  }$&$ 4.31  ^{+ 0.06  }_{ -0.19 }$&$ -0.10 ^{+ 0.12  }_{ -0.14 }$&$ 1.12  ^{+ 0.09  }_{ -0.10 }$&$ 1.21  ^{+ 0.17  }_{ -0.10 }$&$ 1.98  ^{+ 0.68  }_{ -0.45 }$&$ 0.88  \pm{ 0.30 }$ \\
K00094.04  & 6462863    & 297.333069      & 41.891121       & 12.21 & 6184       & 4.18       & -0.76      &$ 6188  ^{+ 49    }_{ -69   }$&$ 4.32  ^{+ 0.05  }_{ -0.05 }$&$ -0.20 ^{+ 0.10  }_{ -0.26 }$&$ 1.10  ^{+ 0.04  }_{ -0.07 }$&$ 1.18  ^{+ 0.05  }_{ -0.07 }$&$ 1.92  ^{+ 0.24  }_{ -0.37 }$&$ 0.95  \pm{ 0.15 }$ \\
K00102.01  & 8456679    & 299.704742      & 44.435749       & 12.57 & 5838       & 4.42       & -0.36      &$ 5803  ^{+ 27    }_{ -68   }$&$ 4.29  ^{+ 0.05  }_{ -0.06 }$&$ 0.32  ^{+ 0.15  }_{ -0.19 }$&$ 1.18  ^{+ 0.02  }_{ -0.06 }$&$ 1.27  ^{+ 0.03  }_{ -0.14 }$&$ 1.74  ^{+ 0.25  }_{ -0.25 }$&$ 0.81  \pm{ 0.16 }$ \\
K00102.02  & 8456679    & 299.704742      & 44.435749       & 12.57 & 5838       & 4.42       & -0.36      &$ 5818  ^{+ 42    }_{ -132  }$&$ 4.42  ^{+ 0.06  }_{ -0.19 }$&$ -0.02 ^{+ 0.32  }_{ -0.31 }$&$ 1.03  ^{+ 0.09  }_{ -0.12 }$&$ 0.99  ^{+ 0.10  }_{ -0.14 }$&$ 1.02  ^{+ 0.24  }_{ -0.26 }$&$ 1.49  \pm{ 0.56 }$ \\
K00108.01  & 4914423    & 288.984558      & 40.064529       & 12.29 & 5975       & 4.33       & -0.10      &$ 5973  ^{+ 40    }_{ -51   }$&$ 4.36  ^{+ 0.03  }_{ -0.33 }$&$ -0.14 ^{+ 0.17  }_{ -0.80 }$&$ 1.08  ^{+ 0.07  }_{ -0.07 }$&$ 1.09  ^{+ 0.06  }_{ -0.14 }$&$ 1.34  ^{+ 0.14  }_{ -0.52 }$&$ 1.17  \pm{ 0.32 }$ \\
K00108.02  & 4914423    & 288.984558      & 40.064529       & 12.29 & 5975       & 4.33       & -0.10      &$ 5946  ^{+ 35    }_{ -102  }$&$ 4.35  ^{+ 0.07  }_{ -0.07 }$&$ 0.08  ^{+ 0.25  }_{ -0.16 }$&$ 1.12  ^{+ 0.08  }_{ -0.08 }$&$ 1.19  ^{+ 0.14  }_{ -0.13 }$&$ 1.53  ^{+ 0.29  }_{ -0.41 }$&$ 0.95  \pm{ 0.33 }$ \\
K00111.01  & 6678383    & 287.604614      & 42.166779       & 12.60 & 5711       & 4.41       & -0.78      &$ 5680  ^{+ 39    }_{ -90   }$&$ 4.49  ^{+ 0.03  }_{ -0.16 }$&$ -0.83 ^{+ 0.21  }_{ -0.76 }$&$ 0.73  ^{+ 0.03  }_{ -0.06 }$&$ 0.79  ^{+ 0.06  }_{ -0.13 }$&$ 0.59  ^{+ 0.09  }_{ -0.19 }$&$ 2.10  \pm{ 0.74 }$ \\
K00111.02  & 6678383    & 287.604614      & 42.166779       & 12.60 & 5711       & 4.41       & -0.78      &$ 5712  ^{+ 49    }_{ -48   }$&$ 4.32  ^{+ 0.01  }_{ -0.09 }$&$ -0.40 ^{+ 0.13  }_{ -0.18 }$&$ 0.82  ^{+ 0.03  }_{ -0.08 }$&$ 1.02  ^{+ 0.03  }_{ -0.04 }$&$ 1.02  ^{+ 0.06  }_{ -0.11 }$&$ 1.09  \pm{ 0.14 }$ \\
K00111.03  & 6678383    & 287.604614      & 42.166779       & 12.60 & 5711       & 4.41       & -0.78      &$ 5741  ^{+ 56    }_{ -40   }$&$ 4.41  ^{+ 0.04  }_{ -0.08 }$&$ -0.44 ^{+ 0.14  }_{ -0.20 }$&$ 0.82  ^{+ 0.05  }_{ -0.04 }$&$ 0.93  ^{+ 0.05  }_{ -0.10 }$&$ 0.85  ^{+ 0.12  }_{ -0.15 }$&$ 1.43  \pm{ 0.34 }$ \\
K00112.01  & 10984090   & 295.648712      & 48.495560       & 12.77 & 5853       & 4.46       & -0.59      &$ 5834  ^{+ 42    }_{ -151  }$&$ 4.46  ^{+ 0.04  }_{ -0.05 }$&$ -0.31 ^{+ 0.16  }_{ -0.71 }$&$ 0.96  ^{+ 0.06  }_{ -0.19 }$&$ 0.93  ^{+ 0.07  }_{ -0.10 }$&$ 0.90  ^{+ 0.15  }_{ -0.20 }$&$ 1.66  \pm{ 0.51 }$ \\
K00112.02  & 10984090   & 295.648712      & 48.495560       & 12.77 & 5853       & 4.46       & -0.59      &$ 5850  ^{+ 45    }_{ -49   }$&$ 4.52  ^{+ 0.07  }_{ -0.05 }$&$ -0.49 ^{+ 0.23  }_{ -0.77 }$&$ 0.90  ^{+ 0.08  }_{ -0.14 }$&$ 0.83  ^{+ 0.08  }_{ -0.12 }$&$ 0.70  ^{+ 0.16  }_{ -0.20 }$&$ 2.22  \pm{ 0.85 }$ \\
K00115.01  & 9579641    & 287.887329      & 46.276241       & 12.79 & 6398       & 4.25       & -0.22      &$ 6345  ^{+ 78    }_{ -129  }$&$ 3.74  ^{+ 0.07  }_{ -0.07 }$&$ -0.46 ^{+ 0.43  }_{ -0.33 }$&$ 1.22  ^{+ 0.09  }_{ -0.09 }$&$ 2.59  ^{+ 0.26  }_{ -0.26 }$&$ 8.89  ^{+ 1.77  }_{ -4.62 }$&$ 0.10  \pm{ 0.03 }$ \\
K00115.02  & 9579641    & 287.887329      & 46.276241       & 12.79 & 6398       & 4.25       & -0.22      &$ 6356  ^{+ 73    }_{ -94   }$&$ 3.58  ^{+ 0.11  }_{ -0.16 }$&$ -0.45 ^{+ 0.55  }_{ -0.37 }$&$ 1.28  ^{+ 0.10  }_{ -0.26 }$&$ 2.61  ^{+ 0.39  }_{ -1.32 }$&$ 9.87  ^{+ 3.01  }_{ -7.41 }$&$ 0.10  \pm{ 0.10 }$ \\
K00115.03  & 9579641    & 287.887329      & 46.276241       & 12.79 & 6398       & 4.25       & -0.22      &$ 6367  ^{+ 74    }_{ -111  }$&$ 3.68  ^{+ 0.07  }_{ -0.08 }$&$ -0.46 ^{+ 0.43  }_{ -0.40 }$&$ 1.25  ^{+ 0.12  }_{ -0.18 }$&$ 2.71  ^{+ 0.22  }_{ -0.39 }$&$ 10.42 ^{+ 2.03  }_{ -8.00 }$&$ 0.09  \pm{ 0.03 }$ \\
K00116.01  & 8395660    & 300.863983      & 44.337551       & 12.88 & 5865       & 4.41       & -0.36      &$ 5784  ^{+ 70    }_{ -253  }$&$ 3.84  ^{+ 0.03  }_{ -0.02 }$&$ -0.45 ^{+ 0.27  }_{ -0.48 }$&$ 1.05  ^{+ 0.14  }_{ -0.17 }$&$ 2.12  ^{+ 0.11  }_{ -0.14 }$&$ 4.73  ^{+ 0.84  }_{ -0.53 }$&$ 0.16  \pm{ 0.04 }$ \\
K00116.02  & 8395660    & 300.863983      & 44.337551       & 12.88 & 5865       & 4.41       & -0.36      &$ 5884  ^{+ 97    }_{ -102  }$&$ 4.39  ^{+ 0.04  }_{ -0.49 }$&$ -0.13 ^{+ 0.31  }_{ -0.26 }$&$ 0.94  ^{+ 0.08  }_{ -0.21 }$&$ 0.97  ^{+ 0.08  }_{ -0.19 }$&$ 1.04  ^{+ 0.19  }_{ -0.44 }$&$ 1.46  \pm{ 0.65 }$ \\
K00116.03  & 8395660    & 300.863983      & 44.337551       & 12.88 & 5865       & 4.41       & -0.36      &$ 5822  ^{+ 77    }_{ -273  }$&$ 4.40  ^{+ 0.08  }_{ -0.53 }$&$ -0.51 ^{+ 0.28  }_{ -1.00 }$&$ 0.88  ^{+ 0.11  }_{ -0.17 }$&$ 0.96  ^{+ 0.19  }_{ -0.26 }$&$ 0.93  ^{+ 0.37  }_{ -0.45 }$&$ 1.38  \pm{ 0.98 }$ \\
K00116.04  & 8395660    & 300.863983      & 44.337551       & 12.88 & 5865       & 4.41       & -0.36      &$ 5878  ^{+ 87    }_{ -94   }$&$ 4.44  ^{+ 0.07  }_{ -0.07 }$&$ -0.38 ^{+ 0.25  }_{ -0.46 }$&$ 0.88  ^{+ 0.09  }_{ -0.16 }$&$ 0.95  ^{+ 0.11  }_{ -0.14 }$&$ 0.90  ^{+ 0.23  }_{ -0.37 }$&$ 1.45  \pm{ 0.62 }$ \\
K00117.01  & 10875245   & 297.028259      & 48.208611       & 12.49 & 5949       & 4.37       & -0.09      &$ 5963  ^{+ 49    }_{ -55   }$&$ 3.41  ^{+ 0.06  }_{ -0.18 }$&$ -0.39 ^{+ 0.36  }_{ -0.79 }$&$ 1.87  ^{+ 0.30  }_{ -0.24 }$&$ 3.97  ^{+ 0.48  }_{ -0.86 }$&$ 16.57 ^{+ 3.49  }_{ -5.70 }$&$ 0.04  \pm{ 0.02 }$ \\
K00117.02  & 10875245   & 297.028259      & 48.208611       & 12.49 & 5949       & 4.37       & -0.09      &$ 5929  ^{+ 51    }_{ -61   }$&$ 3.11  ^{+ 0.15  }_{ -0.18 }$&$ -0.31 ^{+ 0.43  }_{ -0.57 }$&$ 1.95  ^{+ 0.25  }_{ -0.26 }$&$ 3.95  ^{+ 1.13  }_{ -1.07 }$&$ 13.46 ^{+ 9.82  }_{ -4.56 }$&$ 0.04  \pm{ 0.04 }$ \\
K00117.03  & 10875245   & 297.028259      & 48.208611       & 12.49 & 5949       & 4.37       & -0.09      &$ 5940  ^{+ 41    }_{ -55   }$&$ 3.41  ^{+ 0.03  }_{ -0.25 }$&$ -0.44 ^{+ 0.42  }_{ -0.60 }$&$ 1.57  ^{+ 0.22  }_{ -0.34 }$&$ 4.19  ^{+ 0.25  }_{ -0.27 }$&$ 17.73 ^{+ 1.93  }_{ -7.22 }$&$ 0.03  \pm{ 0.01 }$ \\
K00117.04  & 10875245   & 297.028259      & 48.208611       & 12.49 & 5949       & 4.37       & -0.09      &$ 5922  ^{+ 41    }_{ -105  }$&$ 3.40  ^{+ 0.15  }_{ -0.13 }$&$ -0.17 ^{+ 0.45  }_{ -0.50 }$&$ 1.84  ^{+ 0.26  }_{ -0.27 }$&$ 3.77  ^{+ 0.84  }_{ -1.48 }$&$ 23.51 ^{+ 12.18 }_{ -8.42 }$&$ 0.05  \pm{ 0.05 }$ \\
K00119.01  & 9471974    & 294.559174      & 46.062328       & 12.65 & 5632       & 4.44       & -0.03      &$ 5571  ^{+ 114   }_{ -154  }$&$ 3.92  ^{+ 0.17  }_{ -0.09 }$&$ -0.22 ^{+ 0.42  }_{ -0.38 }$&$ 1.09  ^{+ 0.16  }_{ -0.14 }$&$ 1.89  ^{+ 0.27  }_{ -0.39 }$&$ 2.96  ^{+ 0.73  }_{ -1.18 }$&$ 0.23  \pm{ 0.12 }$ \\
K00119.02  & 9471974    & 294.559174      & 46.062328       & 12.65 & 5632       & 4.44       & -0.03      &$ 5583  ^{+ 120   }_{ -126  }$&$ 3.90  ^{+ 0.16  }_{ -0.08 }$&$ -0.62 ^{+ 0.35  }_{ -0.56 }$&$ 1.03  ^{+ 0.14  }_{ -0.14 }$&$ 1.71  ^{+ 0.22  }_{ -0.32 }$&$ 2.70  ^{+ 0.86  }_{ -1.12 }$&$ 0.29  \pm{ 0.14 }$ \\
K00123.01  & 5094751    & 290.392731      & 40.284870       & 12.37 & 5871       & 4.15       & -0.05      &$ 5887  ^{+ 62    }_{ -42   }$&$ 3.85  ^{+ 0.07  }_{ -0.00 }$&$ -0.22 ^{+ 0.22  }_{ -0.20 }$&$ 1.03  ^{+ 0.05  }_{ -0.14 }$&$ 1.82  ^{+ 0.15  }_{ -0.17 }$&$ 3.47  ^{+ 0.56  }_{ -0.71 }$&$ 0.24  \pm{ 0.07 }$ \\
K00123.02  & 5094751    & 290.392731      & 40.284870       & 12.37 & 5871       & 4.15       & -0.05      &$ 5880  ^{+ 56    }_{ -38   }$&$ 3.94  ^{+ 0.06  }_{ -0.07 }$&$ -0.36 ^{+ 0.14  }_{ -0.48 }$&$ 1.05  ^{+ 0.05  }_{ -0.07 }$&$ 1.79  ^{+ 0.12  }_{ -0.16 }$&$ 3.15  ^{+ 0.46  }_{ -1.65 }$&$ 0.26  \pm{ 0.06 }$ \\
K00124.01  & 11086270   & 292.929138      & 48.602810       & 12.94 & 5899       & 4.07       & -0.15      &$ 5877  ^{+ 43    }_{ -86   }$&$ 3.85  ^{+ 0.05  }_{ -0.05 }$&$ -0.52 ^{+ 0.24  }_{ -0.21 }$&$ 1.02  ^{+ 0.05  }_{ -0.12 }$&$ 1.98  ^{+ 0.09  }_{ -0.17 }$&$ 4.19  ^{+ 0.37  }_{ -0.92 }$&$ 0.19  \pm{ 0.04 }$ \\
K00124.02  & 11086270   & 292.929138      & 48.602810       & 12.94 & 5899       & 4.07       & -0.15      &$ 5879  ^{+ 40    }_{ -99   }$&$ 3.85  ^{+ 0.05  }_{ -0.08 }$&$ -0.44 ^{+ 0.22  }_{ -0.24 }$&$ 1.06  ^{+ 0.10  }_{ -0.07 }$&$ 1.98  ^{+ 0.15  }_{ -0.12 }$&$ 3.77  ^{+ 0.47  }_{ -1.45 }$&$ 0.19  \pm{ 0.04 }$ \\
K00139.01  & 8559644    & 291.653168      & 44.688271       & 13.49 & 5952       & 4.38       & 0.01       &$ 5949  ^{+ 39    }_{ -42   }$&$ 4.41  ^{+ 0.04  }_{ -0.04 }$&$ 0.05  ^{+ 0.18  }_{ -0.23 }$&$ 1.13  ^{+ 0.08  }_{ -0.07 }$&$ 1.06  ^{+ 0.07  }_{ -0.14 }$&$ 1.22  ^{+ 0.17  }_{ -0.42 }$&$ 1.32  \pm{ 0.40 }$ \\
K00139.02  & 8559644    & 291.653168      & 44.688271       & 13.49 & 5952       & 4.38       & 0.01       &$ 5957  ^{+ 43    }_{ -41   }$&$ 4.39  ^{+ 0.03  }_{ -0.03 }$&$ 0.17  ^{+ 0.19  }_{ -0.19 }$&$ 1.13  ^{+ 0.05  }_{ -0.08 }$&$ 1.14  ^{+ 0.05  }_{ -0.07 }$&$ 1.43  ^{+ 0.16  }_{ -0.20 }$&$ 1.09  \pm{ 0.19 }$ \\
K00148.01  & 5735762    & 299.139221      & 40.949020       & 13.04 & 5190       & 4.49       & -0.22      &$ 5189  ^{+ 41    }_{ -56   }$&$ 4.45  ^{+ 0.03  }_{ -0.05 }$&$ 0.15  ^{+ 0.18  }_{ -0.32 }$&$ 0.91  ^{+ 0.06  }_{ -0.03 }$&$ 0.98  ^{+ 0.14  }_{ -0.06 }$&$ 0.54  ^{+ 0.07  }_{ -0.11 }$&$ 1.34  \pm{ 0.42 }$ \\
K00148.02  & 5735762    & 299.139221      & 40.949020       & 13.04 & 5190       & 4.49       & -0.22      &$ 5187  ^{+ 36    }_{ -48   }$&$ 4.46  ^{+ 0.03  }_{ -0.16 }$&$ 0.09  ^{+ 0.19  }_{ -0.24 }$&$ 0.89  ^{+ 0.05  }_{ -0.05 }$&$ 0.89  ^{+ 0.05  }_{ -0.06 }$&$ 0.49  ^{+ 0.06  }_{ -0.10 }$&$ 1.80  \pm{ 0.33 }$ \\
K00148.03  & 5735762    & 299.139221      & 40.949020       & 13.04 & 5190       & 4.49       & -0.22      &$ 5182  ^{+ 37    }_{ -53   }$&$ 4.48  ^{+ 0.03  }_{ -0.15 }$&$ 0.08  ^{+ 0.20  }_{ -0.27 }$&$ 0.89  ^{+ 0.06  }_{ -0.05 }$&$ 0.87  ^{+ 0.04  }_{ -0.09 }$&$ 0.50  ^{+ 0.07  }_{ -0.06 }$&$ 1.94  \pm{ 0.44 }$ \\
K00153.01  & 12252424   & 287.997894      & 50.944328       & 13.46 & 4725       & 4.64       & 0.17       &$ 4731  ^{+ 41    }_{ -44   }$&$ 4.61  ^{+ 0.02  }_{ -0.05 }$&$ 0.19  ^{+ 0.21  }_{ -0.27 }$&$ 0.78  ^{+ 0.02  }_{ -0.04 }$&$ 0.72  ^{+ 0.03  }_{ -0.05 }$&$ 0.22  ^{+ 0.03  }_{ -0.05 }$&$ 2.98  \pm{ 0.51 }$ \\
K00153.02  & 12252424   & 287.997894      & 50.944328       & 13.46 & 4725       & 4.64       & 0.17       &$ 4747  ^{+ 42    }_{ -40   }$&$ 4.60  ^{+ 0.02  }_{ -0.03 }$&$ 0.55  ^{+ 0.05  }_{ -0.18 }$&$ 0.78  ^{+ 0.02  }_{ -0.05 }$&$ 0.73  ^{+ 0.02  }_{ -0.12 }$&$ 0.24  ^{+ 0.02  }_{ -0.08 }$&$ 2.88  \pm{ 0.79 }$ \\
K00159.01  & 8972058    & 297.711853      & 45.261921       & 13.43 & 6069       & 4.30       & -0.08      &$ 6070  ^{+ 85    }_{ -85   }$&$ 3.78  ^{+ 0.08  }_{ -0.12 }$&$ -0.42 ^{+ 0.36  }_{ -0.40 }$&$ 1.15  ^{+ 0.13  }_{ -0.17 }$&$ 2.25  ^{+ 0.22  }_{ -0.34 }$&$ 5.48  ^{+ 1.30  }_{ -3.78 }$&$ 0.14  \pm{ 0.06 }$ \\
K00159.02  & 8972058    & 297.711853      & 45.261921       & 13.43 & 6069       & 4.30       & -0.08      &$ 6050  ^{+ 67    }_{ -108  }$&$ 3.73  ^{+ 0.06  }_{ -0.25 }$&$ -0.77 ^{+ 0.33  }_{ -0.78 }$&$ 1.15  ^{+ 0.11  }_{ -0.15 }$&$ 2.44  ^{+ 0.22  }_{ -0.21 }$&$ 6.29  ^{+ 1.16  }_{ -3.42 }$&$ 0.11  \pm{ 0.03 }$ \\
K00168.01  & 11512246   & 294.218933      & 49.479221       & 13.44 & 6142       & 3.97       & -0.33      &$ 6097  ^{+ 109   }_{ -140  }$&$ 3.75  ^{+ 0.06  }_{ -0.09 }$&$ -0.81 ^{+ 0.34  }_{ -0.46 }$&$ 1.06  ^{+ 0.09  }_{ -0.13 }$&$ 2.23  ^{+ 0.22  }_{ -0.66 }$&$ 6.99  ^{+ 1.29  }_{ -1.48 }$&$ 0.13  \pm{ 0.08 }$ \\
K00168.02  & 11512246   & 294.218933      & 49.479221       & 13.44 & 6142       & 3.97       & -0.33      &$ 6123  ^{+ 124   }_{ -97   }$&$ 3.75  ^{+ 0.08  }_{ -0.09 }$&$ -0.71 ^{+ 0.36  }_{ -0.32 }$&$ 1.08  ^{+ 0.08  }_{ -0.12 }$&$ 2.27  ^{+ 0.22  }_{ -0.84 }$&$ 7.36  ^{+ 1.74  }_{ -1.51 }$&$ 0.13  \pm{ 0.09 }$ \\
K00168.03  & 11512246   & 294.218933      & 49.479221       & 13.44 & 6142       & 3.97       & -0.33      &$ 6152  ^{+ 139   }_{ -116  }$&$ 3.77  ^{+ 0.08  }_{ -0.11 }$&$ -0.54 ^{+ 0.58  }_{ -0.35 }$&$ 1.08  ^{+ 0.09  }_{ -0.17 }$&$ 2.33  ^{+ 0.30  }_{ -0.26 }$&$ 5.42  ^{+ 1.43  }_{ -2.96 }$&$ 0.12  \pm{ 0.05 }$ \\
K00244.01  & 4349452    & 286.638397      & 39.487881       & 10.73 & 6103       & 4.07       & \nodata    &$ 6076  ^{+ 34    }_{ -114  }$&$ 4.00  ^{+ 0.15  }_{ -0.13 }$&$ -0.08 ^{+ 0.19  }_{ -0.28 }$&$ 1.21  ^{+ 0.08  }_{ -0.09 }$&$ 2.12  ^{+ 0.40  }_{ -0.28 }$&$ 4.09  ^{+ 1.19  }_{ -2.42 }$&$ 0.18  \pm{ 0.09 }$ \\
K00244.02  & 4349452    & 286.638397      & 39.487881       & 10.73 & 6103       & 4.07       & \nodata    &$ 6096  ^{+ 37    }_{ -53   }$&$ 3.82  ^{+ 0.04  }_{ -0.05 }$&$ -0.46 ^{+ 0.23  }_{ -0.43 }$&$ 1.19  ^{+ 0.09  }_{ -0.14 }$&$ 2.14  ^{+ 0.15  }_{ -0.28 }$&$ 5.89  ^{+ 0.95  }_{ -1.13 }$&$ 0.17  \pm{ 0.05 }$ \\
K00245.01  & 8478994    & 284.059540      & 44.518215       & 9.71  & 5288       & 4.59       & \nodata    &$ 5288  ^{+ 41    }_{ -49   }$&$ 4.44  ^{+ 0.04  }_{ -0.15 }$&$ 0.15  ^{+ 0.22  }_{ -0.25 }$&$ 0.91  ^{+ 0.05  }_{ -0.06 }$&$ 0.94  ^{+ 0.08  }_{ -0.07 }$&$ 0.58  ^{+ 0.08  }_{ -0.10 }$&$ 1.53  \pm{ 0.37 }$ \\
K00245.02  & 8478994    & 284.059540      & 44.518215       & 9.71  & 5288       & 4.59       & \nodata    &$ 5298  ^{+ 43    }_{ -39   }$&$ 4.47  ^{+ 0.05  }_{ -0.05 }$&$ 0.05  ^{+ 0.20  }_{ -0.31 }$&$ 0.93  ^{+ 0.07  }_{ -0.05 }$&$ 0.89  ^{+ 0.06  }_{ -0.25 }$&$ 0.54  ^{+ 0.08  }_{ -0.27 }$&$ 1.88  \pm{ 1.00 }$ \\
K00245.03  & 8478994    & 284.059540      & 44.518215       & 9.71  & 5288       & 4.59       & \nodata    &$ 5293  ^{+ 47    }_{ -42   }$&$ 4.41  ^{+ 0.05  }_{ -0.11 }$&$ -0.01 ^{+ 0.22  }_{ -0.85 }$&$ 0.92  ^{+ 0.07  }_{ -0.06 }$&$ 0.94  ^{+ 0.08  }_{ -0.08 }$&$ 0.54  ^{+ 0.10  }_{ -0.17 }$&$ 1.55  \pm{ 0.40 }$ \\
K00245.04  & 8478994    & 284.059540      & 44.518215       & 9.71  & 5288       & 4.59       & \nodata    &$ 5295  ^{+ 47    }_{ -38   }$&$ 4.45  ^{+ 0.04  }_{ -0.14 }$&$ 0.03  ^{+ 0.23  }_{ -0.33 }$&$ 0.91  ^{+ 0.09  }_{ -0.06 }$&$ 0.94  ^{+ 0.19  }_{ -0.06 }$&$ 0.61  ^{+ 0.11  }_{ -0.10 }$&$ 1.52  \pm{ 0.62 }$ \\
K00246.01  & 11295426   & 291.032318      & 49.040272       & 10.00 & 5793       & 4.28       & 0.15       &$ 5782  ^{+ 32    }_{ -61   }$&$ 4.28  ^{+ 0.01  }_{ -0.01 }$&$ 0.09  ^{+ 0.06  }_{ -0.06 }$&$ 1.07  ^{+ 0.04  }_{ -0.03 }$&$ 1.23  ^{+ 0.02  }_{ -0.03 }$&$ 1.56  ^{+ 0.07  }_{ -0.07 }$&$ 0.80  \pm{ 0.06 }$ \\
K00246.02  & 11295426   & 291.032318      & 49.040272       & 10.00 & 5793       & 4.28       & 0.15       &$ 5807  ^{+ 49    }_{ -37   }$&$ 4.28  ^{+ 0.01  }_{ -0.02 }$&$ 0.04  ^{+ 0.05  }_{ -0.21 }$&$ 1.06  ^{+ 0.03  }_{ -0.04 }$&$ 1.24  ^{+ 0.02  }_{ -0.03 }$&$ 1.56  ^{+ 0.07  }_{ -0.07 }$&$ 0.79  \pm{ 0.05 }$ \\
K00260.01  & 8292840    & 289.347321      & 44.208511       & 10.50 & 6164       & 4.28       & \nodata    &$ 6170  ^{+ 62    }_{ -48   }$&$ 4.38  ^{+ 0.07  }_{ -0.08 }$&$ -0.30 ^{+ 0.19  }_{ -0.29 }$&$ 1.01  ^{+ 0.09  }_{ -0.17 }$&$ 1.10  ^{+ 0.13  }_{ -0.14 }$&$ 1.45  ^{+ 0.36  }_{ -0.58 }$&$ 1.07  \pm{ 0.42 }$ \\
K00260.02  & 8292840    & 289.347321      & 44.208511       & 10.50 & 6164       & 4.28       & \nodata    &$ 6161  ^{+ 53    }_{ -49   }$&$ 3.98  ^{+ 0.06  }_{ -0.00 }$&$ -0.02 ^{+ 0.29  }_{ -0.16 }$&$ 1.26  ^{+ 0.16  }_{ -0.12 }$&$ 1.78  ^{+ 0.20  }_{ -0.44 }$&$ 1.76  ^{+ 0.65  }_{ -0.42 }$&$ 0.32  \pm{ 0.18 }$ \\
K00260.03  & 8292840    & 289.347321      & 44.208511       & 10.50 & 6164       & 4.28       & \nodata    &$ 6141  ^{+ 49    }_{ -74   }$&$ 4.38  ^{+ 0.06  }_{ -0.05 }$&$ -0.34 ^{+ 0.18  }_{ -0.41 }$&$ 1.04  ^{+ 0.08  }_{ -0.10 }$&$ 1.11  ^{+ 0.09  }_{ -0.12 }$&$ 1.52  ^{+ 0.29  }_{ -0.34 }$&$ 1.06  \pm{ 0.31 }$ \\
K00262.01  & 11807274   & 288.100861      & 50.033718       & 10.42 & 6058       & 3.98       & -0.35      &$ 6066  ^{+ 55    }_{ -48   }$&$ 3.69  ^{+ 0.04  }_{ -0.01 }$&$ -0.69 ^{+ 0.21  }_{ -0.31 }$&$ 1.17  ^{+ 0.13  }_{ -0.08 }$&$ 2.39  ^{+ 0.11  }_{ -0.19 }$&$ 6.60  ^{+ 0.73  }_{ -1.51 }$&$ 0.12  \pm{ 0.03 }$ \\
K00262.02  & 11807274   & 288.100861      & 50.033718       & 10.42 & 6058       & 3.98       & -0.35      &$ 6053  ^{+ 48    }_{ -48   }$&$ 3.71  ^{+ 0.03  }_{ -0.03 }$&$ -0.74 ^{+ 0.19  }_{ -0.39 }$&$ 1.16  ^{+ 0.08  }_{ -0.10 }$&$ 2.53  ^{+ 0.32  }_{ -0.10 }$&$ 7.16  ^{+ 0.55  }_{ -1.02 }$&$ 0.10  \pm{ 0.03 }$ \\
K00270.01  & 6528464    & 293.732819      & 41.900829       & 11.41 & 5552       & 4.08       & \nodata    &$ 5535  ^{+ 42    }_{ -75   }$&$ 3.89  ^{+ 0.06  }_{ -0.11 }$&$ -0.42 ^{+ 0.21  }_{ -0.25 }$&$ 0.91  ^{+ 0.06  }_{ -0.05 }$&$ 1.73  ^{+ 0.10  }_{ -0.11 }$&$ 2.46  ^{+ 0.30  }_{ -0.32 }$&$ 0.25  \pm{ 0.05 }$ \\
K00270.02  & 6528464    & 293.732819      & 41.900829       & 11.41 & 5552       & 4.08       & \nodata    &$ 5550  ^{+ 49    }_{ -57   }$&$ 3.96  ^{+ 0.06  }_{ -0.05 }$&$ -0.37 ^{+ 0.22  }_{ -0.19 }$&$ 0.90  ^{+ 0.05  }_{ -0.09 }$&$ 1.62  ^{+ 0.08  }_{ -0.29 }$&$ 2.31  ^{+ 0.24  }_{ -0.62 }$&$ 0.30  \pm{ 0.11 }$ \\
K00271.01  & 9451706    & 285.190002      & 46.027962       & 11.48 & 6169       & 4.33       & -0.15      &$ 6160  ^{+ 43    }_{ -50   }$&$ 4.38  ^{+ 0.02  }_{ -0.04 }$&$ 0.01  ^{+ 0.17  }_{ -0.20 }$&$ 1.16  ^{+ 0.06  }_{ -0.13 }$&$ 1.15  ^{+ 0.05  }_{ -0.07 }$&$ 1.69  ^{+ 0.17  }_{ -0.25 }$&$ 1.07  \pm{ 0.20 }$ \\
K00271.02  & 9451706    & 285.190002      & 46.027962       & 11.48 & 6169       & 4.33       & -0.15      &$ 6135  ^{+ 42    }_{ -113  }$&$ 4.35  ^{+ 0.03  }_{ -0.03 }$&$ 0.21  ^{+ 0.17  }_{ -0.20 }$&$ 1.25  ^{+ 0.04  }_{ -0.10 }$&$ 1.21  ^{+ 0.06  }_{ -0.30 }$&$ 1.88  ^{+ 0.23  }_{ -0.86 }$&$ 0.98  \pm{ 0.45 }$ \\
K00271.03  & 9451706    & 285.190002      & 46.027962       & 11.48 & 6169       & 4.33       & -0.15      &$ 6180  ^{+ 49    }_{ -44   }$&$ 4.34  ^{+ 0.05  }_{ -0.23 }$&$ 0.12  ^{+ 0.25  }_{ -0.28 }$&$ 1.24  ^{+ 0.11  }_{ -0.10 }$&$ 1.21  ^{+ 0.13  }_{ -0.12 }$&$ 1.81  ^{+ 0.37  }_{ -0.36 }$&$ 0.99  \pm{ 0.32 }$ \\
K00274.01  & 8077137    & 282.492218      & 43.980209       & 11.39 & 6090       & 4.13       & -0.05      &$ 6058  ^{+ 84    }_{ -126  }$&$ 3.83  ^{+ 0.07  }_{ -0.00 }$&$ -0.13 ^{+ 0.23  }_{ -0.26 }$&$ 1.09  ^{+ 0.14  }_{ -0.20 }$&$ 1.13  ^{+ 0.71  }_{ -0.16 }$&$ 1.39  ^{+ 1.13  }_{ -0.35 }$&$ 1.06  \pm{ 1.23 }$ \\
K00274.02  & 8077137    & 282.492218      & 43.980209       & 11.39 & 6090       & 4.13       & -0.05      &$ 6098  ^{+ 97    }_{ -89   }$&$ 4.33  ^{+ 0.09  }_{ -0.30 }$&$ -0.09 ^{+ 0.26  }_{ -0.22 }$&$ 1.08  ^{+ 0.11  }_{ -0.18 }$&$ 1.07  ^{+ 0.15  }_{ -0.08 }$&$ 1.52  ^{+ 0.54  }_{ -0.40 }$&$ 1.23  \pm{ 0.42 }$ \\
K00275.01  & 10586004   & 285.311249      & 47.848564       & 11.70 & 5795       & 4.24       & \nodata    &$ 5788  ^{+ 46    }_{ -79   }$&$ 3.99  ^{+ 0.03  }_{ -0.03 }$&$ 0.38  ^{+ 0.13  }_{ -0.13 }$&$ 1.27  ^{+ 0.05  }_{ -0.14 }$&$ 1.89  ^{+ 0.08  }_{ -0.10 }$&$ 3.60  ^{+ 0.32  }_{ -0.42 }$&$ 0.26  \pm{ 0.04 }$ \\
K00275.02  & 10586004   & 285.311249      & 47.848564       & 11.70 & 5795       & 4.24       & \nodata    &$ 5795  ^{+ 48    }_{ -52   }$&$ 4.37  ^{+ 0.07  }_{ -0.29 }$&$ 0.15  ^{+ 0.19  }_{ -0.32 }$&$ 1.07  ^{+ 0.08  }_{ -0.22 }$&$ 1.11  ^{+ 0.28  }_{ -0.18 }$&$ 1.07  ^{+ 0.29  }_{ -0.37 }$&$ 1.10  \pm{ 0.70 }$ \\
K00277.01  & 11401755   & 291.250183      & 49.231834       & 11.87 & 5973       & 4.06       & \nodata    &$ 5979  ^{+ 60    }_{ -46   }$&$ 3.84  ^{+ 0.04  }_{ -0.08 }$&$ -0.41 ^{+ 0.23  }_{ -0.25 }$&$ 1.04  ^{+ 0.07  }_{ -0.12 }$&$ 2.03  ^{+ 0.11  }_{ -0.19 }$&$ 4.64  ^{+ 0.56  }_{ -0.87 }$&$ 0.18  \pm{ 0.04 }$ \\
K00277.02  & 11401755   & 291.250183      & 49.231834       & 11.87 & 5973       & 4.06       & \nodata    &$ 5983  ^{+ 50    }_{ -44   }$&$ 3.84  ^{+ 0.06  }_{ -0.06 }$&$ -0.48 ^{+ 0.22  }_{ -0.30 }$&$ 1.05  ^{+ 0.07  }_{ -0.14 }$&$ 2.04  ^{+ 0.13  }_{ -0.15 }$&$ 4.62  ^{+ 0.57  }_{ -0.84 }$&$ 0.17  \pm{ 0.04 }$ \\
K00279.01  & 12314973   & 295.486511      & 51.013500       & 11.68 & 6418       & 4.28       & -0.34      &$ 6432  ^{+ 83    }_{ -54   }$&$ 3.70  ^{+ 0.07  }_{ -0.09 }$&$ -0.66 ^{+ 0.32  }_{ -0.49 }$&$ 1.29  ^{+ 0.12  }_{ -0.15 }$&$ 2.67  ^{+ 0.26  }_{ -0.90 }$&$ 11.95 ^{+ 2.10  }_{ -2.55 }$&$ 0.10  \pm{ 0.06 }$ \\
K00279.02  & 12314973   & 295.486511      & 51.013500       & 11.68 & 6418       & 4.28       & -0.34      &$ 6408  ^{+ 56    }_{ -67   }$&$ 3.64  ^{+ 0.06  }_{ -0.12 }$&$ -0.87 ^{+ 0.33  }_{ -0.67 }$&$ 1.33  ^{+ 0.13  }_{ -0.15 }$&$ 2.80  ^{+ 0.24  }_{ -0.32 }$&$ 11.83 ^{+ 1.97  }_{ -2.83 }$&$ 0.09  \pm{ 0.03 }$ \\
K00279.03  & 12314973   & 295.486511      & 51.013500       & 11.68 & 6418       & 4.28       & -0.34      &$ 6442  ^{+ 97    }_{ -66   }$&$ 3.39  ^{+ 0.20  }_{ -0.00 }$&$ -0.55 ^{+ 0.31  }_{ -0.43 }$&$ 1.01  ^{+ 0.26  }_{ -0.21 }$&$ 1.09  ^{+ 1.25  }_{ -0.20 }$&$ 1.11  ^{+ 1.41  }_{ -0.00 }$&$ 1.10  \pm{ 2.21 }$ \\
K00282.01  & 5088536    & 288.450653      & 40.245327       & 11.53 & 5873       & 4.33       & \nodata    &$ 5858  ^{+ 38    }_{ -57   }$&$ 4.37  ^{+ 0.08  }_{ -0.05 }$&$ -0.19 ^{+ 0.18  }_{ -0.18 }$&$ 0.96  ^{+ 0.07  }_{ -0.08 }$&$ 1.09  ^{+ 0.08  }_{ -0.08 }$&$ 1.18  ^{+ 0.17  }_{ -0.31 }$&$ 1.05  \pm{ 0.25 }$ \\
K00282.02  & 5088536    & 288.450653      & 40.245327       & 11.53 & 5873       & 4.33       & \nodata    &$ 5868  ^{+ 38    }_{ -53   }$&$ 4.37  ^{+ 0.05  }_{ -0.14 }$&$ -0.29 ^{+ 0.18  }_{ -0.26 }$&$ 0.92  ^{+ 0.07  }_{ -0.09 }$&$ 0.96  ^{+ 0.09  }_{ -0.20 }$&$ 0.95  ^{+ 0.19  }_{ -0.33 }$&$ 1.49  \pm{ 0.67 }$ \\
K00282.03  & 5088536    & 288.450653      & 40.245327       & 11.53 & 5873       & 4.33       & \nodata    &$ 5845  ^{+ 46    }_{ -93   }$&$ 4.44  ^{+ 0.06  }_{ -0.09 }$&$ -0.29 ^{+ 0.22  }_{ -0.26 }$&$ 0.87  ^{+ 0.08  }_{ -0.13 }$&$ 0.87  ^{+ 0.09  }_{ -0.10 }$&$ 0.90  ^{+ 0.28  }_{ -0.30 }$&$ 1.83  \pm{ 0.63 }$ \\
K00283.01  & 5695396    & 288.530823      & 40.942299       & 11.53 & 5687       & 4.42       & 0.06       &$ 5662  ^{+ 34    }_{ -138  }$&$ 4.40  ^{+ 0.04  }_{ -0.19 }$&$ 0.04  ^{+ 0.23  }_{ -0.22 }$&$ 1.06  ^{+ 0.19  }_{ -0.07 }$&$ 1.05  ^{+ 0.11  }_{ -0.07 }$&$ 0.95  ^{+ 0.13  }_{ -0.18 }$&$ 1.27  \pm{ 0.36 }$ \\
K00283.02  & 5695396    & 288.530823      & 40.942299       & 11.53 & 5687       & 4.42       & 0.06       &$ 5661  ^{+ 38    }_{ -108  }$&$ 4.44  ^{+ 0.04  }_{ -0.05 }$&$ -0.02 ^{+ 0.19  }_{ -0.30 }$&$ 0.96  ^{+ 0.06  }_{ -0.24 }$&$ 1.00  ^{+ 0.07  }_{ -0.08 }$&$ 0.87  ^{+ 0.14  }_{ -0.39 }$&$ 1.33  \pm{ 0.36 }$ \\
K00284.01  & 6021275    & 283.235809      & 41.343040       & 11.82 & 5925       & 4.40       & -0.05      &$ 5896  ^{+ 43    }_{ -156  }$&$ 4.39  ^{+ 0.05  }_{ -0.14 }$&$ -0.33 ^{+ 0.20  }_{ -1.00 }$&$ 0.99  ^{+ 0.11  }_{ -0.09 }$&$ 1.00  ^{+ 0.10  }_{ -0.12 }$&$ 0.95  ^{+ 0.20  }_{ -0.37 }$&$ 1.38  \pm{ 0.47 }$ \\
K00284.02  & 6021275    & 283.235809      & 41.343040       & 11.82 & 5925       & 4.40       & -0.05      &$ 5927  ^{+ 53    }_{ -53   }$&$ 4.38  ^{+ 0.05  }_{ -0.27 }$&$ -0.27 ^{+ 0.19  }_{ -0.37 }$&$ 0.96  ^{+ 0.09  }_{ -0.10 }$&$ 1.06  ^{+ 0.13  }_{ -0.09 }$&$ 1.09  ^{+ 0.20  }_{ -0.23 }$&$ 1.14  \pm{ 0.36 }$ \\
K00284.03  & 6021275    & 283.235809      & 41.343040       & 11.82 & 5925       & 4.40       & -0.05      &$ 5923  ^{+ 51    }_{ -55   }$&$ 4.38  ^{+ 0.05  }_{ -0.28 }$&$ -0.33 ^{+ 0.18  }_{ -0.82 }$&$ 0.95  ^{+ 0.08  }_{ -0.18 }$&$ 0.98  ^{+ 0.08  }_{ -0.19 }$&$ 1.19  ^{+ 0.27  }_{ -0.19 }$&$ 1.41  \pm{ 0.61 }$ \\
K00284.04  & 6021275    & 283.235809      & 41.343040       & 11.82 & 5925       & 4.40       & -0.05      &$ 5915  ^{+ 39    }_{ -60   }$&$ 4.43  ^{+ 0.04  }_{ -0.05 }$&$ -0.28 ^{+ 0.26  }_{ -0.33 }$&$ 1.01  ^{+ 0.14  }_{ -0.11 }$&$ 0.98  ^{+ 0.08  }_{ -0.09 }$&$ 0.97  ^{+ 0.16  }_{ -0.29 }$&$ 1.52  \pm{ 0.43 }$ \\
K00285.01  & 6196457    & 289.086060      & 41.562958       & 11.56 & 5883       & 4.14       & \nodata    &$ 5861  ^{+ 43    }_{ -64   }$&$ 3.85  ^{+ 0.03  }_{ -0.01 }$&$ -0.04 ^{+ 0.40  }_{ -0.22 }$&$ 1.19  ^{+ 0.10  }_{ -0.12 }$&$ 2.05  ^{+ 0.11  }_{ -0.18 }$&$ 4.46  ^{+ 0.54  }_{ -0.78 }$&$ 0.19  \pm{ 0.04 }$ \\
K00285.02  & 6196457    & 289.086060      & 41.562958       & 11.56 & 5883       & 4.14       & \nodata    &$ 5867  ^{+ 38    }_{ -58   }$&$ 3.89  ^{+ 0.05  }_{ -0.05 }$&$ -0.12 ^{+ 0.29  }_{ -0.52 }$&$ 1.20  ^{+ 0.08  }_{ -0.22 }$&$ 1.98  ^{+ 0.11  }_{ -0.54 }$&$ 4.48  ^{+ 0.68  }_{ -0.64 }$&$ 0.22  \pm{ 0.11 }$ \\
K00285.03  & 6196457    & 289.086060      & 41.562958       & 11.56 & 5883       & 4.14       & \nodata    &$ 5868  ^{+ 35    }_{ -72   }$&$ 3.88  ^{+ 0.02  }_{ -0.04 }$&$ -0.22 ^{+ 0.23  }_{ -0.37 }$&$ 1.17  ^{+ 0.09  }_{ -0.13 }$&$ 2.00  ^{+ 0.06  }_{ -0.37 }$&$ 4.54  ^{+ 0.40  }_{ -0.38 }$&$ 0.21  \pm{ 0.07 }$ \\
K00289.01  & 10386922   & 282.945648      & 47.574905       & 12.75 & 5812       & 4.46       & \nodata    &$ 5439  ^{+ 337   }_{ -761  }$&$ 3.66  ^{+ 0.10  }_{ -0.19 }$&$ -0.24 ^{+ 0.41  }_{ -0.53 }$&$ 1.23  ^{+ 0.22  }_{ -0.40 }$&$ 2.44  ^{+ 0.45  }_{ -0.72 }$&$ 4.60  ^{+ 2.54  }_{ -2.62 }$&$ 0.12  \pm{ 0.09 }$ \\
K00289.02  & 10386922   & 282.945648      & 47.574905       & 12.75 & 5812       & 4.46       & \nodata    &$ 5459  ^{+ 374   }_{ -512  }$&$ 3.72  ^{+ 0.14  }_{ -0.15 }$&$ -0.26 ^{+ 0.33  }_{ -0.76 }$&$ 1.21  ^{+ 0.22  }_{ -0.38 }$&$ 2.30  ^{+ 0.51  }_{ -0.86 }$&$ 3.99  ^{+ 2.46  }_{ -2.39 }$&$ 0.14  \pm{ 0.13 }$ \\
K00291.01  & 10933561   & 297.277985      & 48.320332       & 12.85 & 5600       & 4.19       & -0.16      &$ 5613  ^{+ 60    }_{ -47   }$&$ 3.96  ^{+ 0.04  }_{ -0.05 }$&$ -0.22 ^{+ 0.18  }_{ -0.27 }$&$ 0.97  ^{+ 0.06  }_{ -0.13 }$&$ 1.77  ^{+ 0.10  }_{ -0.09 }$&$ 2.71  ^{+ 0.32  }_{ -0.30 }$&$ 0.24  \pm{ 0.05 }$ \\
K00291.02  & 10933561   & 297.277985      & 48.320332       & 12.85 & 5600       & 4.19       & -0.16      &$ 5554  ^{+ 38    }_{ -91   }$&$ 3.90  ^{+ 0.02  }_{ -0.01 }$&$ -0.32 ^{+ 0.15  }_{ -0.19 }$&$ 0.95  ^{+ 0.05  }_{ -0.08 }$&$ 1.79  ^{+ 0.05  }_{ -0.07 }$&$ 2.71  ^{+ 0.16  }_{ -0.71 }$&$ 0.23  \pm{ 0.03 }$ \\
K00295.01  & 11547513   & 284.739044      & 49.598400       & 12.32 & 5936       & 4.41       & \nodata    &$ 5866  ^{+ 710   }_{ -399  }$&$ 3.58  ^{+ 0.13  }_{ -0.11 }$&$ 0.14  ^{+ 0.45  }_{ -0.41 }$&$ 1.56  ^{+ 0.36  }_{ -0.29 }$&$ 2.75  ^{+ 0.59  }_{ -0.91 }$&$ 5.67  ^{+ 3.48  }_{ -3.45 }$&$ 0.11  \pm{ 0.09 }$ \\
K00295.02  & 11547513   & 284.739044      & 49.598400       & 12.32 & 5936       & 4.41       & \nodata    &$ 5359  ^{+ 362   }_{ -708  }$&$ 3.62  ^{+ 0.14  }_{ -0.34 }$&$ -0.16 ^{+ 0.41  }_{ -0.43 }$&$ 1.31  ^{+ 0.29  }_{ -0.49 }$&$ 2.38  ^{+ 0.57  }_{ -0.62 }$&$ 4.12  ^{+ 3.25  }_{ -1.93 }$&$ 0.14  \pm{ 0.11 }$ \\
K00298.01  & 12785320   & 290.494263      & 52.055519       & 12.71 & 5445       & 4.48       & \nodata    &$ 5271  ^{+ 361   }_{ -444  }$&$ 3.70  ^{+ 0.76  }_{ -0.34 }$&$ -0.12 ^{+ 0.35  }_{ -0.46 }$&$ 0.88  ^{+ 0.22  }_{ -0.22 }$&$ 0.63  ^{+ 1.65  }_{ -0.00 }$&$ 0.21  ^{+ 3.28  }_{ -0.00 }$&$ 4.93  \pm{ 19.30}$ \\
K00298.02  & 12785320   & 290.494263      & 52.055519       & 12.71 & 5445       & 4.48       & \nodata    &$ 5205  ^{+ 344   }_{ -595  }$&$ 3.66  ^{+ 0.72  }_{ -0.37 }$&$ -0.45 ^{+ 0.40  }_{ -0.95 }$&$ 1.04  ^{+ 0.28  }_{ -0.31 }$&$ 2.36  ^{+ 0.76  }_{ -1.61 }$&$ 3.82  ^{+ 3.87  }_{ -3.54 }$&$ 0.11  \pm{ 0.17 }$ \\
K00301.01  & 3642289    & 290.495117      & 38.795479       & 12.73 & 6337       & 4.33       & 0.04       &$ 6275  ^{+ 78    }_{ -212  }$&$ 3.66  ^{+ 0.06  }_{ -0.08 }$&$ -0.30 ^{+ 0.35  }_{ -0.59 }$&$ 1.69  ^{+ 0.36  }_{ -0.17 }$&$ 3.03  ^{+ 0.30  }_{ -0.30 }$&$ 11.93 ^{+ 2.12  }_{ -7.80 }$&$ 0.09  \pm{ 0.03 }$ \\
K00301.02  & 3642289    & 290.495117      & 38.795479       & 12.73 & 6337       & 4.33       & 0.04       &$ 6307  ^{+ 84    }_{ -101  }$&$ 3.65  ^{+ 0.06  }_{ -0.09 }$&$ -0.21 ^{+ 0.50  }_{ -0.42 }$&$ 1.50  ^{+ 0.19  }_{ -0.22 }$&$ 3.00  ^{+ 0.24  }_{ -0.81 }$&$ 11.91 ^{+ 2.27  }_{ -6.43 }$&$ 0.08  \pm{ 0.04 }$ \\
K00304.01  & 6029239    & 287.089966      & 41.373878       & 12.55 & 6150       & 3.98       & -0.09      &$ 6097  ^{+ 58    }_{ -211  }$&$ 3.76  ^{+ 0.09  }_{ -0.38 }$&$ -0.62 ^{+ 0.38  }_{ -0.89 }$&$ 1.15  ^{+ 0.13  }_{ -0.21 }$&$ 2.27  ^{+ 0.36  }_{ -0.28 }$&$ 4.94  ^{+ 1.43  }_{ -3.17 }$&$ 0.14  \pm{ 0.06 }$ \\
K00304.02  & 6029239    & 287.089966      & 41.373878       & 12.55 & 6150       & 3.98       & -0.09      &$ 6126  ^{+ 66    }_{ -96   }$&$ 3.73  ^{+ 0.20  }_{ -0.35 }$&$ -0.45 ^{+ 0.26  }_{ -0.46 }$&$ 0.99  ^{+ 0.12  }_{ -0.18 }$&$ 1.06  ^{+ 0.91  }_{ -0.19 }$&$ 0.88  ^{+ 1.12  }_{ -0.00 }$&$ 1.17  \pm{ 1.82 }$ \\
K00307.01  & 6289257    & 293.180328      & 41.617760       & 12.80 & 6141       & 4.42       & -0.31      &$ 6111  ^{+ 51    }_{ -190  }$&$ 4.36  ^{+ 0.04  }_{ -0.23 }$&$ 0.05  ^{+ 0.21  }_{ -0.29 }$&$ 1.23  ^{+ 0.18  }_{ -0.09 }$&$ 1.19  ^{+ 0.08  }_{ -0.10 }$&$ 1.76  ^{+ 0.29  }_{ -0.30 }$&$ 1.04  \pm{ 0.26 }$ \\
K00307.02  & 6289257    & 293.180328      & 41.617760       & 12.80 & 6141       & 4.42       & -0.31      &$ 6128  ^{+ 48    }_{ -76   }$&$ 4.38  ^{+ 0.04  }_{ -0.07 }$&$ 0.02  ^{+ 0.23  }_{ -0.24 }$&$ 1.18  ^{+ 0.08  }_{ -0.09 }$&$ 1.14  ^{+ 0.08  }_{ -0.11 }$&$ 1.63  ^{+ 0.24  }_{ -0.33 }$&$ 1.12  \pm{ 0.30 }$ \\
K00312.01  & 7050989    & 296.467316      & 42.598785       & 12.46 & 6158       & 4.35       & \nodata    &$ 6153  ^{+ 51    }_{ -64   }$&$ 4.35  ^{+ 0.04  }_{ -0.30 }$&$ -0.10 ^{+ 0.22  }_{ -0.24 }$&$ 1.09  ^{+ 0.07  }_{ -0.22 }$&$ 1.14  ^{+ 0.09  }_{ -0.11 }$&$ 1.48  ^{+ 0.26  }_{ -0.63 }$&$ 1.05  \pm{ 0.31 }$ \\
K00312.02  & 7050989    & 296.467316      & 42.598785       & 12.46 & 6158       & 4.35       & \nodata    &$ 6173  ^{+ 80    }_{ -47   }$&$ 4.36  ^{+ 0.04  }_{ -0.30 }$&$ -0.22 ^{+ 0.20  }_{ -0.74 }$&$ 1.09  ^{+ 0.08  }_{ -0.23 }$&$ 1.13  ^{+ 0.08  }_{ -0.12 }$&$ 1.73  ^{+ 0.28  }_{ -0.29 }$&$ 1.05  \pm{ 0.32 }$ \\
K00313.01  & 7419318    & 282.135529      & 43.039101       & 12.99 & 5348       & 4.53       & 0.03       &$ 5327  ^{+ 41    }_{ -157  }$&$ 4.49  ^{+ 0.03  }_{ -0.07 }$&$ 0.09  ^{+ 0.20  }_{ -0.30 }$&$ 0.95  ^{+ 0.07  }_{ -0.04 }$&$ 0.89  ^{+ 0.04  }_{ -0.09 }$&$ 0.55  ^{+ 0.06  }_{ -0.27 }$&$ 1.93  \pm{ 0.45 }$ \\
K00313.02  & 7419318    & 282.135529      & 43.039101       & 12.99 & 5348       & 4.53       & 0.03       &$ 5344  ^{+ 44    }_{ -47   }$&$ 4.50  ^{+ 0.04  }_{ -0.03 }$&$ 0.17  ^{+ 0.21  }_{ -0.24 }$&$ 0.95  ^{+ 0.05  }_{ -0.05 }$&$ 0.88  ^{+ 0.04  }_{ -0.10 }$&$ 0.55  ^{+ 0.05  }_{ -0.22 }$&$ 1.96  \pm{ 0.48 }$ \\
K00314.01  & 7603200    & 290.381500      & 43.292988       & 12.93 & 3900       & 4.58       & \nodata    &$ 3000  ^{+ 432   }_{ 0     }$&$ 4.77  ^{+ 0.01  }_{ -0.33 }$&$ -0.11 ^{+ 0.31  }_{ -0.42 }$&$ 0.42  ^{+ 0.06  }_{ -0.02 }$&$ 0.43  ^{+ 0.03  }_{ -0.03 }$&$ 0.01  ^{+ 0.01  }_{ -0.00 }$&$ 7.28  \pm{ 1.73 }$ \\
K00314.02  & 7603200    & 290.381500      & 43.292988       & 12.93 & 3900       & 4.58       & \nodata    &$ 3000  ^{+ 295   }_{ 0     }$&$ 4.77  ^{+ 0.01  }_{ -0.09 }$&$ -0.24 ^{+ 0.30  }_{ -0.72 }$&$ 0.45  ^{+ 0.05  }_{ -0.05 }$&$ 0.44  ^{+ 0.02  }_{ -0.04 }$&$ 0.01  ^{+ 0.01  }_{ -0.00 }$&$ 7.36  \pm{ 1.75 }$ \\
K00314.03  & 7603200    & 290.381500      & 43.292988       & 12.93 & 3900       & 4.58       & \nodata    &$ 3000  ^{+ 302   }_{ 0     }$&$ 4.76  ^{+ 0.01  }_{ -0.07 }$&$ -0.22 ^{+ 0.29  }_{ -0.42 }$&$ 0.42  ^{+ 0.04  }_{ -0.02 }$&$ 0.45  ^{+ 0.02  }_{ -0.04 }$&$ 0.01  ^{+ 0.01  }_{ -0.00 }$&$ 6.60  \pm{ 1.43 }$ \\
K00316.01  & 8008067    & 282.391937      & 43.889351       & 12.70 & 5622       & 4.33       & 0.15       &$ 5605  ^{+ 47    }_{ -64   }$&$ 3.76  ^{+ 0.07  }_{ -0.09 }$&$ -0.16 ^{+ 0.39  }_{ -0.42 }$&$ 1.31  ^{+ 0.18  }_{ -0.15 }$&$ 2.39  ^{+ 0.28  }_{ -0.29 }$&$ 4.58  ^{+ 0.89  }_{ -2.65 }$&$ 0.13  \pm{ 0.05 }$ \\
K00316.02  & 8008067    & 282.391937      & 43.889351       & 12.70 & 5622       & 4.33       & 0.15       &$ 5614  ^{+ 52    }_{ -55   }$&$ 3.72  ^{+ 0.07  }_{ -0.11 }$&$ -0.18 ^{+ 0.41  }_{ -0.38 }$&$ 1.16  ^{+ 0.14  }_{ -0.28 }$&$ 2.32  ^{+ 0.26  }_{ -0.83 }$&$ 5.31  ^{+ 0.99  }_{ -1.65 }$&$ 0.13  \pm{ 0.09 }$ \\
K00316.03  & 8008067    & 282.391937      & 43.889351       & 12.70 & 5622       & 4.33       & 0.15       &$ 5615  ^{+ 51    }_{ -56   }$&$ 3.78  ^{+ 0.05  }_{ -0.12 }$&$ 0.20  ^{+ 0.39  }_{ -0.40 }$&$ 1.33  ^{+ 0.20  }_{ -0.15 }$&$ 2.25  ^{+ 0.22  }_{ -0.42 }$&$ 4.56  ^{+ 1.01  }_{ -1.61 }$&$ 0.16  \pm{ 0.07 }$ \\
K00321.01  & 8753657    & 291.848053      & 44.968220       & 12.52 & 5538       & 4.34       & -0.19      &$ 5532  ^{+ 40    }_{ -45   }$&$ 4.33  ^{+ 0.03  }_{ -0.29 }$&$ 0.14  ^{+ 0.17  }_{ -0.17 }$&$ 0.97  ^{+ 0.05  }_{ -0.05 }$&$ 1.11  ^{+ 0.32  }_{ -0.06 }$&$ 0.95  ^{+ 0.11  }_{ -0.21 }$&$ 1.01  \pm{ 0.52 }$ \\
K00321.02  & 8753657    & 291.848053      & 44.968220       & 12.52 & 5538       & 4.34       & -0.19      &$ 5555  ^{+ 65    }_{ -41   }$&$ 4.43  ^{+ 0.04  }_{ -0.05 }$&$ -0.08 ^{+ 0.21  }_{ -0.24 }$&$ 0.90  ^{+ 0.06  }_{ -0.07 }$&$ 0.95  ^{+ 0.07  }_{ -0.10 }$&$ 0.74  ^{+ 0.11  }_{ -0.23 }$&$ 1.47  \pm{ 0.41 }$ \\
K00326.01  & 9880467    & 286.656036      & 46.783543       & 12.96 & 4746       & 2.54       & \nodata    &$ 4738  ^{+ 50    }_{ -51   }$&$ 2.62  ^{+ 0.04  }_{ -0.32 }$&$ -0.06 ^{+ 0.15  }_{ -0.23 }$&$ 2.01  ^{+ 0.14  }_{ -0.15 }$&$ 10.98 ^{+ 0.59  }_{ -1.12 }$&$ 55.09 ^{+ 7.23  }_{ -8.88 }$&$ 0.00  \pm{ 0.00 }$ \\
K00326.02  & 9880467    & 286.656036      & 46.783543       & 12.96 & 4746       & 2.54       & \nodata    &$ 4760  ^{+ 54    }_{ -47   }$&$ 2.58  ^{+ 0.10  }_{ -0.18 }$&$ -0.09 ^{+ 0.18  }_{ -0.18 }$&$ 1.96  ^{+ 0.12  }_{ -0.19 }$&$ 10.57 ^{+ 1.30  }_{ -1.53 }$&$ 48.64 ^{+ 13.51 }_{ -12.67 }$&$ 0.00  \pm{ 0.00 }$ \\
K00327.01  & 9881662    & 287.369476      & 46.768219       & 13.00 & 6206       & 4.39       & -0.09      &$ 6166  ^{+ 51    }_{ -133  }$&$ 4.36  ^{+ 0.03  }_{ -0.05 }$&$ 0.08  ^{+ 0.18  }_{ -0.25 }$&$ 1.24  ^{+ 0.06  }_{ -0.06 }$&$ 1.19  ^{+ 0.06  }_{ -0.09 }$&$ 1.88  ^{+ 0.25  }_{ -0.23 }$&$ 1.05  \pm{ 0.20 }$ \\
K00327.02  & 9881662    & 287.369476      & 46.768219       & 13.00 & 6206       & 4.39       & -0.09      &$ 6192  ^{+ 50    }_{ -77   }$&$ 4.38  ^{+ 0.03  }_{ -0.05 }$&$ 0.18  ^{+ 0.27  }_{ -0.21 }$&$ 1.17  ^{+ 0.06  }_{ -0.29 }$&$ 1.14  ^{+ 0.07  }_{ -0.29 }$&$ 1.67  ^{+ 0.19  }_{ -0.76 }$&$ 1.10  \pm{ 0.55 }$ \\
K00332.01  & 10290666   & 297.650940      & 47.396290       & 13.05 & 5719       & 4.33       & -0.28      &$ 5696  ^{+ 50    }_{ -169  }$&$ 4.46  ^{+ 0.07  }_{ -0.08 }$&$ 0.06  ^{+ 0.32  }_{ -0.33 }$&$ 1.04  ^{+ 0.17  }_{ -0.10 }$&$ 0.93  ^{+ 0.11  }_{ -0.21 }$&$ 0.82  ^{+ 0.22  }_{ -0.38 }$&$ 1.84  \pm{ 0.99 }$ \\
K00332.02  & 10290666   & 297.650940      & 47.396290       & 13.05 & 5719       & 4.33       & -0.28      &$ 5710  ^{+ 52    }_{ -64   }$&$ 4.44  ^{+ 0.06  }_{ -0.08 }$&$ -0.28 ^{+ 0.30  }_{ -0.37 }$&$ 0.91  ^{+ 0.10  }_{ -0.11 }$&$ 0.94  ^{+ 0.09  }_{ -0.11 }$&$ 0.87  ^{+ 0.20  }_{ -0.19 }$&$ 1.55  \pm{ 0.52 }$ \\
K00338.01  & 10552611   & 297.970886      & 47.731682       & 13.45 & 4104       & 1.87       & 0.54       &$ 5710  ^{+ 52    }_{ -64   }$&$ 4.44  ^{+ 0.06  }_{ -0.08 }$&$ -0.28 ^{+ 0.30  }_{ -0.37 }$&$ 0.91  ^{+ 0.10  }_{ -0.11 }$&$ 0.94  ^{+ 0.09  }_{ -0.11 }$&$ 0.87  ^{+ 0.20  }_{ -0.19 }$&$ 1.55  \pm{ 0.52 }$ \\
K00338.02  & 10552611   & 297.970886      & 47.731682       & 13.45 & 4104       & 1.87       & 0.54       &$ 5710  ^{+ 52    }_{ -64   }$&$ 4.44  ^{+ 0.06  }_{ -0.08 }$&$ -0.28 ^{+ 0.30  }_{ -0.37 }$&$ 0.91  ^{+ 0.10  }_{ -0.11 }$&$ 0.94  ^{+ 0.09  }_{ -0.11 }$&$ 0.87  ^{+ 0.20  }_{ -0.19 }$&$ 1.55  \pm{ 0.52 }$ \\
K00341.01  & 10878263   & 297.961548      & 48.244362       & 13.34 & 5536       & 4.48       & 0.01       &$ 5525  ^{+ 41    }_{ -60   }$&$ 4.45  ^{+ 0.03  }_{ -0.05 }$&$ -0.02 ^{+ 0.22  }_{ -0.68 }$&$ 0.99  ^{+ 0.06  }_{ -0.07 }$&$ 0.97  ^{+ 0.06  }_{ -0.06 }$&$ 0.77  ^{+ 0.09  }_{ -0.14 }$&$ 1.53  \pm{ 0.31 }$ \\
K00341.02  & 10878263   & 297.961548      & 48.244362       & 13.34 & 5536       & 4.48       & 0.01       &$ 5531  ^{+ 44    }_{ -55   }$&$ 4.45  ^{+ 0.04  }_{ -0.05 }$&$ 0.03  ^{+ 0.22  }_{ -0.29 }$&$ 1.01  ^{+ 0.15  }_{ -0.06 }$&$ 0.93  ^{+ 0.06  }_{ -0.23 }$&$ 0.75  ^{+ 0.11  }_{ -0.14 }$&$ 1.77  \pm{ 0.85 }$ \\
K00343.01  & 10982872   & 295.118896      & 48.481281       & 13.20 & 5744       & 4.32       & -0.27      &$ 5708  ^{+ 42    }_{ -123  }$&$ 4.32  ^{+ 0.07  }_{ -0.26 }$&$ -0.18 ^{+ 0.14  }_{ -0.84 }$&$ 0.94  ^{+ 0.07  }_{ -0.22 }$&$ 1.09  ^{+ 0.27  }_{ -0.12 }$&$ 1.06  ^{+ 0.27  }_{ -0.40 }$&$ 1.02  \pm{ 0.57 }$ \\
K00343.02  & 10982872   & 295.118896      & 48.481281       & 13.20 & 5744       & 4.32       & -0.27      &$ 5731  ^{+ 36    }_{ -69   }$&$ 4.02  ^{+ 0.07  }_{ -0.00 }$&$ -0.05 ^{+ 0.25  }_{ -0.20 }$&$ 0.95  ^{+ 0.07  }_{ -0.22 }$&$ 1.04  ^{+ 0.23  }_{ -0.26 }$&$ 0.97  ^{+ 0.36  }_{ -0.42 }$&$ 1.20  \pm{ 0.87 }$ \\
K00343.03  & 10982872   & 295.118896      & 48.481281       & 13.20 & 5744       & 4.32       & -0.27      &$ 5736  ^{+ 44    }_{ -56   }$&$ 4.41  ^{+ 0.04  }_{ -0.10 }$&$ -0.30 ^{+ 0.16  }_{ -0.30 }$&$ 0.91  ^{+ 0.08  }_{ -0.07 }$&$ 0.98  ^{+ 0.08  }_{ -0.09 }$&$ 0.88  ^{+ 0.13  }_{ -0.23 }$&$ 1.39  \pm{ 0.38 }$ \\
K00353.01  & 11566064   & 295.212677      & 49.562180       & 13.37 & 6858       & 4.33       & -0.09      &$ 6856  ^{+ 99    }_{ -117  }$&$ 4.27  ^{+ 0.04  }_{ -0.05 }$&$ 0.05  ^{+ 0.21  }_{ -0.24 }$&$ 1.43  ^{+ 0.10  }_{ -0.12 }$&$ 1.39  ^{+ 0.11  }_{ -0.38 }$&$ 3.89  ^{+ 0.72  }_{ -1.25 }$&$ 0.75  \pm{ 0.40 }$ \\
K00353.02  & 11566064   & 295.212677      & 49.562180       & 13.37 & 6858       & 4.33       & -0.09      &$ 6841  ^{+ 95    }_{ -157  }$&$ 4.28  ^{+ 0.06  }_{ -0.05 }$&$ 0.08  ^{+ 0.24  }_{ -0.31 }$&$ 1.40  ^{+ 0.10  }_{ -0.34 }$&$ 1.37  ^{+ 0.13  }_{ -0.39 }$&$ 3.70  ^{+ 0.81  }_{ -1.92 }$&$ 0.77  \pm{ 0.45 }$ \\
K00354.01  & 11568987   & 296.418549      & 49.540100       & 13.23 & 5935       & 4.44       & -0.84      &$ 5934  ^{+ 51    }_{ -69   }$&$ 4.52  ^{+ 0.04  }_{ -0.04 }$&$ -0.41 ^{+ 0.22  }_{ -0.23 }$&$ 0.88  ^{+ 0.05  }_{ -0.13 }$&$ 0.84  ^{+ 0.05  }_{ -0.14 }$&$ 0.79  ^{+ 0.12  }_{ -0.30 }$&$ 2.06  \pm{ 0.74 }$ \\
K00354.02  & 11568987   & 296.418549      & 49.540100       & 13.23 & 5935       & 4.44       & -0.84      &$ 5924  ^{+ 48    }_{ -90   }$&$ 4.55  ^{+ 0.03  }_{ -0.05 }$&$ -0.67 ^{+ 0.23  }_{ -0.36 }$&$ 0.89  ^{+ 0.06  }_{ -0.05 }$&$ 0.82  ^{+ 0.06  }_{ -0.07 }$&$ 0.70  ^{+ 0.11  }_{ -0.25 }$&$ 2.26  \pm{ 0.52 }$ \\
K00369.01  & 7175184    & 281.915680      & 42.775509       & 11.99 & 6377       & 4.41       & -0.33      &$ 6371  ^{+ 47    }_{ -75   }$&$ 4.35  ^{+ 0.07  }_{ -0.21 }$&$ -0.49 ^{+ 0.31  }_{ -0.79 }$&$ 1.06  ^{+ 0.13  }_{ -0.17 }$&$ 1.00  ^{+ 0.14  }_{ -0.19 }$&$ 1.48  ^{+ 0.46  }_{ -0.58 }$&$ 1.51  \pm{ 0.79 }$ \\
K00369.02  & 7175184    & 281.915680      & 42.775509       & 11.99 & 6377       & 4.41       & -0.33      &$ 6370  ^{+ 50    }_{ -73   }$&$ 4.35  ^{+ 0.07  }_{ -0.17 }$&$ -0.01 ^{+ 0.31  }_{ -0.32 }$&$ 1.24  ^{+ 0.12  }_{ -0.13 }$&$ 1.02  ^{+ 0.15  }_{ -0.21 }$&$ 1.59  ^{+ 0.48  }_{ -0.69 }$&$ 1.64  \pm{ 0.89 }$ \\
K00370.01  & 8494142    & 291.387756      & 44.529110       & 11.93 & 6022       & 3.95       & -0.67      &$ 5995  ^{+ 46    }_{ -132  }$&$ 3.71  ^{+ 0.03  }_{ -0.05 }$&$ -0.83 ^{+ 0.24  }_{ -0.48 }$&$ 1.14  ^{+ 0.08  }_{ -0.15 }$&$ 2.46  ^{+ 0.10  }_{ -0.23 }$&$ 6.91  ^{+ 0.65  }_{ -2.57 }$&$ 0.11  \pm{ 0.02 }$ \\
K00370.02  & 8494142    & 291.387756      & 44.529110       & 11.93 & 6022       & 3.95       & -0.67      &$ 6014  ^{+ 44    }_{ -53   }$&$ 3.72  ^{+ 0.04  }_{ -0.03 }$&$ -0.79 ^{+ 0.22  }_{ -0.49 }$&$ 1.17  ^{+ 0.09  }_{ -0.09 }$&$ 2.49  ^{+ 0.11  }_{ -0.17 }$&$ 7.21  ^{+ 0.68  }_{ -0.94 }$&$ 0.11  \pm{ 0.02 }$ \\
K00623.01  & 12068975   & 295.226440      & 50.558979       & 11.81 & 5877       & 4.23       & -0.53      &$ 5852  ^{+ 44    }_{ -82   }$&$ 4.04  ^{+ 0.10  }_{ -0.05 }$&$ -0.60 ^{+ 0.24  }_{ -0.22 }$&$ 0.86  ^{+ 0.04  }_{ -0.08 }$&$ 1.48  ^{+ 0.06  }_{ -0.18 }$&$ 2.43  ^{+ 0.22  }_{ -0.65 }$&$ 0.38  \pm{ 0.10 }$ \\
K00623.02  & 12068975   & 295.226440      & 50.558979       & 11.81 & 5877       & 4.23       & -0.53      &$ 5870  ^{+ 32    }_{ -146  }$&$ 4.01  ^{+ 0.03  }_{ -0.06 }$&$ -0.80 ^{+ 0.17  }_{ -0.55 }$&$ 0.84  ^{+ 0.04  }_{ -0.07 }$&$ 1.49  ^{+ 0.06  }_{ -0.26 }$&$ 2.46  ^{+ 0.19  }_{ -0.27 }$&$ 0.36  \pm{ 0.12 }$ \\
K00623.03  & 12068975   & 295.226440      & 50.558979       & 11.81 & 5877       & 4.23       & -0.53      &$ 5868  ^{+ 37    }_{ -70   }$&$ 3.97  ^{+ 0.02  }_{ -0.04 }$&$ -0.66 ^{+ 0.23  }_{ -0.20 }$&$ 0.84  ^{+ 0.04  }_{ -0.05 }$&$ 1.61  ^{+ 0.07  }_{ -0.09 }$&$ 2.74  ^{+ 0.22  }_{ -0.29 }$&$ 0.28  \pm{ 0.04 }$ \\
K00623.04  & 12068975   & 295.226440      & 50.558979       & 11.81 & 5877       & 4.23       & -0.53      &$ 5878  ^{+ 42    }_{ -46   }$&$ 4.03  ^{+ 0.31  }_{ -0.10 }$&$ -0.71 ^{+ 0.17  }_{ -0.25 }$&$ 0.80  ^{+ 0.05  }_{ -0.10 }$&$ 0.96  ^{+ 0.42  }_{ -0.20 }$&$ 0.86  ^{+ 0.27  }_{ -0.27 }$&$ 1.29  \pm{ 1.27 }$ \\
K00626.01  & 4478168    & 295.193390      & 39.539669       & 13.49 & 6157       & 4.41       & -0.28      &$ 6157  ^{+ 51    }_{ -57   }$&$ 4.43  ^{+ 0.06  }_{ -0.06 }$&$ -0.27 ^{+ 0.22  }_{ -0.30 }$&$ 1.09  ^{+ 0.11  }_{ -0.10 }$&$ 1.10  ^{+ 0.15  }_{ -0.12 }$&$ 1.34  ^{+ 0.30  }_{ -0.31 }$&$ 1.14  \pm{ 0.44 }$ \\
K00626.02  & 4478168    & 295.193390      & 39.539669       & 13.49 & 6157       & 4.41       & -0.28      &$ 6118  ^{+ 45    }_{ -117  }$&$ 4.46  ^{+ 0.10  }_{ -0.06 }$&$ -0.27 ^{+ 0.28  }_{ -0.25 }$&$ 0.96  ^{+ 0.09  }_{ -0.13 }$&$ 0.96  ^{+ 0.11  }_{ -0.18 }$&$ 1.20  ^{+ 0.31  }_{ -0.47 }$&$ 1.53  \pm{ 0.71 }$ \\
K00627.01  & 4563268    & 292.150452      & 39.637581       & 13.31 & 6125       & 4.37       & 0.09       &$ 6122  ^{+ 53    }_{ -70   }$&$ 4.34  ^{+ 0.03  }_{ -0.27 }$&$ 0.16  ^{+ 0.19  }_{ -0.27 }$&$ 1.22  ^{+ 0.05  }_{ -0.10 }$&$ 1.19  ^{+ 0.07  }_{ -0.10 }$&$ 1.74  ^{+ 0.21  }_{ -0.36 }$&$ 1.03  \pm{ 0.24 }$ \\
K00627.02  & 4563268    & 292.150452      & 39.637581       & 13.31 & 6125       & 4.37       & 0.09       &$ 6112  ^{+ 54    }_{ -66   }$&$ 4.38  ^{+ 0.03  }_{ -0.04 }$&$ 0.07  ^{+ 0.22  }_{ -0.28 }$&$ 1.23  ^{+ 0.08  }_{ -0.07 }$&$ 1.15  ^{+ 0.07  }_{ -0.16 }$&$ 1.70  ^{+ 0.21  }_{ -0.26 }$&$ 1.15  \pm{ 0.34 }$ \\
K00655.01  & 5966154    & 293.626038      & 41.272820       & 13.00 & 6133       & 4.32       & -0.28      &$ 6136  ^{+ 54    }_{ -59   }$&$ 4.34  ^{+ 0.04  }_{ -0.31 }$&$ -0.22 ^{+ 0.16  }_{ -0.27 }$&$ 1.04  ^{+ 0.06  }_{ -0.18 }$&$ 1.10  ^{+ 0.07  }_{ -0.21 }$&$ 1.58  ^{+ 0.22  }_{ -0.24 }$&$ 1.12  \pm{ 0.44 }$ \\
K00655.02  & 5966154    & 293.626038      & 41.272820       & 13.00 & 6133       & 4.32       & -0.28      &$ 6112  ^{+ 44    }_{ -156  }$&$ 4.36  ^{+ 0.04  }_{ -0.06 }$&$ -0.19 ^{+ 0.18  }_{ -0.71 }$&$ 1.09  ^{+ 0.08  }_{ -0.15 }$&$ 1.13  ^{+ 0.08  }_{ -0.26 }$&$ 1.64  ^{+ 0.24  }_{ -0.43 }$&$ 1.07  \pm{ 0.50 }$ \\
K00664.01  & 6442340    & 291.634674      & 41.833858       & 13.48 & 5986       & 4.24       & -0.15      &$ 5999  ^{+ 116   }_{ -77   }$&$ 3.83  ^{+ 0.08  }_{ -0.08 }$&$ -0.64 ^{+ 0.28  }_{ -0.55 }$&$ 1.06  ^{+ 0.11  }_{ -0.14 }$&$ 2.17  ^{+ 0.29  }_{ -0.26 }$&$ 4.99  ^{+ 1.08  }_{ -1.59 }$&$ 0.14  \pm{ 0.06 }$ \\
K00664.02  & 6442340    & 291.634674      & 41.833858       & 13.48 & 5986       & 4.24       & -0.15      &$ 5980  ^{+ 76    }_{ -90   }$&$ 3.76  ^{+ 0.08  }_{ -0.10 }$&$ -0.81 ^{+ 0.35  }_{ -0.76 }$&$ 1.04  ^{+ 0.10  }_{ -0.18 }$&$ 2.25  ^{+ 0.24  }_{ -0.38 }$&$ 5.81  ^{+ 1.34  }_{ -1.84 }$&$ 0.13  \pm{ 0.06 }$ \\
K00664.03  & 6442340    & 291.634674      & 41.833858       & 13.48 & 5986       & 4.24       & -0.15      &$ 5992  ^{+ 101   }_{ -85   }$&$ 3.86  ^{+ 0.50  }_{ -0.13 }$&$ -0.40 ^{+ 0.43  }_{ -0.29 }$&$ 1.02  ^{+ 0.14  }_{ -0.13 }$&$ 0.94  ^{+ 0.94  }_{ -0.17 }$&$ 0.61  ^{+ 2.67  }_{ -0.00 }$&$ 1.75  \pm{ 3.09 }$ \\
K00665.01  & 6685609    & 290.030518      & 42.166050       & 13.18 & 6080       & 4.37       & -0.02      &$ 6093  ^{+ 70    }_{ -89   }$&$ 3.61  ^{+ 0.11  }_{ -0.14 }$&$ -0.20 ^{+ 0.45  }_{ -0.47 }$&$ 1.62  ^{+ 0.33  }_{ -0.20 }$&$ 2.52  ^{+ 0.43  }_{ -0.77 }$&$ 7.46  ^{+ 2.91  }_{ -3.71 }$&$ 0.14  \pm{ 0.10 }$ \\
K00665.02  & 6685609    & 290.030518      & 42.166050       & 13.18 & 6080       & 4.37       & -0.02      &$ 6072  ^{+ 86    }_{ -90   }$&$ 3.74  ^{+ 0.07  }_{ -0.07 }$&$ -0.55 ^{+ 0.36  }_{ -0.84 }$&$ 1.14  ^{+ 0.17  }_{ -0.15 }$&$ 2.66  ^{+ 0.30  }_{ -0.28 }$&$ 7.00  ^{+ 1.48  }_{ -3.94 }$&$ 0.09  \pm{ 0.03 }$ \\
K00665.03  & 6685609    & 290.030518      & 42.166050       & 13.18 & 6080       & 4.37       & -0.02      &$ 6061  ^{+ 68    }_{ -92   }$&$ 3.73  ^{+ 0.11  }_{ -0.12 }$&$ -0.31 ^{+ 0.49  }_{ -0.51 }$&$ 1.25  ^{+ 0.20  }_{ -0.33 }$&$ 2.45  ^{+ 0.36  }_{ -0.80 }$&$ 6.31  ^{+ 2.27  }_{ -2.99 }$&$ 0.12  \pm{ 0.09 }$ \\
K00678.01  & 7509886    & 285.439148      & 43.168480       & 13.28 & 5174       & 3.91       & 0.11       &$ 5139  ^{+ 56    }_{ -89   }$&$ 3.76  ^{+ 0.11  }_{ -0.24 }$&$ -0.50 ^{+ 0.17  }_{ -0.78 }$&$ 0.89  ^{+ 0.05  }_{ -0.06 }$&$ 1.90  ^{+ 0.20  }_{ -0.33 }$&$ 2.04  ^{+ 0.45  }_{ -0.54 }$&$ 0.18  \pm{ 0.08 }$ \\
K00678.02  & 7509886    & 285.439148      & 43.168480       & 13.28 & 5174       & 3.91       & 0.11       &$ 5123  ^{+ 66    }_{ -106  }$&$ 3.77  ^{+ 0.16  }_{ -0.17 }$&$ -0.38 ^{+ 0.43  }_{ -0.23 }$&$ 0.86  ^{+ 0.03  }_{ -0.03 }$&$ 1.96  ^{+ 0.29  }_{ -0.30 }$&$ 2.14  ^{+ 0.66  }_{ -0.41 }$&$ 0.16  \pm{ 0.07 }$ \\
K00679.01  & 7515212    & 287.620819      & 43.141647       & 13.18 & 5913       & 4.37       & \nodata    &$ 5900  ^{+ 42    }_{ -132  }$&$ 3.41  ^{+ 0.06  }_{ -0.23 }$&$ -0.13 ^{+ 0.45  }_{ -0.38 }$&$ 1.87  ^{+ 0.23  }_{ -0.21 }$&$ 4.18  ^{+ 0.50  }_{ -0.65 }$&$ 19.05 ^{+ 4.48  }_{ -5.90 }$&$ 0.04  \pm{ 0.02 }$ \\
K00679.02  & 7515212    & 287.620819      & 43.141647       & 13.18 & 5913       & 4.37       & \nodata    &$ 5900  ^{+ 41    }_{ -55   }$&$ 3.43  ^{+ 0.08  }_{ -0.56 }$&$ -0.20 ^{+ 0.41  }_{ -0.58 }$&$ 1.57  ^{+ 0.24  }_{ -0.49 }$&$ 3.72  ^{+ 0.56  }_{ -0.79 }$&$ 14.35 ^{+ 4.18  }_{ -6.64 }$&$ 0.04  \pm{ 0.03 }$ \\
K00710.01  & 9590976    & 293.037750      & 46.277519       & 13.29 & 6653       & 4.31       & \nodata    &$ 6428  ^{+ 467   }_{ -555  }$&$ 3.45  ^{+ 0.17  }_{ -0.34 }$&$ -0.27 ^{+ 0.42  }_{ -0.57 }$&$ 1.88  ^{+ 0.37  }_{ -0.47 }$&$ 3.82  ^{+ 1.23  }_{ -2.09 }$&$ 25.52 ^{+ 22.61 }_{ -16.62 }$&$ 0.05  \pm{ 0.06 }$ \\
K00710.02  & 9590976    & 293.037750      & 46.277519       & 13.29 & 6653       & 4.31       & \nodata    &$ 6261  ^{+ 411   }_{ -728  }$&$ 3.38  ^{+ 0.18  }_{ -0.24 }$&$ -0.08 ^{+ 0.37  }_{ -0.54 }$&$ 2.01  ^{+ 0.39  }_{ -0.41 }$&$ 3.87  ^{+ 1.29  }_{ -2.11 }$&$ 18.00 ^{+ 16.56 }_{ -15.15 }$&$ 0.05  \pm{ 0.07 }$ \\
K00710.03  & 9590976    & 293.037750      & 46.277519       & 13.29 & 6653       & 4.31       & \nodata    &$ 6553  ^{+ 427   }_{ -549  }$&$ 3.20  ^{+ 0.21  }_{ -0.32 }$&$ -0.09 ^{+ 0.42  }_{ -0.37 }$&$ 1.87  ^{+ 0.37  }_{ -0.62 }$&$ 5.92  ^{+ 4.22  }_{ -1.85 }$&$ 11.20 ^{+ 17.61 }_{ -8.65 }$&$ 0.01  \pm{ 0.02 }$ \\
K00717.01  & 9873254    & 282.212921      & 46.717819       & 13.39 & 5686       & 4.41       & -0.35      &$ 5672  ^{+ 52    }_{ -50   }$&$ 3.51  ^{+ 0.09  }_{ -0.12 }$&$ -0.78 ^{+ 0.38  }_{ -0.80 }$&$ 1.51  ^{+ 0.24  }_{ -0.22 }$&$ 3.52  ^{+ 0.46  }_{ -0.50 }$&$ 7.68  ^{+ 2.93  }_{ -3.57 }$&$ 0.05  \pm{ 0.02 }$ \\
K00717.02  & 9873254    & 282.212921      & 46.717819       & 13.39 & 5686       & 4.41       & -0.35      &$ 5658  ^{+ 40    }_{ -145  }$&$ 4.48  ^{+ 0.17  }_{ -0.83 }$&$ -0.20 ^{+ 0.38  }_{ -0.41 }$&$ 0.92  ^{+ 0.18  }_{ -0.18 }$&$ 0.69  ^{+ 0.29  }_{ -0.00 }$&$ 0.43  ^{+ 0.48  }_{ -0.00 }$&$ 3.95  \pm{ 2.62 }$ \\
K00719.01  & 9950612    & 291.506165      & 46.895741       & 13.18 & 4689       & 4.66       & \nodata    &$ 4682  ^{+ 46    }_{ -60   }$&$ 4.63  ^{+ 0.03  }_{ -0.03 }$&$ 0.13  ^{+ 0.29  }_{ -0.26 }$&$ 0.77  ^{+ 0.06  }_{ -0.05 }$&$ 0.69  ^{+ 0.03  }_{ -0.05 }$&$ 0.20  ^{+ 0.03  }_{ -0.03 }$&$ 3.27  \pm{ 0.62 }$ \\
K00719.02  & 9950612    & 291.506165      & 46.895741       & 13.18 & 4689       & 4.66       & \nodata    &$ 4675  ^{+ 47    }_{ -62   }$&$ 4.63  ^{+ 0.03  }_{ -0.09 }$&$ -0.04 ^{+ 0.23  }_{ -1.08 }$&$ 0.78  ^{+ 0.06  }_{ -0.04 }$&$ 0.70  ^{+ 0.04  }_{ -0.04 }$&$ 0.18  ^{+ 0.03  }_{ -0.08 }$&$ 3.23  \pm{ 0.62 }$ \\
K00719.03  & 9950612    & 291.506165      & 46.895741       & 13.18 & 4689       & 4.66       & \nodata    &$ 4668  ^{+ 47    }_{ -85   }$&$ 4.64  ^{+ 0.03  }_{ -0.04 }$&$ 0.08  ^{+ 0.30  }_{ -0.25 }$&$ 0.72  ^{+ 0.05  }_{ -0.07 }$&$ 0.64  ^{+ 0.04  }_{ -0.11 }$&$ 0.18  ^{+ 0.02  }_{ -0.04 }$&$ 3.90  \pm{ 1.43 }$ \\
K00719.04  & 9950612    & 291.506165      & 46.895741       & 13.18 & 4689       & 4.66       & \nodata    &$ 4666  ^{+ 50    }_{ -127  }$&$ 4.61  ^{+ 0.03  }_{ -0.08 }$&$ 0.20  ^{+ 0.31  }_{ -0.29 }$&$ 0.76  ^{+ 0.04  }_{ -0.05 }$&$ 0.71  ^{+ 0.04  }_{ -0.05 }$&$ 0.21  ^{+ 0.03  }_{ -0.03 }$&$ 3.02  \pm{ 0.59 }$ \\
K00972.01  & 11013201   & 282.000305      & 48.542221       & 9.28  & 8002       & 3.82       & -0.06      &$ 7935  ^{+ 154   }_{ -153  }$&$ 4.07  ^{+ 0.04  }_{ -0.08 }$&$ 0.08  ^{+ 0.24  }_{ -0.17 }$&$ 1.89  ^{+ 0.21  }_{ -0.14 }$&$ 2.08  ^{+ 0.09  }_{ -0.25 }$&$ 11.52 ^{+ 2.75  }_{ -4.31 }$&$ 0.30  \pm{ 0.08 }$ \\
K00972.02  & 11013201   & 282.000305      & 48.542221       & 9.28  & 8002       & 3.82       & -0.06      &$ 7924  ^{+ 129   }_{ -368  }$&$ 4.33  ^{+ 0.02  }_{ -0.07 }$&$ -0.52 ^{+ 0.13  }_{ -0.13 }$&$ 1.38  ^{+ 0.05  }_{ -0.15 }$&$ 1.32  ^{+ 0.05  }_{ -0.08 }$&$ 6.44  ^{+ 0.79  }_{ -0.97 }$&$ 0.84  \pm{ 0.13 }$ \\
K01001.01  & 1871056    & 292.044617      & 37.376240       & 13.04 & 6235       & 3.80       & -0.19      &$ 6231  ^{+ 124   }_{ -116  }$&$ 3.49  ^{+ 0.09  }_{ -0.30 }$&$ -0.66 ^{+ 0.37  }_{ -0.56 }$&$ 1.37  ^{+ 0.18  }_{ -0.30 }$&$ 2.84  ^{+ 0.50  }_{ -0.57 }$&$ 9.62  ^{+ 3.91  }_{ -3.36 }$&$ 0.08  \pm{ 0.05 }$ \\
K01001.02  & 1871056    & 292.044617      & 37.376240       & 13.04 & 6235       & 3.80       & -0.19      &$ 6198  ^{+ 109   }_{ -122  }$&$ 3.69  ^{+ 0.13  }_{ -0.12 }$&$ -0.43 ^{+ 0.49  }_{ -0.42 }$&$ 1.35  ^{+ 0.19  }_{ -0.28 }$&$ 2.67  ^{+ 0.35  }_{ -0.54 }$&$ 10.21 ^{+ 3.39  }_{ -4.45 }$&$ 0.10  \pm{ 0.05 }$ \\
K01151.01  & 8280511    & 283.002960      & 44.284229       & 13.40 & 5759       & 4.43       & -0.95      &$ 5767  ^{+ 85    }_{ -72   }$&$ 3.64  ^{+ 0.06  }_{ -0.05 }$&$ -1.13 ^{+ 0.26  }_{ -0.41 }$&$ 0.95  ^{+ 0.08  }_{ -0.15 }$&$ 2.49  ^{+ 0.18  }_{ -0.27 }$&$ 6.02  ^{+ 0.93  }_{ -1.41 }$&$ 0.09  \pm{ 0.03 }$ \\
K01151.02  & 8280511    & 283.002960      & 44.284229       & 13.40 & 5759       & 4.43       & -0.95      &$ 5757  ^{+ 65    }_{ -67   }$&$ 3.63  ^{+ 0.05  }_{ -0.05 }$&$ -1.19 ^{+ 0.23  }_{ -0.35 }$&$ 0.96  ^{+ 0.07  }_{ -0.14 }$&$ 2.47  ^{+ 0.17  }_{ -0.53 }$&$ 5.88  ^{+ 0.76  }_{ -2.58 }$&$ 0.09  \pm{ 0.04 }$ \\
K01151.03  & 8280511    & 283.002960      & 44.284229       & 13.40 & 5759       & 4.43       & -0.95      &$ 5741  ^{+ 68    }_{ -97   }$&$ 3.64  ^{+ 0.07  }_{ -0.11 }$&$ -1.04 ^{+ 0.31  }_{ -0.52 }$&$ 1.00  ^{+ 0.14  }_{ -0.17 }$&$ 2.29  ^{+ 0.28  }_{ -0.74 }$&$ 5.00  ^{+ 1.38  }_{ -2.80 }$&$ 0.12  \pm{ 0.08 }$ \\
K01151.04  & 8280511    & 283.002960      & 44.284229       & 13.40 & 5759       & 4.43       & -0.95      &$ 5743  ^{+ 64    }_{ -84   }$&$ 3.59  ^{+ 0.08  }_{ -0.05 }$&$ -1.10 ^{+ 0.31  }_{ -0.48 }$&$ 0.98  ^{+ 0.12  }_{ -0.18 }$&$ 2.74  ^{+ 0.35  }_{ -0.29 }$&$ 6.37  ^{+ 1.39  }_{ -1.87 }$&$ 0.07  \pm{ 0.03 }$ \\
K01151.05  & 8280511    & 283.002960      & 44.284229       & 13.40 & 5759       & 4.43       & -0.95      &$ 5775  ^{+ 73    }_{ -68   }$&$ 4.55  ^{+ 0.07  }_{ -0.11 }$&$ -0.74 ^{+ 0.35  }_{ -0.31 }$&$ 0.75  ^{+ 0.07  }_{ -0.08 }$&$ 0.76  ^{+ 0.08  }_{ -0.12 }$&$ 0.58  ^{+ 0.15  }_{ -0.21 }$&$ 2.38  \pm{ 1.00 }$ \\
K01175.01  & 10350571   & 295.920654      & 47.448608       & 13.29 & 5610       & 4.03       & -0.50      &$ 5619  ^{+ 58    }_{ -47   }$&$ 3.81  ^{+ 0.04  }_{ -0.08 }$&$ -0.70 ^{+ 0.22  }_{ -0.75 }$&$ 0.95  ^{+ 0.07  }_{ -0.15 }$&$ 1.91  ^{+ 0.11  }_{ -0.48 }$&$ 3.30  ^{+ 0.39  }_{ -0.90 }$&$ 0.19  \pm{ 0.09 }$ \\
K01175.02  & 10350571   & 295.920654      & 47.448608       & 13.29 & 5610       & 4.03       & -0.50      &$ 5614  ^{+ 50    }_{ -48   }$&$ 3.80  ^{+ 0.05  }_{ -0.07 }$&$ -0.57 ^{+ 0.22  }_{ -0.26 }$&$ 0.93  ^{+ 0.06  }_{ -0.15 }$&$ 1.93  ^{+ 0.11  }_{ -0.46 }$&$ 3.34  ^{+ 0.43  }_{ -0.60 }$&$ 0.18  \pm{ 0.08 }$ \\
K01215.01  & 3939150    & 286.583160      & 39.077202       & 13.42 & 5946       & 4.08       & -0.32      &$ 5938  ^{+ 45    }_{ -57   }$&$ 3.58  ^{+ 0.09  }_{ -0.15 }$&$ -0.93 ^{+ 0.36  }_{ -0.39 }$&$ 1.09  ^{+ 0.07  }_{ -0.10 }$&$ 2.66  ^{+ 0.27  }_{ -0.35 }$&$ 7.69  ^{+ 1.79  }_{ -1.81 }$&$ 0.08  \pm{ 0.03 }$ \\
K01215.02  & 3939150    & 286.583160      & 39.077202       & 13.42 & 5946       & 4.08       & -0.32      &$ 5946  ^{+ 54    }_{ -51   }$&$ 3.67  ^{+ 0.13  }_{ -0.25 }$&$ -0.51 ^{+ 0.29  }_{ -0.49 }$&$ 1.13  ^{+ 0.16  }_{ -0.13 }$&$ 0.90  ^{+ 1.27  }_{ -0.17 }$&$ 0.56  ^{+ 0.90  }_{ -0.00 }$&$ 2.15  \pm{ 5.14 }$ \\
K01221.01  & 3640905    & 290.107178      & 38.702229       & 11.58 & 5128       & 3.94       & 0.42       &$ 5136  ^{+ 48    }_{ -43   }$&$ 3.89  ^{+ 0.03  }_{ -0.05 }$&$ 0.08  ^{+ 0.23  }_{ -0.30 }$&$ 1.10  ^{+ 0.07  }_{ -0.08 }$&$ 1.90  ^{+ 0.09  }_{ -0.25 }$&$ 2.23  ^{+ 0.23  }_{ -0.64 }$&$ 0.23  \pm{ 0.06 }$ \\
K01221.02  & 3640905    & 290.107178      & 38.702229       & 11.58 & 5128       & 3.94       & 0.42       &$ 5147  ^{+ 68    }_{ -48   }$&$ 3.89  ^{+ 0.04  }_{ -0.06 }$&$ 0.06  ^{+ 0.23  }_{ -0.31 }$&$ 1.07  ^{+ 0.06  }_{ -0.10 }$&$ 1.86  ^{+ 0.11  }_{ -0.21 }$&$ 2.17  ^{+ 0.29  }_{ -0.52 }$&$ 0.23  \pm{ 0.06 }$ \\
K01241.01  & 6448890    & 293.758362      & 41.871868       & 12.44 & 4931       & 3.58       & 0.16       &$ 4906  ^{+ 34    }_{ -85   }$&$ 2.75  ^{+ 0.09  }_{ -0.60 }$&$ -0.43 ^{+ 0.17  }_{ -0.22 }$&$ 1.20  ^{+ 0.09  }_{ -0.13 }$&$ 7.13  ^{+ 1.15  }_{ -1.48 }$&$ 26.12 ^{+ 6.80  }_{ -11.17 }$&$ 0.00  \pm{ 0.00 }$ \\
K01241.02  & 6448890    & 293.758362      & 41.871868       & 12.44 & 4931       & 3.58       & 0.16       &$ 4916  ^{+ 46    }_{ -46   }$&$ 2.79  ^{+ 0.30  }_{ -0.35 }$&$ -0.47 ^{+ 0.24  }_{ -0.78 }$&$ 1.16  ^{+ 0.10  }_{ -0.14 }$&$ 6.10  ^{+ 1.81  }_{ -2.82 }$&$ 3.55  ^{+ 12.81 }_{ -0.00 }$&$ 0.01  \pm{ 0.01 }$ \\
K01316.01  & 10794087   & 290.552368      & 48.126263       & 11.93 & 5721       & 4.00       & \nodata    &$ 5724  ^{+ 48    }_{ -47   }$&$ 3.78  ^{+ 0.05  }_{ -0.07 }$&$ -0.45 ^{+ 0.30  }_{ -1.15 }$&$ 1.29  ^{+ 0.44  }_{ -0.12 }$&$ 2.26  ^{+ 0.14  }_{ -0.63 }$&$ 4.76  ^{+ 0.67  }_{ -2.24 }$&$ 0.16  \pm{ 0.09 }$ \\
K01316.02  & 10794087   & 290.552368      & 48.126263       & 11.93 & 5721       & 4.00       & \nodata    &$ 5695  ^{+ 46    }_{ -138  }$&$ 3.74  ^{+ 0.08  }_{ -0.27 }$&$ -0.30 ^{+ 0.33  }_{ -0.46 }$&$ 1.11  ^{+ 0.13  }_{ -0.35 }$&$ 2.35  ^{+ 0.27  }_{ -1.20 }$&$ 5.38  ^{+ 1.33  }_{ -3.96 }$&$ 0.12  \pm{ 0.12 }$ \\
K01445.01  & 11336883   & 283.936798      & 49.110329       & 12.32 & 6182       & 4.35       & 0.06       &$ 6144  ^{+ 45    }_{ -144  }$&$ 4.32  ^{+ 0.05  }_{ -0.06 }$&$ 0.15  ^{+ 0.21  }_{ -0.28 }$&$ 1.29  ^{+ 0.12  }_{ -0.08 }$&$ 1.23  ^{+ 0.09  }_{ -0.28 }$&$ 1.88  ^{+ 0.32  }_{ -0.78 }$&$ 0.97  \pm{ 0.45 }$ \\
K01445.02  & 11336883   & 283.936798      & 49.110329       & 12.32 & 6182       & 4.35       & 0.06       &$ 6151  ^{+ 41    }_{ -116  }$&$ 4.40  ^{+ 0.06  }_{ -0.05 }$&$ -0.19 ^{+ 0.22  }_{ -0.71 }$&$ 1.14  ^{+ 0.10  }_{ -0.12 }$&$ 1.05  ^{+ 0.09  }_{ -0.19 }$&$ 1.48  ^{+ 0.27  }_{ -0.56 }$&$ 1.39  \pm{ 0.58 }$ \\
K01445.03  & 11336883   & 283.936798      & 49.110329       & 12.32 & 6182       & 4.35       & 0.06       &$ 6178  ^{+ 46    }_{ -49   }$&$ 4.36  ^{+ 0.03  }_{ -0.09 }$&$ 0.14  ^{+ 0.39  }_{ -0.26 }$&$ 1.12  ^{+ 0.10  }_{ -0.27 }$&$ 1.18  ^{+ 0.10  }_{ -0.10 }$&$ 1.78  ^{+ 0.29  }_{ -0.30 }$&$ 0.96  \pm{ 0.28 }$ \\
K01525.01  & 7869917    & 281.971252      & 43.672771       & 12.08 & 6905       & 4.24       & 0.01       &$ 6840  ^{+ 63    }_{ -214  }$&$ 3.62  ^{+ 0.04  }_{ -0.04 }$&$ 0.28  ^{+ 0.32  }_{ -0.38 }$&$ 2.03  ^{+ 0.27  }_{ -0.11 }$&$ 3.60  ^{+ 0.18  }_{ -0.23 }$&$ 25.56 ^{+ 2.78  }_{ -5.54 }$&$ 0.06  \pm{ 0.01 }$ \\
K01525.02  & 7869917    & 281.971252      & 43.672771       & 12.08 & 6905       & 4.24       & 0.01       &$ 6925  ^{+ 82    }_{ -84   }$&$ 3.48  ^{+ 0.10  }_{ -0.14 }$&$ -0.07 ^{+ 0.47  }_{ -0.47 }$&$ 2.08  ^{+ 0.39  }_{ -0.27 }$&$ 3.93  ^{+ 0.57  }_{ -1.28 }$&$ 32.55 ^{+ 11.45 }_{ -12.53 }$&$ 0.05  \pm{ 0.03 }$ \\
K01534.01  & 4741126    & 290.090820      & 39.816990       & 13.47 & 6401       & 4.40       & -0.06      &$ 6431  ^{+ 70    }_{ -114  }$&$ 3.50  ^{+ 0.03  }_{ -0.00 }$&$ -0.27 ^{+ 0.37  }_{ -0.64 }$&$ 1.92  ^{+ 0.21  }_{ -0.15 }$&$ 3.89  ^{+ 0.29  }_{ -0.34 }$&$ 23.64 ^{+ 4.21  }_{ -4.11 }$&$ 0.05  \pm{ 0.01 }$ \\
K01534.02  & 4741126    & 290.090820      & 39.816990       & 13.47 & 6401       & 4.40       & -0.06      &$ 6387  ^{+ 67    }_{ -265  }$&$ 3.53  ^{+ 0.04  }_{ -0.03 }$&$ -0.03 ^{+ 0.22  }_{ -1.08 }$&$ 1.90  ^{+ 0.09  }_{ -0.16 }$&$ 3.88  ^{+ 0.19  }_{ -0.47 }$&$ 21.06 ^{+ 3.11  }_{ -5.18 }$&$ 0.05  \pm{ 0.01 }$ \\
K01613.01  & 6268648    & 285.476593      & 41.632717       & 11.05 & 5945       & 4.41       & \nodata    &$ 5790  ^{+ 484   }_{ -359  }$&$ 3.66  ^{+ 0.14  }_{ -0.19 }$&$ -0.20 ^{+ 0.40  }_{ -0.52 }$&$ 1.24  ^{+ 0.26  }_{ -0.42 }$&$ 2.72  ^{+ 0.68  }_{ -0.95 }$&$ 6.26  ^{+ 4.29  }_{ -5.12 }$&$ 0.09  \pm{ 0.08 }$ \\
K01613.02  & 6268648    & 285.476593      & 41.632717       & 11.05 & 5945       & 4.41       & \nodata    &$ 5587  ^{+ 378   }_{ -469  }$&$ 3.71  ^{+ 0.64  }_{ -0.21 }$&$ -0.19 ^{+ 0.37  }_{ -0.44 }$&$ 1.23  ^{+ 0.29  }_{ -0.32 }$&$ 2.42  ^{+ 0.82  }_{ -1.51 }$&$ 3.81  ^{+ 3.81  }_{ -3.51 }$&$ 0.12  \pm{ 0.18 }$ \\
K01628.01  & 6975129    & 298.395752      & 42.459751       & 12.95 & 6197       & 4.38       & 0.08       &$ 6190  ^{+ 40    }_{ -70   }$&$ 4.34  ^{+ 0.03  }_{ -0.20 }$&$ 0.08  ^{+ 0.20  }_{ -0.90 }$&$ 1.29  ^{+ 0.16  }_{ -0.06 }$&$ 1.23  ^{+ 0.08  }_{ -0.08 }$&$ 1.95  ^{+ 0.22  }_{ -0.29 }$&$ 0.97  \pm{ 0.20 }$ \\
K01628.02  & 6975129    & 298.395752      & 42.459751       & 12.95 & 6197       & 4.38       & 0.08       &$ 6191  ^{+ 44    }_{ -49   }$&$ 4.35  ^{+ 0.04  }_{ -0.06 }$&$ -0.32 ^{+ 0.27  }_{ -0.40 }$&$ 1.04  ^{+ 0.12  }_{ -0.14 }$&$ 1.07  ^{+ 0.09  }_{ -0.22 }$&$ 1.58  ^{+ 0.31  }_{ -0.48 }$&$ 1.21  \pm{ 0.56 }$ \\
K01692.01  & 6616218    & 294.674103      & 42.075581       & 12.56 & 5501       & 4.49       & 0.16       &$ 5502  ^{+ 49    }_{ -46   }$&$ 4.47  ^{+ 0.02  }_{ -0.09 }$&$ 0.35  ^{+ 0.22  }_{ -0.19 }$&$ 1.00  ^{+ 0.03  }_{ -0.06 }$&$ 0.96  ^{+ 0.04  }_{ -0.04 }$&$ 0.75  ^{+ 0.08  }_{ -0.07 }$&$ 1.58  \pm{ 0.20 }$ \\
K01692.02  & 6616218    & 294.674103      & 42.075581       & 12.56 & 5501       & 4.49       & 0.16       &$ 5479  ^{+ 40    }_{ -138  }$&$ 4.47  ^{+ 0.02  }_{ -0.10 }$&$ 0.29  ^{+ 0.20  }_{ -0.23 }$&$ 1.02  ^{+ 0.03  }_{ -0.03 }$&$ 0.96  ^{+ 0.03  }_{ -0.06 }$&$ 0.75  ^{+ 0.06  }_{ -0.08 }$&$ 1.63  \pm{ 0.23 }$ \\
K01779.01  & 9909735    & 298.482819      & 46.793621       & 13.30 & 5812       & 4.14       & 0.14       &$ 5731  ^{+ 76    }_{ -245  }$&$ 3.82  ^{+ 0.04  }_{ -0.23 }$&$ -0.73 ^{+ 0.25  }_{ -0.60 }$&$ 1.00  ^{+ 0.08  }_{ -0.12 }$&$ 1.91  ^{+ 0.13  }_{ -0.22 }$&$ 3.77  ^{+ 0.55  }_{ -0.73 }$&$ 0.20  \pm{ 0.06 }$ \\
K01779.02  & 9909735    & 298.482819      & 46.793621       & 13.30 & 5812       & 4.14       & 0.14       &$ 5725  ^{+ 87    }_{ -288  }$&$ 3.94  ^{+ 0.06  }_{ -0.11 }$&$ -0.59 ^{+ 0.25  }_{ -0.85 }$&$ 0.94  ^{+ 0.08  }_{ -0.15 }$&$ 1.58  ^{+ 0.13  }_{ -0.49 }$&$ 2.52  ^{+ 0.45  }_{ -1.32 }$&$ 0.33  \pm{ 0.20 }$ \\
K01781.01  & 11551692   & 287.605591      & 49.523258       & 12.23 & 4977       & 4.59       & 0.22       &$ 4957  ^{+ 37    }_{ -120  }$&$ 4.57  ^{+ 0.01  }_{ -0.02 }$&$ 0.36  ^{+ 0.19  }_{ -0.18 }$&$ 0.86  ^{+ 0.02  }_{ -0.04 }$&$ 0.80  ^{+ 0.02  }_{ -0.02 }$&$ 0.34  ^{+ 0.02  }_{ -0.04 }$&$ 2.35  \pm{ 0.20 }$ \\
K01781.02  & 11551692   & 287.605591      & 49.523258       & 12.23 & 4977       & 4.59       & 0.22       &$ 4997  ^{+ 45    }_{ -44   }$&$ 4.54  ^{+ 0.01  }_{ -0.05 }$&$ 0.41  ^{+ 0.18  }_{ -0.15 }$&$ 0.86  ^{+ 0.02  }_{ -0.04 }$&$ 0.81  ^{+ 0.01  }_{ -0.06 }$&$ 0.37  ^{+ 0.03  }_{ -0.02 }$&$ 2.26  \pm{ 0.32 }$ \\
K01781.03  & 11551692   & 287.605591      & 49.523258       & 12.23 & 4977       & 4.59       & 0.22       &$ 4990  ^{+ 45    }_{ -49   }$&$ 4.54  ^{+ 0.03  }_{ -0.10 }$&$ 0.13  ^{+ 0.19  }_{ -0.81 }$&$ 0.85  ^{+ 0.03  }_{ -0.03 }$&$ 0.81  ^{+ 0.03  }_{ -0.04 }$&$ 0.35  ^{+ 0.03  }_{ -0.05 }$&$ 2.26  \pm{ 0.27 }$ \\
           &            & 0.000000        & 0.000000        & 0.00  & \nodata    & \nodata    & -0.24      &$ 4990  ^{+ 45    }_{ -49   }$&$ 4.54  ^{+ 0.03  }_{ -0.10 }$&$ 0.13  ^{+ 0.19  }_{ -0.81 }$&$ 0.85  ^{+ 0.03  }_{ -0.03 }$&$ 0.81  ^{+ 0.03  }_{ -0.04 }$&$ 0.35  ^{+ 0.03  }_{ -0.05 }$&$ 2.26  \pm{ 0.27 }$ \\
K01806.02  & 9529744    & 293.213562      & 46.175129       & 13.47 & 6440       & 4.41       & -0.24      &$ 6409  ^{+ 81    }_{ -106  }$&$ 4.34  ^{+ 0.16  }_{ -0.46 }$&$ -0.54 ^{+ 0.38  }_{ -0.48 }$&$ 1.01  ^{+ 0.19  }_{ -0.20 }$&$ 1.05  ^{+ 0.26  }_{ -0.16 }$&$ 1.07  ^{+ 1.26  }_{ -0.00 }$&$ 1.22  \pm{ 0.77 }$ \\
K01806.03  & 9529744    & 293.213562      & 46.175129       & 13.47 & 6440       & 4.41       & \nodata    &$ 6406  ^{+ 78    }_{ -128  }$&$ 3.56  ^{+ 0.15  }_{ -0.05 }$&$ -0.56 ^{+ 0.30  }_{ -0.76 }$&$ 1.01  ^{+ 0.21  }_{ -0.19 }$&$ 1.06  ^{+ 0.56  }_{ -0.16 }$&$ 1.15  ^{+ 1.54  }_{ -0.00 }$&$ 1.18  \pm{ 1.22 }$ \\
K01809.01  & 8240797    & 294.453857      & 44.145973       & 12.71 & 5692       & 4.47       & \nodata    &$ 5363  ^{+ 293   }_{ -674  }$&$ 3.74  ^{+ 0.10  }_{ -0.16 }$&$ 0.03  ^{+ 0.51  }_{ -0.34 }$&$ 1.17  ^{+ 0.19  }_{ -0.36 }$&$ 2.35  ^{+ 0.44  }_{ -0.60 }$&$ 3.39  ^{+ 2.19  }_{ -1.95 }$&$ 0.13  \pm{ 0.09 }$ \\
K01809.02  & 8240797    & 294.453857      & 44.145973       & 12.71 & 5692       & 4.47       & -0.08      &$ 5588  ^{+ 421   }_{ -460  }$&$ 3.71  ^{+ 0.13  }_{ -0.17 }$&$ -0.23 ^{+ 0.39  }_{ -0.55 }$&$ 1.26  ^{+ 0.26  }_{ -0.39 }$&$ 2.28  ^{+ 0.50  }_{ -0.95 }$&$ 4.62  ^{+ 3.16  }_{ -3.10 }$&$ 0.15  \pm{ 0.15 }$ \\
K01824.01  & 2989404    & 291.382233      & 38.127468       & 12.72 & 6255       & 4.21       & -0.08      &$ 6285  ^{+ 163   }_{ -76   }$&$ 3.76  ^{+ 0.17  }_{ -0.04 }$&$ -0.61 ^{+ 0.39  }_{ -0.33 }$&$ 1.19  ^{+ 0.10  }_{ -0.16 }$&$ 2.34  ^{+ 0.15  }_{ -0.49 }$&$ 8.33  ^{+ 1.07  }_{ -1.40 }$&$ 0.13  \pm{ 0.06 }$ \\
K01824.02  & 2989404    & 291.382233      & 38.127468       & 12.72 & 6255       & 4.21       & -0.07      &$ 6186  ^{+ 68    }_{ -169  }$&$ 3.71  ^{+ 0.06  }_{ -0.07 }$&$ -0.78 ^{+ 0.36  }_{ -0.72 }$&$ 1.20  ^{+ 0.11  }_{ -0.18 }$&$ 2.55  ^{+ 0.20  }_{ -0.34 }$&$ 8.27  ^{+ 1.24  }_{ -4.72 }$&$ 0.10  \pm{ 0.03 }$ \\
K01909.01  & 10130039   & 287.140656      & 47.115189       & 12.78 & 6095       & 4.46       & -0.07      &$ 6075  ^{+ 58    }_{ -86   }$&$ 3.60  ^{+ 0.03  }_{ -0.04 }$&$ -0.22 ^{+ 0.39  }_{ -0.52 }$&$ 1.64  ^{+ 0.14  }_{ -0.14 }$&$ 3.22  ^{+ 0.40  }_{ -0.31 }$&$ 12.12 ^{+ 1.64  }_{ -2.39 }$&$ 0.07  \pm{ 0.02 }$ \\
K01909.02  & 10130039   & 287.140656      & 47.115189       & 12.78 & 6095       & 4.46       & -0.07      &$ 6092  ^{+ 76    }_{ -70   }$&$ 3.58  ^{+ 0.06  }_{ -0.02 }$&$ -0.30 ^{+ 0.26  }_{ -0.81 }$&$ 1.53  ^{+ 0.13  }_{ -0.24 }$&$ 3.11  ^{+ 0.30  }_{ -0.39 }$&$ 13.50 ^{+ 3.21  }_{ -2.75 }$&$ 0.07  \pm{ 0.03 }$ \\
K01909.03  & 10130039   & 287.140656      & 47.115189       & 12.78 & 6095       & 4.46       & -0.13      &$ 6130  ^{+ 125   }_{ -68   }$&$ 3.66  ^{+ 0.12  }_{ -0.10 }$&$ -0.26 ^{+ 0.35  }_{ -0.95 }$&$ 1.27  ^{+ 0.26  }_{ -0.35 }$&$ 1.07  ^{+ 1.48  }_{ -0.15 }$&$ 1.00  ^{+ 6.37  }_{ -0.00 }$&$ 1.48  \pm{ 3.40 }$ \\
K01929.01  & 10136549   & 290.060486      & 47.163960       & 12.73 & 5900       & 4.12       & -0.13      &$ 5871  ^{+ 74    }_{ -61   }$&$ 3.73  ^{+ 0.04  }_{ -0.15 }$&$ -0.82 ^{+ 0.29  }_{ -0.40 }$&$ 0.95  ^{+ 0.09  }_{ -0.11 }$&$ 2.10  ^{+ 0.17  }_{ -0.17 }$&$ 4.89  ^{+ 0.80  }_{ -1.11 }$&$ 0.15  \pm{ 0.04 }$ \\
K01929.02  & 10136549   & 290.060486      & 47.163960       & 12.73 & 5900       & 4.12       & -0.11      &$ 5827  ^{+ 58    }_{ -189  }$&$ 3.87  ^{+ 0.09  }_{ -0.09 }$&$ -0.41 ^{+ 0.84  }_{ -0.35 }$&$ 0.97  ^{+ 0.06  }_{ -0.13 }$&$ 1.95  ^{+ 0.18  }_{ -0.48 }$&$ 3.72  ^{+ 0.76  }_{ -1.52 }$&$ 0.18  \pm{ 0.09 }$ \\
K01930.01  & 5511081    & 282.978973      & 40.784351       & 12.12 & 5897       & 4.12       & -0.11      &$ 5861  ^{+ 51    }_{ -174  }$&$ 3.82  ^{+ 0.06  }_{ -0.00 }$&$ -0.31 ^{+ 0.27  }_{ -0.22 }$&$ 1.06  ^{+ 0.07  }_{ -0.17 }$&$ 2.00  ^{+ 0.16  }_{ -0.17 }$&$ 4.33  ^{+ 1.03  }_{ -0.66 }$&$ 0.19  \pm{ 0.05 }$ \\
K01930.02  & 5511081    & 282.978973      & 40.784351       & 12.12 & 5897       & 4.12       & -0.11      &$ 5907  ^{+ 71    }_{ -50   }$&$ 3.89  ^{+ 0.06  }_{ -0.05 }$&$ -0.34 ^{+ 0.23  }_{ -0.30 }$&$ 1.08  ^{+ 0.08  }_{ -0.11 }$&$ 1.96  ^{+ 0.15  }_{ -0.13 }$&$ 3.73  ^{+ 0.48  }_{ -1.53 }$&$ 0.20  \pm{ 0.05 }$ \\
K01930.03  & 5511081    & 282.978973      & 40.784351       & 12.12 & 5897       & 4.12       & -0.11      &$ 5896  ^{+ 57    }_{ -52   }$&$ 3.86  ^{+ 0.05  }_{ -0.04 }$&$ -0.34 ^{+ 0.16  }_{ -0.35 }$&$ 1.10  ^{+ 0.08  }_{ -0.08 }$&$ 1.98  ^{+ 0.15  }_{ -0.14 }$&$ 4.12  ^{+ 0.53  }_{ -0.65 }$&$ 0.20  \pm{ 0.05 }$ \\
K01930.04  & 5511081    & 282.978973      & 40.784351       & 12.12 & 5897       & 4.12       & -0.09      &$ 5899  ^{+ 66    }_{ -54   }$&$ 3.85  ^{+ 0.04  }_{ -0.03 }$&$ -0.44 ^{+ 0.20  }_{ -0.55 }$&$ 1.08  ^{+ 0.07  }_{ -0.09 }$&$ 1.97  ^{+ 0.11  }_{ -0.16 }$&$ 4.30  ^{+ 0.46  }_{ -0.59 }$&$ 0.20  \pm{ 0.04 }$ \\
K01932.01  & 5202905    & 295.933472      & 40.300571       & 12.35 & 8229       & 3.86       & -0.09      &$ 8119  ^{+ 165   }_{ -529  }$&$ 3.56  ^{+ 0.04  }_{ -0.10 }$&$ -0.31 ^{+ 0.49  }_{ -0.54 }$&$ 2.50  ^{+ 0.69  }_{ -0.26 }$&$ 4.11  ^{+ 0.28  }_{ -0.39 }$&$ 63.09 ^{+ 10.65 }_{ -41.95 }$&$ 0.05  \pm{ 0.02 }$ \\
K01932.02  & 5202905    & 295.933472      & 40.300571       & 12.35 & 8229       & 3.86       & -0.05      &$ 8132  ^{+ 153   }_{ -398  }$&$ 3.46  ^{+ 0.20  }_{ -0.22 }$&$ -0.54 ^{+ 0.34  }_{ -1.03 }$&$ 2.27  ^{+ 0.42  }_{ -1.07 }$&$ 3.93  ^{+ 1.40  }_{ -2.53 }$&$ 49.55 ^{+ 44.82 }_{ -42.86 }$&$ 0.05  \pm{ 0.08 }$ \\
K01955.01  & 9892816    & 292.678070      & 46.726711       & 13.15 & 6464       & 4.41       & -0.05      &$ 6452  ^{+ 57    }_{ -101  }$&$ 3.67  ^{+ 0.14  }_{ -0.09 }$&$ 0.44  ^{+ 0.15  }_{ -0.25 }$&$ 1.98  ^{+ 0.23  }_{ -0.14 }$&$ 3.23  ^{+ 0.18  }_{ -0.70 }$&$ 15.53 ^{+ 2.64  }_{ -5.16 }$&$ 0.08  \pm{ 0.03 }$ \\
K01955.02  & 9892816    & 292.678070      & 46.726711       & 13.15 & 6464       & 4.41       & -0.05      &$ 6474  ^{+ 53    }_{ -91   }$&$ 3.65  ^{+ 0.04  }_{ -0.11 }$&$ 0.51  ^{+ 0.09  }_{ -0.34 }$&$ 1.87  ^{+ 0.09  }_{ -0.16 }$&$ 3.90  ^{+ 0.16  }_{ -0.52 }$&$ 17.41 ^{+ 3.07  }_{ -8.07 }$&$ 0.04  \pm{ 0.01 }$ \\
K01955.03  & 9892816    & 292.678070      & 46.726711       & 13.15 & 6464       & 4.41       & -0.05      &$ 6428  ^{+ 59    }_{ -239  }$&$ 3.58  ^{+ 0.07  }_{ -0.06 }$&$ -0.51 ^{+ 0.40  }_{ -0.81 }$&$ 1.43  ^{+ 0.16  }_{ -0.39 }$&$ 3.27  ^{+ 0.27  }_{ -0.29 }$&$ 15.27 ^{+ 2.79  }_{ -8.83 }$&$ 0.06  \pm{ 0.02 }$ \\
K01955.04  & 9892816    & 292.678070      & 46.726711       & 13.15 & 6464       & 4.41       & -0.03      &$ 6472  ^{+ 86    }_{ -79   }$&$ 3.66  ^{+ 0.09  }_{ -0.14 }$&$ -0.50 ^{+ 0.42  }_{ -0.79 }$&$ 1.31  ^{+ 0.30  }_{ -0.31 }$&$ 3.06  ^{+ 0.96  }_{ -0.64 }$&$ 1.38  ^{+ 5.89  }_{ -0.00 }$&$ 0.06  \pm{ 0.05 }$ \\
K02004.01  & 12154526   & 288.646271      & 50.788979       & 13.35 & 5760       & 4.47       & -0.03      &$ 5700  ^{+ 66    }_{ -200  }$&$ 3.81  ^{+ 0.09  }_{ -0.07 }$&$ -0.47 ^{+ 0.33  }_{ -0.96 }$&$ 1.05  ^{+ 0.13  }_{ -0.22 }$&$ 2.22  ^{+ 0.22  }_{ -0.38 }$&$ 4.71  ^{+ 0.95  }_{ -2.39 }$&$ 0.14  \pm{ 0.06 }$ \\
K02004.02  & 12154526   & 288.646271      & 50.788979       & 13.35 & 5760       & 4.47       & -0.03      &$ 5748  ^{+ 61    }_{ -172  }$&$ 3.71  ^{+ 0.03  }_{ -0.13 }$&$ -0.01 ^{+ 0.53  }_{ -0.47 }$&$ 1.45  ^{+ 0.21  }_{ -0.19 }$&$ 2.45  ^{+ 0.20  }_{ -0.72 }$&$ 6.31  ^{+ 1.24  }_{ -1.13 }$&$ 0.14  \pm{ 0.08 }$ \\
K02004.03  & 12154526   & 288.646271      & 50.788979       & 13.35 & 5760       & 4.47       & -0.03      &$ 5733  ^{+ 90    }_{ -79   }$&$ 4.02  ^{+ 0.04  }_{ -0.18 }$&$ 0.14  ^{+ 0.33  }_{ -0.39 }$&$ 1.15  ^{+ 0.13  }_{ -0.11 }$&$ 1.65  ^{+ 0.14  }_{ -0.15 }$&$ 2.53  ^{+ 0.39  }_{ -0.63 }$&$ 0.36  \pm{ 0.10 }$ \\
K02011.01  & 5384079    & 297.255035      & 40.548370       & 12.56 & 6361       & 4.43       & -0.04      &$ 6444  ^{+ 167   }_{ -95   }$&$ 3.54  ^{+ 0.04  }_{ -0.00 }$&$ 0.19  ^{+ 0.31  }_{ -0.33 }$&$ 1.81  ^{+ 0.09  }_{ -0.17 }$&$ 3.23  ^{+ 0.27  }_{ -0.44 }$&$ 15.00 ^{+ 2.37  }_{ -3.77 }$&$ 0.08  \pm{ 0.03 }$ \\
K02011.02  & 5384079    & 297.255035      & 40.548370       & 12.56 & 6361       & 4.43       & -0.04      &$ 6287  ^{+ 88    }_{ -280  }$&$ 4.29  ^{+ 0.13  }_{ -0.53 }$&$ -0.37 ^{+ 0.39  }_{ -0.50 }$&$ 1.05  ^{+ 0.21  }_{ -0.24 }$&$ 1.05  ^{+ 0.23  }_{ -0.16 }$&$ 1.04  ^{+ 1.22  }_{ -0.00 }$&$ 1.27  \pm{ 0.76 }$ \\
K02029.01  & 9489524    & 299.896515      & 46.051971       & 12.96 & 5227       & 4.63       & -0.17      &$ 5214  ^{+ 44    }_{ -186  }$&$ 3.73  ^{+ 0.03  }_{ -0.00 }$&$ 0.11  ^{+ 0.22  }_{ -0.27 }$&$ 1.32  ^{+ 0.09  }_{ -0.12 }$&$ 2.43  ^{+ 0.16  }_{ -0.17 }$&$ 3.92  ^{+ 0.67  }_{ -0.53 }$&$ 0.13  \pm{ 0.03 }$ \\
K02029.02  & 9489524    & 299.896515      & 46.051971       & 12.96 & 5227       & 4.63       & -0.17      &$ 5221  ^{+ 59    }_{ -60   }$&$ 3.81  ^{+ 0.04  }_{ -0.05 }$&$ 0.00  ^{+ 0.18  }_{ -0.43 }$&$ 1.29  ^{+ 0.13  }_{ -0.09 }$&$ 2.32  ^{+ 0.19  }_{ -0.14 }$&$ 3.43  ^{+ 0.42  }_{ -1.14 }$&$ 0.15  \pm{ 0.03 }$ \\
K02029.03  & 9489524    & 299.896515      & 46.051971       & 12.96 & 5227       & 4.63       & -0.17      &$ 5176  ^{+ 59    }_{ -138  }$&$ 4.54  ^{+ 0.12  }_{ -0.08 }$&$ -0.03 ^{+ 0.28  }_{ -0.70 }$&$ 0.91  ^{+ 0.13  }_{ -0.10 }$&$ 0.86  ^{+ 0.11  }_{ -0.20 }$&$ 0.42  ^{+ 0.12  }_{ -0.15 }$&$ 2.04  \pm{ 1.15 }$ \\
K02029.04  & 9489524    & 299.896515      & 46.051971       & 12.96 & 5227       & 4.63       & -0.17      &$ 5221  ^{+ 48    }_{ -86   }$&$ 4.51  ^{+ 0.07  }_{ -0.08 }$&$ 0.13  ^{+ 0.24  }_{ -0.26 }$&$ 0.90  ^{+ 0.07  }_{ -0.08 }$&$ 0.84  ^{+ 0.08  }_{ -0.16 }$&$ 0.45  ^{+ 0.09  }_{ -0.16 }$&$ 2.12  \pm{ 0.91 }$ \\
K02053.01  & 2307415    & 292.421082      & 37.682819       & 12.99 & 6310       & 4.34       & -0.33      &$ 6305  ^{+ 77    }_{ -74   }$&$ 3.65  ^{+ 0.08  }_{ -0.10 }$&$ -0.27 ^{+ 0.74  }_{ -0.46 }$&$ 1.49  ^{+ 0.19  }_{ -0.19 }$&$ 2.91  ^{+ 0.26  }_{ -0.69 }$&$ 12.06 ^{+ 2.25  }_{ -5.66 }$&$ 0.09  \pm{ 0.04 }$ \\
K02053.02  & 2307415    & 292.421082      & 37.682819       & 12.99 & 6310       & 4.34       & -0.33      &$ 6263  ^{+ 69    }_{ -193  }$&$ 3.47  ^{+ 0.05  }_{ -0.03 }$&$ -0.51 ^{+ 0.47  }_{ -0.50 }$&$ 1.40  ^{+ 0.18  }_{ -0.23 }$&$ 3.56  ^{+ 0.51  }_{ -0.56 }$&$ 11.23 ^{+ 4.34  }_{ -4.91 }$&$ 0.04  \pm{ 0.02 }$ \\
K02059.01  & 12301181   & 287.590088      & 51.060570       & 12.91 & 4790       & 4.63       & -1.13      &$ 4812  ^{+ 69    }_{ -58   }$&$ 4.73  ^{+ 0.02  }_{ -0.03 }$&$ -0.96 ^{+ 0.25  }_{ -0.64 }$&$ 0.57  ^{+ 0.03  }_{ -0.05 }$&$ 0.54  ^{+ 0.03  }_{ -0.07 }$&$ 0.14  ^{+ 0.02  }_{ -0.02 }$&$ 5.20  \pm{ 1.36 }$ \\
K02059.02  & 12301181   & 287.590088      & 51.060570       & 12.91 & 4790       & 4.63       & -1.13      &$ 0     ^{+ 0     }_{ 0     }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  ^{+ 0.00  }_{ 0.00  }$&$ 0.00  \pm{ 0.00 }$ \\
K02148.01  & 6021193    & 283.192078      & 41.305389       & 13.35 & 5604       & 3.90       & 0.30       &$ 5571  ^{+ 109   }_{ -109  }$&$ 4.37  ^{+ 0.03  }_{ -0.21 }$&$ 0.07  ^{+ 0.21  }_{ -0.25 }$&$ 0.95  ^{+ 0.05  }_{ -0.15 }$&$ 1.04  ^{+ 0.06  }_{ -0.05 }$&$ 0.85  ^{+ 0.12  }_{ -0.23 }$&$ 1.20  \pm{ 0.24 }$ \\
K02148.02  & 6021193    & 283.192078      & 41.305389       & 13.35 & 5604       & 3.90       & 0.30       &$ 5582  ^{+ 115   }_{ -123  }$&$ 3.89  ^{+ 0.09  }_{ -0.09 }$&$ -0.04 ^{+ 0.32  }_{ -0.34 }$&$ 1.15  ^{+ 0.15  }_{ -0.13 }$&$ 1.89  ^{+ 0.17  }_{ -0.53 }$&$ 3.35  ^{+ 0.81  }_{ -1.16 }$&$ 0.24  \pm{ 0.14 }$ \\
K02148.03  & 6021193    & 283.192078      & 41.305389       & 13.35 & 5604       & 3.90       & 0.30       &$ 5615  ^{+ 148   }_{ -114  }$&$ 3.82  ^{+ 0.06  }_{ -0.09 }$&$ -0.33 ^{+ 0.35  }_{ -0.84 }$&$ 1.16  ^{+ 0.13  }_{ -0.18 }$&$ 2.13  ^{+ 0.21  }_{ -0.31 }$&$ 3.46  ^{+ 0.91  }_{ -1.59 }$&$ 0.17  \pm{ 0.06 }$ \\
K02158.01  & 5211199    & 297.651428      & 40.352551       & 13.05 & 5404       & 4.02       & -0.09      &$ 5414  ^{+ 73    }_{ -65   }$&$ 3.78  ^{+ 0.08  }_{ -0.31 }$&$ -0.73 ^{+ 0.25  }_{ -0.67 }$&$ 0.85  ^{+ 0.04  }_{ -0.07 }$&$ 1.80  ^{+ 0.17  }_{ -0.17 }$&$ 2.72  ^{+ 0.75  }_{ -0.48 }$&$ 0.21  \pm{ 0.06 }$ \\
K02158.02  & 5211199    & 297.651428      & 40.352551       & 13.05 & 5404       & 4.02       & -0.09      &$ 5419  ^{+ 65    }_{ -68   }$&$ 3.65  ^{+ 0.09  }_{ -0.22 }$&$ -0.43 ^{+ 0.33  }_{ -0.66 }$&$ 1.31  ^{+ 0.28  }_{ -0.22 }$&$ 2.71  ^{+ 0.53  }_{ -0.42 }$&$ 4.73  ^{+ 1.48  }_{ -2.87 }$&$ 0.09  \pm{ 0.05 }$ \\
K02169.01  & 9006186    & 285.207489      & 45.384350       & 12.40 & 5447       & 4.42       & 0.03       &$ 5403  ^{+ 58    }_{ -156  }$&$ 3.93  ^{+ 0.44  }_{ -0.08 }$&$ -0.53 ^{+ 0.26  }_{ -1.01 }$&$ 0.87  ^{+ 0.08  }_{ -0.08 }$&$ 1.75  ^{+ 0.16  }_{ -0.74 }$&$ 2.42  ^{+ 0.48  }_{ -1.66 }$&$ 0.23  \pm{ 0.18 }$ \\
K02169.02  & 9006186    & 285.207489      & 45.384350       & 12.40 & 5447       & 4.42       & 0.03       &$ 5433  ^{+ 63    }_{ -83   }$&$ 3.86  ^{+ 0.06  }_{ -0.32 }$&$ -0.50 ^{+ 0.28  }_{ -0.92 }$&$ 0.86  ^{+ 0.08  }_{ -0.07 }$&$ 1.84  ^{+ 0.18  }_{ -0.15 }$&$ 2.41  ^{+ 0.36  }_{ -1.57 }$&$ 0.20  \pm{ 0.05 }$ \\
K02169.03  & 9006186    & 285.207489      & 45.384350       & 12.40 & 5447       & 4.42       & 0.03       &$ 5401  ^{+ 54    }_{ -199  }$&$ 3.96  ^{+ 0.47  }_{ -0.13 }$&$ -0.31 ^{+ 0.31  }_{ -0.46 }$&$ 0.90  ^{+ 0.07  }_{ -0.11 }$&$ 1.55  ^{+ 0.27  }_{ -0.64 }$&$ 2.17  ^{+ 0.88  }_{ -1.57 }$&$ 0.34  \pm{ 0.30 }$ \\
K02169.04  & 9006186    & 285.207489      & 45.384350       & 12.40 & 5447       & 4.42       & 0.03       &$ 5466  ^{+ 213   }_{ -67   }$&$ 3.88  ^{+ 0.11  }_{ -0.34 }$&$ -0.18 ^{+ 0.37  }_{ -0.33 }$&$ 0.85  ^{+ 0.07  }_{ -0.17 }$&$ 1.84  ^{+ 0.34  }_{ -0.72 }$&$ 2.04  ^{+ 0.73  }_{ -1.67 }$&$ 0.19  \pm{ 0.17 }$ \\
K02173.01  & 11774991   & 297.292419      & 49.981628       & 12.88 & 4739       & 4.64       & 0.25       &$ 4784  ^{+ 61    }_{ -52   }$&$ 4.53  ^{+ 0.02  }_{ -0.06 }$&$ 0.49  ^{+ 0.11  }_{ -0.13 }$&$ 0.79  ^{+ 0.02  }_{ -0.02 }$&$ 0.77  ^{+ 0.02  }_{ -0.12 }$&$ 0.28  ^{+ 0.02  }_{ -0.03 }$&$ 2.40  \pm{ 0.68 }$ \\
K02173.02  & 11774991   & 297.292419      & 49.981628       & 12.88 & 4739       & 4.64       & 0.25       &$ 4787  ^{+ 59    }_{ -66   }$&$ 4.50  ^{+ 0.05  }_{ -0.74 }$&$ 0.49  ^{+ 0.11  }_{ -0.16 }$&$ 0.78  ^{+ 0.03  }_{ -0.16 }$&$ 0.77  ^{+ 0.06  }_{ -0.18 }$&$ 0.27  ^{+ 0.06  }_{ -0.13 }$&$ 2.42  \pm{ 1.15 }$ \\
K02175.01  & 9022166    & 291.880035      & 45.387932       & 12.85 & 5293       & 4.58       & -0.49      &$ 5320  ^{+ 182   }_{ -187  }$&$ 3.79  ^{+ 0.06  }_{ -0.05 }$&$ -0.12 ^{+ 0.42  }_{ -0.36 }$&$ 1.00  ^{+ 0.15  }_{ -0.18 }$&$ 2.12  ^{+ 0.16  }_{ -0.47 }$&$ 2.75  ^{+ 0.73  }_{ -1.12 }$&$ 0.15  \pm{ 0.07 }$ \\
K02175.02  & 9022166    & 291.880035      & 45.387932       & 12.85 & 5293       & 4.58       & -0.49      &$ 5311  ^{+ 159   }_{ -216  }$&$ 4.49  ^{+ 0.13  }_{ -0.67 }$&$ -0.37 ^{+ 0.32  }_{ -0.86 }$&$ 0.88  ^{+ 0.13  }_{ -0.21 }$&$ 0.79  ^{+ 0.22  }_{ -0.11 }$&$ 0.26  ^{+ 0.34  }_{ -0.00 }$&$ 2.48  \pm{ 1.64 }$ \\
K02289.01  & 3867615    & 295.701111      & 38.945831       & 13.36 & 6255       & 4.38       & -0.04      &$ 6257  ^{+ 90    }_{ -85   }$&$ 3.70  ^{+ 0.62  }_{ -0.17 }$&$ -0.19 ^{+ 0.32  }_{ -0.51 }$&$ 1.56  ^{+ 0.30  }_{ -0.30 }$&$ 1.04  ^{+ 1.54  }_{ -0.18 }$&$ 0.84  ^{+ 4.69  }_{ -0.00 }$&$ 1.96  \pm{ 4.90 }$ \\
K02289.02  & 3867615    & 295.701111      & 38.945831       & 13.36 & 6255       & 4.38       & -0.04      &$ 6194  ^{+ 75    }_{ -229  }$&$ 4.32  ^{+ 0.16  }_{ -0.56 }$&$ -0.20 ^{+ 0.46  }_{ -0.40 }$&$ 1.22  ^{+ 0.29  }_{ -0.43 }$&$ 1.07  ^{+ 0.73  }_{ -0.17 }$&$ 1.05  ^{+ 1.66  }_{ -0.00 }$&$ 1.40  \pm{ 1.82 }$ \\
K02311.01  & 4247991    & 287.241180      & 39.332760       & 12.57 & 5765       & 4.48       & -0.29      &$ 5746  ^{+ 37    }_{ -103  }$&$ 3.16  ^{+ 0.22  }_{ -0.18 }$&$ -0.55 ^{+ 0.37  }_{ -0.78 }$&$ 1.85  ^{+ 0.40  }_{ -0.31 }$&$ 3.53  ^{+ 0.75  }_{ -0.61 }$&$ 11.85 ^{+ 5.93  }_{ -3.60 }$&$ 0.06  \pm{ 0.04 }$ \\
K02311.02  & 4247991    & 287.241180      & 39.332760       & 12.57 & 5765       & 4.48       & -0.29      &$ 5758  ^{+ 44    }_{ -60   }$&$ 3.11  ^{+ 0.11  }_{ -0.13 }$&$ -0.65 ^{+ 0.39  }_{ -0.90 }$&$ 1.76  ^{+ 0.27  }_{ -0.34 }$&$ 5.77  ^{+ 0.89  }_{ -1.94 }$&$ 13.51 ^{+ 17.16 }_{ -7.71 }$&$ 0.01  \pm{ 0.01 }$ \\
K02352.01  & 8013439    & 285.182800      & 43.831078       & 10.42 & 6638       & 4.32       & \nodata    &$ 6057  ^{+ 450   }_{ -1292 }$&$ 3.60  ^{+ 0.19  }_{ -0.19 }$&$ 0.03  ^{+ 0.56  }_{ -0.45 }$&$ 1.90  ^{+ 0.66  }_{ -0.40 }$&$ 3.03  ^{+ 0.78  }_{ -1.75 }$&$ 7.19  ^{+ 10.64 }_{ -5.42 }$&$ 0.10  \pm{ 0.12 }$ \\
K02352.02  & 8013439    & 285.182800      & 43.831078       & 10.42 & 6638       & 4.32       & \nodata    &$ 6334  ^{+ 415   }_{ -647  }$&$ 3.50  ^{+ 0.30  }_{ -0.24 }$&$ -0.50 ^{+ 0.42  }_{ -0.99 }$&$ 1.93  ^{+ 0.54  }_{ -0.40 }$&$ 3.48  ^{+ 1.23  }_{ -2.14 }$&$ 10.03 ^{+ 16.49 }_{ -8.50 }$&$ 0.06  \pm{ 0.10 }$ \\
K02352.03  & 8013439    & 285.182800      & 43.831078       & 10.42 & 6638       & 4.32       & \nodata    &$ 6469  ^{+ 426   }_{ -514  }$&$ 3.25  ^{+ 0.17  }_{ -0.43 }$&$ -0.09 ^{+ 0.45  }_{ -0.44 }$&$ 1.87  ^{+ 0.32  }_{ -0.59 }$&$ 4.89  ^{+ 1.31  }_{ -1.61 }$&$ 18.14 ^{+ 18.42 }_{ -16.22 }$&$ 0.02  \pm{ 0.02 }$ \\
K02541.01  & 12306058   & 290.621826      & 51.057301       & 13.01 & 5214       & 3.74       & 0.02       &$ 5236  ^{+ 102   }_{ -76   }$&$ 3.75  ^{+ 0.09  }_{ -0.08 }$&$ -0.17 ^{+ 0.27  }_{ -0.38 }$&$ 1.19  ^{+ 0.11  }_{ -0.12 }$&$ 2.46  ^{+ 0.23  }_{ -0.28 }$&$ 3.68  ^{+ 0.71  }_{ -1.39 }$&$ 0.11  \pm{ 0.04 }$ \\
K02541.02  & 12306058   & 290.621826      & 51.057301       & 13.01 & 5214       & 3.74       & 0.02       &$ 5204  ^{+ 72    }_{ -83   }$&$ 3.69  ^{+ 0.15  }_{ -0.15 }$&$ -0.25 ^{+ 0.36  }_{ -0.46 }$&$ 1.10  ^{+ 0.22  }_{ -0.27 }$&$ 2.53  ^{+ 0.51  }_{ -0.86 }$&$ 4.01  ^{+ 1.56  }_{ -2.30 }$&$ 0.10  \pm{ 0.08 }$ \\
K02585.01  & 7673841    & 288.660767      & 43.368080       & 13.46 & 6482       & 4.20       & -0.30      &$ 6509  ^{+ 148   }_{ -97   }$&$ 3.57  ^{+ 0.07  }_{ -0.23 }$&$ -0.67 ^{+ 0.41  }_{ -0.49 }$&$ 1.38  ^{+ 0.16  }_{ -0.20 }$&$ 2.87  ^{+ 0.25  }_{ -0.72 }$&$ 13.74 ^{+ 3.31  }_{ -3.76 }$&$ 0.08  \pm{ 0.04 }$ \\
K02585.02  & 7673841    & 288.660767      & 43.368080       & 13.46 & 6482       & 4.20       & -0.30      &$ 6472  ^{+ 92    }_{ -101  }$&$ 4.27  ^{+ 0.17  }_{ -0.56 }$&$ -0.55 ^{+ 0.35  }_{ -0.44 }$&$ 1.03  ^{+ 0.22  }_{ -0.24 }$&$ 1.10  ^{+ 0.26  }_{ -0.25 }$&$ 1.03  ^{+ 1.54  }_{ -0.00 }$&$ 1.10  \pm{ 0.81 }$ \\
K02585.03  & 7673841    & 288.660767      & 43.368080       & 13.46 & 6482       & 4.20       & -0.30      &$ 6492  ^{+ 116   }_{ -91   }$&$ 4.29  ^{+ 0.26  }_{ -0.59 }$&$ -0.45 ^{+ 0.38  }_{ -0.40 }$&$ 0.99  ^{+ 0.23  }_{ -0.18 }$&$ 1.10  ^{+ 0.95  }_{ -0.26 }$&$ 1.03  ^{+ 1.95  }_{ -0.00 }$&$ 1.06  \pm{ 1.77 }$ \\
K02595.01  & 8883329    & 290.995270      & 45.192211       & 13.22 & 6742       & 4.11       & -0.22      &$ 6706  ^{+ 90    }_{ -157  }$&$ 3.56  ^{+ 0.16  }_{ -0.08 }$&$ -0.44 ^{+ 1.03  }_{ -0.35 }$&$ 1.58  ^{+ 0.14  }_{ -0.28 }$&$ 4.04  ^{+ 0.51  }_{ -0.56 }$&$ 21.62 ^{+ 6.38  }_{ -8.56 }$&$ 0.03  \pm{ 0.01 }$ \\
K02595.02  & 8883329    & 290.995270      & 45.192211       & 13.22 & 6742       & 4.11       & -0.22      &$ 6724  ^{+ 99    }_{ -115  }$&$ 3.60  ^{+ 0.06  }_{ -0.10 }$&$ -0.64 ^{+ 0.34  }_{ -0.58 }$&$ 1.49  ^{+ 0.16  }_{ -0.24 }$&$ 3.16  ^{+ 0.28  }_{ -0.36 }$&$ 18.37 ^{+ 3.44  }_{ -4.20 }$&$ 0.07  \pm{ 0.02 }$ \\
K02672.01  & 11253827   & 296.132812      & 48.977402       & 11.92 & 5565       & 4.33       & -0.13      &$ 5553  ^{+ 56    }_{ -71   }$&$ 4.37  ^{+ 0.11  }_{ -0.45 }$&$ -0.36 ^{+ 0.22  }_{ -0.48 }$&$ 0.87  ^{+ 0.08  }_{ -0.07 }$&$ 0.93  ^{+ 0.22  }_{ -0.24 }$&$ 0.73  ^{+ 0.37  }_{ -0.35 }$&$ 1.54  \pm{ 1.16 }$ \\
K02672.02  & 11253827   & 296.132812      & 48.977402       & 11.92 & 5565       & 4.33       & -0.13      &$ 5555  ^{+ 59    }_{ -64   }$&$ 4.38  ^{+ 0.15  }_{ -0.44 }$&$ -0.30 ^{+ 0.32  }_{ -0.35 }$&$ 0.85  ^{+ 0.08  }_{ -0.12 }$&$ 0.91  ^{+ 0.31  }_{ -0.21 }$&$ 0.70  ^{+ 0.54  }_{ -0.30 }$&$ 1.58  \pm{ 1.36 }$ \\
K02674.01  & 8022489    & 289.651245      & 43.824421       & 13.35 & 5973       & 4.26       & -0.12      &$ 5885  ^{+ 68    }_{ -171  }$&$ 3.87  ^{+ 0.08  }_{ -0.09 }$&$ -0.57 ^{+ 0.28  }_{ -0.60 }$&$ 0.99  ^{+ 0.10  }_{ -0.14 }$&$ 1.86  ^{+ 0.18  }_{ -0.50 }$&$ 3.74  ^{+ 0.75  }_{ -1.78 }$&$ 0.22  \pm{ 0.12 }$ \\
K02674.02  & 8022489    & 289.651245      & 43.824421       & 13.35 & 5973       & 4.26       & -0.12      &$ 5975  ^{+ 90    }_{ -86   }$&$ 4.36  ^{+ 0.09  }_{ -0.50 }$&$ -0.44 ^{+ 0.28  }_{ -0.37 }$&$ 0.93  ^{+ 0.09  }_{ -0.17 }$&$ 0.95  ^{+ 0.15  }_{ -0.17 }$&$ 0.93  ^{+ 0.36  }_{ -0.30 }$&$ 1.51  \pm{ 0.79 }$ \\
K02674.03  & 8022489    & 289.651245      & 43.824421       & 13.35 & 5973       & 4.26       & -0.12      &$ 5977  ^{+ 102   }_{ -87   }$&$ 3.83  ^{+ 0.08  }_{ -0.11 }$&$ -0.77 ^{+ 0.33  }_{ -0.75 }$&$ 1.07  ^{+ 0.12  }_{ -0.11 }$&$ 2.09  ^{+ 0.26  }_{ -0.22 }$&$ 4.42  ^{+ 0.97  }_{ -2.33 }$&$ 0.17  \pm{ 0.06 }$ \\
K02675.01  & 5794570    & 292.971252      & 41.035770       & 12.43 & 5706       & 4.56       & -0.35      &$ 5711  ^{+ 57    }_{ -57   }$&$ 3.74  ^{+ 0.05  }_{ -0.05 }$&$ -0.50 ^{+ 0.29  }_{ -0.63 }$&$ 1.16  ^{+ 0.16  }_{ -0.30 }$&$ 2.44  ^{+ 0.18  }_{ -0.24 }$&$ 6.31  ^{+ 2.42  }_{ -0.98 }$&$ 0.11  \pm{ 0.04 }$ \\
K02675.02  & 5794570    & 292.971252      & 41.035770       & 12.43 & 5706       & 4.56       & -0.35      &$ 5674  ^{+ 50    }_{ -101  }$&$ 3.74  ^{+ 0.02  }_{ -0.05 }$&$ -0.29 ^{+ 0.22  }_{ -0.48 }$&$ 1.29  ^{+ 0.10  }_{ -0.25 }$&$ 2.51  ^{+ 0.07  }_{ -0.20 }$&$ 5.40  ^{+ 0.53  }_{ -1.66 }$&$ 0.12  \pm{ 0.02 }$ \\
K02687.01  & 7202957    & 292.615112      & 42.764252       & 10.16 & 5803       & 3.91       & 0.15       &$ 5765  ^{+ 76    }_{ -87   }$&$ 3.80  ^{+ 0.06  }_{ -0.06 }$&$ -0.52 ^{+ 0.32  }_{ -0.81 }$&$ 1.03  ^{+ 0.14  }_{ -0.15 }$&$ 2.24  ^{+ 0.19  }_{ -0.26 }$&$ 4.78  ^{+ 0.77  }_{ -2.05 }$&$ 0.13  \pm{ 0.04 }$ \\
K02687.02  & 7202957    & 292.615112      & 42.764252       & 10.16 & 5803       & 3.91       & 0.15       &$ 5781  ^{+ 72    }_{ -81   }$&$ 3.82  ^{+ 0.10  }_{ -0.09 }$&$ -0.30 ^{+ 0.38  }_{ -0.41 }$&$ 1.13  ^{+ 0.12  }_{ -0.21 }$&$ 2.15  ^{+ 0.25  }_{ -0.38 }$&$ 4.50  ^{+ 1.16  }_{ -2.62 }$&$ 0.16  \pm{ 0.07 }$ \\
K02693.01  & 5185897    & 291.468658      & 40.343849       & 13.26 & 4476       & 4.73       & -0.05      &$ 4463  ^{+ 37    }_{ -138  }$&$ 4.67  ^{+ 0.01  }_{ -0.02 }$&$ 0.27  ^{+ 0.23  }_{ -0.21 }$&$ 0.72  ^{+ 0.03  }_{ -0.02 }$&$ 0.65  ^{+ 0.02  }_{ -0.02 }$&$ 0.14  ^{+ 0.01  }_{ -0.02 }$&$ 3.73  \pm{ 0.41 }$ \\
K02693.02  & 5185897    & 291.468658      & 40.343849       & 13.26 & 4476       & 4.73       & -0.05      &$ 4458  ^{+ 50    }_{ -76   }$&$ 4.68  ^{+ 0.04  }_{ -0.08 }$&$ 0.04  ^{+ 0.43  }_{ -0.58 }$&$ 0.72  ^{+ 0.06  }_{ -0.07 }$&$ 0.64  ^{+ 0.09  }_{ -0.07 }$&$ 0.15  ^{+ 0.08  }_{ -0.03 }$&$ 3.94  \pm{ 1.49 }$ \\
K02693.03  & 5185897    & 291.468658      & 40.343849       & 13.26 & 4476       & 4.73       & -0.05      &$ 4458  ^{+ 45    }_{ -164  }$&$ 4.67  ^{+ 0.03  }_{ -0.04 }$&$ 0.29  ^{+ 0.31  }_{ -0.42 }$&$ 0.72  ^{+ 0.06  }_{ -0.07 }$&$ 0.63  ^{+ 0.03  }_{ -0.10 }$&$ 0.14  ^{+ 0.02  }_{ -0.04 }$&$ 4.02  \pm{ 1.30 }$ \\
K02696.01  & 11071200   & 284.415924      & 48.658020       & 13.00 & 7036       & 4.15       & -0.14      &$ 6999  ^{+ 79    }_{ -248  }$&$ 3.63  ^{+ 0.07  }_{ -0.06 }$&$ -0.58 ^{+ 0.34  }_{ -0.85 }$&$ 1.67  ^{+ 0.16  }_{ -0.30 }$&$ 3.47  ^{+ 0.18  }_{ -0.28 }$&$ 26.16 ^{+ 3.21  }_{ -3.87 }$&$ 0.06  \pm{ 0.01 }$ \\
K02696.02  & 11071200   & 284.415924      & 48.658020       & 13.00 & 7036       & 4.15       & -0.14      &$ 7026  ^{+ 89    }_{ -115  }$&$ 3.58  ^{+ 0.06  }_{ -0.07 }$&$ -0.39 ^{+ 0.40  }_{ -0.41 }$&$ 1.63  ^{+ 0.14  }_{ -0.25 }$&$ 3.49  ^{+ 0.25  }_{ -0.39 }$&$ 25.68 ^{+ 3.81  }_{ -7.63 }$&$ 0.05  \pm{ 0.02 }$ \\
K02714.01  & 12206313   & 290.082764      & 50.863480       & 13.31 & 6362       & 4.19       & -0.30      &$ 6355  ^{+ 75    }_{ -98   }$&$ 3.75  ^{+ 0.06  }_{ -0.06 }$&$ -0.67 ^{+ 0.38  }_{ -0.34 }$&$ 1.22  ^{+ 0.10  }_{ -0.13 }$&$ 2.43  ^{+ 0.15  }_{ -0.67 }$&$ 8.36  ^{+ 1.05  }_{ -3.92 }$&$ 0.12  \pm{ 0.06 }$ \\
K02714.02  & 12206313   & 290.082764      & 50.863480       & 13.31 & 6362       & 4.19       & -0.30      &$ 6320  ^{+ 77    }_{ -128  }$&$ 3.67  ^{+ 0.05  }_{ -0.30 }$&$ -1.01 ^{+ 0.33  }_{ -0.50 }$&$ 1.20  ^{+ 0.10  }_{ -0.14 }$&$ 2.46  ^{+ 0.22  }_{ -0.95 }$&$ 8.89  ^{+ 1.93  }_{ -5.77 }$&$ 0.11  \pm{ 0.08 }$ \\
K02722.01  & 7673192    & 288.370239      & 43.354610       & 13.27 & 6534       & 4.34       & -0.22      &$ 6519  ^{+ 68    }_{ -103  }$&$ 3.47  ^{+ 0.03  }_{ -0.03 }$&$ -0.18 ^{+ 0.38  }_{ -0.40 }$&$ 1.94  ^{+ 0.23  }_{ -0.20 }$&$ 4.07  ^{+ 0.21  }_{ -0.42 }$&$ 26.80 ^{+ 3.71  }_{ -5.22 }$&$ 0.04  \pm{ 0.01 }$ \\
K02722.02  & 7673192    & 288.370239      & 43.354610       & 13.27 & 6534       & 4.34       & -0.22      &$ 6556  ^{+ 111   }_{ -88   }$&$ 3.50  ^{+ 0.03  }_{ -0.06 }$&$ -0.43 ^{+ 0.34  }_{ -1.13 }$&$ 1.80  ^{+ 0.18  }_{ -0.25 }$&$ 4.04  ^{+ 0.50  }_{ -0.36 }$&$ 25.87 ^{+ 3.97  }_{ -5.39 }$&$ 0.04  \pm{ 0.01 }$ \\
K02722.03  & 7673192    & 288.370239      & 43.354610       & 13.27 & 6534       & 4.34       & -0.22      &$ 6576  ^{+ 168   }_{ -71   }$&$ 3.46  ^{+ 0.02  }_{ -0.02 }$&$ -0.27 ^{+ 0.27  }_{ -0.42 }$&$ 1.78  ^{+ 0.15  }_{ -0.42 }$&$ 4.20  ^{+ 0.27  }_{ -0.22 }$&$ 29.83 ^{+ 7.56  }_{ -3.89 }$&$ 0.03  \pm{ 0.01 }$ \\
K02722.04  & 7673192    & 288.370239      & 43.354610       & 13.27 & 6534       & 4.34       & -0.22      &$ 6559  ^{+ 92    }_{ -77   }$&$ 3.44  ^{+ 0.05  }_{ -0.00 }$&$ -0.47 ^{+ 0.38  }_{ -0.96 }$&$ 1.78  ^{+ 0.18  }_{ -0.29 }$&$ 4.24  ^{+ 0.24  }_{ -0.44 }$&$ 23.65 ^{+ 5.28  }_{ -6.36 }$&$ 0.03  \pm{ 0.01 }$ \\
K02722.05  & 7673192    & 288.370239      & 43.354610       & 13.27 & 6534       & 4.34       & -0.22      &$ 6489  ^{+ 72    }_{ -160  }$&$ 3.71  ^{+ 0.55  }_{ -0.20 }$&$ -0.54 ^{+ 0.39  }_{ -0.47 }$&$ 1.03  ^{+ 0.26  }_{ -0.21 }$&$ 0.96  ^{+ 0.52  }_{ -0.00 }$&$ 1.34  ^{+ 2.27  }_{ -0.00 }$&$ 1.62  \pm{ 1.36 }$ \\
K02732.01  & 9886361    & 289.921448      & 46.744560       & 12.80 & 6303       & 4.44       & -0.14      &$ 6343  ^{+ 74    }_{ -62   }$&$ 2.97  ^{+ 0.02  }_{ -0.02 }$&$ 0.10  ^{+ 0.25  }_{ -0.50 }$&$ 2.88  ^{+ 0.10  }_{ -0.26 }$&$ 9.18  ^{+ 0.53  }_{ -0.48 }$&$ 106.58 ^{+ 9.67  }_{ -37.81 }$&$ 0.01  \pm{ 0.00 }$ \\
K02732.02  & 9886361    & 289.921448      & 46.744560       & 12.80 & 6303       & 4.44       & -0.14      &$ 6287  ^{+ 51    }_{ -111  }$&$ 3.32  ^{+ 0.16  }_{ -0.24 }$&$ -0.63 ^{+ 0.39  }_{ -0.88 }$&$ 2.11  ^{+ 0.49  }_{ -0.34 }$&$ 4.69  ^{+ 1.49  }_{ -2.16 }$&$ 30.91 ^{+ 22.14 }_{ -23.08 }$&$ 0.03  \pm{ 0.03 }$ \\
K02732.03  & 9886361    & 289.921448      & 46.744560       & 12.80 & 6303       & 4.44       & -0.14      &$ 6275  ^{+ 63    }_{ -89   }$&$ 3.31  ^{+ 0.27  }_{ -0.16 }$&$ -0.31 ^{+ 0.38  }_{ -0.55 }$&$ 2.10  ^{+ 0.25  }_{ -0.39 }$&$ 4.69  ^{+ 0.78  }_{ -1.29 }$&$ 34.09 ^{+ 15.44 }_{ -18.02 }$&$ 0.03  \pm{ 0.02 }$ \\
K02732.04  & 9886361    & 289.921448      & 46.744560       & 12.80 & 6303       & 4.44       & -0.14      &$ 6264  ^{+ 58    }_{ -225  }$&$ 3.38  ^{+ 0.25  }_{ -0.41 }$&$ -0.33 ^{+ 0.45  }_{ -0.42 }$&$ 0.99  ^{+ 0.39  }_{ -0.23 }$&$ 0.83  ^{+ 1.75  }_{ -0.00 }$&$ 0.92  ^{+ 8.50  }_{ -0.00 }$&$ 2.48  \pm{ 7.93 }$ \\
K02949.01  & 6026737    & 285.875793      & 41.332432       & 13.31 & 6176       & 4.00       & -0.07      &$ 6194  ^{+ 141   }_{ -78   }$&$ 4.34  ^{+ 0.19  }_{ -0.51 }$&$ -0.31 ^{+ 0.69  }_{ -0.28 }$&$ 1.06  ^{+ 0.13  }_{ -0.14 }$&$ 1.03  ^{+ 0.70  }_{ -0.20 }$&$ 0.81  ^{+ 0.99  }_{ -0.00 }$&$ 1.36  \pm{ 1.78 }$ \\
K02949.02  & 6026737    & 285.875793      & 41.332432       & 13.31 & 6176       & 4.00       & -0.07      &$ 6124  ^{+ 71    }_{ -247  }$&$ 3.42  ^{+ 0.24  }_{ -0.29 }$&$ -0.19 ^{+ 0.47  }_{ -0.42 }$&$ 1.05  ^{+ 0.34  }_{ -0.27 }$&$ 0.89  ^{+ 1.19  }_{ -0.00 }$&$ 0.92  ^{+ 4.71  }_{ -0.00 }$&$ 2.12  \pm{ 4.30 }$ \\
K03083.01  & 7106173    & 287.978851      & 42.679359       & 12.86 & 5923       & 4.53       & -0.07      &$ 5899  ^{+ 55    }_{ -106  }$&$ 3.71  ^{+ 0.07  }_{ -0.06 }$&$ -0.06 ^{+ 0.29  }_{ -0.39 }$&$ 1.45  ^{+ 0.12  }_{ -0.14 }$&$ 2.62  ^{+ 0.22  }_{ -0.48 }$&$ 7.54  ^{+ 1.44  }_{ -1.91 }$&$ 0.11  \pm{ 0.05 }$ \\
K03083.02  & 7106173    & 287.978851      & 42.679359       & 12.86 & 5923       & 4.53       & -0.07      &$ 5927  ^{+ 73    }_{ -78   }$&$ 4.41  ^{+ 0.08  }_{ -0.56 }$&$ 0.12  ^{+ 0.35  }_{ -0.33 }$&$ 1.08  ^{+ 0.11  }_{ -0.17 }$&$ 0.99  ^{+ 0.14  }_{ -0.24 }$&$ 1.10  ^{+ 0.32  }_{ -0.55 }$&$ 1.59  \pm{ 0.94 }$ \\
K03083.03  & 7106173    & 287.978851      & 42.679359       & 12.86 & 5923       & 4.53       & -0.07      &$ 5907  ^{+ 66    }_{ -102  }$&$ 4.38  ^{+ 0.06  }_{ -0.75 }$&$ -0.21 ^{+ 0.25  }_{ -1.10 }$&$ 1.10  ^{+ 0.11  }_{ -0.11 }$&$ 1.10  ^{+ 1.34  }_{ -0.12 }$&$ 0.96  ^{+ 0.27  }_{ -0.46 }$&$ 1.16  \pm{ 2.30 }$ \\
K03097.01  & 7582689    & 281.112335      & 43.227791       & 11.97 & 6306       & 4.01       & -0.29      &$ 6295  ^{+ 61    }_{ -84   }$&$ 3.57  ^{+ 0.08  }_{ -0.06 }$&$ -1.12 ^{+ 0.35  }_{ -0.46 }$&$ 1.16  ^{+ 0.06  }_{ -0.15 }$&$ 2.93  ^{+ 0.77  }_{ -0.44 }$&$ 12.34 ^{+ 6.25  }_{ -3.41 }$&$ 0.06  \pm{ 0.04 }$ \\
K03097.02  & 7582689    & 281.112335      & 43.227791       & 11.97 & 6306       & 4.01       & -0.29      &$ 6301  ^{+ 67    }_{ -73   }$&$ 3.74  ^{+ 0.06  }_{ -0.11 }$&$ -0.57 ^{+ 1.12  }_{ -0.28 }$&$ 1.14  ^{+ 0.07  }_{ -0.13 }$&$ 2.24  ^{+ 0.17  }_{ -0.71 }$&$ 7.13  ^{+ 1.19  }_{ -3.73 }$&$ 0.14  \pm{ 0.08 }$ \\
K03097.03  & 7582689    & 281.112335      & 43.227791       & 11.97 & 6306       & 4.01       & -0.29      &$ 6259  ^{+ 56    }_{ -83   }$&$ 3.76  ^{+ 0.10  }_{ -0.06 }$&$ -0.69 ^{+ 0.34  }_{ -0.30 }$&$ 1.12  ^{+ 0.07  }_{ -0.14 }$&$ 2.39  ^{+ 0.16  }_{ -0.28 }$&$ 8.33  ^{+ 1.46  }_{ -1.29 }$&$ 0.12  \pm{ 0.03 }$ \\
K03111.01  & 8581240    & 298.576874      & 44.621609       & 12.86 & 6034       & 3.92       & -0.06      &$ 5956  ^{+ 82    }_{ -259  }$&$ 3.67  ^{+ 0.08  }_{ -0.11 }$&$ -0.80 ^{+ 0.34  }_{ -0.80 }$&$ 1.19  ^{+ 0.17  }_{ -0.29 }$&$ 2.57  ^{+ 0.34  }_{ -0.34 }$&$ 7.98  ^{+ 2.46  }_{ -1.84 }$&$ 0.10  \pm{ 0.04 }$ \\
K03111.02  & 8581240    & 298.576874      & 44.621609       & 12.86 & 6034       & 3.92       & -0.06      &$ 5968  ^{+ 87    }_{ -180  }$&$ 3.71  ^{+ 0.08  }_{ -0.39 }$&$ -0.48 ^{+ 0.39  }_{ -0.42 }$&$ 1.17  ^{+ 0.15  }_{ -0.15 }$&$ 2.31  ^{+ 0.28  }_{ -0.37 }$&$ 5.16  ^{+ 1.39  }_{ -3.84 }$&$ 0.13  \pm{ 0.06 }$ \\
K03158.01  & 6278762    & 289.752289      & 41.634605       & 8.72  & 5105       & \nodata    & \nodata    &$ 5081  ^{+ 44    }_{ -71   }$&$ 3.07  ^{+ 0.04  }_{ -0.06 }$&$ -0.54 ^{+ 0.64  }_{ -0.28 }$&$ 1.09  ^{+ 0.35  }_{ -0.24 }$&$ 4.78  ^{+ 0.44  }_{ -0.56 }$&$ 15.40 ^{+ 6.85  }_{ -5.20 }$&$ 0.01  \pm{ 0.01 }$ \\
K03158.02  & 6278762    & 289.752289      & 41.634605       & 8.72  & 5105       & \nodata    & \nodata    &$ 5108  ^{+ 46    }_{ -57   }$&$ 3.01  ^{+ 0.03  }_{ -0.00 }$&$ -0.16 ^{+ 0.16  }_{ -0.52 }$&$ 2.04  ^{+ 0.28  }_{ -0.30 }$&$ 6.97  ^{+ 0.34  }_{ -0.64 }$&$ 30.00 ^{+ 6.86  }_{ -4.34 }$&$ 0.01  \pm{ 0.00 }$ \\
K03158.03  & 6278762    & 289.752289      & 41.634605       & 8.72  & 5105       & \nodata    & \nodata    &$ 5044  ^{+ 49    }_{ -82   }$&$ 3.02  ^{+ 0.07  }_{ -0.02 }$&$ 0.03  ^{+ 0.43  }_{ -0.58 }$&$ 1.95  ^{+ 0.41  }_{ -0.82 }$&$ 5.04  ^{+ 0.89  }_{ -1.45 }$&$ 15.79 ^{+ 8.73  }_{ -8.28 }$&$ 0.02  \pm{ 0.02 }$ \\
K03158.04  & 6278762    & 289.752289      & 41.634605       & 8.72  & 5105       & \nodata    & \nodata    &$ 5063  ^{+ 63    }_{ -165  }$&$ 3.46  ^{+ 0.18  }_{ -0.29 }$&$ -0.36 ^{+ 0.30  }_{ -0.69 }$&$ 1.10  ^{+ 0.26  }_{ -0.26 }$&$ 3.37  ^{+ 0.87  }_{ -0.85 }$&$ 2.93  ^{+ 3.06  }_{ -1.26 }$&$ 0.04  \pm{ 0.03 }$ \\
K03158.05  & 6278762    & 289.752289      & 41.634605       & 8.72  & 5105       & \nodata    & \nodata    &$ 5118  ^{+ 67    }_{ -65   }$&$ 3.75  ^{+ 0.04  }_{ -0.27 }$&$ -0.16 ^{+ 0.36  }_{ -0.38 }$&$ 1.30  ^{+ 0.62  }_{ -0.21 }$&$ 2.17  ^{+ 0.30  }_{ -0.00 }$&$ 2.86  ^{+ 0.88  }_{ -0.00 }$&$ 0.18  \pm{ 0.07 }$ \\
K03196.01  & 9002538    & 283.350464      & 45.339111       & 11.53 & 6408       & \nodata    & -0.07      &$ 6015  ^{+ 376   }_{ -952  }$&$ 3.38  ^{+ 0.13  }_{ -0.37 }$&$ -0.31 ^{+ 0.42  }_{ -0.67 }$&$ 2.00  ^{+ 1.31  }_{ -0.35 }$&$ 4.55  ^{+ 1.97  }_{ -1.01 }$&$ 16.68 ^{+ 12.22 }_{ -12.01 }$&$ 0.03  \pm{ 0.03 }$ \\
K03196.02  & 9002538    & 283.350464      & 45.339111       & 11.53 & 6408       & \nodata    & -0.07      &$ 6092  ^{+ 434   }_{ -641  }$&$ 3.40  ^{+ 0.24  }_{ -0.39 }$&$ -0.41 ^{+ 0.34  }_{ -0.78 }$&$ 1.92  ^{+ 0.84  }_{ -0.40 }$&$ 2.51  ^{+ 1.21  }_{ -1.19 }$&$ 6.64  ^{+ 10.67 }_{ -5.31 }$&$ 0.17  \pm{ 0.25 }$ \\
K03384.01  & 8644365    & 298.095428      & 44.737061       & 13.20 & 5962       & \nodata    & -0.18      &$ 5314  ^{+ 419   }_{ -647  }$&$ 3.17  ^{+ 0.38  }_{ -0.16 }$&$ -0.20 ^{+ 0.44  }_{ -0.47 }$&$ 1.05  ^{+ 0.39  }_{ -0.23 }$&$ 2.73  ^{+ 1.87  }_{ -1.17 }$&$ 1.94  ^{+ 6.76  }_{ -0.00 }$&$ 0.07  \pm{ 0.12 }$ \\
K03384.02  & 8644365    & 298.095428      & 44.737061       & 13.20 & 5962       & \nodata    & -0.18      &$ 5523  ^{+ 438   }_{ -756  }$&$ 3.39  ^{+ 0.13  }_{ -0.39 }$&$ -0.38 ^{+ 0.45  }_{ -0.50 }$&$ 1.26  ^{+ 0.38  }_{ -0.45 }$&$ 3.89  ^{+ 1.22  }_{ -0.92 }$&$ 5.61  ^{+ 6.66  }_{ -3.63 }$&$ 0.03  \pm{ 0.03 }$ \\
K03398.01  & 3561464    & 295.498108      & 38.644501       & 13.49 & 6483       & \nodata    & -0.43      &$ 6192  ^{+ 349   }_{ -994  }$&$ 3.01  ^{+ 0.10  }_{ -0.00 }$&$ -0.35 ^{+ 0.78  }_{ -0.51 }$&$ 2.43  ^{+ 0.39  }_{ -0.57 }$&$ 6.15  ^{+ 1.51  }_{ -2.55 }$&$ 14.57 ^{+ 27.42 }_{ -6.96 }$&$ 0.01  \pm{ 0.01 }$ \\
K03398.02  & 3561464    & 295.498108      & 38.644501       & 13.49 & 6483       & \nodata    & -0.43      &$ 6168  ^{+ 471   }_{ -467  }$&$ 3.69  ^{+ 0.28  }_{ -0.21 }$&$ -0.57 ^{+ 0.48  }_{ -0.41 }$&$ 1.12  ^{+ 0.26  }_{ -0.35 }$&$ 2.54  ^{+ 0.75  }_{ -1.60 }$&$ 6.69  ^{+ 5.82  }_{ -5.93 }$&$ 0.10  \pm{ 0.14 }$ \\
K03398.03  & 3561464    & 295.498108      & 38.644501       & 13.49 & 6483       & \nodata    & -0.43      &$ 6392  ^{+ 661   }_{ -487  }$&$ 3.53  ^{+ 0.14  }_{ -0.39 }$&$ -0.68 ^{+ 0.44  }_{ -0.50 }$&$ 1.17  ^{+ 0.27  }_{ -0.38 }$&$ 2.21  ^{+ 0.71  }_{ -0.94 }$&$ 5.08  ^{+ 5.58  }_{ -3.08 }$&$ 0.15  \pm{ 0.18 }$ \\
K03403.01  & 11754430   & 286.646423      & 49.937778       & 13.10 & 6011       & \nodata    & -0.15      &$ 5379  ^{+ 371   }_{ -708  }$&$ 3.66  ^{+ 0.16  }_{ -0.19 }$&$ -0.55 ^{+ 0.43  }_{ -0.96 }$&$ 1.25  ^{+ 0.31  }_{ -0.30 }$&$ 2.62  ^{+ 0.65  }_{ -0.84 }$&$ 4.36  ^{+ 2.87  }_{ -3.46 }$&$ 0.10  \pm{ 0.09 }$ \\
K03403.02  & 11754430   & 286.646423      & 49.937778       & 13.10 & 6011       & \nodata    & -0.15      &$ 5563  ^{+ 383   }_{ -998  }$&$ 3.64  ^{+ 0.10  }_{ -0.20 }$&$ -0.55 ^{+ 0.40  }_{ -1.03 }$&$ 1.20  ^{+ 0.26  }_{ -0.39 }$&$ 2.49  ^{+ 0.45  }_{ -1.38 }$&$ 6.27  ^{+ 3.62  }_{ -5.14 }$&$ 0.11  \pm{ 0.12 }$ \\
K03425.01  & 9117416    & 300.316193      & 45.495380       & 13.27 & 5133       & \nodata    & \nodata    &$ 5151  ^{+ 282   }_{ -328  }$&$ 3.73  ^{+ 0.26  }_{ -0.15 }$&$ -0.17 ^{+ 0.32  }_{ -0.80 }$&$ 1.21  ^{+ 0.19  }_{ -0.22 }$&$ 2.60  ^{+ 0.58  }_{ -0.57 }$&$ 4.29  ^{+ 1.97  }_{ -2.60 }$&$ 0.10  \pm{ 0.07 }$ \\
K03425.02  & 9117416    & 300.316193      & 45.495380       & 13.27 & 5133       & \nodata    & \nodata    &$ 5389  ^{+ 953   }_{ -314  }$&$ 3.69  ^{+ 0.12  }_{ -0.13 }$&$ 0.13  ^{+ 0.47  }_{ -0.36 }$&$ 1.24  ^{+ 0.20  }_{ -0.20 }$&$ 2.52  ^{+ 0.38  }_{ -0.76 }$&$ 3.24  ^{+ 1.64  }_{ -1.61 }$&$ 0.11  \pm{ 0.08 }$ \\
K03500.01  & 6058816    & 296.354614      & 41.335560       & 13.21 & 6086       & \nodata    & -0.26      &$ 5719  ^{+ 346   }_{ -584  }$&$ 3.66  ^{+ 0.08  }_{ -0.66 }$&$ -0.33 ^{+ 0.45  }_{ -0.42 }$&$ 1.20  ^{+ 0.22  }_{ -0.28 }$&$ 2.43  ^{+ 0.34  }_{ -0.58 }$&$ 3.96  ^{+ 2.43  }_{ -2.49 }$&$ 0.12  \pm{ 0.07 }$ \\
K03500.02  & 6058816    & 296.354614      & 41.335560       & 13.21 & 6086       & \nodata    & -0.26      &$ 5827  ^{+ 372   }_{ -564  }$&$ 4.37  ^{+ 0.26  }_{ -0.74 }$&$ -0.40 ^{+ 0.43  }_{ -0.45 }$&$ 0.94  ^{+ 0.28  }_{ -0.23 }$&$ 0.70  ^{+ 0.95  }_{ -0.00 }$&$ 0.28  ^{+ 2.54  }_{ -0.00 }$&$ 3.87  \pm{ 7.98 }$ \\
K03681.01  & 2581316    & 292.627472      & 37.860142       & 11.69 & 6294       & \nodata    & \nodata    &$ 6158  ^{+ 156   }_{ -363  }$&$ 3.48  ^{+ 0.08  }_{ -0.40 }$&$ -0.26 ^{+ 0.35  }_{ -0.57 }$&$ 1.84  ^{+ 0.27  }_{ -0.29 }$&$ 3.93  ^{+ 1.08  }_{ -0.77 }$&$ 12.97 ^{+ 6.21  }_{ -6.42 }$&$ 0.04  \pm{ 0.03 }$ \\
K03681.02  & 2581316    & 292.627472      & 37.860142       & 11.69 & 6294       & \nodata    & \nodata    &$ 6186  ^{+ 172   }_{ -333  }$&$ 3.45  ^{+ 0.34  }_{ -0.38 }$&$ -0.29 ^{+ 0.39  }_{ -0.58 }$&$ 1.74  ^{+ 0.47  }_{ -0.58 }$&$ 1.04  ^{+ 2.37  }_{ -0.00 }$&$ 1.27  ^{+ 13.95 }_{ -0.00 }$&$ 2.19  \pm{ 7.51 }$ \\
K03864.01  & 4164922    & 293.344971      & 39.257809       & 12.91 & 5013       & \nodata    & -0.26      &$ 5188  ^{+ 271   }_{ -488  }$&$ 3.67  ^{+ 0.04  }_{ -0.13 }$&$ -0.46 ^{+ 0.33  }_{ -0.76 }$&$ 1.14  ^{+ 0.20  }_{ -0.14 }$&$ 2.56  ^{+ 0.19  }_{ -0.19 }$&$ 4.24  ^{+ 1.03  }_{ -1.94 }$&$ 0.10  \pm{ 0.03 }$ \\
K03864.02  & 4164922    & 293.344971      & 39.257809       & 12.91 & 5013       & \nodata    & -0.26      &$ 5227  ^{+ 345   }_{ -302  }$&$ 3.45  ^{+ 0.20  }_{ -0.45 }$&$ -0.32 ^{+ 0.39  }_{ -0.57 }$&$ 1.16  ^{+ 0.34  }_{ -0.28 }$&$ 2.63  ^{+ 0.90  }_{ -2.03 }$&$ 4.91  ^{+ 3.83  }_{ -4.56 }$&$ 0.09  \pm{ 0.15 }$ \\
K04021.01  & 11967788   & 294.034363      & 50.371651       & 13.17 & 6456       & \nodata    & -0.17      &$ 6422  ^{+ 137   }_{ -140  }$&$ 3.14  ^{+ 0.11  }_{ -0.13 }$&$ -0.41 ^{+ 0.37  }_{ -1.11 }$&$ 2.54  ^{+ 0.27  }_{ -0.33 }$&$ 6.94  ^{+ 1.69  }_{ -1.49 }$&$ 74.17 ^{+ 47.56 }_{ -30.80 }$&$ 0.01  \pm{ 0.01 }$ \\
K04021.02  & 11967788   & 294.034363      & 50.371651       & 13.17 & 6456       & \nodata    & -0.17      &$ 6451  ^{+ 152   }_{ -190  }$&$ 3.28  ^{+ 0.23  }_{ -0.28 }$&$ -0.43 ^{+ 0.45  }_{ -0.57 }$&$ 1.93  ^{+ 0.45  }_{ -0.53 }$&$ 3.61  ^{+ 1.69  }_{ -2.45 }$&$ 7.99  ^{+ 19.59 }_{ -6.52 }$&$ 0.06  \pm{ 0.10 }$ \\
K04032.01  & 7100673    & 285.728485      & 42.654530       & 12.64 & 5730       & \nodata    & -0.26      &$ 5280  ^{+ 361   }_{ -516  }$&$ 3.60  ^{+ 0.16  }_{ -0.43 }$&$ -0.55 ^{+ 0.40  }_{ -0.97 }$&$ 1.07  ^{+ 0.29  }_{ -0.27 }$&$ 2.32  ^{+ 0.71  }_{ -1.08 }$&$ 4.85  ^{+ 4.95  }_{ -3.51 }$&$ 0.12  \pm{ 0.14 }$ \\
K04032.02  & 7100673    & 285.728485      & 42.654530       & 12.64 & 5730       & \nodata    & -0.26      &$ 5389  ^{+ 340   }_{ -645  }$&$ 3.69  ^{+ 0.21  }_{ -0.13 }$&$ -0.40 ^{+ 0.43  }_{ -0.43 }$&$ 1.09  ^{+ 0.23  }_{ -0.29 }$&$ 2.45  ^{+ 0.54  }_{ -0.65 }$&$ 5.18  ^{+ 2.81  }_{ -2.80 }$&$ 0.10  \pm{ 0.08 }$ \\
K04097.01  & 5688683    & 285.690002      & 40.994530       & 13.44 & 4350       & \nodata    & -0.18      &$ 4835  ^{+ 186   }_{ -203  }$&$ 3.36  ^{+ 0.12  }_{ -0.25 }$&$ -0.36 ^{+ 0.33  }_{ -0.70 }$&$ 1.03  ^{+ 0.15  }_{ -0.13 }$&$ 3.44  ^{+ 0.66  }_{ -0.70 }$&$ 4.04  ^{+ 1.82  }_{ -2.34 }$&$ 0.04  \pm{ 0.02 }$ \\
K04097.02  & 5688683    & 285.690002      & 40.994530       & 13.44 & 4350       & \nodata    & -0.18      &$ 4860  ^{+ 1085  }_{ -449  }$&$ 4.74  ^{+ 0.13  }_{ -0.10 }$&$ -0.42 ^{+ 0.34  }_{ -1.14 }$&$ 0.57  ^{+ 0.11  }_{ -0.17 }$&$ 0.52  ^{+ 0.09  }_{ -0.13 }$&$ 0.05  ^{+ 0.07  }_{ -0.04 }$&$ 5.80  \pm{ 4.00 }$ \\
K04269.01  & 8890924    & 293.796844      & 45.160728       & 13.26 & 5106       & \nodata    & -0.04      &$ 5088  ^{+ 296   }_{ -553  }$&$ 3.64  ^{+ 0.14  }_{ -0.33 }$&$ -0.12 ^{+ 0.41  }_{ -0.39 }$&$ 1.23  ^{+ 0.28  }_{ -0.22 }$&$ 2.26  ^{+ 0.46  }_{ -1.40 }$&$ 2.77  ^{+ 2.31  }_{ -2.32 }$&$ 0.15  \pm{ 0.19 }$ \\
K04269.02  & 8890924    & 293.796844      & 45.160728       & 13.26 & 5106       & \nodata    & -0.04      &$ 5045  ^{+ 279   }_{ -462  }$&$ 3.55  ^{+ 0.19  }_{ -0.29 }$&$ -0.01 ^{+ 0.42  }_{ -0.42 }$&$ 1.04  ^{+ 0.24  }_{ -0.20 }$&$ 2.67  ^{+ 0.81  }_{ -1.09 }$&$ 3.07  ^{+ 2.97  }_{ -1.58 }$&$ 0.08  \pm{ 0.08 }$ \\
K04288.01  & 4548011    & 287.371246      & 39.603569       & 12.40 & 6207       & \nodata    & -0.08      &$ 5761  ^{+ 401   }_{ -1056 }$&$ 3.65  ^{+ 0.67  }_{ -0.23 }$&$ -0.54 ^{+ 0.35  }_{ -1.02 }$&$ 1.30  ^{+ 0.42  }_{ -0.54 }$&$ 2.43  ^{+ 1.09  }_{ -1.60 }$&$ 4.18  ^{+ 7.47  }_{ -3.74 }$&$ 0.13  \pm{ 0.22 }$ \\
K04288.02  & 4548011    & 287.371246      & 39.603569       & 12.40 & 6207       & \nodata    & -0.08      &$ 5809  ^{+ 373   }_{ -804  }$&$ 3.62  ^{+ 0.26  }_{ -0.33 }$&$ -0.20 ^{+ 0.42  }_{ -0.49 }$&$ 0.97  ^{+ 0.34  }_{ -0.27 }$&$ 2.44  ^{+ 1.13  }_{ -1.75 }$&$ 0.30  ^{+ 5.76  }_{ -0.00 }$&$ 0.09  \pm{ 0.17 }$ \\


\enddata


\tablecomments{Columns marked with a $^{\dagger}$ are values from NASA Exoplanet Archive. Stars marked with a $^{\dagger\dagger}$ have missing $T_{\rm{eff}}$. Their $T_{\rm{eff}}$ values are estimated based on $g-r$ and $g-i$ values~\citep{Pinsonneault2012}, the adopted $T_{\rm{eff}}$ is the average of the results. There are three exceptions, values of $T_{\rm{eff}}$ for K03158 and K0368 are adopted from~\citet{Ammons2006} and $T_{\rm{eff}}$ for K04021 is based on the infrared flux method in ~\citet{Pinsonneault2012}}


\end{deluxetable}

\clearpage
 \end{landscape}


==> table_1.tex <==
00005&8554498&289.739716&44.647419&11.665&5861.00&4.190&2& 54983.516& 56486.440&21&Keck Palomar&J \\
00007&11853905&285.615326&50.135750&12.211&5858.00&4.280&1& 55041.491& 56134.480&22&Keck Palomar&J \\
00010&6922244&281.288116&42.451080&13.563&6025.00&4.110&1& 54983.540& 55781.534&50&Palomar&J \\
00017&10874614&296.837250&48.239944&13.303&5826.00&4.420&1& 54984.561& 55043.520&10&Palomar&J \\
00018&8191672&299.407013&44.035053&13.369&6297.00&3.990&1& 54985.594& 55110.314&9&Gemini Gemini Palomar&R Y J \\
00020&11804465&286.243439&50.040379&13.438&6011.00&4.230&1& 55014.412& 55761.325&16&Palomar&J \\
00022&9631995&282.629669&46.323360&13.435&5972.00&4.410&1& 55014.403& 55792.438&16&Palomar&J \\
00041&6521045&291.385986&41.990269&11.197&5909.00&4.300&3& 54988.511& 56533.359&64&Keck Palomar&J \\
00069&3544595&291.418304&38.672359&9.931&5593.00&4.510&1& 55042.587& 56547.339&61&Keck MMT MMT Palomar&J K J \\
00070&6850504&287.697998&42.338718&12.498&5443.00&4.450&5& 55073.386& 56533.484&38&Palomar&J \\
00072&11904151&285.679382&50.241299&10.961&5627.00&4.390&2& 55073.400& 56172.301&54&MMT MMT Palomar&J K J \\
00082&10187017&281.482727&47.208031&11.492&4908.00&4.610&5& 55311.579& 56533.335&65&Keck MMT MMT&J K \\
00084&2571238&290.420807&37.851799&11.898&5541.00&4.530&1& 55073.419& 55723.450&20&Palomar&J \\
00085&5866724&288.688690&41.151180&11.018&6172.00&4.360&3& 55696.490& 55738.516&6&MMT MMT&J K \\
00087&10593626&289.217499&47.884460&11.664&5510.00&4.500&1& 55425.386& 56521.486&26&Palomar Palomar&J K \\
00103&2444412&291.683350&37.751591&12.593&5531.00&4.440&1& 55073.441& 55797.539&16&Palomar&J \\
00104&10318874&281.194733&47.497131&12.895&4786.00&4.590&1& 55377.342& 56525.316&30&Keck Palomar Palomar&J K \\
00108&4914423&288.984558&40.064529&12.287&5975.00&4.330&2& 55073.469& 56145.498&22&Keck Palomar&J \\
00111&6678383&287.604614&42.166779&12.596&5711.00&4.410&4& 55372.555& 56521.442&14&Palomar&J \\
00116&8395660&300.863983&44.337551&12.882&5865.00&4.410&4& 55133.397& 56532.332&33&Keck MMT&K \\
00122&8349582&284.482452&44.398041&12.346&5714.00&4.390&1& 55073.495& 56151.511&33&Keck Palomar&J \\
00123&5094751&290.392731&40.284870&12.365&5871.00&4.150&2& 55074.492& 56166.345&15&Keck Palomar&J \\
00137&8644288&298.079437&44.746319&13.549&5385.00&4.430&3& 55075.509& 56146.484&20&Palomar&J \\
00148&5735762&299.139221&40.949020&13.040&5190.00&4.490&3& 55073.527& 56532.436&43&Keck Palomar&J \\
00153&12252424&287.997894&50.944328&13.461&4725.00&4.640&2& 55313.592& 56524.353&29&Keck MMT Palomar Palomar&K J K \\
00157&6541920&297.115112&41.909142&13.709&5685.00&4.380&6& 55440.501& 56533.434&7&& \\
00180&9573539&284.394287&46.249081&13.024&5680.00&4.500&1& 55074.466& 55083.341&6&Palomar&J \\
00244&4349452&286.638397&39.487881&10.734&6103.00&4.070&2& 55366.603& 56519.408&104&Keck Palomar Palomar&J K \\
00245&8478994&284.059540&44.518215&9.705&5288.00&4.590&4& 55312.586& 56523.237&59&Gemini Gemini Keck MMT MMT Palomar&R Y J K K \\
00246&11295426&291.032318&49.040272&9.997&5793.00&4.281&2& 55312.582& 56519.420&65&Keck MMT MMT&J K \\
00261&5383248&297.069611&40.525131&10.297&5692.00&4.420&1& 55404.530& 56518.546&36&Keck MMT MMT&J K \\
00263&10514430&281.273804&47.774399&10.821&5820.00&4.150&1& 55395.529& 55788.482&6&MMT MMT Palomar Palomar&J K J K \\
00265&12024120&297.018829&50.408981&11.994&6040.00&4.360&1& 55782.522& 56532.354&27&Gemini Gemini Palomar Palomar&R Y J K \\
00273&3102384&287.478516&38.228840&11.457&5783.00&4.430&1& 55431.309& 56613.223&20&MMT MMT&J K \\
00274&8077137&282.492218&43.980209&11.390&6090.00&4.130&2& 55403.447& 56474.522&8&Gemini Gemini MMT MMT&R Y J K \\
00283&5695396&288.530823&40.942299&11.525&5687.00&4.420&2& 55433.368& 56524.331&30&Keck Palomar Palomar&J K \\
00289&10386922&282.945648&47.574905&12.747&5812.00&4.458&2& 56449.401& 56532.291&5&Lick&J \\
00292&11075737&287.326630&48.673431&12.872&5780.00&4.430&1& 55377.475& 56166.411&21&Keck Palomar Palomar&J K \\
00299&2692377&285.661652&37.964500&12.899&5538.00&4.340&1& 55403.512& 56530.414&32&Keck& \\
00305&6063220&297.354004&41.300049&12.970&4782.00&4.610&1& 55403.543& 56531.340&36&Keck& \\
00321&8753657&291.848053&44.968220&12.520&5538.00&4.340&2& 55378.534& 56493.368&47&Keck Lick&J \\
00364&7296438&295.872314&42.881149&10.087&5798.00&4.240&1& 55376.346& 55699.442&3&& \\
00365&11623629&297.486908&49.623451&11.195&5451.00&4.490&2& 55402.354& 56532.377&24&Palomar Palomar&J K \\
00377&3323887&285.573975&38.400902&13.803&5777.00&4.450&3& 55342.448& 56506.363&16&Palomar Palomar&J K \\
00701&9002278&283.212738&45.349861&13.725&4807.00&4.690&5& 56137.475& 56507.530&15&Keck& \\
00975&3632418&287.361816&38.714016&8.224&6131.00&3.950&1& 55439.438& 56486.562&44&MMT MMT&J K \\
01431&11075279&287.022278&48.681938&13.460&5649.00&4.460&1& 56472.391& 56532.502&6&& \\
01439&11027624&290.851776&48.521339&12.849&5930.00&4.090&1& 55075.273& 56531.312&6&Lick&J \\
01442&11600889&286.036346&49.614510&12.521&5476.00&4.448&1& 55696.518& 56446.424&17&Keck Lick&J \\
01463&7672940&288.258636&43.376465&12.328&6020.00&4.380&1& 56027.511& 56530.292&3&& \\
01612&10963065&284.786194&48.423229&8.769&6027.00&4.220&1& 55697.588& 56494.420&42&Keck Lick&J \\
01781&11551692&287.605591&49.523258&12.231&4977.00&4.590&3& 56076.566& 56112.331&9&& \\
01925&9955598&293.679199&46.852760&9.439&5365.00&4.430&1& 55999.646& 56547.332&40&Keck Palomar&K \\
02169&9006186&285.207489&45.384350&12.404&5447.00&4.420&4& 56099.455& 56171.456&4&& \\
02687&7202957&292.615112&42.764252&10.158&5803.00&3.910&2& 55999.652& 56531.383&22&Palomar&K \\
02720&8176564&295.439667&44.039162&10.338&6109.00&4.410&1& 56018.575& 56519.389&18&Keck Palomar&K \\


==> table_2.tex <==
00005&8554498& 94.9& 4.2&$\surd$& &$\surd$& 23.7&$\surd$ \\
00007&11853905& 7.9& 2.1& & & & 4.5& \\
00010&6922244& 53.8& 13.2& & & & 47.1& \\
00017&10874614& 57.8& 3.6&$\surd$& & & 7.1& \\
00018&8191672& 178.1& 6.1&$\surd$& & & 18.2& \\
00020&11804465& 44.5& 4.1&$\surd$& & & 22.0&$\surd$ \\
00022&9631995& 44.2& 3.8&$\surd$& & & 40.9&$\surd$ \\
00041&6521045& 5.4& 1.6& & & & 5.4& \\
00069&3544595& 21.2& 1.3&$\surd$&$\surd$& & 3.0& \\
00070&6850504& 11.0& 1.9&$\surd$& & & 10.2&$\surd$ \\
00072&11904151& 4.6& 1.6& & & & 3.7& \\
00082&10187017& 4.5& 1.2& & & & 4.2& \\
00084&2571238& 11.2& 1.8&$\surd$& & & 11.2&$\surd$ \\
00085&5866724& 10.1& 1.9&$\surd$& & & 15.5&$\surd$ \\
00087&10593626& 5.0& 1.6& & & & 4.8& \\
00103&2444412& 6.8& 1.9& & & & 6.2& \\
00104&10318874& 96.1& 2.0&$\surd$& &$\surd$& 6.1& \\
00108&4914423& 7.6& 2.2& & & & 7.4& \\
00111&6678383& 6.1& 2.6& & & & 6.6& \\
00116&8395660& 6.5& 2.4& & & & 6.5& \\
00122&8349582& 5.1& 1.7& & & & 4.7& \\
00123&5094751& 7.1& 2.4& & & & 6.9& \\
00137&8644288& 9.7& 2.5& & & & 8.0& \\
00148&5735762& 32.7& 2.3&$\surd$& &$\surd$& 14.2&$\surd$ \\
00153&12252424& 9.7& 2.4& & & & 8.9& \\
00157&6541920& 36.7& 8.1& & & & 49.9&$\surd$ \\
00180&9573539& 15.7& 2.1&$\surd$& & & 15.6&$\surd$ \\
00244&4349452& 8.3& 3.5& & &$\surd$& 6.5& \\
00245&8478994& 5.0& 1.3& & & & 3.3& \\
00246&11295426& 16.9& 1.3&$\surd$& &$\surd$& 3.6& \\
00261&5383248& 5.2& 1.5& & & & 5.3& \\
00263&10514430& 11.1& 3.2& & & & 13.9& \\
00265&12024120& 4.7& 1.8& & & & 4.5& \\
00273&3102384& 91.7& 1.4&$\surd$& & & 10.3&$\surd$ \\
00274&8077137& 4.0& 1.9& & & & 3.7& \\
00283&5695396& 5.7& 1.6& & & & 5.7& \\
00289&10386922& 12.1& 2.1&$\surd$& & & 12.1&$\surd$ \\
00292&11075737& 6.2& 2.3& &$\surd$& & 4.5& \\
00299&2692377& 6.6& 1.9& & & & 6.0& \\
00305&6063220& 5.8& 1.7& & & & 5.6& \\
00321&8753657& 4.3& 1.7& & & & 4.0& \\
00364&7296438& 51.3& 0.3&$\surd$& & & 51.3&$\surd$ \\
00365&11623629& 4.3& 1.3& & & & 4.0& \\
00377&3323887& 13.3& 6.0& & & & 12.3& \\
00701&9002278& 4.7& 3.0& & & & 4.9& \\
00975&3632418& 8.9& 3.0& & & & 8.9& \\
01431&11075279& 8.3& 2.1& & & & 7.1& \\
01439&11027624& 10.2& 2.3& & & & 15.4&$\surd$ \\
01442&11600889& 89.0& 2.0&$\surd$& & & 3.1& \\
01463&7672940& 116.1& 2.8&$\surd$& & & 116.1&$\surd$ \\
01612&10963065& 4.1& 1.5& & & & 4.0& \\
01781&11551692& 21.7& 1.4&$\surd$& & & 24.3&$\surd$ \\
01925&9955598& 3.4& 1.1& & & & 2.5& \\
02169&9006186& 6.6& 0.9&$\surd$& & & 6.6&$\surd$ \\
02687&7202957& 9.2& 1.3&$\surd$& & & 10.2&$\surd$ \\
02720&8176564& 3.8& 1.4& & & & 3.6& \\


==> table_3.tex <==
%from /home/jwang/2014/03/JW_2013_plot/ContrastCurve
K00005 & 2.3 & 40.9 & 290.9 & 28.2 & 51.1 \\
K00005 & 4.6 & 93.7 & 290.9 & 28.0 & 268.6 \\
K00005 & 5.0 & 92.9 & 290.9 & 15.8 & 211.2 \\
K00010 & 6.8 & 3663.9 & 944.5 & 22.0 & 270.7 \\
K00017 & 3.9 & 2130.7 & 517.9 & 206.2 & 320.5 \\
K00018 & 3.9 & 8241.0 & 1135.9 & 323.2 & 211.8 \\
K00018 & 6.6 & 3971.8 & 1135.9 & 28.5 & 249.9 \\
K00018 & 7.3 & 5783.0 & 1135.9 & 14.1 & 148.7 \\
K00070 & 4.3 & 1058.9 & 279.5 & 217.7 & 308.2 \\
K00087 & 6.2 & 956.9 & 174.4 & 78.2 & 182.8 \\
K00087 & 7.4 & 964.1 & 174.4 & 28.4 & 284.8 \\
K00103 & 7.3 & 2985.6 & 304.4 & 9.5 & 81.5 \\
K00108 & 5.5 & 3357.4 & 352.7 & 98.8 & 11.4 \\
K00108 & 7.4 & 3139.4 & 352.7 & 17.1 & 340.8 \\
K00116 & 3.8 & 1453.5 & 363.2 & 164.1 & 275.4 \\
K00116 & 4.8 & 2353.8 & 363.2 & 51.9 & 66.2 \\
K00116 & 6.2 & 1355.1 & 363.2 & 18.1 & 29.0 \\
K00116 & 6.3 & 2453.6 & 363.2 & 13.2 & 35.7 \\
K00116 & 7.3 & 1050.7 & 363.2 & 6.3 & 63.0 \\
K00123 & 5.2 & 4749.5 & 498.7 & 62.3 & 161.2 \\
K00123 & 6.4 & 5083.7 & 498.7 & 19.2 & 264.8 \\
K00137 & 5.9 & 2471.4 & 438.2 & 44.4 & 9.3 \\
K00148 & 3.5 & 1369.1 & 308.7 & 519.8 & 139.4 \\
K00148 & 5.4 & 3391.9 & 308.7 & 77.0 & 129.9 \\
K00148 & 5.5 & 785.2 & 308.7 & 69.7 & 114.2 \\
K00148 & 6.3 & 2486.4 & 308.7 & 35.5 & 116.0 \\
K00153 & 6.0 & 906.0 & 226.2 & 11.2 & 277.4 \\
K00153 & 7.6 & 1395.3 & 226.2 & 4.5 & 61.6 \\
K00244 & 2.0 & 2741.0 & 326.3 & 3231.4 & 72.4 \\
K00263 & 0.6 & 704.5 & 240.7 & 3234.0 & 44.7 \\
K00263 & 1.0 & 788.5 & 240.7 & 2430.8 & 91.8 \\
K00273 & 5.6 & 1201.8 & 239.6 & 32.6 & 128.2 \\
K00365 & 7.7 & 1129.9 & 158.8 & 13.3 & 46.3 \\
K00377 & 4.8 & 3721.9 & 617.9 & 133.8 & 268.1 \\
K00377 & 6.9 & 4969.8 & 617.9 & 18.1 & 138.1 \\
K00377 & 7.3 & 1780.8 & 617.9 & 12.3 & 322.5 \\
K00975 & 4.0 & 90.4 & 123.7 & 31.2 & 49.4 \\
K01442 & 4.7 & 637.4 & 302.3 & 25.3 & 283.7 \\

